A Synthetic Benchmark for Target-Centric Causal Discovery in Industrial Processes

Causal discovery promises to find which recorded variables drive a process target such as product quality, yield or energy use. Process data with known causes are rare, and in existing benchmarks the difficulty of identifying the causes of a target is either fixed by the recorded data or set for the whole graph. We present a synthetic benchmark for target-centric causal discovery in industrial processes. Its generator is a two-level structural causal model inspired by batch production, assembled from components that each model one phenomenon of process data, such as a control loop or a delayed effect. The graph is built around the target: without sensor error, every non-cause can be distinguished from the direct causes by conditioning on them or by time order. Each component is set independently, so the difficulty can be varied one condition at a time. We evaluate eight methods, from association measures to effect estimation, with an error analysis by the role of the selected candidate; all degrade as the difficulties combine, each in a way consistent with its assumptions.

==> generated/numbers.tex <==
\makeatletter
\newcommand{\R}[4]{\ifcsname res@#1@#2@#3@#4\endcsname\csname res@#1@#2@#3@#4\endcsname\else\PackageError{numbers}{missing result #1/#2/#3/#4}{}\fi}
\newcommand{\CS}[2]{\ifcsname cs@#1@#2\endcsname\csname cs@#1@#2\endcsname\else\PackageError{numbers}{missing strength #1/#2}{}\fi}
\expandafter\def\csname res@v4@signal_0.4@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v4@signal_0.4@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v4@signal_0.4@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@correlation@tt\endcsname{0.62}
\expandafter\def\csname res@v4@signal_0.4@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v4@signal_0.4@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@correlation@bw\endcsname{2}
\expandafter\def\csname res@v4@signal_0.4@correlation@len\endcsname{17.7}
\expandafter\def\csname res@v4@signal_0.4@correlation@rp\endcsname{0.57}
\expandafter\def\csname res@v4@signal_0.4@correlation@map\endcsname{0.72}
\expandafter\def\csname res@v4@signal_0.4@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v4@signal_0.4@granger@fpn\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@granger@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v4@signal_0.4@granger@prec\endcsname{0.16}
\expandafter\def\csname res@v4@signal_0.4@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@granger@len\endcsname{15.8}
\expandafter\def\csname res@v4@signal_0.4@granger@rp\endcsname{0.68}
\expandafter\def\csname res@v4@signal_0.4@granger@map\endcsname{0.79}
\expandafter\def\csname res@v4@signal_0.4@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v4@signal_0.4@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v4@signal_0.4@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@pcmciplus@tt\endcsname{0.77}
\expandafter\def\csname res@v4@signal_0.4@pcmciplus@prec\endcsname{0.81}
\expandafter\def\csname res@v4@signal_0.4@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@pcmciplus@len\endcsname{2.6}
\expandafter\def\csname res@v4@signal_0.4@pcmciplus@rp\endcsname{0.77}
\expandafter\def\csname res@v4@signal_0.4@pcmciplus@map\endcsname{0.87}
\expandafter\def\csname res@v4@signal_0.4@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v4@signal_0.4@pc@fpn\endcsname{4}
\expandafter\def\csname res@v4@signal_0.4@pc@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v4@signal_0.4@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v4@signal_0.4@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@pc@bw\endcsname{4}
\expandafter\def\csname res@v4@signal_0.4@pc@len\endcsname{4.6}
\expandafter\def\csname res@v4@signal_0.4@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v4@signal_0.4@pc@map\endcsname{0.30}
\expandafter\def\csname res@v4@signal_0.4@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v4@signal_0.4@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v4@signal_0.4@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v4@signal_0.4@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v4@signal_0.4@dynotears@rp\endcsname{0.83}
\expandafter\def\csname res@v4@signal_0.4@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v4@signal_0.4@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v4@signal_0.4@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v4@signal_0.4@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@doubleml@tt\endcsname{0.73}
\expandafter\def\csname res@v4@signal_0.4@doubleml@prec\endcsname{0.75}
\expandafter\def\csname res@v4@signal_0.4@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v4@signal_0.4@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@doubleml@len\endcsname{3.1}
\expandafter\def\csname res@v4@signal_0.4@doubleml@rp\endcsname{0.72}
\expandafter\def\csname res@v4@signal_0.4@doubleml@map\endcsname{0.84}
\expandafter\def\csname res@v4@signal_0.4@varlingam@fp\endcsname{8/10}
\expandafter\def\csname res@v4@signal_0.4@varlingam@fpn\endcsname{8}
\expandafter\def\csname res@v4@signal_0.4@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@varlingam@tt\endcsname{0.46}
\expandafter\def\csname res@v4@signal_0.4@varlingam@prec\endcsname{0.26}
\expandafter\def\csname res@v4@signal_0.4@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v4@signal_0.4@varlingam@len\endcsname{9.3}
\expandafter\def\csname res@v4@signal_0.4@varlingam@rp\endcsname{0.43}
\expandafter\def\csname res@v4@signal_0.4@varlingam@map\endcsname{0.63}
\expandafter\def\csname res@v4@signal_0.4@spacetime_rule@fp\endcsname{5/10}
\expandafter\def\csname res@v4@signal_0.4@spacetime_rule@fpn\endcsname{5}
\expandafter\def\csname res@v4@signal_0.4@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@spacetime_rule@tt\endcsname{0.19}
\expandafter\def\csname res@v4@signal_0.4@spacetime_rule@prec\endcsname{0.71}
\expandafter\def\csname res@v4@signal_0.4@spacetime_rule@ab\endcsname{3}
\expandafter\def\csname res@v4@signal_0.4@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@spacetime_rule@len\endcsname{0.7}
\expandafter\def\csname res@v4@signal_0.4@spacetime_rule@rp\endcsname{0.46}
\expandafter\def\csname res@v4@signal_0.4@spacetime_rule@map\endcsname{0.60}
\expandafter\def\csname res@v4@signal_0.4@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@signal_0.4@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4@signal_0.4@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4@signal_0.4@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4@signal_0.4@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v4@signal_0.4@varsort@rp\endcsname{0.21}
\expandafter\def\csname res@v4@signal_0.4@varsort@map\endcsname{0.21}
\expandafter\def\csname res@v4@signal_0.4@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@signal_0.4@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.4@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v4@signal_0.4@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v4@signal_0.4@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.4@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v4@signal_0.4@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4@signal_0.4@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v4@signal_0.4@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v4@signal_0.9@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v4@signal_0.9@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@correlation@tt\endcsname{0.62}
\expandafter\def\csname res@v4@signal_0.9@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v4@signal_0.9@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@correlation@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v4@signal_0.9@correlation@rp\endcsname{0.70}
\expandafter\def\csname res@v4@signal_0.9@correlation@map\endcsname{0.81}
\expandafter\def\csname res@v4@signal_0.9@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v4@signal_0.9@granger@fpn\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@granger@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v4@signal_0.9@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v4@signal_0.9@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@granger@len\endcsname{17.1}
\expandafter\def\csname res@v4@signal_0.9@granger@rp\endcsname{0.70}
\expandafter\def\csname res@v4@signal_0.9@granger@map\endcsname{0.78}
\expandafter\def\csname res@v4@signal_0.9@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4@signal_0.9@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@pcmciplus@tt\endcsname{0.77}
\expandafter\def\csname res@v4@signal_0.9@pcmciplus@prec\endcsname{0.73}
\expandafter\def\csname res@v4@signal_0.9@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@pcmciplus@len\endcsname{3.0}
\expandafter\def\csname res@v4@signal_0.9@pcmciplus@rp\endcsname{0.93}
\expandafter\def\csname res@v4@signal_0.9@pcmciplus@map\endcsname{0.97}
\expandafter\def\csname res@v4@signal_0.9@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4@signal_0.9@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4@signal_0.9@pc@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v4@signal_0.9@pc@prec\endcsname{0.36}
\expandafter\def\csname res@v4@signal_0.9@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@pc@bw\endcsname{3}
\expandafter\def\csname res@v4@signal_0.9@pc@len\endcsname{5.5}
\expandafter\def\csname res@v4@signal_0.9@pc@rp\endcsname{0.36}
\expandafter\def\csname res@v4@signal_0.9@pc@map\endcsname{0.32}
\expandafter\def\csname res@v4@signal_0.9@dynotears@fp\endcsname{7/10}
\expandafter\def\csname res@v4@signal_0.9@dynotears@fpn\endcsname{7}
\expandafter\def\csname res@v4@signal_0.9@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@dynotears@tt\endcsname{0.46}
\expandafter\def\csname res@v4@signal_0.9@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4@signal_0.9@dynotears@ab\endcsname{3}
\expandafter\def\csname res@v4@signal_0.9@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@dynotears@len\endcsname{1.2}
\expandafter\def\csname res@v4@signal_0.9@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v4@signal_0.9@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v4@signal_0.9@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v4@signal_0.9@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v4@signal_0.9@doubleml@prec\endcsname{0.78}
\expandafter\def\csname res@v4@signal_0.9@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@doubleml@len\endcsname{3.6}
\expandafter\def\csname res@v4@signal_0.9@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v4@signal_0.9@doubleml@map\endcsname{0.94}
\expandafter\def\csname res@v4@signal_0.9@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v4@signal_0.9@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v4@signal_0.9@varlingam@prec\endcsname{0.24}
\expandafter\def\csname res@v4@signal_0.9@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@varlingam@len\endcsname{11.9}
\expandafter\def\csname res@v4@signal_0.9@varlingam@rp\endcsname{0.82}
\expandafter\def\csname res@v4@signal_0.9@varlingam@map\endcsname{0.89}
\expandafter\def\csname res@v4@signal_0.9@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v4@signal_0.9@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v4@signal_0.9@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@spacetime_rule@tt\endcsname{0.50}
\expandafter\def\csname res@v4@signal_0.9@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v4@signal_0.9@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v4@signal_0.9@spacetime_rule@rp\endcsname{0.71}
\expandafter\def\csname res@v4@signal_0.9@spacetime_rule@map\endcsname{0.78}
\expandafter\def\csname res@v4@signal_0.9@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@signal_0.9@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4@signal_0.9@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4@signal_0.9@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@varsort@bw\endcsname{2}
\expandafter\def\csname res@v4@signal_0.9@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v4@signal_0.9@varsort@rp\endcsname{0.16}
\expandafter\def\csname res@v4@signal_0.9@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v4@signal_0.9@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@signal_0.9@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@signal_0.9@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v4@signal_0.9@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v4@signal_0.9@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@signal_0.9@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v4@signal_0.9@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4@signal_0.9@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v4@signal_0.9@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v4@confound_0.1@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v4@confound_0.1@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@correlation@tt\endcsname{0.65}
\expandafter\def\csname res@v4@confound_0.1@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v4@confound_0.1@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@correlation@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@correlation@len\endcsname{18.2}
\expandafter\def\csname res@v4@confound_0.1@correlation@rp\endcsname{0.68}
\expandafter\def\csname res@v4@confound_0.1@correlation@map\endcsname{0.80}
\expandafter\def\csname res@v4@confound_0.1@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v4@confound_0.1@granger@fpn\endcsname{9}
\expandafter\def\csname res@v4@confound_0.1@granger@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v4@confound_0.1@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v4@confound_0.1@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@granger@len\endcsname{17.6}
\expandafter\def\csname res@v4@confound_0.1@granger@rp\endcsname{0.71}
\expandafter\def\csname res@v4@confound_0.1@granger@map\endcsname{0.76}
\expandafter\def\csname res@v4@confound_0.1@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4@confound_0.1@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@pcmciplus@tt\endcsname{0.81}
\expandafter\def\csname res@v4@confound_0.1@pcmciplus@prec\endcsname{0.74}
\expandafter\def\csname res@v4@confound_0.1@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@pcmciplus@len\endcsname{3.5}
\expandafter\def\csname res@v4@confound_0.1@pcmciplus@rp\endcsname{0.91}
\expandafter\def\csname res@v4@confound_0.1@pcmciplus@map\endcsname{0.97}
\expandafter\def\csname res@v4@confound_0.1@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4@confound_0.1@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4@confound_0.1@pc@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v4@confound_0.1@pc@prec\endcsname{0.36}
\expandafter\def\csname res@v4@confound_0.1@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@pc@bw\endcsname{3}
\expandafter\def\csname res@v4@confound_0.1@pc@len\endcsname{5.3}
\expandafter\def\csname res@v4@confound_0.1@pc@rp\endcsname{0.36}
\expandafter\def\csname res@v4@confound_0.1@pc@map\endcsname{0.32}
\expandafter\def\csname res@v4@confound_0.1@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v4@confound_0.1@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v4@confound_0.1@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@dynotears@tt\endcsname{0.31}
\expandafter\def\csname res@v4@confound_0.1@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4@confound_0.1@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v4@confound_0.1@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@dynotears@len\endcsname{0.8}
\expandafter\def\csname res@v4@confound_0.1@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v4@confound_0.1@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v4@confound_0.1@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v4@confound_0.1@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v4@confound_0.1@doubleml@prec\endcsname{0.74}
\expandafter\def\csname res@v4@confound_0.1@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@doubleml@len\endcsname{3.8}
\expandafter\def\csname res@v4@confound_0.1@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v4@confound_0.1@doubleml@map\endcsname{0.95}
\expandafter\def\csname res@v4@confound_0.1@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v4@confound_0.1@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v4@confound_0.1@varlingam@prec\endcsname{0.23}
\expandafter\def\csname res@v4@confound_0.1@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@varlingam@len\endcsname{12.0}
\expandafter\def\csname res@v4@confound_0.1@varlingam@rp\endcsname{0.66}
\expandafter\def\csname res@v4@confound_0.1@varlingam@map\endcsname{0.81}
\expandafter\def\csname res@v4@confound_0.1@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v4@confound_0.1@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v4@confound_0.1@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@spacetime_rule@tt\endcsname{0.38}
\expandafter\def\csname res@v4@confound_0.1@spacetime_rule@prec\endcsname{0.94}
\expandafter\def\csname res@v4@confound_0.1@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v4@confound_0.1@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v4@confound_0.1@spacetime_rule@rp\endcsname{0.64}
\expandafter\def\csname res@v4@confound_0.1@spacetime_rule@map\endcsname{0.76}
\expandafter\def\csname res@v4@confound_0.1@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v4@confound_0.1@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v4@confound_0.1@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4@confound_0.1@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4@confound_0.1@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@varsort@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v4@confound_0.1@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v4@confound_0.1@varsort@map\endcsname{0.24}
\expandafter\def\csname res@v4@confound_0.1@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v4@confound_0.1@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v4@confound_0.1@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.1@r2sort@tt\endcsname{0.19}
\expandafter\def\csname res@v4@confound_0.1@r2sort@prec\endcsname{0.17}
\expandafter\def\csname res@v4@confound_0.1@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.1@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v4@confound_0.1@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4@confound_0.1@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v4@confound_0.1@r2sort@map\endcsname{0.22}
\expandafter\def\csname res@v4@confound_0.6@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v4@confound_0.6@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v4@confound_0.6@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@correlation@tt\endcsname{0.50}
\expandafter\def\csname res@v4@confound_0.6@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v4@confound_0.6@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@correlation@bw\endcsname{1}
\expandafter\def\csname res@v4@confound_0.6@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v4@confound_0.6@correlation@rp\endcsname{0.57}
\expandafter\def\csname res@v4@confound_0.6@correlation@map\endcsname{0.67}
\expandafter\def\csname res@v4@confound_0.6@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v4@confound_0.6@granger@fpn\endcsname{9}
\expandafter\def\csname res@v4@confound_0.6@granger@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@granger@tt\endcsname{0.46}
\expandafter\def\csname res@v4@confound_0.6@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v4@confound_0.6@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@granger@len\endcsname{16.2}
\expandafter\def\csname res@v4@confound_0.6@granger@rp\endcsname{0.56}
\expandafter\def\csname res@v4@confound_0.6@granger@map\endcsname{0.70}
\expandafter\def\csname res@v4@confound_0.6@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4@confound_0.6@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v4@confound_0.6@pcmciplus@prec\endcsname{0.80}
\expandafter\def\csname res@v4@confound_0.6@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@pcmciplus@len\endcsname{2.4}
\expandafter\def\csname res@v4@confound_0.6@pcmciplus@rp\endcsname{0.93}
\expandafter\def\csname res@v4@confound_0.6@pcmciplus@map\endcsname{0.93}
\expandafter\def\csname res@v4@confound_0.6@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4@confound_0.6@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4@confound_0.6@pc@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v4@confound_0.6@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v4@confound_0.6@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@pc@bw\endcsname{3}
\expandafter\def\csname res@v4@confound_0.6@pc@len\endcsname{5.4}
\expandafter\def\csname res@v4@confound_0.6@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v4@confound_0.6@pc@map\endcsname{0.29}
\expandafter\def\csname res@v4@confound_0.6@dynotears@fp\endcsname{3/10}
\expandafter\def\csname res@v4@confound_0.6@dynotears@fpn\endcsname{3}
\expandafter\def\csname res@v4@confound_0.6@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@dynotears@tt\endcsname{0.15}
\expandafter\def\csname res@v4@confound_0.6@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4@confound_0.6@dynotears@ab\endcsname{7}
\expandafter\def\csname res@v4@confound_0.6@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@dynotears@len\endcsname{0.4}
\expandafter\def\csname res@v4@confound_0.6@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v4@confound_0.6@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v4@confound_0.6@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v4@confound_0.6@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v4@confound_0.6@doubleml@prec\endcsname{0.73}
\expandafter\def\csname res@v4@confound_0.6@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@doubleml@len\endcsname{3.8}
\expandafter\def\csname res@v4@confound_0.6@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v4@confound_0.6@doubleml@map\endcsname{0.94}
\expandafter\def\csname res@v4@confound_0.6@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v4@confound_0.6@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v4@confound_0.6@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v4@confound_0.6@varlingam@prec\endcsname{0.28}
\expandafter\def\csname res@v4@confound_0.6@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@varlingam@len\endcsname{9.6}
\expandafter\def\csname res@v4@confound_0.6@varlingam@rp\endcsname{0.72}
\expandafter\def\csname res@v4@confound_0.6@varlingam@map\endcsname{0.80}
\expandafter\def\csname res@v4@confound_0.6@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v4@confound_0.6@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v4@confound_0.6@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v4@confound_0.6@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v4@confound_0.6@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v4@confound_0.6@spacetime_rule@rp\endcsname{0.59}
\expandafter\def\csname res@v4@confound_0.6@spacetime_rule@map\endcsname{0.70}
\expandafter\def\csname res@v4@confound_0.6@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v4@confound_0.6@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v4@confound_0.6@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4@confound_0.6@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4@confound_0.6@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@varsort@bw\endcsname{2}
\expandafter\def\csname res@v4@confound_0.6@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v4@confound_0.6@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v4@confound_0.6@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v4@confound_0.6@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v4@confound_0.6@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v4@confound_0.6@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@confound_0.6@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v4@confound_0.6@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v4@confound_0.6@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@confound_0.6@r2sort@bw\endcsname{3}
\expandafter\def\csname res@v4@confound_0.6@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v4@confound_0.6@r2sort@rp\endcsname{0.14}
\expandafter\def\csname res@v4@confound_0.6@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v4@conseq_0.1@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v4@conseq_0.1@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@correlation@tt\endcsname{0.62}
\expandafter\def\csname res@v4@conseq_0.1@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v4@conseq_0.1@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@correlation@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@correlation@len\endcsname{18.1}
\expandafter\def\csname res@v4@conseq_0.1@correlation@rp\endcsname{0.68}
\expandafter\def\csname res@v4@conseq_0.1@correlation@map\endcsname{0.80}
\expandafter\def\csname res@v4@conseq_0.1@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v4@conseq_0.1@granger@fpn\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@granger@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v4@conseq_0.1@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v4@conseq_0.1@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@granger@len\endcsname{17.2}
\expandafter\def\csname res@v4@conseq_0.1@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v4@conseq_0.1@granger@map\endcsname{0.78}
\expandafter\def\csname res@v4@conseq_0.1@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4@conseq_0.1@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v4@conseq_0.1@pcmciplus@prec\endcsname{0.79}
\expandafter\def\csname res@v4@conseq_0.1@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@pcmciplus@len\endcsname{2.7}
\expandafter\def\csname res@v4@conseq_0.1@pcmciplus@rp\endcsname{0.89}
\expandafter\def\csname res@v4@conseq_0.1@pcmciplus@map\endcsname{0.96}
\expandafter\def\csname res@v4@conseq_0.1@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4@conseq_0.1@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4@conseq_0.1@pc@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v4@conseq_0.1@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v4@conseq_0.1@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@pc@bw\endcsname{3}
\expandafter\def\csname res@v4@conseq_0.1@pc@len\endcsname{5.2}
\expandafter\def\csname res@v4@conseq_0.1@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v4@conseq_0.1@pc@map\endcsname{0.30}
\expandafter\def\csname res@v4@conseq_0.1@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v4@conseq_0.1@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v4@conseq_0.1@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@dynotears@tt\endcsname{0.27}
\expandafter\def\csname res@v4@conseq_0.1@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4@conseq_0.1@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v4@conseq_0.1@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v4@conseq_0.1@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v4@conseq_0.1@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v4@conseq_0.1@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v4@conseq_0.1@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v4@conseq_0.1@doubleml@prec\endcsname{0.66}
\expandafter\def\csname res@v4@conseq_0.1@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@doubleml@len\endcsname{4.1}
\expandafter\def\csname res@v4@conseq_0.1@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v4@conseq_0.1@doubleml@map\endcsname{0.93}
\expandafter\def\csname res@v4@conseq_0.1@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v4@conseq_0.1@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@varlingam@tt\endcsname{0.73}
\expandafter\def\csname res@v4@conseq_0.1@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v4@conseq_0.1@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@varlingam@len\endcsname{10.0}
\expandafter\def\csname res@v4@conseq_0.1@varlingam@rp\endcsname{0.79}
\expandafter\def\csname res@v4@conseq_0.1@varlingam@map\endcsname{0.88}
\expandafter\def\csname res@v4@conseq_0.1@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v4@conseq_0.1@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v4@conseq_0.1@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v4@conseq_0.1@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v4@conseq_0.1@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v4@conseq_0.1@spacetime_rule@rp\endcsname{0.59}
\expandafter\def\csname res@v4@conseq_0.1@spacetime_rule@map\endcsname{0.76}
\expandafter\def\csname res@v4@conseq_0.1@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@conseq_0.1@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4@conseq_0.1@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4@conseq_0.1@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4@conseq_0.1@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v4@conseq_0.1@varsort@rp\endcsname{0.21}
\expandafter\def\csname res@v4@conseq_0.1@varsort@map\endcsname{0.21}
\expandafter\def\csname res@v4@conseq_0.1@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@conseq_0.1@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.1@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v4@conseq_0.1@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v4@conseq_0.1@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.1@r2sort@bw\endcsname{4}
\expandafter\def\csname res@v4@conseq_0.1@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4@conseq_0.1@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v4@conseq_0.1@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v4@conseq_0.5@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v4@conseq_0.5@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v4@conseq_0.5@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v4@conseq_0.5@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v4@conseq_0.5@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@correlation@bw\endcsname{2}
\expandafter\def\csname res@v4@conseq_0.5@correlation@len\endcsname{18.2}
\expandafter\def\csname res@v4@conseq_0.5@correlation@rp\endcsname{0.57}
\expandafter\def\csname res@v4@conseq_0.5@correlation@map\endcsname{0.69}
\expandafter\def\csname res@v4@conseq_0.5@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v4@conseq_0.5@granger@fpn\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@granger@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v4@conseq_0.5@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v4@conseq_0.5@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@granger@len\endcsname{17.1}
\expandafter\def\csname res@v4@conseq_0.5@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v4@conseq_0.5@granger@map\endcsname{0.78}
\expandafter\def\csname res@v4@conseq_0.5@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4@conseq_0.5@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v4@conseq_0.5@pcmciplus@prec\endcsname{0.74}
\expandafter\def\csname res@v4@conseq_0.5@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@pcmciplus@len\endcsname{2.8}
\expandafter\def\csname res@v4@conseq_0.5@pcmciplus@rp\endcsname{0.89}
\expandafter\def\csname res@v4@conseq_0.5@pcmciplus@map\endcsname{0.96}
\expandafter\def\csname res@v4@conseq_0.5@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4@conseq_0.5@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4@conseq_0.5@pc@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v4@conseq_0.5@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v4@conseq_0.5@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@pc@bw\endcsname{4}
\expandafter\def\csname res@v4@conseq_0.5@pc@len\endcsname{5.2}
\expandafter\def\csname res@v4@conseq_0.5@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v4@conseq_0.5@pc@map\endcsname{0.30}
\expandafter\def\csname res@v4@conseq_0.5@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v4@conseq_0.5@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v4@conseq_0.5@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@dynotears@tt\endcsname{0.27}
\expandafter\def\csname res@v4@conseq_0.5@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4@conseq_0.5@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v4@conseq_0.5@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v4@conseq_0.5@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v4@conseq_0.5@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v4@conseq_0.5@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v4@conseq_0.5@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v4@conseq_0.5@doubleml@prec\endcsname{0.71}
\expandafter\def\csname res@v4@conseq_0.5@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@doubleml@len\endcsname{3.9}
\expandafter\def\csname res@v4@conseq_0.5@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v4@conseq_0.5@doubleml@map\endcsname{0.94}
\expandafter\def\csname res@v4@conseq_0.5@varlingam@fp\endcsname{7/10}
\expandafter\def\csname res@v4@conseq_0.5@varlingam@fpn\endcsname{7}
\expandafter\def\csname res@v4@conseq_0.5@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@varlingam@tt\endcsname{0.62}
\expandafter\def\csname res@v4@conseq_0.5@varlingam@prec\endcsname{0.26}
\expandafter\def\csname res@v4@conseq_0.5@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@varlingam@bw\endcsname{3}
\expandafter\def\csname res@v4@conseq_0.5@varlingam@len\endcsname{10.8}
\expandafter\def\csname res@v4@conseq_0.5@varlingam@rp\endcsname{0.58}
\expandafter\def\csname res@v4@conseq_0.5@varlingam@map\endcsname{0.72}
\expandafter\def\csname res@v4@conseq_0.5@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v4@conseq_0.5@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v4@conseq_0.5@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v4@conseq_0.5@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v4@conseq_0.5@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v4@conseq_0.5@spacetime_rule@rp\endcsname{0.59}
\expandafter\def\csname res@v4@conseq_0.5@spacetime_rule@map\endcsname{0.77}
\expandafter\def\csname res@v4@conseq_0.5@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@conseq_0.5@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4@conseq_0.5@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4@conseq_0.5@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@varsort@bw\endcsname{3}
\expandafter\def\csname res@v4@conseq_0.5@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v4@conseq_0.5@varsort@rp\endcsname{0.16}
\expandafter\def\csname res@v4@conseq_0.5@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v4@conseq_0.5@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@conseq_0.5@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@conseq_0.5@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v4@conseq_0.5@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v4@conseq_0.5@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v4@conseq_0.5@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4@conseq_0.5@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v4@conseq_0.5@r2sort@map\endcsname{0.19}
\expandafter\def\csname res@v4@echo_0.1@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v4@echo_0.1@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v4@echo_0.1@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@correlation@tt\endcsname{0.62}
\expandafter\def\csname res@v4@echo_0.1@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v4@echo_0.1@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@correlation@bw\endcsname{1}
\expandafter\def\csname res@v4@echo_0.1@correlation@len\endcsname{17.7}
\expandafter\def\csname res@v4@echo_0.1@correlation@rp\endcsname{0.71}
\expandafter\def\csname res@v4@echo_0.1@correlation@map\endcsname{0.76}
\expandafter\def\csname res@v4@echo_0.1@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v4@echo_0.1@granger@fpn\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@granger@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@granger@tt\endcsname{0.69}
\expandafter\def\csname res@v4@echo_0.1@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v4@echo_0.1@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@granger@len\endcsname{17.1}
\expandafter\def\csname res@v4@echo_0.1@granger@rp\endcsname{0.74}
\expandafter\def\csname res@v4@echo_0.1@granger@map\endcsname{0.81}
\expandafter\def\csname res@v4@echo_0.1@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4@echo_0.1@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@pcmciplus@tt\endcsname{0.85}
\expandafter\def\csname res@v4@echo_0.1@pcmciplus@prec\endcsname{0.75}
\expandafter\def\csname res@v4@echo_0.1@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@pcmciplus@len\endcsname{3.1}
\expandafter\def\csname res@v4@echo_0.1@pcmciplus@rp\endcsname{0.97}
\expandafter\def\csname res@v4@echo_0.1@pcmciplus@map\endcsname{0.98}
\expandafter\def\csname res@v4@echo_0.1@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4@echo_0.1@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4@echo_0.1@pc@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v4@echo_0.1@pc@prec\endcsname{0.38}
\expandafter\def\csname res@v4@echo_0.1@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@pc@bw\endcsname{4}
\expandafter\def\csname res@v4@echo_0.1@pc@len\endcsname{5.0}
\expandafter\def\csname res@v4@echo_0.1@pc@rp\endcsname{0.38}
\expandafter\def\csname res@v4@echo_0.1@pc@map\endcsname{0.33}
\expandafter\def\csname res@v4@echo_0.1@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v4@echo_0.1@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v4@echo_0.1@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@dynotears@tt\endcsname{0.31}
\expandafter\def\csname res@v4@echo_0.1@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4@echo_0.1@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v4@echo_0.1@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@dynotears@len\endcsname{0.8}
\expandafter\def\csname res@v4@echo_0.1@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v4@echo_0.1@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v4@echo_0.1@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v4@echo_0.1@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v4@echo_0.1@doubleml@prec\endcsname{0.77}
\expandafter\def\csname res@v4@echo_0.1@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@doubleml@len\endcsname{3.5}
\expandafter\def\csname res@v4@echo_0.1@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v4@echo_0.1@doubleml@map\endcsname{0.95}
\expandafter\def\csname res@v4@echo_0.1@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v4@echo_0.1@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@varlingam@tt\endcsname{0.81}
\expandafter\def\csname res@v4@echo_0.1@varlingam@prec\endcsname{0.36}
\expandafter\def\csname res@v4@echo_0.1@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@varlingam@len\endcsname{9.5}
\expandafter\def\csname res@v4@echo_0.1@varlingam@rp\endcsname{0.80}
\expandafter\def\csname res@v4@echo_0.1@varlingam@map\endcsname{0.91}
\expandafter\def\csname res@v4@echo_0.1@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v4@echo_0.1@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v4@echo_0.1@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v4@echo_0.1@spacetime_rule@prec\endcsname{0.94}
\expandafter\def\csname res@v4@echo_0.1@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v4@echo_0.1@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v4@echo_0.1@spacetime_rule@rp\endcsname{0.65}
\expandafter\def\csname res@v4@echo_0.1@spacetime_rule@map\endcsname{0.79}
\expandafter\def\csname res@v4@echo_0.1@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v4@echo_0.1@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v4@echo_0.1@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v4@echo_0.1@varsort@prec\endcsname{0.20}
\expandafter\def\csname res@v4@echo_0.1@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4@echo_0.1@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v4@echo_0.1@varsort@rp\endcsname{0.11}
\expandafter\def\csname res@v4@echo_0.1@varsort@map\endcsname{0.33}
\expandafter\def\csname res@v4@echo_0.1@r2sort@fp\endcsname{2/10}
\expandafter\def\csname res@v4@echo_0.1@r2sort@fpn\endcsname{2}
\expandafter\def\csname res@v4@echo_0.1@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.1@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v4@echo_0.1@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v4@echo_0.1@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.1@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v4@echo_0.1@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4@echo_0.1@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v4@echo_0.1@r2sort@map\endcsname{0.22}
\expandafter\def\csname res@v4@echo_0.6@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v4@echo_0.6@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v4@echo_0.6@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v4@echo_0.6@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@correlation@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@correlation@len\endcsname{18.4}
\expandafter\def\csname res@v4@echo_0.6@correlation@rp\endcsname{0.64}
\expandafter\def\csname res@v4@echo_0.6@correlation@map\endcsname{0.79}
\expandafter\def\csname res@v4@echo_0.6@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v4@echo_0.6@granger@fpn\endcsname{9}
\expandafter\def\csname res@v4@echo_0.6@granger@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v4@echo_0.6@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v4@echo_0.6@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@granger@len\endcsname{17.8}
\expandafter\def\csname res@v4@echo_0.6@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v4@echo_0.6@granger@map\endcsname{0.76}
\expandafter\def\csname res@v4@echo_0.6@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4@echo_0.6@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@pcmciplus@tt\endcsname{0.65}
\expandafter\def\csname res@v4@echo_0.6@pcmciplus@prec\endcsname{0.65}
\expandafter\def\csname res@v4@echo_0.6@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@pcmciplus@len\endcsname{3.2}
\expandafter\def\csname res@v4@echo_0.6@pcmciplus@rp\endcsname{0.93}
\expandafter\def\csname res@v4@echo_0.6@pcmciplus@map\endcsname{0.96}
\expandafter\def\csname res@v4@echo_0.6@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v4@echo_0.6@pc@fpn\endcsname{4}
\expandafter\def\csname res@v4@echo_0.6@pc@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@pc@tt\endcsname{0.42}
\expandafter\def\csname res@v4@echo_0.6@pc@prec\endcsname{0.33}
\expandafter\def\csname res@v4@echo_0.6@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@pc@bw\endcsname{4}
\expandafter\def\csname res@v4@echo_0.6@pc@len\endcsname{5.4}
\expandafter\def\csname res@v4@echo_0.6@pc@rp\endcsname{0.31}
\expandafter\def\csname res@v4@echo_0.6@pc@map\endcsname{0.30}
\expandafter\def\csname res@v4@echo_0.6@dynotears@fp\endcsname{5/10}
\expandafter\def\csname res@v4@echo_0.6@dynotears@fpn\endcsname{5}
\expandafter\def\csname res@v4@echo_0.6@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@dynotears@tt\endcsname{0.23}
\expandafter\def\csname res@v4@echo_0.6@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4@echo_0.6@dynotears@ab\endcsname{5}
\expandafter\def\csname res@v4@echo_0.6@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@dynotears@len\endcsname{0.6}
\expandafter\def\csname res@v4@echo_0.6@dynotears@rp\endcsname{0.88}
\expandafter\def\csname res@v4@echo_0.6@dynotears@map\endcsname{0.91}
\expandafter\def\csname res@v4@echo_0.6@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v4@echo_0.6@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@doubleml@tt\endcsname{0.73}
\expandafter\def\csname res@v4@echo_0.6@doubleml@prec\endcsname{0.81}
\expandafter\def\csname res@v4@echo_0.6@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@doubleml@len\endcsname{3.2}
\expandafter\def\csname res@v4@echo_0.6@doubleml@rp\endcsname{0.81}
\expandafter\def\csname res@v4@echo_0.6@doubleml@map\endcsname{0.92}
\expandafter\def\csname res@v4@echo_0.6@varlingam@fp\endcsname{7/10}
\expandafter\def\csname res@v4@echo_0.6@varlingam@fpn\endcsname{7}
\expandafter\def\csname res@v4@echo_0.6@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@varlingam@tt\endcsname{0.54}
\expandafter\def\csname res@v4@echo_0.6@varlingam@prec\endcsname{0.22}
\expandafter\def\csname res@v4@echo_0.6@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v4@echo_0.6@varlingam@len\endcsname{11.4}
\expandafter\def\csname res@v4@echo_0.6@varlingam@rp\endcsname{0.60}
\expandafter\def\csname res@v4@echo_0.6@varlingam@map\endcsname{0.65}
\expandafter\def\csname res@v4@echo_0.6@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v4@echo_0.6@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v4@echo_0.6@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v4@echo_0.6@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v4@echo_0.6@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v4@echo_0.6@spacetime_rule@rp\endcsname{0.53}
\expandafter\def\csname res@v4@echo_0.6@spacetime_rule@map\endcsname{0.73}
\expandafter\def\csname res@v4@echo_0.6@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v4@echo_0.6@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v4@echo_0.6@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v4@echo_0.6@varsort@prec\endcsname{0.20}
\expandafter\def\csname res@v4@echo_0.6@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4@echo_0.6@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v4@echo_0.6@varsort@rp\endcsname{0.19}
\expandafter\def\csname res@v4@echo_0.6@varsort@map\endcsname{0.25}
\expandafter\def\csname res@v4@echo_0.6@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@echo_0.6@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@echo_0.6@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v4@echo_0.6@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v4@echo_0.6@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@echo_0.6@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v4@echo_0.6@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4@echo_0.6@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v4@echo_0.6@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v4@control_0.3@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v4@control_0.3@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v4@control_0.3@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@correlation@tt\endcsname{0.69}
\expandafter\def\csname res@v4@control_0.3@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v4@control_0.3@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@correlation@bw\endcsname{1}
\expandafter\def\csname res@v4@control_0.3@correlation@len\endcsname{16.1}
\expandafter\def\csname res@v4@control_0.3@correlation@rp\endcsname{0.64}
\expandafter\def\csname res@v4@control_0.3@correlation@map\endcsname{0.73}
\expandafter\def\csname res@v4@control_0.3@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v4@control_0.3@granger@fpn\endcsname{9}
\expandafter\def\csname res@v4@control_0.3@granger@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@granger@tt\endcsname{0.69}
\expandafter\def\csname res@v4@control_0.3@granger@prec\endcsname{0.19}
\expandafter\def\csname res@v4@control_0.3@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@granger@len\endcsname{14.6}
\expandafter\def\csname res@v4@control_0.3@granger@rp\endcsname{0.70}
\expandafter\def\csname res@v4@control_0.3@granger@map\endcsname{0.83}
\expandafter\def\csname res@v4@control_0.3@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4@control_0.3@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@pcmciplus@tt\endcsname{0.85}
\expandafter\def\csname res@v4@control_0.3@pcmciplus@prec\endcsname{0.73}
\expandafter\def\csname res@v4@control_0.3@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@pcmciplus@len\endcsname{3.1}
\expandafter\def\csname res@v4@control_0.3@pcmciplus@rp\endcsname{0.88}
\expandafter\def\csname res@v4@control_0.3@pcmciplus@map\endcsname{0.92}
\expandafter\def\csname res@v4@control_0.3@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4@control_0.3@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4@control_0.3@pc@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v4@control_0.3@pc@prec\endcsname{0.31}
\expandafter\def\csname res@v4@control_0.3@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@pc@bw\endcsname{4}
\expandafter\def\csname res@v4@control_0.3@pc@len\endcsname{5.2}
\expandafter\def\csname res@v4@control_0.3@pc@rp\endcsname{0.31}
\expandafter\def\csname res@v4@control_0.3@pc@map\endcsname{0.28}
\expandafter\def\csname res@v4@control_0.3@dynotears@fp\endcsname{3/10}
\expandafter\def\csname res@v4@control_0.3@dynotears@fpn\endcsname{3}
\expandafter\def\csname res@v4@control_0.3@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@dynotears@tt\endcsname{0.12}
\expandafter\def\csname res@v4@control_0.3@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4@control_0.3@dynotears@ab\endcsname{7}
\expandafter\def\csname res@v4@control_0.3@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@dynotears@len\endcsname{0.3}
\expandafter\def\csname res@v4@control_0.3@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v4@control_0.3@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v4@control_0.3@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v4@control_0.3@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v4@control_0.3@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v4@control_0.3@doubleml@prec\endcsname{0.75}
\expandafter\def\csname res@v4@control_0.3@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v4@control_0.3@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@doubleml@len\endcsname{3.0}
\expandafter\def\csname res@v4@control_0.3@doubleml@rp\endcsname{0.85}
\expandafter\def\csname res@v4@control_0.3@doubleml@map\endcsname{0.85}
\expandafter\def\csname res@v4@control_0.3@varlingam@fp\endcsname{8/10}
\expandafter\def\csname res@v4@control_0.3@varlingam@fpn\endcsname{8}
\expandafter\def\csname res@v4@control_0.3@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v4@control_0.3@varlingam@prec\endcsname{0.31}
\expandafter\def\csname res@v4@control_0.3@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v4@control_0.3@varlingam@len\endcsname{7.5}
\expandafter\def\csname res@v4@control_0.3@varlingam@rp\endcsname{0.68}
\expandafter\def\csname res@v4@control_0.3@varlingam@map\endcsname{0.75}
\expandafter\def\csname res@v4@control_0.3@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v4@control_0.3@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v4@control_0.3@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v4@control_0.3@spacetime_rule@prec\endcsname{0.80}
\expandafter\def\csname res@v4@control_0.3@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v4@control_0.3@spacetime_rule@rp\endcsname{0.60}
\expandafter\def\csname res@v4@control_0.3@spacetime_rule@map\endcsname{0.67}
\expandafter\def\csname res@v4@control_0.3@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@control_0.3@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4@control_0.3@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4@control_0.3@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4@control_0.3@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v4@control_0.3@varsort@rp\endcsname{0.22}
\expandafter\def\csname res@v4@control_0.3@varsort@map\endcsname{0.29}
\expandafter\def\csname res@v4@control_0.3@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v4@control_0.3@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v4@control_0.3@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.3@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v4@control_0.3@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v4@control_0.3@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.3@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v4@control_0.3@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4@control_0.3@r2sort@rp\endcsname{0.20}
\expandafter\def\csname res@v4@control_0.3@r2sort@map\endcsname{0.29}
\expandafter\def\csname res@v4@control_0.6@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v4@control_0.6@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v4@control_0.6@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@correlation@tt\endcsname{0.69}
\expandafter\def\csname res@v4@control_0.6@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v4@control_0.6@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@correlation@bw\endcsname{1}
\expandafter\def\csname res@v4@control_0.6@correlation@len\endcsname{16.0}
\expandafter\def\csname res@v4@control_0.6@correlation@rp\endcsname{0.67}
\expandafter\def\csname res@v4@control_0.6@correlation@map\endcsname{0.74}
\expandafter\def\csname res@v4@control_0.6@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v4@control_0.6@granger@fpn\endcsname{9}
\expandafter\def\csname res@v4@control_0.6@granger@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v4@control_0.6@granger@prec\endcsname{0.18}
\expandafter\def\csname res@v4@control_0.6@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@granger@len\endcsname{14.6}
\expandafter\def\csname res@v4@control_0.6@granger@rp\endcsname{0.70}
\expandafter\def\csname res@v4@control_0.6@granger@map\endcsname{0.81}
\expandafter\def\csname res@v4@control_0.6@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4@control_0.6@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@pcmciplus@tt\endcsname{0.85}
\expandafter\def\csname res@v4@control_0.6@pcmciplus@prec\endcsname{0.83}
\expandafter\def\csname res@v4@control_0.6@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@pcmciplus@len\endcsname{2.8}
\expandafter\def\csname res@v4@control_0.6@pcmciplus@rp\endcsname{0.88}
\expandafter\def\csname res@v4@control_0.6@pcmciplus@map\endcsname{0.92}
\expandafter\def\csname res@v4@control_0.6@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4@control_0.6@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4@control_0.6@pc@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v4@control_0.6@pc@prec\endcsname{0.32}
\expandafter\def\csname res@v4@control_0.6@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@pc@bw\endcsname{4}
\expandafter\def\csname res@v4@control_0.6@pc@len\endcsname{5.0}
\expandafter\def\csname res@v4@control_0.6@pc@rp\endcsname{0.32}
\expandafter\def\csname res@v4@control_0.6@pc@map\endcsname{0.28}
\expandafter\def\csname res@v4@control_0.6@dynotears@fp\endcsname{3/10}
\expandafter\def\csname res@v4@control_0.6@dynotears@fpn\endcsname{3}
\expandafter\def\csname res@v4@control_0.6@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@dynotears@tt\endcsname{0.12}
\expandafter\def\csname res@v4@control_0.6@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4@control_0.6@dynotears@ab\endcsname{7}
\expandafter\def\csname res@v4@control_0.6@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@dynotears@len\endcsname{0.3}
\expandafter\def\csname res@v4@control_0.6@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v4@control_0.6@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v4@control_0.6@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v4@control_0.6@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v4@control_0.6@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v4@control_0.6@doubleml@prec\endcsname{0.81}
\expandafter\def\csname res@v4@control_0.6@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v4@control_0.6@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@doubleml@len\endcsname{2.9}
\expandafter\def\csname res@v4@control_0.6@doubleml@rp\endcsname{0.82}
\expandafter\def\csname res@v4@control_0.6@doubleml@map\endcsname{0.86}
\expandafter\def\csname res@v4@control_0.6@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v4@control_0.6@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v4@control_0.6@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@varlingam@tt\endcsname{0.73}
\expandafter\def\csname res@v4@control_0.6@varlingam@prec\endcsname{0.34}
\expandafter\def\csname res@v4@control_0.6@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v4@control_0.6@varlingam@len\endcsname{7.4}
\expandafter\def\csname res@v4@control_0.6@varlingam@rp\endcsname{0.69}
\expandafter\def\csname res@v4@control_0.6@varlingam@map\endcsname{0.80}
\expandafter\def\csname res@v4@control_0.6@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v4@control_0.6@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v4@control_0.6@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v4@control_0.6@spacetime_rule@prec\endcsname{0.80}
\expandafter\def\csname res@v4@control_0.6@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v4@control_0.6@spacetime_rule@rp\endcsname{0.60}
\expandafter\def\csname res@v4@control_0.6@spacetime_rule@map\endcsname{0.67}
\expandafter\def\csname res@v4@control_0.6@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v4@control_0.6@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4@control_0.6@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4@control_0.6@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4@control_0.6@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v4@control_0.6@varsort@rp\endcsname{0.22}
\expandafter\def\csname res@v4@control_0.6@varsort@map\endcsname{0.29}
\expandafter\def\csname res@v4@control_0.6@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v4@control_0.6@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v4@control_0.6@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@control_0.6@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v4@control_0.6@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v4@control_0.6@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@control_0.6@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v4@control_0.6@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4@control_0.6@r2sort@rp\endcsname{0.20}
\expandafter\def\csname res@v4@control_0.6@r2sort@map\endcsname{0.29}
\expandafter\def\csname res@v4@control_1.0@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v4@control_1.0@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v4@control_1.0@correlation@n\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@correlation@tt\endcsname{0.69}
\expandafter\def\csname res@v4@control_1.0@correlation@prec\endcsname{0.16}
\expandafter\def\csname res@v4@control_1.0@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@correlation@bw\endcsname{1}
\expandafter\def\csname res@v4@control_1.0@correlation@len\endcsname{16.0}
\expandafter\def\csname res@v4@control_1.0@correlation@rp\endcsname{0.67}
\expandafter\def\csname res@v4@control_1.0@correlation@map\endcsname{0.74}
\expandafter\def\csname res@v4@control_1.0@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v4@control_1.0@granger@fpn\endcsname{9}
\expandafter\def\csname res@v4@control_1.0@granger@n\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v4@control_1.0@granger@prec\endcsname{0.19}
\expandafter\def\csname res@v4@control_1.0@granger@ab\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@granger@bw\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@granger@len\endcsname{14.5}
\expandafter\def\csname res@v4@control_1.0@granger@rp\endcsname{0.70}
\expandafter\def\csname res@v4@control_1.0@granger@map\endcsname{0.81}
\expandafter\def\csname res@v4@control_1.0@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4@control_1.0@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@pcmciplus@tt\endcsname{0.85}
\expandafter\def\csname res@v4@control_1.0@pcmciplus@prec\endcsname{0.83}
\expandafter\def\csname res@v4@control_1.0@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@pcmciplus@len\endcsname{2.8}
\expandafter\def\csname res@v4@control_1.0@pcmciplus@rp\endcsname{0.85}
\expandafter\def\csname res@v4@control_1.0@pcmciplus@map\endcsname{0.90}
\expandafter\def\csname res@v4@control_1.0@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4@control_1.0@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4@control_1.0@pc@n\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v4@control_1.0@pc@prec\endcsname{0.32}
\expandafter\def\csname res@v4@control_1.0@pc@ab\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@pc@bw\endcsname{4}
\expandafter\def\csname res@v4@control_1.0@pc@len\endcsname{5.0}
\expandafter\def\csname res@v4@control_1.0@pc@rp\endcsname{0.32}
\expandafter\def\csname res@v4@control_1.0@pc@map\endcsname{0.28}
\expandafter\def\csname res@v4@control_1.0@dynotears@fp\endcsname{3/10}
\expandafter\def\csname res@v4@control_1.0@dynotears@fpn\endcsname{3}
\expandafter\def\csname res@v4@control_1.0@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@dynotears@tt\endcsname{0.12}
\expandafter\def\csname res@v4@control_1.0@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4@control_1.0@dynotears@ab\endcsname{7}
\expandafter\def\csname res@v4@control_1.0@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@dynotears@len\endcsname{0.3}
\expandafter\def\csname res@v4@control_1.0@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v4@control_1.0@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v4@control_1.0@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v4@control_1.0@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v4@control_1.0@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v4@control_1.0@doubleml@prec\endcsname{0.77}
\expandafter\def\csname res@v4@control_1.0@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v4@control_1.0@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@doubleml@len\endcsname{2.9}
\expandafter\def\csname res@v4@control_1.0@doubleml@rp\endcsname{0.85}
\expandafter\def\csname res@v4@control_1.0@doubleml@map\endcsname{0.85}
\expandafter\def\csname res@v4@control_1.0@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v4@control_1.0@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v4@control_1.0@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v4@control_1.0@varlingam@prec\endcsname{0.33}
\expandafter\def\csname res@v4@control_1.0@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v4@control_1.0@varlingam@len\endcsname{7.8}
\expandafter\def\csname res@v4@control_1.0@varlingam@rp\endcsname{0.66}
\expandafter\def\csname res@v4@control_1.0@varlingam@map\endcsname{0.77}
\expandafter\def\csname res@v4@control_1.0@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v4@control_1.0@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v4@control_1.0@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v4@control_1.0@spacetime_rule@prec\endcsname{0.80}
\expandafter\def\csname res@v4@control_1.0@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v4@control_1.0@spacetime_rule@rp\endcsname{0.60}
\expandafter\def\csname res@v4@control_1.0@spacetime_rule@map\endcsname{0.67}
\expandafter\def\csname res@v4@control_1.0@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v4@control_1.0@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v4@control_1.0@varsort@n\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v4@control_1.0@varsort@prec\endcsname{0.20}
\expandafter\def\csname res@v4@control_1.0@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@varsort@bw\endcsname{2}
\expandafter\def\csname res@v4@control_1.0@varsort@len\endcsname{2.6}
\expandafter\def\csname res@v4@control_1.0@varsort@rp\endcsname{0.17}
\expandafter\def\csname res@v4@control_1.0@varsort@map\endcsname{0.26}
\expandafter\def\csname res@v4@control_1.0@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v4@control_1.0@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v4@control_1.0@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4@control_1.0@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v4@control_1.0@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v4@control_1.0@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4@control_1.0@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v4@control_1.0@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4@control_1.0@r2sort@rp\endcsname{0.20}
\expandafter\def\csname res@v4@control_1.0@r2sort@map\endcsname{0.29}
\expandafter\def\csname res@v4h@signal_0.2@correlation@fp\endcsname{4/10}
\expandafter\def\csname res@v4h@signal_0.2@correlation@fpn\endcsname{4}
\expandafter\def\csname res@v4h@signal_0.2@correlation@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@correlation@tt\endcsname{0.50}
\expandafter\def\csname res@v4h@signal_0.2@correlation@prec\endcsname{0.16}
\expandafter\def\csname res@v4h@signal_0.2@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@correlation@bw\endcsname{6}
\expandafter\def\csname res@v4h@signal_0.2@correlation@len\endcsname{16.3}
\expandafter\def\csname res@v4h@signal_0.2@correlation@rp\endcsname{0.36}
\expandafter\def\csname res@v4h@signal_0.2@correlation@map\endcsname{0.54}
\expandafter\def\csname res@v4h@signal_0.2@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v4h@signal_0.2@granger@fpn\endcsname{9}
\expandafter\def\csname res@v4h@signal_0.2@granger@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v4h@signal_0.2@granger@prec\endcsname{0.23}
\expandafter\def\csname res@v4h@signal_0.2@granger@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@granger@bw\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@granger@len\endcsname{11.9}
\expandafter\def\csname res@v4h@signal_0.2@granger@rp\endcsname{0.68}
\expandafter\def\csname res@v4h@signal_0.2@granger@map\endcsname{0.77}
\expandafter\def\csname res@v4h@signal_0.2@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v4h@signal_0.2@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v4h@signal_0.2@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@pcmciplus@tt\endcsname{0.65}
\expandafter\def\csname res@v4h@signal_0.2@pcmciplus@prec\endcsname{0.72}
\expandafter\def\csname res@v4h@signal_0.2@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@pcmciplus@len\endcsname{2.5}
\expandafter\def\csname res@v4h@signal_0.2@pcmciplus@rp\endcsname{0.76}
\expandafter\def\csname res@v4h@signal_0.2@pcmciplus@map\endcsname{0.87}
\expandafter\def\csname res@v4h@signal_0.2@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4h@signal_0.2@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4h@signal_0.2@pc@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v4h@signal_0.2@pc@prec\endcsname{0.30}
\expandafter\def\csname res@v4h@signal_0.2@pc@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@pc@bw\endcsname{3}
\expandafter\def\csname res@v4h@signal_0.2@pc@len\endcsname{5.0}
\expandafter\def\csname res@v4h@signal_0.2@pc@rp\endcsname{0.30}
\expandafter\def\csname res@v4h@signal_0.2@pc@map\endcsname{0.27}
\expandafter\def\csname res@v4h@signal_0.2@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@signal_0.2@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v4h@signal_0.2@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v4h@signal_0.2@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v4h@signal_0.2@dynotears@rp\endcsname{0.86}
\expandafter\def\csname res@v4h@signal_0.2@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v4h@signal_0.2@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v4h@signal_0.2@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v4h@signal_0.2@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@doubleml@tt\endcsname{0.50}
\expandafter\def\csname res@v4h@signal_0.2@doubleml@prec\endcsname{0.93}
\expandafter\def\csname res@v4h@signal_0.2@doubleml@ab\endcsname{2}
\expandafter\def\csname res@v4h@signal_0.2@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@doubleml@len\endcsname{1.6}
\expandafter\def\csname res@v4h@signal_0.2@doubleml@rp\endcsname{0.62}
\expandafter\def\csname res@v4h@signal_0.2@doubleml@map\endcsname{0.78}
\expandafter\def\csname res@v4h@signal_0.2@varlingam@fp\endcsname{6/10}
\expandafter\def\csname res@v4h@signal_0.2@varlingam@fpn\endcsname{6}
\expandafter\def\csname res@v4h@signal_0.2@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@varlingam@tt\endcsname{0.46}
\expandafter\def\csname res@v4h@signal_0.2@varlingam@prec\endcsname{0.27}
\expandafter\def\csname res@v4h@signal_0.2@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@varlingam@bw\endcsname{4}
\expandafter\def\csname res@v4h@signal_0.2@varlingam@len\endcsname{6.8}
\expandafter\def\csname res@v4h@signal_0.2@varlingam@rp\endcsname{0.38}
\expandafter\def\csname res@v4h@signal_0.2@varlingam@map\endcsname{0.53}
\expandafter\def\csname res@v4h@signal_0.2@spacetime_rule@fp\endcsname{1/10}
\expandafter\def\csname res@v4h@signal_0.2@spacetime_rule@fpn\endcsname{1}
\expandafter\def\csname res@v4h@signal_0.2@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@spacetime_rule@tt\endcsname{0.04}
\expandafter\def\csname res@v4h@signal_0.2@spacetime_rule@prec\endcsname{0.20}
\expandafter\def\csname res@v4h@signal_0.2@spacetime_rule@ab\endcsname{5}
\expandafter\def\csname res@v4h@signal_0.2@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v4h@signal_0.2@spacetime_rule@len\endcsname{0.5}
\expandafter\def\csname res@v4h@signal_0.2@spacetime_rule@rp\endcsname{0.28}
\expandafter\def\csname res@v4h@signal_0.2@spacetime_rule@map\endcsname{0.39}
\expandafter\def\csname res@v4h@signal_0.2@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@signal_0.2@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@varsort@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4h@signal_0.2@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4h@signal_0.2@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4h@signal_0.2@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v4h@signal_0.2@varsort@rp\endcsname{0.21}
\expandafter\def\csname res@v4h@signal_0.2@varsort@map\endcsname{0.21}
\expandafter\def\csname res@v4h@signal_0.2@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@signal_0.2@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.2@r2sort@tt\endcsname{0.19}
\expandafter\def\csname res@v4h@signal_0.2@r2sort@prec\endcsname{0.17}
\expandafter\def\csname res@v4h@signal_0.2@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.2@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v4h@signal_0.2@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4h@signal_0.2@r2sort@rp\endcsname{0.14}
\expandafter\def\csname res@v4h@signal_0.2@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v4h@signal_0.1@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@signal_0.1@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@correlation@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@correlation@tt\endcsname{0.35}
\expandafter\def\csname res@v4h@signal_0.1@correlation@prec\endcsname{0.18}
\expandafter\def\csname res@v4h@signal_0.1@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@correlation@bw\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@correlation@len\endcsname{13.1}
\expandafter\def\csname res@v4h@signal_0.1@correlation@rp\endcsname{0.17}
\expandafter\def\csname res@v4h@signal_0.1@correlation@map\endcsname{0.40}
\expandafter\def\csname res@v4h@signal_0.1@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v4h@signal_0.1@granger@fpn\endcsname{8}
\expandafter\def\csname res@v4h@signal_0.1@granger@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v4h@signal_0.1@granger@prec\endcsname{0.28}
\expandafter\def\csname res@v4h@signal_0.1@granger@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@granger@bw\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@granger@len\endcsname{7.8}
\expandafter\def\csname res@v4h@signal_0.1@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v4h@signal_0.1@granger@map\endcsname{0.74}
\expandafter\def\csname res@v4h@signal_0.1@pcmciplus@fp\endcsname{8/10}
\expandafter\def\csname res@v4h@signal_0.1@pcmciplus@fpn\endcsname{8}
\expandafter\def\csname res@v4h@signal_0.1@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@pcmciplus@tt\endcsname{0.46}
\expandafter\def\csname res@v4h@signal_0.1@pcmciplus@prec\endcsname{0.65}
\expandafter\def\csname res@v4h@signal_0.1@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@pcmciplus@len\endcsname{1.8}
\expandafter\def\csname res@v4h@signal_0.1@pcmciplus@rp\endcsname{0.71}
\expandafter\def\csname res@v4h@signal_0.1@pcmciplus@map\endcsname{0.79}
\expandafter\def\csname res@v4h@signal_0.1@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4h@signal_0.1@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4h@signal_0.1@pc@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v4h@signal_0.1@pc@prec\endcsname{0.32}
\expandafter\def\csname res@v4h@signal_0.1@pc@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@pc@bw\endcsname{4}
\expandafter\def\csname res@v4h@signal_0.1@pc@len\endcsname{4.4}
\expandafter\def\csname res@v4h@signal_0.1@pc@rp\endcsname{0.31}
\expandafter\def\csname res@v4h@signal_0.1@pc@map\endcsname{0.29}
\expandafter\def\csname res@v4h@signal_0.1@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@signal_0.1@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v4h@signal_0.1@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v4h@signal_0.1@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v4h@signal_0.1@dynotears@rp\endcsname{0.71}
\expandafter\def\csname res@v4h@signal_0.1@dynotears@map\endcsname{0.86}
\expandafter\def\csname res@v4h@signal_0.1@doubleml@fp\endcsname{5/10}
\expandafter\def\csname res@v4h@signal_0.1@doubleml@fpn\endcsname{5}
\expandafter\def\csname res@v4h@signal_0.1@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@doubleml@tt\endcsname{0.38}
\expandafter\def\csname res@v4h@signal_0.1@doubleml@prec\endcsname{1.00}
\expandafter\def\csname res@v4h@signal_0.1@doubleml@ab\endcsname{5}
\expandafter\def\csname res@v4h@signal_0.1@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@doubleml@len\endcsname{1.0}
\expandafter\def\csname res@v4h@signal_0.1@doubleml@rp\endcsname{0.57}
\expandafter\def\csname res@v4h@signal_0.1@doubleml@map\endcsname{0.69}
\expandafter\def\csname res@v4h@signal_0.1@varlingam@fp\endcsname{4/10}
\expandafter\def\csname res@v4h@signal_0.1@varlingam@fpn\endcsname{4}
\expandafter\def\csname res@v4h@signal_0.1@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@varlingam@tt\endcsname{0.42}
\expandafter\def\csname res@v4h@signal_0.1@varlingam@prec\endcsname{0.40}
\expandafter\def\csname res@v4h@signal_0.1@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@varlingam@bw\endcsname{6}
\expandafter\def\csname res@v4h@signal_0.1@varlingam@len\endcsname{5.2}
\expandafter\def\csname res@v4h@signal_0.1@varlingam@rp\endcsname{0.36}
\expandafter\def\csname res@v4h@signal_0.1@varlingam@map\endcsname{0.44}
\expandafter\def\csname res@v4h@signal_0.1@spacetime_rule@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@signal_0.1@spacetime_rule@fpn\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@spacetime_rule@tt\endcsname{0.00}
\expandafter\def\csname res@v4h@signal_0.1@spacetime_rule@prec\endcsname{0.00}
\expandafter\def\csname res@v4h@signal_0.1@spacetime_rule@ab\endcsname{6}
\expandafter\def\csname res@v4h@signal_0.1@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v4h@signal_0.1@spacetime_rule@len\endcsname{0.4}
\expandafter\def\csname res@v4h@signal_0.1@spacetime_rule@rp\endcsname{0.15}
\expandafter\def\csname res@v4h@signal_0.1@spacetime_rule@map\endcsname{0.29}
\expandafter\def\csname res@v4h@signal_0.1@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@signal_0.1@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@varsort@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4h@signal_0.1@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4h@signal_0.1@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4h@signal_0.1@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v4h@signal_0.1@varsort@rp\endcsname{0.21}
\expandafter\def\csname res@v4h@signal_0.1@varsort@map\endcsname{0.21}
\expandafter\def\csname res@v4h@signal_0.1@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@signal_0.1@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4h@signal_0.1@r2sort@tt\endcsname{0.19}
\expandafter\def\csname res@v4h@signal_0.1@r2sort@prec\endcsname{0.17}
\expandafter\def\csname res@v4h@signal_0.1@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4h@signal_0.1@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v4h@signal_0.1@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4h@signal_0.1@r2sort@rp\endcsname{0.14}
\expandafter\def\csname res@v4h@signal_0.1@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v4h@echo_0.8@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v4h@echo_0.8@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v4h@echo_0.8@correlation@n\endcsname{10}
\expandafter\def\csname res@v4h@echo_0.8@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v4h@echo_0.8@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v4h@echo_0.8@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@correlation@bw\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@correlation@len\endcsname{18.7}
\expandafter\def\csname res@v4h@echo_0.8@correlation@rp\endcsname{0.61}
\expandafter\def\csname res@v4h@echo_0.8@correlation@map\endcsname{0.73}
\expandafter\def\csname res@v4h@echo_0.8@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v4h@echo_0.8@granger@fpn\endcsname{9}
\expandafter\def\csname res@v4h@echo_0.8@granger@n\endcsname{10}
\expandafter\def\csname res@v4h@echo_0.8@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v4h@echo_0.8@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v4h@echo_0.8@granger@ab\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@granger@bw\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@granger@len\endcsname{17.6}
\expandafter\def\csname res@v4h@echo_0.8@granger@rp\endcsname{0.58}
\expandafter\def\csname res@v4h@echo_0.8@granger@map\endcsname{0.72}
\expandafter\def\csname res@v4h@echo_0.8@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v4h@echo_0.8@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v4h@echo_0.8@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4h@echo_0.8@pcmciplus@tt\endcsname{0.62}
\expandafter\def\csname res@v4h@echo_0.8@pcmciplus@prec\endcsname{0.70}
\expandafter\def\csname res@v4h@echo_0.8@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v4h@echo_0.8@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@pcmciplus@len\endcsname{2.7}
\expandafter\def\csname res@v4h@echo_0.8@pcmciplus@rp\endcsname{0.90}
\expandafter\def\csname res@v4h@echo_0.8@pcmciplus@map\endcsname{0.95}
\expandafter\def\csname res@v4h@echo_0.8@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v4h@echo_0.8@pc@fpn\endcsname{3}
\expandafter\def\csname res@v4h@echo_0.8@pc@n\endcsname{10}
\expandafter\def\csname res@v4h@echo_0.8@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v4h@echo_0.8@pc@prec\endcsname{0.34}
\expandafter\def\csname res@v4h@echo_0.8@pc@ab\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@pc@bw\endcsname{3}
\expandafter\def\csname res@v4h@echo_0.8@pc@len\endcsname{5.0}
\expandafter\def\csname res@v4h@echo_0.8@pc@rp\endcsname{0.33}
\expandafter\def\csname res@v4h@echo_0.8@pc@map\endcsname{0.30}
\expandafter\def\csname res@v4h@echo_0.8@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v4h@echo_0.8@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v4h@echo_0.8@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4h@echo_0.8@dynotears@tt\endcsname{0.19}
\expandafter\def\csname res@v4h@echo_0.8@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4h@echo_0.8@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v4h@echo_0.8@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@dynotears@len\endcsname{0.5}
\expandafter\def\csname res@v4h@echo_0.8@dynotears@rp\endcsname{0.85}
\expandafter\def\csname res@v4h@echo_0.8@dynotears@map\endcsname{0.89}
\expandafter\def\csname res@v4h@echo_0.8@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v4h@echo_0.8@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v4h@echo_0.8@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4h@echo_0.8@doubleml@tt\endcsname{0.65}
\expandafter\def\csname res@v4h@echo_0.8@doubleml@prec\endcsname{0.60}
\expandafter\def\csname res@v4h@echo_0.8@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v4h@echo_0.8@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@doubleml@len\endcsname{3.5}
\expandafter\def\csname res@v4h@echo_0.8@doubleml@rp\endcsname{0.65}
\expandafter\def\csname res@v4h@echo_0.8@doubleml@map\endcsname{0.81}
\expandafter\def\csname res@v4h@echo_0.8@varlingam@fp\endcsname{5/10}
\expandafter\def\csname res@v4h@echo_0.8@varlingam@fpn\endcsname{5}
\expandafter\def\csname res@v4h@echo_0.8@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4h@echo_0.8@varlingam@tt\endcsname{0.50}
\expandafter\def\csname res@v4h@echo_0.8@varlingam@prec\endcsname{0.22}
\expandafter\def\csname res@v4h@echo_0.8@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v4h@echo_0.8@varlingam@len\endcsname{11.1}
\expandafter\def\csname res@v4h@echo_0.8@varlingam@rp\endcsname{0.53}
\expandafter\def\csname res@v4h@echo_0.8@varlingam@map\endcsname{0.54}
\expandafter\def\csname res@v4h@echo_0.8@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v4h@echo_0.8@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v4h@echo_0.8@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4h@echo_0.8@spacetime_rule@tt\endcsname{0.35}
\expandafter\def\csname res@v4h@echo_0.8@spacetime_rule@prec\endcsname{0.72}
\expandafter\def\csname res@v4h@echo_0.8@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v4h@echo_0.8@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v4h@echo_0.8@spacetime_rule@rp\endcsname{0.57}
\expandafter\def\csname res@v4h@echo_0.8@spacetime_rule@map\endcsname{0.68}
\expandafter\def\csname res@v4h@echo_0.8@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v4h@echo_0.8@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v4h@echo_0.8@varsort@n\endcsname{10}
\expandafter\def\csname res@v4h@echo_0.8@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v4h@echo_0.8@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v4h@echo_0.8@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@varsort@bw\endcsname{2}
\expandafter\def\csname res@v4h@echo_0.8@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v4h@echo_0.8@varsort@rp\endcsname{0.13}
\expandafter\def\csname res@v4h@echo_0.8@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v4h@echo_0.8@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@echo_0.8@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4h@echo_0.8@r2sort@tt\endcsname{0.08}
\expandafter\def\csname res@v4h@echo_0.8@r2sort@prec\endcsname{0.07}
\expandafter\def\csname res@v4h@echo_0.8@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4h@echo_0.8@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v4h@echo_0.8@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4h@echo_0.8@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v4h@echo_0.8@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v4h@confound_0.8@correlation@fp\endcsname{7/10}
\expandafter\def\csname res@v4h@confound_0.8@correlation@fpn\endcsname{7}
\expandafter\def\csname res@v4h@confound_0.8@correlation@n\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@correlation@tt\endcsname{0.42}
\expandafter\def\csname res@v4h@confound_0.8@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v4h@confound_0.8@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@correlation@bw\endcsname{2}
\expandafter\def\csname res@v4h@confound_0.8@correlation@len\endcsname{17.5}
\expandafter\def\csname res@v4h@confound_0.8@correlation@rp\endcsname{0.47}
\expandafter\def\csname res@v4h@confound_0.8@correlation@map\endcsname{0.57}
\expandafter\def\csname res@v4h@confound_0.8@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v4h@confound_0.8@granger@fpn\endcsname{9}
\expandafter\def\csname res@v4h@confound_0.8@granger@n\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@granger@tt\endcsname{0.42}
\expandafter\def\csname res@v4h@confound_0.8@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v4h@confound_0.8@granger@ab\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@granger@bw\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@granger@len\endcsname{16.0}
\expandafter\def\csname res@v4h@confound_0.8@granger@rp\endcsname{0.55}
\expandafter\def\csname res@v4h@confound_0.8@granger@map\endcsname{0.67}
\expandafter\def\csname res@v4h@confound_0.8@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4h@confound_0.8@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@pcmciplus@tt\endcsname{0.58}
\expandafter\def\csname res@v4h@confound_0.8@pcmciplus@prec\endcsname{0.81}
\expandafter\def\csname res@v4h@confound_0.8@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@pcmciplus@len\endcsname{2.1}
\expandafter\def\csname res@v4h@confound_0.8@pcmciplus@rp\endcsname{0.84}
\expandafter\def\csname res@v4h@confound_0.8@pcmciplus@map\endcsname{0.92}
\expandafter\def\csname res@v4h@confound_0.8@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v4h@confound_0.8@pc@fpn\endcsname{4}
\expandafter\def\csname res@v4h@confound_0.8@pc@n\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v4h@confound_0.8@pc@prec\endcsname{0.39}
\expandafter\def\csname res@v4h@confound_0.8@pc@ab\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@pc@bw\endcsname{3}
\expandafter\def\csname res@v4h@confound_0.8@pc@len\endcsname{4.8}
\expandafter\def\csname res@v4h@confound_0.8@pc@rp\endcsname{0.39}
\expandafter\def\csname res@v4h@confound_0.8@pc@map\endcsname{0.32}
\expandafter\def\csname res@v4h@confound_0.8@dynotears@fp\endcsname{3/10}
\expandafter\def\csname res@v4h@confound_0.8@dynotears@fpn\endcsname{3}
\expandafter\def\csname res@v4h@confound_0.8@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@dynotears@tt\endcsname{0.12}
\expandafter\def\csname res@v4h@confound_0.8@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4h@confound_0.8@dynotears@ab\endcsname{7}
\expandafter\def\csname res@v4h@confound_0.8@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@dynotears@len\endcsname{0.3}
\expandafter\def\csname res@v4h@confound_0.8@dynotears@rp\endcsname{0.78}
\expandafter\def\csname res@v4h@confound_0.8@dynotears@map\endcsname{0.90}
\expandafter\def\csname res@v4h@confound_0.8@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v4h@confound_0.8@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@doubleml@tt\endcsname{0.77}
\expandafter\def\csname res@v4h@confound_0.8@doubleml@prec\endcsname{0.69}
\expandafter\def\csname res@v4h@confound_0.8@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@doubleml@len\endcsname{3.6}
\expandafter\def\csname res@v4h@confound_0.8@doubleml@rp\endcsname{0.86}
\expandafter\def\csname res@v4h@confound_0.8@doubleml@map\endcsname{0.90}
\expandafter\def\csname res@v4h@confound_0.8@varlingam@fp\endcsname{5/10}
\expandafter\def\csname res@v4h@confound_0.8@varlingam@fpn\endcsname{5}
\expandafter\def\csname res@v4h@confound_0.8@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@varlingam@tt\endcsname{0.38}
\expandafter\def\csname res@v4h@confound_0.8@varlingam@prec\endcsname{0.19}
\expandafter\def\csname res@v4h@confound_0.8@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v4h@confound_0.8@varlingam@len\endcsname{11.1}
\expandafter\def\csname res@v4h@confound_0.8@varlingam@rp\endcsname{0.43}
\expandafter\def\csname res@v4h@confound_0.8@varlingam@map\endcsname{0.54}
\expandafter\def\csname res@v4h@confound_0.8@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v4h@confound_0.8@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v4h@confound_0.8@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@spacetime_rule@tt\endcsname{0.38}
\expandafter\def\csname res@v4h@confound_0.8@spacetime_rule@prec\endcsname{0.62}
\expandafter\def\csname res@v4h@confound_0.8@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v4h@confound_0.8@spacetime_rule@rp\endcsname{0.46}
\expandafter\def\csname res@v4h@confound_0.8@spacetime_rule@map\endcsname{0.59}
\expandafter\def\csname res@v4h@confound_0.8@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@confound_0.8@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@varsort@n\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v4h@confound_0.8@varsort@prec\endcsname{0.22}
\expandafter\def\csname res@v4h@confound_0.8@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4h@confound_0.8@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v4h@confound_0.8@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v4h@confound_0.8@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v4h@confound_0.8@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@confound_0.8@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4h@confound_0.8@r2sort@tt\endcsname{0.08}
\expandafter\def\csname res@v4h@confound_0.8@r2sort@prec\endcsname{0.08}
\expandafter\def\csname res@v4h@confound_0.8@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4h@confound_0.8@r2sort@bw\endcsname{3}
\expandafter\def\csname res@v4h@confound_0.8@r2sort@len\endcsname{2.8}
\expandafter\def\csname res@v4h@confound_0.8@r2sort@rp\endcsname{0.08}
\expandafter\def\csname res@v4h@confound_0.8@r2sort@map\endcsname{0.17}
\expandafter\def\csname res@v4h@causes_4to6@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v4h@causes_4to6@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v4h@causes_4to6@correlation@n\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@correlation@tt\endcsname{0.39}
\expandafter\def\csname res@v4h@causes_4to6@correlation@prec\endcsname{0.29}
\expandafter\def\csname res@v4h@causes_4to6@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@correlation@bw\endcsname{2}
\expandafter\def\csname res@v4h@causes_4to6@correlation@len\endcsname{17.2}
\expandafter\def\csname res@v4h@causes_4to6@correlation@rp\endcsname{0.52}
\expandafter\def\csname res@v4h@causes_4to6@correlation@map\endcsname{0.61}
\expandafter\def\csname res@v4h@causes_4to6@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v4h@causes_4to6@granger@fpn\endcsname{9}
\expandafter\def\csname res@v4h@causes_4to6@granger@n\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@granger@tt\endcsname{0.35}
\expandafter\def\csname res@v4h@causes_4to6@granger@prec\endcsname{0.28}
\expandafter\def\csname res@v4h@causes_4to6@granger@ab\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@granger@bw\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@granger@len\endcsname{16.6}
\expandafter\def\csname res@v4h@causes_4to6@granger@rp\endcsname{0.53}
\expandafter\def\csname res@v4h@causes_4to6@granger@map\endcsname{0.63}
\expandafter\def\csname res@v4h@causes_4to6@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v4h@causes_4to6@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@pcmciplus@tt\endcsname{0.51}
\expandafter\def\csname res@v4h@causes_4to6@pcmciplus@prec\endcsname{0.86}
\expandafter\def\csname res@v4h@causes_4to6@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@pcmciplus@len\endcsname{4.0}
\expandafter\def\csname res@v4h@causes_4to6@pcmciplus@rp\endcsname{0.71}
\expandafter\def\csname res@v4h@causes_4to6@pcmciplus@map\endcsname{0.83}
\expandafter\def\csname res@v4h@causes_4to6@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v4h@causes_4to6@pc@fpn\endcsname{4}
\expandafter\def\csname res@v4h@causes_4to6@pc@n\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@pc@tt\endcsname{0.24}
\expandafter\def\csname res@v4h@causes_4to6@pc@prec\endcsname{0.46}
\expandafter\def\csname res@v4h@causes_4to6@pc@ab\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@pc@bw\endcsname{4}
\expandafter\def\csname res@v4h@causes_4to6@pc@len\endcsname{6.0}
\expandafter\def\csname res@v4h@causes_4to6@pc@rp\endcsname{0.39}
\expandafter\def\csname res@v4h@causes_4to6@pc@map\endcsname{0.38}
\expandafter\def\csname res@v4h@causes_4to6@dynotears@fp\endcsname{2/10}
\expandafter\def\csname res@v4h@causes_4to6@dynotears@fpn\endcsname{2}
\expandafter\def\csname res@v4h@causes_4to6@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v4h@causes_4to6@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v4h@causes_4to6@dynotears@ab\endcsname{8}
\expandafter\def\csname res@v4h@causes_4to6@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@dynotears@len\endcsname{0.2}
\expandafter\def\csname res@v4h@causes_4to6@dynotears@rp\endcsname{0.63}
\expandafter\def\csname res@v4h@causes_4to6@dynotears@map\endcsname{0.79}
\expandafter\def\csname res@v4h@causes_4to6@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v4h@causes_4to6@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@doubleml@tt\endcsname{0.53}
\expandafter\def\csname res@v4h@causes_4to6@doubleml@prec\endcsname{0.82}
\expandafter\def\csname res@v4h@causes_4to6@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@doubleml@len\endcsname{4.3}
\expandafter\def\csname res@v4h@causes_4to6@doubleml@rp\endcsname{0.70}
\expandafter\def\csname res@v4h@causes_4to6@doubleml@map\endcsname{0.82}
\expandafter\def\csname res@v4h@causes_4to6@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v4h@causes_4to6@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v4h@causes_4to6@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@varlingam@tt\endcsname{0.43}
\expandafter\def\csname res@v4h@causes_4to6@varlingam@prec\endcsname{0.42}
\expandafter\def\csname res@v4h@causes_4to6@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v4h@causes_4to6@varlingam@len\endcsname{11.1}
\expandafter\def\csname res@v4h@causes_4to6@varlingam@rp\endcsname{0.63}
\expandafter\def\csname res@v4h@causes_4to6@varlingam@map\endcsname{0.74}
\expandafter\def\csname res@v4h@causes_4to6@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v4h@causes_4to6@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v4h@causes_4to6@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@spacetime_rule@tt\endcsname{0.20}
\expandafter\def\csname res@v4h@causes_4to6@spacetime_rule@prec\endcsname{0.90}
\expandafter\def\csname res@v4h@causes_4to6@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v4h@causes_4to6@spacetime_rule@rp\endcsname{0.54}
\expandafter\def\csname res@v4h@causes_4to6@spacetime_rule@map\endcsname{0.61}
\expandafter\def\csname res@v4h@causes_4to6@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v4h@causes_4to6@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v4h@causes_4to6@varsort@n\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@varsort@tt\endcsname{0.22}
\expandafter\def\csname res@v4h@causes_4to6@varsort@prec\endcsname{0.37}
\expandafter\def\csname res@v4h@causes_4to6@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4h@causes_4to6@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v4h@causes_4to6@varsort@rp\endcsname{0.28}
\expandafter\def\csname res@v4h@causes_4to6@varsort@map\endcsname{0.32}
\expandafter\def\csname res@v4h@causes_4to6@r2sort@fp\endcsname{4/10}
\expandafter\def\csname res@v4h@causes_4to6@r2sort@fpn\endcsname{4}
\expandafter\def\csname res@v4h@causes_4to6@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4h@causes_4to6@r2sort@tt\endcsname{0.16}
\expandafter\def\csname res@v4h@causes_4to6@r2sort@prec\endcsname{0.27}
\expandafter\def\csname res@v4h@causes_4to6@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4h@causes_4to6@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v4h@causes_4to6@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v4h@causes_4to6@r2sort@rp\endcsname{0.30}
\expandafter\def\csname res@v4h@causes_4to6@r2sort@map\endcsname{0.38}
\expandafter\def\csname res@v4h@combo_hard@correlation@fp\endcsname{4/10}
\expandafter\def\csname res@v4h@combo_hard@correlation@fpn\endcsname{4}
\expandafter\def\csname res@v4h@combo_hard@correlation@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@correlation@tt\endcsname{0.42}
\expandafter\def\csname res@v4h@combo_hard@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v4h@combo_hard@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@correlation@bw\endcsname{5}
\expandafter\def\csname res@v4h@combo_hard@correlation@len\endcsname{17.0}
\expandafter\def\csname res@v4h@combo_hard@correlation@rp\endcsname{0.35}
\expandafter\def\csname res@v4h@combo_hard@correlation@map\endcsname{0.50}
\expandafter\def\csname res@v4h@combo_hard@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v4h@combo_hard@granger@fpn\endcsname{8}
\expandafter\def\csname res@v4h@combo_hard@granger@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v4h@combo_hard@granger@prec\endcsname{0.16}
\expandafter\def\csname res@v4h@combo_hard@granger@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@granger@bw\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@granger@len\endcsname{14.9}
\expandafter\def\csname res@v4h@combo_hard@granger@rp\endcsname{0.58}
\expandafter\def\csname res@v4h@combo_hard@granger@map\endcsname{0.71}
\expandafter\def\csname res@v4h@combo_hard@pcmciplus@fp\endcsname{7/10}
\expandafter\def\csname res@v4h@combo_hard@pcmciplus@fpn\endcsname{7}
\expandafter\def\csname res@v4h@combo_hard@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v4h@combo_hard@pcmciplus@prec\endcsname{0.73}
\expandafter\def\csname res@v4h@combo_hard@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v4h@combo_hard@pcmciplus@len\endcsname{2.7}
\expandafter\def\csname res@v4h@combo_hard@pcmciplus@rp\endcsname{0.69}
\expandafter\def\csname res@v4h@combo_hard@pcmciplus@map\endcsname{0.78}
\expandafter\def\csname res@v4h@combo_hard@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v4h@combo_hard@pc@fpn\endcsname{2}
\expandafter\def\csname res@v4h@combo_hard@pc@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v4h@combo_hard@pc@prec\endcsname{0.32}
\expandafter\def\csname res@v4h@combo_hard@pc@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@pc@bw\endcsname{3}
\expandafter\def\csname res@v4h@combo_hard@pc@len\endcsname{4.2}
\expandafter\def\csname res@v4h@combo_hard@pc@rp\endcsname{0.31}
\expandafter\def\csname res@v4h@combo_hard@pc@map\endcsname{0.27}
\expandafter\def\csname res@v4h@combo_hard@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@combo_hard@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v4h@combo_hard@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v4h@combo_hard@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v4h@combo_hard@dynotears@rp\endcsname{0.82}
\expandafter\def\csname res@v4h@combo_hard@dynotears@map\endcsname{0.90}
\expandafter\def\csname res@v4h@combo_hard@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v4h@combo_hard@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v4h@combo_hard@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@doubleml@tt\endcsname{0.46}
\expandafter\def\csname res@v4h@combo_hard@doubleml@prec\endcsname{0.84}
\expandafter\def\csname res@v4h@combo_hard@doubleml@ab\endcsname{2}
\expandafter\def\csname res@v4h@combo_hard@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@doubleml@len\endcsname{1.8}
\expandafter\def\csname res@v4h@combo_hard@doubleml@rp\endcsname{0.59}
\expandafter\def\csname res@v4h@combo_hard@doubleml@map\endcsname{0.75}
\expandafter\def\csname res@v4h@combo_hard@varlingam@fp\endcsname{3/10}
\expandafter\def\csname res@v4h@combo_hard@varlingam@fpn\endcsname{3}
\expandafter\def\csname res@v4h@combo_hard@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@varlingam@tt\endcsname{0.38}
\expandafter\def\csname res@v4h@combo_hard@varlingam@prec\endcsname{0.21}
\expandafter\def\csname res@v4h@combo_hard@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@varlingam@bw\endcsname{7}
\expandafter\def\csname res@v4h@combo_hard@varlingam@len\endcsname{9.5}
\expandafter\def\csname res@v4h@combo_hard@varlingam@rp\endcsname{0.33}
\expandafter\def\csname res@v4h@combo_hard@varlingam@map\endcsname{0.41}
\expandafter\def\csname res@v4h@combo_hard@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v4h@combo_hard@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v4h@combo_hard@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@spacetime_rule@tt\endcsname{0.23}
\expandafter\def\csname res@v4h@combo_hard@spacetime_rule@prec\endcsname{0.60}
\expandafter\def\csname res@v4h@combo_hard@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v4h@combo_hard@spacetime_rule@rp\endcsname{0.45}
\expandafter\def\csname res@v4h@combo_hard@spacetime_rule@map\endcsname{0.57}
\expandafter\def\csname res@v4h@combo_hard@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v4h@combo_hard@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v4h@combo_hard@varsort@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v4h@combo_hard@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v4h@combo_hard@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@varsort@bw\endcsname{2}
\expandafter\def\csname res@v4h@combo_hard@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v4h@combo_hard@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v4h@combo_hard@varsort@map\endcsname{0.20}
\expandafter\def\csname res@v4h@combo_hard@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v4h@combo_hard@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v4h@combo_hard@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_hard@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v4h@combo_hard@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v4h@combo_hard@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_hard@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v4h@combo_hard@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v4h@combo_hard@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v4h@combo_hard@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v4h@combo_extreme@correlation@fp\endcsname{2/10}
\expandafter\def\csname res@v4h@combo_extreme@correlation@fpn\endcsname{2}
\expandafter\def\csname res@v4h@combo_extreme@correlation@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@correlation@tt\endcsname{0.31}
\expandafter\def\csname res@v4h@combo_extreme@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v4h@combo_extreme@correlation@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@correlation@bw\endcsname{8}
\expandafter\def\csname res@v4h@combo_extreme@correlation@len\endcsname{16.4}
\expandafter\def\csname res@v4h@combo_extreme@correlation@rp\endcsname{0.18}
\expandafter\def\csname res@v4h@combo_extreme@correlation@map\endcsname{0.39}
\expandafter\def\csname res@v4h@combo_extreme@granger@fp\endcsname{6/10}
\expandafter\def\csname res@v4h@combo_extreme@granger@fpn\endcsname{6}
\expandafter\def\csname res@v4h@combo_extreme@granger@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v4h@combo_extreme@granger@prec\endcsname{0.18}
\expandafter\def\csname res@v4h@combo_extreme@granger@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@granger@bw\endcsname{1}
\expandafter\def\csname res@v4h@combo_extreme@granger@len\endcsname{13.4}
\expandafter\def\csname res@v4h@combo_extreme@granger@rp\endcsname{0.56}
\expandafter\def\csname res@v4h@combo_extreme@granger@map\endcsname{0.64}
\expandafter\def\csname res@v4h@combo_extreme@pcmciplus@fp\endcsname{5/10}
\expandafter\def\csname res@v4h@combo_extreme@pcmciplus@fpn\endcsname{5}
\expandafter\def\csname res@v4h@combo_extreme@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@pcmciplus@tt\endcsname{0.27}
\expandafter\def\csname res@v4h@combo_extreme@pcmciplus@prec\endcsname{0.55}
\expandafter\def\csname res@v4h@combo_extreme@pcmciplus@ab\endcsname{3}
\expandafter\def\csname res@v4h@combo_extreme@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@pcmciplus@len\endcsname{1.2}
\expandafter\def\csname res@v4h@combo_extreme@pcmciplus@rp\endcsname{0.53}
\expandafter\def\csname res@v4h@combo_extreme@pcmciplus@map\endcsname{0.66}
\expandafter\def\csname res@v4h@combo_extreme@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v4h@combo_extreme@pc@fpn\endcsname{1}
\expandafter\def\csname res@v4h@combo_extreme@pc@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@pc@tt\endcsname{0.23}
\expandafter\def\csname res@v4h@combo_extreme@pc@prec\endcsname{0.27}
\expandafter\def\csname res@v4h@combo_extreme@pc@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@pc@bw\endcsname{7}
\expandafter\def\csname res@v4h@combo_extreme@pc@len\endcsname{2.9}
\expandafter\def\csname res@v4h@combo_extreme@pc@rp\endcsname{0.24}
\expandafter\def\csname res@v4h@combo_extreme@pc@map\endcsname{0.21}
\expandafter\def\csname res@v4h@combo_extreme@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v4h@combo_extreme@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@dynotears@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v4h@combo_extreme@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v4h@combo_extreme@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v4h@combo_extreme@dynotears@rp\endcsname{0.56}
\expandafter\def\csname res@v4h@combo_extreme@dynotears@map\endcsname{0.67}
\expandafter\def\csname res@v4h@combo_extreme@doubleml@fp\endcsname{3/10}
\expandafter\def\csname res@v4h@combo_extreme@doubleml@fpn\endcsname{3}
\expandafter\def\csname res@v4h@combo_extreme@doubleml@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@doubleml@tt\endcsname{0.15}
\expandafter\def\csname res@v4h@combo_extreme@doubleml@prec\endcsname{0.62}
\expandafter\def\csname res@v4h@combo_extreme@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v4h@combo_extreme@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@doubleml@len\endcsname{0.6}
\expandafter\def\csname res@v4h@combo_extreme@doubleml@rp\endcsname{0.48}
\expandafter\def\csname res@v4h@combo_extreme@doubleml@map\endcsname{0.57}
\expandafter\def\csname res@v4h@combo_extreme@varlingam@fp\endcsname{3/10}
\expandafter\def\csname res@v4h@combo_extreme@varlingam@fpn\endcsname{3}
\expandafter\def\csname res@v4h@combo_extreme@varlingam@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@varlingam@tt\endcsname{0.27}
\expandafter\def\csname res@v4h@combo_extreme@varlingam@prec\endcsname{0.24}
\expandafter\def\csname res@v4h@combo_extreme@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@varlingam@bw\endcsname{7}
\expandafter\def\csname res@v4h@combo_extreme@varlingam@len\endcsname{8.2}
\expandafter\def\csname res@v4h@combo_extreme@varlingam@rp\endcsname{0.19}
\expandafter\def\csname res@v4h@combo_extreme@varlingam@map\endcsname{0.36}
\expandafter\def\csname res@v4h@combo_extreme@spacetime_rule@fp\endcsname{2/10}
\expandafter\def\csname res@v4h@combo_extreme@spacetime_rule@fpn\endcsname{2}
\expandafter\def\csname res@v4h@combo_extreme@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@spacetime_rule@tt\endcsname{0.15}
\expandafter\def\csname res@v4h@combo_extreme@spacetime_rule@prec\endcsname{0.24}
\expandafter\def\csname res@v4h@combo_extreme@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v4h@combo_extreme@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v4h@combo_extreme@spacetime_rule@rp\endcsname{0.19}
\expandafter\def\csname res@v4h@combo_extreme@spacetime_rule@map\endcsname{0.35}
\expandafter\def\csname res@v4h@combo_extreme@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v4h@combo_extreme@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v4h@combo_extreme@varsort@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v4h@combo_extreme@varsort@prec\endcsname{0.20}
\expandafter\def\csname res@v4h@combo_extreme@varsort@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@varsort@bw\endcsname{1}
\expandafter\def\csname res@v4h@combo_extreme@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v4h@combo_extreme@varsort@rp\endcsname{0.11}
\expandafter\def\csname res@v4h@combo_extreme@varsort@map\endcsname{0.17}
\expandafter\def\csname res@v4h@combo_extreme@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v4h@combo_extreme@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v4h@combo_extreme@r2sort@n\endcsname{10}
\expandafter\def\csname res@v4h@combo_extreme@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v4h@combo_extreme@r2sort@prec\endcsname{0.15}
\expandafter\def\csname res@v4h@combo_extreme@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v4h@combo_extreme@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v4h@combo_extreme@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v4h@combo_extreme@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v4h@combo_extreme@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v5a@interaction_0.0@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v5a@interaction_0.0@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@correlation@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@correlation@tt\endcsname{0.62}
\expandafter\def\csname res@v5a@interaction_0.0@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v5a@interaction_0.0@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@correlation@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@correlation@len\endcsname{18.2}
\expandafter\def\csname res@v5a@interaction_0.0@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v5a@interaction_0.0@correlation@map\endcsname{0.79}
\expandafter\def\csname res@v5a@interaction_0.0@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v5a@interaction_0.0@granger@fpn\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@granger@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v5a@interaction_0.0@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v5a@interaction_0.0@granger@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@granger@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@granger@len\endcsname{17.1}
\expandafter\def\csname res@v5a@interaction_0.0@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v5a@interaction_0.0@granger@map\endcsname{0.78}
\expandafter\def\csname res@v5a@interaction_0.0@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v5a@interaction_0.0@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v5a@interaction_0.0@pcmciplus@prec\endcsname{0.79}
\expandafter\def\csname res@v5a@interaction_0.0@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@pcmciplus@len\endcsname{2.7}
\expandafter\def\csname res@v5a@interaction_0.0@pcmciplus@rp\endcsname{0.89}
\expandafter\def\csname res@v5a@interaction_0.0@pcmciplus@map\endcsname{0.96}
\expandafter\def\csname res@v5a@interaction_0.0@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v5a@interaction_0.0@pc@fpn\endcsname{3}
\expandafter\def\csname res@v5a@interaction_0.0@pc@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v5a@interaction_0.0@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v5a@interaction_0.0@pc@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@pc@bw\endcsname{3}
\expandafter\def\csname res@v5a@interaction_0.0@pc@len\endcsname{5.4}
\expandafter\def\csname res@v5a@interaction_0.0@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v5a@interaction_0.0@pc@map\endcsname{0.31}
\expandafter\def\csname res@v5a@interaction_0.0@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v5a@interaction_0.0@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v5a@interaction_0.0@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@dynotears@tt\endcsname{0.27}
\expandafter\def\csname res@v5a@interaction_0.0@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5a@interaction_0.0@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v5a@interaction_0.0@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v5a@interaction_0.0@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v5a@interaction_0.0@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v5a@interaction_0.0@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v5a@interaction_0.0@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v5a@interaction_0.0@doubleml@prec\endcsname{0.70}
\expandafter\def\csname res@v5a@interaction_0.0@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@doubleml@len\endcsname{3.9}
\expandafter\def\csname res@v5a@interaction_0.0@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v5a@interaction_0.0@doubleml@map\endcsname{0.94}
\expandafter\def\csname res@v5a@interaction_0.0@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v5a@interaction_0.0@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v5a@interaction_0.0@varlingam@prec\endcsname{0.33}
\expandafter\def\csname res@v5a@interaction_0.0@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@varlingam@len\endcsname{9.7}
\expandafter\def\csname res@v5a@interaction_0.0@varlingam@rp\endcsname{0.73}
\expandafter\def\csname res@v5a@interaction_0.0@varlingam@map\endcsname{0.84}
\expandafter\def\csname res@v5a@interaction_0.0@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v5a@interaction_0.0@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v5a@interaction_0.0@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v5a@interaction_0.0@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v5a@interaction_0.0@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v5a@interaction_0.0@spacetime_rule@rp\endcsname{0.59}
\expandafter\def\csname res@v5a@interaction_0.0@spacetime_rule@map\endcsname{0.77}
\expandafter\def\csname res@v5a@interaction_0.0@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@interaction_0.0@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.0@varsort@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@interaction_0.0@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@interaction_0.0@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.0@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5a@interaction_0.0@varsort@rp\endcsname{nan}
\expandafter\def\csname res@v5a@interaction_0.0@varsort@map\endcsname{nan}
\expandafter\def\csname res@v5a@interaction_0.0@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@interaction_0.0@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.0@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5a@interaction_0.0@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5a@interaction_0.0@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.0@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.0@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5a@interaction_0.0@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5a@interaction_0.0@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5a@interaction_0.25@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v5a@interaction_0.25@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@correlation@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v5a@interaction_0.25@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v5a@interaction_0.25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@correlation@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@correlation@len\endcsname{17.9}
\expandafter\def\csname res@v5a@interaction_0.25@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v5a@interaction_0.25@correlation@map\endcsname{0.79}
\expandafter\def\csname res@v5a@interaction_0.25@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v5a@interaction_0.25@granger@fpn\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@granger@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v5a@interaction_0.25@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v5a@interaction_0.25@granger@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@granger@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@granger@len\endcsname{16.4}
\expandafter\def\csname res@v5a@interaction_0.25@granger@rp\endcsname{0.64}
\expandafter\def\csname res@v5a@interaction_0.25@granger@map\endcsname{0.77}
\expandafter\def\csname res@v5a@interaction_0.25@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v5a@interaction_0.25@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@pcmciplus@tt\endcsname{0.77}
\expandafter\def\csname res@v5a@interaction_0.25@pcmciplus@prec\endcsname{0.81}
\expandafter\def\csname res@v5a@interaction_0.25@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@pcmciplus@len\endcsname{2.6}
\expandafter\def\csname res@v5a@interaction_0.25@pcmciplus@rp\endcsname{0.84}
\expandafter\def\csname res@v5a@interaction_0.25@pcmciplus@map\endcsname{0.88}
\expandafter\def\csname res@v5a@interaction_0.25@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v5a@interaction_0.25@pc@fpn\endcsname{4}
\expandafter\def\csname res@v5a@interaction_0.25@pc@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v5a@interaction_0.25@pc@prec\endcsname{0.31}
\expandafter\def\csname res@v5a@interaction_0.25@pc@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@pc@bw\endcsname{4}
\expandafter\def\csname res@v5a@interaction_0.25@pc@len\endcsname{5.0}
\expandafter\def\csname res@v5a@interaction_0.25@pc@rp\endcsname{0.31}
\expandafter\def\csname res@v5a@interaction_0.25@pc@map\endcsname{0.27}
\expandafter\def\csname res@v5a@interaction_0.25@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v5a@interaction_0.25@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v5a@interaction_0.25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@dynotears@tt\endcsname{0.15}
\expandafter\def\csname res@v5a@interaction_0.25@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5a@interaction_0.25@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v5a@interaction_0.25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@dynotears@len\endcsname{0.4}
\expandafter\def\csname res@v5a@interaction_0.25@dynotears@rp\endcsname{0.79}
\expandafter\def\csname res@v5a@interaction_0.25@dynotears@map\endcsname{0.89}
\expandafter\def\csname res@v5a@interaction_0.25@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_0.25@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@doubleml@tt\endcsname{0.69}
\expandafter\def\csname res@v5a@interaction_0.25@doubleml@prec\endcsname{0.64}
\expandafter\def\csname res@v5a@interaction_0.25@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@doubleml@len\endcsname{3.2}
\expandafter\def\csname res@v5a@interaction_0.25@doubleml@rp\endcsname{0.81}
\expandafter\def\csname res@v5a@interaction_0.25@doubleml@map\endcsname{0.87}
\expandafter\def\csname res@v5a@interaction_0.25@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v5a@interaction_0.25@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v5a@interaction_0.25@varlingam@prec\endcsname{0.24}
\expandafter\def\csname res@v5a@interaction_0.25@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@varlingam@len\endcsname{11.0}
\expandafter\def\csname res@v5a@interaction_0.25@varlingam@rp\endcsname{0.68}
\expandafter\def\csname res@v5a@interaction_0.25@varlingam@map\endcsname{0.81}
\expandafter\def\csname res@v5a@interaction_0.25@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_0.25@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@spacetime_rule@tt\endcsname{0.62}
\expandafter\def\csname res@v5a@interaction_0.25@spacetime_rule@prec\endcsname{0.95}
\expandafter\def\csname res@v5a@interaction_0.25@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@spacetime_rule@len\endcsname{1.7}
\expandafter\def\csname res@v5a@interaction_0.25@spacetime_rule@rp\endcsname{0.64}
\expandafter\def\csname res@v5a@interaction_0.25@spacetime_rule@map\endcsname{0.79}
\expandafter\def\csname res@v5a@interaction_0.25@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@interaction_0.25@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.25@varsort@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@interaction_0.25@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@interaction_0.25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.25@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5a@interaction_0.25@varsort@rp\endcsname{nan}
\expandafter\def\csname res@v5a@interaction_0.25@varsort@map\endcsname{nan}
\expandafter\def\csname res@v5a@interaction_0.25@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@interaction_0.25@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.25@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5a@interaction_0.25@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5a@interaction_0.25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.25@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5a@interaction_0.25@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5a@interaction_0.25@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5a@interaction_0.5@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_0.5@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.5@correlation@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.5@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v5a@interaction_0.5@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v5a@interaction_0.5@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@correlation@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.5@correlation@len\endcsname{17.3}
\expandafter\def\csname res@v5a@interaction_0.5@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v5a@interaction_0.5@correlation@map\endcsname{0.75}
\expandafter\def\csname res@v5a@interaction_0.5@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_0.5@granger@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.5@granger@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.5@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v5a@interaction_0.5@granger@prec\endcsname{0.18}
\expandafter\def\csname res@v5a@interaction_0.5@granger@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@granger@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@granger@len\endcsname{14.7}
\expandafter\def\csname res@v5a@interaction_0.5@granger@rp\endcsname{0.59}
\expandafter\def\csname res@v5a@interaction_0.5@granger@map\endcsname{0.73}
\expandafter\def\csname res@v5a@interaction_0.5@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_0.5@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.5@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.5@pcmciplus@tt\endcsname{0.62}
\expandafter\def\csname res@v5a@interaction_0.5@pcmciplus@prec\endcsname{0.89}
\expandafter\def\csname res@v5a@interaction_0.5@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.5@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@pcmciplus@len\endcsname{1.9}
\expandafter\def\csname res@v5a@interaction_0.5@pcmciplus@rp\endcsname{0.75}
\expandafter\def\csname res@v5a@interaction_0.5@pcmciplus@map\endcsname{0.80}
\expandafter\def\csname res@v5a@interaction_0.5@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v5a@interaction_0.5@pc@fpn\endcsname{4}
\expandafter\def\csname res@v5a@interaction_0.5@pc@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.5@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v5a@interaction_0.5@pc@prec\endcsname{0.32}
\expandafter\def\csname res@v5a@interaction_0.5@pc@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@pc@bw\endcsname{3}
\expandafter\def\csname res@v5a@interaction_0.5@pc@len\endcsname{5.2}
\expandafter\def\csname res@v5a@interaction_0.5@pc@rp\endcsname{0.32}
\expandafter\def\csname res@v5a@interaction_0.5@pc@map\endcsname{0.30}
\expandafter\def\csname res@v5a@interaction_0.5@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@interaction_0.5@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.5@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.5@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v5a@interaction_0.5@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5a@interaction_0.5@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.5@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v5a@interaction_0.5@dynotears@rp\endcsname{0.80}
\expandafter\def\csname res@v5a@interaction_0.5@dynotears@map\endcsname{0.87}
\expandafter\def\csname res@v5a@interaction_0.5@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_0.5@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.5@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.5@doubleml@tt\endcsname{0.62}
\expandafter\def\csname res@v5a@interaction_0.5@doubleml@prec\endcsname{0.80}
\expandafter\def\csname res@v5a@interaction_0.5@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.5@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@doubleml@len\endcsname{2.3}
\expandafter\def\csname res@v5a@interaction_0.5@doubleml@rp\endcsname{0.68}
\expandafter\def\csname res@v5a@interaction_0.5@doubleml@map\endcsname{0.77}
\expandafter\def\csname res@v5a@interaction_0.5@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_0.5@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.5@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.5@varlingam@tt\endcsname{0.62}
\expandafter\def\csname res@v5a@interaction_0.5@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v5a@interaction_0.5@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.5@varlingam@len\endcsname{9.6}
\expandafter\def\csname res@v5a@interaction_0.5@varlingam@rp\endcsname{0.68}
\expandafter\def\csname res@v5a@interaction_0.5@varlingam@map\endcsname{0.76}
\expandafter\def\csname res@v5a@interaction_0.5@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_0.5@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.5@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.5@spacetime_rule@tt\endcsname{0.54}
\expandafter\def\csname res@v5a@interaction_0.5@spacetime_rule@prec\endcsname{0.95}
\expandafter\def\csname res@v5a@interaction_0.5@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v5a@interaction_0.5@spacetime_rule@rp\endcsname{0.69}
\expandafter\def\csname res@v5a@interaction_0.5@spacetime_rule@map\endcsname{0.83}
\expandafter\def\csname res@v5a@interaction_0.5@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@interaction_0.5@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.5@varsort@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.5@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@interaction_0.5@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@interaction_0.5@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.5@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5a@interaction_0.5@varsort@rp\endcsname{nan}
\expandafter\def\csname res@v5a@interaction_0.5@varsort@map\endcsname{nan}
\expandafter\def\csname res@v5a@interaction_0.5@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@interaction_0.5@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.5@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5a@interaction_0.5@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5a@interaction_0.5@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.5@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.5@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5a@interaction_0.5@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5a@interaction_0.5@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5a@interaction_0.75@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v5a@interaction_0.75@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v5a@interaction_0.75@correlation@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@correlation@tt\endcsname{0.50}
\expandafter\def\csname res@v5a@interaction_0.75@correlation@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@interaction_0.75@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@correlation@bw\endcsname{2}
\expandafter\def\csname res@v5a@interaction_0.75@correlation@len\endcsname{15.1}
\expandafter\def\csname res@v5a@interaction_0.75@correlation@rp\endcsname{0.54}
\expandafter\def\csname res@v5a@interaction_0.75@correlation@map\endcsname{0.67}
\expandafter\def\csname res@v5a@interaction_0.75@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_0.75@granger@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.75@granger@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@granger@tt\endcsname{0.69}
\expandafter\def\csname res@v5a@interaction_0.75@granger@prec\endcsname{0.23}
\expandafter\def\csname res@v5a@interaction_0.75@granger@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@granger@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@granger@len\endcsname{12.5}
\expandafter\def\csname res@v5a@interaction_0.75@granger@rp\endcsname{0.72}
\expandafter\def\csname res@v5a@interaction_0.75@granger@map\endcsname{0.82}
\expandafter\def\csname res@v5a@interaction_0.75@pcmciplus@fp\endcsname{7/10}
\expandafter\def\csname res@v5a@interaction_0.75@pcmciplus@fpn\endcsname{7}
\expandafter\def\csname res@v5a@interaction_0.75@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@pcmciplus@tt\endcsname{0.65}
\expandafter\def\csname res@v5a@interaction_0.75@pcmciplus@prec\endcsname{0.70}
\expandafter\def\csname res@v5a@interaction_0.75@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.75@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@pcmciplus@len\endcsname{2.3}
\expandafter\def\csname res@v5a@interaction_0.75@pcmciplus@rp\endcsname{0.60}
\expandafter\def\csname res@v5a@interaction_0.75@pcmciplus@map\endcsname{0.75}
\expandafter\def\csname res@v5a@interaction_0.75@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v5a@interaction_0.75@pc@fpn\endcsname{4}
\expandafter\def\csname res@v5a@interaction_0.75@pc@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v5a@interaction_0.75@pc@prec\endcsname{0.37}
\expandafter\def\csname res@v5a@interaction_0.75@pc@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@pc@bw\endcsname{5}
\expandafter\def\csname res@v5a@interaction_0.75@pc@len\endcsname{4.7}
\expandafter\def\csname res@v5a@interaction_0.75@pc@rp\endcsname{0.37}
\expandafter\def\csname res@v5a@interaction_0.75@pc@map\endcsname{0.33}
\expandafter\def\csname res@v5a@interaction_0.75@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@interaction_0.75@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5a@interaction_0.75@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5a@interaction_0.75@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5a@interaction_0.75@dynotears@rp\endcsname{0.79}
\expandafter\def\csname res@v5a@interaction_0.75@dynotears@map\endcsname{0.86}
\expandafter\def\csname res@v5a@interaction_0.75@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v5a@interaction_0.75@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v5a@interaction_0.75@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@doubleml@tt\endcsname{0.54}
\expandafter\def\csname res@v5a@interaction_0.75@doubleml@prec\endcsname{0.73}
\expandafter\def\csname res@v5a@interaction_0.75@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.75@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@doubleml@len\endcsname{2.1}
\expandafter\def\csname res@v5a@interaction_0.75@doubleml@rp\endcsname{0.74}
\expandafter\def\csname res@v5a@interaction_0.75@doubleml@map\endcsname{0.79}
\expandafter\def\csname res@v5a@interaction_0.75@varlingam@fp\endcsname{8/10}
\expandafter\def\csname res@v5a@interaction_0.75@varlingam@fpn\endcsname{8}
\expandafter\def\csname res@v5a@interaction_0.75@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@varlingam@tt\endcsname{0.54}
\expandafter\def\csname res@v5a@interaction_0.75@varlingam@prec\endcsname{0.31}
\expandafter\def\csname res@v5a@interaction_0.75@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v5a@interaction_0.75@varlingam@len\endcsname{8.8}
\expandafter\def\csname res@v5a@interaction_0.75@varlingam@rp\endcsname{0.59}
\expandafter\def\csname res@v5a@interaction_0.75@varlingam@map\endcsname{0.69}
\expandafter\def\csname res@v5a@interaction_0.75@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_0.75@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_0.75@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@spacetime_rule@tt\endcsname{0.50}
\expandafter\def\csname res@v5a@interaction_0.75@spacetime_rule@prec\endcsname{0.95}
\expandafter\def\csname res@v5a@interaction_0.75@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v5a@interaction_0.75@spacetime_rule@rp\endcsname{0.69}
\expandafter\def\csname res@v5a@interaction_0.75@spacetime_rule@map\endcsname{0.83}
\expandafter\def\csname res@v5a@interaction_0.75@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@interaction_0.75@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.75@varsort@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@interaction_0.75@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@interaction_0.75@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.75@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5a@interaction_0.75@varsort@rp\endcsname{nan}
\expandafter\def\csname res@v5a@interaction_0.75@varsort@map\endcsname{nan}
\expandafter\def\csname res@v5a@interaction_0.75@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@interaction_0.75@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_0.75@r2sort@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@interaction_0.75@r2sort@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@interaction_0.75@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_0.75@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_0.75@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5a@interaction_0.75@r2sort@rp\endcsname{0.14}
\expandafter\def\csname res@v5a@interaction_0.75@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5a@interaction_1.0@correlation@fp\endcsname{2/10}
\expandafter\def\csname res@v5a@interaction_1.0@correlation@fpn\endcsname{2}
\expandafter\def\csname res@v5a@interaction_1.0@correlation@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@correlation@tt\endcsname{0.23}
\expandafter\def\csname res@v5a@interaction_1.0@correlation@prec\endcsname{0.20}
\expandafter\def\csname res@v5a@interaction_1.0@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@correlation@bw\endcsname{8}
\expandafter\def\csname res@v5a@interaction_1.0@correlation@len\endcsname{9.7}
\expandafter\def\csname res@v5a@interaction_1.0@correlation@rp\endcsname{0.18}
\expandafter\def\csname res@v5a@interaction_1.0@correlation@map\endcsname{0.38}
\expandafter\def\csname res@v5a@interaction_1.0@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v5a@interaction_1.0@granger@fpn\endcsname{8}
\expandafter\def\csname res@v5a@interaction_1.0@granger@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v5a@interaction_1.0@granger@prec\endcsname{0.29}
\expandafter\def\csname res@v5a@interaction_1.0@granger@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@granger@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@granger@len\endcsname{8.8}
\expandafter\def\csname res@v5a@interaction_1.0@granger@rp\endcsname{0.52}
\expandafter\def\csname res@v5a@interaction_1.0@granger@map\endcsname{0.68}
\expandafter\def\csname res@v5a@interaction_1.0@pcmciplus@fp\endcsname{8/10}
\expandafter\def\csname res@v5a@interaction_1.0@pcmciplus@fpn\endcsname{8}
\expandafter\def\csname res@v5a@interaction_1.0@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@pcmciplus@tt\endcsname{0.50}
\expandafter\def\csname res@v5a@interaction_1.0@pcmciplus@prec\endcsname{0.70}
\expandafter\def\csname res@v5a@interaction_1.0@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@pcmciplus@len\endcsname{1.9}
\expandafter\def\csname res@v5a@interaction_1.0@pcmciplus@rp\endcsname{0.67}
\expandafter\def\csname res@v5a@interaction_1.0@pcmciplus@map\endcsname{0.75}
\expandafter\def\csname res@v5a@interaction_1.0@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@interaction_1.0@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5a@interaction_1.0@pc@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@pc@tt\endcsname{0.12}
\expandafter\def\csname res@v5a@interaction_1.0@pc@prec\endcsname{0.14}
\expandafter\def\csname res@v5a@interaction_1.0@pc@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@pc@bw\endcsname{9}
\expandafter\def\csname res@v5a@interaction_1.0@pc@len\endcsname{3.4}
\expandafter\def\csname res@v5a@interaction_1.0@pc@rp\endcsname{0.16}
\expandafter\def\csname res@v5a@interaction_1.0@pc@map\endcsname{0.21}
\expandafter\def\csname res@v5a@interaction_1.0@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@interaction_1.0@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5a@interaction_1.0@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5a@interaction_1.0@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5a@interaction_1.0@dynotears@rp\endcsname{0.54}
\expandafter\def\csname res@v5a@interaction_1.0@dynotears@map\endcsname{0.67}
\expandafter\def\csname res@v5a@interaction_1.0@doubleml@fp\endcsname{3/10}
\expandafter\def\csname res@v5a@interaction_1.0@doubleml@fpn\endcsname{3}
\expandafter\def\csname res@v5a@interaction_1.0@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@doubleml@tt\endcsname{0.15}
\expandafter\def\csname res@v5a@interaction_1.0@doubleml@prec\endcsname{0.75}
\expandafter\def\csname res@v5a@interaction_1.0@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v5a@interaction_1.0@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@doubleml@len\endcsname{0.6}
\expandafter\def\csname res@v5a@interaction_1.0@doubleml@rp\endcsname{0.45}
\expandafter\def\csname res@v5a@interaction_1.0@doubleml@map\endcsname{0.53}
\expandafter\def\csname res@v5a@interaction_1.0@varlingam@fp\endcsname{2/10}
\expandafter\def\csname res@v5a@interaction_1.0@varlingam@fpn\endcsname{2}
\expandafter\def\csname res@v5a@interaction_1.0@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@varlingam@tt\endcsname{0.23}
\expandafter\def\csname res@v5a@interaction_1.0@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v5a@interaction_1.0@varlingam@ab\endcsname{3}
\expandafter\def\csname res@v5a@interaction_1.0@varlingam@bw\endcsname{3}
\expandafter\def\csname res@v5a@interaction_1.0@varlingam@len\endcsname{3.8}
\expandafter\def\csname res@v5a@interaction_1.0@varlingam@rp\endcsname{0.48}
\expandafter\def\csname res@v5a@interaction_1.0@varlingam@map\endcsname{0.41}
\expandafter\def\csname res@v5a@interaction_1.0@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v5a@interaction_1.0@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v5a@interaction_1.0@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@spacetime_rule@tt\endcsname{0.50}
\expandafter\def\csname res@v5a@interaction_1.0@spacetime_rule@prec\endcsname{0.95}
\expandafter\def\csname res@v5a@interaction_1.0@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v5a@interaction_1.0@spacetime_rule@rp\endcsname{0.62}
\expandafter\def\csname res@v5a@interaction_1.0@spacetime_rule@map\endcsname{0.76}
\expandafter\def\csname res@v5a@interaction_1.0@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@interaction_1.0@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5a@interaction_1.0@varsort@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@interaction_1.0@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@interaction_1.0@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_1.0@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5a@interaction_1.0@varsort@rp\endcsname{nan}
\expandafter\def\csname res@v5a@interaction_1.0@varsort@map\endcsname{nan}
\expandafter\def\csname res@v5a@interaction_1.0@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@interaction_1.0@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5a@interaction_1.0@r2sort@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@interaction_1.0@r2sort@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@interaction_1.0@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5a@interaction_1.0@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5a@interaction_1.0@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5a@interaction_1.0@r2sort@rp\endcsname{0.14}
\expandafter\def\csname res@v5a@interaction_1.0@r2sort@map\endcsname{0.19}
\expandafter\def\csname res@v5a@combo_interaction@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@combo_interaction@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@correlation@n\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@correlation@tt\endcsname{0.12}
\expandafter\def\csname res@v5a@combo_interaction@correlation@prec\endcsname{0.11}
\expandafter\def\csname res@v5a@combo_interaction@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@correlation@bw\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@correlation@len\endcsname{5.6}
\expandafter\def\csname res@v5a@combo_interaction@correlation@rp\endcsname{0.03}
\expandafter\def\csname res@v5a@combo_interaction@correlation@map\endcsname{0.25}
\expandafter\def\csname res@v5a@combo_interaction@granger@fp\endcsname{4/10}
\expandafter\def\csname res@v5a@combo_interaction@granger@fpn\endcsname{4}
\expandafter\def\csname res@v5a@combo_interaction@granger@n\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@granger@tt\endcsname{0.23}
\expandafter\def\csname res@v5a@combo_interaction@granger@prec\endcsname{0.20}
\expandafter\def\csname res@v5a@combo_interaction@granger@ab\endcsname{4}
\expandafter\def\csname res@v5a@combo_interaction@granger@bw\endcsname{1}
\expandafter\def\csname res@v5a@combo_interaction@granger@len\endcsname{3.9}
\expandafter\def\csname res@v5a@combo_interaction@granger@rp\endcsname{0.55}
\expandafter\def\csname res@v5a@combo_interaction@granger@map\endcsname{0.61}
\expandafter\def\csname res@v5a@combo_interaction@pcmciplus@fp\endcsname{4/10}
\expandafter\def\csname res@v5a@combo_interaction@pcmciplus@fpn\endcsname{4}
\expandafter\def\csname res@v5a@combo_interaction@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@pcmciplus@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@combo_interaction@pcmciplus@prec\endcsname{0.58}
\expandafter\def\csname res@v5a@combo_interaction@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v5a@combo_interaction@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@pcmciplus@len\endcsname{0.9}
\expandafter\def\csname res@v5a@combo_interaction@pcmciplus@rp\endcsname{0.42}
\expandafter\def\csname res@v5a@combo_interaction@pcmciplus@map\endcsname{0.60}
\expandafter\def\csname res@v5a@combo_interaction@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@combo_interaction@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5a@combo_interaction@pc@n\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@pc@tt\endcsname{0.04}
\expandafter\def\csname res@v5a@combo_interaction@pc@prec\endcsname{0.05}
\expandafter\def\csname res@v5a@combo_interaction@pc@ab\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@pc@bw\endcsname{8}
\expandafter\def\csname res@v5a@combo_interaction@pc@len\endcsname{2.5}
\expandafter\def\csname res@v5a@combo_interaction@pc@rp\endcsname{0.11}
\expandafter\def\csname res@v5a@combo_interaction@pc@map\endcsname{0.18}
\expandafter\def\csname res@v5a@combo_interaction@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@combo_interaction@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5a@combo_interaction@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5a@combo_interaction@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5a@combo_interaction@dynotears@rp\endcsname{0.55}
\expandafter\def\csname res@v5a@combo_interaction@dynotears@map\endcsname{0.71}
\expandafter\def\csname res@v5a@combo_interaction@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@combo_interaction@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v5a@combo_interaction@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v5a@combo_interaction@doubleml@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@combo_interaction@doubleml@ab\endcsname{7}
\expandafter\def\csname res@v5a@combo_interaction@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@doubleml@len\endcsname{0.4}
\expandafter\def\csname res@v5a@combo_interaction@doubleml@rp\endcsname{0.22}
\expandafter\def\csname res@v5a@combo_interaction@doubleml@map\endcsname{0.36}
\expandafter\def\csname res@v5a@combo_interaction@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@combo_interaction@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@varlingam@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@combo_interaction@varlingam@prec\endcsname{0.16}
\expandafter\def\csname res@v5a@combo_interaction@varlingam@ab\endcsname{1}
\expandafter\def\csname res@v5a@combo_interaction@varlingam@bw\endcsname{9}
\expandafter\def\csname res@v5a@combo_interaction@varlingam@len\endcsname{3.4}
\expandafter\def\csname res@v5a@combo_interaction@varlingam@rp\endcsname{0.19}
\expandafter\def\csname res@v5a@combo_interaction@varlingam@map\endcsname{0.24}
\expandafter\def\csname res@v5a@combo_interaction@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v5a@combo_interaction@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v5a@combo_interaction@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v5a@combo_interaction@spacetime_rule@prec\endcsname{0.53}
\expandafter\def\csname res@v5a@combo_interaction@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v5a@combo_interaction@spacetime_rule@rp\endcsname{0.34}
\expandafter\def\csname res@v5a@combo_interaction@spacetime_rule@map\endcsname{0.50}
\expandafter\def\csname res@v5a@combo_interaction@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v5a@combo_interaction@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v5a@combo_interaction@varsort@n\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v5a@combo_interaction@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v5a@combo_interaction@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5a@combo_interaction@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v5a@combo_interaction@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v5a@combo_interaction@varsort@map\endcsname{0.21}
\expandafter\def\csname res@v5a@combo_interaction@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@combo_interaction@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5a@combo_interaction@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5a@combo_interaction@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5a@combo_interaction@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v5a@combo_interaction@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5a@combo_interaction@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5a@combo_interaction@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5a@combo_interaction@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v5a@control_weak@correlation@fp\endcsname{2/10}
\expandafter\def\csname res@v5a@control_weak@correlation@fpn\endcsname{2}
\expandafter\def\csname res@v5a@control_weak@correlation@n\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@correlation@tt\endcsname{0.50}
\expandafter\def\csname res@v5a@control_weak@correlation@prec\endcsname{0.18}
\expandafter\def\csname res@v5a@control_weak@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@correlation@bw\endcsname{8}
\expandafter\def\csname res@v5a@control_weak@correlation@len\endcsname{12.8}
\expandafter\def\csname res@v5a@control_weak@correlation@rp\endcsname{0.44}
\expandafter\def\csname res@v5a@control_weak@correlation@map\endcsname{0.47}
\expandafter\def\csname res@v5a@control_weak@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v5a@control_weak@granger@fpn\endcsname{8}
\expandafter\def\csname res@v5a@control_weak@granger@n\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v5a@control_weak@granger@prec\endcsname{0.28}
\expandafter\def\csname res@v5a@control_weak@granger@ab\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@granger@bw\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@granger@len\endcsname{8.6}
\expandafter\def\csname res@v5a@control_weak@granger@rp\endcsname{0.63}
\expandafter\def\csname res@v5a@control_weak@granger@map\endcsname{0.75}
\expandafter\def\csname res@v5a@control_weak@pcmciplus@fp\endcsname{8/10}
\expandafter\def\csname res@v5a@control_weak@pcmciplus@fpn\endcsname{8}
\expandafter\def\csname res@v5a@control_weak@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@pcmciplus@tt\endcsname{0.58}
\expandafter\def\csname res@v5a@control_weak@pcmciplus@prec\endcsname{0.72}
\expandafter\def\csname res@v5a@control_weak@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v5a@control_weak@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@pcmciplus@len\endcsname{2.2}
\expandafter\def\csname res@v5a@control_weak@pcmciplus@rp\endcsname{0.66}
\expandafter\def\csname res@v5a@control_weak@pcmciplus@map\endcsname{0.74}
\expandafter\def\csname res@v5a@control_weak@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5a@control_weak@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5a@control_weak@pc@n\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@pc@tt\endcsname{0.23}
\expandafter\def\csname res@v5a@control_weak@pc@prec\endcsname{0.27}
\expandafter\def\csname res@v5a@control_weak@pc@ab\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@pc@bw\endcsname{5}
\expandafter\def\csname res@v5a@control_weak@pc@len\endcsname{4.5}
\expandafter\def\csname res@v5a@control_weak@pc@rp\endcsname{0.27}
\expandafter\def\csname res@v5a@control_weak@pc@map\endcsname{0.26}
\expandafter\def\csname res@v5a@control_weak@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@control_weak@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5a@control_weak@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5a@control_weak@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5a@control_weak@dynotears@rp\endcsname{0.79}
\expandafter\def\csname res@v5a@control_weak@dynotears@map\endcsname{0.85}
\expandafter\def\csname res@v5a@control_weak@doubleml@fp\endcsname{7/10}
\expandafter\def\csname res@v5a@control_weak@doubleml@fpn\endcsname{7}
\expandafter\def\csname res@v5a@control_weak@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@doubleml@tt\endcsname{0.46}
\expandafter\def\csname res@v5a@control_weak@doubleml@prec\endcsname{0.86}
\expandafter\def\csname res@v5a@control_weak@doubleml@ab\endcsname{3}
\expandafter\def\csname res@v5a@control_weak@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@doubleml@len\endcsname{1.7}
\expandafter\def\csname res@v5a@control_weak@doubleml@rp\endcsname{0.59}
\expandafter\def\csname res@v5a@control_weak@doubleml@map\endcsname{0.71}
\expandafter\def\csname res@v5a@control_weak@varlingam@fp\endcsname{4/10}
\expandafter\def\csname res@v5a@control_weak@varlingam@fpn\endcsname{4}
\expandafter\def\csname res@v5a@control_weak@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@varlingam@tt\endcsname{0.38}
\expandafter\def\csname res@v5a@control_weak@varlingam@prec\endcsname{0.43}
\expandafter\def\csname res@v5a@control_weak@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@varlingam@bw\endcsname{6}
\expandafter\def\csname res@v5a@control_weak@varlingam@len\endcsname{5.2}
\expandafter\def\csname res@v5a@control_weak@varlingam@rp\endcsname{0.34}
\expandafter\def\csname res@v5a@control_weak@varlingam@map\endcsname{0.47}
\expandafter\def\csname res@v5a@control_weak@spacetime_rule@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@control_weak@spacetime_rule@fpn\endcsname{1}
\expandafter\def\csname res@v5a@control_weak@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@spacetime_rule@tt\endcsname{0.04}
\expandafter\def\csname res@v5a@control_weak@spacetime_rule@prec\endcsname{0.33}
\expandafter\def\csname res@v5a@control_weak@spacetime_rule@ab\endcsname{7}
\expandafter\def\csname res@v5a@control_weak@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@spacetime_rule@len\endcsname{0.3}
\expandafter\def\csname res@v5a@control_weak@spacetime_rule@rp\endcsname{0.31}
\expandafter\def\csname res@v5a@control_weak@spacetime_rule@map\endcsname{0.38}
\expandafter\def\csname res@v5a@control_weak@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@control_weak@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5a@control_weak@varsort@n\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v5a@control_weak@varsort@prec\endcsname{0.20}
\expandafter\def\csname res@v5a@control_weak@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5a@control_weak@varsort@len\endcsname{2.6}
\expandafter\def\csname res@v5a@control_weak@varsort@rp\endcsname{0.19}
\expandafter\def\csname res@v5a@control_weak@varsort@map\endcsname{0.33}
\expandafter\def\csname res@v5a@control_weak@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5a@control_weak@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5a@control_weak@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5a@control_weak@r2sort@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@control_weak@r2sort@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@control_weak@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5a@control_weak@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5a@control_weak@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5a@control_weak@r2sort@rp\endcsname{0.23}
\expandafter\def\csname res@v5a@control_weak@r2sort@map\endcsname{0.29}
\expandafter\def\csname res@v5a@signal_0.05@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@signal_0.05@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@correlation@n\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@correlation@tt\endcsname{0.27}
\expandafter\def\csname res@v5a@signal_0.05@correlation@prec\endcsname{0.22}
\expandafter\def\csname res@v5a@signal_0.05@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@correlation@bw\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@correlation@len\endcsname{10.0}
\expandafter\def\csname res@v5a@signal_0.05@correlation@rp\endcsname{0.12}
\expandafter\def\csname res@v5a@signal_0.05@correlation@map\endcsname{0.34}
\expandafter\def\csname res@v5a@signal_0.05@granger@fp\endcsname{6/10}
\expandafter\def\csname res@v5a@signal_0.05@granger@fpn\endcsname{6}
\expandafter\def\csname res@v5a@signal_0.05@granger@n\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v5a@signal_0.05@granger@prec\endcsname{0.55}
\expandafter\def\csname res@v5a@signal_0.05@granger@ab\endcsname{1}
\expandafter\def\csname res@v5a@signal_0.05@granger@bw\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@granger@len\endcsname{4.5}
\expandafter\def\csname res@v5a@signal_0.05@granger@rp\endcsname{0.48}
\expandafter\def\csname res@v5a@signal_0.05@granger@map\endcsname{0.64}
\expandafter\def\csname res@v5a@signal_0.05@pcmciplus@fp\endcsname{4/10}
\expandafter\def\csname res@v5a@signal_0.05@pcmciplus@fpn\endcsname{4}
\expandafter\def\csname res@v5a@signal_0.05@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@pcmciplus@tt\endcsname{0.27}
\expandafter\def\csname res@v5a@signal_0.05@pcmciplus@prec\endcsname{0.44}
\expandafter\def\csname res@v5a@signal_0.05@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v5a@signal_0.05@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@pcmciplus@len\endcsname{1.6}
\expandafter\def\csname res@v5a@signal_0.05@pcmciplus@rp\endcsname{0.50}
\expandafter\def\csname res@v5a@signal_0.05@pcmciplus@map\endcsname{0.62}
\expandafter\def\csname res@v5a@signal_0.05@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5a@signal_0.05@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5a@signal_0.05@pc@n\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v5a@signal_0.05@pc@prec\endcsname{0.25}
\expandafter\def\csname res@v5a@signal_0.05@pc@ab\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@pc@bw\endcsname{6}
\expandafter\def\csname res@v5a@signal_0.05@pc@len\endcsname{4.2}
\expandafter\def\csname res@v5a@signal_0.05@pc@rp\endcsname{0.27}
\expandafter\def\csname res@v5a@signal_0.05@pc@map\endcsname{0.23}
\expandafter\def\csname res@v5a@signal_0.05@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@signal_0.05@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5a@signal_0.05@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5a@signal_0.05@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5a@signal_0.05@dynotears@rp\endcsname{0.40}
\expandafter\def\csname res@v5a@signal_0.05@dynotears@map\endcsname{0.56}
\expandafter\def\csname res@v5a@signal_0.05@doubleml@fp\endcsname{3/10}
\expandafter\def\csname res@v5a@signal_0.05@doubleml@fpn\endcsname{3}
\expandafter\def\csname res@v5a@signal_0.05@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@doubleml@tt\endcsname{0.15}
\expandafter\def\csname res@v5a@signal_0.05@doubleml@prec\endcsname{0.92}
\expandafter\def\csname res@v5a@signal_0.05@doubleml@ab\endcsname{7}
\expandafter\def\csname res@v5a@signal_0.05@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@doubleml@len\endcsname{0.6}
\expandafter\def\csname res@v5a@signal_0.05@doubleml@rp\endcsname{0.38}
\expandafter\def\csname res@v5a@signal_0.05@doubleml@map\endcsname{0.52}
\expandafter\def\csname res@v5a@signal_0.05@varlingam@fp\endcsname{2/10}
\expandafter\def\csname res@v5a@signal_0.05@varlingam@fpn\endcsname{2}
\expandafter\def\csname res@v5a@signal_0.05@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@varlingam@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@signal_0.05@varlingam@prec\endcsname{0.26}
\expandafter\def\csname res@v5a@signal_0.05@varlingam@ab\endcsname{1}
\expandafter\def\csname res@v5a@signal_0.05@varlingam@bw\endcsname{7}
\expandafter\def\csname res@v5a@signal_0.05@varlingam@len\endcsname{4.0}
\expandafter\def\csname res@v5a@signal_0.05@varlingam@rp\endcsname{0.27}
\expandafter\def\csname res@v5a@signal_0.05@varlingam@map\endcsname{0.30}
\expandafter\def\csname res@v5a@signal_0.05@spacetime_rule@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@signal_0.05@spacetime_rule@fpn\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@spacetime_rule@tt\endcsname{0.00}
\expandafter\def\csname res@v5a@signal_0.05@spacetime_rule@prec\endcsname{0.00}
\expandafter\def\csname res@v5a@signal_0.05@spacetime_rule@ab\endcsname{8}
\expandafter\def\csname res@v5a@signal_0.05@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@spacetime_rule@len\endcsname{0.2}
\expandafter\def\csname res@v5a@signal_0.05@spacetime_rule@rp\endcsname{0.15}
\expandafter\def\csname res@v5a@signal_0.05@spacetime_rule@map\endcsname{0.26}
\expandafter\def\csname res@v5a@signal_0.05@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@signal_0.05@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@varsort@n\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@signal_0.05@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@signal_0.05@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@varsort@bw\endcsname{2}
\expandafter\def\csname res@v5a@signal_0.05@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5a@signal_0.05@varsort@rp\endcsname{0.16}
\expandafter\def\csname res@v5a@signal_0.05@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v5a@signal_0.05@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5a@signal_0.05@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5a@signal_0.05@r2sort@tt\endcsname{0.19}
\expandafter\def\csname res@v5a@signal_0.05@r2sort@prec\endcsname{0.17}
\expandafter\def\csname res@v5a@signal_0.05@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5a@signal_0.05@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5a@signal_0.05@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5a@signal_0.05@r2sort@rp\endcsname{0.14}
\expandafter\def\csname res@v5a@signal_0.05@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5b@default@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v5b@default@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v5b@default@correlation@n\endcsname{10}
\expandafter\def\csname res@v5b@default@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v5b@default@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v5b@default@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5b@default@correlation@bw\endcsname{1}
\expandafter\def\csname res@v5b@default@correlation@len\endcsname{36.1}
\expandafter\def\csname res@v5b@default@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v5b@default@correlation@map\endcsname{0.64}
\expandafter\def\csname res@v5b@default@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v5b@default@granger@fpn\endcsname{8}
\expandafter\def\csname res@v5b@default@granger@n\endcsname{10}
\expandafter\def\csname res@v5b@default@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v5b@default@granger@prec\endcsname{0.08}
\expandafter\def\csname res@v5b@default@granger@ab\endcsname{0}
\expandafter\def\csname res@v5b@default@granger@bw\endcsname{0}
\expandafter\def\csname res@v5b@default@granger@len\endcsname{32.6}
\expandafter\def\csname res@v5b@default@granger@rp\endcsname{0.59}
\expandafter\def\csname res@v5b@default@granger@map\endcsname{0.63}
\expandafter\def\csname res@v5b@default@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v5b@default@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v5b@default@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5b@default@pcmciplus@tt\endcsname{0.88}
\expandafter\def\csname res@v5b@default@pcmciplus@prec\endcsname{0.71}
\expandafter\def\csname res@v5b@default@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v5b@default@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5b@default@pcmciplus@len\endcsname{3.3}
\expandafter\def\csname res@v5b@default@pcmciplus@rp\endcsname{0.85}
\expandafter\def\csname res@v5b@default@pcmciplus@map\endcsname{0.92}
\expandafter\def\csname res@v5b@default@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5b@default@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5b@default@pc@n\endcsname{10}
\expandafter\def\csname res@v5b@default@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v5b@default@pc@prec\endcsname{0.29}
\expandafter\def\csname res@v5b@default@pc@ab\endcsname{0}
\expandafter\def\csname res@v5b@default@pc@bw\endcsname{3}
\expandafter\def\csname res@v5b@default@pc@len\endcsname{5.6}
\expandafter\def\csname res@v5b@default@pc@rp\endcsname{0.29}
\expandafter\def\csname res@v5b@default@pc@map\endcsname{0.22}
\expandafter\def\csname res@v5b@default@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v5b@default@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v5b@default@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5b@default@dynotears@tt\endcsname{0.19}
\expandafter\def\csname res@v5b@default@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5b@default@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v5b@default@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5b@default@dynotears@len\endcsname{0.5}
\expandafter\def\csname res@v5b@default@dynotears@rp\endcsname{0.95}
\expandafter\def\csname res@v5b@default@dynotears@map\endcsname{0.96}
\expandafter\def\csname res@v5b@default@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v5b@default@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v5b@default@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5b@default@doubleml@tt\endcsname{0.62}
\expandafter\def\csname res@v5b@default@doubleml@prec\endcsname{0.77}
\expandafter\def\csname res@v5b@default@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v5b@default@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5b@default@doubleml@len\endcsname{2.8}
\expandafter\def\csname res@v5b@default@doubleml@rp\endcsname{0.66}
\expandafter\def\csname res@v5b@default@doubleml@map\endcsname{0.77}
\expandafter\def\csname res@v5b@default@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v5b@default@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v5b@default@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5b@default@varlingam@tt\endcsname{0.62}
\expandafter\def\csname res@v5b@default@varlingam@prec\endcsname{0.25}
\expandafter\def\csname res@v5b@default@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5b@default@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v5b@default@varlingam@len\endcsname{10.3}
\expandafter\def\csname res@v5b@default@varlingam@rp\endcsname{0.64}
\expandafter\def\csname res@v5b@default@varlingam@map\endcsname{0.78}
\expandafter\def\csname res@v5b@default@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v5b@default@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v5b@default@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5b@default@spacetime_rule@tt\endcsname{0.35}
\expandafter\def\csname res@v5b@default@spacetime_rule@prec\endcsname{0.80}
\expandafter\def\csname res@v5b@default@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5b@default@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5b@default@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v5b@default@spacetime_rule@rp\endcsname{0.55}
\expandafter\def\csname res@v5b@default@spacetime_rule@map\endcsname{0.65}
\expandafter\def\csname res@v5b@default@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@default@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@default@varsort@n\endcsname{10}
\expandafter\def\csname res@v5b@default@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@default@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@default@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5b@default@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5b@default@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5b@default@varsort@rp\endcsname{0.03}
\expandafter\def\csname res@v5b@default@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@default@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@default@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@default@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5b@default@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@default@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@default@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5b@default@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5b@default@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5b@default@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v5b@default@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@signal_0.1@correlation@fp\endcsname{1/10}
\expandafter\def\csname res@v5b@signal_0.1@correlation@fpn\endcsname{1}
\expandafter\def\csname res@v5b@signal_0.1@correlation@n\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@correlation@tt\endcsname{0.35}
\expandafter\def\csname res@v5b@signal_0.1@correlation@prec\endcsname{0.13}
\expandafter\def\csname res@v5b@signal_0.1@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@correlation@bw\endcsname{9}
\expandafter\def\csname res@v5b@signal_0.1@correlation@len\endcsname{23.7}
\expandafter\def\csname res@v5b@signal_0.1@correlation@rp\endcsname{0.33}
\expandafter\def\csname res@v5b@signal_0.1@correlation@map\endcsname{0.42}
\expandafter\def\csname res@v5b@signal_0.1@granger@fp\endcsname{7/10}
\expandafter\def\csname res@v5b@signal_0.1@granger@fpn\endcsname{7}
\expandafter\def\csname res@v5b@signal_0.1@granger@n\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v5b@signal_0.1@granger@prec\endcsname{0.18}
\expandafter\def\csname res@v5b@signal_0.1@granger@ab\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@granger@bw\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@granger@len\endcsname{14.5}
\expandafter\def\csname res@v5b@signal_0.1@granger@rp\endcsname{0.52}
\expandafter\def\csname res@v5b@signal_0.1@granger@map\endcsname{0.56}
\expandafter\def\csname res@v5b@signal_0.1@pcmciplus@fp\endcsname{5/10}
\expandafter\def\csname res@v5b@signal_0.1@pcmciplus@fpn\endcsname{5}
\expandafter\def\csname res@v5b@signal_0.1@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@pcmciplus@tt\endcsname{0.23}
\expandafter\def\csname res@v5b@signal_0.1@pcmciplus@prec\endcsname{0.47}
\expandafter\def\csname res@v5b@signal_0.1@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v5b@signal_0.1@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@pcmciplus@len\endcsname{1.6}
\expandafter\def\csname res@v5b@signal_0.1@pcmciplus@rp\endcsname{0.71}
\expandafter\def\csname res@v5b@signal_0.1@pcmciplus@map\endcsname{0.72}
\expandafter\def\csname res@v5b@signal_0.1@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5b@signal_0.1@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5b@signal_0.1@pc@n\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@pc@tt\endcsname{0.19}
\expandafter\def\csname res@v5b@signal_0.1@pc@prec\endcsname{0.21}
\expandafter\def\csname res@v5b@signal_0.1@pc@ab\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@pc@bw\endcsname{6}
\expandafter\def\csname res@v5b@signal_0.1@pc@len\endcsname{3.6}
\expandafter\def\csname res@v5b@signal_0.1@pc@rp\endcsname{0.21}
\expandafter\def\csname res@v5b@signal_0.1@pc@map\endcsname{0.16}
\expandafter\def\csname res@v5b@signal_0.1@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@signal_0.1@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@signal_0.1@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5b@signal_0.1@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5b@signal_0.1@dynotears@rp\endcsname{0.68}
\expandafter\def\csname res@v5b@signal_0.1@dynotears@map\endcsname{0.77}
\expandafter\def\csname res@v5b@signal_0.1@doubleml@fp\endcsname{3/10}
\expandafter\def\csname res@v5b@signal_0.1@doubleml@fpn\endcsname{3}
\expandafter\def\csname res@v5b@signal_0.1@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@doubleml@tt\endcsname{0.12}
\expandafter\def\csname res@v5b@signal_0.1@doubleml@prec\endcsname{0.75}
\expandafter\def\csname res@v5b@signal_0.1@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v5b@signal_0.1@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@doubleml@len\endcsname{0.4}
\expandafter\def\csname res@v5b@signal_0.1@doubleml@rp\endcsname{0.48}
\expandafter\def\csname res@v5b@signal_0.1@doubleml@map\endcsname{0.49}
\expandafter\def\csname res@v5b@signal_0.1@varlingam@fp\endcsname{3/10}
\expandafter\def\csname res@v5b@signal_0.1@varlingam@fpn\endcsname{3}
\expandafter\def\csname res@v5b@signal_0.1@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@varlingam@tt\endcsname{0.35}
\expandafter\def\csname res@v5b@signal_0.1@varlingam@prec\endcsname{0.25}
\expandafter\def\csname res@v5b@signal_0.1@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@varlingam@bw\endcsname{7}
\expandafter\def\csname res@v5b@signal_0.1@varlingam@len\endcsname{6.4}
\expandafter\def\csname res@v5b@signal_0.1@varlingam@rp\endcsname{0.36}
\expandafter\def\csname res@v5b@signal_0.1@varlingam@map\endcsname{0.36}
\expandafter\def\csname res@v5b@signal_0.1@spacetime_rule@fp\endcsname{4/10}
\expandafter\def\csname res@v5b@signal_0.1@spacetime_rule@fpn\endcsname{4}
\expandafter\def\csname res@v5b@signal_0.1@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@spacetime_rule@tt\endcsname{0.15}
\expandafter\def\csname res@v5b@signal_0.1@spacetime_rule@prec\endcsname{0.50}
\expandafter\def\csname res@v5b@signal_0.1@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v5b@signal_0.1@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@spacetime_rule@len\endcsname{0.8}
\expandafter\def\csname res@v5b@signal_0.1@spacetime_rule@rp\endcsname{0.32}
\expandafter\def\csname res@v5b@signal_0.1@spacetime_rule@map\endcsname{0.41}
\expandafter\def\csname res@v5b@signal_0.1@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@signal_0.1@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@varsort@n\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@signal_0.1@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@signal_0.1@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5b@signal_0.1@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5b@signal_0.1@varsort@rp\endcsname{0.03}
\expandafter\def\csname res@v5b@signal_0.1@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@signal_0.1@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@signal_0.1@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5b@signal_0.1@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@signal_0.1@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@signal_0.1@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5b@signal_0.1@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5b@signal_0.1@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v5b@signal_0.1@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@echo_0.8@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v5b@echo_0.8@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v5b@echo_0.8@correlation@n\endcsname{10}
\expandafter\def\csname res@v5b@echo_0.8@correlation@tt\endcsname{0.42}
\expandafter\def\csname res@v5b@echo_0.8@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v5b@echo_0.8@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@correlation@bw\endcsname{1}
\expandafter\def\csname res@v5b@echo_0.8@correlation@len\endcsname{37.1}
\expandafter\def\csname res@v5b@echo_0.8@correlation@rp\endcsname{0.49}
\expandafter\def\csname res@v5b@echo_0.8@correlation@map\endcsname{0.57}
\expandafter\def\csname res@v5b@echo_0.8@granger@fp\endcsname{7/10}
\expandafter\def\csname res@v5b@echo_0.8@granger@fpn\endcsname{7}
\expandafter\def\csname res@v5b@echo_0.8@granger@n\endcsname{10}
\expandafter\def\csname res@v5b@echo_0.8@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v5b@echo_0.8@granger@prec\endcsname{0.08}
\expandafter\def\csname res@v5b@echo_0.8@granger@ab\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@granger@bw\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@granger@len\endcsname{33.5}
\expandafter\def\csname res@v5b@echo_0.8@granger@rp\endcsname{0.56}
\expandafter\def\csname res@v5b@echo_0.8@granger@map\endcsname{0.59}
\expandafter\def\csname res@v5b@echo_0.8@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v5b@echo_0.8@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v5b@echo_0.8@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5b@echo_0.8@pcmciplus@tt\endcsname{0.58}
\expandafter\def\csname res@v5b@echo_0.8@pcmciplus@prec\endcsname{0.57}
\expandafter\def\csname res@v5b@echo_0.8@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@pcmciplus@len\endcsname{2.9}
\expandafter\def\csname res@v5b@echo_0.8@pcmciplus@rp\endcsname{0.76}
\expandafter\def\csname res@v5b@echo_0.8@pcmciplus@map\endcsname{0.81}
\expandafter\def\csname res@v5b@echo_0.8@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5b@echo_0.8@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5b@echo_0.8@pc@n\endcsname{10}
\expandafter\def\csname res@v5b@echo_0.8@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v5b@echo_0.8@pc@prec\endcsname{0.24}
\expandafter\def\csname res@v5b@echo_0.8@pc@ab\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@pc@bw\endcsname{3}
\expandafter\def\csname res@v5b@echo_0.8@pc@len\endcsname{5.4}
\expandafter\def\csname res@v5b@echo_0.8@pc@rp\endcsname{0.24}
\expandafter\def\csname res@v5b@echo_0.8@pc@map\endcsname{0.16}
\expandafter\def\csname res@v5b@echo_0.8@dynotears@fp\endcsname{3/10}
\expandafter\def\csname res@v5b@echo_0.8@dynotears@fpn\endcsname{3}
\expandafter\def\csname res@v5b@echo_0.8@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5b@echo_0.8@dynotears@tt\endcsname{0.12}
\expandafter\def\csname res@v5b@echo_0.8@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5b@echo_0.8@dynotears@ab\endcsname{7}
\expandafter\def\csname res@v5b@echo_0.8@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@dynotears@len\endcsname{0.3}
\expandafter\def\csname res@v5b@echo_0.8@dynotears@rp\endcsname{0.92}
\expandafter\def\csname res@v5b@echo_0.8@dynotears@map\endcsname{0.95}
\expandafter\def\csname res@v5b@echo_0.8@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v5b@echo_0.8@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v5b@echo_0.8@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5b@echo_0.8@doubleml@tt\endcsname{0.54}
\expandafter\def\csname res@v5b@echo_0.8@doubleml@prec\endcsname{0.67}
\expandafter\def\csname res@v5b@echo_0.8@doubleml@ab\endcsname{2}
\expandafter\def\csname res@v5b@echo_0.8@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@doubleml@len\endcsname{2.7}
\expandafter\def\csname res@v5b@echo_0.8@doubleml@rp\endcsname{0.55}
\expandafter\def\csname res@v5b@echo_0.8@doubleml@map\endcsname{0.66}
\expandafter\def\csname res@v5b@echo_0.8@varlingam@fp\endcsname{6/10}
\expandafter\def\csname res@v5b@echo_0.8@varlingam@fpn\endcsname{6}
\expandafter\def\csname res@v5b@echo_0.8@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5b@echo_0.8@varlingam@tt\endcsname{0.38}
\expandafter\def\csname res@v5b@echo_0.8@varlingam@prec\endcsname{0.17}
\expandafter\def\csname res@v5b@echo_0.8@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@varlingam@len\endcsname{14.7}
\expandafter\def\csname res@v5b@echo_0.8@varlingam@rp\endcsname{0.48}
\expandafter\def\csname res@v5b@echo_0.8@varlingam@map\endcsname{0.51}
\expandafter\def\csname res@v5b@echo_0.8@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v5b@echo_0.8@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v5b@echo_0.8@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5b@echo_0.8@spacetime_rule@tt\endcsname{0.27}
\expandafter\def\csname res@v5b@echo_0.8@spacetime_rule@prec\endcsname{0.70}
\expandafter\def\csname res@v5b@echo_0.8@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@spacetime_rule@len\endcsname{1.0}
\expandafter\def\csname res@v5b@echo_0.8@spacetime_rule@rp\endcsname{0.42}
\expandafter\def\csname res@v5b@echo_0.8@spacetime_rule@map\endcsname{0.53}
\expandafter\def\csname res@v5b@echo_0.8@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@echo_0.8@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@varsort@n\endcsname{10}
\expandafter\def\csname res@v5b@echo_0.8@varsort@tt\endcsname{0.04}
\expandafter\def\csname res@v5b@echo_0.8@varsort@prec\endcsname{0.03}
\expandafter\def\csname res@v5b@echo_0.8@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5b@echo_0.8@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5b@echo_0.8@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v5b@echo_0.8@varsort@map\endcsname{0.11}
\expandafter\def\csname res@v5b@echo_0.8@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@echo_0.8@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5b@echo_0.8@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@echo_0.8@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@echo_0.8@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5b@echo_0.8@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5b@echo_0.8@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v5b@echo_0.8@r2sort@map\endcsname{0.09}
\expandafter\def\csname res@v5b@confound_0.8@correlation@fp\endcsname{6/10}
\expandafter\def\csname res@v5b@confound_0.8@correlation@fpn\endcsname{6}
\expandafter\def\csname res@v5b@confound_0.8@correlation@n\endcsname{10}
\expandafter\def\csname res@v5b@confound_0.8@correlation@tt\endcsname{0.31}
\expandafter\def\csname res@v5b@confound_0.8@correlation@prec\endcsname{0.06}
\expandafter\def\csname res@v5b@confound_0.8@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@correlation@bw\endcsname{2}
\expandafter\def\csname res@v5b@confound_0.8@correlation@len\endcsname{37.1}
\expandafter\def\csname res@v5b@confound_0.8@correlation@rp\endcsname{0.39}
\expandafter\def\csname res@v5b@confound_0.8@correlation@map\endcsname{0.42}
\expandafter\def\csname res@v5b@confound_0.8@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v5b@confound_0.8@granger@fpn\endcsname{8}
\expandafter\def\csname res@v5b@confound_0.8@granger@n\endcsname{10}
\expandafter\def\csname res@v5b@confound_0.8@granger@tt\endcsname{0.38}
\expandafter\def\csname res@v5b@confound_0.8@granger@prec\endcsname{0.07}
\expandafter\def\csname res@v5b@confound_0.8@granger@ab\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@granger@bw\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@granger@len\endcsname{33.5}
\expandafter\def\csname res@v5b@confound_0.8@granger@rp\endcsname{0.47}
\expandafter\def\csname res@v5b@confound_0.8@granger@map\endcsname{0.52}
\expandafter\def\csname res@v5b@confound_0.8@pcmciplus@fp\endcsname{8/10}
\expandafter\def\csname res@v5b@confound_0.8@pcmciplus@fpn\endcsname{8}
\expandafter\def\csname res@v5b@confound_0.8@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5b@confound_0.8@pcmciplus@tt\endcsname{0.58}
\expandafter\def\csname res@v5b@confound_0.8@pcmciplus@prec\endcsname{0.71}
\expandafter\def\csname res@v5b@confound_0.8@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@pcmciplus@len\endcsname{2.1}
\expandafter\def\csname res@v5b@confound_0.8@pcmciplus@rp\endcsname{0.82}
\expandafter\def\csname res@v5b@confound_0.8@pcmciplus@map\endcsname{0.87}
\expandafter\def\csname res@v5b@confound_0.8@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v5b@confound_0.8@pc@fpn\endcsname{3}
\expandafter\def\csname res@v5b@confound_0.8@pc@n\endcsname{10}
\expandafter\def\csname res@v5b@confound_0.8@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v5b@confound_0.8@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v5b@confound_0.8@pc@ab\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@pc@bw\endcsname{3}
\expandafter\def\csname res@v5b@confound_0.8@pc@len\endcsname{3.8}
\expandafter\def\csname res@v5b@confound_0.8@pc@rp\endcsname{0.32}
\expandafter\def\csname res@v5b@confound_0.8@pc@map\endcsname{0.23}
\expandafter\def\csname res@v5b@confound_0.8@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v5b@confound_0.8@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v5b@confound_0.8@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5b@confound_0.8@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v5b@confound_0.8@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5b@confound_0.8@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v5b@confound_0.8@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v5b@confound_0.8@dynotears@rp\endcsname{0.62}
\expandafter\def\csname res@v5b@confound_0.8@dynotears@map\endcsname{0.77}
\expandafter\def\csname res@v5b@confound_0.8@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v5b@confound_0.8@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v5b@confound_0.8@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5b@confound_0.8@doubleml@tt\endcsname{0.58}
\expandafter\def\csname res@v5b@confound_0.8@doubleml@prec\endcsname{0.84}
\expandafter\def\csname res@v5b@confound_0.8@doubleml@ab\endcsname{2}
\expandafter\def\csname res@v5b@confound_0.8@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@doubleml@len\endcsname{2.4}
\expandafter\def\csname res@v5b@confound_0.8@doubleml@rp\endcsname{0.71}
\expandafter\def\csname res@v5b@confound_0.8@doubleml@map\endcsname{0.75}
\expandafter\def\csname res@v5b@confound_0.8@varlingam@fp\endcsname{7/10}
\expandafter\def\csname res@v5b@confound_0.8@varlingam@fpn\endcsname{7}
\expandafter\def\csname res@v5b@confound_0.8@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5b@confound_0.8@varlingam@tt\endcsname{0.54}
\expandafter\def\csname res@v5b@confound_0.8@varlingam@prec\endcsname{0.22}
\expandafter\def\csname res@v5b@confound_0.8@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v5b@confound_0.8@varlingam@len\endcsname{11.2}
\expandafter\def\csname res@v5b@confound_0.8@varlingam@rp\endcsname{0.48}
\expandafter\def\csname res@v5b@confound_0.8@varlingam@map\endcsname{0.62}
\expandafter\def\csname res@v5b@confound_0.8@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v5b@confound_0.8@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v5b@confound_0.8@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5b@confound_0.8@spacetime_rule@tt\endcsname{0.35}
\expandafter\def\csname res@v5b@confound_0.8@spacetime_rule@prec\endcsname{0.51}
\expandafter\def\csname res@v5b@confound_0.8@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v5b@confound_0.8@spacetime_rule@len\endcsname{2.1}
\expandafter\def\csname res@v5b@confound_0.8@spacetime_rule@rp\endcsname{0.47}
\expandafter\def\csname res@v5b@confound_0.8@spacetime_rule@map\endcsname{0.53}
\expandafter\def\csname res@v5b@confound_0.8@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@confound_0.8@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@varsort@n\endcsname{10}
\expandafter\def\csname res@v5b@confound_0.8@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@confound_0.8@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@confound_0.8@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5b@confound_0.8@varsort@rp\endcsname{0.06}
\expandafter\def\csname res@v5b@confound_0.8@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@confound_0.8@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@confound_0.8@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5b@confound_0.8@r2sort@tt\endcsname{0.04}
\expandafter\def\csname res@v5b@confound_0.8@r2sort@prec\endcsname{0.03}
\expandafter\def\csname res@v5b@confound_0.8@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5b@confound_0.8@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5b@confound_0.8@r2sort@rp\endcsname{0.03}
\expandafter\def\csname res@v5b@confound_0.8@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@combo_hard@correlation@fp\endcsname{3/10}
\expandafter\def\csname res@v5b@combo_hard@correlation@fpn\endcsname{3}
\expandafter\def\csname res@v5b@combo_hard@correlation@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@correlation@tt\endcsname{0.38}
\expandafter\def\csname res@v5b@combo_hard@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v5b@combo_hard@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@correlation@bw\endcsname{5}
\expandafter\def\csname res@v5b@combo_hard@correlation@len\endcsname{34.8}
\expandafter\def\csname res@v5b@combo_hard@correlation@rp\endcsname{0.25}
\expandafter\def\csname res@v5b@combo_hard@correlation@map\endcsname{0.38}
\expandafter\def\csname res@v5b@combo_hard@granger@fp\endcsname{7/10}
\expandafter\def\csname res@v5b@combo_hard@granger@fpn\endcsname{7}
\expandafter\def\csname res@v5b@combo_hard@granger@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@granger@tt\endcsname{0.38}
\expandafter\def\csname res@v5b@combo_hard@granger@prec\endcsname{0.09}
\expandafter\def\csname res@v5b@combo_hard@granger@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@granger@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@granger@len\endcsname{28.3}
\expandafter\def\csname res@v5b@combo_hard@granger@rp\endcsname{0.42}
\expandafter\def\csname res@v5b@combo_hard@granger@map\endcsname{0.50}
\expandafter\def\csname res@v5b@combo_hard@pcmciplus@fp\endcsname{6/10}
\expandafter\def\csname res@v5b@combo_hard@pcmciplus@fpn\endcsname{6}
\expandafter\def\csname res@v5b@combo_hard@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@pcmciplus@tt\endcsname{0.38}
\expandafter\def\csname res@v5b@combo_hard@pcmciplus@prec\endcsname{0.52}
\expandafter\def\csname res@v5b@combo_hard@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v5b@combo_hard@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@pcmciplus@len\endcsname{2.0}
\expandafter\def\csname res@v5b@combo_hard@pcmciplus@rp\endcsname{0.65}
\expandafter\def\csname res@v5b@combo_hard@pcmciplus@map\endcsname{0.71}
\expandafter\def\csname res@v5b@combo_hard@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5b@combo_hard@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5b@combo_hard@pc@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@pc@tt\endcsname{0.23}
\expandafter\def\csname res@v5b@combo_hard@pc@prec\endcsname{0.27}
\expandafter\def\csname res@v5b@combo_hard@pc@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@pc@bw\endcsname{5}
\expandafter\def\csname res@v5b@combo_hard@pc@len\endcsname{3.5}
\expandafter\def\csname res@v5b@combo_hard@pc@rp\endcsname{0.23}
\expandafter\def\csname res@v5b@combo_hard@pc@map\endcsname{0.19}
\expandafter\def\csname res@v5b@combo_hard@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_hard@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@combo_hard@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5b@combo_hard@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5b@combo_hard@dynotears@rp\endcsname{0.71}
\expandafter\def\csname res@v5b@combo_hard@dynotears@map\endcsname{0.77}
\expandafter\def\csname res@v5b@combo_hard@doubleml@fp\endcsname{7/10}
\expandafter\def\csname res@v5b@combo_hard@doubleml@fpn\endcsname{7}
\expandafter\def\csname res@v5b@combo_hard@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@doubleml@tt\endcsname{0.42}
\expandafter\def\csname res@v5b@combo_hard@doubleml@prec\endcsname{0.86}
\expandafter\def\csname res@v5b@combo_hard@doubleml@ab\endcsname{3}
\expandafter\def\csname res@v5b@combo_hard@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@doubleml@len\endcsname{1.6}
\expandafter\def\csname res@v5b@combo_hard@doubleml@rp\endcsname{0.59}
\expandafter\def\csname res@v5b@combo_hard@doubleml@map\endcsname{0.61}
\expandafter\def\csname res@v5b@combo_hard@varlingam@fp\endcsname{2/10}
\expandafter\def\csname res@v5b@combo_hard@varlingam@fpn\endcsname{2}
\expandafter\def\csname res@v5b@combo_hard@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@varlingam@tt\endcsname{0.31}
\expandafter\def\csname res@v5b@combo_hard@varlingam@prec\endcsname{0.18}
\expandafter\def\csname res@v5b@combo_hard@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@varlingam@bw\endcsname{8}
\expandafter\def\csname res@v5b@combo_hard@varlingam@len\endcsname{9.5}
\expandafter\def\csname res@v5b@combo_hard@varlingam@rp\endcsname{0.27}
\expandafter\def\csname res@v5b@combo_hard@varlingam@map\endcsname{0.31}
\expandafter\def\csname res@v5b@combo_hard@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v5b@combo_hard@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v5b@combo_hard@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@spacetime_rule@tt\endcsname{0.27}
\expandafter\def\csname res@v5b@combo_hard@spacetime_rule@prec\endcsname{0.65}
\expandafter\def\csname res@v5b@combo_hard@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v5b@combo_hard@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v5b@combo_hard@spacetime_rule@rp\endcsname{0.34}
\expandafter\def\csname res@v5b@combo_hard@spacetime_rule@map\endcsname{0.46}
\expandafter\def\csname res@v5b@combo_hard@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_hard@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@varsort@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@combo_hard@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@combo_hard@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5b@combo_hard@varsort@rp\endcsname{0.06}
\expandafter\def\csname res@v5b@combo_hard@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@combo_hard@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_hard@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_hard@r2sort@tt\endcsname{0.04}
\expandafter\def\csname res@v5b@combo_hard@r2sort@prec\endcsname{0.03}
\expandafter\def\csname res@v5b@combo_hard@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_hard@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5b@combo_hard@r2sort@rp\endcsname{0.03}
\expandafter\def\csname res@v5b@combo_hard@r2sort@map\endcsname{0.08}
\expandafter\def\csname res@v5b@combo_extreme@correlation@fp\endcsname{2/10}
\expandafter\def\csname res@v5b@combo_extreme@correlation@fpn\endcsname{2}
\expandafter\def\csname res@v5b@combo_extreme@correlation@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@correlation@tt\endcsname{0.19}
\expandafter\def\csname res@v5b@combo_extreme@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v5b@combo_extreme@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@correlation@bw\endcsname{7}
\expandafter\def\csname res@v5b@combo_extreme@correlation@len\endcsname{32.9}
\expandafter\def\csname res@v5b@combo_extreme@correlation@rp\endcsname{0.14}
\expandafter\def\csname res@v5b@combo_extreme@correlation@map\endcsname{0.28}
\expandafter\def\csname res@v5b@combo_extreme@granger@fp\endcsname{5/10}
\expandafter\def\csname res@v5b@combo_extreme@granger@fpn\endcsname{5}
\expandafter\def\csname res@v5b@combo_extreme@granger@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@granger@tt\endcsname{0.23}
\expandafter\def\csname res@v5b@combo_extreme@granger@prec\endcsname{0.08}
\expandafter\def\csname res@v5b@combo_extreme@granger@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@granger@bw\endcsname{1}
\expandafter\def\csname res@v5b@combo_extreme@granger@len\endcsname{25.6}
\expandafter\def\csname res@v5b@combo_extreme@granger@rp\endcsname{0.29}
\expandafter\def\csname res@v5b@combo_extreme@granger@map\endcsname{0.40}
\expandafter\def\csname res@v5b@combo_extreme@pcmciplus@fp\endcsname{2/10}
\expandafter\def\csname res@v5b@combo_extreme@pcmciplus@fpn\endcsname{2}
\expandafter\def\csname res@v5b@combo_extreme@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@pcmciplus@tt\endcsname{0.15}
\expandafter\def\csname res@v5b@combo_extreme@pcmciplus@prec\endcsname{0.31}
\expandafter\def\csname res@v5b@combo_extreme@pcmciplus@ab\endcsname{3}
\expandafter\def\csname res@v5b@combo_extreme@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v5b@combo_extreme@pcmciplus@len\endcsname{1.3}
\expandafter\def\csname res@v5b@combo_extreme@pcmciplus@rp\endcsname{0.51}
\expandafter\def\csname res@v5b@combo_extreme@pcmciplus@map\endcsname{0.58}
\expandafter\def\csname res@v5b@combo_extreme@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5b@combo_extreme@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5b@combo_extreme@pc@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@pc@tt\endcsname{0.19}
\expandafter\def\csname res@v5b@combo_extreme@pc@prec\endcsname{0.15}
\expandafter\def\csname res@v5b@combo_extreme@pc@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@pc@bw\endcsname{6}
\expandafter\def\csname res@v5b@combo_extreme@pc@len\endcsname{2.6}
\expandafter\def\csname res@v5b@combo_extreme@pc@rp\endcsname{0.11}
\expandafter\def\csname res@v5b@combo_extreme@pc@map\endcsname{0.10}
\expandafter\def\csname res@v5b@combo_extreme@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_extreme@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@combo_extreme@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5b@combo_extreme@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5b@combo_extreme@dynotears@rp\endcsname{0.46}
\expandafter\def\csname res@v5b@combo_extreme@dynotears@map\endcsname{0.51}
\expandafter\def\csname res@v5b@combo_extreme@doubleml@fp\endcsname{2/10}
\expandafter\def\csname res@v5b@combo_extreme@doubleml@fpn\endcsname{2}
\expandafter\def\csname res@v5b@combo_extreme@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@doubleml@tt\endcsname{0.12}
\expandafter\def\csname res@v5b@combo_extreme@doubleml@prec\endcsname{0.62}
\expandafter\def\csname res@v5b@combo_extreme@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v5b@combo_extreme@doubleml@bw\endcsname{1}
\expandafter\def\csname res@v5b@combo_extreme@doubleml@len\endcsname{0.5}
\expandafter\def\csname res@v5b@combo_extreme@doubleml@rp\endcsname{0.28}
\expandafter\def\csname res@v5b@combo_extreme@doubleml@map\endcsname{0.41}
\expandafter\def\csname res@v5b@combo_extreme@varlingam@fp\endcsname{2/10}
\expandafter\def\csname res@v5b@combo_extreme@varlingam@fpn\endcsname{2}
\expandafter\def\csname res@v5b@combo_extreme@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@varlingam@tt\endcsname{0.15}
\expandafter\def\csname res@v5b@combo_extreme@varlingam@prec\endcsname{0.13}
\expandafter\def\csname res@v5b@combo_extreme@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@varlingam@bw\endcsname{8}
\expandafter\def\csname res@v5b@combo_extreme@varlingam@len\endcsname{10.2}
\expandafter\def\csname res@v5b@combo_extreme@varlingam@rp\endcsname{0.11}
\expandafter\def\csname res@v5b@combo_extreme@varlingam@map\endcsname{0.26}
\expandafter\def\csname res@v5b@combo_extreme@spacetime_rule@fp\endcsname{2/10}
\expandafter\def\csname res@v5b@combo_extreme@spacetime_rule@fpn\endcsname{2}
\expandafter\def\csname res@v5b@combo_extreme@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@spacetime_rule@tt\endcsname{0.08}
\expandafter\def\csname res@v5b@combo_extreme@spacetime_rule@prec\endcsname{0.11}
\expandafter\def\csname res@v5b@combo_extreme@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v5b@combo_extreme@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v5b@combo_extreme@spacetime_rule@rp\endcsname{0.19}
\expandafter\def\csname res@v5b@combo_extreme@spacetime_rule@map\endcsname{0.24}
\expandafter\def\csname res@v5b@combo_extreme@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_extreme@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@varsort@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@combo_extreme@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@combo_extreme@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5b@combo_extreme@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5b@combo_extreme@varsort@rp\endcsname{0.07}
\expandafter\def\csname res@v5b@combo_extreme@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@combo_extreme@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_extreme@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_extreme@r2sort@tt\endcsname{0.04}
\expandafter\def\csname res@v5b@combo_extreme@r2sort@prec\endcsname{0.03}
\expandafter\def\csname res@v5b@combo_extreme@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_extreme@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5b@combo_extreme@r2sort@rp\endcsname{0.03}
\expandafter\def\csname res@v5b@combo_extreme@r2sort@map\endcsname{0.10}
\expandafter\def\csname res@v5b@interaction_1.0@correlation@fp\endcsname{1/10}
\expandafter\def\csname res@v5b@interaction_1.0@correlation@fpn\endcsname{1}
\expandafter\def\csname res@v5b@interaction_1.0@correlation@n\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@correlation@tt\endcsname{0.15}
\expandafter\def\csname res@v5b@interaction_1.0@correlation@prec\endcsname{0.08}
\expandafter\def\csname res@v5b@interaction_1.0@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@correlation@bw\endcsname{9}
\expandafter\def\csname res@v5b@interaction_1.0@correlation@len\endcsname{14.5}
\expandafter\def\csname res@v5b@interaction_1.0@correlation@rp\endcsname{0.15}
\expandafter\def\csname res@v5b@interaction_1.0@correlation@map\endcsname{0.25}
\expandafter\def\csname res@v5b@interaction_1.0@granger@fp\endcsname{6/10}
\expandafter\def\csname res@v5b@interaction_1.0@granger@fpn\endcsname{6}
\expandafter\def\csname res@v5b@interaction_1.0@granger@n\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@granger@tt\endcsname{0.23}
\expandafter\def\csname res@v5b@interaction_1.0@granger@prec\endcsname{0.16}
\expandafter\def\csname res@v5b@interaction_1.0@granger@ab\endcsname{3}
\expandafter\def\csname res@v5b@interaction_1.0@granger@bw\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@granger@len\endcsname{12.4}
\expandafter\def\csname res@v5b@interaction_1.0@granger@rp\endcsname{0.35}
\expandafter\def\csname res@v5b@interaction_1.0@granger@map\endcsname{0.45}
\expandafter\def\csname res@v5b@interaction_1.0@pcmciplus@fp\endcsname{6/10}
\expandafter\def\csname res@v5b@interaction_1.0@pcmciplus@fpn\endcsname{6}
\expandafter\def\csname res@v5b@interaction_1.0@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@pcmciplus@tt\endcsname{0.31}
\expandafter\def\csname res@v5b@interaction_1.0@pcmciplus@prec\endcsname{0.37}
\expandafter\def\csname res@v5b@interaction_1.0@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v5b@interaction_1.0@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@pcmciplus@len\endcsname{1.8}
\expandafter\def\csname res@v5b@interaction_1.0@pcmciplus@rp\endcsname{0.49}
\expandafter\def\csname res@v5b@interaction_1.0@pcmciplus@map\endcsname{0.55}
\expandafter\def\csname res@v5b@interaction_1.0@pc@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@interaction_1.0@pc@fpn\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@pc@n\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@pc@tt\endcsname{0.08}
\expandafter\def\csname res@v5b@interaction_1.0@pc@prec\endcsname{0.06}
\expandafter\def\csname res@v5b@interaction_1.0@pc@ab\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@pc@bw\endcsname{4}
\expandafter\def\csname res@v5b@interaction_1.0@pc@len\endcsname{4.3}
\expandafter\def\csname res@v5b@interaction_1.0@pc@rp\endcsname{0.06}
\expandafter\def\csname res@v5b@interaction_1.0@pc@map\endcsname{0.09}
\expandafter\def\csname res@v5b@interaction_1.0@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@interaction_1.0@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@interaction_1.0@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5b@interaction_1.0@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5b@interaction_1.0@dynotears@rp\endcsname{0.37}
\expandafter\def\csname res@v5b@interaction_1.0@dynotears@map\endcsname{0.50}
\expandafter\def\csname res@v5b@interaction_1.0@doubleml@fp\endcsname{2/10}
\expandafter\def\csname res@v5b@interaction_1.0@doubleml@fpn\endcsname{2}
\expandafter\def\csname res@v5b@interaction_1.0@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@doubleml@tt\endcsname{0.08}
\expandafter\def\csname res@v5b@interaction_1.0@doubleml@prec\endcsname{0.50}
\expandafter\def\csname res@v5b@interaction_1.0@doubleml@ab\endcsname{7}
\expandafter\def\csname res@v5b@interaction_1.0@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@doubleml@len\endcsname{0.4}
\expandafter\def\csname res@v5b@interaction_1.0@doubleml@rp\endcsname{0.35}
\expandafter\def\csname res@v5b@interaction_1.0@doubleml@map\endcsname{0.30}
\expandafter\def\csname res@v5b@interaction_1.0@varlingam@fp\endcsname{4/10}
\expandafter\def\csname res@v5b@interaction_1.0@varlingam@fpn\endcsname{4}
\expandafter\def\csname res@v5b@interaction_1.0@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@varlingam@tt\endcsname{0.27}
\expandafter\def\csname res@v5b@interaction_1.0@varlingam@prec\endcsname{0.32}
\expandafter\def\csname res@v5b@interaction_1.0@varlingam@ab\endcsname{2}
\expandafter\def\csname res@v5b@interaction_1.0@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v5b@interaction_1.0@varlingam@len\endcsname{5.2}
\expandafter\def\csname res@v5b@interaction_1.0@varlingam@rp\endcsname{0.30}
\expandafter\def\csname res@v5b@interaction_1.0@varlingam@map\endcsname{0.42}
\expandafter\def\csname res@v5b@interaction_1.0@spacetime_rule@fp\endcsname{10/10}
\expandafter\def\csname res@v5b@interaction_1.0@spacetime_rule@fpn\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@spacetime_rule@tt\endcsname{0.62}
\expandafter\def\csname res@v5b@interaction_1.0@spacetime_rule@prec\endcsname{0.95}
\expandafter\def\csname res@v5b@interaction_1.0@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@spacetime_rule@len\endcsname{1.7}
\expandafter\def\csname res@v5b@interaction_1.0@spacetime_rule@rp\endcsname{0.77}
\expandafter\def\csname res@v5b@interaction_1.0@spacetime_rule@map\endcsname{0.83}
\expandafter\def\csname res@v5b@interaction_1.0@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@interaction_1.0@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@varsort@n\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@interaction_1.0@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@interaction_1.0@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@varsort@bw\endcsname{2}
\expandafter\def\csname res@v5b@interaction_1.0@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5b@interaction_1.0@varsort@rp\endcsname{0.05}
\expandafter\def\csname res@v5b@interaction_1.0@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@interaction_1.0@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@interaction_1.0@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5b@interaction_1.0@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@interaction_1.0@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@interaction_1.0@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5b@interaction_1.0@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5b@interaction_1.0@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v5b@interaction_1.0@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@combo_interaction@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_interaction@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@correlation@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@correlation@tt\endcsname{0.08}
\expandafter\def\csname res@v5b@combo_interaction@correlation@prec\endcsname{0.06}
\expandafter\def\csname res@v5b@combo_interaction@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@correlation@bw\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@correlation@len\endcsname{8.9}
\expandafter\def\csname res@v5b@combo_interaction@correlation@rp\endcsname{0.05}
\expandafter\def\csname res@v5b@combo_interaction@correlation@map\endcsname{0.18}
\expandafter\def\csname res@v5b@combo_interaction@granger@fp\endcsname{5/10}
\expandafter\def\csname res@v5b@combo_interaction@granger@fpn\endcsname{5}
\expandafter\def\csname res@v5b@combo_interaction@granger@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@granger@tt\endcsname{0.23}
\expandafter\def\csname res@v5b@combo_interaction@granger@prec\endcsname{0.16}
\expandafter\def\csname res@v5b@combo_interaction@granger@ab\endcsname{3}
\expandafter\def\csname res@v5b@combo_interaction@granger@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@granger@len\endcsname{9.1}
\expandafter\def\csname res@v5b@combo_interaction@granger@rp\endcsname{0.27}
\expandafter\def\csname res@v5b@combo_interaction@granger@map\endcsname{0.36}
\expandafter\def\csname res@v5b@combo_interaction@pcmciplus@fp\endcsname{1/10}
\expandafter\def\csname res@v5b@combo_interaction@pcmciplus@fpn\endcsname{1}
\expandafter\def\csname res@v5b@combo_interaction@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@pcmciplus@tt\endcsname{0.12}
\expandafter\def\csname res@v5b@combo_interaction@pcmciplus@prec\endcsname{0.23}
\expandafter\def\csname res@v5b@combo_interaction@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v5b@combo_interaction@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v5b@combo_interaction@pcmciplus@len\endcsname{1.6}
\expandafter\def\csname res@v5b@combo_interaction@pcmciplus@rp\endcsname{0.14}
\expandafter\def\csname res@v5b@combo_interaction@pcmciplus@map\endcsname{0.24}
\expandafter\def\csname res@v5b@combo_interaction@pc@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_interaction@pc@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@pc@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@pc@tt\endcsname{0.08}
\expandafter\def\csname res@v5b@combo_interaction@pc@prec\endcsname{0.07}
\expandafter\def\csname res@v5b@combo_interaction@pc@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@pc@bw\endcsname{8}
\expandafter\def\csname res@v5b@combo_interaction@pc@len\endcsname{2.6}
\expandafter\def\csname res@v5b@combo_interaction@pc@rp\endcsname{0.09}
\expandafter\def\csname res@v5b@combo_interaction@pc@map\endcsname{0.12}
\expandafter\def\csname res@v5b@combo_interaction@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_interaction@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@combo_interaction@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5b@combo_interaction@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5b@combo_interaction@dynotears@rp\endcsname{0.25}
\expandafter\def\csname res@v5b@combo_interaction@dynotears@map\endcsname{0.38}
\expandafter\def\csname res@v5b@combo_interaction@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v5b@combo_interaction@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v5b@combo_interaction@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v5b@combo_interaction@doubleml@prec\endcsname{0.25}
\expandafter\def\csname res@v5b@combo_interaction@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v5b@combo_interaction@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@doubleml@len\endcsname{0.4}
\expandafter\def\csname res@v5b@combo_interaction@doubleml@rp\endcsname{0.17}
\expandafter\def\csname res@v5b@combo_interaction@doubleml@map\endcsname{0.23}
\expandafter\def\csname res@v5b@combo_interaction@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_interaction@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@varlingam@tt\endcsname{0.23}
\expandafter\def\csname res@v5b@combo_interaction@varlingam@prec\endcsname{0.17}
\expandafter\def\csname res@v5b@combo_interaction@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@varlingam@bw\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@varlingam@len\endcsname{5.0}
\expandafter\def\csname res@v5b@combo_interaction@varlingam@rp\endcsname{0.15}
\expandafter\def\csname res@v5b@combo_interaction@varlingam@map\endcsname{0.19}
\expandafter\def\csname res@v5b@combo_interaction@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v5b@combo_interaction@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v5b@combo_interaction@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v5b@combo_interaction@spacetime_rule@prec\endcsname{0.63}
\expandafter\def\csname res@v5b@combo_interaction@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v5b@combo_interaction@spacetime_rule@rp\endcsname{0.40}
\expandafter\def\csname res@v5b@combo_interaction@spacetime_rule@map\endcsname{0.47}
\expandafter\def\csname res@v5b@combo_interaction@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_interaction@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@varsort@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@combo_interaction@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@combo_interaction@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@varsort@bw\endcsname{3}
\expandafter\def\csname res@v5b@combo_interaction@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5b@combo_interaction@varsort@rp\endcsname{0.06}
\expandafter\def\csname res@v5b@combo_interaction@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v5b@combo_interaction@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@combo_interaction@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5b@combo_interaction@r2sort@tt\endcsname{0.04}
\expandafter\def\csname res@v5b@combo_interaction@r2sort@prec\endcsname{0.03}
\expandafter\def\csname res@v5b@combo_interaction@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5b@combo_interaction@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5b@combo_interaction@r2sort@rp\endcsname{0.03}
\expandafter\def\csname res@v5b@combo_interaction@r2sort@map\endcsname{0.08}
\expandafter\def\csname res@v5b@control_weak@correlation@fp\endcsname{3/10}
\expandafter\def\csname res@v5b@control_weak@correlation@fpn\endcsname{3}
\expandafter\def\csname res@v5b@control_weak@correlation@n\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@correlation@tt\endcsname{0.35}
\expandafter\def\csname res@v5b@control_weak@correlation@prec\endcsname{0.09}
\expandafter\def\csname res@v5b@control_weak@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@correlation@bw\endcsname{7}
\expandafter\def\csname res@v5b@control_weak@correlation@len\endcsname{22.2}
\expandafter\def\csname res@v5b@control_weak@correlation@rp\endcsname{0.28}
\expandafter\def\csname res@v5b@control_weak@correlation@map\endcsname{0.39}
\expandafter\def\csname res@v5b@control_weak@granger@fp\endcsname{6/10}
\expandafter\def\csname res@v5b@control_weak@granger@fpn\endcsname{6}
\expandafter\def\csname res@v5b@control_weak@granger@n\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@granger@tt\endcsname{0.46}
\expandafter\def\csname res@v5b@control_weak@granger@prec\endcsname{0.23}
\expandafter\def\csname res@v5b@control_weak@granger@ab\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@granger@bw\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@granger@len\endcsname{13.0}
\expandafter\def\csname res@v5b@control_weak@granger@rp\endcsname{0.41}
\expandafter\def\csname res@v5b@control_weak@granger@map\endcsname{0.51}
\expandafter\def\csname res@v5b@control_weak@pcmciplus@fp\endcsname{8/10}
\expandafter\def\csname res@v5b@control_weak@pcmciplus@fpn\endcsname{8}
\expandafter\def\csname res@v5b@control_weak@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@pcmciplus@tt\endcsname{0.38}
\expandafter\def\csname res@v5b@control_weak@pcmciplus@prec\endcsname{0.56}
\expandafter\def\csname res@v5b@control_weak@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@pcmciplus@len\endcsname{2.3}
\expandafter\def\csname res@v5b@control_weak@pcmciplus@rp\endcsname{0.70}
\expandafter\def\csname res@v5b@control_weak@pcmciplus@map\endcsname{0.78}
\expandafter\def\csname res@v5b@control_weak@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v5b@control_weak@pc@fpn\endcsname{4}
\expandafter\def\csname res@v5b@control_weak@pc@n\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v5b@control_weak@pc@prec\endcsname{0.22}
\expandafter\def\csname res@v5b@control_weak@pc@ab\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@pc@bw\endcsname{3}
\expandafter\def\csname res@v5b@control_weak@pc@len\endcsname{3.9}
\expandafter\def\csname res@v5b@control_weak@pc@rp\endcsname{0.22}
\expandafter\def\csname res@v5b@control_weak@pc@map\endcsname{0.15}
\expandafter\def\csname res@v5b@control_weak@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@control_weak@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@control_weak@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5b@control_weak@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5b@control_weak@dynotears@rp\endcsname{0.70}
\expandafter\def\csname res@v5b@control_weak@dynotears@map\endcsname{0.79}
\expandafter\def\csname res@v5b@control_weak@doubleml@fp\endcsname{6/10}
\expandafter\def\csname res@v5b@control_weak@doubleml@fpn\endcsname{6}
\expandafter\def\csname res@v5b@control_weak@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@doubleml@tt\endcsname{0.35}
\expandafter\def\csname res@v5b@control_weak@doubleml@prec\endcsname{0.74}
\expandafter\def\csname res@v5b@control_weak@doubleml@ab\endcsname{3}
\expandafter\def\csname res@v5b@control_weak@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@doubleml@len\endcsname{1.2}
\expandafter\def\csname res@v5b@control_weak@doubleml@rp\endcsname{0.44}
\expandafter\def\csname res@v5b@control_weak@doubleml@map\endcsname{0.53}
\expandafter\def\csname res@v5b@control_weak@varlingam@fp\endcsname{5/10}
\expandafter\def\csname res@v5b@control_weak@varlingam@fpn\endcsname{5}
\expandafter\def\csname res@v5b@control_weak@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@varlingam@tt\endcsname{0.42}
\expandafter\def\csname res@v5b@control_weak@varlingam@prec\endcsname{0.32}
\expandafter\def\csname res@v5b@control_weak@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@varlingam@bw\endcsname{4}
\expandafter\def\csname res@v5b@control_weak@varlingam@len\endcsname{5.4}
\expandafter\def\csname res@v5b@control_weak@varlingam@rp\endcsname{0.40}
\expandafter\def\csname res@v5b@control_weak@varlingam@map\endcsname{0.44}
\expandafter\def\csname res@v5b@control_weak@spacetime_rule@fp\endcsname{3/10}
\expandafter\def\csname res@v5b@control_weak@spacetime_rule@fpn\endcsname{3}
\expandafter\def\csname res@v5b@control_weak@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@spacetime_rule@tt\endcsname{0.12}
\expandafter\def\csname res@v5b@control_weak@spacetime_rule@prec\endcsname{0.38}
\expandafter\def\csname res@v5b@control_weak@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v5b@control_weak@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@spacetime_rule@len\endcsname{0.8}
\expandafter\def\csname res@v5b@control_weak@spacetime_rule@rp\endcsname{0.23}
\expandafter\def\csname res@v5b@control_weak@spacetime_rule@map\endcsname{0.34}
\expandafter\def\csname res@v5b@control_weak@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@control_weak@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@varsort@n\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@control_weak@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@control_weak@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@varsort@bw\endcsname{3}
\expandafter\def\csname res@v5b@control_weak@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v5b@control_weak@varsort@rp\endcsname{0.06}
\expandafter\def\csname res@v5b@control_weak@varsort@map\endcsname{0.08}
\expandafter\def\csname res@v5b@control_weak@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5b@control_weak@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5b@control_weak@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v5b@control_weak@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v5b@control_weak@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5b@control_weak@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5b@control_weak@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v5b@control_weak@r2sort@map\endcsname{0.11}
\expandafter\def\csname res@v5d@default_b25@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@default_b25@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v5d@default_b25@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b25@correlation@tt\endcsname{0.69}
\expandafter\def\csname res@v5d@default_b25@correlation@prec\endcsname{0.20}
\expandafter\def\csname res@v5d@default_b25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@correlation@bw\endcsname{1}
\expandafter\def\csname res@v5d@default_b25@correlation@len\endcsname{12.2}
\expandafter\def\csname res@v5d@default_b25@correlation@rp\endcsname{0.73}
\expandafter\def\csname res@v5d@default_b25@correlation@map\endcsname{0.80}
\expandafter\def\csname res@v5d@default_b25@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@default_b25@granger@fpn\endcsname{9}
\expandafter\def\csname res@v5d@default_b25@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b25@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@default_b25@granger@prec\endcsname{0.48}
\expandafter\def\csname res@v5d@default_b25@granger@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@granger@len\endcsname{5.0}
\expandafter\def\csname res@v5d@default_b25@granger@rp\endcsname{0.62}
\expandafter\def\csname res@v5d@default_b25@granger@map\endcsname{0.70}
\expandafter\def\csname res@v5d@default_b25@pcmciplus@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@default_b25@pcmciplus@fpn\endcsname{7}
\expandafter\def\csname res@v5d@default_b25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b25@pcmciplus@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@default_b25@pcmciplus@prec\endcsname{0.65}
\expandafter\def\csname res@v5d@default_b25@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v5d@default_b25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@pcmciplus@len\endcsname{1.6}
\expandafter\def\csname res@v5d@default_b25@pcmciplus@rp\endcsname{0.73}
\expandafter\def\csname res@v5d@default_b25@pcmciplus@map\endcsname{0.81}
\expandafter\def\csname res@v5d@default_b25@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@default_b25@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5d@default_b25@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b25@pc@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@default_b25@pc@prec\endcsname{0.45}
\expandafter\def\csname res@v5d@default_b25@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@pc@bw\endcsname{3}
\expandafter\def\csname res@v5d@default_b25@pc@len\endcsname{4.0}
\expandafter\def\csname res@v5d@default_b25@pc@rp\endcsname{0.42}
\expandafter\def\csname res@v5d@default_b25@pc@map\endcsname{0.39}
\expandafter\def\csname res@v5d@default_b25@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@default_b25@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v5d@default_b25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b25@dynotears@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@default_b25@dynotears@prec\endcsname{0.92}
\expandafter\def\csname res@v5d@default_b25@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v5d@default_b25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v5d@default_b25@dynotears@rp\endcsname{0.82}
\expandafter\def\csname res@v5d@default_b25@dynotears@map\endcsname{0.88}
\expandafter\def\csname res@v5d@default_b25@doubleml@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@default_b25@doubleml@fpn\endcsname{6}
\expandafter\def\csname res@v5d@default_b25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b25@doubleml@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@default_b25@doubleml@prec\endcsname{0.60}
\expandafter\def\csname res@v5d@default_b25@doubleml@ab\endcsname{2}
\expandafter\def\csname res@v5d@default_b25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@doubleml@len\endcsname{1.9}
\expandafter\def\csname res@v5d@default_b25@doubleml@rp\endcsname{0.50}
\expandafter\def\csname res@v5d@default_b25@doubleml@map\endcsname{0.61}
\expandafter\def\csname res@v5d@default_b25@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@default_b25@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v5d@default_b25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b25@varlingam@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@default_b25@varlingam@prec\endcsname{0.42}
\expandafter\def\csname res@v5d@default_b25@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v5d@default_b25@varlingam@len\endcsname{4.7}
\expandafter\def\csname res@v5d@default_b25@varlingam@rp\endcsname{0.54}
\expandafter\def\csname res@v5d@default_b25@varlingam@map\endcsname{0.67}
\expandafter\def\csname res@v5d@default_b25@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@default_b25@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v5d@default_b25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b25@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@default_b25@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@default_b25@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v5d@default_b25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v5d@default_b25@spacetime_rule@rp\endcsname{0.62}
\expandafter\def\csname res@v5d@default_b25@spacetime_rule@map\endcsname{0.73}
\expandafter\def\csname res@v5d@default_b25@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@default_b25@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@default_b25@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b25@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@default_b25@varsort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@default_b25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v5d@default_b25@varsort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@default_b25@varsort@map\endcsname{0.18}
\expandafter\def\csname res@v5d@default_b25@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@default_b25@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@default_b25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b25@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@default_b25@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@default_b25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b25@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v5d@default_b25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@default_b25@r2sort@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@default_b25@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v5d@signal_0.1_b25@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@signal_0.1_b25@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@correlation@tt\endcsname{0.35}
\expandafter\def\csname res@v5d@signal_0.1_b25@correlation@prec\endcsname{0.24}
\expandafter\def\csname res@v5d@signal_0.1_b25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@correlation@bw\endcsname{9}
\expandafter\def\csname res@v5d@signal_0.1_b25@correlation@len\endcsname{4.6}
\expandafter\def\csname res@v5d@signal_0.1_b25@correlation@rp\endcsname{0.22}
\expandafter\def\csname res@v5d@signal_0.1_b25@correlation@map\endcsname{0.34}
\expandafter\def\csname res@v5d@signal_0.1_b25@granger@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@signal_0.1_b25@granger@fpn\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b25@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@granger@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@signal_0.1_b25@granger@prec\endcsname{0.50}
\expandafter\def\csname res@v5d@signal_0.1_b25@granger@ab\endcsname{8}
\expandafter\def\csname res@v5d@signal_0.1_b25@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@granger@len\endcsname{0.3}
\expandafter\def\csname res@v5d@signal_0.1_b25@granger@rp\endcsname{0.27}
\expandafter\def\csname res@v5d@signal_0.1_b25@granger@map\endcsname{0.37}
\expandafter\def\csname res@v5d@signal_0.1_b25@pcmciplus@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@signal_0.1_b25@pcmciplus@fpn\endcsname{5}
\expandafter\def\csname res@v5d@signal_0.1_b25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@pcmciplus@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@signal_0.1_b25@pcmciplus@prec\endcsname{0.94}
\expandafter\def\csname res@v5d@signal_0.1_b25@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v5d@signal_0.1_b25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@pcmciplus@len\endcsname{0.8}
\expandafter\def\csname res@v5d@signal_0.1_b25@pcmciplus@rp\endcsname{0.30}
\expandafter\def\csname res@v5d@signal_0.1_b25@pcmciplus@map\endcsname{0.41}
\expandafter\def\csname res@v5d@signal_0.1_b25@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@signal_0.1_b25@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5d@signal_0.1_b25@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@pc@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@signal_0.1_b25@pc@prec\endcsname{0.14}
\expandafter\def\csname res@v5d@signal_0.1_b25@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@pc@bw\endcsname{7}
\expandafter\def\csname res@v5d@signal_0.1_b25@pc@len\endcsname{2.4}
\expandafter\def\csname res@v5d@signal_0.1_b25@pc@rp\endcsname{0.15}
\expandafter\def\csname res@v5d@signal_0.1_b25@pc@map\endcsname{0.17}
\expandafter\def\csname res@v5d@signal_0.1_b25@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@signal_0.1_b25@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@signal_0.1_b25@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@signal_0.1_b25@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@signal_0.1_b25@dynotears@rp\endcsname{0.29}
\expandafter\def\csname res@v5d@signal_0.1_b25@dynotears@map\endcsname{0.41}
\expandafter\def\csname res@v5d@signal_0.1_b25@doubleml@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@signal_0.1_b25@doubleml@fpn\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@doubleml@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@signal_0.1_b25@doubleml@prec\endcsname{0.00}
\expandafter\def\csname res@v5d@signal_0.1_b25@doubleml@ab\endcsname{5}
\expandafter\def\csname res@v5d@signal_0.1_b25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@doubleml@len\endcsname{0.7}
\expandafter\def\csname res@v5d@signal_0.1_b25@doubleml@rp\endcsname{0.06}
\expandafter\def\csname res@v5d@signal_0.1_b25@doubleml@map\endcsname{0.18}
\expandafter\def\csname res@v5d@signal_0.1_b25@varlingam@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@signal_0.1_b25@varlingam@fpn\endcsname{2}
\expandafter\def\csname res@v5d@signal_0.1_b25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@varlingam@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@signal_0.1_b25@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v5d@signal_0.1_b25@varlingam@ab\endcsname{6}
\expandafter\def\csname res@v5d@signal_0.1_b25@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b25@varlingam@len\endcsname{1.5}
\expandafter\def\csname res@v5d@signal_0.1_b25@varlingam@rp\endcsname{0.30}
\expandafter\def\csname res@v5d@signal_0.1_b25@varlingam@map\endcsname{0.42}
\expandafter\def\csname res@v5d@signal_0.1_b25@spacetime_rule@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@signal_0.1_b25@spacetime_rule@fpn\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@spacetime_rule@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@signal_0.1_b25@spacetime_rule@prec\endcsname{0.00}
\expandafter\def\csname res@v5d@signal_0.1_b25@spacetime_rule@ab\endcsname{5}
\expandafter\def\csname res@v5d@signal_0.1_b25@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b25@spacetime_rule@len\endcsname{0.7}
\expandafter\def\csname res@v5d@signal_0.1_b25@spacetime_rule@rp\endcsname{0.17}
\expandafter\def\csname res@v5d@signal_0.1_b25@spacetime_rule@map\endcsname{0.25}
\expandafter\def\csname res@v5d@signal_0.1_b25@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@signal_0.1_b25@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b25@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@signal_0.1_b25@varsort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@signal_0.1_b25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@signal_0.1_b25@varsort@rp\endcsname{0.09}
\expandafter\def\csname res@v5d@signal_0.1_b25@varsort@map\endcsname{0.19}
\expandafter\def\csname res@v5d@signal_0.1_b25@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@signal_0.1_b25@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b25@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@signal_0.1_b25@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@signal_0.1_b25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b25@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v5d@signal_0.1_b25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@signal_0.1_b25@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v5d@signal_0.1_b25@r2sort@map\endcsname{0.22}
\expandafter\def\csname res@v5d@echo_0.8_b25@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v5d@echo_0.8_b25@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@correlation@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@echo_0.8_b25@correlation@prec\endcsname{0.18}
\expandafter\def\csname res@v5d@echo_0.8_b25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@correlation@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@correlation@len\endcsname{14.3}
\expandafter\def\csname res@v5d@echo_0.8_b25@correlation@rp\endcsname{0.51}
\expandafter\def\csname res@v5d@echo_0.8_b25@correlation@map\endcsname{0.70}
\expandafter\def\csname res@v5d@echo_0.8_b25@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@echo_0.8_b25@granger@fpn\endcsname{8}
\expandafter\def\csname res@v5d@echo_0.8_b25@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@echo_0.8_b25@granger@prec\endcsname{0.35}
\expandafter\def\csname res@v5d@echo_0.8_b25@granger@ab\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b25@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@granger@len\endcsname{6.4}
\expandafter\def\csname res@v5d@echo_0.8_b25@granger@rp\endcsname{0.58}
\expandafter\def\csname res@v5d@echo_0.8_b25@granger@map\endcsname{0.70}
\expandafter\def\csname res@v5d@echo_0.8_b25@pcmciplus@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@echo_0.8_b25@pcmciplus@fpn\endcsname{6}
\expandafter\def\csname res@v5d@echo_0.8_b25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@pcmciplus@tt\endcsname{0.31}
\expandafter\def\csname res@v5d@echo_0.8_b25@pcmciplus@prec\endcsname{0.56}
\expandafter\def\csname res@v5d@echo_0.8_b25@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@pcmciplus@len\endcsname{1.5}
\expandafter\def\csname res@v5d@echo_0.8_b25@pcmciplus@rp\endcsname{0.68}
\expandafter\def\csname res@v5d@echo_0.8_b25@pcmciplus@map\endcsname{0.71}
\expandafter\def\csname res@v5d@echo_0.8_b25@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@echo_0.8_b25@pc@fpn\endcsname{4}
\expandafter\def\csname res@v5d@echo_0.8_b25@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@pc@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@echo_0.8_b25@pc@prec\endcsname{0.47}
\expandafter\def\csname res@v5d@echo_0.8_b25@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@pc@bw\endcsname{3}
\expandafter\def\csname res@v5d@echo_0.8_b25@pc@len\endcsname{3.1}
\expandafter\def\csname res@v5d@echo_0.8_b25@pc@rp\endcsname{0.31}
\expandafter\def\csname res@v5d@echo_0.8_b25@pc@map\endcsname{0.36}
\expandafter\def\csname res@v5d@echo_0.8_b25@dynotears@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@echo_0.8_b25@dynotears@fpn\endcsname{5}
\expandafter\def\csname res@v5d@echo_0.8_b25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@dynotears@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@echo_0.8_b25@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@echo_0.8_b25@dynotears@ab\endcsname{5}
\expandafter\def\csname res@v5d@echo_0.8_b25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@dynotears@len\endcsname{0.5}
\expandafter\def\csname res@v5d@echo_0.8_b25@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v5d@echo_0.8_b25@dynotears@map\endcsname{0.89}
\expandafter\def\csname res@v5d@echo_0.8_b25@doubleml@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@echo_0.8_b25@doubleml@fpn\endcsname{5}
\expandafter\def\csname res@v5d@echo_0.8_b25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@doubleml@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@echo_0.8_b25@doubleml@prec\endcsname{0.67}
\expandafter\def\csname res@v5d@echo_0.8_b25@doubleml@ab\endcsname{3}
\expandafter\def\csname res@v5d@echo_0.8_b25@doubleml@bw\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b25@doubleml@len\endcsname{1.0}
\expandafter\def\csname res@v5d@echo_0.8_b25@doubleml@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@echo_0.8_b25@doubleml@map\endcsname{0.48}
\expandafter\def\csname res@v5d@echo_0.8_b25@varlingam@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@echo_0.8_b25@varlingam@fpn\endcsname{6}
\expandafter\def\csname res@v5d@echo_0.8_b25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@varlingam@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@echo_0.8_b25@varlingam@prec\endcsname{0.26}
\expandafter\def\csname res@v5d@echo_0.8_b25@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b25@varlingam@len\endcsname{7.4}
\expandafter\def\csname res@v5d@echo_0.8_b25@varlingam@rp\endcsname{0.50}
\expandafter\def\csname res@v5d@echo_0.8_b25@varlingam@map\endcsname{0.57}
\expandafter\def\csname res@v5d@echo_0.8_b25@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@echo_0.8_b25@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v5d@echo_0.8_b25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@spacetime_rule@tt\endcsname{0.35}
\expandafter\def\csname res@v5d@echo_0.8_b25@spacetime_rule@prec\endcsname{0.72}
\expandafter\def\csname res@v5d@echo_0.8_b25@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b25@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b25@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v5d@echo_0.8_b25@spacetime_rule@rp\endcsname{0.57}
\expandafter\def\csname res@v5d@echo_0.8_b25@spacetime_rule@map\endcsname{0.68}
\expandafter\def\csname res@v5d@echo_0.8_b25@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@echo_0.8_b25@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@echo_0.8_b25@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v5d@echo_0.8_b25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b25@varsort@len\endcsname{2.6}
\expandafter\def\csname res@v5d@echo_0.8_b25@varsort@rp\endcsname{0.06}
\expandafter\def\csname res@v5d@echo_0.8_b25@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v5d@echo_0.8_b25@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@echo_0.8_b25@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b25@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@echo_0.8_b25@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@echo_0.8_b25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b25@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v5d@echo_0.8_b25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@echo_0.8_b25@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@echo_0.8_b25@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5d@confound_0.8_b25@correlation@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@confound_0.8_b25@correlation@fpn\endcsname{6}
\expandafter\def\csname res@v5d@confound_0.8_b25@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b25@correlation@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@confound_0.8_b25@correlation@prec\endcsname{0.16}
\expandafter\def\csname res@v5d@confound_0.8_b25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@correlation@bw\endcsname{3}
\expandafter\def\csname res@v5d@confound_0.8_b25@correlation@len\endcsname{14.5}
\expandafter\def\csname res@v5d@confound_0.8_b25@correlation@rp\endcsname{0.47}
\expandafter\def\csname res@v5d@confound_0.8_b25@correlation@map\endcsname{0.55}
\expandafter\def\csname res@v5d@confound_0.8_b25@granger@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@confound_0.8_b25@granger@fpn\endcsname{7}
\expandafter\def\csname res@v5d@confound_0.8_b25@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b25@granger@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@confound_0.8_b25@granger@prec\endcsname{0.29}
\expandafter\def\csname res@v5d@confound_0.8_b25@granger@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@granger@len\endcsname{8.3}
\expandafter\def\csname res@v5d@confound_0.8_b25@granger@rp\endcsname{0.58}
\expandafter\def\csname res@v5d@confound_0.8_b25@granger@map\endcsname{0.64}
\expandafter\def\csname res@v5d@confound_0.8_b25@pcmciplus@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@confound_0.8_b25@pcmciplus@fpn\endcsname{3}
\expandafter\def\csname res@v5d@confound_0.8_b25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b25@pcmciplus@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@confound_0.8_b25@pcmciplus@prec\endcsname{0.44}
\expandafter\def\csname res@v5d@confound_0.8_b25@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v5d@confound_0.8_b25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@pcmciplus@len\endcsname{0.8}
\expandafter\def\csname res@v5d@confound_0.8_b25@pcmciplus@rp\endcsname{0.52}
\expandafter\def\csname res@v5d@confound_0.8_b25@pcmciplus@map\endcsname{0.61}
\expandafter\def\csname res@v5d@confound_0.8_b25@pc@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@confound_0.8_b25@pc@fpn\endcsname{5}
\expandafter\def\csname res@v5d@confound_0.8_b25@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b25@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@confound_0.8_b25@pc@prec\endcsname{0.53}
\expandafter\def\csname res@v5d@confound_0.8_b25@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@pc@bw\endcsname{1}
\expandafter\def\csname res@v5d@confound_0.8_b25@pc@len\endcsname{3.0}
\expandafter\def\csname res@v5d@confound_0.8_b25@pc@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@confound_0.8_b25@pc@map\endcsname{0.37}
\expandafter\def\csname res@v5d@confound_0.8_b25@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@confound_0.8_b25@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v5d@confound_0.8_b25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b25@dynotears@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@confound_0.8_b25@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@confound_0.8_b25@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v5d@confound_0.8_b25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@dynotears@len\endcsname{0.4}
\expandafter\def\csname res@v5d@confound_0.8_b25@dynotears@rp\endcsname{0.76}
\expandafter\def\csname res@v5d@confound_0.8_b25@dynotears@map\endcsname{0.82}
\expandafter\def\csname res@v5d@confound_0.8_b25@doubleml@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@confound_0.8_b25@doubleml@fpn\endcsname{3}
\expandafter\def\csname res@v5d@confound_0.8_b25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b25@doubleml@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@confound_0.8_b25@doubleml@prec\endcsname{0.39}
\expandafter\def\csname res@v5d@confound_0.8_b25@doubleml@ab\endcsname{4}
\expandafter\def\csname res@v5d@confound_0.8_b25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@doubleml@len\endcsname{1.8}
\expandafter\def\csname res@v5d@confound_0.8_b25@doubleml@rp\endcsname{0.45}
\expandafter\def\csname res@v5d@confound_0.8_b25@doubleml@map\endcsname{0.59}
\expandafter\def\csname res@v5d@confound_0.8_b25@varlingam@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@confound_0.8_b25@varlingam@fpn\endcsname{7}
\expandafter\def\csname res@v5d@confound_0.8_b25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b25@varlingam@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@confound_0.8_b25@varlingam@prec\endcsname{0.40}
\expandafter\def\csname res@v5d@confound_0.8_b25@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v5d@confound_0.8_b25@varlingam@len\endcsname{5.2}
\expandafter\def\csname res@v5d@confound_0.8_b25@varlingam@rp\endcsname{0.68}
\expandafter\def\csname res@v5d@confound_0.8_b25@varlingam@map\endcsname{0.70}
\expandafter\def\csname res@v5d@confound_0.8_b25@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@confound_0.8_b25@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v5d@confound_0.8_b25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b25@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v5d@confound_0.8_b25@spacetime_rule@prec\endcsname{0.70}
\expandafter\def\csname res@v5d@confound_0.8_b25@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v5d@confound_0.8_b25@spacetime_rule@rp\endcsname{0.53}
\expandafter\def\csname res@v5d@confound_0.8_b25@spacetime_rule@map\endcsname{0.62}
\expandafter\def\csname res@v5d@confound_0.8_b25@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@confound_0.8_b25@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v5d@confound_0.8_b25@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b25@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@confound_0.8_b25@varsort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@confound_0.8_b25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@varsort@bw\endcsname{2}
\expandafter\def\csname res@v5d@confound_0.8_b25@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@confound_0.8_b25@varsort@rp\endcsname{0.06}
\expandafter\def\csname res@v5d@confound_0.8_b25@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v5d@confound_0.8_b25@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@confound_0.8_b25@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@confound_0.8_b25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b25@r2sort@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@confound_0.8_b25@r2sort@prec\endcsname{0.05}
\expandafter\def\csname res@v5d@confound_0.8_b25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b25@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v5d@confound_0.8_b25@r2sort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@confound_0.8_b25@r2sort@rp\endcsname{0.05}
\expandafter\def\csname res@v5d@confound_0.8_b25@r2sort@map\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_hard_b25@correlation@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@combo_hard_b25@correlation@fpn\endcsname{5}
\expandafter\def\csname res@v5d@combo_hard_b25@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@correlation@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@combo_hard_b25@correlation@prec\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_hard_b25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@correlation@bw\endcsname{5}
\expandafter\def\csname res@v5d@combo_hard_b25@correlation@len\endcsname{11.8}
\expandafter\def\csname res@v5d@combo_hard_b25@correlation@rp\endcsname{0.37}
\expandafter\def\csname res@v5d@combo_hard_b25@correlation@map\endcsname{0.54}
\expandafter\def\csname res@v5d@combo_hard_b25@granger@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_hard_b25@granger@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_hard_b25@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@granger@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@combo_hard_b25@granger@prec\endcsname{0.40}
\expandafter\def\csname res@v5d@combo_hard_b25@granger@ab\endcsname{3}
\expandafter\def\csname res@v5d@combo_hard_b25@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@granger@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_hard_b25@granger@rp\endcsname{0.58}
\expandafter\def\csname res@v5d@combo_hard_b25@granger@map\endcsname{0.63}
\expandafter\def\csname res@v5d@combo_hard_b25@pcmciplus@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@combo_hard_b25@pcmciplus@fpn\endcsname{4}
\expandafter\def\csname res@v5d@combo_hard_b25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@pcmciplus@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_hard_b25@pcmciplus@prec\endcsname{0.47}
\expandafter\def\csname res@v5d@combo_hard_b25@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v5d@combo_hard_b25@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b25@pcmciplus@len\endcsname{1.0}
\expandafter\def\csname res@v5d@combo_hard_b25@pcmciplus@rp\endcsname{0.52}
\expandafter\def\csname res@v5d@combo_hard_b25@pcmciplus@map\endcsname{0.58}
\expandafter\def\csname res@v5d@combo_hard_b25@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_hard_b25@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_hard_b25@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v5d@combo_hard_b25@pc@prec\endcsname{0.39}
\expandafter\def\csname res@v5d@combo_hard_b25@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@pc@bw\endcsname{5}
\expandafter\def\csname res@v5d@combo_hard_b25@pc@len\endcsname{2.7}
\expandafter\def\csname res@v5d@combo_hard_b25@pc@rp\endcsname{0.26}
\expandafter\def\csname res@v5d@combo_hard_b25@pc@map\endcsname{0.30}
\expandafter\def\csname res@v5d@combo_hard_b25@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_hard_b25@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_hard_b25@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@combo_hard_b25@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@combo_hard_b25@dynotears@rp\endcsname{0.72}
\expandafter\def\csname res@v5d@combo_hard_b25@dynotears@map\endcsname{0.81}
\expandafter\def\csname res@v5d@combo_hard_b25@doubleml@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_hard_b25@doubleml@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@combo_hard_b25@doubleml@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_hard_b25@doubleml@ab\endcsname{8}
\expandafter\def\csname res@v5d@combo_hard_b25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@doubleml@len\endcsname{0.4}
\expandafter\def\csname res@v5d@combo_hard_b25@doubleml@rp\endcsname{0.25}
\expandafter\def\csname res@v5d@combo_hard_b25@doubleml@map\endcsname{0.35}
\expandafter\def\csname res@v5d@combo_hard_b25@varlingam@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@combo_hard_b25@varlingam@fpn\endcsname{4}
\expandafter\def\csname res@v5d@combo_hard_b25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@varlingam@tt\endcsname{0.35}
\expandafter\def\csname res@v5d@combo_hard_b25@varlingam@prec\endcsname{0.36}
\expandafter\def\csname res@v5d@combo_hard_b25@varlingam@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b25@varlingam@bw\endcsname{3}
\expandafter\def\csname res@v5d@combo_hard_b25@varlingam@len\endcsname{4.4}
\expandafter\def\csname res@v5d@combo_hard_b25@varlingam@rp\endcsname{0.41}
\expandafter\def\csname res@v5d@combo_hard_b25@varlingam@map\endcsname{0.49}
\expandafter\def\csname res@v5d@combo_hard_b25@spacetime_rule@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_hard_b25@spacetime_rule@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_hard_b25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@spacetime_rule@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_hard_b25@spacetime_rule@prec\endcsname{0.38}
\expandafter\def\csname res@v5d@combo_hard_b25@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v5d@combo_hard_b25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@spacetime_rule@len\endcsname{1.0}
\expandafter\def\csname res@v5d@combo_hard_b25@spacetime_rule@rp\endcsname{0.25}
\expandafter\def\csname res@v5d@combo_hard_b25@spacetime_rule@map\endcsname{0.42}
\expandafter\def\csname res@v5d@combo_hard_b25@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_hard_b25@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b25@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_hard_b25@varsort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@combo_hard_b25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@combo_hard_b25@varsort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_hard_b25@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v5d@combo_hard_b25@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_hard_b25@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b25@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_hard_b25@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@combo_hard_b25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b25@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b25@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_hard_b25@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_hard_b25@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v5d@combo_extreme_b25@correlation@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@combo_extreme_b25@correlation@fpn\endcsname{4}
\expandafter\def\csname res@v5d@combo_extreme_b25@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b25@correlation@tt\endcsname{0.31}
\expandafter\def\csname res@v5d@combo_extreme_b25@correlation@prec\endcsname{0.21}
\expandafter\def\csname res@v5d@combo_extreme_b25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b25@correlation@bw\endcsname{6}
\expandafter\def\csname res@v5d@combo_extreme_b25@correlation@len\endcsname{9.4}
\expandafter\def\csname res@v5d@combo_extreme_b25@correlation@rp\endcsname{0.22}
\expandafter\def\csname res@v5d@combo_extreme_b25@correlation@map\endcsname{0.41}
\expandafter\def\csname res@v5d@combo_extreme_b25@granger@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_extreme_b25@granger@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b25@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b25@granger@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_extreme_b25@granger@prec\endcsname{0.28}
\expandafter\def\csname res@v5d@combo_extreme_b25@granger@ab\endcsname{6}
\expandafter\def\csname res@v5d@combo_extreme_b25@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b25@granger@len\endcsname{1.4}
\expandafter\def\csname res@v5d@combo_extreme_b25@granger@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@combo_extreme_b25@granger@map\endcsname{0.52}
\expandafter\def\csname res@v5d@combo_extreme_b25@pcmciplus@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_extreme_b25@pcmciplus@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_extreme_b25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b25@pcmciplus@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b25@pcmciplus@prec\endcsname{0.50}
\expandafter\def\csname res@v5d@combo_extreme_b25@pcmciplus@ab\endcsname{5}
\expandafter\def\csname res@v5d@combo_extreme_b25@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b25@pcmciplus@len\endcsname{0.6}
\expandafter\def\csname res@v5d@combo_extreme_b25@pcmciplus@rp\endcsname{0.36}
\expandafter\def\csname res@v5d@combo_extreme_b25@pcmciplus@map\endcsname{0.45}
\expandafter\def\csname res@v5d@combo_extreme_b25@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_extreme_b25@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b25@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b25@pc@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@combo_extreme_b25@pc@prec\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_extreme_b25@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b25@pc@bw\endcsname{7}
\expandafter\def\csname res@v5d@combo_extreme_b25@pc@len\endcsname{2.2}
\expandafter\def\csname res@v5d@combo_extreme_b25@pc@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b25@pc@map\endcsname{0.18}
\expandafter\def\csname res@v5d@combo_extreme_b25@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_extreme_b25@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b25@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@combo_extreme_b25@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@combo_extreme_b25@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v5d@combo_extreme_b25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b25@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v5d@combo_extreme_b25@dynotears@rp\endcsname{0.38}
\expandafter\def\csname res@v5d@combo_extreme_b25@dynotears@map\endcsname{0.55}
\expandafter\def\csname res@v5d@combo_extreme_b25@doubleml@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_extreme_b25@doubleml@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b25@doubleml@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_extreme_b25@doubleml@prec\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_extreme_b25@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v5d@combo_extreme_b25@doubleml@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b25@doubleml@len\endcsname{0.5}
\expandafter\def\csname res@v5d@combo_extreme_b25@doubleml@rp\endcsname{0.07}
\expandafter\def\csname res@v5d@combo_extreme_b25@doubleml@map\endcsname{0.20}
\expandafter\def\csname res@v5d@combo_extreme_b25@varlingam@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_extreme_b25@varlingam@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_extreme_b25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b25@varlingam@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b25@varlingam@prec\endcsname{0.22}
\expandafter\def\csname res@v5d@combo_extreme_b25@varlingam@ab\endcsname{3}
\expandafter\def\csname res@v5d@combo_extreme_b25@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b25@varlingam@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_extreme_b25@varlingam@rp\endcsname{0.30}
\expandafter\def\csname res@v5d@combo_extreme_b25@varlingam@map\endcsname{0.38}
\expandafter\def\csname res@v5d@combo_extreme_b25@spacetime_rule@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_extreme_b25@spacetime_rule@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_extreme_b25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b25@spacetime_rule@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b25@spacetime_rule@prec\endcsname{0.31}
\expandafter\def\csname res@v5d@combo_extreme_b25@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b25@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v5d@combo_extreme_b25@spacetime_rule@rp\endcsname{0.16}
\expandafter\def\csname res@v5d@combo_extreme_b25@spacetime_rule@map\endcsname{0.33}
\expandafter\def\csname res@v5d@combo_extreme_b25@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_extreme_b25@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b25@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b25@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_extreme_b25@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_extreme_b25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b25@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b25@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@combo_extreme_b25@varsort@rp\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_extreme_b25@varsort@map\endcsname{0.23}
\expandafter\def\csname res@v5d@combo_extreme_b25@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_extreme_b25@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b25@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b25@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@combo_extreme_b25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b25@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b25@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_extreme_b25@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_extreme_b25@r2sort@map\endcsname{0.22}
\expandafter\def\csname res@v5d@interaction_1.0_b25@correlation@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@correlation@fpn\endcsname{3}
\expandafter\def\csname res@v5d@interaction_1.0_b25@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@correlation@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@interaction_1.0_b25@correlation@prec\endcsname{0.23}
\expandafter\def\csname res@v5d@interaction_1.0_b25@correlation@ab\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b25@correlation@bw\endcsname{4}
\expandafter\def\csname res@v5d@interaction_1.0_b25@correlation@len\endcsname{3.2}
\expandafter\def\csname res@v5d@interaction_1.0_b25@correlation@rp\endcsname{0.28}
\expandafter\def\csname res@v5d@interaction_1.0_b25@correlation@map\endcsname{0.40}
\expandafter\def\csname res@v5d@interaction_1.0_b25@granger@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@granger@fpn\endcsname{3}
\expandafter\def\csname res@v5d@interaction_1.0_b25@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@granger@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@interaction_1.0_b25@granger@prec\endcsname{0.39}
\expandafter\def\csname res@v5d@interaction_1.0_b25@granger@ab\endcsname{6}
\expandafter\def\csname res@v5d@interaction_1.0_b25@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@granger@len\endcsname{1.7}
\expandafter\def\csname res@v5d@interaction_1.0_b25@granger@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@interaction_1.0_b25@granger@map\endcsname{0.44}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pcmciplus@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pcmciplus@fpn\endcsname{3}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pcmciplus@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pcmciplus@prec\endcsname{0.31}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pcmciplus@ab\endcsname{3}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pcmciplus@len\endcsname{1.5}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pcmciplus@rp\endcsname{0.30}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pcmciplus@map\endcsname{0.40}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pc@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pc@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pc@bw\endcsname{5}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pc@len\endcsname{2.5}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pc@rp\endcsname{0.24}
\expandafter\def\csname res@v5d@interaction_1.0_b25@pc@map\endcsname{0.25}
\expandafter\def\csname res@v5d@interaction_1.0_b25@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@interaction_1.0_b25@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@interaction_1.0_b25@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v5d@interaction_1.0_b25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v5d@interaction_1.0_b25@dynotears@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@interaction_1.0_b25@dynotears@map\endcsname{0.39}
\expandafter\def\csname res@v5d@interaction_1.0_b25@doubleml@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@doubleml@fpn\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@interaction_1.0_b25@doubleml@prec\endcsname{0.50}
\expandafter\def\csname res@v5d@interaction_1.0_b25@doubleml@ab\endcsname{9}
\expandafter\def\csname res@v5d@interaction_1.0_b25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@doubleml@len\endcsname{0.2}
\expandafter\def\csname res@v5d@interaction_1.0_b25@doubleml@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@interaction_1.0_b25@doubleml@map\endcsname{0.29}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varlingam@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varlingam@fpn\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varlingam@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varlingam@prec\endcsname{0.33}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varlingam@ab\endcsname{5}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varlingam@len\endcsname{1.1}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varlingam@rp\endcsname{0.34}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varlingam@map\endcsname{0.42}
\expandafter\def\csname res@v5d@interaction_1.0_b25@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v5d@interaction_1.0_b25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@interaction_1.0_b25@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@interaction_1.0_b25@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v5d@interaction_1.0_b25@spacetime_rule@rp\endcsname{0.60}
\expandafter\def\csname res@v5d@interaction_1.0_b25@spacetime_rule@map\endcsname{0.75}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varsort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varsort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@interaction_1.0_b25@varsort@map\endcsname{0.18}
\expandafter\def\csname res@v5d@interaction_1.0_b25@r2sort@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@r2sort@fpn\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@interaction_1.0_b25@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@interaction_1.0_b25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@r2sort@bw\endcsname{3}
\expandafter\def\csname res@v5d@interaction_1.0_b25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@interaction_1.0_b25@r2sort@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@interaction_1.0_b25@r2sort@map\endcsname{0.22}
\expandafter\def\csname res@v5d@combo_interaction_b25@correlation@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b25@correlation@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b25@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@correlation@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_interaction_b25@correlation@prec\endcsname{0.08}
\expandafter\def\csname res@v5d@combo_interaction_b25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@correlation@bw\endcsname{9}
\expandafter\def\csname res@v5d@combo_interaction_b25@correlation@len\endcsname{4.0}
\expandafter\def\csname res@v5d@combo_interaction_b25@correlation@rp\endcsname{0.05}
\expandafter\def\csname res@v5d@combo_interaction_b25@correlation@map\endcsname{0.29}
\expandafter\def\csname res@v5d@combo_interaction_b25@granger@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_interaction_b25@granger@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b25@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@granger@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_interaction_b25@granger@prec\endcsname{0.44}
\expandafter\def\csname res@v5d@combo_interaction_b25@granger@ab\endcsname{7}
\expandafter\def\csname res@v5d@combo_interaction_b25@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@granger@len\endcsname{1.2}
\expandafter\def\csname res@v5d@combo_interaction_b25@granger@rp\endcsname{0.28}
\expandafter\def\csname res@v5d@combo_interaction_b25@granger@map\endcsname{0.36}
\expandafter\def\csname res@v5d@combo_interaction_b25@pcmciplus@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b25@pcmciplus@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@pcmciplus@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@combo_interaction_b25@pcmciplus@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_interaction_b25@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v5d@combo_interaction_b25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@pcmciplus@len\endcsname{1.0}
\expandafter\def\csname res@v5d@combo_interaction_b25@pcmciplus@rp\endcsname{0.31}
\expandafter\def\csname res@v5d@combo_interaction_b25@pcmciplus@map\endcsname{0.40}
\expandafter\def\csname res@v5d@combo_interaction_b25@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_interaction_b25@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b25@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@pc@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b25@pc@prec\endcsname{0.20}
\expandafter\def\csname res@v5d@combo_interaction_b25@pc@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b25@pc@bw\endcsname{5}
\expandafter\def\csname res@v5d@combo_interaction_b25@pc@len\endcsname{2.0}
\expandafter\def\csname res@v5d@combo_interaction_b25@pc@rp\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_interaction_b25@pc@map\endcsname{0.23}
\expandafter\def\csname res@v5d@combo_interaction_b25@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_interaction_b25@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_interaction_b25@dynotears@prec\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_interaction_b25@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v5d@combo_interaction_b25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v5d@combo_interaction_b25@dynotears@rp\endcsname{0.18}
\expandafter\def\csname res@v5d@combo_interaction_b25@dynotears@map\endcsname{0.27}
\expandafter\def\csname res@v5d@combo_interaction_b25@doubleml@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_interaction_b25@doubleml@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@doubleml@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_interaction_b25@doubleml@prec\endcsname{--}
\expandafter\def\csname res@v5d@combo_interaction_b25@doubleml@ab\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@doubleml@len\endcsname{0.0}
\expandafter\def\csname res@v5d@combo_interaction_b25@doubleml@rp\endcsname{0.18}
\expandafter\def\csname res@v5d@combo_interaction_b25@doubleml@map\endcsname{0.30}
\expandafter\def\csname res@v5d@combo_interaction_b25@varlingam@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b25@varlingam@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@varlingam@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@combo_interaction_b25@varlingam@prec\endcsname{0.34}
\expandafter\def\csname res@v5d@combo_interaction_b25@varlingam@ab\endcsname{6}
\expandafter\def\csname res@v5d@combo_interaction_b25@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b25@varlingam@len\endcsname{1.7}
\expandafter\def\csname res@v5d@combo_interaction_b25@varlingam@rp\endcsname{0.38}
\expandafter\def\csname res@v5d@combo_interaction_b25@varlingam@map\endcsname{0.40}
\expandafter\def\csname res@v5d@combo_interaction_b25@spacetime_rule@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@combo_interaction_b25@spacetime_rule@fpn\endcsname{5}
\expandafter\def\csname res@v5d@combo_interaction_b25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@spacetime_rule@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@combo_interaction_b25@spacetime_rule@prec\endcsname{0.64}
\expandafter\def\csname res@v5d@combo_interaction_b25@spacetime_rule@ab\endcsname{3}
\expandafter\def\csname res@v5d@combo_interaction_b25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@spacetime_rule@len\endcsname{0.9}
\expandafter\def\csname res@v5d@combo_interaction_b25@spacetime_rule@rp\endcsname{0.47}
\expandafter\def\csname res@v5d@combo_interaction_b25@spacetime_rule@map\endcsname{0.54}
\expandafter\def\csname res@v5d@combo_interaction_b25@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b25@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b25@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b25@varsort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@combo_interaction_b25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@combo_interaction_b25@varsort@rp\endcsname{0.13}
\expandafter\def\csname res@v5d@combo_interaction_b25@varsort@map\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_interaction_b25@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b25@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b25@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_interaction_b25@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@combo_interaction_b25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b25@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b25@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_interaction_b25@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_interaction_b25@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v5d@control_weak_b25@correlation@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@control_weak_b25@correlation@fpn\endcsname{3}
\expandafter\def\csname res@v5d@control_weak_b25@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@correlation@tt\endcsname{0.35}
\expandafter\def\csname res@v5d@control_weak_b25@correlation@prec\endcsname{0.28}
\expandafter\def\csname res@v5d@control_weak_b25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b25@correlation@bw\endcsname{6}
\expandafter\def\csname res@v5d@control_weak_b25@correlation@len\endcsname{5.4}
\expandafter\def\csname res@v5d@control_weak_b25@correlation@rp\endcsname{0.27}
\expandafter\def\csname res@v5d@control_weak_b25@correlation@map\endcsname{0.40}
\expandafter\def\csname res@v5d@control_weak_b25@granger@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@control_weak_b25@granger@fpn\endcsname{2}
\expandafter\def\csname res@v5d@control_weak_b25@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@granger@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@control_weak_b25@granger@prec\endcsname{0.67}
\expandafter\def\csname res@v5d@control_weak_b25@granger@ab\endcsname{7}
\expandafter\def\csname res@v5d@control_weak_b25@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b25@granger@len\endcsname{0.5}
\expandafter\def\csname res@v5d@control_weak_b25@granger@rp\endcsname{0.39}
\expandafter\def\csname res@v5d@control_weak_b25@granger@map\endcsname{0.49}
\expandafter\def\csname res@v5d@control_weak_b25@pcmciplus@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@control_weak_b25@pcmciplus@fpn\endcsname{5}
\expandafter\def\csname res@v5d@control_weak_b25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@pcmciplus@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@control_weak_b25@pcmciplus@prec\endcsname{0.56}
\expandafter\def\csname res@v5d@control_weak_b25@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b25@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b25@pcmciplus@len\endcsname{1.1}
\expandafter\def\csname res@v5d@control_weak_b25@pcmciplus@rp\endcsname{0.38}
\expandafter\def\csname res@v5d@control_weak_b25@pcmciplus@map\endcsname{0.48}
\expandafter\def\csname res@v5d@control_weak_b25@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@control_weak_b25@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b25@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@pc@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@control_weak_b25@pc@prec\endcsname{0.20}
\expandafter\def\csname res@v5d@control_weak_b25@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b25@pc@bw\endcsname{5}
\expandafter\def\csname res@v5d@control_weak_b25@pc@len\endcsname{3.1}
\expandafter\def\csname res@v5d@control_weak_b25@pc@rp\endcsname{0.21}
\expandafter\def\csname res@v5d@control_weak_b25@pc@map\endcsname{0.20}
\expandafter\def\csname res@v5d@control_weak_b25@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@control_weak_b25@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@control_weak_b25@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@control_weak_b25@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b25@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@control_weak_b25@dynotears@rp\endcsname{0.48}
\expandafter\def\csname res@v5d@control_weak_b25@dynotears@map\endcsname{0.50}
\expandafter\def\csname res@v5d@control_weak_b25@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@control_weak_b25@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@control_weak_b25@doubleml@prec\endcsname{0.20}
\expandafter\def\csname res@v5d@control_weak_b25@doubleml@ab\endcsname{5}
\expandafter\def\csname res@v5d@control_weak_b25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b25@doubleml@len\endcsname{0.8}
\expandafter\def\csname res@v5d@control_weak_b25@doubleml@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@control_weak_b25@doubleml@map\endcsname{0.32}
\expandafter\def\csname res@v5d@control_weak_b25@varlingam@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@control_weak_b25@varlingam@fpn\endcsname{6}
\expandafter\def\csname res@v5d@control_weak_b25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@varlingam@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@control_weak_b25@varlingam@prec\endcsname{0.61}
\expandafter\def\csname res@v5d@control_weak_b25@varlingam@ab\endcsname{3}
\expandafter\def\csname res@v5d@control_weak_b25@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b25@varlingam@len\endcsname{1.9}
\expandafter\def\csname res@v5d@control_weak_b25@varlingam@rp\endcsname{0.29}
\expandafter\def\csname res@v5d@control_weak_b25@varlingam@map\endcsname{0.56}
\expandafter\def\csname res@v5d@control_weak_b25@spacetime_rule@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@control_weak_b25@spacetime_rule@fpn\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@spacetime_rule@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@control_weak_b25@spacetime_rule@prec\endcsname{0.20}
\expandafter\def\csname res@v5d@control_weak_b25@spacetime_rule@ab\endcsname{5}
\expandafter\def\csname res@v5d@control_weak_b25@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b25@spacetime_rule@len\endcsname{0.6}
\expandafter\def\csname res@v5d@control_weak_b25@spacetime_rule@rp\endcsname{0.17}
\expandafter\def\csname res@v5d@control_weak_b25@spacetime_rule@map\endcsname{0.28}
\expandafter\def\csname res@v5d@control_weak_b25@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@control_weak_b25@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v5d@control_weak_b25@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@control_weak_b25@varsort@prec\endcsname{0.12}
\expandafter\def\csname res@v5d@control_weak_b25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b25@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b25@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v5d@control_weak_b25@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@control_weak_b25@varsort@map\endcsname{0.19}
\expandafter\def\csname res@v5d@control_weak_b25@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@control_weak_b25@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b25@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@control_weak_b25@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@control_weak_b25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b25@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@control_weak_b25@r2sort@rp\endcsname{0.17}
\expandafter\def\csname res@v5d@control_weak_b25@r2sort@map\endcsname{0.29}
\expandafter\def\csname res@v5d@default_b50@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@default_b50@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v5d@default_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@correlation@tt\endcsname{0.69}
\expandafter\def\csname res@v5d@default_b50@correlation@prec\endcsname{0.16}
\expandafter\def\csname res@v5d@default_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@correlation@bw\endcsname{1}
\expandafter\def\csname res@v5d@default_b50@correlation@len\endcsname{16.7}
\expandafter\def\csname res@v5d@default_b50@correlation@rp\endcsname{0.75}
\expandafter\def\csname res@v5d@default_b50@correlation@map\endcsname{0.82}
\expandafter\def\csname res@v5d@default_b50@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@default_b50@granger@fpn\endcsname{8}
\expandafter\def\csname res@v5d@default_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@default_b50@granger@prec\endcsname{0.25}
\expandafter\def\csname res@v5d@default_b50@granger@ab\endcsname{1}
\expandafter\def\csname res@v5d@default_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@granger@len\endcsname{10.3}
\expandafter\def\csname res@v5d@default_b50@granger@rp\endcsname{0.68}
\expandafter\def\csname res@v5d@default_b50@granger@map\endcsname{0.75}
\expandafter\def\csname res@v5d@default_b50@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@default_b50@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v5d@default_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v5d@default_b50@pcmciplus@prec\endcsname{0.88}
\expandafter\def\csname res@v5d@default_b50@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@pcmciplus@len\endcsname{2.3}
\expandafter\def\csname res@v5d@default_b50@pcmciplus@rp\endcsname{0.87}
\expandafter\def\csname res@v5d@default_b50@pcmciplus@map\endcsname{0.89}
\expandafter\def\csname res@v5d@default_b50@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@default_b50@pc@fpn\endcsname{3}
\expandafter\def\csname res@v5d@default_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@pc@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@default_b50@pc@prec\endcsname{0.50}
\expandafter\def\csname res@v5d@default_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@pc@bw\endcsname{3}
\expandafter\def\csname res@v5d@default_b50@pc@len\endcsname{4.1}
\expandafter\def\csname res@v5d@default_b50@pc@rp\endcsname{0.46}
\expandafter\def\csname res@v5d@default_b50@pc@map\endcsname{0.44}
\expandafter\def\csname res@v5d@default_b50@dynotears@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@default_b50@dynotears@fpn\endcsname{8}
\expandafter\def\csname res@v5d@default_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@dynotears@tt\endcsname{0.35}
\expandafter\def\csname res@v5d@default_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@default_b50@dynotears@ab\endcsname{2}
\expandafter\def\csname res@v5d@default_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@dynotears@len\endcsname{0.9}
\expandafter\def\csname res@v5d@default_b50@dynotears@rp\endcsname{0.90}
\expandafter\def\csname res@v5d@default_b50@dynotears@map\endcsname{0.95}
\expandafter\def\csname res@v5d@default_b50@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@default_b50@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v5d@default_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@doubleml@tt\endcsname{0.65}
\expandafter\def\csname res@v5d@default_b50@doubleml@prec\endcsname{0.82}
\expandafter\def\csname res@v5d@default_b50@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v5d@default_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@doubleml@len\endcsname{2.3}
\expandafter\def\csname res@v5d@default_b50@doubleml@rp\endcsname{0.84}
\expandafter\def\csname res@v5d@default_b50@doubleml@map\endcsname{0.87}
\expandafter\def\csname res@v5d@default_b50@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v5d@default_b50@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v5d@default_b50@varlingam@prec\endcsname{0.46}
\expandafter\def\csname res@v5d@default_b50@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@varlingam@len\endcsname{5.8}
\expandafter\def\csname res@v5d@default_b50@varlingam@rp\endcsname{0.69}
\expandafter\def\csname res@v5d@default_b50@varlingam@map\endcsname{0.83}
\expandafter\def\csname res@v5d@default_b50@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@default_b50@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v5d@default_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v5d@default_b50@spacetime_rule@prec\endcsname{0.94}
\expandafter\def\csname res@v5d@default_b50@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v5d@default_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@spacetime_rule@len\endcsname{0.9}
\expandafter\def\csname res@v5d@default_b50@spacetime_rule@rp\endcsname{0.51}
\expandafter\def\csname res@v5d@default_b50@spacetime_rule@map\endcsname{0.63}
\expandafter\def\csname res@v5d@default_b50@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@default_b50@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@varsort@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@default_b50@varsort@prec\endcsname{0.03}
\expandafter\def\csname res@v5d@default_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@default_b50@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@default_b50@varsort@rp\endcsname{0.06}
\expandafter\def\csname res@v5d@default_b50@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v5d@default_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@default_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@default_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b50@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@default_b50@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@default_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@default_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@default_b50@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v5d@default_b50@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v5d@signal_0.1_b50@correlation@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@signal_0.1_b50@correlation@fpn\endcsname{3}
\expandafter\def\csname res@v5d@signal_0.1_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@correlation@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@signal_0.1_b50@correlation@prec\endcsname{0.24}
\expandafter\def\csname res@v5d@signal_0.1_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@correlation@bw\endcsname{7}
\expandafter\def\csname res@v5d@signal_0.1_b50@correlation@len\endcsname{9.0}
\expandafter\def\csname res@v5d@signal_0.1_b50@correlation@rp\endcsname{0.32}
\expandafter\def\csname res@v5d@signal_0.1_b50@correlation@map\endcsname{0.47}
\expandafter\def\csname res@v5d@signal_0.1_b50@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@signal_0.1_b50@granger@fpn\endcsname{8}
\expandafter\def\csname res@v5d@signal_0.1_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v5d@signal_0.1_b50@granger@prec\endcsname{0.52}
\expandafter\def\csname res@v5d@signal_0.1_b50@granger@ab\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@granger@len\endcsname{2.6}
\expandafter\def\csname res@v5d@signal_0.1_b50@granger@rp\endcsname{0.68}
\expandafter\def\csname res@v5d@signal_0.1_b50@granger@map\endcsname{0.79}
\expandafter\def\csname res@v5d@signal_0.1_b50@pcmciplus@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@signal_0.1_b50@pcmciplus@fpn\endcsname{5}
\expandafter\def\csname res@v5d@signal_0.1_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@pcmciplus@tt\endcsname{0.31}
\expandafter\def\csname res@v5d@signal_0.1_b50@pcmciplus@prec\endcsname{0.57}
\expandafter\def\csname res@v5d@signal_0.1_b50@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@pcmciplus@len\endcsname{1.3}
\expandafter\def\csname res@v5d@signal_0.1_b50@pcmciplus@rp\endcsname{0.63}
\expandafter\def\csname res@v5d@signal_0.1_b50@pcmciplus@map\endcsname{0.71}
\expandafter\def\csname res@v5d@signal_0.1_b50@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@signal_0.1_b50@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@pc@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@signal_0.1_b50@pc@prec\endcsname{0.23}
\expandafter\def\csname res@v5d@signal_0.1_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@pc@bw\endcsname{7}
\expandafter\def\csname res@v5d@signal_0.1_b50@pc@len\endcsname{3.4}
\expandafter\def\csname res@v5d@signal_0.1_b50@pc@rp\endcsname{0.22}
\expandafter\def\csname res@v5d@signal_0.1_b50@pc@map\endcsname{0.22}
\expandafter\def\csname res@v5d@signal_0.1_b50@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@signal_0.1_b50@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@signal_0.1_b50@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@signal_0.1_b50@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@signal_0.1_b50@dynotears@rp\endcsname{0.42}
\expandafter\def\csname res@v5d@signal_0.1_b50@dynotears@map\endcsname{0.56}
\expandafter\def\csname res@v5d@signal_0.1_b50@doubleml@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@signal_0.1_b50@doubleml@fpn\endcsname{3}
\expandafter\def\csname res@v5d@signal_0.1_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@doubleml@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@signal_0.1_b50@doubleml@prec\endcsname{0.67}
\expandafter\def\csname res@v5d@signal_0.1_b50@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v5d@signal_0.1_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@doubleml@len\endcsname{0.9}
\expandafter\def\csname res@v5d@signal_0.1_b50@doubleml@rp\endcsname{0.53}
\expandafter\def\csname res@v5d@signal_0.1_b50@doubleml@map\endcsname{0.57}
\expandafter\def\csname res@v5d@signal_0.1_b50@varlingam@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@signal_0.1_b50@varlingam@fpn\endcsname{5}
\expandafter\def\csname res@v5d@signal_0.1_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@varlingam@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@signal_0.1_b50@varlingam@prec\endcsname{0.45}
\expandafter\def\csname res@v5d@signal_0.1_b50@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@varlingam@bw\endcsname{3}
\expandafter\def\csname res@v5d@signal_0.1_b50@varlingam@len\endcsname{3.3}
\expandafter\def\csname res@v5d@signal_0.1_b50@varlingam@rp\endcsname{0.32}
\expandafter\def\csname res@v5d@signal_0.1_b50@varlingam@map\endcsname{0.42}
\expandafter\def\csname res@v5d@signal_0.1_b50@spacetime_rule@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@signal_0.1_b50@spacetime_rule@fpn\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@spacetime_rule@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@signal_0.1_b50@spacetime_rule@prec\endcsname{--}
\expandafter\def\csname res@v5d@signal_0.1_b50@spacetime_rule@ab\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@spacetime_rule@len\endcsname{0.0}
\expandafter\def\csname res@v5d@signal_0.1_b50@spacetime_rule@rp\endcsname{0.28}
\expandafter\def\csname res@v5d@signal_0.1_b50@spacetime_rule@map\endcsname{0.38}
\expandafter\def\csname res@v5d@signal_0.1_b50@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@signal_0.1_b50@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@varsort@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@signal_0.1_b50@varsort@prec\endcsname{0.07}
\expandafter\def\csname res@v5d@signal_0.1_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b50@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@signal_0.1_b50@varsort@rp\endcsname{0.07}
\expandafter\def\csname res@v5d@signal_0.1_b50@varsort@map\endcsname{0.14}
\expandafter\def\csname res@v5d@signal_0.1_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@signal_0.1_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b50@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@signal_0.1_b50@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@signal_0.1_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@signal_0.1_b50@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v5d@signal_0.1_b50@r2sort@map\endcsname{0.22}
\expandafter\def\csname res@v5d@echo_0.8_b50@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@echo_0.8_b50@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v5d@echo_0.8_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b50@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@echo_0.8_b50@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v5d@echo_0.8_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@correlation@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@correlation@len\endcsname{17.1}
\expandafter\def\csname res@v5d@echo_0.8_b50@correlation@rp\endcsname{0.64}
\expandafter\def\csname res@v5d@echo_0.8_b50@correlation@map\endcsname{0.73}
\expandafter\def\csname res@v5d@echo_0.8_b50@granger@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@echo_0.8_b50@granger@fpn\endcsname{7}
\expandafter\def\csname res@v5d@echo_0.8_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b50@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@echo_0.8_b50@granger@prec\endcsname{0.21}
\expandafter\def\csname res@v5d@echo_0.8_b50@granger@ab\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@granger@len\endcsname{10.9}
\expandafter\def\csname res@v5d@echo_0.8_b50@granger@rp\endcsname{0.53}
\expandafter\def\csname res@v5d@echo_0.8_b50@granger@map\endcsname{0.67}
\expandafter\def\csname res@v5d@echo_0.8_b50@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@echo_0.8_b50@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v5d@echo_0.8_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b50@pcmciplus@tt\endcsname{0.54}
\expandafter\def\csname res@v5d@echo_0.8_b50@pcmciplus@prec\endcsname{0.87}
\expandafter\def\csname res@v5d@echo_0.8_b50@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@pcmciplus@len\endcsname{1.8}
\expandafter\def\csname res@v5d@echo_0.8_b50@pcmciplus@rp\endcsname{0.87}
\expandafter\def\csname res@v5d@echo_0.8_b50@pcmciplus@map\endcsname{0.87}
\expandafter\def\csname res@v5d@echo_0.8_b50@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@echo_0.8_b50@pc@fpn\endcsname{3}
\expandafter\def\csname res@v5d@echo_0.8_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b50@pc@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@echo_0.8_b50@pc@prec\endcsname{0.39}
\expandafter\def\csname res@v5d@echo_0.8_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@pc@bw\endcsname{5}
\expandafter\def\csname res@v5d@echo_0.8_b50@pc@len\endcsname{4.1}
\expandafter\def\csname res@v5d@echo_0.8_b50@pc@rp\endcsname{0.37}
\expandafter\def\csname res@v5d@echo_0.8_b50@pc@map\endcsname{0.33}
\expandafter\def\csname res@v5d@echo_0.8_b50@dynotears@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@echo_0.8_b50@dynotears@fpn\endcsname{5}
\expandafter\def\csname res@v5d@echo_0.8_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b50@dynotears@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@echo_0.8_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@echo_0.8_b50@dynotears@ab\endcsname{5}
\expandafter\def\csname res@v5d@echo_0.8_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@dynotears@len\endcsname{0.5}
\expandafter\def\csname res@v5d@echo_0.8_b50@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v5d@echo_0.8_b50@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v5d@echo_0.8_b50@doubleml@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@echo_0.8_b50@doubleml@fpn\endcsname{7}
\expandafter\def\csname res@v5d@echo_0.8_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b50@doubleml@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@echo_0.8_b50@doubleml@prec\endcsname{0.83}
\expandafter\def\csname res@v5d@echo_0.8_b50@doubleml@ab\endcsname{3}
\expandafter\def\csname res@v5d@echo_0.8_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@doubleml@len\endcsname{1.4}
\expandafter\def\csname res@v5d@echo_0.8_b50@doubleml@rp\endcsname{0.55}
\expandafter\def\csname res@v5d@echo_0.8_b50@doubleml@map\endcsname{0.67}
\expandafter\def\csname res@v5d@echo_0.8_b50@varlingam@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@echo_0.8_b50@varlingam@fpn\endcsname{8}
\expandafter\def\csname res@v5d@echo_0.8_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b50@varlingam@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@echo_0.8_b50@varlingam@prec\endcsname{0.38}
\expandafter\def\csname res@v5d@echo_0.8_b50@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@varlingam@len\endcsname{5.6}
\expandafter\def\csname res@v5d@echo_0.8_b50@varlingam@rp\endcsname{0.64}
\expandafter\def\csname res@v5d@echo_0.8_b50@varlingam@map\endcsname{0.62}
\expandafter\def\csname res@v5d@echo_0.8_b50@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@echo_0.8_b50@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v5d@echo_0.8_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b50@spacetime_rule@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@echo_0.8_b50@spacetime_rule@prec\endcsname{0.55}
\expandafter\def\csname res@v5d@echo_0.8_b50@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b50@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v5d@echo_0.8_b50@spacetime_rule@rp\endcsname{0.54}
\expandafter\def\csname res@v5d@echo_0.8_b50@spacetime_rule@map\endcsname{0.63}
\expandafter\def\csname res@v5d@echo_0.8_b50@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@echo_0.8_b50@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b50@varsort@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@echo_0.8_b50@varsort@prec\endcsname{0.07}
\expandafter\def\csname res@v5d@echo_0.8_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b50@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@echo_0.8_b50@varsort@rp\endcsname{0.08}
\expandafter\def\csname res@v5d@echo_0.8_b50@varsort@map\endcsname{0.14}
\expandafter\def\csname res@v5d@echo_0.8_b50@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@echo_0.8_b50@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b50@r2sort@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@echo_0.8_b50@r2sort@prec\endcsname{0.07}
\expandafter\def\csname res@v5d@echo_0.8_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@echo_0.8_b50@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@echo_0.8_b50@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5d@confound_0.8_b50@correlation@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@confound_0.8_b50@correlation@fpn\endcsname{6}
\expandafter\def\csname res@v5d@confound_0.8_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b50@correlation@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@confound_0.8_b50@correlation@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@confound_0.8_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@correlation@bw\endcsname{3}
\expandafter\def\csname res@v5d@confound_0.8_b50@correlation@len\endcsname{16.4}
\expandafter\def\csname res@v5d@confound_0.8_b50@correlation@rp\endcsname{0.50}
\expandafter\def\csname res@v5d@confound_0.8_b50@correlation@map\endcsname{0.57}
\expandafter\def\csname res@v5d@confound_0.8_b50@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@confound_0.8_b50@granger@fpn\endcsname{9}
\expandafter\def\csname res@v5d@confound_0.8_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b50@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@confound_0.8_b50@granger@prec\endcsname{0.19}
\expandafter\def\csname res@v5d@confound_0.8_b50@granger@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@granger@len\endcsname{11.7}
\expandafter\def\csname res@v5d@confound_0.8_b50@granger@rp\endcsname{0.56}
\expandafter\def\csname res@v5d@confound_0.8_b50@granger@map\endcsname{0.66}
\expandafter\def\csname res@v5d@confound_0.8_b50@pcmciplus@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@confound_0.8_b50@pcmciplus@fpn\endcsname{7}
\expandafter\def\csname res@v5d@confound_0.8_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b50@pcmciplus@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@confound_0.8_b50@pcmciplus@prec\endcsname{0.70}
\expandafter\def\csname res@v5d@confound_0.8_b50@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v5d@confound_0.8_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@pcmciplus@len\endcsname{1.9}
\expandafter\def\csname res@v5d@confound_0.8_b50@pcmciplus@rp\endcsname{0.73}
\expandafter\def\csname res@v5d@confound_0.8_b50@pcmciplus@map\endcsname{0.85}
\expandafter\def\csname res@v5d@confound_0.8_b50@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@confound_0.8_b50@pc@fpn\endcsname{4}
\expandafter\def\csname res@v5d@confound_0.8_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b50@pc@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@confound_0.8_b50@pc@prec\endcsname{0.43}
\expandafter\def\csname res@v5d@confound_0.8_b50@pc@ab\endcsname{1}
\expandafter\def\csname res@v5d@confound_0.8_b50@pc@bw\endcsname{1}
\expandafter\def\csname res@v5d@confound_0.8_b50@pc@len\endcsname{3.5}
\expandafter\def\csname res@v5d@confound_0.8_b50@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v5d@confound_0.8_b50@pc@map\endcsname{0.33}
\expandafter\def\csname res@v5d@confound_0.8_b50@dynotears@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@confound_0.8_b50@dynotears@fpn\endcsname{3}
\expandafter\def\csname res@v5d@confound_0.8_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b50@dynotears@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@confound_0.8_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@confound_0.8_b50@dynotears@ab\endcsname{7}
\expandafter\def\csname res@v5d@confound_0.8_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@dynotears@len\endcsname{0.3}
\expandafter\def\csname res@v5d@confound_0.8_b50@dynotears@rp\endcsname{0.77}
\expandafter\def\csname res@v5d@confound_0.8_b50@dynotears@map\endcsname{0.88}
\expandafter\def\csname res@v5d@confound_0.8_b50@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@confound_0.8_b50@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v5d@confound_0.8_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b50@doubleml@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@confound_0.8_b50@doubleml@prec\endcsname{0.72}
\expandafter\def\csname res@v5d@confound_0.8_b50@doubleml@ab\endcsname{2}
\expandafter\def\csname res@v5d@confound_0.8_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@doubleml@len\endcsname{2.1}
\expandafter\def\csname res@v5d@confound_0.8_b50@doubleml@rp\endcsname{0.62}
\expandafter\def\csname res@v5d@confound_0.8_b50@doubleml@map\endcsname{0.75}
\expandafter\def\csname res@v5d@confound_0.8_b50@varlingam@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@confound_0.8_b50@varlingam@fpn\endcsname{7}
\expandafter\def\csname res@v5d@confound_0.8_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b50@varlingam@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@confound_0.8_b50@varlingam@prec\endcsname{0.39}
\expandafter\def\csname res@v5d@confound_0.8_b50@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v5d@confound_0.8_b50@varlingam@len\endcsname{5.0}
\expandafter\def\csname res@v5d@confound_0.8_b50@varlingam@rp\endcsname{0.48}
\expandafter\def\csname res@v5d@confound_0.8_b50@varlingam@map\endcsname{0.61}
\expandafter\def\csname res@v5d@confound_0.8_b50@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@confound_0.8_b50@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v5d@confound_0.8_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b50@spacetime_rule@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@confound_0.8_b50@spacetime_rule@prec\endcsname{0.50}
\expandafter\def\csname res@v5d@confound_0.8_b50@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v5d@confound_0.8_b50@spacetime_rule@rp\endcsname{0.51}
\expandafter\def\csname res@v5d@confound_0.8_b50@spacetime_rule@map\endcsname{0.57}
\expandafter\def\csname res@v5d@confound_0.8_b50@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@confound_0.8_b50@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@confound_0.8_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b50@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@confound_0.8_b50@varsort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@confound_0.8_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@confound_0.8_b50@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v5d@confound_0.8_b50@varsort@map\endcsname{0.19}
\expandafter\def\csname res@v5d@confound_0.8_b50@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@confound_0.8_b50@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b50@r2sort@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@confound_0.8_b50@r2sort@prec\endcsname{0.08}
\expandafter\def\csname res@v5d@confound_0.8_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b50@r2sort@bw\endcsname{3}
\expandafter\def\csname res@v5d@confound_0.8_b50@r2sort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@confound_0.8_b50@r2sort@rp\endcsname{0.08}
\expandafter\def\csname res@v5d@confound_0.8_b50@r2sort@map\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_hard_b50@correlation@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@combo_hard_b50@correlation@fpn\endcsname{5}
\expandafter\def\csname res@v5d@combo_hard_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@correlation@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@combo_hard_b50@correlation@prec\endcsname{0.16}
\expandafter\def\csname res@v5d@combo_hard_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b50@correlation@bw\endcsname{5}
\expandafter\def\csname res@v5d@combo_hard_b50@correlation@len\endcsname{14.8}
\expandafter\def\csname res@v5d@combo_hard_b50@correlation@rp\endcsname{0.27}
\expandafter\def\csname res@v5d@combo_hard_b50@correlation@map\endcsname{0.50}
\expandafter\def\csname res@v5d@combo_hard_b50@granger@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@combo_hard_b50@granger@fpn\endcsname{6}
\expandafter\def\csname res@v5d@combo_hard_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@granger@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@combo_hard_b50@granger@prec\endcsname{0.41}
\expandafter\def\csname res@v5d@combo_hard_b50@granger@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b50@granger@len\endcsname{6.2}
\expandafter\def\csname res@v5d@combo_hard_b50@granger@rp\endcsname{0.48}
\expandafter\def\csname res@v5d@combo_hard_b50@granger@map\endcsname{0.63}
\expandafter\def\csname res@v5d@combo_hard_b50@pcmciplus@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@combo_hard_b50@pcmciplus@fpn\endcsname{6}
\expandafter\def\csname res@v5d@combo_hard_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@pcmciplus@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@combo_hard_b50@pcmciplus@prec\endcsname{0.86}
\expandafter\def\csname res@v5d@combo_hard_b50@pcmciplus@ab\endcsname{3}
\expandafter\def\csname res@v5d@combo_hard_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b50@pcmciplus@len\endcsname{1.2}
\expandafter\def\csname res@v5d@combo_hard_b50@pcmciplus@rp\endcsname{0.72}
\expandafter\def\csname res@v5d@combo_hard_b50@pcmciplus@map\endcsname{0.74}
\expandafter\def\csname res@v5d@combo_hard_b50@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_hard_b50@pc@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_hard_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@combo_hard_b50@pc@prec\endcsname{0.39}
\expandafter\def\csname res@v5d@combo_hard_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b50@pc@bw\endcsname{6}
\expandafter\def\csname res@v5d@combo_hard_b50@pc@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_hard_b50@pc@rp\endcsname{0.29}
\expandafter\def\csname res@v5d@combo_hard_b50@pc@map\endcsname{0.28}
\expandafter\def\csname res@v5d@combo_hard_b50@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_hard_b50@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_hard_b50@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@combo_hard_b50@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b50@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@combo_hard_b50@dynotears@rp\endcsname{0.70}
\expandafter\def\csname res@v5d@combo_hard_b50@dynotears@map\endcsname{0.79}
\expandafter\def\csname res@v5d@combo_hard_b50@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_hard_b50@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@combo_hard_b50@doubleml@prec\endcsname{0.25}
\expandafter\def\csname res@v5d@combo_hard_b50@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v5d@combo_hard_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b50@doubleml@len\endcsname{0.5}
\expandafter\def\csname res@v5d@combo_hard_b50@doubleml@rp\endcsname{0.43}
\expandafter\def\csname res@v5d@combo_hard_b50@doubleml@map\endcsname{0.48}
\expandafter\def\csname res@v5d@combo_hard_b50@varlingam@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@combo_hard_b50@varlingam@fpn\endcsname{4}
\expandafter\def\csname res@v5d@combo_hard_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@varlingam@tt\endcsname{0.31}
\expandafter\def\csname res@v5d@combo_hard_b50@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v5d@combo_hard_b50@varlingam@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b50@varlingam@bw\endcsname{4}
\expandafter\def\csname res@v5d@combo_hard_b50@varlingam@len\endcsname{5.9}
\expandafter\def\csname res@v5d@combo_hard_b50@varlingam@rp\endcsname{0.27}
\expandafter\def\csname res@v5d@combo_hard_b50@varlingam@map\endcsname{0.44}
\expandafter\def\csname res@v5d@combo_hard_b50@spacetime_rule@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_hard_b50@spacetime_rule@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_hard_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@spacetime_rule@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_hard_b50@spacetime_rule@prec\endcsname{0.28}
\expandafter\def\csname res@v5d@combo_hard_b50@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b50@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b50@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v5d@combo_hard_b50@spacetime_rule@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@combo_hard_b50@spacetime_rule@map\endcsname{0.41}
\expandafter\def\csname res@v5d@combo_hard_b50@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_hard_b50@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_hard_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_hard_b50@varsort@prec\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_hard_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b50@varsort@bw\endcsname{2}
\expandafter\def\csname res@v5d@combo_hard_b50@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@combo_hard_b50@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_hard_b50@varsort@map\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_hard_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_hard_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b50@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_hard_b50@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@combo_hard_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b50@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_hard_b50@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_hard_b50@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v5d@combo_extreme_b50@correlation@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_extreme_b50@correlation@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_extreme_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@correlation@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@combo_extreme_b50@correlation@prec\endcsname{0.16}
\expandafter\def\csname res@v5d@combo_extreme_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@correlation@bw\endcsname{7}
\expandafter\def\csname res@v5d@combo_extreme_b50@correlation@len\endcsname{13.6}
\expandafter\def\csname res@v5d@combo_extreme_b50@correlation@rp\endcsname{0.25}
\expandafter\def\csname res@v5d@combo_extreme_b50@correlation@map\endcsname{0.43}
\expandafter\def\csname res@v5d@combo_extreme_b50@granger@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@combo_extreme_b50@granger@fpn\endcsname{5}
\expandafter\def\csname res@v5d@combo_extreme_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@granger@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@combo_extreme_b50@granger@prec\endcsname{0.36}
\expandafter\def\csname res@v5d@combo_extreme_b50@granger@ab\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@granger@len\endcsname{6.6}
\expandafter\def\csname res@v5d@combo_extreme_b50@granger@rp\endcsname{0.51}
\expandafter\def\csname res@v5d@combo_extreme_b50@granger@map\endcsname{0.62}
\expandafter\def\csname res@v5d@combo_extreme_b50@pcmciplus@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@combo_extreme_b50@pcmciplus@fpn\endcsname{4}
\expandafter\def\csname res@v5d@combo_extreme_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@pcmciplus@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_extreme_b50@pcmciplus@prec\endcsname{0.58}
\expandafter\def\csname res@v5d@combo_extreme_b50@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v5d@combo_extreme_b50@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b50@pcmciplus@len\endcsname{0.7}
\expandafter\def\csname res@v5d@combo_extreme_b50@pcmciplus@rp\endcsname{0.34}
\expandafter\def\csname res@v5d@combo_extreme_b50@pcmciplus@map\endcsname{0.53}
\expandafter\def\csname res@v5d@combo_extreme_b50@pc@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_extreme_b50@pc@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@pc@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_extreme_b50@pc@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_extreme_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@pc@bw\endcsname{9}
\expandafter\def\csname res@v5d@combo_extreme_b50@pc@len\endcsname{2.5}
\expandafter\def\csname res@v5d@combo_extreme_b50@pc@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b50@pc@map\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_extreme_b50@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_extreme_b50@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_extreme_b50@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@combo_extreme_b50@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@combo_extreme_b50@dynotears@rp\endcsname{0.59}
\expandafter\def\csname res@v5d@combo_extreme_b50@dynotears@map\endcsname{0.68}
\expandafter\def\csname res@v5d@combo_extreme_b50@doubleml@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_extreme_b50@doubleml@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@doubleml@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_extreme_b50@doubleml@prec\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_extreme_b50@doubleml@ab\endcsname{8}
\expandafter\def\csname res@v5d@combo_extreme_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@doubleml@len\endcsname{0.2}
\expandafter\def\csname res@v5d@combo_extreme_b50@doubleml@rp\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_extreme_b50@doubleml@map\endcsname{0.30}
\expandafter\def\csname res@v5d@combo_extreme_b50@varlingam@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_extreme_b50@varlingam@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@varlingam@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_extreme_b50@varlingam@prec\endcsname{0.21}
\expandafter\def\csname res@v5d@combo_extreme_b50@varlingam@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b50@varlingam@bw\endcsname{7}
\expandafter\def\csname res@v5d@combo_extreme_b50@varlingam@len\endcsname{5.3}
\expandafter\def\csname res@v5d@combo_extreme_b50@varlingam@rp\endcsname{0.22}
\expandafter\def\csname res@v5d@combo_extreme_b50@varlingam@map\endcsname{0.26}
\expandafter\def\csname res@v5d@combo_extreme_b50@spacetime_rule@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_extreme_b50@spacetime_rule@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_extreme_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@spacetime_rule@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_extreme_b50@spacetime_rule@prec\endcsname{0.44}
\expandafter\def\csname res@v5d@combo_extreme_b50@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@spacetime_rule@len\endcsname{1.0}
\expandafter\def\csname res@v5d@combo_extreme_b50@spacetime_rule@rp\endcsname{0.22}
\expandafter\def\csname res@v5d@combo_extreme_b50@spacetime_rule@map\endcsname{0.34}
\expandafter\def\csname res@v5d@combo_extreme_b50@varsort@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_extreme_b50@varsort@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_extreme_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@varsort@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@combo_extreme_b50@varsort@prec\endcsname{0.27}
\expandafter\def\csname res@v5d@combo_extreme_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@varsort@bw\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b50@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@combo_extreme_b50@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v5d@combo_extreme_b50@varsort@map\endcsname{0.25}
\expandafter\def\csname res@v5d@combo_extreme_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_extreme_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b50@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_extreme_b50@r2sort@prec\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_extreme_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b50@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b50@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_extreme_b50@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_extreme_b50@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v5d@interaction_1.0_b50@correlation@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@correlation@fpn\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@correlation@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@interaction_1.0_b50@correlation@prec\endcsname{0.20}
\expandafter\def\csname res@v5d@interaction_1.0_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@correlation@bw\endcsname{7}
\expandafter\def\csname res@v5d@interaction_1.0_b50@correlation@len\endcsname{5.8}
\expandafter\def\csname res@v5d@interaction_1.0_b50@correlation@rp\endcsname{0.22}
\expandafter\def\csname res@v5d@interaction_1.0_b50@correlation@map\endcsname{0.36}
\expandafter\def\csname res@v5d@interaction_1.0_b50@granger@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@granger@fpn\endcsname{3}
\expandafter\def\csname res@v5d@interaction_1.0_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@granger@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@interaction_1.0_b50@granger@prec\endcsname{0.19}
\expandafter\def\csname res@v5d@interaction_1.0_b50@granger@ab\endcsname{4}
\expandafter\def\csname res@v5d@interaction_1.0_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@granger@len\endcsname{4.1}
\expandafter\def\csname res@v5d@interaction_1.0_b50@granger@rp\endcsname{0.35}
\expandafter\def\csname res@v5d@interaction_1.0_b50@granger@map\endcsname{0.44}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pcmciplus@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pcmciplus@fpn\endcsname{6}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pcmciplus@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pcmciplus@prec\endcsname{0.58}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pcmciplus@len\endcsname{1.4}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pcmciplus@rp\endcsname{0.49}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pcmciplus@map\endcsname{0.60}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pc@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pc@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pc@bw\endcsname{6}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pc@len\endcsname{2.9}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pc@rp\endcsname{0.14}
\expandafter\def\csname res@v5d@interaction_1.0_b50@pc@map\endcsname{0.19}
\expandafter\def\csname res@v5d@interaction_1.0_b50@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@interaction_1.0_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@interaction_1.0_b50@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v5d@interaction_1.0_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v5d@interaction_1.0_b50@dynotears@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@interaction_1.0_b50@dynotears@map\endcsname{0.44}
\expandafter\def\csname res@v5d@interaction_1.0_b50@doubleml@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@doubleml@fpn\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@doubleml@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@interaction_1.0_b50@doubleml@prec\endcsname{0.40}
\expandafter\def\csname res@v5d@interaction_1.0_b50@doubleml@ab\endcsname{5}
\expandafter\def\csname res@v5d@interaction_1.0_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@doubleml@len\endcsname{0.6}
\expandafter\def\csname res@v5d@interaction_1.0_b50@doubleml@rp\endcsname{0.22}
\expandafter\def\csname res@v5d@interaction_1.0_b50@doubleml@map\endcsname{0.37}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varlingam@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varlingam@fpn\endcsname{3}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varlingam@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varlingam@prec\endcsname{0.35}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varlingam@ab\endcsname{4}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varlingam@len\endcsname{1.7}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varlingam@rp\endcsname{0.29}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varlingam@map\endcsname{0.40}
\expandafter\def\csname res@v5d@interaction_1.0_b50@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v5d@interaction_1.0_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@spacetime_rule@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@interaction_1.0_b50@spacetime_rule@prec\endcsname{0.80}
\expandafter\def\csname res@v5d@interaction_1.0_b50@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v5d@interaction_1.0_b50@spacetime_rule@rp\endcsname{0.62}
\expandafter\def\csname res@v5d@interaction_1.0_b50@spacetime_rule@map\endcsname{0.70}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varsort@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varsort@prec\endcsname{0.07}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varsort@rp\endcsname{0.06}
\expandafter\def\csname res@v5d@interaction_1.0_b50@varsort@map\endcsname{0.14}
\expandafter\def\csname res@v5d@interaction_1.0_b50@r2sort@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@r2sort@fpn\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b50@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@interaction_1.0_b50@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@interaction_1.0_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@interaction_1.0_b50@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v5d@interaction_1.0_b50@r2sort@map\endcsname{0.22}
\expandafter\def\csname res@v5d@combo_interaction_b50@correlation@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b50@correlation@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@correlation@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_interaction_b50@correlation@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@combo_interaction_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@correlation@bw\endcsname{9}
\expandafter\def\csname res@v5d@combo_interaction_b50@correlation@len\endcsname{4.9}
\expandafter\def\csname res@v5d@combo_interaction_b50@correlation@rp\endcsname{0.05}
\expandafter\def\csname res@v5d@combo_interaction_b50@correlation@map\endcsname{0.30}
\expandafter\def\csname res@v5d@combo_interaction_b50@granger@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_interaction_b50@granger@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@granger@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_interaction_b50@granger@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_interaction_b50@granger@ab\endcsname{7}
\expandafter\def\csname res@v5d@combo_interaction_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@granger@len\endcsname{2.7}
\expandafter\def\csname res@v5d@combo_interaction_b50@granger@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@combo_interaction_b50@granger@map\endcsname{0.39}
\expandafter\def\csname res@v5d@combo_interaction_b50@pcmciplus@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_interaction_b50@pcmciplus@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_interaction_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@pcmciplus@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b50@pcmciplus@prec\endcsname{0.62}
\expandafter\def\csname res@v5d@combo_interaction_b50@pcmciplus@ab\endcsname{6}
\expandafter\def\csname res@v5d@combo_interaction_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@pcmciplus@len\endcsname{0.5}
\expandafter\def\csname res@v5d@combo_interaction_b50@pcmciplus@rp\endcsname{0.31}
\expandafter\def\csname res@v5d@combo_interaction_b50@pcmciplus@map\endcsname{0.41}
\expandafter\def\csname res@v5d@combo_interaction_b50@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_interaction_b50@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@pc@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b50@pc@prec\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@pc@bw\endcsname{6}
\expandafter\def\csname res@v5d@combo_interaction_b50@pc@len\endcsname{2.4}
\expandafter\def\csname res@v5d@combo_interaction_b50@pc@rp\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_interaction_b50@pc@map\endcsname{0.20}
\expandafter\def\csname res@v5d@combo_interaction_b50@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_interaction_b50@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_interaction_b50@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@combo_interaction_b50@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@combo_interaction_b50@dynotears@rp\endcsname{0.29}
\expandafter\def\csname res@v5d@combo_interaction_b50@dynotears@map\endcsname{0.34}
\expandafter\def\csname res@v5d@combo_interaction_b50@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b50@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@doubleml@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@combo_interaction_b50@doubleml@prec\endcsname{0.75}
\expandafter\def\csname res@v5d@combo_interaction_b50@doubleml@ab\endcsname{8}
\expandafter\def\csname res@v5d@combo_interaction_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@doubleml@len\endcsname{0.3}
\expandafter\def\csname res@v5d@combo_interaction_b50@doubleml@rp\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_interaction_b50@doubleml@map\endcsname{0.31}
\expandafter\def\csname res@v5d@combo_interaction_b50@varlingam@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b50@varlingam@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@varlingam@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b50@varlingam@prec\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_interaction_b50@varlingam@ab\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b50@varlingam@bw\endcsname{4}
\expandafter\def\csname res@v5d@combo_interaction_b50@varlingam@len\endcsname{1.8}
\expandafter\def\csname res@v5d@combo_interaction_b50@varlingam@rp\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_interaction_b50@varlingam@map\endcsname{0.27}
\expandafter\def\csname res@v5d@combo_interaction_b50@spacetime_rule@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_interaction_b50@spacetime_rule@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@spacetime_rule@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@combo_interaction_b50@spacetime_rule@prec\endcsname{0.29}
\expandafter\def\csname res@v5d@combo_interaction_b50@spacetime_rule@ab\endcsname{3}
\expandafter\def\csname res@v5d@combo_interaction_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@spacetime_rule@len\endcsname{0.7}
\expandafter\def\csname res@v5d@combo_interaction_b50@spacetime_rule@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@combo_interaction_b50@spacetime_rule@map\endcsname{0.36}
\expandafter\def\csname res@v5d@combo_interaction_b50@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_interaction_b50@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_interaction_b50@varsort@prec\endcsname{0.18}
\expandafter\def\csname res@v5d@combo_interaction_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@combo_interaction_b50@varsort@rp\endcsname{0.13}
\expandafter\def\csname res@v5d@combo_interaction_b50@varsort@map\endcsname{0.20}
\expandafter\def\csname res@v5d@combo_interaction_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b50@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b50@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@combo_interaction_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b50@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_interaction_b50@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_interaction_b50@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v5d@control_weak_b50@correlation@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@control_weak_b50@correlation@fpn\endcsname{5}
\expandafter\def\csname res@v5d@control_weak_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@correlation@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@control_weak_b50@correlation@prec\endcsname{0.23}
\expandafter\def\csname res@v5d@control_weak_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@correlation@bw\endcsname{5}
\expandafter\def\csname res@v5d@control_weak_b50@correlation@len\endcsname{8.2}
\expandafter\def\csname res@v5d@control_weak_b50@correlation@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@control_weak_b50@correlation@map\endcsname{0.49}
\expandafter\def\csname res@v5d@control_weak_b50@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@control_weak_b50@granger@fpn\endcsname{8}
\expandafter\def\csname res@v5d@control_weak_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v5d@control_weak_b50@granger@prec\endcsname{0.60}
\expandafter\def\csname res@v5d@control_weak_b50@granger@ab\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@granger@len\endcsname{3.2}
\expandafter\def\csname res@v5d@control_weak_b50@granger@rp\endcsname{0.60}
\expandafter\def\csname res@v5d@control_weak_b50@granger@map\endcsname{0.75}
\expandafter\def\csname res@v5d@control_weak_b50@pcmciplus@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@control_weak_b50@pcmciplus@fpn\endcsname{8}
\expandafter\def\csname res@v5d@control_weak_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@pcmciplus@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@control_weak_b50@pcmciplus@prec\endcsname{0.83}
\expandafter\def\csname res@v5d@control_weak_b50@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v5d@control_weak_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@pcmciplus@len\endcsname{1.6}
\expandafter\def\csname res@v5d@control_weak_b50@pcmciplus@rp\endcsname{0.70}
\expandafter\def\csname res@v5d@control_weak_b50@pcmciplus@map\endcsname{0.78}
\expandafter\def\csname res@v5d@control_weak_b50@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@control_weak_b50@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@control_weak_b50@pc@prec\endcsname{0.28}
\expandafter\def\csname res@v5d@control_weak_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@pc@bw\endcsname{7}
\expandafter\def\csname res@v5d@control_weak_b50@pc@len\endcsname{3.9}
\expandafter\def\csname res@v5d@control_weak_b50@pc@rp\endcsname{0.26}
\expandafter\def\csname res@v5d@control_weak_b50@pc@map\endcsname{0.26}
\expandafter\def\csname res@v5d@control_weak_b50@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@control_weak_b50@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@control_weak_b50@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@control_weak_b50@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@control_weak_b50@dynotears@rp\endcsname{0.51}
\expandafter\def\csname res@v5d@control_weak_b50@dynotears@map\endcsname{0.69}
\expandafter\def\csname res@v5d@control_weak_b50@doubleml@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@control_weak_b50@doubleml@fpn\endcsname{6}
\expandafter\def\csname res@v5d@control_weak_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@doubleml@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@control_weak_b50@doubleml@prec\endcsname{0.79}
\expandafter\def\csname res@v5d@control_weak_b50@doubleml@ab\endcsname{4}
\expandafter\def\csname res@v5d@control_weak_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@doubleml@len\endcsname{1.5}
\expandafter\def\csname res@v5d@control_weak_b50@doubleml@rp\endcsname{0.54}
\expandafter\def\csname res@v5d@control_weak_b50@doubleml@map\endcsname{0.62}
\expandafter\def\csname res@v5d@control_weak_b50@varlingam@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@control_weak_b50@varlingam@fpn\endcsname{5}
\expandafter\def\csname res@v5d@control_weak_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@varlingam@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@control_weak_b50@varlingam@prec\endcsname{0.54}
\expandafter\def\csname res@v5d@control_weak_b50@varlingam@ab\endcsname{4}
\expandafter\def\csname res@v5d@control_weak_b50@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b50@varlingam@len\endcsname{2.6}
\expandafter\def\csname res@v5d@control_weak_b50@varlingam@rp\endcsname{0.60}
\expandafter\def\csname res@v5d@control_weak_b50@varlingam@map\endcsname{0.70}
\expandafter\def\csname res@v5d@control_weak_b50@spacetime_rule@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@control_weak_b50@spacetime_rule@fpn\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@spacetime_rule@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@control_weak_b50@spacetime_rule@prec\endcsname{--}
\expandafter\def\csname res@v5d@control_weak_b50@spacetime_rule@ab\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@spacetime_rule@len\endcsname{0.0}
\expandafter\def\csname res@v5d@control_weak_b50@spacetime_rule@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@control_weak_b50@spacetime_rule@map\endcsname{0.43}
\expandafter\def\csname res@v5d@control_weak_b50@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@control_weak_b50@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@varsort@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@control_weak_b50@varsort@prec\endcsname{0.07}
\expandafter\def\csname res@v5d@control_weak_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@control_weak_b50@varsort@rp\endcsname{0.10}
\expandafter\def\csname res@v5d@control_weak_b50@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v5d@control_weak_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@control_weak_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b50@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@control_weak_b50@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@control_weak_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@control_weak_b50@r2sort@rp\endcsname{0.15}
\expandafter\def\csname res@v5d@control_weak_b50@r2sort@map\endcsname{0.28}
\expandafter\def\csname res@v5d@default_b100@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@default_b100@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v5d@default_b100@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@correlation@tt\endcsname{0.77}
\expandafter\def\csname res@v5d@default_b100@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v5d@default_b100@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@correlation@bw\endcsname{1}
\expandafter\def\csname res@v5d@default_b100@correlation@len\endcsname{17.3}
\expandafter\def\csname res@v5d@default_b100@correlation@rp\endcsname{0.79}
\expandafter\def\csname res@v5d@default_b100@correlation@map\endcsname{0.83}
\expandafter\def\csname res@v5d@default_b100@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@default_b100@granger@fpn\endcsname{9}
\expandafter\def\csname res@v5d@default_b100@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v5d@default_b100@granger@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@default_b100@granger@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@granger@len\endcsname{14.6}
\expandafter\def\csname res@v5d@default_b100@granger@rp\endcsname{0.68}
\expandafter\def\csname res@v5d@default_b100@granger@map\endcsname{0.76}
\expandafter\def\csname res@v5d@default_b100@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v5d@default_b100@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@pcmciplus@tt\endcsname{0.81}
\expandafter\def\csname res@v5d@default_b100@pcmciplus@prec\endcsname{0.78}
\expandafter\def\csname res@v5d@default_b100@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@pcmciplus@len\endcsname{3.0}
\expandafter\def\csname res@v5d@default_b100@pcmciplus@rp\endcsname{0.92}
\expandafter\def\csname res@v5d@default_b100@pcmciplus@map\endcsname{0.96}
\expandafter\def\csname res@v5d@default_b100@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@default_b100@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5d@default_b100@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@pc@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@default_b100@pc@prec\endcsname{0.37}
\expandafter\def\csname res@v5d@default_b100@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@pc@bw\endcsname{5}
\expandafter\def\csname res@v5d@default_b100@pc@len\endcsname{4.6}
\expandafter\def\csname res@v5d@default_b100@pc@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@default_b100@pc@map\endcsname{0.31}
\expandafter\def\csname res@v5d@default_b100@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@default_b100@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v5d@default_b100@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@dynotears@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@default_b100@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@default_b100@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v5d@default_b100@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v5d@default_b100@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v5d@default_b100@dynotears@map\endcsname{0.93}
\expandafter\def\csname res@v5d@default_b100@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v5d@default_b100@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@doubleml@tt\endcsname{0.77}
\expandafter\def\csname res@v5d@default_b100@doubleml@prec\endcsname{0.83}
\expandafter\def\csname res@v5d@default_b100@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@doubleml@len\endcsname{3.1}
\expandafter\def\csname res@v5d@default_b100@doubleml@rp\endcsname{0.76}
\expandafter\def\csname res@v5d@default_b100@doubleml@map\endcsname{0.88}
\expandafter\def\csname res@v5d@default_b100@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v5d@default_b100@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@varlingam@tt\endcsname{0.73}
\expandafter\def\csname res@v5d@default_b100@varlingam@prec\endcsname{0.27}
\expandafter\def\csname res@v5d@default_b100@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@varlingam@len\endcsname{9.5}
\expandafter\def\csname res@v5d@default_b100@varlingam@rp\endcsname{0.83}
\expandafter\def\csname res@v5d@default_b100@varlingam@map\endcsname{0.87}
\expandafter\def\csname res@v5d@default_b100@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@default_b100@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v5d@default_b100@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@default_b100@spacetime_rule@prec\endcsname{0.94}
\expandafter\def\csname res@v5d@default_b100@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v5d@default_b100@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v5d@default_b100@spacetime_rule@rp\endcsname{0.54}
\expandafter\def\csname res@v5d@default_b100@spacetime_rule@map\endcsname{0.71}
\expandafter\def\csname res@v5d@default_b100@varsort@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@default_b100@varsort@fpn\endcsname{3}
\expandafter\def\csname res@v5d@default_b100@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@default_b100@varsort@prec\endcsname{0.20}
\expandafter\def\csname res@v5d@default_b100@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@default_b100@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v5d@default_b100@varsort@map\endcsname{0.19}
\expandafter\def\csname res@v5d@default_b100@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@default_b100@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@default_b100@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@default_b100@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@default_b100@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@default_b100@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@default_b100@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@default_b100@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@default_b100@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5d@signal_0.1_b100@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@signal_0.1_b100@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@correlation@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@signal_0.1_b100@correlation@prec\endcsname{0.21}
\expandafter\def\csname res@v5d@signal_0.1_b100@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@correlation@bw\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@correlation@len\endcsname{11.2}
\expandafter\def\csname res@v5d@signal_0.1_b100@correlation@rp\endcsname{0.26}
\expandafter\def\csname res@v5d@signal_0.1_b100@correlation@map\endcsname{0.41}
\expandafter\def\csname res@v5d@signal_0.1_b100@granger@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@signal_0.1_b100@granger@fpn\endcsname{7}
\expandafter\def\csname res@v5d@signal_0.1_b100@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@signal_0.1_b100@granger@prec\endcsname{0.47}
\expandafter\def\csname res@v5d@signal_0.1_b100@granger@ab\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b100@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@granger@len\endcsname{4.6}
\expandafter\def\csname res@v5d@signal_0.1_b100@granger@rp\endcsname{0.56}
\expandafter\def\csname res@v5d@signal_0.1_b100@granger@map\endcsname{0.68}
\expandafter\def\csname res@v5d@signal_0.1_b100@pcmciplus@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@signal_0.1_b100@pcmciplus@fpn\endcsname{8}
\expandafter\def\csname res@v5d@signal_0.1_b100@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@pcmciplus@tt\endcsname{0.31}
\expandafter\def\csname res@v5d@signal_0.1_b100@pcmciplus@prec\endcsname{0.67}
\expandafter\def\csname res@v5d@signal_0.1_b100@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v5d@signal_0.1_b100@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@pcmciplus@len\endcsname{1.4}
\expandafter\def\csname res@v5d@signal_0.1_b100@pcmciplus@rp\endcsname{0.64}
\expandafter\def\csname res@v5d@signal_0.1_b100@pcmciplus@map\endcsname{0.70}
\expandafter\def\csname res@v5d@signal_0.1_b100@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@signal_0.1_b100@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5d@signal_0.1_b100@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v5d@signal_0.1_b100@pc@prec\endcsname{0.29}
\expandafter\def\csname res@v5d@signal_0.1_b100@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@pc@bw\endcsname{6}
\expandafter\def\csname res@v5d@signal_0.1_b100@pc@len\endcsname{3.8}
\expandafter\def\csname res@v5d@signal_0.1_b100@pc@rp\endcsname{0.26}
\expandafter\def\csname res@v5d@signal_0.1_b100@pc@map\endcsname{0.24}
\expandafter\def\csname res@v5d@signal_0.1_b100@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@signal_0.1_b100@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@signal_0.1_b100@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@signal_0.1_b100@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@signal_0.1_b100@dynotears@rp\endcsname{0.66}
\expandafter\def\csname res@v5d@signal_0.1_b100@dynotears@map\endcsname{0.77}
\expandafter\def\csname res@v5d@signal_0.1_b100@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@signal_0.1_b100@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b100@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@doubleml@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@signal_0.1_b100@doubleml@prec\endcsname{0.75}
\expandafter\def\csname res@v5d@signal_0.1_b100@doubleml@ab\endcsname{8}
\expandafter\def\csname res@v5d@signal_0.1_b100@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@doubleml@len\endcsname{0.3}
\expandafter\def\csname res@v5d@signal_0.1_b100@doubleml@rp\endcsname{0.42}
\expandafter\def\csname res@v5d@signal_0.1_b100@doubleml@map\endcsname{0.51}
\expandafter\def\csname res@v5d@signal_0.1_b100@varlingam@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@signal_0.1_b100@varlingam@fpn\endcsname{3}
\expandafter\def\csname res@v5d@signal_0.1_b100@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@varlingam@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@signal_0.1_b100@varlingam@prec\endcsname{0.36}
\expandafter\def\csname res@v5d@signal_0.1_b100@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@varlingam@bw\endcsname{7}
\expandafter\def\csname res@v5d@signal_0.1_b100@varlingam@len\endcsname{5.0}
\expandafter\def\csname res@v5d@signal_0.1_b100@varlingam@rp\endcsname{0.34}
\expandafter\def\csname res@v5d@signal_0.1_b100@varlingam@map\endcsname{0.44}
\expandafter\def\csname res@v5d@signal_0.1_b100@spacetime_rule@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@signal_0.1_b100@spacetime_rule@fpn\endcsname{2}
\expandafter\def\csname res@v5d@signal_0.1_b100@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@spacetime_rule@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@signal_0.1_b100@spacetime_rule@prec\endcsname{0.33}
\expandafter\def\csname res@v5d@signal_0.1_b100@spacetime_rule@ab\endcsname{4}
\expandafter\def\csname res@v5d@signal_0.1_b100@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@spacetime_rule@len\endcsname{0.6}
\expandafter\def\csname res@v5d@signal_0.1_b100@spacetime_rule@rp\endcsname{0.30}
\expandafter\def\csname res@v5d@signal_0.1_b100@spacetime_rule@map\endcsname{0.35}
\expandafter\def\csname res@v5d@signal_0.1_b100@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@signal_0.1_b100@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v5d@signal_0.1_b100@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@signal_0.1_b100@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@signal_0.1_b100@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@varsort@bw\endcsname{2}
\expandafter\def\csname res@v5d@signal_0.1_b100@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@signal_0.1_b100@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v5d@signal_0.1_b100@varsort@map\endcsname{0.17}
\expandafter\def\csname res@v5d@signal_0.1_b100@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@signal_0.1_b100@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b100@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@signal_0.1_b100@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@signal_0.1_b100@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@signal_0.1_b100@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@signal_0.1_b100@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@signal_0.1_b100@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@signal_0.1_b100@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@signal_0.1_b100@r2sort@map\endcsname{0.19}
\expandafter\def\csname res@v5d@echo_0.8_b100@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@echo_0.8_b100@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v5d@echo_0.8_b100@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b100@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@echo_0.8_b100@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v5d@echo_0.8_b100@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@correlation@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@correlation@len\endcsname{18.2}
\expandafter\def\csname res@v5d@echo_0.8_b100@correlation@rp\endcsname{0.63}
\expandafter\def\csname res@v5d@echo_0.8_b100@correlation@map\endcsname{0.76}
\expandafter\def\csname res@v5d@echo_0.8_b100@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@echo_0.8_b100@granger@fpn\endcsname{9}
\expandafter\def\csname res@v5d@echo_0.8_b100@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b100@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v5d@echo_0.8_b100@granger@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@echo_0.8_b100@granger@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@granger@len\endcsname{14.8}
\expandafter\def\csname res@v5d@echo_0.8_b100@granger@rp\endcsname{0.53}
\expandafter\def\csname res@v5d@echo_0.8_b100@granger@map\endcsname{0.72}
\expandafter\def\csname res@v5d@echo_0.8_b100@pcmciplus@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@echo_0.8_b100@pcmciplus@fpn\endcsname{7}
\expandafter\def\csname res@v5d@echo_0.8_b100@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b100@pcmciplus@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@echo_0.8_b100@pcmciplus@prec\endcsname{0.78}
\expandafter\def\csname res@v5d@echo_0.8_b100@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b100@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@pcmciplus@len\endcsname{2.2}
\expandafter\def\csname res@v5d@echo_0.8_b100@pcmciplus@rp\endcsname{0.84}
\expandafter\def\csname res@v5d@echo_0.8_b100@pcmciplus@map\endcsname{0.86}
\expandafter\def\csname res@v5d@echo_0.8_b100@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@echo_0.8_b100@pc@fpn\endcsname{3}
\expandafter\def\csname res@v5d@echo_0.8_b100@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b100@pc@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@echo_0.8_b100@pc@prec\endcsname{0.32}
\expandafter\def\csname res@v5d@echo_0.8_b100@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@pc@bw\endcsname{3}
\expandafter\def\csname res@v5d@echo_0.8_b100@pc@len\endcsname{4.7}
\expandafter\def\csname res@v5d@echo_0.8_b100@pc@rp\endcsname{0.31}
\expandafter\def\csname res@v5d@echo_0.8_b100@pc@map\endcsname{0.28}
\expandafter\def\csname res@v5d@echo_0.8_b100@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@echo_0.8_b100@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v5d@echo_0.8_b100@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b100@dynotears@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@echo_0.8_b100@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@echo_0.8_b100@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v5d@echo_0.8_b100@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@dynotears@len\endcsname{0.4}
\expandafter\def\csname res@v5d@echo_0.8_b100@dynotears@rp\endcsname{0.85}
\expandafter\def\csname res@v5d@echo_0.8_b100@dynotears@map\endcsname{0.88}
\expandafter\def\csname res@v5d@echo_0.8_b100@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@echo_0.8_b100@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v5d@echo_0.8_b100@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b100@doubleml@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@echo_0.8_b100@doubleml@prec\endcsname{0.67}
\expandafter\def\csname res@v5d@echo_0.8_b100@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b100@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@doubleml@len\endcsname{2.3}
\expandafter\def\csname res@v5d@echo_0.8_b100@doubleml@rp\endcsname{0.62}
\expandafter\def\csname res@v5d@echo_0.8_b100@doubleml@map\endcsname{0.75}
\expandafter\def\csname res@v5d@echo_0.8_b100@varlingam@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@echo_0.8_b100@varlingam@fpn\endcsname{8}
\expandafter\def\csname res@v5d@echo_0.8_b100@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b100@varlingam@tt\endcsname{0.54}
\expandafter\def\csname res@v5d@echo_0.8_b100@varlingam@prec\endcsname{0.24}
\expandafter\def\csname res@v5d@echo_0.8_b100@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v5d@echo_0.8_b100@varlingam@len\endcsname{9.6}
\expandafter\def\csname res@v5d@echo_0.8_b100@varlingam@rp\endcsname{0.55}
\expandafter\def\csname res@v5d@echo_0.8_b100@varlingam@map\endcsname{0.64}
\expandafter\def\csname res@v5d@echo_0.8_b100@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@echo_0.8_b100@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v5d@echo_0.8_b100@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b100@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v5d@echo_0.8_b100@spacetime_rule@prec\endcsname{0.70}
\expandafter\def\csname res@v5d@echo_0.8_b100@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v5d@echo_0.8_b100@spacetime_rule@rp\endcsname{0.54}
\expandafter\def\csname res@v5d@echo_0.8_b100@spacetime_rule@map\endcsname{0.64}
\expandafter\def\csname res@v5d@echo_0.8_b100@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@echo_0.8_b100@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v5d@echo_0.8_b100@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b100@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@echo_0.8_b100@varsort@prec\endcsname{0.18}
\expandafter\def\csname res@v5d@echo_0.8_b100@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b100@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@echo_0.8_b100@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@echo_0.8_b100@varsort@map\endcsname{0.19}
\expandafter\def\csname res@v5d@echo_0.8_b100@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@echo_0.8_b100@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@echo_0.8_b100@r2sort@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@echo_0.8_b100@r2sort@prec\endcsname{0.07}
\expandafter\def\csname res@v5d@echo_0.8_b100@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@echo_0.8_b100@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@echo_0.8_b100@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@echo_0.8_b100@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@echo_0.8_b100@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5d@confound_0.8_b100@correlation@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@confound_0.8_b100@correlation@fpn\endcsname{7}
\expandafter\def\csname res@v5d@confound_0.8_b100@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b100@correlation@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@confound_0.8_b100@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v5d@confound_0.8_b100@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@correlation@bw\endcsname{2}
\expandafter\def\csname res@v5d@confound_0.8_b100@correlation@len\endcsname{17.5}
\expandafter\def\csname res@v5d@confound_0.8_b100@correlation@rp\endcsname{0.47}
\expandafter\def\csname res@v5d@confound_0.8_b100@correlation@map\endcsname{0.58}
\expandafter\def\csname res@v5d@confound_0.8_b100@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@confound_0.8_b100@granger@fpn\endcsname{9}
\expandafter\def\csname res@v5d@confound_0.8_b100@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b100@granger@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@confound_0.8_b100@granger@prec\endcsname{0.16}
\expandafter\def\csname res@v5d@confound_0.8_b100@granger@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@granger@len\endcsname{14.9}
\expandafter\def\csname res@v5d@confound_0.8_b100@granger@rp\endcsname{0.52}
\expandafter\def\csname res@v5d@confound_0.8_b100@granger@map\endcsname{0.67}
\expandafter\def\csname res@v5d@confound_0.8_b100@pcmciplus@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@confound_0.8_b100@pcmciplus@fpn\endcsname{8}
\expandafter\def\csname res@v5d@confound_0.8_b100@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b100@pcmciplus@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@confound_0.8_b100@pcmciplus@prec\endcsname{0.64}
\expandafter\def\csname res@v5d@confound_0.8_b100@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v5d@confound_0.8_b100@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@pcmciplus@len\endcsname{2.5}
\expandafter\def\csname res@v5d@confound_0.8_b100@pcmciplus@rp\endcsname{0.69}
\expandafter\def\csname res@v5d@confound_0.8_b100@pcmciplus@map\endcsname{0.83}
\expandafter\def\csname res@v5d@confound_0.8_b100@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@confound_0.8_b100@pc@fpn\endcsname{4}
\expandafter\def\csname res@v5d@confound_0.8_b100@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b100@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@confound_0.8_b100@pc@prec\endcsname{0.47}
\expandafter\def\csname res@v5d@confound_0.8_b100@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@pc@bw\endcsname{2}
\expandafter\def\csname res@v5d@confound_0.8_b100@pc@len\endcsname{4.0}
\expandafter\def\csname res@v5d@confound_0.8_b100@pc@rp\endcsname{0.34}
\expandafter\def\csname res@v5d@confound_0.8_b100@pc@map\endcsname{0.34}
\expandafter\def\csname res@v5d@confound_0.8_b100@dynotears@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@confound_0.8_b100@dynotears@fpn\endcsname{3}
\expandafter\def\csname res@v5d@confound_0.8_b100@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b100@dynotears@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@confound_0.8_b100@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@confound_0.8_b100@dynotears@ab\endcsname{7}
\expandafter\def\csname res@v5d@confound_0.8_b100@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@dynotears@len\endcsname{0.3}
\expandafter\def\csname res@v5d@confound_0.8_b100@dynotears@rp\endcsname{0.79}
\expandafter\def\csname res@v5d@confound_0.8_b100@dynotears@map\endcsname{0.88}
\expandafter\def\csname res@v5d@confound_0.8_b100@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@confound_0.8_b100@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v5d@confound_0.8_b100@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b100@doubleml@tt\endcsname{0.62}
\expandafter\def\csname res@v5d@confound_0.8_b100@doubleml@prec\endcsname{0.82}
\expandafter\def\csname res@v5d@confound_0.8_b100@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v5d@confound_0.8_b100@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@doubleml@len\endcsname{2.6}
\expandafter\def\csname res@v5d@confound_0.8_b100@doubleml@rp\endcsname{0.70}
\expandafter\def\csname res@v5d@confound_0.8_b100@doubleml@map\endcsname{0.80}
\expandafter\def\csname res@v5d@confound_0.8_b100@varlingam@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@confound_0.8_b100@varlingam@fpn\endcsname{6}
\expandafter\def\csname res@v5d@confound_0.8_b100@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b100@varlingam@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@confound_0.8_b100@varlingam@prec\endcsname{0.33}
\expandafter\def\csname res@v5d@confound_0.8_b100@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v5d@confound_0.8_b100@varlingam@len\endcsname{7.3}
\expandafter\def\csname res@v5d@confound_0.8_b100@varlingam@rp\endcsname{0.31}
\expandafter\def\csname res@v5d@confound_0.8_b100@varlingam@map\endcsname{0.56}
\expandafter\def\csname res@v5d@confound_0.8_b100@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@confound_0.8_b100@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v5d@confound_0.8_b100@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b100@spacetime_rule@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@confound_0.8_b100@spacetime_rule@prec\endcsname{0.58}
\expandafter\def\csname res@v5d@confound_0.8_b100@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@spacetime_rule@len\endcsname{1.6}
\expandafter\def\csname res@v5d@confound_0.8_b100@spacetime_rule@rp\endcsname{0.41}
\expandafter\def\csname res@v5d@confound_0.8_b100@spacetime_rule@map\endcsname{0.57}
\expandafter\def\csname res@v5d@confound_0.8_b100@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@confound_0.8_b100@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b100@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@confound_0.8_b100@varsort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@confound_0.8_b100@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@confound_0.8_b100@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@confound_0.8_b100@varsort@rp\endcsname{0.10}
\expandafter\def\csname res@v5d@confound_0.8_b100@varsort@map\endcsname{0.14}
\expandafter\def\csname res@v5d@confound_0.8_b100@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@confound_0.8_b100@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@confound_0.8_b100@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@confound_0.8_b100@r2sort@prec\endcsname{0.12}
\expandafter\def\csname res@v5d@confound_0.8_b100@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@confound_0.8_b100@r2sort@bw\endcsname{3}
\expandafter\def\csname res@v5d@confound_0.8_b100@r2sort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@confound_0.8_b100@r2sort@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@confound_0.8_b100@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5d@combo_hard_b100@correlation@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@combo_hard_b100@correlation@fpn\endcsname{5}
\expandafter\def\csname res@v5d@combo_hard_b100@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@correlation@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@combo_hard_b100@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_hard_b100@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@correlation@bw\endcsname{4}
\expandafter\def\csname res@v5d@combo_hard_b100@correlation@len\endcsname{16.0}
\expandafter\def\csname res@v5d@combo_hard_b100@correlation@rp\endcsname{0.37}
\expandafter\def\csname res@v5d@combo_hard_b100@correlation@map\endcsname{0.54}
\expandafter\def\csname res@v5d@combo_hard_b100@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v5d@combo_hard_b100@granger@fpn\endcsname{9}
\expandafter\def\csname res@v5d@combo_hard_b100@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v5d@combo_hard_b100@granger@prec\endcsname{0.23}
\expandafter\def\csname res@v5d@combo_hard_b100@granger@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@granger@len\endcsname{11.8}
\expandafter\def\csname res@v5d@combo_hard_b100@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v5d@combo_hard_b100@granger@map\endcsname{0.75}
\expandafter\def\csname res@v5d@combo_hard_b100@pcmciplus@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@combo_hard_b100@pcmciplus@fpn\endcsname{7}
\expandafter\def\csname res@v5d@combo_hard_b100@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@pcmciplus@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@combo_hard_b100@pcmciplus@prec\endcsname{0.67}
\expandafter\def\csname res@v5d@combo_hard_b100@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b100@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@pcmciplus@len\endcsname{2.3}
\expandafter\def\csname res@v5d@combo_hard_b100@pcmciplus@rp\endcsname{0.84}
\expandafter\def\csname res@v5d@combo_hard_b100@pcmciplus@map\endcsname{0.87}
\expandafter\def\csname res@v5d@combo_hard_b100@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_hard_b100@pc@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_hard_b100@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@combo_hard_b100@pc@prec\endcsname{0.37}
\expandafter\def\csname res@v5d@combo_hard_b100@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@pc@bw\endcsname{6}
\expandafter\def\csname res@v5d@combo_hard_b100@pc@len\endcsname{3.2}
\expandafter\def\csname res@v5d@combo_hard_b100@pc@rp\endcsname{0.32}
\expandafter\def\csname res@v5d@combo_hard_b100@pc@map\endcsname{0.29}
\expandafter\def\csname res@v5d@combo_hard_b100@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_hard_b100@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_hard_b100@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@combo_hard_b100@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@combo_hard_b100@dynotears@rp\endcsname{0.90}
\expandafter\def\csname res@v5d@combo_hard_b100@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v5d@combo_hard_b100@doubleml@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@combo_hard_b100@doubleml@fpn\endcsname{6}
\expandafter\def\csname res@v5d@combo_hard_b100@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@doubleml@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@combo_hard_b100@doubleml@prec\endcsname{0.83}
\expandafter\def\csname res@v5d@combo_hard_b100@doubleml@ab\endcsname{4}
\expandafter\def\csname res@v5d@combo_hard_b100@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@doubleml@len\endcsname{1.2}
\expandafter\def\csname res@v5d@combo_hard_b100@doubleml@rp\endcsname{0.51}
\expandafter\def\csname res@v5d@combo_hard_b100@doubleml@map\endcsname{0.59}
\expandafter\def\csname res@v5d@combo_hard_b100@varlingam@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_hard_b100@varlingam@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_hard_b100@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@varlingam@tt\endcsname{0.35}
\expandafter\def\csname res@v5d@combo_hard_b100@varlingam@prec\endcsname{0.25}
\expandafter\def\csname res@v5d@combo_hard_b100@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@varlingam@bw\endcsname{6}
\expandafter\def\csname res@v5d@combo_hard_b100@varlingam@len\endcsname{7.6}
\expandafter\def\csname res@v5d@combo_hard_b100@varlingam@rp\endcsname{0.23}
\expandafter\def\csname res@v5d@combo_hard_b100@varlingam@map\endcsname{0.39}
\expandafter\def\csname res@v5d@combo_hard_b100@spacetime_rule@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@combo_hard_b100@spacetime_rule@fpn\endcsname{4}
\expandafter\def\csname res@v5d@combo_hard_b100@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@spacetime_rule@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_hard_b100@spacetime_rule@prec\endcsname{0.50}
\expandafter\def\csname res@v5d@combo_hard_b100@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b100@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@spacetime_rule@len\endcsname{1.0}
\expandafter\def\csname res@v5d@combo_hard_b100@spacetime_rule@rp\endcsname{0.25}
\expandafter\def\csname res@v5d@combo_hard_b100@spacetime_rule@map\endcsname{0.44}
\expandafter\def\csname res@v5d@combo_hard_b100@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_hard_b100@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_hard_b100@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_hard_b100@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@varsort@bw\endcsname{2}
\expandafter\def\csname res@v5d@combo_hard_b100@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@combo_hard_b100@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v5d@combo_hard_b100@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_hard_b100@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_hard_b100@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_hard_b100@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_hard_b100@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_hard_b100@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@combo_hard_b100@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_hard_b100@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_hard_b100@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_hard_b100@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v5d@combo_extreme_b100@correlation@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_extreme_b100@correlation@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b100@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@correlation@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@combo_extreme_b100@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_extreme_b100@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@correlation@bw\endcsname{8}
\expandafter\def\csname res@v5d@combo_extreme_b100@correlation@len\endcsname{15.5}
\expandafter\def\csname res@v5d@combo_extreme_b100@correlation@rp\endcsname{0.24}
\expandafter\def\csname res@v5d@combo_extreme_b100@correlation@map\endcsname{0.40}
\expandafter\def\csname res@v5d@combo_extreme_b100@granger@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@combo_extreme_b100@granger@fpn\endcsname{7}
\expandafter\def\csname res@v5d@combo_extreme_b100@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@combo_extreme_b100@granger@prec\endcsname{0.31}
\expandafter\def\csname res@v5d@combo_extreme_b100@granger@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@granger@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b100@granger@len\endcsname{10.4}
\expandafter\def\csname res@v5d@combo_extreme_b100@granger@rp\endcsname{0.56}
\expandafter\def\csname res@v5d@combo_extreme_b100@granger@map\endcsname{0.67}
\expandafter\def\csname res@v5d@combo_extreme_b100@pcmciplus@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@combo_extreme_b100@pcmciplus@fpn\endcsname{5}
\expandafter\def\csname res@v5d@combo_extreme_b100@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@pcmciplus@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_extreme_b100@pcmciplus@prec\endcsname{0.72}
\expandafter\def\csname res@v5d@combo_extreme_b100@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v5d@combo_extreme_b100@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b100@pcmciplus@len\endcsname{0.8}
\expandafter\def\csname res@v5d@combo_extreme_b100@pcmciplus@rp\endcsname{0.50}
\expandafter\def\csname res@v5d@combo_extreme_b100@pcmciplus@map\endcsname{0.65}
\expandafter\def\csname res@v5d@combo_extreme_b100@pc@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_extreme_b100@pc@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@pc@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@combo_extreme_b100@pc@prec\endcsname{0.23}
\expandafter\def\csname res@v5d@combo_extreme_b100@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@pc@bw\endcsname{9}
\expandafter\def\csname res@v5d@combo_extreme_b100@pc@len\endcsname{2.4}
\expandafter\def\csname res@v5d@combo_extreme_b100@pc@rp\endcsname{0.20}
\expandafter\def\csname res@v5d@combo_extreme_b100@pc@map\endcsname{0.21}
\expandafter\def\csname res@v5d@combo_extreme_b100@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_extreme_b100@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_extreme_b100@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@combo_extreme_b100@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@combo_extreme_b100@dynotears@rp\endcsname{0.62}
\expandafter\def\csname res@v5d@combo_extreme_b100@dynotears@map\endcsname{0.71}
\expandafter\def\csname res@v5d@combo_extreme_b100@doubleml@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_extreme_b100@doubleml@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b100@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@doubleml@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b100@doubleml@prec\endcsname{0.58}
\expandafter\def\csname res@v5d@combo_extreme_b100@doubleml@ab\endcsname{8}
\expandafter\def\csname res@v5d@combo_extreme_b100@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@doubleml@len\endcsname{0.7}
\expandafter\def\csname res@v5d@combo_extreme_b100@doubleml@rp\endcsname{0.40}
\expandafter\def\csname res@v5d@combo_extreme_b100@doubleml@map\endcsname{0.52}
\expandafter\def\csname res@v5d@combo_extreme_b100@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_extreme_b100@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@varlingam@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_extreme_b100@varlingam@prec\endcsname{0.18}
\expandafter\def\csname res@v5d@combo_extreme_b100@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@varlingam@bw\endcsname{9}
\expandafter\def\csname res@v5d@combo_extreme_b100@varlingam@len\endcsname{7.2}
\expandafter\def\csname res@v5d@combo_extreme_b100@varlingam@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b100@varlingam@map\endcsname{0.23}
\expandafter\def\csname res@v5d@combo_extreme_b100@spacetime_rule@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_extreme_b100@spacetime_rule@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_extreme_b100@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@spacetime_rule@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b100@spacetime_rule@prec\endcsname{0.28}
\expandafter\def\csname res@v5d@combo_extreme_b100@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b100@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v5d@combo_extreme_b100@spacetime_rule@rp\endcsname{0.22}
\expandafter\def\csname res@v5d@combo_extreme_b100@spacetime_rule@map\endcsname{0.35}
\expandafter\def\csname res@v5d@combo_extreme_b100@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_extreme_b100@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b100@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_extreme_b100@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_extreme_b100@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@combo_extreme_b100@varsort@rp\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_extreme_b100@varsort@map\endcsname{0.20}
\expandafter\def\csname res@v5d@combo_extreme_b100@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_extreme_b100@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_extreme_b100@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_extreme_b100@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b100@r2sort@prec\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_extreme_b100@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_extreme_b100@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v5d@combo_extreme_b100@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_extreme_b100@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_extreme_b100@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v5d@interaction_1.0_b100@correlation@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@correlation@fpn\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b100@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@correlation@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@interaction_1.0_b100@correlation@prec\endcsname{0.18}
\expandafter\def\csname res@v5d@interaction_1.0_b100@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@correlation@bw\endcsname{9}
\expandafter\def\csname res@v5d@interaction_1.0_b100@correlation@len\endcsname{7.5}
\expandafter\def\csname res@v5d@interaction_1.0_b100@correlation@rp\endcsname{0.23}
\expandafter\def\csname res@v5d@interaction_1.0_b100@correlation@map\endcsname{0.36}
\expandafter\def\csname res@v5d@interaction_1.0_b100@granger@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@granger@fpn\endcsname{4}
\expandafter\def\csname res@v5d@interaction_1.0_b100@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@granger@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@interaction_1.0_b100@granger@prec\endcsname{0.36}
\expandafter\def\csname res@v5d@interaction_1.0_b100@granger@ab\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b100@granger@bw\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b100@granger@len\endcsname{5.1}
\expandafter\def\csname res@v5d@interaction_1.0_b100@granger@rp\endcsname{0.51}
\expandafter\def\csname res@v5d@interaction_1.0_b100@granger@map\endcsname{0.58}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pcmciplus@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pcmciplus@fpn\endcsname{5}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pcmciplus@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pcmciplus@prec\endcsname{0.62}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pcmciplus@len\endcsname{1.6}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pcmciplus@rp\endcsname{0.48}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pcmciplus@map\endcsname{0.59}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pc@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pc@fpn\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pc@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pc@prec\endcsname{0.11}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pc@bw\endcsname{9}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pc@len\endcsname{2.8}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pc@rp\endcsname{0.14}
\expandafter\def\csname res@v5d@interaction_1.0_b100@pc@map\endcsname{0.15}
\expandafter\def\csname res@v5d@interaction_1.0_b100@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@interaction_1.0_b100@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@interaction_1.0_b100@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@dynotears@rp\endcsname{0.49}
\expandafter\def\csname res@v5d@interaction_1.0_b100@dynotears@map\endcsname{0.54}
\expandafter\def\csname res@v5d@interaction_1.0_b100@doubleml@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@doubleml@fpn\endcsname{2}
\expandafter\def\csname res@v5d@interaction_1.0_b100@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@doubleml@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@interaction_1.0_b100@doubleml@prec\endcsname{0.56}
\expandafter\def\csname res@v5d@interaction_1.0_b100@doubleml@ab\endcsname{7}
\expandafter\def\csname res@v5d@interaction_1.0_b100@doubleml@bw\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b100@doubleml@len\endcsname{0.5}
\expandafter\def\csname res@v5d@interaction_1.0_b100@doubleml@rp\endcsname{0.33}
\expandafter\def\csname res@v5d@interaction_1.0_b100@doubleml@map\endcsname{0.45}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varlingam@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varlingam@fpn\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varlingam@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varlingam@prec\endcsname{0.12}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varlingam@ab\endcsname{5}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varlingam@bw\endcsname{3}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varlingam@len\endcsname{1.7}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varlingam@rp\endcsname{0.36}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varlingam@map\endcsname{0.36}
\expandafter\def\csname res@v5d@interaction_1.0_b100@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v5d@interaction_1.0_b100@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v5d@interaction_1.0_b100@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v5d@interaction_1.0_b100@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v5d@interaction_1.0_b100@spacetime_rule@rp\endcsname{0.54}
\expandafter\def\csname res@v5d@interaction_1.0_b100@spacetime_rule@map\endcsname{0.69}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varsort@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varsort@fpn\endcsname{3}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varsort@prec\endcsname{0.20}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varsort@bw\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varsort@rp\endcsname{0.13}
\expandafter\def\csname res@v5d@interaction_1.0_b100@varsort@map\endcsname{0.19}
\expandafter\def\csname res@v5d@interaction_1.0_b100@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@interaction_1.0_b100@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@interaction_1.0_b100@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@interaction_1.0_b100@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@interaction_1.0_b100@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@interaction_1.0_b100@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@interaction_1.0_b100@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v5d@combo_interaction_b100@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_interaction_b100@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@correlation@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_interaction_b100@correlation@prec\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b100@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@correlation@bw\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@correlation@len\endcsname{5.2}
\expandafter\def\csname res@v5d@combo_interaction_b100@correlation@rp\endcsname{0.03}
\expandafter\def\csname res@v5d@combo_interaction_b100@correlation@map\endcsname{0.29}
\expandafter\def\csname res@v5d@combo_interaction_b100@granger@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_interaction_b100@granger@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b100@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@granger@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_interaction_b100@granger@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_interaction_b100@granger@ab\endcsname{7}
\expandafter\def\csname res@v5d@combo_interaction_b100@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@granger@len\endcsname{2.8}
\expandafter\def\csname res@v5d@combo_interaction_b100@granger@rp\endcsname{0.42}
\expandafter\def\csname res@v5d@combo_interaction_b100@granger@map\endcsname{0.53}
\expandafter\def\csname res@v5d@combo_interaction_b100@pcmciplus@fp\endcsname{2/10}
\expandafter\def\csname res@v5d@combo_interaction_b100@pcmciplus@fpn\endcsname{2}
\expandafter\def\csname res@v5d@combo_interaction_b100@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@pcmciplus@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b100@pcmciplus@prec\endcsname{0.25}
\expandafter\def\csname res@v5d@combo_interaction_b100@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v5d@combo_interaction_b100@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b100@pcmciplus@len\endcsname{0.9}
\expandafter\def\csname res@v5d@combo_interaction_b100@pcmciplus@rp\endcsname{0.42}
\expandafter\def\csname res@v5d@combo_interaction_b100@pcmciplus@map\endcsname{0.52}
\expandafter\def\csname res@v5d@combo_interaction_b100@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b100@pc@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b100@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@pc@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@combo_interaction_b100@pc@prec\endcsname{0.05}
\expandafter\def\csname res@v5d@combo_interaction_b100@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@pc@bw\endcsname{8}
\expandafter\def\csname res@v5d@combo_interaction_b100@pc@len\endcsname{2.1}
\expandafter\def\csname res@v5d@combo_interaction_b100@pc@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_interaction_b100@pc@map\endcsname{0.18}
\expandafter\def\csname res@v5d@combo_interaction_b100@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_interaction_b100@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@combo_interaction_b100@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@combo_interaction_b100@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@combo_interaction_b100@dynotears@rp\endcsname{0.49}
\expandafter\def\csname res@v5d@combo_interaction_b100@dynotears@map\endcsname{0.53}
\expandafter\def\csname res@v5d@combo_interaction_b100@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b100@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b100@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@combo_interaction_b100@doubleml@prec\endcsname{1.00}
\expandafter\def\csname res@v5d@combo_interaction_b100@doubleml@ab\endcsname{9}
\expandafter\def\csname res@v5d@combo_interaction_b100@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@doubleml@len\endcsname{0.1}
\expandafter\def\csname res@v5d@combo_interaction_b100@doubleml@rp\endcsname{0.26}
\expandafter\def\csname res@v5d@combo_interaction_b100@doubleml@map\endcsname{0.38}
\expandafter\def\csname res@v5d@combo_interaction_b100@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_interaction_b100@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@varlingam@tt\endcsname{0.08}
\expandafter\def\csname res@v5d@combo_interaction_b100@varlingam@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@combo_interaction_b100@varlingam@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b100@varlingam@bw\endcsname{9}
\expandafter\def\csname res@v5d@combo_interaction_b100@varlingam@len\endcsname{2.8}
\expandafter\def\csname res@v5d@combo_interaction_b100@varlingam@rp\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b100@varlingam@map\endcsname{0.22}
\expandafter\def\csname res@v5d@combo_interaction_b100@spacetime_rule@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@combo_interaction_b100@spacetime_rule@fpn\endcsname{3}
\expandafter\def\csname res@v5d@combo_interaction_b100@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@spacetime_rule@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_interaction_b100@spacetime_rule@prec\endcsname{0.44}
\expandafter\def\csname res@v5d@combo_interaction_b100@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b100@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v5d@combo_interaction_b100@spacetime_rule@rp\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_interaction_b100@spacetime_rule@map\endcsname{0.41}
\expandafter\def\csname res@v5d@combo_interaction_b100@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@combo_interaction_b100@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v5d@combo_interaction_b100@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v5d@combo_interaction_b100@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b100@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@combo_interaction_b100@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_interaction_b100@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v5d@combo_interaction_b100@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@combo_interaction_b100@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@combo_interaction_b100@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@combo_interaction_b100@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v5d@combo_interaction_b100@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v5d@combo_interaction_b100@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v5d@combo_interaction_b100@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v5d@combo_interaction_b100@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v5d@combo_interaction_b100@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v5d@control_weak_b100@correlation@fp\endcsname{6/10}
\expandafter\def\csname res@v5d@control_weak_b100@correlation@fpn\endcsname{6}
\expandafter\def\csname res@v5d@control_weak_b100@correlation@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@correlation@tt\endcsname{0.50}
\expandafter\def\csname res@v5d@control_weak_b100@correlation@prec\endcsname{0.20}
\expandafter\def\csname res@v5d@control_weak_b100@correlation@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b100@correlation@bw\endcsname{4}
\expandafter\def\csname res@v5d@control_weak_b100@correlation@len\endcsname{10.2}
\expandafter\def\csname res@v5d@control_weak_b100@correlation@rp\endcsname{0.42}
\expandafter\def\csname res@v5d@control_weak_b100@correlation@map\endcsname{0.53}
\expandafter\def\csname res@v5d@control_weak_b100@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v5d@control_weak_b100@granger@fpn\endcsname{8}
\expandafter\def\csname res@v5d@control_weak_b100@granger@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v5d@control_weak_b100@granger@prec\endcsname{0.49}
\expandafter\def\csname res@v5d@control_weak_b100@granger@ab\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b100@granger@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b100@granger@len\endcsname{5.4}
\expandafter\def\csname res@v5d@control_weak_b100@granger@rp\endcsname{0.63}
\expandafter\def\csname res@v5d@control_weak_b100@granger@map\endcsname{0.71}
\expandafter\def\csname res@v5d@control_weak_b100@pcmciplus@fp\endcsname{7/10}
\expandafter\def\csname res@v5d@control_weak_b100@pcmciplus@fpn\endcsname{7}
\expandafter\def\csname res@v5d@control_weak_b100@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@pcmciplus@tt\endcsname{0.38}
\expandafter\def\csname res@v5d@control_weak_b100@pcmciplus@prec\endcsname{0.73}
\expandafter\def\csname res@v5d@control_weak_b100@pcmciplus@ab\endcsname{3}
\expandafter\def\csname res@v5d@control_weak_b100@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b100@pcmciplus@len\endcsname{1.6}
\expandafter\def\csname res@v5d@control_weak_b100@pcmciplus@rp\endcsname{0.61}
\expandafter\def\csname res@v5d@control_weak_b100@pcmciplus@map\endcsname{0.69}
\expandafter\def\csname res@v5d@control_weak_b100@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@control_weak_b100@pc@fpn\endcsname{3}
\expandafter\def\csname res@v5d@control_weak_b100@pc@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v5d@control_weak_b100@pc@prec\endcsname{0.26}
\expandafter\def\csname res@v5d@control_weak_b100@pc@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b100@pc@bw\endcsname{6}
\expandafter\def\csname res@v5d@control_weak_b100@pc@len\endcsname{3.6}
\expandafter\def\csname res@v5d@control_weak_b100@pc@rp\endcsname{0.25}
\expandafter\def\csname res@v5d@control_weak_b100@pc@map\endcsname{0.27}
\expandafter\def\csname res@v5d@control_weak_b100@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v5d@control_weak_b100@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b100@dynotears@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v5d@control_weak_b100@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v5d@control_weak_b100@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b100@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v5d@control_weak_b100@dynotears@rp\endcsname{0.73}
\expandafter\def\csname res@v5d@control_weak_b100@dynotears@map\endcsname{0.83}
\expandafter\def\csname res@v5d@control_weak_b100@doubleml@fp\endcsname{4/10}
\expandafter\def\csname res@v5d@control_weak_b100@doubleml@fpn\endcsname{4}
\expandafter\def\csname res@v5d@control_weak_b100@doubleml@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@doubleml@tt\endcsname{0.27}
\expandafter\def\csname res@v5d@control_weak_b100@doubleml@prec\endcsname{0.92}
\expandafter\def\csname res@v5d@control_weak_b100@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v5d@control_weak_b100@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b100@doubleml@len\endcsname{0.8}
\expandafter\def\csname res@v5d@control_weak_b100@doubleml@rp\endcsname{0.43}
\expandafter\def\csname res@v5d@control_weak_b100@doubleml@map\endcsname{0.60}
\expandafter\def\csname res@v5d@control_weak_b100@varlingam@fp\endcsname{5/10}
\expandafter\def\csname res@v5d@control_weak_b100@varlingam@fpn\endcsname{5}
\expandafter\def\csname res@v5d@control_weak_b100@varlingam@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@varlingam@tt\endcsname{0.46}
\expandafter\def\csname res@v5d@control_weak_b100@varlingam@prec\endcsname{0.54}
\expandafter\def\csname res@v5d@control_weak_b100@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b100@varlingam@bw\endcsname{5}
\expandafter\def\csname res@v5d@control_weak_b100@varlingam@len\endcsname{4.3}
\expandafter\def\csname res@v5d@control_weak_b100@varlingam@rp\endcsname{0.30}
\expandafter\def\csname res@v5d@control_weak_b100@varlingam@map\endcsname{0.50}
\expandafter\def\csname res@v5d@control_weak_b100@spacetime_rule@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@control_weak_b100@spacetime_rule@fpn\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b100@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@spacetime_rule@tt\endcsname{0.04}
\expandafter\def\csname res@v5d@control_weak_b100@spacetime_rule@prec\endcsname{0.20}
\expandafter\def\csname res@v5d@control_weak_b100@spacetime_rule@ab\endcsname{5}
\expandafter\def\csname res@v5d@control_weak_b100@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b100@spacetime_rule@len\endcsname{0.5}
\expandafter\def\csname res@v5d@control_weak_b100@spacetime_rule@rp\endcsname{0.25}
\expandafter\def\csname res@v5d@control_weak_b100@spacetime_rule@map\endcsname{0.31}
\expandafter\def\csname res@v5d@control_weak_b100@varsort@fp\endcsname{3/10}
\expandafter\def\csname res@v5d@control_weak_b100@varsort@fpn\endcsname{3}
\expandafter\def\csname res@v5d@control_weak_b100@varsort@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v5d@control_weak_b100@varsort@prec\endcsname{0.22}
\expandafter\def\csname res@v5d@control_weak_b100@varsort@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b100@varsort@bw\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b100@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v5d@control_weak_b100@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v5d@control_weak_b100@varsort@map\endcsname{0.20}
\expandafter\def\csname res@v5d@control_weak_b100@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v5d@control_weak_b100@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b100@r2sort@n\endcsname{10}
\expandafter\def\csname res@v5d@control_weak_b100@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v5d@control_weak_b100@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v5d@control_weak_b100@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v5d@control_weak_b100@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v5d@control_weak_b100@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v5d@control_weak_b100@r2sort@rp\endcsname{0.25}
\expandafter\def\csname res@v5d@control_weak_b100@r2sort@map\endcsname{0.30}
\expandafter\def\csname res@v6@meas_0.1@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@meas_0.1@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v6@meas_0.1@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@meas_0.1@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v6@meas_0.1@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v6@meas_0.1@correlation@map\endcsname{0.78}
\expandafter\def\csname res@v6@meas_0.1@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@meas_0.1@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@granger@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v6@meas_0.1@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v6@meas_0.1@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@granger@len\endcsname{16.9}
\expandafter\def\csname res@v6@meas_0.1@granger@rp\endcsname{0.68}
\expandafter\def\csname res@v6@meas_0.1@granger@map\endcsname{0.78}
\expandafter\def\csname res@v6@meas_0.1@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@meas_0.1@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@pcmciplus@tt\endcsname{0.77}
\expandafter\def\csname res@v6@meas_0.1@pcmciplus@prec\endcsname{0.64}
\expandafter\def\csname res@v6@meas_0.1@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@pcmciplus@len\endcsname{3.2}
\expandafter\def\csname res@v6@meas_0.1@pcmciplus@rp\endcsname{0.95}
\expandafter\def\csname res@v6@meas_0.1@pcmciplus@map\endcsname{0.97}
\expandafter\def\csname res@v6@meas_0.1@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@meas_0.1@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@meas_0.1@pc@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@meas_0.1@pc@prec\endcsname{0.33}
\expandafter\def\csname res@v6@meas_0.1@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@meas_0.1@pc@len\endcsname{5.6}
\expandafter\def\csname res@v6@meas_0.1@pc@rp\endcsname{0.33}
\expandafter\def\csname res@v6@meas_0.1@pc@map\endcsname{0.29}
\expandafter\def\csname res@v6@meas_0.1@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v6@meas_0.1@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v6@meas_0.1@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@dynotears@tt\endcsname{0.15}
\expandafter\def\csname res@v6@meas_0.1@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@meas_0.1@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v6@meas_0.1@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@dynotears@len\endcsname{0.4}
\expandafter\def\csname res@v6@meas_0.1@dynotears@rp\endcsname{0.90}
\expandafter\def\csname res@v6@meas_0.1@dynotears@map\endcsname{0.93}
\expandafter\def\csname res@v6@meas_0.1@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@meas_0.1@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v6@meas_0.1@doubleml@prec\endcsname{0.67}
\expandafter\def\csname res@v6@meas_0.1@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@doubleml@len\endcsname{3.9}
\expandafter\def\csname res@v6@meas_0.1@doubleml@rp\endcsname{0.74}
\expandafter\def\csname res@v6@meas_0.1@doubleml@map\endcsname{0.87}
\expandafter\def\csname res@v6@meas_0.1@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.1@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.1@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@varlingam@tt\endcsname{0.73}
\expandafter\def\csname res@v6@meas_0.1@varlingam@prec\endcsname{0.31}
\expandafter\def\csname res@v6@meas_0.1@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@varlingam@len\endcsname{9.9}
\expandafter\def\csname res@v6@meas_0.1@varlingam@rp\endcsname{0.74}
\expandafter\def\csname res@v6@meas_0.1@varlingam@map\endcsname{0.83}
\expandafter\def\csname res@v6@meas_0.1@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v6@meas_0.1@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v6@meas_0.1@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v6@meas_0.1@spacetime_rule@prec\endcsname{0.94}
\expandafter\def\csname res@v6@meas_0.1@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v6@meas_0.1@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v6@meas_0.1@spacetime_rule@rp\endcsname{0.63}
\expandafter\def\csname res@v6@meas_0.1@spacetime_rule@map\endcsname{0.77}
\expandafter\def\csname res@v6@meas_0.1@varsort@fp\endcsname{3/10}
\expandafter\def\csname res@v6@meas_0.1@varsort@fpn\endcsname{3}
\expandafter\def\csname res@v6@meas_0.1@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@varsort@tt\endcsname{0.27}
\expandafter\def\csname res@v6@meas_0.1@varsort@prec\endcsname{0.23}
\expandafter\def\csname res@v6@meas_0.1@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@varsort@bw\endcsname{3}
\expandafter\def\csname res@v6@meas_0.1@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v6@meas_0.1@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v6@meas_0.1@varsort@map\endcsname{0.21}
\expandafter\def\csname res@v6@meas_0.1@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.1@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.1@r2sort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@meas_0.1@r2sort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@meas_0.1@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.1@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v6@meas_0.1@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@meas_0.1@r2sort@rp\endcsname{0.14}
\expandafter\def\csname res@v6@meas_0.1@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@meas_0.2@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@meas_0.2@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v6@meas_0.2@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@meas_0.2@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v6@meas_0.2@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v6@meas_0.2@correlation@map\endcsname{0.77}
\expandafter\def\csname res@v6@meas_0.2@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.2@granger@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.2@granger@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v6@meas_0.2@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v6@meas_0.2@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@granger@len\endcsname{16.6}
\expandafter\def\csname res@v6@meas_0.2@granger@rp\endcsname{0.68}
\expandafter\def\csname res@v6@meas_0.2@granger@map\endcsname{0.76}
\expandafter\def\csname res@v6@meas_0.2@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@meas_0.2@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@pcmciplus@tt\endcsname{0.81}
\expandafter\def\csname res@v6@meas_0.2@pcmciplus@prec\endcsname{0.62}
\expandafter\def\csname res@v6@meas_0.2@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@pcmciplus@len\endcsname{3.8}
\expandafter\def\csname res@v6@meas_0.2@pcmciplus@rp\endcsname{0.90}
\expandafter\def\csname res@v6@meas_0.2@pcmciplus@map\endcsname{0.95}
\expandafter\def\csname res@v6@meas_0.2@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@meas_0.2@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@meas_0.2@pc@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@meas_0.2@pc@prec\endcsname{0.33}
\expandafter\def\csname res@v6@meas_0.2@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@meas_0.2@pc@len\endcsname{6.1}
\expandafter\def\csname res@v6@meas_0.2@pc@rp\endcsname{0.33}
\expandafter\def\csname res@v6@meas_0.2@pc@map\endcsname{0.28}
\expandafter\def\csname res@v6@meas_0.2@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.2@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.2@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v6@meas_0.2@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@meas_0.2@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v6@meas_0.2@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v6@meas_0.2@dynotears@rp\endcsname{0.90}
\expandafter\def\csname res@v6@meas_0.2@dynotears@map\endcsname{0.93}
\expandafter\def\csname res@v6@meas_0.2@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.2@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.2@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@doubleml@tt\endcsname{0.73}
\expandafter\def\csname res@v6@meas_0.2@doubleml@prec\endcsname{0.64}
\expandafter\def\csname res@v6@meas_0.2@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@meas_0.2@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@doubleml@len\endcsname{3.8}
\expandafter\def\csname res@v6@meas_0.2@doubleml@rp\endcsname{0.82}
\expandafter\def\csname res@v6@meas_0.2@doubleml@map\endcsname{0.90}
\expandafter\def\csname res@v6@meas_0.2@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.2@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.2@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v6@meas_0.2@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v6@meas_0.2@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@varlingam@len\endcsname{11.1}
\expandafter\def\csname res@v6@meas_0.2@varlingam@rp\endcsname{0.65}
\expandafter\def\csname res@v6@meas_0.2@varlingam@map\endcsname{0.79}
\expandafter\def\csname res@v6@meas_0.2@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v6@meas_0.2@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v6@meas_0.2@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@spacetime_rule@tt\endcsname{0.35}
\expandafter\def\csname res@v6@meas_0.2@spacetime_rule@prec\endcsname{0.94}
\expandafter\def\csname res@v6@meas_0.2@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v6@meas_0.2@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@spacetime_rule@len\endcsname{1.0}
\expandafter\def\csname res@v6@meas_0.2@spacetime_rule@rp\endcsname{0.59}
\expandafter\def\csname res@v6@meas_0.2@spacetime_rule@map\endcsname{0.74}
\expandafter\def\csname res@v6@meas_0.2@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.2@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.2@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v6@meas_0.2@varsort@prec\endcsname{0.20}
\expandafter\def\csname res@v6@meas_0.2@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@meas_0.2@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@meas_0.2@varsort@rp\endcsname{0.18}
\expandafter\def\csname res@v6@meas_0.2@varsort@map\endcsname{0.20}
\expandafter\def\csname res@v6@meas_0.2@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.2@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.2@r2sort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@meas_0.2@r2sort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@meas_0.2@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.2@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v6@meas_0.2@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@meas_0.2@r2sort@rp\endcsname{0.14}
\expandafter\def\csname res@v6@meas_0.2@r2sort@map\endcsname{0.19}
\expandafter\def\csname res@v6@meas_0.3@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@meas_0.3@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v6@meas_0.3@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@meas_0.3@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@correlation@len\endcsname{18.1}
\expandafter\def\csname res@v6@meas_0.3@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v6@meas_0.3@correlation@map\endcsname{0.77}
\expandafter\def\csname res@v6@meas_0.3@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.3@granger@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3@granger@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v6@meas_0.3@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v6@meas_0.3@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@granger@len\endcsname{16.1}
\expandafter\def\csname res@v6@meas_0.3@granger@rp\endcsname{0.68}
\expandafter\def\csname res@v6@meas_0.3@granger@map\endcsname{0.76}
\expandafter\def\csname res@v6@meas_0.3@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.3@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v6@meas_0.3@pcmciplus@prec\endcsname{0.53}
\expandafter\def\csname res@v6@meas_0.3@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@pcmciplus@len\endcsname{3.9}
\expandafter\def\csname res@v6@meas_0.3@pcmciplus@rp\endcsname{0.79}
\expandafter\def\csname res@v6@meas_0.3@pcmciplus@map\endcsname{0.91}
\expandafter\def\csname res@v6@meas_0.3@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v6@meas_0.3@pc@fpn\endcsname{2}
\expandafter\def\csname res@v6@meas_0.3@pc@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v6@meas_0.3@pc@prec\endcsname{0.26}
\expandafter\def\csname res@v6@meas_0.3@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@meas_0.3@pc@len\endcsname{7.1}
\expandafter\def\csname res@v6@meas_0.3@pc@rp\endcsname{0.26}
\expandafter\def\csname res@v6@meas_0.3@pc@map\endcsname{0.23}
\expandafter\def\csname res@v6@meas_0.3@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.3@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v6@meas_0.3@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v6@meas_0.3@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v6@meas_0.3@dynotears@rp\endcsname{0.86}
\expandafter\def\csname res@v6@meas_0.3@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v6@meas_0.3@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.3@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@doubleml@tt\endcsname{0.69}
\expandafter\def\csname res@v6@meas_0.3@doubleml@prec\endcsname{0.56}
\expandafter\def\csname res@v6@meas_0.3@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@doubleml@len\endcsname{4.4}
\expandafter\def\csname res@v6@meas_0.3@doubleml@rp\endcsname{0.70}
\expandafter\def\csname res@v6@meas_0.3@doubleml@map\endcsname{0.86}
\expandafter\def\csname res@v6@meas_0.3@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v6@meas_0.3@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@varlingam@tt\endcsname{0.62}
\expandafter\def\csname res@v6@meas_0.3@varlingam@prec\endcsname{0.37}
\expandafter\def\csname res@v6@meas_0.3@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@varlingam@len\endcsname{9.4}
\expandafter\def\csname res@v6@meas_0.3@varlingam@rp\endcsname{0.64}
\expandafter\def\csname res@v6@meas_0.3@varlingam@map\endcsname{0.80}
\expandafter\def\csname res@v6@meas_0.3@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v6@meas_0.3@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v6@meas_0.3@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@spacetime_rule@tt\endcsname{0.27}
\expandafter\def\csname res@v6@meas_0.3@spacetime_rule@prec\endcsname{0.81}
\expandafter\def\csname res@v6@meas_0.3@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v6@meas_0.3@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3@spacetime_rule@len\endcsname{0.9}
\expandafter\def\csname res@v6@meas_0.3@spacetime_rule@rp\endcsname{0.54}
\expandafter\def\csname res@v6@meas_0.3@spacetime_rule@map\endcsname{0.67}
\expandafter\def\csname res@v6@meas_0.3@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.3@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@meas_0.3@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@meas_0.3@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@meas_0.3@varsort@rp\endcsname{0.10}
\expandafter\def\csname res@v6@meas_0.3@varsort@map\endcsname{0.13}
\expandafter\def\csname res@v6@meas_0.3@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.3@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3@r2sort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@meas_0.3@r2sort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@meas_0.3@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v6@meas_0.3@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@meas_0.3@r2sort@rp\endcsname{0.14}
\expandafter\def\csname res@v6@meas_0.3@r2sort@map\endcsname{0.19}
\expandafter\def\csname res@v6@meas_0.5@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@meas_0.5@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v6@meas_0.5@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v6@meas_0.5@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@correlation@len\endcsname{17.8}
\expandafter\def\csname res@v6@meas_0.5@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v6@meas_0.5@correlation@map\endcsname{0.76}
\expandafter\def\csname res@v6@meas_0.5@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.5@granger@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.5@granger@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v6@meas_0.5@granger@prec\endcsname{0.17}
\expandafter\def\csname res@v6@meas_0.5@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@granger@len\endcsname{14.1}
\expandafter\def\csname res@v6@meas_0.5@granger@rp\endcsname{0.64}
\expandafter\def\csname res@v6@meas_0.5@granger@map\endcsname{0.74}
\expandafter\def\csname res@v6@meas_0.5@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.5@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.5@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@pcmciplus@tt\endcsname{0.69}
\expandafter\def\csname res@v6@meas_0.5@pcmciplus@prec\endcsname{0.47}
\expandafter\def\csname res@v6@meas_0.5@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@pcmciplus@len\endcsname{5.0}
\expandafter\def\csname res@v6@meas_0.5@pcmciplus@rp\endcsname{0.82}
\expandafter\def\csname res@v6@meas_0.5@pcmciplus@map\endcsname{0.88}
\expandafter\def\csname res@v6@meas_0.5@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v6@meas_0.5@pc@fpn\endcsname{2}
\expandafter\def\csname res@v6@meas_0.5@pc@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v6@meas_0.5@pc@prec\endcsname{0.21}
\expandafter\def\csname res@v6@meas_0.5@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@meas_0.5@pc@len\endcsname{8.9}
\expandafter\def\csname res@v6@meas_0.5@pc@rp\endcsname{0.21}
\expandafter\def\csname res@v6@meas_0.5@pc@map\endcsname{0.20}
\expandafter\def\csname res@v6@meas_0.5@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.5@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v6@meas_0.5@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v6@meas_0.5@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v6@meas_0.5@dynotears@rp\endcsname{0.78}
\expandafter\def\csname res@v6@meas_0.5@dynotears@map\endcsname{0.84}
\expandafter\def\csname res@v6@meas_0.5@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@meas_0.5@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@doubleml@tt\endcsname{0.73}
\expandafter\def\csname res@v6@meas_0.5@doubleml@prec\endcsname{0.57}
\expandafter\def\csname res@v6@meas_0.5@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@doubleml@len\endcsname{4.7}
\expandafter\def\csname res@v6@meas_0.5@doubleml@rp\endcsname{0.76}
\expandafter\def\csname res@v6@meas_0.5@doubleml@map\endcsname{0.86}
\expandafter\def\csname res@v6@meas_0.5@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.5@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.5@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@varlingam@tt\endcsname{0.62}
\expandafter\def\csname res@v6@meas_0.5@varlingam@prec\endcsname{0.34}
\expandafter\def\csname res@v6@meas_0.5@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@varlingam@len\endcsname{9.2}
\expandafter\def\csname res@v6@meas_0.5@varlingam@rp\endcsname{0.69}
\expandafter\def\csname res@v6@meas_0.5@varlingam@map\endcsname{0.77}
\expandafter\def\csname res@v6@meas_0.5@spacetime_rule@fp\endcsname{3/10}
\expandafter\def\csname res@v6@meas_0.5@spacetime_rule@fpn\endcsname{3}
\expandafter\def\csname res@v6@meas_0.5@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@spacetime_rule@tt\endcsname{0.12}
\expandafter\def\csname res@v6@meas_0.5@spacetime_rule@prec\endcsname{0.75}
\expandafter\def\csname res@v6@meas_0.5@spacetime_rule@ab\endcsname{6}
\expandafter\def\csname res@v6@meas_0.5@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v6@meas_0.5@spacetime_rule@len\endcsname{0.4}
\expandafter\def\csname res@v6@meas_0.5@spacetime_rule@rp\endcsname{0.62}
\expandafter\def\csname res@v6@meas_0.5@spacetime_rule@map\endcsname{0.71}
\expandafter\def\csname res@v6@meas_0.5@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.5@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.5@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@meas_0.5@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@meas_0.5@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@meas_0.5@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v6@meas_0.5@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v6@meas_0.5@varsort@map\endcsname{0.13}
\expandafter\def\csname res@v6@meas_0.5@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.5@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.5@r2sort@tt\endcsname{0.08}
\expandafter\def\csname res@v6@meas_0.5@r2sort@prec\endcsname{0.07}
\expandafter\def\csname res@v6@meas_0.5@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.5@r2sort@bw\endcsname{3}
\expandafter\def\csname res@v6@meas_0.5@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v6@meas_0.5@r2sort@rp\endcsname{0.08}
\expandafter\def\csname res@v6@meas_0.5@r2sort@map\endcsname{0.17}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@correlation@tt\endcsname{0.12}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@correlation@bw\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@correlation@len\endcsname{5.2}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@correlation@rp\endcsname{0.00}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@correlation@map\endcsname{0.26}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@granger@fp\endcsname{4/10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@granger@fpn\endcsname{4}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@granger@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@granger@tt\endcsname{0.19}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@granger@prec\endcsname{0.25}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@granger@ab\endcsname{4}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@granger@bw\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@granger@len\endcsname{3.3}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@granger@rp\endcsname{0.50}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@granger@map\endcsname{0.60}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pcmciplus@fp\endcsname{3/10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pcmciplus@fpn\endcsname{3}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pcmciplus@tt\endcsname{0.15}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pcmciplus@prec\endcsname{0.33}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pcmciplus@len\endcsname{1.4}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pcmciplus@rp\endcsname{0.28}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pcmciplus@map\endcsname{0.45}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pc@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pc@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pc@tt\endcsname{0.08}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pc@prec\endcsname{0.07}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pc@bw\endcsname{8}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pc@len\endcsname{2.8}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pc@rp\endcsname{0.11}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@pc@map\endcsname{0.17}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@dynotears@rp\endcsname{0.75}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@dynotears@map\endcsname{0.78}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@doubleml@prec\endcsname{0.25}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@doubleml@ab\endcsname{8}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@doubleml@len\endcsname{0.3}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@doubleml@rp\endcsname{0.33}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@doubleml@map\endcsname{0.44}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varlingam@tt\endcsname{0.08}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varlingam@prec\endcsname{0.11}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varlingam@ab\endcsname{2}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varlingam@bw\endcsname{8}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varlingam@len\endcsname{3.1}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varlingam@rp\endcsname{0.12}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varlingam@map\endcsname{0.17}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@spacetime_rule@fp\endcsname{5/10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@spacetime_rule@fpn\endcsname{5}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@spacetime_rule@tt\endcsname{0.19}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@spacetime_rule@prec\endcsname{0.71}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@spacetime_rule@ab\endcsname{3}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@spacetime_rule@len\endcsname{0.7}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@spacetime_rule@rp\endcsname{0.30}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@spacetime_rule@map\endcsname{0.52}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varsort@bw\endcsname{2}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@varsort@map\endcsname{0.13}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@r2sort@tt\endcsname{0.08}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@r2sort@prec\endcsname{0.08}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@r2sort@len\endcsname{2.8}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@meas_0.3_combo_interaction@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v6@meas_0.3_s40@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.3_s40@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3_s40@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_s40@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v6@meas_0.3_s40@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v6@meas_0.3_s40@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@correlation@len\endcsname{35.0}
\expandafter\def\csname res@v6@meas_0.3_s40@correlation@rp\endcsname{0.54}
\expandafter\def\csname res@v6@meas_0.3_s40@correlation@map\endcsname{0.64}
\expandafter\def\csname res@v6@meas_0.3_s40@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.3_s40@granger@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3_s40@granger@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_s40@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v6@meas_0.3_s40@granger@prec\endcsname{0.17}
\expandafter\def\csname res@v6@meas_0.3_s40@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@granger@len\endcsname{30.0}
\expandafter\def\csname res@v6@meas_0.3_s40@granger@rp\endcsname{0.54}
\expandafter\def\csname res@v6@meas_0.3_s40@granger@map\endcsname{0.63}
\expandafter\def\csname res@v6@meas_0.3_s40@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.3_s40@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3_s40@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_s40@pcmciplus@tt\endcsname{0.69}
\expandafter\def\csname res@v6@meas_0.3_s40@pcmciplus@prec\endcsname{0.44}
\expandafter\def\csname res@v6@meas_0.3_s40@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@pcmciplus@len\endcsname{4.8}
\expandafter\def\csname res@v6@meas_0.3_s40@pcmciplus@rp\endcsname{0.69}
\expandafter\def\csname res@v6@meas_0.3_s40@pcmciplus@map\endcsname{0.81}
\expandafter\def\csname res@v6@meas_0.3_s40@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v6@meas_0.3_s40@pc@fpn\endcsname{2}
\expandafter\def\csname res@v6@meas_0.3_s40@pc@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_s40@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v6@meas_0.3_s40@pc@prec\endcsname{0.21}
\expandafter\def\csname res@v6@meas_0.3_s40@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@meas_0.3_s40@pc@len\endcsname{9.5}
\expandafter\def\csname res@v6@meas_0.3_s40@pc@rp\endcsname{0.21}
\expandafter\def\csname res@v6@meas_0.3_s40@pc@map\endcsname{0.19}
\expandafter\def\csname res@v6@meas_0.3_s40@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.3_s40@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_s40@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_s40@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v6@meas_0.3_s40@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@meas_0.3_s40@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3_s40@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v6@meas_0.3_s40@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v6@meas_0.3_s40@dynotears@map\endcsname{0.93}
\expandafter\def\csname res@v6@meas_0.3_s40@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.3_s40@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3_s40@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_s40@doubleml@tt\endcsname{0.62}
\expandafter\def\csname res@v6@meas_0.3_s40@doubleml@prec\endcsname{0.69}
\expandafter\def\csname res@v6@meas_0.3_s40@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_s40@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@doubleml@len\endcsname{2.8}
\expandafter\def\csname res@v6@meas_0.3_s40@doubleml@rp\endcsname{0.72}
\expandafter\def\csname res@v6@meas_0.3_s40@doubleml@map\endcsname{0.75}
\expandafter\def\csname res@v6@meas_0.3_s40@varlingam@fp\endcsname{8/10}
\expandafter\def\csname res@v6@meas_0.3_s40@varlingam@fpn\endcsname{8}
\expandafter\def\csname res@v6@meas_0.3_s40@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_s40@varlingam@tt\endcsname{0.46}
\expandafter\def\csname res@v6@meas_0.3_s40@varlingam@prec\endcsname{0.25}
\expandafter\def\csname res@v6@meas_0.3_s40@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@varlingam@len\endcsname{13.3}
\expandafter\def\csname res@v6@meas_0.3_s40@varlingam@rp\endcsname{0.53}
\expandafter\def\csname res@v6@meas_0.3_s40@varlingam@map\endcsname{0.62}
\expandafter\def\csname res@v6@meas_0.3_s40@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v6@meas_0.3_s40@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v6@meas_0.3_s40@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_s40@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v6@meas_0.3_s40@spacetime_rule@prec\endcsname{0.89}
\expandafter\def\csname res@v6@meas_0.3_s40@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_s40@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@spacetime_rule@len\endcsname{0.9}
\expandafter\def\csname res@v6@meas_0.3_s40@spacetime_rule@rp\endcsname{0.47}
\expandafter\def\csname res@v6@meas_0.3_s40@spacetime_rule@map\endcsname{0.55}
\expandafter\def\csname res@v6@meas_0.3_s40@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.3_s40@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_s40@varsort@tt\endcsname{0.08}
\expandafter\def\csname res@v6@meas_0.3_s40@varsort@prec\endcsname{0.07}
\expandafter\def\csname res@v6@meas_0.3_s40@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@meas_0.3_s40@varsort@rp\endcsname{0.05}
\expandafter\def\csname res@v6@meas_0.3_s40@varsort@map\endcsname{0.08}
\expandafter\def\csname res@v6@meas_0.3_s40@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.3_s40@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_s40@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v6@meas_0.3_s40@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v6@meas_0.3_s40@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_s40@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@meas_0.3_s40@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v6@meas_0.3_s40@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v6@meas_0.3_b50@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v6@meas_0.3_b50@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v6@meas_0.3_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_b50@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v6@meas_0.3_b50@correlation@prec\endcsname{0.17}
\expandafter\def\csname res@v6@meas_0.3_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@correlation@bw\endcsname{2}
\expandafter\def\csname res@v6@meas_0.3_b50@correlation@len\endcsname{14.6}
\expandafter\def\csname res@v6@meas_0.3_b50@correlation@rp\endcsname{0.66}
\expandafter\def\csname res@v6@meas_0.3_b50@correlation@map\endcsname{0.74}
\expandafter\def\csname res@v6@meas_0.3_b50@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v6@meas_0.3_b50@granger@fpn\endcsname{8}
\expandafter\def\csname res@v6@meas_0.3_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_b50@granger@tt\endcsname{0.46}
\expandafter\def\csname res@v6@meas_0.3_b50@granger@prec\endcsname{0.38}
\expandafter\def\csname res@v6@meas_0.3_b50@granger@ab\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@granger@len\endcsname{7.3}
\expandafter\def\csname res@v6@meas_0.3_b50@granger@rp\endcsname{0.54}
\expandafter\def\csname res@v6@meas_0.3_b50@granger@map\endcsname{0.67}
\expandafter\def\csname res@v6@meas_0.3_b50@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.3_b50@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_b50@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v6@meas_0.3_b50@pcmciplus@prec\endcsname{0.75}
\expandafter\def\csname res@v6@meas_0.3_b50@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@pcmciplus@len\endcsname{2.7}
\expandafter\def\csname res@v6@meas_0.3_b50@pcmciplus@rp\endcsname{0.81}
\expandafter\def\csname res@v6@meas_0.3_b50@pcmciplus@map\endcsname{0.88}
\expandafter\def\csname res@v6@meas_0.3_b50@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.3_b50@pc@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_b50@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@meas_0.3_b50@pc@prec\endcsname{0.32}
\expandafter\def\csname res@v6@meas_0.3_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@pc@bw\endcsname{2}
\expandafter\def\csname res@v6@meas_0.3_b50@pc@len\endcsname{5.6}
\expandafter\def\csname res@v6@meas_0.3_b50@pc@rp\endcsname{0.32}
\expandafter\def\csname res@v6@meas_0.3_b50@pc@map\endcsname{0.28}
\expandafter\def\csname res@v6@meas_0.3_b50@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.3_b50@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_b50@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v6@meas_0.3_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@meas_0.3_b50@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v6@meas_0.3_b50@dynotears@rp\endcsname{0.84}
\expandafter\def\csname res@v6@meas_0.3_b50@dynotears@map\endcsname{0.93}
\expandafter\def\csname res@v6@meas_0.3_b50@doubleml@fp\endcsname{6/10}
\expandafter\def\csname res@v6@meas_0.3_b50@doubleml@fpn\endcsname{6}
\expandafter\def\csname res@v6@meas_0.3_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_b50@doubleml@tt\endcsname{0.58}
\expandafter\def\csname res@v6@meas_0.3_b50@doubleml@prec\endcsname{0.65}
\expandafter\def\csname res@v6@meas_0.3_b50@doubleml@ab\endcsname{3}
\expandafter\def\csname res@v6@meas_0.3_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@doubleml@len\endcsname{2.8}
\expandafter\def\csname res@v6@meas_0.3_b50@doubleml@rp\endcsname{0.65}
\expandafter\def\csname res@v6@meas_0.3_b50@doubleml@map\endcsname{0.70}
\expandafter\def\csname res@v6@meas_0.3_b50@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@meas_0.3_b50@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@meas_0.3_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_b50@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v6@meas_0.3_b50@varlingam@prec\endcsname{0.41}
\expandafter\def\csname res@v6@meas_0.3_b50@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_b50@varlingam@len\endcsname{6.5}
\expandafter\def\csname res@v6@meas_0.3_b50@varlingam@rp\endcsname{0.67}
\expandafter\def\csname res@v6@meas_0.3_b50@varlingam@map\endcsname{0.77}
\expandafter\def\csname res@v6@meas_0.3_b50@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v6@meas_0.3_b50@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v6@meas_0.3_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_b50@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v6@meas_0.3_b50@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v6@meas_0.3_b50@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v6@meas_0.3_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@spacetime_rule@len\endcsname{0.8}
\expandafter\def\csname res@v6@meas_0.3_b50@spacetime_rule@rp\endcsname{0.46}
\expandafter\def\csname res@v6@meas_0.3_b50@spacetime_rule@map\endcsname{0.65}
\expandafter\def\csname res@v6@meas_0.3_b50@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@meas_0.3_b50@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_b50@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@meas_0.3_b50@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@meas_0.3_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v6@meas_0.3_b50@varsort@rp\endcsname{0.16}
\expandafter\def\csname res@v6@meas_0.3_b50@varsort@map\endcsname{0.18}
\expandafter\def\csname res@v6@meas_0.3_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@meas_0.3_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@meas_0.3_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@meas_0.3_b50@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@meas_0.3_b50@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@meas_0.3_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@meas_0.3_b50@r2sort@bw\endcsname{3}
\expandafter\def\csname res@v6@meas_0.3_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@meas_0.3_b50@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@meas_0.3_b50@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@context_0.25@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@context_0.25@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v6@context_0.25@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@context_0.25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v6@context_0.25@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v6@context_0.25@correlation@map\endcsname{0.78}
\expandafter\def\csname res@v6@context_0.25@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@context_0.25@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@granger@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v6@context_0.25@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.25@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@granger@len\endcsname{16.8}
\expandafter\def\csname res@v6@context_0.25@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v6@context_0.25@granger@map\endcsname{0.77}
\expandafter\def\csname res@v6@context_0.25@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@context_0.25@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@pcmciplus@tt\endcsname{0.69}
\expandafter\def\csname res@v6@context_0.25@pcmciplus@prec\endcsname{0.70}
\expandafter\def\csname res@v6@context_0.25@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@pcmciplus@len\endcsname{2.9}
\expandafter\def\csname res@v6@context_0.25@pcmciplus@rp\endcsname{0.92}
\expandafter\def\csname res@v6@context_0.25@pcmciplus@map\endcsname{0.97}
\expandafter\def\csname res@v6@context_0.25@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@context_0.25@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@context_0.25@pc@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@context_0.25@pc@prec\endcsname{0.33}
\expandafter\def\csname res@v6@context_0.25@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@pc@bw\endcsname{4}
\expandafter\def\csname res@v6@context_0.25@pc@len\endcsname{5.7}
\expandafter\def\csname res@v6@context_0.25@pc@rp\endcsname{0.33}
\expandafter\def\csname res@v6@context_0.25@pc@map\endcsname{0.29}
\expandafter\def\csname res@v6@context_0.25@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v6@context_0.25@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v6@context_0.25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@dynotears@tt\endcsname{0.19}
\expandafter\def\csname res@v6@context_0.25@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@context_0.25@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v6@context_0.25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@dynotears@len\endcsname{0.5}
\expandafter\def\csname res@v6@context_0.25@dynotears@rp\endcsname{0.88}
\expandafter\def\csname res@v6@context_0.25@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v6@context_0.25@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v6@context_0.25@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v6@context_0.25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@doubleml@tt\endcsname{0.73}
\expandafter\def\csname res@v6@context_0.25@doubleml@prec\endcsname{0.76}
\expandafter\def\csname res@v6@context_0.25@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@context_0.25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@doubleml@len\endcsname{3.0}
\expandafter\def\csname res@v6@context_0.25@doubleml@rp\endcsname{0.78}
\expandafter\def\csname res@v6@context_0.25@doubleml@map\endcsname{0.86}
\expandafter\def\csname res@v6@context_0.25@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v6@context_0.25@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@varlingam@tt\endcsname{0.73}
\expandafter\def\csname res@v6@context_0.25@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v6@context_0.25@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@varlingam@len\endcsname{10.2}
\expandafter\def\csname res@v6@context_0.25@varlingam@rp\endcsname{0.74}
\expandafter\def\csname res@v6@context_0.25@varlingam@map\endcsname{0.87}
\expandafter\def\csname res@v6@context_0.25@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v6@context_0.25@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v6@context_0.25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v6@context_0.25@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v6@context_0.25@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v6@context_0.25@spacetime_rule@rp\endcsname{0.63}
\expandafter\def\csname res@v6@context_0.25@spacetime_rule@map\endcsname{0.77}
\expandafter\def\csname res@v6@context_0.25@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@context_0.25@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@context_0.25@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@context_0.25@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@context_0.25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@context_0.25@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v6@context_0.25@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.25@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_0.25@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.25@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.25@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@context_0.25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.25@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@context_0.25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@context_0.25@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@context_0.25@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@context_0.5@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v6@context_0.5@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v6@context_0.5@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v6@context_0.5@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.5@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@correlation@bw\endcsname{2}
\expandafter\def\csname res@v6@context_0.5@correlation@len\endcsname{17.4}
\expandafter\def\csname res@v6@context_0.5@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v6@context_0.5@correlation@map\endcsname{0.74}
\expandafter\def\csname res@v6@context_0.5@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v6@context_0.5@granger@fpn\endcsname{9}
\expandafter\def\csname res@v6@context_0.5@granger@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v6@context_0.5@granger@prec\endcsname{0.16}
\expandafter\def\csname res@v6@context_0.5@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@granger@len\endcsname{16.0}
\expandafter\def\csname res@v6@context_0.5@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v6@context_0.5@granger@map\endcsname{0.74}
\expandafter\def\csname res@v6@context_0.5@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@context_0.5@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@context_0.5@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v6@context_0.5@pcmciplus@prec\endcsname{0.62}
\expandafter\def\csname res@v6@context_0.5@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@pcmciplus@len\endcsname{3.4}
\expandafter\def\csname res@v6@context_0.5@pcmciplus@rp\endcsname{0.79}
\expandafter\def\csname res@v6@context_0.5@pcmciplus@map\endcsname{0.90}
\expandafter\def\csname res@v6@context_0.5@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v6@context_0.5@pc@fpn\endcsname{4}
\expandafter\def\csname res@v6@context_0.5@pc@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@pc@tt\endcsname{0.42}
\expandafter\def\csname res@v6@context_0.5@pc@prec\endcsname{0.33}
\expandafter\def\csname res@v6@context_0.5@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@context_0.5@pc@len\endcsname{5.4}
\expandafter\def\csname res@v6@context_0.5@pc@rp\endcsname{0.33}
\expandafter\def\csname res@v6@context_0.5@pc@map\endcsname{0.30}
\expandafter\def\csname res@v6@context_0.5@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v6@context_0.5@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v6@context_0.5@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v6@context_0.5@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@context_0.5@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v6@context_0.5@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v6@context_0.5@dynotears@rp\endcsname{0.81}
\expandafter\def\csname res@v6@context_0.5@dynotears@map\endcsname{0.91}
\expandafter\def\csname res@v6@context_0.5@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v6@context_0.5@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v6@context_0.5@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@doubleml@tt\endcsname{0.65}
\expandafter\def\csname res@v6@context_0.5@doubleml@prec\endcsname{0.73}
\expandafter\def\csname res@v6@context_0.5@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@context_0.5@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@doubleml@len\endcsname{3.0}
\expandafter\def\csname res@v6@context_0.5@doubleml@rp\endcsname{0.78}
\expandafter\def\csname res@v6@context_0.5@doubleml@map\endcsname{0.85}
\expandafter\def\csname res@v6@context_0.5@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@context_0.5@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@context_0.5@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@varlingam@tt\endcsname{0.58}
\expandafter\def\csname res@v6@context_0.5@varlingam@prec\endcsname{0.35}
\expandafter\def\csname res@v6@context_0.5@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v6@context_0.5@varlingam@len\endcsname{8.5}
\expandafter\def\csname res@v6@context_0.5@varlingam@rp\endcsname{0.53}
\expandafter\def\csname res@v6@context_0.5@varlingam@map\endcsname{0.72}
\expandafter\def\csname res@v6@context_0.5@spacetime_rule@fp\endcsname{10/10}
\expandafter\def\csname res@v6@context_0.5@spacetime_rule@fpn\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v6@context_0.5@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v6@context_0.5@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v6@context_0.5@spacetime_rule@rp\endcsname{0.69}
\expandafter\def\csname res@v6@context_0.5@spacetime_rule@map\endcsname{0.80}
\expandafter\def\csname res@v6@context_0.5@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@context_0.5@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@context_0.5@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@context_0.5@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@context_0.5@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@context_0.5@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.5@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v6@context_0.5@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_0.5@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.5@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.5@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@context_0.5@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.5@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@context_0.5@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@context_0.5@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@context_0.5@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@context_0.75@correlation@fp\endcsname{7/10}
\expandafter\def\csname res@v6@context_0.75@correlation@fpn\endcsname{7}
\expandafter\def\csname res@v6@context_0.75@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v6@context_0.75@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.75@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@correlation@bw\endcsname{3}
\expandafter\def\csname res@v6@context_0.75@correlation@len\endcsname{17.0}
\expandafter\def\csname res@v6@context_0.75@correlation@rp\endcsname{0.52}
\expandafter\def\csname res@v6@context_0.75@correlation@map\endcsname{0.68}
\expandafter\def\csname res@v6@context_0.75@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v6@context_0.75@granger@fpn\endcsname{8}
\expandafter\def\csname res@v6@context_0.75@granger@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v6@context_0.75@granger@prec\endcsname{0.17}
\expandafter\def\csname res@v6@context_0.75@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@granger@len\endcsname{14.8}
\expandafter\def\csname res@v6@context_0.75@granger@rp\endcsname{0.54}
\expandafter\def\csname res@v6@context_0.75@granger@map\endcsname{0.69}
\expandafter\def\csname res@v6@context_0.75@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@context_0.75@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@pcmciplus@tt\endcsname{0.69}
\expandafter\def\csname res@v6@context_0.75@pcmciplus@prec\endcsname{0.62}
\expandafter\def\csname res@v6@context_0.75@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@pcmciplus@len\endcsname{3.3}
\expandafter\def\csname res@v6@context_0.75@pcmciplus@rp\endcsname{0.84}
\expandafter\def\csname res@v6@context_0.75@pcmciplus@map\endcsname{0.92}
\expandafter\def\csname res@v6@context_0.75@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v6@context_0.75@pc@fpn\endcsname{4}
\expandafter\def\csname res@v6@context_0.75@pc@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v6@context_0.75@pc@prec\endcsname{0.31}
\expandafter\def\csname res@v6@context_0.75@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@context_0.75@pc@len\endcsname{5.3}
\expandafter\def\csname res@v6@context_0.75@pc@rp\endcsname{0.31}
\expandafter\def\csname res@v6@context_0.75@pc@map\endcsname{0.28}
\expandafter\def\csname res@v6@context_0.75@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v6@context_0.75@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v6@context_0.75@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v6@context_0.75@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@context_0.75@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v6@context_0.75@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v6@context_0.75@dynotears@rp\endcsname{0.81}
\expandafter\def\csname res@v6@context_0.75@dynotears@map\endcsname{0.91}
\expandafter\def\csname res@v6@context_0.75@doubleml@fp\endcsname{7/10}
\expandafter\def\csname res@v6@context_0.75@doubleml@fpn\endcsname{7}
\expandafter\def\csname res@v6@context_0.75@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@doubleml@tt\endcsname{0.54}
\expandafter\def\csname res@v6@context_0.75@doubleml@prec\endcsname{0.61}
\expandafter\def\csname res@v6@context_0.75@doubleml@ab\endcsname{2}
\expandafter\def\csname res@v6@context_0.75@doubleml@bw\endcsname{1}
\expandafter\def\csname res@v6@context_0.75@doubleml@len\endcsname{2.5}
\expandafter\def\csname res@v6@context_0.75@doubleml@rp\endcsname{0.66}
\expandafter\def\csname res@v6@context_0.75@doubleml@map\endcsname{0.74}
\expandafter\def\csname res@v6@context_0.75@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@context_0.75@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@context_0.75@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@varlingam@tt\endcsname{0.58}
\expandafter\def\csname res@v6@context_0.75@varlingam@prec\endcsname{0.38}
\expandafter\def\csname res@v6@context_0.75@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@varlingam@len\endcsname{7.4}
\expandafter\def\csname res@v6@context_0.75@varlingam@rp\endcsname{0.57}
\expandafter\def\csname res@v6@context_0.75@varlingam@map\endcsname{0.72}
\expandafter\def\csname res@v6@context_0.75@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v6@context_0.75@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v6@context_0.75@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@spacetime_rule@tt\endcsname{0.35}
\expandafter\def\csname res@v6@context_0.75@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v6@context_0.75@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v6@context_0.75@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@spacetime_rule@len\endcsname{0.9}
\expandafter\def\csname res@v6@context_0.75@spacetime_rule@rp\endcsname{0.56}
\expandafter\def\csname res@v6@context_0.75@spacetime_rule@map\endcsname{0.72}
\expandafter\def\csname res@v6@context_0.75@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@context_0.75@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@context_0.75@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@context_0.75@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@context_0.75@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@varsort@bw\endcsname{2}
\expandafter\def\csname res@v6@context_0.75@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@context_0.75@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.75@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v6@context_0.75@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_0.75@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.75@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@context_0.75@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@context_0.75@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@context_0.75@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@context_0.75@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@context_1.0@correlation@fp\endcsname{6/10}
\expandafter\def\csname res@v6@context_1.0@correlation@fpn\endcsname{6}
\expandafter\def\csname res@v6@context_1.0@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v6@context_1.0@correlation@prec\endcsname{0.16}
\expandafter\def\csname res@v6@context_1.0@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@correlation@bw\endcsname{4}
\expandafter\def\csname res@v6@context_1.0@correlation@len\endcsname{16.3}
\expandafter\def\csname res@v6@context_1.0@correlation@rp\endcsname{0.47}
\expandafter\def\csname res@v6@context_1.0@correlation@map\endcsname{0.63}
\expandafter\def\csname res@v6@context_1.0@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v6@context_1.0@granger@fpn\endcsname{8}
\expandafter\def\csname res@v6@context_1.0@granger@n\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v6@context_1.0@granger@prec\endcsname{0.16}
\expandafter\def\csname res@v6@context_1.0@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@granger@len\endcsname{13.4}
\expandafter\def\csname res@v6@context_1.0@granger@rp\endcsname{0.54}
\expandafter\def\csname res@v6@context_1.0@granger@map\endcsname{0.68}
\expandafter\def\csname res@v6@context_1.0@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@context_1.0@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v6@context_1.0@pcmciplus@prec\endcsname{0.63}
\expandafter\def\csname res@v6@context_1.0@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@pcmciplus@len\endcsname{3.4}
\expandafter\def\csname res@v6@context_1.0@pcmciplus@rp\endcsname{0.87}
\expandafter\def\csname res@v6@context_1.0@pcmciplus@map\endcsname{0.93}
\expandafter\def\csname res@v6@context_1.0@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v6@context_1.0@pc@fpn\endcsname{4}
\expandafter\def\csname res@v6@context_1.0@pc@n\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v6@context_1.0@pc@prec\endcsname{0.30}
\expandafter\def\csname res@v6@context_1.0@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@context_1.0@pc@len\endcsname{5.1}
\expandafter\def\csname res@v6@context_1.0@pc@rp\endcsname{0.30}
\expandafter\def\csname res@v6@context_1.0@pc@map\endcsname{0.27}
\expandafter\def\csname res@v6@context_1.0@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_1.0@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v6@context_1.0@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v6@context_1.0@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v6@context_1.0@dynotears@rp\endcsname{0.84}
\expandafter\def\csname res@v6@context_1.0@dynotears@map\endcsname{0.90}
\expandafter\def\csname res@v6@context_1.0@doubleml@fp\endcsname{7/10}
\expandafter\def\csname res@v6@context_1.0@doubleml@fpn\endcsname{7}
\expandafter\def\csname res@v6@context_1.0@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@doubleml@tt\endcsname{0.50}
\expandafter\def\csname res@v6@context_1.0@doubleml@prec\endcsname{0.80}
\expandafter\def\csname res@v6@context_1.0@doubleml@ab\endcsname{3}
\expandafter\def\csname res@v6@context_1.0@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@doubleml@len\endcsname{2.1}
\expandafter\def\csname res@v6@context_1.0@doubleml@rp\endcsname{0.57}
\expandafter\def\csname res@v6@context_1.0@doubleml@map\endcsname{0.72}
\expandafter\def\csname res@v6@context_1.0@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@context_1.0@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@context_1.0@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v6@context_1.0@varlingam@prec\endcsname{0.46}
\expandafter\def\csname res@v6@context_1.0@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@varlingam@len\endcsname{6.6}
\expandafter\def\csname res@v6@context_1.0@varlingam@rp\endcsname{0.60}
\expandafter\def\csname res@v6@context_1.0@varlingam@map\endcsname{0.78}
\expandafter\def\csname res@v6@context_1.0@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v6@context_1.0@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v6@context_1.0@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v6@context_1.0@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v6@context_1.0@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v6@context_1.0@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@spacetime_rule@len\endcsname{0.8}
\expandafter\def\csname res@v6@context_1.0@spacetime_rule@rp\endcsname{0.59}
\expandafter\def\csname res@v6@context_1.0@spacetime_rule@map\endcsname{0.75}
\expandafter\def\csname res@v6@context_1.0@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@context_1.0@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@context_1.0@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@context_1.0@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@context_1.0@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@context_1.0@varsort@rp\endcsname{0.16}
\expandafter\def\csname res@v6@context_1.0@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v6@context_1.0@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_1.0@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@context_1.0@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@context_1.0@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@context_1.0@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_1.0@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@context_1.0@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@context_1.0@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@context_1.0@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@correlation@tt\endcsname{0.12}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@correlation@prec\endcsname{0.12}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@correlation@bw\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@correlation@len\endcsname{5.4}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@correlation@rp\endcsname{0.03}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@correlation@map\endcsname{0.24}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@granger@fp\endcsname{5/10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@granger@fpn\endcsname{5}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@granger@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@granger@tt\endcsname{0.27}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@granger@prec\endcsname{0.32}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@granger@ab\endcsname{3}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@granger@bw\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@granger@len\endcsname{3.2}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@granger@rp\endcsname{0.43}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@granger@map\endcsname{0.56}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pcmciplus@fp\endcsname{3/10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pcmciplus@fpn\endcsname{3}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pcmciplus@tt\endcsname{0.12}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pcmciplus@prec\endcsname{0.62}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pcmciplus@ab\endcsname{6}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pcmciplus@len\endcsname{0.5}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pcmciplus@rp\endcsname{0.37}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pcmciplus@map\endcsname{0.48}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pc@fpn\endcsname{2}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pc@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pc@tt\endcsname{0.08}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pc@prec\endcsname{0.08}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pc@bw\endcsname{7}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pc@len\endcsname{2.4}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pc@rp\endcsname{0.14}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@pc@map\endcsname{0.19}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@dynotears@rp\endcsname{0.46}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@dynotears@map\endcsname{0.64}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@doubleml@fp\endcsname{2/10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@doubleml@fpn\endcsname{2}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@doubleml@tt\endcsname{0.08}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@doubleml@prec\endcsname{0.38}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@doubleml@len\endcsname{0.5}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@doubleml@rp\endcsname{0.32}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@doubleml@map\endcsname{0.39}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varlingam@tt\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varlingam@prec\endcsname{0.12}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varlingam@bw\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varlingam@len\endcsname{2.7}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varlingam@rp\endcsname{0.18}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varlingam@map\endcsname{0.20}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@spacetime_rule@fp\endcsname{4/10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@spacetime_rule@fpn\endcsname{4}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@spacetime_rule@tt\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@spacetime_rule@prec\endcsname{0.39}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@spacetime_rule@len\endcsname{1.0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@spacetime_rule@rp\endcsname{0.27}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@spacetime_rule@map\endcsname{0.42}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@varsort@map\endcsname{0.22}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@context_0.75_combo_interaction@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v6@context_0.75_s40@correlation@fp\endcsname{5/10}
\expandafter\def\csname res@v6@context_0.75_s40@correlation@fpn\endcsname{5}
\expandafter\def\csname res@v6@context_0.75_s40@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@correlation@tt\endcsname{0.50}
\expandafter\def\csname res@v6@context_0.75_s40@correlation@prec\endcsname{0.08}
\expandafter\def\csname res@v6@context_0.75_s40@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@correlation@bw\endcsname{4}
\expandafter\def\csname res@v6@context_0.75_s40@correlation@len\endcsname{32.4}
\expandafter\def\csname res@v6@context_0.75_s40@correlation@rp\endcsname{0.49}
\expandafter\def\csname res@v6@context_0.75_s40@correlation@map\endcsname{0.56}
\expandafter\def\csname res@v6@context_0.75_s40@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v6@context_0.75_s40@granger@fpn\endcsname{9}
\expandafter\def\csname res@v6@context_0.75_s40@granger@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@granger@tt\endcsname{0.50}
\expandafter\def\csname res@v6@context_0.75_s40@granger@prec\endcsname{0.10}
\expandafter\def\csname res@v6@context_0.75_s40@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@granger@len\endcsname{26.9}
\expandafter\def\csname res@v6@context_0.75_s40@granger@rp\endcsname{0.53}
\expandafter\def\csname res@v6@context_0.75_s40@granger@map\endcsname{0.61}
\expandafter\def\csname res@v6@context_0.75_s40@pcmciplus@fp\endcsname{8/10}
\expandafter\def\csname res@v6@context_0.75_s40@pcmciplus@fpn\endcsname{8}
\expandafter\def\csname res@v6@context_0.75_s40@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@pcmciplus@tt\endcsname{0.54}
\expandafter\def\csname res@v6@context_0.75_s40@pcmciplus@prec\endcsname{0.57}
\expandafter\def\csname res@v6@context_0.75_s40@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_s40@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@pcmciplus@len\endcsname{2.5}
\expandafter\def\csname res@v6@context_0.75_s40@pcmciplus@rp\endcsname{0.78}
\expandafter\def\csname res@v6@context_0.75_s40@pcmciplus@map\endcsname{0.78}
\expandafter\def\csname res@v6@context_0.75_s40@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@context_0.75_s40@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@context_0.75_s40@pc@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@context_0.75_s40@pc@prec\endcsname{0.31}
\expandafter\def\csname res@v6@context_0.75_s40@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@context_0.75_s40@pc@len\endcsname{4.7}
\expandafter\def\csname res@v6@context_0.75_s40@pc@rp\endcsname{0.29}
\expandafter\def\csname res@v6@context_0.75_s40@pc@map\endcsname{0.20}
\expandafter\def\csname res@v6@context_0.75_s40@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_0.75_s40@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v6@context_0.75_s40@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v6@context_0.75_s40@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v6@context_0.75_s40@dynotears@rp\endcsname{0.88}
\expandafter\def\csname res@v6@context_0.75_s40@dynotears@map\endcsname{0.93}
\expandafter\def\csname res@v6@context_0.75_s40@doubleml@fp\endcsname{7/10}
\expandafter\def\csname res@v6@context_0.75_s40@doubleml@fpn\endcsname{7}
\expandafter\def\csname res@v6@context_0.75_s40@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@doubleml@tt\endcsname{0.46}
\expandafter\def\csname res@v6@context_0.75_s40@doubleml@prec\endcsname{0.82}
\expandafter\def\csname res@v6@context_0.75_s40@doubleml@ab\endcsname{3}
\expandafter\def\csname res@v6@context_0.75_s40@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@doubleml@len\endcsname{1.7}
\expandafter\def\csname res@v6@context_0.75_s40@doubleml@rp\endcsname{0.55}
\expandafter\def\csname res@v6@context_0.75_s40@doubleml@map\endcsname{0.65}
\expandafter\def\csname res@v6@context_0.75_s40@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@context_0.75_s40@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@context_0.75_s40@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@varlingam@tt\endcsname{0.46}
\expandafter\def\csname res@v6@context_0.75_s40@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v6@context_0.75_s40@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@varlingam@len\endcsname{8.7}
\expandafter\def\csname res@v6@context_0.75_s40@varlingam@rp\endcsname{0.52}
\expandafter\def\csname res@v6@context_0.75_s40@varlingam@map\endcsname{0.60}
\expandafter\def\csname res@v6@context_0.75_s40@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v6@context_0.75_s40@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v6@context_0.75_s40@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v6@context_0.75_s40@spacetime_rule@prec\endcsname{0.90}
\expandafter\def\csname res@v6@context_0.75_s40@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v6@context_0.75_s40@spacetime_rule@rp\endcsname{0.62}
\expandafter\def\csname res@v6@context_0.75_s40@spacetime_rule@map\endcsname{0.69}
\expandafter\def\csname res@v6@context_0.75_s40@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_0.75_s40@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v6@context_0.75_s40@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v6@context_0.75_s40@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_s40@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@context_0.75_s40@varsort@rp\endcsname{0.05}
\expandafter\def\csname res@v6@context_0.75_s40@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v6@context_0.75_s40@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_0.75_s40@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_s40@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v6@context_0.75_s40@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v6@context_0.75_s40@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_s40@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@context_0.75_s40@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v6@context_0.75_s40@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v6@context_0.75_b50@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v6@context_0.75_b50@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v6@context_0.75_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_b50@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v6@context_0.75_b50@correlation@prec\endcsname{0.17}
\expandafter\def\csname res@v6@context_0.75_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@correlation@bw\endcsname{2}
\expandafter\def\csname res@v6@context_0.75_b50@correlation@len\endcsname{13.0}
\expandafter\def\csname res@v6@context_0.75_b50@correlation@rp\endcsname{0.60}
\expandafter\def\csname res@v6@context_0.75_b50@correlation@map\endcsname{0.71}
\expandafter\def\csname res@v6@context_0.75_b50@granger@fp\endcsname{7/10}
\expandafter\def\csname res@v6@context_0.75_b50@granger@fpn\endcsname{7}
\expandafter\def\csname res@v6@context_0.75_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_b50@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v6@context_0.75_b50@granger@prec\endcsname{0.40}
\expandafter\def\csname res@v6@context_0.75_b50@granger@ab\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@granger@len\endcsname{6.6}
\expandafter\def\csname res@v6@context_0.75_b50@granger@rp\endcsname{0.55}
\expandafter\def\csname res@v6@context_0.75_b50@granger@map\endcsname{0.64}
\expandafter\def\csname res@v6@context_0.75_b50@pcmciplus@fp\endcsname{7/10}
\expandafter\def\csname res@v6@context_0.75_b50@pcmciplus@fpn\endcsname{7}
\expandafter\def\csname res@v6@context_0.75_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_b50@pcmciplus@tt\endcsname{0.38}
\expandafter\def\csname res@v6@context_0.75_b50@pcmciplus@prec\endcsname{0.67}
\expandafter\def\csname res@v6@context_0.75_b50@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@pcmciplus@len\endcsname{1.7}
\expandafter\def\csname res@v6@context_0.75_b50@pcmciplus@rp\endcsname{0.70}
\expandafter\def\csname res@v6@context_0.75_b50@pcmciplus@map\endcsname{0.80}
\expandafter\def\csname res@v6@context_0.75_b50@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@context_0.75_b50@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@context_0.75_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_b50@pc@tt\endcsname{0.54}
\expandafter\def\csname res@v6@context_0.75_b50@pc@prec\endcsname{0.36}
\expandafter\def\csname res@v6@context_0.75_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@pc@bw\endcsname{6}
\expandafter\def\csname res@v6@context_0.75_b50@pc@len\endcsname{4.3}
\expandafter\def\csname res@v6@context_0.75_b50@pc@rp\endcsname{0.34}
\expandafter\def\csname res@v6@context_0.75_b50@pc@map\endcsname{0.33}
\expandafter\def\csname res@v6@context_0.75_b50@dynotears@fp\endcsname{2/10}
\expandafter\def\csname res@v6@context_0.75_b50@dynotears@fpn\endcsname{2}
\expandafter\def\csname res@v6@context_0.75_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_b50@dynotears@tt\endcsname{0.08}
\expandafter\def\csname res@v6@context_0.75_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@context_0.75_b50@dynotears@ab\endcsname{8}
\expandafter\def\csname res@v6@context_0.75_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@dynotears@len\endcsname{0.2}
\expandafter\def\csname res@v6@context_0.75_b50@dynotears@rp\endcsname{0.74}
\expandafter\def\csname res@v6@context_0.75_b50@dynotears@map\endcsname{0.84}
\expandafter\def\csname res@v6@context_0.75_b50@doubleml@fp\endcsname{5/10}
\expandafter\def\csname res@v6@context_0.75_b50@doubleml@fpn\endcsname{5}
\expandafter\def\csname res@v6@context_0.75_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_b50@doubleml@tt\endcsname{0.31}
\expandafter\def\csname res@v6@context_0.75_b50@doubleml@prec\endcsname{0.73}
\expandafter\def\csname res@v6@context_0.75_b50@doubleml@ab\endcsname{5}
\expandafter\def\csname res@v6@context_0.75_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@doubleml@len\endcsname{1.1}
\expandafter\def\csname res@v6@context_0.75_b50@doubleml@rp\endcsname{0.42}
\expandafter\def\csname res@v6@context_0.75_b50@doubleml@map\endcsname{0.57}
\expandafter\def\csname res@v6@context_0.75_b50@varlingam@fp\endcsname{7/10}
\expandafter\def\csname res@v6@context_0.75_b50@varlingam@fpn\endcsname{7}
\expandafter\def\csname res@v6@context_0.75_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_b50@varlingam@tt\endcsname{0.38}
\expandafter\def\csname res@v6@context_0.75_b50@varlingam@prec\endcsname{0.35}
\expandafter\def\csname res@v6@context_0.75_b50@varlingam@ab\endcsname{3}
\expandafter\def\csname res@v6@context_0.75_b50@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@varlingam@len\endcsname{3.9}
\expandafter\def\csname res@v6@context_0.75_b50@varlingam@rp\endcsname{0.54}
\expandafter\def\csname res@v6@context_0.75_b50@varlingam@map\endcsname{0.67}
\expandafter\def\csname res@v6@context_0.75_b50@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v6@context_0.75_b50@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v6@context_0.75_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_b50@spacetime_rule@tt\endcsname{0.27}
\expandafter\def\csname res@v6@context_0.75_b50@spacetime_rule@prec\endcsname{0.93}
\expandafter\def\csname res@v6@context_0.75_b50@spacetime_rule@ab\endcsname{3}
\expandafter\def\csname res@v6@context_0.75_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@spacetime_rule@len\endcsname{0.8}
\expandafter\def\csname res@v6@context_0.75_b50@spacetime_rule@rp\endcsname{0.44}
\expandafter\def\csname res@v6@context_0.75_b50@spacetime_rule@map\endcsname{0.55}
\expandafter\def\csname res@v6@context_0.75_b50@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@context_0.75_b50@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_b50@varsort@tt\endcsname{0.08}
\expandafter\def\csname res@v6@context_0.75_b50@varsort@prec\endcsname{0.07}
\expandafter\def\csname res@v6@context_0.75_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@context_0.75_b50@varsort@rp\endcsname{0.08}
\expandafter\def\csname res@v6@context_0.75_b50@varsort@map\endcsname{0.14}
\expandafter\def\csname res@v6@context_0.75_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@context_0.75_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@context_0.75_b50@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@context_0.75_b50@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@context_0.75_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@context_0.75_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@context_0.75_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@context_0.75_b50@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v6@context_0.75_b50@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@jitter_0.25@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.25@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@correlation@tt\endcsname{0.62}
\expandafter\def\csname res@v6@jitter_0.25@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@jitter_0.25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@correlation@len\endcsname{18.5}
\expandafter\def\csname res@v6@jitter_0.25@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v6@jitter_0.25@correlation@map\endcsname{0.79}
\expandafter\def\csname res@v6@jitter_0.25@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.25@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@granger@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@granger@tt\endcsname{0.73}
\expandafter\def\csname res@v6@jitter_0.25@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v6@jitter_0.25@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@granger@len\endcsname{17.1}
\expandafter\def\csname res@v6@jitter_0.25@granger@rp\endcsname{0.73}
\expandafter\def\csname res@v6@jitter_0.25@granger@map\endcsname{0.84}
\expandafter\def\csname res@v6@jitter_0.25@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.25@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@pcmciplus@tt\endcsname{0.92}
\expandafter\def\csname res@v6@jitter_0.25@pcmciplus@prec\endcsname{0.73}
\expandafter\def\csname res@v6@jitter_0.25@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@pcmciplus@len\endcsname{3.5}
\expandafter\def\csname res@v6@jitter_0.25@pcmciplus@rp\endcsname{0.93}
\expandafter\def\csname res@v6@jitter_0.25@pcmciplus@map\endcsname{0.97}
\expandafter\def\csname res@v6@jitter_0.25@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@jitter_0.25@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@jitter_0.25@pc@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@jitter_0.25@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v6@jitter_0.25@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@jitter_0.25@pc@len\endcsname{5.6}
\expandafter\def\csname res@v6@jitter_0.25@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v6@jitter_0.25@pc@map\endcsname{0.30}
\expandafter\def\csname res@v6@jitter_0.25@dynotears@fp\endcsname{7/10}
\expandafter\def\csname res@v6@jitter_0.25@dynotears@fpn\endcsname{7}
\expandafter\def\csname res@v6@jitter_0.25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@dynotears@tt\endcsname{0.31}
\expandafter\def\csname res@v6@jitter_0.25@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@jitter_0.25@dynotears@ab\endcsname{3}
\expandafter\def\csname res@v6@jitter_0.25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@dynotears@len\endcsname{0.8}
\expandafter\def\csname res@v6@jitter_0.25@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v6@jitter_0.25@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v6@jitter_0.25@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.25@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@doubleml@tt\endcsname{0.88}
\expandafter\def\csname res@v6@jitter_0.25@doubleml@prec\endcsname{0.68}
\expandafter\def\csname res@v6@jitter_0.25@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@doubleml@len\endcsname{4.1}
\expandafter\def\csname res@v6@jitter_0.25@doubleml@rp\endcsname{0.95}
\expandafter\def\csname res@v6@jitter_0.25@doubleml@map\endcsname{0.96}
\expandafter\def\csname res@v6@jitter_0.25@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.25@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v6@jitter_0.25@varlingam@prec\endcsname{0.33}
\expandafter\def\csname res@v6@jitter_0.25@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@varlingam@len\endcsname{9.9}
\expandafter\def\csname res@v6@jitter_0.25@varlingam@rp\endcsname{0.78}
\expandafter\def\csname res@v6@jitter_0.25@varlingam@map\endcsname{0.90}
\expandafter\def\csname res@v6@jitter_0.25@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v6@jitter_0.25@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v6@jitter_0.25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v6@jitter_0.25@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v6@jitter_0.25@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v6@jitter_0.25@spacetime_rule@rp\endcsname{0.76}
\expandafter\def\csname res@v6@jitter_0.25@spacetime_rule@map\endcsname{0.82}
\expandafter\def\csname res@v6@jitter_0.25@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@jitter_0.25@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.25@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@jitter_0.25@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@jitter_0.25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.25@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@jitter_0.25@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.25@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.25@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@jitter_0.25@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.25@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.25@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@jitter_0.25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.25@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@jitter_0.25@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@jitter_0.25@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@jitter_0.5@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.5@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@correlation@tt\endcsname{0.65}
\expandafter\def\csname res@v6@jitter_0.5@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@jitter_0.5@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@correlation@len\endcsname{18.4}
\expandafter\def\csname res@v6@jitter_0.5@correlation@rp\endcsname{0.63}
\expandafter\def\csname res@v6@jitter_0.5@correlation@map\endcsname{0.79}
\expandafter\def\csname res@v6@jitter_0.5@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.5@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@granger@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@granger@tt\endcsname{0.77}
\expandafter\def\csname res@v6@jitter_0.5@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v6@jitter_0.5@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@granger@len\endcsname{17.3}
\expandafter\def\csname res@v6@jitter_0.5@granger@rp\endcsname{0.78}
\expandafter\def\csname res@v6@jitter_0.5@granger@map\endcsname{0.87}
\expandafter\def\csname res@v6@jitter_0.5@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.5@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@pcmciplus@tt\endcsname{0.85}
\expandafter\def\csname res@v6@jitter_0.5@pcmciplus@prec\endcsname{0.74}
\expandafter\def\csname res@v6@jitter_0.5@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@pcmciplus@len\endcsname{3.3}
\expandafter\def\csname res@v6@jitter_0.5@pcmciplus@rp\endcsname{0.94}
\expandafter\def\csname res@v6@jitter_0.5@pcmciplus@map\endcsname{0.98}
\expandafter\def\csname res@v6@jitter_0.5@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@jitter_0.5@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@jitter_0.5@pc@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@jitter_0.5@pc@prec\endcsname{0.32}
\expandafter\def\csname res@v6@jitter_0.5@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@jitter_0.5@pc@len\endcsname{5.7}
\expandafter\def\csname res@v6@jitter_0.5@pc@rp\endcsname{0.32}
\expandafter\def\csname res@v6@jitter_0.5@pc@map\endcsname{0.28}
\expandafter\def\csname res@v6@jitter_0.5@dynotears@fp\endcsname{8/10}
\expandafter\def\csname res@v6@jitter_0.5@dynotears@fpn\endcsname{8}
\expandafter\def\csname res@v6@jitter_0.5@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@dynotears@tt\endcsname{0.54}
\expandafter\def\csname res@v6@jitter_0.5@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@jitter_0.5@dynotears@ab\endcsname{2}
\expandafter\def\csname res@v6@jitter_0.5@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@dynotears@len\endcsname{1.4}
\expandafter\def\csname res@v6@jitter_0.5@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v6@jitter_0.5@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v6@jitter_0.5@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.5@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@doubleml@tt\endcsname{0.88}
\expandafter\def\csname res@v6@jitter_0.5@doubleml@prec\endcsname{0.75}
\expandafter\def\csname res@v6@jitter_0.5@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@doubleml@len\endcsname{3.7}
\expandafter\def\csname res@v6@jitter_0.5@doubleml@rp\endcsname{0.93}
\expandafter\def\csname res@v6@jitter_0.5@doubleml@map\endcsname{0.95}
\expandafter\def\csname res@v6@jitter_0.5@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.5@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v6@jitter_0.5@varlingam@prec\endcsname{0.28}
\expandafter\def\csname res@v6@jitter_0.5@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@varlingam@len\endcsname{9.6}
\expandafter\def\csname res@v6@jitter_0.5@varlingam@rp\endcsname{0.78}
\expandafter\def\csname res@v6@jitter_0.5@varlingam@map\endcsname{0.87}
\expandafter\def\csname res@v6@jitter_0.5@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v6@jitter_0.5@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v6@jitter_0.5@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v6@jitter_0.5@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v6@jitter_0.5@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v6@jitter_0.5@spacetime_rule@rp\endcsname{0.76}
\expandafter\def\csname res@v6@jitter_0.5@spacetime_rule@map\endcsname{0.80}
\expandafter\def\csname res@v6@jitter_0.5@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@jitter_0.5@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.5@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@jitter_0.5@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@varsort@bw\endcsname{2}
\expandafter\def\csname res@v6@jitter_0.5@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@jitter_0.5@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v6@jitter_0.5@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.5@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@jitter_0.5@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.5@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.5@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@jitter_0.5@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.5@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.5@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@jitter_0.5@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@jitter_0.5@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@jitter_1.0@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_1.0@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v6@jitter_1.0@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@jitter_1.0@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@correlation@len\endcsname{18.2}
\expandafter\def\csname res@v6@jitter_1.0@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v6@jitter_1.0@correlation@map\endcsname{0.78}
\expandafter\def\csname res@v6@jitter_1.0@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_1.0@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@granger@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@granger@tt\endcsname{0.81}
\expandafter\def\csname res@v6@jitter_1.0@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_1.0@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@granger@len\endcsname{17.2}
\expandafter\def\csname res@v6@jitter_1.0@granger@rp\endcsname{0.78}
\expandafter\def\csname res@v6@jitter_1.0@granger@map\endcsname{0.88}
\expandafter\def\csname res@v6@jitter_1.0@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_1.0@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@pcmciplus@tt\endcsname{0.92}
\expandafter\def\csname res@v6@jitter_1.0@pcmciplus@prec\endcsname{0.65}
\expandafter\def\csname res@v6@jitter_1.0@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@pcmciplus@len\endcsname{4.0}
\expandafter\def\csname res@v6@jitter_1.0@pcmciplus@rp\endcsname{0.97}
\expandafter\def\csname res@v6@jitter_1.0@pcmciplus@map\endcsname{0.99}
\expandafter\def\csname res@v6@jitter_1.0@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v6@jitter_1.0@pc@fpn\endcsname{4}
\expandafter\def\csname res@v6@jitter_1.0@pc@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v6@jitter_1.0@pc@prec\endcsname{0.30}
\expandafter\def\csname res@v6@jitter_1.0@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@jitter_1.0@pc@len\endcsname{6.2}
\expandafter\def\csname res@v6@jitter_1.0@pc@rp\endcsname{0.30}
\expandafter\def\csname res@v6@jitter_1.0@pc@map\endcsname{0.26}
\expandafter\def\csname res@v6@jitter_1.0@dynotears@fp\endcsname{9/10}
\expandafter\def\csname res@v6@jitter_1.0@dynotears@fpn\endcsname{9}
\expandafter\def\csname res@v6@jitter_1.0@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@dynotears@tt\endcsname{0.58}
\expandafter\def\csname res@v6@jitter_1.0@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@jitter_1.0@dynotears@ab\endcsname{1}
\expandafter\def\csname res@v6@jitter_1.0@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@dynotears@len\endcsname{1.5}
\expandafter\def\csname res@v6@jitter_1.0@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v6@jitter_1.0@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v6@jitter_1.0@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_1.0@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v6@jitter_1.0@doubleml@prec\endcsname{0.84}
\expandafter\def\csname res@v6@jitter_1.0@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@doubleml@len\endcsname{3.1}
\expandafter\def\csname res@v6@jitter_1.0@doubleml@rp\endcsname{0.84}
\expandafter\def\csname res@v6@jitter_1.0@doubleml@map\endcsname{0.92}
\expandafter\def\csname res@v6@jitter_1.0@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@jitter_1.0@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@jitter_1.0@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v6@jitter_1.0@varlingam@prec\endcsname{0.37}
\expandafter\def\csname res@v6@jitter_1.0@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@varlingam@len\endcsname{8.9}
\expandafter\def\csname res@v6@jitter_1.0@varlingam@rp\endcsname{0.67}
\expandafter\def\csname res@v6@jitter_1.0@varlingam@map\endcsname{0.83}
\expandafter\def\csname res@v6@jitter_1.0@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v6@jitter_1.0@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v6@jitter_1.0@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@spacetime_rule@tt\endcsname{0.35}
\expandafter\def\csname res@v6@jitter_1.0@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v6@jitter_1.0@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v6@jitter_1.0@spacetime_rule@rp\endcsname{0.57}
\expandafter\def\csname res@v6@jitter_1.0@spacetime_rule@map\endcsname{0.75}
\expandafter\def\csname res@v6@jitter_1.0@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@jitter_1.0@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@jitter_1.0@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@jitter_1.0@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@jitter_1.0@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@jitter_1.0@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_1.0@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v6@jitter_1.0@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@jitter_1.0@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_1.0@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_1.0@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@jitter_1.0@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_1.0@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_1.0@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@jitter_1.0@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@jitter_1.0@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@jitter_0.75@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@correlation@tt\endcsname{0.62}
\expandafter\def\csname res@v6@jitter_0.75@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@jitter_0.75@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@correlation@len\endcsname{18.4}
\expandafter\def\csname res@v6@jitter_0.75@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v6@jitter_0.75@correlation@map\endcsname{0.79}
\expandafter\def\csname res@v6@jitter_0.75@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@granger@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@granger@tt\endcsname{0.81}
\expandafter\def\csname res@v6@jitter_0.75@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v6@jitter_0.75@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@granger@len\endcsname{17.5}
\expandafter\def\csname res@v6@jitter_0.75@granger@rp\endcsname{0.81}
\expandafter\def\csname res@v6@jitter_0.75@granger@map\endcsname{0.88}
\expandafter\def\csname res@v6@jitter_0.75@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@pcmciplus@tt\endcsname{0.88}
\expandafter\def\csname res@v6@jitter_0.75@pcmciplus@prec\endcsname{0.77}
\expandafter\def\csname res@v6@jitter_0.75@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@pcmciplus@len\endcsname{3.3}
\expandafter\def\csname res@v6@jitter_0.75@pcmciplus@rp\endcsname{0.97}
\expandafter\def\csname res@v6@jitter_0.75@pcmciplus@map\endcsname{0.98}
\expandafter\def\csname res@v6@jitter_0.75@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v6@jitter_0.75@pc@fpn\endcsname{4}
\expandafter\def\csname res@v6@jitter_0.75@pc@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v6@jitter_0.75@pc@prec\endcsname{0.33}
\expandafter\def\csname res@v6@jitter_0.75@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@jitter_0.75@pc@len\endcsname{5.8}
\expandafter\def\csname res@v6@jitter_0.75@pc@rp\endcsname{0.33}
\expandafter\def\csname res@v6@jitter_0.75@pc@map\endcsname{0.28}
\expandafter\def\csname res@v6@jitter_0.75@dynotears@fp\endcsname{8/10}
\expandafter\def\csname res@v6@jitter_0.75@dynotears@fpn\endcsname{8}
\expandafter\def\csname res@v6@jitter_0.75@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@dynotears@tt\endcsname{0.58}
\expandafter\def\csname res@v6@jitter_0.75@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@jitter_0.75@dynotears@ab\endcsname{2}
\expandafter\def\csname res@v6@jitter_0.75@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@dynotears@len\endcsname{1.5}
\expandafter\def\csname res@v6@jitter_0.75@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v6@jitter_0.75@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v6@jitter_0.75@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v6@jitter_0.75@doubleml@prec\endcsname{0.76}
\expandafter\def\csname res@v6@jitter_0.75@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@doubleml@len\endcsname{3.2}
\expandafter\def\csname res@v6@jitter_0.75@doubleml@rp\endcsname{0.90}
\expandafter\def\csname res@v6@jitter_0.75@doubleml@map\endcsname{0.94}
\expandafter\def\csname res@v6@jitter_0.75@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v6@jitter_0.75@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v6@jitter_0.75@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@varlingam@len\endcsname{8.9}
\expandafter\def\csname res@v6@jitter_0.75@varlingam@rp\endcsname{0.78}
\expandafter\def\csname res@v6@jitter_0.75@varlingam@map\endcsname{0.87}
\expandafter\def\csname res@v6@jitter_0.75@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v6@jitter_0.75@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v6@jitter_0.75@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v6@jitter_0.75@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v6@jitter_0.75@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v6@jitter_0.75@spacetime_rule@rp\endcsname{0.72}
\expandafter\def\csname res@v6@jitter_0.75@spacetime_rule@map\endcsname{0.81}
\expandafter\def\csname res@v6@jitter_0.75@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@jitter_0.75@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@jitter_0.75@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@jitter_0.75@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@jitter_0.75@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.75@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v6@jitter_0.75@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@jitter_0.75@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.75@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@jitter_0.75@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@jitter_0.75@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@jitter_0.75@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@correlation@tt\endcsname{0.08}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@correlation@prec\endcsname{0.10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@correlation@bw\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@correlation@len\endcsname{5.7}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@correlation@rp\endcsname{0.06}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@correlation@map\endcsname{0.24}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@granger@fp\endcsname{5/10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@granger@fpn\endcsname{5}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@granger@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@granger@tt\endcsname{0.23}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@granger@prec\endcsname{0.38}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@granger@ab\endcsname{5}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@granger@len\endcsname{3.4}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@granger@rp\endcsname{0.44}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@granger@map\endcsname{0.53}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pcmciplus@fp\endcsname{6/10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pcmciplus@fpn\endcsname{6}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pcmciplus@tt\endcsname{0.27}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pcmciplus@prec\endcsname{0.52}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pcmciplus@ab\endcsname{2}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pcmciplus@len\endcsname{1.4}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pcmciplus@rp\endcsname{0.44}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pcmciplus@map\endcsname{0.58}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pc@fpn\endcsname{2}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pc@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pc@tt\endcsname{0.08}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pc@prec\endcsname{0.07}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pc@bw\endcsname{7}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pc@len\endcsname{2.6}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pc@rp\endcsname{0.12}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@pc@map\endcsname{0.18}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@dynotears@rp\endcsname{0.35}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@dynotears@map\endcsname{0.47}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@doubleml@prec\endcsname{0.12}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@doubleml@len\endcsname{0.5}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@doubleml@rp\endcsname{0.24}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@doubleml@map\endcsname{0.34}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varlingam@fp\endcsname{1/10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varlingam@fpn\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varlingam@tt\endcsname{0.08}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varlingam@prec\endcsname{0.17}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varlingam@bw\endcsname{9}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varlingam@len\endcsname{4.6}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varlingam@rp\endcsname{0.13}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varlingam@map\endcsname{0.25}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@spacetime_rule@fp\endcsname{5/10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@spacetime_rule@fpn\endcsname{5}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@spacetime_rule@tt\endcsname{0.19}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@spacetime_rule@prec\endcsname{0.45}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@spacetime_rule@rp\endcsname{0.30}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@spacetime_rule@map\endcsname{0.48}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@varsort@map\endcsname{0.21}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@jitter_0.75_combo_interaction@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v6@jitter_0.75_s40@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v6@jitter_0.75_s40@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v6@jitter_0.75_s40@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v6@jitter_0.75_s40@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v6@jitter_0.75_s40@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@correlation@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_s40@correlation@len\endcsname{36.6}
\expandafter\def\csname res@v6@jitter_0.75_s40@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v6@jitter_0.75_s40@correlation@map\endcsname{0.64}
\expandafter\def\csname res@v6@jitter_0.75_s40@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75_s40@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@granger@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@granger@tt\endcsname{0.73}
\expandafter\def\csname res@v6@jitter_0.75_s40@granger@prec\endcsname{0.08}
\expandafter\def\csname res@v6@jitter_0.75_s40@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@granger@len\endcsname{33.7}
\expandafter\def\csname res@v6@jitter_0.75_s40@granger@rp\endcsname{0.71}
\expandafter\def\csname res@v6@jitter_0.75_s40@granger@map\endcsname{0.81}
\expandafter\def\csname res@v6@jitter_0.75_s40@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75_s40@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@pcmciplus@tt\endcsname{0.88}
\expandafter\def\csname res@v6@jitter_0.75_s40@pcmciplus@prec\endcsname{0.78}
\expandafter\def\csname res@v6@jitter_0.75_s40@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@pcmciplus@len\endcsname{3.4}
\expandafter\def\csname res@v6@jitter_0.75_s40@pcmciplus@rp\endcsname{0.92}
\expandafter\def\csname res@v6@jitter_0.75_s40@pcmciplus@map\endcsname{0.97}
\expandafter\def\csname res@v6@jitter_0.75_s40@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v6@jitter_0.75_s40@pc@fpn\endcsname{2}
\expandafter\def\csname res@v6@jitter_0.75_s40@pc@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v6@jitter_0.75_s40@pc@prec\endcsname{0.23}
\expandafter\def\csname res@v6@jitter_0.75_s40@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@jitter_0.75_s40@pc@len\endcsname{6.0}
\expandafter\def\csname res@v6@jitter_0.75_s40@pc@rp\endcsname{0.23}
\expandafter\def\csname res@v6@jitter_0.75_s40@pc@map\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.75_s40@dynotears@fp\endcsname{7/10}
\expandafter\def\csname res@v6@jitter_0.75_s40@dynotears@fpn\endcsname{7}
\expandafter\def\csname res@v6@jitter_0.75_s40@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@dynotears@tt\endcsname{0.46}
\expandafter\def\csname res@v6@jitter_0.75_s40@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@jitter_0.75_s40@dynotears@ab\endcsname{3}
\expandafter\def\csname res@v6@jitter_0.75_s40@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@dynotears@len\endcsname{1.3}
\expandafter\def\csname res@v6@jitter_0.75_s40@dynotears@rp\endcsname{0.92}
\expandafter\def\csname res@v6@jitter_0.75_s40@dynotears@map\endcsname{0.95}
\expandafter\def\csname res@v6@jitter_0.75_s40@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75_s40@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v6@jitter_0.75_s40@doubleml@prec\endcsname{0.78}
\expandafter\def\csname res@v6@jitter_0.75_s40@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@doubleml@len\endcsname{3.2}
\expandafter\def\csname res@v6@jitter_0.75_s40@doubleml@rp\endcsname{0.85}
\expandafter\def\csname res@v6@jitter_0.75_s40@doubleml@map\endcsname{0.90}
\expandafter\def\csname res@v6@jitter_0.75_s40@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@jitter_0.75_s40@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@jitter_0.75_s40@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v6@jitter_0.75_s40@varlingam@prec\endcsname{0.30}
\expandafter\def\csname res@v6@jitter_0.75_s40@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_s40@varlingam@len\endcsname{9.3}
\expandafter\def\csname res@v6@jitter_0.75_s40@varlingam@rp\endcsname{0.76}
\expandafter\def\csname res@v6@jitter_0.75_s40@varlingam@map\endcsname{0.78}
\expandafter\def\csname res@v6@jitter_0.75_s40@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v6@jitter_0.75_s40@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v6@jitter_0.75_s40@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v6@jitter_0.75_s40@spacetime_rule@prec\endcsname{0.80}
\expandafter\def\csname res@v6@jitter_0.75_s40@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v6@jitter_0.75_s40@spacetime_rule@rp\endcsname{0.44}
\expandafter\def\csname res@v6@jitter_0.75_s40@spacetime_rule@map\endcsname{0.57}
\expandafter\def\csname res@v6@jitter_0.75_s40@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@jitter_0.75_s40@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v6@jitter_0.75_s40@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v6@jitter_0.75_s40@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_s40@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@jitter_0.75_s40@varsort@rp\endcsname{0.05}
\expandafter\def\csname res@v6@jitter_0.75_s40@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v6@jitter_0.75_s40@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@jitter_0.75_s40@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_s40@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v6@jitter_0.75_s40@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v6@jitter_0.75_s40@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_s40@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@jitter_0.75_s40@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v6@jitter_0.75_s40@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v6@jitter_0.75_b50@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v6@jitter_0.75_b50@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v6@jitter_0.75_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@correlation@tt\endcsname{0.69}
\expandafter\def\csname res@v6@jitter_0.75_b50@correlation@prec\endcsname{0.17}
\expandafter\def\csname res@v6@jitter_0.75_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@correlation@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_b50@correlation@len\endcsname{15.5}
\expandafter\def\csname res@v6@jitter_0.75_b50@correlation@rp\endcsname{0.75}
\expandafter\def\csname res@v6@jitter_0.75_b50@correlation@map\endcsname{0.80}
\expandafter\def\csname res@v6@jitter_0.75_b50@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75_b50@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@granger@tt\endcsname{0.85}
\expandafter\def\csname res@v6@jitter_0.75_b50@granger@prec\endcsname{0.30}
\expandafter\def\csname res@v6@jitter_0.75_b50@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@granger@len\endcsname{10.5}
\expandafter\def\csname res@v6@jitter_0.75_b50@granger@rp\endcsname{0.82}
\expandafter\def\csname res@v6@jitter_0.75_b50@granger@map\endcsname{0.89}
\expandafter\def\csname res@v6@jitter_0.75_b50@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75_b50@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@pcmciplus@tt\endcsname{0.85}
\expandafter\def\csname res@v6@jitter_0.75_b50@pcmciplus@prec\endcsname{0.79}
\expandafter\def\csname res@v6@jitter_0.75_b50@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@pcmciplus@len\endcsname{2.8}
\expandafter\def\csname res@v6@jitter_0.75_b50@pcmciplus@rp\endcsname{0.97}
\expandafter\def\csname res@v6@jitter_0.75_b50@pcmciplus@map\endcsname{0.98}
\expandafter\def\csname res@v6@jitter_0.75_b50@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@jitter_0.75_b50@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@jitter_0.75_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@pc@tt\endcsname{0.46}
\expandafter\def\csname res@v6@jitter_0.75_b50@pc@prec\endcsname{0.42}
\expandafter\def\csname res@v6@jitter_0.75_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@jitter_0.75_b50@pc@len\endcsname{4.1}
\expandafter\def\csname res@v6@jitter_0.75_b50@pc@rp\endcsname{0.39}
\expandafter\def\csname res@v6@jitter_0.75_b50@pc@map\endcsname{0.35}
\expandafter\def\csname res@v6@jitter_0.75_b50@dynotears@fp\endcsname{9/10}
\expandafter\def\csname res@v6@jitter_0.75_b50@dynotears@fpn\endcsname{9}
\expandafter\def\csname res@v6@jitter_0.75_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@dynotears@tt\endcsname{0.54}
\expandafter\def\csname res@v6@jitter_0.75_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@jitter_0.75_b50@dynotears@ab\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@dynotears@len\endcsname{1.4}
\expandafter\def\csname res@v6@jitter_0.75_b50@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v6@jitter_0.75_b50@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v6@jitter_0.75_b50@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v6@jitter_0.75_b50@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v6@jitter_0.75_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@doubleml@tt\endcsname{0.69}
\expandafter\def\csname res@v6@jitter_0.75_b50@doubleml@prec\endcsname{0.83}
\expandafter\def\csname res@v6@jitter_0.75_b50@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@doubleml@len\endcsname{2.4}
\expandafter\def\csname res@v6@jitter_0.75_b50@doubleml@rp\endcsname{0.83}
\expandafter\def\csname res@v6@jitter_0.75_b50@doubleml@map\endcsname{0.86}
\expandafter\def\csname res@v6@jitter_0.75_b50@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v6@jitter_0.75_b50@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@varlingam@tt\endcsname{0.73}
\expandafter\def\csname res@v6@jitter_0.75_b50@varlingam@prec\endcsname{0.38}
\expandafter\def\csname res@v6@jitter_0.75_b50@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@varlingam@len\endcsname{7.1}
\expandafter\def\csname res@v6@jitter_0.75_b50@varlingam@rp\endcsname{0.74}
\expandafter\def\csname res@v6@jitter_0.75_b50@varlingam@map\endcsname{0.84}
\expandafter\def\csname res@v6@jitter_0.75_b50@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v6@jitter_0.75_b50@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v6@jitter_0.75_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@spacetime_rule@tt\endcsname{0.27}
\expandafter\def\csname res@v6@jitter_0.75_b50@spacetime_rule@prec\endcsname{0.88}
\expandafter\def\csname res@v6@jitter_0.75_b50@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v6@jitter_0.75_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@spacetime_rule@len\endcsname{0.8}
\expandafter\def\csname res@v6@jitter_0.75_b50@spacetime_rule@rp\endcsname{0.42}
\expandafter\def\csname res@v6@jitter_0.75_b50@spacetime_rule@map\endcsname{0.57}
\expandafter\def\csname res@v6@jitter_0.75_b50@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@jitter_0.75_b50@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@varsort@tt\endcsname{0.08}
\expandafter\def\csname res@v6@jitter_0.75_b50@varsort@prec\endcsname{0.07}
\expandafter\def\csname res@v6@jitter_0.75_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@varsort@bw\endcsname{2}
\expandafter\def\csname res@v6@jitter_0.75_b50@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@jitter_0.75_b50@varsort@rp\endcsname{0.07}
\expandafter\def\csname res@v6@jitter_0.75_b50@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.75_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@jitter_0.75_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@jitter_0.75_b50@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@jitter_0.75_b50@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@jitter_0.75_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@jitter_0.75_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@jitter_0.75_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@jitter_0.75_b50@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v6@jitter_0.75_b50@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@cumul_0.25@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v6@cumul_0.25@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v6@cumul_0.25@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@correlation@tt\endcsname{0.69}
\expandafter\def\csname res@v6@cumul_0.25@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@cumul_0.25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@correlation@bw\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.25@correlation@len\endcsname{18.0}
\expandafter\def\csname res@v6@cumul_0.25@correlation@rp\endcsname{0.76}
\expandafter\def\csname res@v6@cumul_0.25@correlation@map\endcsname{0.82}
\expandafter\def\csname res@v6@cumul_0.25@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_0.25@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@granger@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v6@cumul_0.25@granger@prec\endcsname{0.16}
\expandafter\def\csname res@v6@cumul_0.25@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@granger@len\endcsname{16.0}
\expandafter\def\csname res@v6@cumul_0.25@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v6@cumul_0.25@granger@map\endcsname{0.79}
\expandafter\def\csname res@v6@cumul_0.25@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_0.25@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@pcmciplus@tt\endcsname{0.85}
\expandafter\def\csname res@v6@cumul_0.25@pcmciplus@prec\endcsname{0.93}
\expandafter\def\csname res@v6@cumul_0.25@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@pcmciplus@len\endcsname{2.5}
\expandafter\def\csname res@v6@cumul_0.25@pcmciplus@rp\endcsname{0.93}
\expandafter\def\csname res@v6@cumul_0.25@pcmciplus@map\endcsname{0.94}
\expandafter\def\csname res@v6@cumul_0.25@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@cumul_0.25@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.25@pc@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v6@cumul_0.25@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v6@cumul_0.25@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.25@pc@len\endcsname{5.7}
\expandafter\def\csname res@v6@cumul_0.25@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v6@cumul_0.25@pc@map\endcsname{0.33}
\expandafter\def\csname res@v6@cumul_0.25@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v6@cumul_0.25@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v6@cumul_0.25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@dynotears@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.25@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_0.25@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v6@cumul_0.25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@dynotears@len\endcsname{0.4}
\expandafter\def\csname res@v6@cumul_0.25@dynotears@rp\endcsname{0.83}
\expandafter\def\csname res@v6@cumul_0.25@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v6@cumul_0.25@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.25@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@doubleml@tt\endcsname{0.77}
\expandafter\def\csname res@v6@cumul_0.25@doubleml@prec\endcsname{0.78}
\expandafter\def\csname res@v6@cumul_0.25@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@doubleml@len\endcsname{3.1}
\expandafter\def\csname res@v6@cumul_0.25@doubleml@rp\endcsname{0.90}
\expandafter\def\csname res@v6@cumul_0.25@doubleml@map\endcsname{0.93}
\expandafter\def\csname res@v6@cumul_0.25@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.25@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v6@cumul_0.25@varlingam@prec\endcsname{0.25}
\expandafter\def\csname res@v6@cumul_0.25@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@varlingam@len\endcsname{10.8}
\expandafter\def\csname res@v6@cumul_0.25@varlingam@rp\endcsname{0.73}
\expandafter\def\csname res@v6@cumul_0.25@varlingam@map\endcsname{0.81}
\expandafter\def\csname res@v6@cumul_0.25@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v6@cumul_0.25@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v6@cumul_0.25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@spacetime_rule@tt\endcsname{0.27}
\expandafter\def\csname res@v6@cumul_0.25@spacetime_rule@prec\endcsname{0.88}
\expandafter\def\csname res@v6@cumul_0.25@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@spacetime_rule@len\endcsname{0.8}
\expandafter\def\csname res@v6@cumul_0.25@spacetime_rule@rp\endcsname{0.57}
\expandafter\def\csname res@v6@cumul_0.25@spacetime_rule@map\endcsname{0.67}
\expandafter\def\csname res@v6@cumul_0.25@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@cumul_0.25@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.25@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@cumul_0.25@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@cumul_0.25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.25@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v6@cumul_0.25@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.25@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.25@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@cumul_0.25@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.25@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.25@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@cumul_0.25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.25@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@cumul_0.25@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@cumul_0.25@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@cumul_0.5@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v6@cumul_0.5@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v6@cumul_0.5@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@correlation@tt\endcsname{0.69}
\expandafter\def\csname res@v6@cumul_0.5@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@cumul_0.5@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@correlation@bw\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.5@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v6@cumul_0.5@correlation@rp\endcsname{0.76}
\expandafter\def\csname res@v6@cumul_0.5@correlation@map\endcsname{0.82}
\expandafter\def\csname res@v6@cumul_0.5@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_0.5@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@granger@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@granger@tt\endcsname{0.69}
\expandafter\def\csname res@v6@cumul_0.5@granger@prec\endcsname{0.16}
\expandafter\def\csname res@v6@cumul_0.5@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@granger@len\endcsname{16.0}
\expandafter\def\csname res@v6@cumul_0.5@granger@rp\endcsname{0.76}
\expandafter\def\csname res@v6@cumul_0.5@granger@map\endcsname{0.82}
\expandafter\def\csname res@v6@cumul_0.5@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_0.5@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@pcmciplus@tt\endcsname{0.77}
\expandafter\def\csname res@v6@cumul_0.5@pcmciplus@prec\endcsname{0.93}
\expandafter\def\csname res@v6@cumul_0.5@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@pcmciplus@len\endcsname{2.3}
\expandafter\def\csname res@v6@cumul_0.5@pcmciplus@rp\endcsname{0.91}
\expandafter\def\csname res@v6@cumul_0.5@pcmciplus@map\endcsname{0.94}
\expandafter\def\csname res@v6@cumul_0.5@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@cumul_0.5@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.5@pc@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@cumul_0.5@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v6@cumul_0.5@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.5@pc@len\endcsname{5.8}
\expandafter\def\csname res@v6@cumul_0.5@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v6@cumul_0.5@pc@map\endcsname{0.32}
\expandafter\def\csname res@v6@cumul_0.5@dynotears@fp\endcsname{5/10}
\expandafter\def\csname res@v6@cumul_0.5@dynotears@fpn\endcsname{5}
\expandafter\def\csname res@v6@cumul_0.5@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@dynotears@tt\endcsname{0.19}
\expandafter\def\csname res@v6@cumul_0.5@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_0.5@dynotears@ab\endcsname{5}
\expandafter\def\csname res@v6@cumul_0.5@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@dynotears@len\endcsname{0.5}
\expandafter\def\csname res@v6@cumul_0.5@dynotears@rp\endcsname{0.83}
\expandafter\def\csname res@v6@cumul_0.5@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v6@cumul_0.5@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.5@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.5@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@doubleml@tt\endcsname{0.77}
\expandafter\def\csname res@v6@cumul_0.5@doubleml@prec\endcsname{0.80}
\expandafter\def\csname res@v6@cumul_0.5@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.5@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@doubleml@len\endcsname{2.8}
\expandafter\def\csname res@v6@cumul_0.5@doubleml@rp\endcsname{0.90}
\expandafter\def\csname res@v6@cumul_0.5@doubleml@map\endcsname{0.93}
\expandafter\def\csname res@v6@cumul_0.5@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.5@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.5@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v6@cumul_0.5@varlingam@prec\endcsname{0.23}
\expandafter\def\csname res@v6@cumul_0.5@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@varlingam@len\endcsname{11.3}
\expandafter\def\csname res@v6@cumul_0.5@varlingam@rp\endcsname{0.73}
\expandafter\def\csname res@v6@cumul_0.5@varlingam@map\endcsname{0.78}
\expandafter\def\csname res@v6@cumul_0.5@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v6@cumul_0.5@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v6@cumul_0.5@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@spacetime_rule@tt\endcsname{0.23}
\expandafter\def\csname res@v6@cumul_0.5@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_0.5@spacetime_rule@ab\endcsname{4}
\expandafter\def\csname res@v6@cumul_0.5@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@spacetime_rule@len\endcsname{0.6}
\expandafter\def\csname res@v6@cumul_0.5@spacetime_rule@rp\endcsname{0.57}
\expandafter\def\csname res@v6@cumul_0.5@spacetime_rule@map\endcsname{0.65}
\expandafter\def\csname res@v6@cumul_0.5@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@cumul_0.5@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.5@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.5@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@cumul_0.5@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.5@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@cumul_0.5@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.5@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v6@cumul_0.5@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@cumul_0.5@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.5@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.5@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@cumul_0.5@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.5@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.5@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@cumul_0.5@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@cumul_0.5@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@cumul_0.75@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.75@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.75@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@correlation@tt\endcsname{0.69}
\expandafter\def\csname res@v6@cumul_0.75@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@cumul_0.75@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@correlation@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75@correlation@len\endcsname{18.6}
\expandafter\def\csname res@v6@cumul_0.75@correlation@rp\endcsname{0.76}
\expandafter\def\csname res@v6@cumul_0.75@correlation@map\endcsname{0.84}
\expandafter\def\csname res@v6@cumul_0.75@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_0.75@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@granger@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@granger@tt\endcsname{0.73}
\expandafter\def\csname res@v6@cumul_0.75@granger@prec\endcsname{0.16}
\expandafter\def\csname res@v6@cumul_0.75@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@granger@len\endcsname{16.7}
\expandafter\def\csname res@v6@cumul_0.75@granger@rp\endcsname{0.78}
\expandafter\def\csname res@v6@cumul_0.75@granger@map\endcsname{0.88}
\expandafter\def\csname res@v6@cumul_0.75@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.75@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.75@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v6@cumul_0.75@pcmciplus@prec\endcsname{0.73}
\expandafter\def\csname res@v6@cumul_0.75@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@pcmciplus@len\endcsname{2.7}
\expandafter\def\csname res@v6@cumul_0.75@pcmciplus@rp\endcsname{0.83}
\expandafter\def\csname res@v6@cumul_0.75@pcmciplus@map\endcsname{0.90}
\expandafter\def\csname res@v6@cumul_0.75@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v6@cumul_0.75@pc@fpn\endcsname{4}
\expandafter\def\csname res@v6@cumul_0.75@pc@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v6@cumul_0.75@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v6@cumul_0.75@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.75@pc@len\endcsname{5.8}
\expandafter\def\csname res@v6@cumul_0.75@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v6@cumul_0.75@pc@map\endcsname{0.32}
\expandafter\def\csname res@v6@cumul_0.75@dynotears@fp\endcsname{5/10}
\expandafter\def\csname res@v6@cumul_0.75@dynotears@fpn\endcsname{5}
\expandafter\def\csname res@v6@cumul_0.75@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@dynotears@tt\endcsname{0.19}
\expandafter\def\csname res@v6@cumul_0.75@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_0.75@dynotears@ab\endcsname{5}
\expandafter\def\csname res@v6@cumul_0.75@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@dynotears@len\endcsname{0.5}
\expandafter\def\csname res@v6@cumul_0.75@dynotears@rp\endcsname{0.95}
\expandafter\def\csname res@v6@cumul_0.75@dynotears@map\endcsname{0.96}
\expandafter\def\csname res@v6@cumul_0.75@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.75@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.75@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@doubleml@tt\endcsname{0.69}
\expandafter\def\csname res@v6@cumul_0.75@doubleml@prec\endcsname{0.84}
\expandafter\def\csname res@v6@cumul_0.75@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@doubleml@len\endcsname{2.4}
\expandafter\def\csname res@v6@cumul_0.75@doubleml@rp\endcsname{0.85}
\expandafter\def\csname res@v6@cumul_0.75@doubleml@map\endcsname{0.89}
\expandafter\def\csname res@v6@cumul_0.75@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.75@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.75@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@varlingam@tt\endcsname{0.81}
\expandafter\def\csname res@v6@cumul_0.75@varlingam@prec\endcsname{0.31}
\expandafter\def\csname res@v6@cumul_0.75@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@varlingam@len\endcsname{9.8}
\expandafter\def\csname res@v6@cumul_0.75@varlingam@rp\endcsname{0.74}
\expandafter\def\csname res@v6@cumul_0.75@varlingam@map\endcsname{0.85}
\expandafter\def\csname res@v6@cumul_0.75@spacetime_rule@fp\endcsname{4/10}
\expandafter\def\csname res@v6@cumul_0.75@spacetime_rule@fpn\endcsname{4}
\expandafter\def\csname res@v6@cumul_0.75@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@spacetime_rule@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.75@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_0.75@spacetime_rule@ab\endcsname{6}
\expandafter\def\csname res@v6@cumul_0.75@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@spacetime_rule@len\endcsname{0.4}
\expandafter\def\csname res@v6@cumul_0.75@spacetime_rule@rp\endcsname{0.42}
\expandafter\def\csname res@v6@cumul_0.75@spacetime_rule@map\endcsname{0.57}
\expandafter\def\csname res@v6@cumul_0.75@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@cumul_0.75@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@cumul_0.75@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@cumul_0.75@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@cumul_0.75@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.75@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v6@cumul_0.75@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@cumul_0.75@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.75@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@cumul_0.75@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@cumul_0.75@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@cumul_0.75@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@cumul_1.0@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_1.0@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_1.0@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@correlation@tt\endcsname{0.65}
\expandafter\def\csname res@v6@cumul_1.0@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@cumul_1.0@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@correlation@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_1.0@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v6@cumul_1.0@correlation@rp\endcsname{0.70}
\expandafter\def\csname res@v6@cumul_1.0@correlation@map\endcsname{0.82}
\expandafter\def\csname res@v6@cumul_1.0@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_1.0@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@granger@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@granger@tt\endcsname{0.77}
\expandafter\def\csname res@v6@cumul_1.0@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_1.0@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@granger@len\endcsname{17.3}
\expandafter\def\csname res@v6@cumul_1.0@granger@rp\endcsname{0.83}
\expandafter\def\csname res@v6@cumul_1.0@granger@map\endcsname{0.90}
\expandafter\def\csname res@v6@cumul_1.0@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_1.0@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@pcmciplus@tt\endcsname{0.92}
\expandafter\def\csname res@v6@cumul_1.0@pcmciplus@prec\endcsname{0.82}
\expandafter\def\csname res@v6@cumul_1.0@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@pcmciplus@len\endcsname{3.2}
\expandafter\def\csname res@v6@cumul_1.0@pcmciplus@rp\endcsname{0.97}
\expandafter\def\csname res@v6@cumul_1.0@pcmciplus@map\endcsname{0.99}
\expandafter\def\csname res@v6@cumul_1.0@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v6@cumul_1.0@pc@fpn\endcsname{4}
\expandafter\def\csname res@v6@cumul_1.0@pc@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@cumul_1.0@pc@prec\endcsname{0.33}
\expandafter\def\csname res@v6@cumul_1.0@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@cumul_1.0@pc@len\endcsname{5.5}
\expandafter\def\csname res@v6@cumul_1.0@pc@rp\endcsname{0.33}
\expandafter\def\csname res@v6@cumul_1.0@pc@map\endcsname{0.29}
\expandafter\def\csname res@v6@cumul_1.0@dynotears@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_1.0@dynotears@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_1.0@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@dynotears@tt\endcsname{0.46}
\expandafter\def\csname res@v6@cumul_1.0@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_1.0@dynotears@ab\endcsname{1}
\expandafter\def\csname res@v6@cumul_1.0@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@dynotears@len\endcsname{1.2}
\expandafter\def\csname res@v6@cumul_1.0@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v6@cumul_1.0@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v6@cumul_1.0@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_1.0@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@doubleml@tt\endcsname{0.77}
\expandafter\def\csname res@v6@cumul_1.0@doubleml@prec\endcsname{0.82}
\expandafter\def\csname res@v6@cumul_1.0@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@doubleml@len\endcsname{2.7}
\expandafter\def\csname res@v6@cumul_1.0@doubleml@rp\endcsname{0.82}
\expandafter\def\csname res@v6@cumul_1.0@doubleml@map\endcsname{0.89}
\expandafter\def\csname res@v6@cumul_1.0@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_1.0@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v6@cumul_1.0@varlingam@prec\endcsname{0.33}
\expandafter\def\csname res@v6@cumul_1.0@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@varlingam@len\endcsname{7.9}
\expandafter\def\csname res@v6@cumul_1.0@varlingam@rp\endcsname{0.84}
\expandafter\def\csname res@v6@cumul_1.0@varlingam@map\endcsname{0.91}
\expandafter\def\csname res@v6@cumul_1.0@spacetime_rule@fp\endcsname{5/10}
\expandafter\def\csname res@v6@cumul_1.0@spacetime_rule@fpn\endcsname{5}
\expandafter\def\csname res@v6@cumul_1.0@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@spacetime_rule@tt\endcsname{0.19}
\expandafter\def\csname res@v6@cumul_1.0@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_1.0@spacetime_rule@ab\endcsname{5}
\expandafter\def\csname res@v6@cumul_1.0@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@spacetime_rule@len\endcsname{0.5}
\expandafter\def\csname res@v6@cumul_1.0@spacetime_rule@rp\endcsname{0.50}
\expandafter\def\csname res@v6@cumul_1.0@spacetime_rule@map\endcsname{0.66}
\expandafter\def\csname res@v6@cumul_1.0@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@cumul_1.0@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@cumul_1.0@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@cumul_1.0@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@cumul_1.0@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@cumul_1.0@varsort@rp\endcsname{0.16}
\expandafter\def\csname res@v6@cumul_1.0@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v6@cumul_1.0@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@cumul_1.0@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_1.0@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_1.0@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@cumul_1.0@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_1.0@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_1.0@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@cumul_1.0@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@cumul_1.0@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@correlation@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@correlation@prec\endcsname{0.17}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@correlation@bw\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@correlation@len\endcsname{7.1}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@correlation@rp\endcsname{0.03}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@correlation@map\endcsname{0.29}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@granger@fp\endcsname{7/10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@granger@fpn\endcsname{7}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@granger@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@granger@tt\endcsname{0.38}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@granger@prec\endcsname{0.48}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@granger@ab\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@granger@len\endcsname{4.7}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@granger@rp\endcsname{0.54}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@granger@map\endcsname{0.64}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pcmciplus@fp\endcsname{6/10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pcmciplus@fpn\endcsname{6}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pcmciplus@tt\endcsname{0.35}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pcmciplus@prec\endcsname{0.60}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pcmciplus@len\endcsname{1.4}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pcmciplus@rp\endcsname{0.40}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pcmciplus@map\endcsname{0.58}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pc@fpn\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pc@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pc@tt\endcsname{0.08}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pc@prec\endcsname{0.09}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pc@bw\endcsname{7}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pc@len\endcsname{3.1}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pc@rp\endcsname{0.11}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@pc@map\endcsname{0.18}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@dynotears@rp\endcsname{0.61}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@dynotears@map\endcsname{0.71}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@doubleml@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@doubleml@ab\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@doubleml@len\endcsname{0.1}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@doubleml@rp\endcsname{0.27}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@doubleml@map\endcsname{0.39}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varlingam@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varlingam@prec\endcsname{0.20}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varlingam@bw\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varlingam@len\endcsname{6.8}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varlingam@rp\endcsname{0.13}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varlingam@map\endcsname{0.22}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@spacetime_rule@fp\endcsname{3/10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@spacetime_rule@fpn\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@spacetime_rule@tt\endcsname{0.12}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@spacetime_rule@prec\endcsname{0.31}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@spacetime_rule@ab\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@spacetime_rule@len\endcsname{0.9}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@spacetime_rule@rp\endcsname{0.26}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@spacetime_rule@map\endcsname{0.41}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@varsort@map\endcsname{0.22}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@cumul_0.75_combo_interaction@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v6@cumul_0.75_s40@correlation@fp\endcsname{7/10}
\expandafter\def\csname res@v6@cumul_0.75_s40@correlation@fpn\endcsname{7}
\expandafter\def\csname res@v6@cumul_0.75_s40@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@correlation@tt\endcsname{0.50}
\expandafter\def\csname res@v6@cumul_0.75_s40@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v6@cumul_0.75_s40@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@correlation@bw\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.75_s40@correlation@len\endcsname{35.8}
\expandafter\def\csname res@v6@cumul_0.75_s40@correlation@rp\endcsname{0.51}
\expandafter\def\csname res@v6@cumul_0.75_s40@correlation@map\endcsname{0.62}
\expandafter\def\csname res@v6@cumul_0.75_s40@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_0.75_s40@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@granger@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v6@cumul_0.75_s40@granger@prec\endcsname{0.10}
\expandafter\def\csname res@v6@cumul_0.75_s40@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@granger@len\endcsname{29.4}
\expandafter\def\csname res@v6@cumul_0.75_s40@granger@rp\endcsname{0.64}
\expandafter\def\csname res@v6@cumul_0.75_s40@granger@map\endcsname{0.72}
\expandafter\def\csname res@v6@cumul_0.75_s40@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@cumul_0.75_s40@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@pcmciplus@tt\endcsname{0.77}
\expandafter\def\csname res@v6@cumul_0.75_s40@pcmciplus@prec\endcsname{0.73}
\expandafter\def\csname res@v6@cumul_0.75_s40@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@pcmciplus@len\endcsname{3.0}
\expandafter\def\csname res@v6@cumul_0.75_s40@pcmciplus@rp\endcsname{0.85}
\expandafter\def\csname res@v6@cumul_0.75_s40@pcmciplus@map\endcsname{0.89}
\expandafter\def\csname res@v6@cumul_0.75_s40@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@cumul_0.75_s40@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.75_s40@pc@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@cumul_0.75_s40@pc@prec\endcsname{0.24}
\expandafter\def\csname res@v6@cumul_0.75_s40@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.75_s40@pc@len\endcsname{6.0}
\expandafter\def\csname res@v6@cumul_0.75_s40@pc@rp\endcsname{0.22}
\expandafter\def\csname res@v6@cumul_0.75_s40@pc@map\endcsname{0.19}
\expandafter\def\csname res@v6@cumul_0.75_s40@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v6@cumul_0.75_s40@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v6@cumul_0.75_s40@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@dynotears@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.75_s40@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_0.75_s40@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v6@cumul_0.75_s40@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@dynotears@len\endcsname{0.4}
\expandafter\def\csname res@v6@cumul_0.75_s40@dynotears@rp\endcsname{0.91}
\expandafter\def\csname res@v6@cumul_0.75_s40@dynotears@map\endcsname{0.96}
\expandafter\def\csname res@v6@cumul_0.75_s40@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.75_s40@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.75_s40@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@doubleml@tt\endcsname{0.62}
\expandafter\def\csname res@v6@cumul_0.75_s40@doubleml@prec\endcsname{0.88}
\expandafter\def\csname res@v6@cumul_0.75_s40@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75_s40@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@doubleml@len\endcsname{2.0}
\expandafter\def\csname res@v6@cumul_0.75_s40@doubleml@rp\endcsname{0.69}
\expandafter\def\csname res@v6@cumul_0.75_s40@doubleml@map\endcsname{0.77}
\expandafter\def\csname res@v6@cumul_0.75_s40@varlingam@fp\endcsname{6/10}
\expandafter\def\csname res@v6@cumul_0.75_s40@varlingam@fpn\endcsname{6}
\expandafter\def\csname res@v6@cumul_0.75_s40@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@varlingam@tt\endcsname{0.54}
\expandafter\def\csname res@v6@cumul_0.75_s40@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v6@cumul_0.75_s40@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@varlingam@bw\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.75_s40@varlingam@len\endcsname{11.7}
\expandafter\def\csname res@v6@cumul_0.75_s40@varlingam@rp\endcsname{0.63}
\expandafter\def\csname res@v6@cumul_0.75_s40@varlingam@map\endcsname{0.69}
\expandafter\def\csname res@v6@cumul_0.75_s40@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v6@cumul_0.75_s40@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v6@cumul_0.75_s40@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@spacetime_rule@tt\endcsname{0.23}
\expandafter\def\csname res@v6@cumul_0.75_s40@spacetime_rule@prec\endcsname{0.86}
\expandafter\def\csname res@v6@cumul_0.75_s40@spacetime_rule@ab\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.75_s40@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@spacetime_rule@len\endcsname{0.7}
\expandafter\def\csname res@v6@cumul_0.75_s40@spacetime_rule@rp\endcsname{0.38}
\expandafter\def\csname res@v6@cumul_0.75_s40@spacetime_rule@map\endcsname{0.49}
\expandafter\def\csname res@v6@cumul_0.75_s40@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@cumul_0.75_s40@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v6@cumul_0.75_s40@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v6@cumul_0.75_s40@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@varsort@bw\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.75_s40@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@cumul_0.75_s40@varsort@rp\endcsname{0.05}
\expandafter\def\csname res@v6@cumul_0.75_s40@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v6@cumul_0.75_s40@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@cumul_0.75_s40@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_s40@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v6@cumul_0.75_s40@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v6@cumul_0.75_s40@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_s40@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@cumul_0.75_s40@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v6@cumul_0.75_s40@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v6@cumul_0.75_b50@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v6@cumul_0.75_b50@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v6@cumul_0.75_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_b50@correlation@tt\endcsname{0.69}
\expandafter\def\csname res@v6@cumul_0.75_b50@correlation@prec\endcsname{0.18}
\expandafter\def\csname res@v6@cumul_0.75_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@correlation@bw\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.75_b50@correlation@len\endcsname{14.4}
\expandafter\def\csname res@v6@cumul_0.75_b50@correlation@rp\endcsname{0.73}
\expandafter\def\csname res@v6@cumul_0.75_b50@correlation@map\endcsname{0.81}
\expandafter\def\csname res@v6@cumul_0.75_b50@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.75_b50@granger@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.75_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_b50@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v6@cumul_0.75_b50@granger@prec\endcsname{0.28}
\expandafter\def\csname res@v6@cumul_0.75_b50@granger@ab\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@granger@len\endcsname{9.6}
\expandafter\def\csname res@v6@cumul_0.75_b50@granger@rp\endcsname{0.60}
\expandafter\def\csname res@v6@cumul_0.75_b50@granger@map\endcsname{0.75}
\expandafter\def\csname res@v6@cumul_0.75_b50@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.75_b50@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.75_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_b50@pcmciplus@tt\endcsname{0.65}
\expandafter\def\csname res@v6@cumul_0.75_b50@pcmciplus@prec\endcsname{0.86}
\expandafter\def\csname res@v6@cumul_0.75_b50@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@pcmciplus@len\endcsname{2.0}
\expandafter\def\csname res@v6@cumul_0.75_b50@pcmciplus@rp\endcsname{0.89}
\expandafter\def\csname res@v6@cumul_0.75_b50@pcmciplus@map\endcsname{0.92}
\expandafter\def\csname res@v6@cumul_0.75_b50@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v6@cumul_0.75_b50@pc@fpn\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.75_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_b50@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v6@cumul_0.75_b50@pc@prec\endcsname{0.34}
\expandafter\def\csname res@v6@cumul_0.75_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@cumul_0.75_b50@pc@len\endcsname{4.7}
\expandafter\def\csname res@v6@cumul_0.75_b50@pc@rp\endcsname{0.34}
\expandafter\def\csname res@v6@cumul_0.75_b50@pc@map\endcsname{0.32}
\expandafter\def\csname res@v6@cumul_0.75_b50@dynotears@fp\endcsname{5/10}
\expandafter\def\csname res@v6@cumul_0.75_b50@dynotears@fpn\endcsname{5}
\expandafter\def\csname res@v6@cumul_0.75_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_b50@dynotears@tt\endcsname{0.23}
\expandafter\def\csname res@v6@cumul_0.75_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_0.75_b50@dynotears@ab\endcsname{5}
\expandafter\def\csname res@v6@cumul_0.75_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@dynotears@len\endcsname{0.6}
\expandafter\def\csname res@v6@cumul_0.75_b50@dynotears@rp\endcsname{0.88}
\expandafter\def\csname res@v6@cumul_0.75_b50@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v6@cumul_0.75_b50@doubleml@fp\endcsname{6/10}
\expandafter\def\csname res@v6@cumul_0.75_b50@doubleml@fpn\endcsname{6}
\expandafter\def\csname res@v6@cumul_0.75_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_b50@doubleml@tt\endcsname{0.58}
\expandafter\def\csname res@v6@cumul_0.75_b50@doubleml@prec\endcsname{0.79}
\expandafter\def\csname res@v6@cumul_0.75_b50@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75_b50@doubleml@bw\endcsname{2}
\expandafter\def\csname res@v6@cumul_0.75_b50@doubleml@len\endcsname{2.3}
\expandafter\def\csname res@v6@cumul_0.75_b50@doubleml@rp\endcsname{0.57}
\expandafter\def\csname res@v6@cumul_0.75_b50@doubleml@map\endcsname{0.70}
\expandafter\def\csname res@v6@cumul_0.75_b50@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@cumul_0.75_b50@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@cumul_0.75_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_b50@varlingam@tt\endcsname{0.62}
\expandafter\def\csname res@v6@cumul_0.75_b50@varlingam@prec\endcsname{0.34}
\expandafter\def\csname res@v6@cumul_0.75_b50@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@varlingam@len\endcsname{6.9}
\expandafter\def\csname res@v6@cumul_0.75_b50@varlingam@rp\endcsname{0.68}
\expandafter\def\csname res@v6@cumul_0.75_b50@varlingam@map\endcsname{0.76}
\expandafter\def\csname res@v6@cumul_0.75_b50@spacetime_rule@fp\endcsname{5/10}
\expandafter\def\csname res@v6@cumul_0.75_b50@spacetime_rule@fpn\endcsname{5}
\expandafter\def\csname res@v6@cumul_0.75_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_b50@spacetime_rule@tt\endcsname{0.19}
\expandafter\def\csname res@v6@cumul_0.75_b50@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v6@cumul_0.75_b50@spacetime_rule@ab\endcsname{5}
\expandafter\def\csname res@v6@cumul_0.75_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@spacetime_rule@len\endcsname{0.5}
\expandafter\def\csname res@v6@cumul_0.75_b50@spacetime_rule@rp\endcsname{0.46}
\expandafter\def\csname res@v6@cumul_0.75_b50@spacetime_rule@map\endcsname{0.56}
\expandafter\def\csname res@v6@cumul_0.75_b50@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@cumul_0.75_b50@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_b50@varsort@tt\endcsname{0.08}
\expandafter\def\csname res@v6@cumul_0.75_b50@varsort@prec\endcsname{0.07}
\expandafter\def\csname res@v6@cumul_0.75_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75_b50@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@cumul_0.75_b50@varsort@rp\endcsname{0.06}
\expandafter\def\csname res@v6@cumul_0.75_b50@varsort@map\endcsname{0.14}
\expandafter\def\csname res@v6@cumul_0.75_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@cumul_0.75_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@cumul_0.75_b50@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@cumul_0.75_b50@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@cumul_0.75_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@cumul_0.75_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@cumul_0.75_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@cumul_0.75_b50@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v6@cumul_0.75_b50@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@operator_0.1@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.1@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.1@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@correlation@tt\endcsname{0.65}
\expandafter\def\csname res@v6@operator_0.1@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@operator_0.1@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@correlation@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.1@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v6@operator_0.1@correlation@rp\endcsname{0.71}
\expandafter\def\csname res@v6@operator_0.1@correlation@map\endcsname{0.81}
\expandafter\def\csname res@v6@operator_0.1@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.1@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@granger@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v6@operator_0.1@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v6@operator_0.1@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@granger@len\endcsname{17.3}
\expandafter\def\csname res@v6@operator_0.1@granger@rp\endcsname{0.73}
\expandafter\def\csname res@v6@operator_0.1@granger@map\endcsname{0.80}
\expandafter\def\csname res@v6@operator_0.1@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.1@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.1@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@pcmciplus@tt\endcsname{0.77}
\expandafter\def\csname res@v6@operator_0.1@pcmciplus@prec\endcsname{0.79}
\expandafter\def\csname res@v6@operator_0.1@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@pcmciplus@len\endcsname{2.7}
\expandafter\def\csname res@v6@operator_0.1@pcmciplus@rp\endcsname{0.95}
\expandafter\def\csname res@v6@operator_0.1@pcmciplus@map\endcsname{0.99}
\expandafter\def\csname res@v6@operator_0.1@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@operator_0.1@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@operator_0.1@pc@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@operator_0.1@pc@prec\endcsname{0.37}
\expandafter\def\csname res@v6@operator_0.1@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@pc@bw\endcsname{4}
\expandafter\def\csname res@v6@operator_0.1@pc@len\endcsname{5.5}
\expandafter\def\csname res@v6@operator_0.1@pc@rp\endcsname{0.37}
\expandafter\def\csname res@v6@operator_0.1@pc@map\endcsname{0.32}
\expandafter\def\csname res@v6@operator_0.1@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v6@operator_0.1@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v6@operator_0.1@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@dynotears@tt\endcsname{0.31}
\expandafter\def\csname res@v6@operator_0.1@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@operator_0.1@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v6@operator_0.1@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@dynotears@len\endcsname{0.8}
\expandafter\def\csname res@v6@operator_0.1@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v6@operator_0.1@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v6@operator_0.1@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.1@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v6@operator_0.1@doubleml@prec\endcsname{0.80}
\expandafter\def\csname res@v6@operator_0.1@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@doubleml@len\endcsname{3.4}
\expandafter\def\csname res@v6@operator_0.1@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v6@operator_0.1@doubleml@map\endcsname{0.94}
\expandafter\def\csname res@v6@operator_0.1@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.1@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v6@operator_0.1@varlingam@prec\endcsname{0.27}
\expandafter\def\csname res@v6@operator_0.1@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@varlingam@len\endcsname{10.0}
\expandafter\def\csname res@v6@operator_0.1@varlingam@rp\endcsname{0.68}
\expandafter\def\csname res@v6@operator_0.1@varlingam@map\endcsname{0.82}
\expandafter\def\csname res@v6@operator_0.1@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.1@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.1@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@spacetime_rule@tt\endcsname{0.50}
\expandafter\def\csname res@v6@operator_0.1@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v6@operator_0.1@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.1@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v6@operator_0.1@spacetime_rule@rp\endcsname{0.83}
\expandafter\def\csname res@v6@operator_0.1@spacetime_rule@map\endcsname{0.87}
\expandafter\def\csname res@v6@operator_0.1@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@operator_0.1@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.1@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.1@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.1@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@operator_0.1@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v6@operator_0.1@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.1@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.1@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.1@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.1@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.1@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.1@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.1@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.1@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@operator_0.1@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v6@operator_0.1@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@operator_0.2@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.2@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.2@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@correlation@tt\endcsname{0.73}
\expandafter\def\csname res@v6@operator_0.2@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@operator_0.2@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@correlation@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.2@correlation@len\endcsname{18.4}
\expandafter\def\csname res@v6@operator_0.2@correlation@rp\endcsname{0.73}
\expandafter\def\csname res@v6@operator_0.2@correlation@map\endcsname{0.84}
\expandafter\def\csname res@v6@operator_0.2@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.2@granger@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.2@granger@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v6@operator_0.2@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v6@operator_0.2@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@granger@len\endcsname{17.2}
\expandafter\def\csname res@v6@operator_0.2@granger@rp\endcsname{0.73}
\expandafter\def\csname res@v6@operator_0.2@granger@map\endcsname{0.78}
\expandafter\def\csname res@v6@operator_0.2@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.2@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@pcmciplus@tt\endcsname{0.81}
\expandafter\def\csname res@v6@operator_0.2@pcmciplus@prec\endcsname{0.75}
\expandafter\def\csname res@v6@operator_0.2@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@pcmciplus@len\endcsname{2.9}
\expandafter\def\csname res@v6@operator_0.2@pcmciplus@rp\endcsname{0.95}
\expandafter\def\csname res@v6@operator_0.2@pcmciplus@map\endcsname{0.97}
\expandafter\def\csname res@v6@operator_0.2@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@operator_0.2@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@operator_0.2@pc@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@operator_0.2@pc@prec\endcsname{0.38}
\expandafter\def\csname res@v6@operator_0.2@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@pc@bw\endcsname{4}
\expandafter\def\csname res@v6@operator_0.2@pc@len\endcsname{5.6}
\expandafter\def\csname res@v6@operator_0.2@pc@rp\endcsname{0.38}
\expandafter\def\csname res@v6@operator_0.2@pc@map\endcsname{0.34}
\expandafter\def\csname res@v6@operator_0.2@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v6@operator_0.2@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v6@operator_0.2@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@dynotears@tt\endcsname{0.31}
\expandafter\def\csname res@v6@operator_0.2@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@operator_0.2@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v6@operator_0.2@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@dynotears@len\endcsname{0.8}
\expandafter\def\csname res@v6@operator_0.2@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v6@operator_0.2@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v6@operator_0.2@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.2@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v6@operator_0.2@doubleml@prec\endcsname{0.79}
\expandafter\def\csname res@v6@operator_0.2@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@doubleml@len\endcsname{3.5}
\expandafter\def\csname res@v6@operator_0.2@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v6@operator_0.2@doubleml@map\endcsname{0.94}
\expandafter\def\csname res@v6@operator_0.2@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.2@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.2@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v6@operator_0.2@varlingam@prec\endcsname{0.28}
\expandafter\def\csname res@v6@operator_0.2@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.2@varlingam@len\endcsname{9.2}
\expandafter\def\csname res@v6@operator_0.2@varlingam@rp\endcsname{0.76}
\expandafter\def\csname res@v6@operator_0.2@varlingam@map\endcsname{0.83}
\expandafter\def\csname res@v6@operator_0.2@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.2@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.2@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@spacetime_rule@tt\endcsname{0.50}
\expandafter\def\csname res@v6@operator_0.2@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v6@operator_0.2@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.2@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v6@operator_0.2@spacetime_rule@rp\endcsname{0.83}
\expandafter\def\csname res@v6@operator_0.2@spacetime_rule@map\endcsname{0.87}
\expandafter\def\csname res@v6@operator_0.2@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@operator_0.2@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.2@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.2@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@varsort@bw\endcsname{2}
\expandafter\def\csname res@v6@operator_0.2@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@operator_0.2@varsort@rp\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.2@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.2@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.2@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.2@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.2@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.2@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.2@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.2@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.2@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@operator_0.2@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v6@operator_0.2@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@operator_0.3@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.3@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@correlation@tt\endcsname{0.77}
\expandafter\def\csname res@v6@operator_0.3@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@operator_0.3@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v6@operator_0.3@correlation@rp\endcsname{0.77}
\expandafter\def\csname res@v6@operator_0.3@correlation@map\endcsname{0.87}
\expandafter\def\csname res@v6@operator_0.3@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.3@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@granger@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@granger@tt\endcsname{0.69}
\expandafter\def\csname res@v6@operator_0.3@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v6@operator_0.3@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@granger@len\endcsname{17.2}
\expandafter\def\csname res@v6@operator_0.3@granger@rp\endcsname{0.73}
\expandafter\def\csname res@v6@operator_0.3@granger@map\endcsname{0.80}
\expandafter\def\csname res@v6@operator_0.3@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.3@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.3@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v6@operator_0.3@pcmciplus@prec\endcsname{0.75}
\expandafter\def\csname res@v6@operator_0.3@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@pcmciplus@len\endcsname{2.7}
\expandafter\def\csname res@v6@operator_0.3@pcmciplus@rp\endcsname{0.97}
\expandafter\def\csname res@v6@operator_0.3@pcmciplus@map\endcsname{0.98}
\expandafter\def\csname res@v6@operator_0.3@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@operator_0.3@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@operator_0.3@pc@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v6@operator_0.3@pc@prec\endcsname{0.36}
\expandafter\def\csname res@v6@operator_0.3@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@pc@bw\endcsname{4}
\expandafter\def\csname res@v6@operator_0.3@pc@len\endcsname{5.6}
\expandafter\def\csname res@v6@operator_0.3@pc@rp\endcsname{0.36}
\expandafter\def\csname res@v6@operator_0.3@pc@map\endcsname{0.31}
\expandafter\def\csname res@v6@operator_0.3@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v6@operator_0.3@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v6@operator_0.3@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@dynotears@tt\endcsname{0.31}
\expandafter\def\csname res@v6@operator_0.3@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@operator_0.3@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v6@operator_0.3@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@dynotears@len\endcsname{0.8}
\expandafter\def\csname res@v6@operator_0.3@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v6@operator_0.3@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v6@operator_0.3@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.3@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@doubleml@tt\endcsname{0.88}
\expandafter\def\csname res@v6@operator_0.3@doubleml@prec\endcsname{0.77}
\expandafter\def\csname res@v6@operator_0.3@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@doubleml@len\endcsname{3.7}
\expandafter\def\csname res@v6@operator_0.3@doubleml@rp\endcsname{0.95}
\expandafter\def\csname res@v6@operator_0.3@doubleml@map\endcsname{0.96}
\expandafter\def\csname res@v6@operator_0.3@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.3@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.3@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v6@operator_0.3@varlingam@prec\endcsname{0.31}
\expandafter\def\csname res@v6@operator_0.3@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3@varlingam@len\endcsname{8.7}
\expandafter\def\csname res@v6@operator_0.3@varlingam@rp\endcsname{0.73}
\expandafter\def\csname res@v6@operator_0.3@varlingam@map\endcsname{0.80}
\expandafter\def\csname res@v6@operator_0.3@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.3@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.3@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@spacetime_rule@tt\endcsname{0.50}
\expandafter\def\csname res@v6@operator_0.3@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v6@operator_0.3@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v6@operator_0.3@spacetime_rule@rp\endcsname{0.83}
\expandafter\def\csname res@v6@operator_0.3@spacetime_rule@map\endcsname{0.86}
\expandafter\def\csname res@v6@operator_0.3@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.3@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.3@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.3@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@varsort@bw\endcsname{2}
\expandafter\def\csname res@v6@operator_0.3@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v6@operator_0.3@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v6@operator_0.3@varsort@map\endcsname{0.22}
\expandafter\def\csname res@v6@operator_0.3@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.3@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.3@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.3@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@operator_0.3@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v6@operator_0.3@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@operator_0.5@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.5@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@correlation@tt\endcsname{0.77}
\expandafter\def\csname res@v6@operator_0.5@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v6@operator_0.5@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@correlation@len\endcsname{18.4}
\expandafter\def\csname res@v6@operator_0.5@correlation@rp\endcsname{0.77}
\expandafter\def\csname res@v6@operator_0.5@correlation@map\endcsname{0.86}
\expandafter\def\csname res@v6@operator_0.5@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.5@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@granger@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v6@operator_0.5@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v6@operator_0.5@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@granger@len\endcsname{17.2}
\expandafter\def\csname res@v6@operator_0.5@granger@rp\endcsname{0.70}
\expandafter\def\csname res@v6@operator_0.5@granger@map\endcsname{0.79}
\expandafter\def\csname res@v6@operator_0.5@pcmciplus@fp\endcsname{8/10}
\expandafter\def\csname res@v6@operator_0.5@pcmciplus@fpn\endcsname{8}
\expandafter\def\csname res@v6@operator_0.5@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v6@operator_0.5@pcmciplus@prec\endcsname{0.75}
\expandafter\def\csname res@v6@operator_0.5@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v6@operator_0.5@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@pcmciplus@len\endcsname{2.6}
\expandafter\def\csname res@v6@operator_0.5@pcmciplus@rp\endcsname{0.95}
\expandafter\def\csname res@v6@operator_0.5@pcmciplus@map\endcsname{0.97}
\expandafter\def\csname res@v6@operator_0.5@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v6@operator_0.5@pc@fpn\endcsname{3}
\expandafter\def\csname res@v6@operator_0.5@pc@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v6@operator_0.5@pc@prec\endcsname{0.36}
\expandafter\def\csname res@v6@operator_0.5@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@pc@bw\endcsname{5}
\expandafter\def\csname res@v6@operator_0.5@pc@len\endcsname{5.7}
\expandafter\def\csname res@v6@operator_0.5@pc@rp\endcsname{0.36}
\expandafter\def\csname res@v6@operator_0.5@pc@map\endcsname{0.31}
\expandafter\def\csname res@v6@operator_0.5@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v6@operator_0.5@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v6@operator_0.5@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@dynotears@tt\endcsname{0.27}
\expandafter\def\csname res@v6@operator_0.5@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@operator_0.5@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v6@operator_0.5@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v6@operator_0.5@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v6@operator_0.5@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v6@operator_0.5@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.5@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v6@operator_0.5@doubleml@prec\endcsname{0.68}
\expandafter\def\csname res@v6@operator_0.5@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@doubleml@len\endcsname{4.1}
\expandafter\def\csname res@v6@operator_0.5@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v6@operator_0.5@doubleml@map\endcsname{0.94}
\expandafter\def\csname res@v6@operator_0.5@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.5@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.5@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v6@operator_0.5@varlingam@prec\endcsname{0.29}
\expandafter\def\csname res@v6@operator_0.5@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@varlingam@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.5@varlingam@len\endcsname{9.0}
\expandafter\def\csname res@v6@operator_0.5@varlingam@rp\endcsname{0.70}
\expandafter\def\csname res@v6@operator_0.5@varlingam@map\endcsname{0.80}
\expandafter\def\csname res@v6@operator_0.5@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.5@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.5@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v6@operator_0.5@spacetime_rule@prec\endcsname{0.90}
\expandafter\def\csname res@v6@operator_0.5@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.5@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v6@operator_0.5@spacetime_rule@rp\endcsname{0.83}
\expandafter\def\csname res@v6@operator_0.5@spacetime_rule@map\endcsname{0.85}
\expandafter\def\csname res@v6@operator_0.5@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@operator_0.5@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.5@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.5@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@varsort@bw\endcsname{2}
\expandafter\def\csname res@v6@operator_0.5@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@operator_0.5@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v6@operator_0.5@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.5@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.5@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.5@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.5@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v6@operator_0.5@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v6@operator_0.5@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.5@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@operator_0.5@r2sort@rp\endcsname{0.12}
\expandafter\def\csname res@v6@operator_0.5@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@correlation@tt\endcsname{0.35}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@correlation@prec\endcsname{0.20}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@correlation@bw\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@correlation@len\endcsname{7.2}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@correlation@rp\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@correlation@map\endcsname{0.30}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@granger@fp\endcsname{4/10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@granger@fpn\endcsname{4}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@granger@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@granger@tt\endcsname{0.31}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@granger@prec\endcsname{0.39}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@granger@ab\endcsname{4}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@granger@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@granger@len\endcsname{3.4}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@granger@rp\endcsname{0.50}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@granger@map\endcsname{0.57}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pcmciplus@fp\endcsname{4/10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pcmciplus@fpn\endcsname{4}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pcmciplus@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pcmciplus@prec\endcsname{0.47}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pcmciplus@len\endcsname{1.1}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pcmciplus@rp\endcsname{0.38}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pcmciplus@map\endcsname{0.54}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pc@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pc@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pc@tt\endcsname{0.23}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pc@prec\endcsname{0.16}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pc@bw\endcsname{8}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pc@len\endcsname{2.8}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pc@rp\endcsname{0.17}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@pc@map\endcsname{0.18}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@dynotears@rp\endcsname{0.44}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@dynotears@map\endcsname{0.59}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@doubleml@prec\endcsname{0.25}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@doubleml@ab\endcsname{8}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@doubleml@len\endcsname{0.3}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@doubleml@rp\endcsname{0.33}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@doubleml@map\endcsname{0.43}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varlingam@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varlingam@prec\endcsname{0.17}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varlingam@ab\endcsname{2}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varlingam@bw\endcsname{8}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varlingam@len\endcsname{4.6}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varlingam@rp\endcsname{0.16}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varlingam@map\endcsname{0.27}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@spacetime_rule@fp\endcsname{6/10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@spacetime_rule@fpn\endcsname{6}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@spacetime_rule@tt\endcsname{0.23}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@spacetime_rule@prec\endcsname{0.56}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@spacetime_rule@rp\endcsname{0.38}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@spacetime_rule@map\endcsname{0.48}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varsort@bw\endcsname{6}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varsort@len\endcsname{2.7}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varsort@rp\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@varsort@map\endcsname{0.14}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@operator_0.3_combo_interaction@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@operator_0.3_s40@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v6@operator_0.3_s40@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v6@operator_0.3_s40@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@correlation@tt\endcsname{0.46}
\expandafter\def\csname res@v6@operator_0.3_s40@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v6@operator_0.3_s40@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@correlation@bw\endcsname{2}
\expandafter\def\csname res@v6@operator_0.3_s40@correlation@len\endcsname{35.9}
\expandafter\def\csname res@v6@operator_0.3_s40@correlation@rp\endcsname{0.53}
\expandafter\def\csname res@v6@operator_0.3_s40@correlation@map\endcsname{0.60}
\expandafter\def\csname res@v6@operator_0.3_s40@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.3_s40@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@granger@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v6@operator_0.3_s40@granger@prec\endcsname{0.08}
\expandafter\def\csname res@v6@operator_0.3_s40@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@granger@len\endcsname{32.0}
\expandafter\def\csname res@v6@operator_0.3_s40@granger@rp\endcsname{0.59}
\expandafter\def\csname res@v6@operator_0.3_s40@granger@map\endcsname{0.68}
\expandafter\def\csname res@v6@operator_0.3_s40@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.3_s40@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@pcmciplus@tt\endcsname{0.81}
\expandafter\def\csname res@v6@operator_0.3_s40@pcmciplus@prec\endcsname{0.71}
\expandafter\def\csname res@v6@operator_0.3_s40@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@pcmciplus@len\endcsname{3.0}
\expandafter\def\csname res@v6@operator_0.3_s40@pcmciplus@rp\endcsname{0.88}
\expandafter\def\csname res@v6@operator_0.3_s40@pcmciplus@map\endcsname{0.92}
\expandafter\def\csname res@v6@operator_0.3_s40@pc@fp\endcsname{0/10}
\expandafter\def\csname res@v6@operator_0.3_s40@pc@fpn\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@pc@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v6@operator_0.3_s40@pc@prec\endcsname{0.30}
\expandafter\def\csname res@v6@operator_0.3_s40@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@operator_0.3_s40@pc@len\endcsname{5.6}
\expandafter\def\csname res@v6@operator_0.3_s40@pc@rp\endcsname{0.30}
\expandafter\def\csname res@v6@operator_0.3_s40@pc@map\endcsname{0.23}
\expandafter\def\csname res@v6@operator_0.3_s40@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v6@operator_0.3_s40@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v6@operator_0.3_s40@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@dynotears@tt\endcsname{0.23}
\expandafter\def\csname res@v6@operator_0.3_s40@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@operator_0.3_s40@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v6@operator_0.3_s40@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@dynotears@len\endcsname{0.6}
\expandafter\def\csname res@v6@operator_0.3_s40@dynotears@rp\endcsname{0.95}
\expandafter\def\csname res@v6@operator_0.3_s40@dynotears@map\endcsname{0.96}
\expandafter\def\csname res@v6@operator_0.3_s40@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.3_s40@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.3_s40@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@doubleml@tt\endcsname{0.65}
\expandafter\def\csname res@v6@operator_0.3_s40@doubleml@prec\endcsname{0.77}
\expandafter\def\csname res@v6@operator_0.3_s40@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_s40@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@doubleml@len\endcsname{2.6}
\expandafter\def\csname res@v6@operator_0.3_s40@doubleml@rp\endcsname{0.77}
\expandafter\def\csname res@v6@operator_0.3_s40@doubleml@map\endcsname{0.82}
\expandafter\def\csname res@v6@operator_0.3_s40@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.3_s40@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v6@operator_0.3_s40@varlingam@prec\endcsname{0.27}
\expandafter\def\csname res@v6@operator_0.3_s40@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@varlingam@len\endcsname{13.9}
\expandafter\def\csname res@v6@operator_0.3_s40@varlingam@rp\endcsname{0.59}
\expandafter\def\csname res@v6@operator_0.3_s40@varlingam@map\endcsname{0.78}
\expandafter\def\csname res@v6@operator_0.3_s40@spacetime_rule@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.3_s40@spacetime_rule@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v6@operator_0.3_s40@spacetime_rule@prec\endcsname{1.00}
\expandafter\def\csname res@v6@operator_0.3_s40@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v6@operator_0.3_s40@spacetime_rule@rp\endcsname{0.60}
\expandafter\def\csname res@v6@operator_0.3_s40@spacetime_rule@map\endcsname{0.74}
\expandafter\def\csname res@v6@operator_0.3_s40@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@operator_0.3_s40@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v6@operator_0.3_s40@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v6@operator_0.3_s40@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@varsort@bw\endcsname{5}
\expandafter\def\csname res@v6@operator_0.3_s40@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@operator_0.3_s40@varsort@rp\endcsname{0.05}
\expandafter\def\csname res@v6@operator_0.3_s40@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v6@operator_0.3_s40@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@operator_0.3_s40@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_s40@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v6@operator_0.3_s40@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v6@operator_0.3_s40@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_s40@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_s40@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@operator_0.3_s40@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v6@operator_0.3_s40@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v6@operator_0.3_b50@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v6@operator_0.3_b50@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@correlation@tt\endcsname{0.73}
\expandafter\def\csname res@v6@operator_0.3_b50@correlation@prec\endcsname{0.16}
\expandafter\def\csname res@v6@operator_0.3_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@correlation@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@correlation@len\endcsname{16.6}
\expandafter\def\csname res@v6@operator_0.3_b50@correlation@rp\endcsname{0.76}
\expandafter\def\csname res@v6@operator_0.3_b50@correlation@map\endcsname{0.85}
\expandafter\def\csname res@v6@operator_0.3_b50@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v6@operator_0.3_b50@granger@fpn\endcsname{8}
\expandafter\def\csname res@v6@operator_0.3_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v6@operator_0.3_b50@granger@prec\endcsname{0.23}
\expandafter\def\csname res@v6@operator_0.3_b50@granger@ab\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@granger@len\endcsname{10.6}
\expandafter\def\csname res@v6@operator_0.3_b50@granger@rp\endcsname{0.63}
\expandafter\def\csname res@v6@operator_0.3_b50@granger@map\endcsname{0.70}
\expandafter\def\csname res@v6@operator_0.3_b50@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.3_b50@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.3_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@pcmciplus@tt\endcsname{0.81}
\expandafter\def\csname res@v6@operator_0.3_b50@pcmciplus@prec\endcsname{0.89}
\expandafter\def\csname res@v6@operator_0.3_b50@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@pcmciplus@len\endcsname{2.7}
\expandafter\def\csname res@v6@operator_0.3_b50@pcmciplus@rp\endcsname{0.97}
\expandafter\def\csname res@v6@operator_0.3_b50@pcmciplus@map\endcsname{0.98}
\expandafter\def\csname res@v6@operator_0.3_b50@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v6@operator_0.3_b50@pc@fpn\endcsname{2}
\expandafter\def\csname res@v6@operator_0.3_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@pc@tt\endcsname{0.50}
\expandafter\def\csname res@v6@operator_0.3_b50@pc@prec\endcsname{0.42}
\expandafter\def\csname res@v6@operator_0.3_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@pc@bw\endcsname{3}
\expandafter\def\csname res@v6@operator_0.3_b50@pc@len\endcsname{4.0}
\expandafter\def\csname res@v6@operator_0.3_b50@pc@rp\endcsname{0.42}
\expandafter\def\csname res@v6@operator_0.3_b50@pc@map\endcsname{0.39}
\expandafter\def\csname res@v6@operator_0.3_b50@dynotears@fp\endcsname{8/10}
\expandafter\def\csname res@v6@operator_0.3_b50@dynotears@fpn\endcsname{8}
\expandafter\def\csname res@v6@operator_0.3_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@dynotears@tt\endcsname{0.31}
\expandafter\def\csname res@v6@operator_0.3_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@operator_0.3_b50@dynotears@ab\endcsname{2}
\expandafter\def\csname res@v6@operator_0.3_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@dynotears@len\endcsname{0.8}
\expandafter\def\csname res@v6@operator_0.3_b50@dynotears@rp\endcsname{0.90}
\expandafter\def\csname res@v6@operator_0.3_b50@dynotears@map\endcsname{0.93}
\expandafter\def\csname res@v6@operator_0.3_b50@doubleml@fp\endcsname{8/10}
\expandafter\def\csname res@v6@operator_0.3_b50@doubleml@fpn\endcsname{8}
\expandafter\def\csname res@v6@operator_0.3_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@doubleml@tt\endcsname{0.69}
\expandafter\def\csname res@v6@operator_0.3_b50@doubleml@prec\endcsname{0.77}
\expandafter\def\csname res@v6@operator_0.3_b50@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@doubleml@len\endcsname{2.7}
\expandafter\def\csname res@v6@operator_0.3_b50@doubleml@rp\endcsname{0.67}
\expandafter\def\csname res@v6@operator_0.3_b50@doubleml@map\endcsname{0.79}
\expandafter\def\csname res@v6@operator_0.3_b50@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.3_b50@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.3_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v6@operator_0.3_b50@varlingam@prec\endcsname{0.46}
\expandafter\def\csname res@v6@operator_0.3_b50@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@varlingam@len\endcsname{6.9}
\expandafter\def\csname res@v6@operator_0.3_b50@varlingam@rp\endcsname{0.87}
\expandafter\def\csname res@v6@operator_0.3_b50@varlingam@map\endcsname{0.88}
\expandafter\def\csname res@v6@operator_0.3_b50@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v6@operator_0.3_b50@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v6@operator_0.3_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v6@operator_0.3_b50@spacetime_rule@prec\endcsname{0.94}
\expandafter\def\csname res@v6@operator_0.3_b50@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v6@operator_0.3_b50@spacetime_rule@rp\endcsname{0.69}
\expandafter\def\csname res@v6@operator_0.3_b50@spacetime_rule@map\endcsname{0.78}
\expandafter\def\csname res@v6@operator_0.3_b50@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.3_b50@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v6@operator_0.3_b50@varsort@prec\endcsname{0.12}
\expandafter\def\csname res@v6@operator_0.3_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_b50@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@operator_0.3_b50@varsort@rp\endcsname{0.07}
\expandafter\def\csname res@v6@operator_0.3_b50@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v6@operator_0.3_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@operator_0.3_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@operator_0.3_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@operator_0.3_b50@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v6@operator_0.3_b50@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v6@operator_0.3_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@operator_0.3_b50@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v6@operator_0.3_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@operator_0.3_b50@r2sort@rp\endcsname{0.12}
\expandafter\def\csname res@v6@operator_0.3_b50@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@all_knobs@correlation@fp\endcsname{7/10}
\expandafter\def\csname res@v6@all_knobs@correlation@fpn\endcsname{7}
\expandafter\def\csname res@v6@all_knobs@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v6@all_knobs@correlation@prec\endcsname{0.17}
\expandafter\def\csname res@v6@all_knobs@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@correlation@bw\endcsname{3}
\expandafter\def\csname res@v6@all_knobs@correlation@len\endcsname{15.1}
\expandafter\def\csname res@v6@all_knobs@correlation@rp\endcsname{0.52}
\expandafter\def\csname res@v6@all_knobs@correlation@map\endcsname{0.70}
\expandafter\def\csname res@v6@all_knobs@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v6@all_knobs@granger@fpn\endcsname{9}
\expandafter\def\csname res@v6@all_knobs@granger@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs@granger@tt\endcsname{0.69}
\expandafter\def\csname res@v6@all_knobs@granger@prec\endcsname{0.22}
\expandafter\def\csname res@v6@all_knobs@granger@ab\endcsname{1}
\expandafter\def\csname res@v6@all_knobs@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@granger@len\endcsname{11.2}
\expandafter\def\csname res@v6@all_knobs@granger@rp\endcsname{0.68}
\expandafter\def\csname res@v6@all_knobs@granger@map\endcsname{0.81}
\expandafter\def\csname res@v6@all_knobs@pcmciplus@fp\endcsname{7/10}
\expandafter\def\csname res@v6@all_knobs@pcmciplus@fpn\endcsname{7}
\expandafter\def\csname res@v6@all_knobs@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs@pcmciplus@tt\endcsname{0.69}
\expandafter\def\csname res@v6@all_knobs@pcmciplus@prec\endcsname{0.52}
\expandafter\def\csname res@v6@all_knobs@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@pcmciplus@bw\endcsname{1}
\expandafter\def\csname res@v6@all_knobs@pcmciplus@len\endcsname{3.6}
\expandafter\def\csname res@v6@all_knobs@pcmciplus@rp\endcsname{0.62}
\expandafter\def\csname res@v6@all_knobs@pcmciplus@map\endcsname{0.77}
\expandafter\def\csname res@v6@all_knobs@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v6@all_knobs@pc@fpn\endcsname{2}
\expandafter\def\csname res@v6@all_knobs@pc@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs@pc@tt\endcsname{0.27}
\expandafter\def\csname res@v6@all_knobs@pc@prec\endcsname{0.26}
\expandafter\def\csname res@v6@all_knobs@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@pc@bw\endcsname{6}
\expandafter\def\csname res@v6@all_knobs@pc@len\endcsname{6.5}
\expandafter\def\csname res@v6@all_knobs@pc@rp\endcsname{0.26}
\expandafter\def\csname res@v6@all_knobs@pc@map\endcsname{0.25}
\expandafter\def\csname res@v6@all_knobs@dynotears@fp\endcsname{1/10}
\expandafter\def\csname res@v6@all_knobs@dynotears@fpn\endcsname{1}
\expandafter\def\csname res@v6@all_knobs@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs@dynotears@tt\endcsname{0.04}
\expandafter\def\csname res@v6@all_knobs@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v6@all_knobs@dynotears@ab\endcsname{9}
\expandafter\def\csname res@v6@all_knobs@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@dynotears@len\endcsname{0.1}
\expandafter\def\csname res@v6@all_knobs@dynotears@rp\endcsname{0.72}
\expandafter\def\csname res@v6@all_knobs@dynotears@map\endcsname{0.84}
\expandafter\def\csname res@v6@all_knobs@doubleml@fp\endcsname{7/10}
\expandafter\def\csname res@v6@all_knobs@doubleml@fpn\endcsname{7}
\expandafter\def\csname res@v6@all_knobs@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs@doubleml@tt\endcsname{0.54}
\expandafter\def\csname res@v6@all_knobs@doubleml@prec\endcsname{0.85}
\expandafter\def\csname res@v6@all_knobs@doubleml@ab\endcsname{3}
\expandafter\def\csname res@v6@all_knobs@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@doubleml@len\endcsname{1.9}
\expandafter\def\csname res@v6@all_knobs@doubleml@rp\endcsname{0.73}
\expandafter\def\csname res@v6@all_knobs@doubleml@map\endcsname{0.81}
\expandafter\def\csname res@v6@all_knobs@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v6@all_knobs@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v6@all_knobs@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs@varlingam@tt\endcsname{0.62}
\expandafter\def\csname res@v6@all_knobs@varlingam@prec\endcsname{0.52}
\expandafter\def\csname res@v6@all_knobs@varlingam@ab\endcsname{1}
\expandafter\def\csname res@v6@all_knobs@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@varlingam@len\endcsname{5.3}
\expandafter\def\csname res@v6@all_knobs@varlingam@rp\endcsname{0.67}
\expandafter\def\csname res@v6@all_knobs@varlingam@map\endcsname{0.83}
\expandafter\def\csname res@v6@all_knobs@spacetime_rule@fp\endcsname{0/10}
\expandafter\def\csname res@v6@all_knobs@spacetime_rule@fpn\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs@spacetime_rule@tt\endcsname{0.00}
\expandafter\def\csname res@v6@all_knobs@spacetime_rule@prec\endcsname{0.00}
\expandafter\def\csname res@v6@all_knobs@spacetime_rule@ab\endcsname{9}
\expandafter\def\csname res@v6@all_knobs@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v6@all_knobs@spacetime_rule@len\endcsname{0.1}
\expandafter\def\csname res@v6@all_knobs@spacetime_rule@rp\endcsname{0.49}
\expandafter\def\csname res@v6@all_knobs@spacetime_rule@map\endcsname{0.58}
\expandafter\def\csname res@v6@all_knobs@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@all_knobs@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v6@all_knobs@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@all_knobs@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@all_knobs@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@varsort@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@all_knobs@varsort@rp\endcsname{0.10}
\expandafter\def\csname res@v6@all_knobs@varsort@map\endcsname{0.12}
\expandafter\def\csname res@v6@all_knobs@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@all_knobs@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@all_knobs@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v6@all_knobs@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v6@all_knobs@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs@r2sort@bw\endcsname{3}
\expandafter\def\csname res@v6@all_knobs@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@all_knobs@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@all_knobs@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@correlation@tt\endcsname{0.31}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@correlation@prec\endcsname{0.26}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@correlation@bw\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@correlation@len\endcsname{6.6}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@correlation@rp\endcsname{0.12}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@correlation@map\endcsname{0.32}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@granger@fp\endcsname{5/10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@granger@fpn\endcsname{5}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@granger@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@granger@tt\endcsname{0.27}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@granger@prec\endcsname{0.51}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@granger@ab\endcsname{4}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@granger@len\endcsname{3.1}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@granger@rp\endcsname{0.42}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@granger@map\endcsname{0.52}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pcmciplus@fp\endcsname{5/10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pcmciplus@fpn\endcsname{5}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pcmciplus@tt\endcsname{0.31}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pcmciplus@prec\endcsname{0.51}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pcmciplus@bw\endcsname{3}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pcmciplus@len\endcsname{1.8}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pcmciplus@rp\endcsname{0.48}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pcmciplus@map\endcsname{0.59}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pc@fpn\endcsname{1}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pc@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pc@prec\endcsname{0.23}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pc@bw\endcsname{8}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pc@len\endcsname{3.1}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pc@rp\endcsname{0.24}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@pc@map\endcsname{0.20}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@dynotears@rp\endcsname{0.56}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@dynotears@map\endcsname{0.66}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@doubleml@fp\endcsname{2/10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@doubleml@fpn\endcsname{2}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@doubleml@tt\endcsname{0.08}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@doubleml@prec\endcsname{0.50}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@doubleml@ab\endcsname{6}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@doubleml@bw\endcsname{1}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@doubleml@len\endcsname{0.5}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@doubleml@rp\endcsname{0.27}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@doubleml@map\endcsname{0.34}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varlingam@tt\endcsname{0.15}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varlingam@prec\endcsname{0.14}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varlingam@bw\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varlingam@len\endcsname{3.5}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varlingam@rp\endcsname{0.10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varlingam@map\endcsname{0.21}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@spacetime_rule@fp\endcsname{3/10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@spacetime_rule@fpn\endcsname{3}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@spacetime_rule@tt\endcsname{0.12}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@spacetime_rule@prec\endcsname{0.50}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@spacetime_rule@ab\endcsname{4}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@spacetime_rule@len\endcsname{0.6}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@spacetime_rule@rp\endcsname{0.38}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@spacetime_rule@map\endcsname{0.48}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varsort@bw\endcsname{2}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varsort@rp\endcsname{0.11}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@varsort@map\endcsname{0.12}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@r2sort@tt\endcsname{0.04}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@r2sort@prec\endcsname{0.03}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@r2sort@len\endcsname{2.7}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@r2sort@rp\endcsname{0.06}
\expandafter\def\csname res@v6@all_knobs_combo_interaction@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v6@all_knobs_s40@correlation@fp\endcsname{6/10}
\expandafter\def\csname res@v6@all_knobs_s40@correlation@fpn\endcsname{6}
\expandafter\def\csname res@v6@all_knobs_s40@correlation@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@correlation@tt\endcsname{0.42}
\expandafter\def\csname res@v6@all_knobs_s40@correlation@prec\endcsname{0.09}
\expandafter\def\csname res@v6@all_knobs_s40@correlation@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@correlation@bw\endcsname{3}
\expandafter\def\csname res@v6@all_knobs_s40@correlation@len\endcsname{30.0}
\expandafter\def\csname res@v6@all_knobs_s40@correlation@rp\endcsname{0.40}
\expandafter\def\csname res@v6@all_knobs_s40@correlation@map\endcsname{0.53}
\expandafter\def\csname res@v6@all_knobs_s40@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v6@all_knobs_s40@granger@fpn\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@granger@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v6@all_knobs_s40@granger@prec\endcsname{0.21}
\expandafter\def\csname res@v6@all_knobs_s40@granger@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@granger@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@granger@len\endcsname{18.5}
\expandafter\def\csname res@v6@all_knobs_s40@granger@rp\endcsname{0.63}
\expandafter\def\csname res@v6@all_knobs_s40@granger@map\endcsname{0.68}
\expandafter\def\csname res@v6@all_knobs_s40@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v6@all_knobs_s40@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v6@all_knobs_s40@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@pcmciplus@tt\endcsname{0.50}
\expandafter\def\csname res@v6@all_knobs_s40@pcmciplus@prec\endcsname{0.50}
\expandafter\def\csname res@v6@all_knobs_s40@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@pcmciplus@len\endcsname{3.4}
\expandafter\def\csname res@v6@all_knobs_s40@pcmciplus@rp\endcsname{0.57}
\expandafter\def\csname res@v6@all_knobs_s40@pcmciplus@map\endcsname{0.66}
\expandafter\def\csname res@v6@all_knobs_s40@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v6@all_knobs_s40@pc@fpn\endcsname{1}
\expandafter\def\csname res@v6@all_knobs_s40@pc@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@pc@tt\endcsname{0.15}
\expandafter\def\csname res@v6@all_knobs_s40@pc@prec\endcsname{0.16}
\expandafter\def\csname res@v6@all_knobs_s40@pc@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@pc@bw\endcsname{5}
\expandafter\def\csname res@v6@all_knobs_s40@pc@len\endcsname{7.1}
\expandafter\def\csname res@v6@all_knobs_s40@pc@rp\endcsname{0.16}
\expandafter\def\csname res@v6@all_knobs_s40@pc@map\endcsname{0.14}
\expandafter\def\csname res@v6@all_knobs_s40@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v6@all_knobs_s40@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@dynotears@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v6@all_knobs_s40@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v6@all_knobs_s40@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v6@all_knobs_s40@dynotears@rp\endcsname{0.66}
\expandafter\def\csname res@v6@all_knobs_s40@dynotears@map\endcsname{0.80}
\expandafter\def\csname res@v6@all_knobs_s40@doubleml@fp\endcsname{5/10}
\expandafter\def\csname res@v6@all_knobs_s40@doubleml@fpn\endcsname{5}
\expandafter\def\csname res@v6@all_knobs_s40@doubleml@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@doubleml@tt\endcsname{0.38}
\expandafter\def\csname res@v6@all_knobs_s40@doubleml@prec\endcsname{0.68}
\expandafter\def\csname res@v6@all_knobs_s40@doubleml@ab\endcsname{5}
\expandafter\def\csname res@v6@all_knobs_s40@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@doubleml@len\endcsname{1.6}
\expandafter\def\csname res@v6@all_knobs_s40@doubleml@rp\endcsname{0.56}
\expandafter\def\csname res@v6@all_knobs_s40@doubleml@map\endcsname{0.63}
\expandafter\def\csname res@v6@all_knobs_s40@varlingam@fp\endcsname{7/10}
\expandafter\def\csname res@v6@all_knobs_s40@varlingam@fpn\endcsname{7}
\expandafter\def\csname res@v6@all_knobs_s40@varlingam@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@varlingam@tt\endcsname{0.58}
\expandafter\def\csname res@v6@all_knobs_s40@varlingam@prec\endcsname{0.45}
\expandafter\def\csname res@v6@all_knobs_s40@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@varlingam@len\endcsname{7.3}
\expandafter\def\csname res@v6@all_knobs_s40@varlingam@rp\endcsname{0.58}
\expandafter\def\csname res@v6@all_knobs_s40@varlingam@map\endcsname{0.62}
\expandafter\def\csname res@v6@all_knobs_s40@spacetime_rule@fp\endcsname{0/10}
\expandafter\def\csname res@v6@all_knobs_s40@spacetime_rule@fpn\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@spacetime_rule@tt\endcsname{0.00}
\expandafter\def\csname res@v6@all_knobs_s40@spacetime_rule@prec\endcsname{--}
\expandafter\def\csname res@v6@all_knobs_s40@spacetime_rule@ab\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@spacetime_rule@len\endcsname{0.0}
\expandafter\def\csname res@v6@all_knobs_s40@spacetime_rule@rp\endcsname{0.42}
\expandafter\def\csname res@v6@all_knobs_s40@spacetime_rule@map\endcsname{0.49}
\expandafter\def\csname res@v6@all_knobs_s40@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@all_knobs_s40@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@varsort@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@varsort@tt\endcsname{0.08}
\expandafter\def\csname res@v6@all_knobs_s40@varsort@prec\endcsname{0.07}
\expandafter\def\csname res@v6@all_knobs_s40@varsort@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@varsort@bw\endcsname{1}
\expandafter\def\csname res@v6@all_knobs_s40@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v6@all_knobs_s40@varsort@rp\endcsname{0.05}
\expandafter\def\csname res@v6@all_knobs_s40@varsort@map\endcsname{0.08}
\expandafter\def\csname res@v6@all_knobs_s40@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v6@all_knobs_s40@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@r2sort@n\endcsname{10}
\expandafter\def\csname res@v6@all_knobs_s40@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v6@all_knobs_s40@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v6@all_knobs_s40@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v6@all_knobs_s40@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v6@all_knobs_s40@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v6@all_knobs_s40@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v6@all_knobs_s40@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v7@no_parameter_edges@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v7@no_parameter_edges@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@correlation@n\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v7@no_parameter_edges@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v7@no_parameter_edges@correlation@ab\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@correlation@bw\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@correlation@len\endcsname{18.2}
\expandafter\def\csname res@v7@no_parameter_edges@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v7@no_parameter_edges@correlation@map\endcsname{0.77}
\expandafter\def\csname res@v7@no_parameter_edges@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v7@no_parameter_edges@granger@fpn\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@granger@n\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v7@no_parameter_edges@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v7@no_parameter_edges@granger@ab\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@granger@bw\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@granger@len\endcsname{16.8}
\expandafter\def\csname res@v7@no_parameter_edges@granger@rp\endcsname{0.70}
\expandafter\def\csname res@v7@no_parameter_edges@granger@map\endcsname{0.79}
\expandafter\def\csname res@v7@no_parameter_edges@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v7@no_parameter_edges@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v7@no_parameter_edges@pcmciplus@prec\endcsname{0.78}
\expandafter\def\csname res@v7@no_parameter_edges@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@pcmciplus@len\endcsname{2.9}
\expandafter\def\csname res@v7@no_parameter_edges@pcmciplus@rp\endcsname{0.94}
\expandafter\def\csname res@v7@no_parameter_edges@pcmciplus@map\endcsname{0.97}
\expandafter\def\csname res@v7@no_parameter_edges@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v7@no_parameter_edges@pc@fpn\endcsname{2}
\expandafter\def\csname res@v7@no_parameter_edges@pc@n\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v7@no_parameter_edges@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v7@no_parameter_edges@pc@ab\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@pc@bw\endcsname{4}
\expandafter\def\csname res@v7@no_parameter_edges@pc@len\endcsname{4.9}
\expandafter\def\csname res@v7@no_parameter_edges@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v7@no_parameter_edges@pc@map\endcsname{0.31}
\expandafter\def\csname res@v7@no_parameter_edges@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v7@no_parameter_edges@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v7@no_parameter_edges@dynotears@n\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@dynotears@tt\endcsname{0.31}
\expandafter\def\csname res@v7@no_parameter_edges@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v7@no_parameter_edges@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v7@no_parameter_edges@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@dynotears@len\endcsname{0.8}
\expandafter\def\csname res@v7@no_parameter_edges@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v7@no_parameter_edges@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v7@no_parameter_edges@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v7@no_parameter_edges@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@doubleml@n\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v7@no_parameter_edges@doubleml@prec\endcsname{0.72}
\expandafter\def\csname res@v7@no_parameter_edges@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@doubleml@len\endcsname{3.7}
\expandafter\def\csname res@v7@no_parameter_edges@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v7@no_parameter_edges@doubleml@map\endcsname{0.94}
\expandafter\def\csname res@v7@no_parameter_edges@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v7@no_parameter_edges@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@varlingam@n\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@varlingam@tt\endcsname{0.73}
\expandafter\def\csname res@v7@no_parameter_edges@varlingam@prec\endcsname{0.33}
\expandafter\def\csname res@v7@no_parameter_edges@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@varlingam@len\endcsname{9.1}
\expandafter\def\csname res@v7@no_parameter_edges@varlingam@rp\endcsname{0.79}
\expandafter\def\csname res@v7@no_parameter_edges@varlingam@map\endcsname{0.87}
\expandafter\def\csname res@v7@no_parameter_edges@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v7@no_parameter_edges@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v7@no_parameter_edges@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@spacetime_rule@tt\endcsname{0.50}
\expandafter\def\csname res@v7@no_parameter_edges@spacetime_rule@prec\endcsname{0.80}
\expandafter\def\csname res@v7@no_parameter_edges@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@spacetime_rule@len\endcsname{1.6}
\expandafter\def\csname res@v7@no_parameter_edges@spacetime_rule@rp\endcsname{0.68}
\expandafter\def\csname res@v7@no_parameter_edges@spacetime_rule@map\endcsname{0.79}
\expandafter\def\csname res@v7@no_parameter_edges@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v7@no_parameter_edges@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v7@no_parameter_edges@varsort@n\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v7@no_parameter_edges@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v7@no_parameter_edges@varsort@ab\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@varsort@bw\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v7@no_parameter_edges@varsort@rp\endcsname{0.11}
\expandafter\def\csname res@v7@no_parameter_edges@varsort@map\endcsname{0.12}
\expandafter\def\csname res@v7@no_parameter_edges@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v7@no_parameter_edges@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@r2sort@n\endcsname{10}
\expandafter\def\csname res@v7@no_parameter_edges@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v7@no_parameter_edges@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v7@no_parameter_edges@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v7@no_parameter_edges@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v7@no_parameter_edges@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v7@no_parameter_edges@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v7@no_parameter_edges@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v7@no_temporal_edges@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v7@no_temporal_edges@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@correlation@n\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@correlation@tt\endcsname{0.65}
\expandafter\def\csname res@v7@no_temporal_edges@correlation@prec\endcsname{0.16}
\expandafter\def\csname res@v7@no_temporal_edges@correlation@ab\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@correlation@bw\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@correlation@len\endcsname{16.7}
\expandafter\def\csname res@v7@no_temporal_edges@correlation@rp\endcsname{0.66}
\expandafter\def\csname res@v7@no_temporal_edges@correlation@map\endcsname{0.75}
\expandafter\def\csname res@v7@no_temporal_edges@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v7@no_temporal_edges@granger@fpn\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@granger@n\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v7@no_temporal_edges@granger@prec\endcsname{0.17}
\expandafter\def\csname res@v7@no_temporal_edges@granger@ab\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@granger@bw\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@granger@len\endcsname{16.3}
\expandafter\def\csname res@v7@no_temporal_edges@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v7@no_temporal_edges@granger@map\endcsname{0.79}
\expandafter\def\csname res@v7@no_temporal_edges@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v7@no_temporal_edges@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@pcmciplus@tt\endcsname{0.85}
\expandafter\def\csname res@v7@no_temporal_edges@pcmciplus@prec\endcsname{0.77}
\expandafter\def\csname res@v7@no_temporal_edges@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@pcmciplus@len\endcsname{3.1}
\expandafter\def\csname res@v7@no_temporal_edges@pcmciplus@rp\endcsname{1.00}
\expandafter\def\csname res@v7@no_temporal_edges@pcmciplus@map\endcsname{1.00}
\expandafter\def\csname res@v7@no_temporal_edges@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v7@no_temporal_edges@pc@fpn\endcsname{2}
\expandafter\def\csname res@v7@no_temporal_edges@pc@n\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@pc@tt\endcsname{0.42}
\expandafter\def\csname res@v7@no_temporal_edges@pc@prec\endcsname{0.39}
\expandafter\def\csname res@v7@no_temporal_edges@pc@ab\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@pc@bw\endcsname{5}
\expandafter\def\csname res@v7@no_temporal_edges@pc@len\endcsname{4.9}
\expandafter\def\csname res@v7@no_temporal_edges@pc@rp\endcsname{0.39}
\expandafter\def\csname res@v7@no_temporal_edges@pc@map\endcsname{0.35}
\expandafter\def\csname res@v7@no_temporal_edges@dynotears@fp\endcsname{5/10}
\expandafter\def\csname res@v7@no_temporal_edges@dynotears@fpn\endcsname{5}
\expandafter\def\csname res@v7@no_temporal_edges@dynotears@n\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@dynotears@tt\endcsname{0.23}
\expandafter\def\csname res@v7@no_temporal_edges@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v7@no_temporal_edges@dynotears@ab\endcsname{5}
\expandafter\def\csname res@v7@no_temporal_edges@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@dynotears@len\endcsname{0.6}
\expandafter\def\csname res@v7@no_temporal_edges@dynotears@rp\endcsname{0.92}
\expandafter\def\csname res@v7@no_temporal_edges@dynotears@map\endcsname{0.98}
\expandafter\def\csname res@v7@no_temporal_edges@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v7@no_temporal_edges@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@doubleml@n\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v7@no_temporal_edges@doubleml@prec\endcsname{0.86}
\expandafter\def\csname res@v7@no_temporal_edges@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@doubleml@len\endcsname{2.9}
\expandafter\def\csname res@v7@no_temporal_edges@doubleml@rp\endcsname{0.87}
\expandafter\def\csname res@v7@no_temporal_edges@doubleml@map\endcsname{0.91}
\expandafter\def\csname res@v7@no_temporal_edges@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v7@no_temporal_edges@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@varlingam@n\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@varlingam@tt\endcsname{0.81}
\expandafter\def\csname res@v7@no_temporal_edges@varlingam@prec\endcsname{0.40}
\expandafter\def\csname res@v7@no_temporal_edges@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@varlingam@len\endcsname{8.9}
\expandafter\def\csname res@v7@no_temporal_edges@varlingam@rp\endcsname{0.87}
\expandafter\def\csname res@v7@no_temporal_edges@varlingam@map\endcsname{0.93}
\expandafter\def\csname res@v7@no_temporal_edges@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v7@no_temporal_edges@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v7@no_temporal_edges@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@spacetime_rule@tt\endcsname{0.35}
\expandafter\def\csname res@v7@no_temporal_edges@spacetime_rule@prec\endcsname{0.78}
\expandafter\def\csname res@v7@no_temporal_edges@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v7@no_temporal_edges@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v7@no_temporal_edges@spacetime_rule@rp\endcsname{0.47}
\expandafter\def\csname res@v7@no_temporal_edges@spacetime_rule@map\endcsname{0.62}
\expandafter\def\csname res@v7@no_temporal_edges@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v7@no_temporal_edges@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v7@no_temporal_edges@varsort@n\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v7@no_temporal_edges@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v7@no_temporal_edges@varsort@ab\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@varsort@bw\endcsname{1}
\expandafter\def\csname res@v7@no_temporal_edges@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v7@no_temporal_edges@varsort@rp\endcsname{0.11}
\expandafter\def\csname res@v7@no_temporal_edges@varsort@map\endcsname{0.13}
\expandafter\def\csname res@v7@no_temporal_edges@r2sort@fp\endcsname{3/10}
\expandafter\def\csname res@v7@no_temporal_edges@r2sort@fpn\endcsname{3}
\expandafter\def\csname res@v7@no_temporal_edges@r2sort@n\endcsname{10}
\expandafter\def\csname res@v7@no_temporal_edges@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v7@no_temporal_edges@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v7@no_temporal_edges@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v7@no_temporal_edges@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v7@no_temporal_edges@r2sort@rp\endcsname{0.16}
\expandafter\def\csname res@v7@no_temporal_edges@r2sort@map\endcsname{0.26}
\expandafter\def\csname res@v8@phase_0.25@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.25@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@correlation@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@correlation@tt\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.25@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v8@phase_0.25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@correlation@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@correlation@len\endcsname{18.0}
\expandafter\def\csname res@v8@phase_0.25@correlation@rp\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.25@correlation@map\endcsname{0.81}
\expandafter\def\csname res@v8@phase_0.25@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.25@granger@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.25@granger@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.25@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v8@phase_0.25@granger@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@granger@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@granger@len\endcsname{17.2}
\expandafter\def\csname res@v8@phase_0.25@granger@rp\endcsname{0.71}
\expandafter\def\csname res@v8@phase_0.25@granger@map\endcsname{0.77}
\expandafter\def\csname res@v8@phase_0.25@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.25@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v8@phase_0.25@pcmciplus@prec\endcsname{0.79}
\expandafter\def\csname res@v8@phase_0.25@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@pcmciplus@len\endcsname{3.0}
\expandafter\def\csname res@v8@phase_0.25@pcmciplus@rp\endcsname{0.88}
\expandafter\def\csname res@v8@phase_0.25@pcmciplus@map\endcsname{0.94}
\expandafter\def\csname res@v8@phase_0.25@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v8@phase_0.25@pc@fpn\endcsname{3}
\expandafter\def\csname res@v8@phase_0.25@pc@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v8@phase_0.25@pc@prec\endcsname{0.36}
\expandafter\def\csname res@v8@phase_0.25@pc@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@pc@bw\endcsname{3}
\expandafter\def\csname res@v8@phase_0.25@pc@len\endcsname{5.6}
\expandafter\def\csname res@v8@phase_0.25@pc@rp\endcsname{0.36}
\expandafter\def\csname res@v8@phase_0.25@pc@map\endcsname{0.31}
\expandafter\def\csname res@v8@phase_0.25@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v8@phase_0.25@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v8@phase_0.25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@dynotears@tt\endcsname{0.31}
\expandafter\def\csname res@v8@phase_0.25@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v8@phase_0.25@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v8@phase_0.25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@dynotears@len\endcsname{0.8}
\expandafter\def\csname res@v8@phase_0.25@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v8@phase_0.25@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v8@phase_0.25@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.25@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v8@phase_0.25@doubleml@prec\endcsname{0.72}
\expandafter\def\csname res@v8@phase_0.25@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@doubleml@len\endcsname{3.7}
\expandafter\def\csname res@v8@phase_0.25@doubleml@rp\endcsname{0.83}
\expandafter\def\csname res@v8@phase_0.25@doubleml@map\endcsname{0.91}
\expandafter\def\csname res@v8@phase_0.25@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.25@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v8@phase_0.25@varlingam@prec\endcsname{0.35}
\expandafter\def\csname res@v8@phase_0.25@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@varlingam@len\endcsname{9.3}
\expandafter\def\csname res@v8@phase_0.25@varlingam@rp\endcsname{0.78}
\expandafter\def\csname res@v8@phase_0.25@varlingam@map\endcsname{0.87}
\expandafter\def\csname res@v8@phase_0.25@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.25@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v8@phase_0.25@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v8@phase_0.25@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v8@phase_0.25@spacetime_rule@rp\endcsname{0.68}
\expandafter\def\csname res@v8@phase_0.25@spacetime_rule@map\endcsname{0.79}
\expandafter\def\csname res@v8@phase_0.25@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v8@phase_0.25@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v8@phase_0.25@varsort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v8@phase_0.25@varsort@prec\endcsname{0.20}
\expandafter\def\csname res@v8@phase_0.25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@varsort@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v8@phase_0.25@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.25@varsort@map\endcsname{0.21}
\expandafter\def\csname res@v8@phase_0.25@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.25@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.25@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.25@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v8@phase_0.25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.25@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v8@phase_0.25@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v8@phase_0.25@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v8@phase_0.5@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.5@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@correlation@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@correlation@tt\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.5@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v8@phase_0.5@correlation@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@correlation@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@correlation@len\endcsname{18.0}
\expandafter\def\csname res@v8@phase_0.5@correlation@rp\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.5@correlation@map\endcsname{0.81}
\expandafter\def\csname res@v8@phase_0.5@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.5@granger@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.5@granger@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.5@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v8@phase_0.5@granger@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@granger@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@granger@len\endcsname{16.7}
\expandafter\def\csname res@v8@phase_0.5@granger@rp\endcsname{0.71}
\expandafter\def\csname res@v8@phase_0.5@granger@map\endcsname{0.77}
\expandafter\def\csname res@v8@phase_0.5@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.5@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v8@phase_0.5@pcmciplus@prec\endcsname{0.76}
\expandafter\def\csname res@v8@phase_0.5@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@pcmciplus@len\endcsname{3.2}
\expandafter\def\csname res@v8@phase_0.5@pcmciplus@rp\endcsname{0.85}
\expandafter\def\csname res@v8@phase_0.5@pcmciplus@map\endcsname{0.93}
\expandafter\def\csname res@v8@phase_0.5@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v8@phase_0.5@pc@fpn\endcsname{3}
\expandafter\def\csname res@v8@phase_0.5@pc@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v8@phase_0.5@pc@prec\endcsname{0.36}
\expandafter\def\csname res@v8@phase_0.5@pc@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@pc@bw\endcsname{3}
\expandafter\def\csname res@v8@phase_0.5@pc@len\endcsname{5.6}
\expandafter\def\csname res@v8@phase_0.5@pc@rp\endcsname{0.36}
\expandafter\def\csname res@v8@phase_0.5@pc@map\endcsname{0.31}
\expandafter\def\csname res@v8@phase_0.5@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v8@phase_0.5@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v8@phase_0.5@dynotears@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@dynotears@tt\endcsname{0.27}
\expandafter\def\csname res@v8@phase_0.5@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v8@phase_0.5@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v8@phase_0.5@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v8@phase_0.5@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v8@phase_0.5@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v8@phase_0.5@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.5@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@doubleml@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v8@phase_0.5@doubleml@prec\endcsname{0.69}
\expandafter\def\csname res@v8@phase_0.5@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@doubleml@len\endcsname{3.7}
\expandafter\def\csname res@v8@phase_0.5@doubleml@rp\endcsname{0.87}
\expandafter\def\csname res@v8@phase_0.5@doubleml@map\endcsname{0.92}
\expandafter\def\csname res@v8@phase_0.5@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.5@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.5@varlingam@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@varlingam@tt\endcsname{0.73}
\expandafter\def\csname res@v8@phase_0.5@varlingam@prec\endcsname{0.31}
\expandafter\def\csname res@v8@phase_0.5@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@varlingam@len\endcsname{9.6}
\expandafter\def\csname res@v8@phase_0.5@varlingam@rp\endcsname{0.72}
\expandafter\def\csname res@v8@phase_0.5@varlingam@map\endcsname{0.82}
\expandafter\def\csname res@v8@phase_0.5@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.5@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.5@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@spacetime_rule@tt\endcsname{0.50}
\expandafter\def\csname res@v8@phase_0.5@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v8@phase_0.5@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v8@phase_0.5@spacetime_rule@rp\endcsname{0.68}
\expandafter\def\csname res@v8@phase_0.5@spacetime_rule@map\endcsname{0.79}
\expandafter\def\csname res@v8@phase_0.5@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.5@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@varsort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v8@phase_0.5@varsort@prec\endcsname{0.10}
\expandafter\def\csname res@v8@phase_0.5@varsort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@varsort@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.5@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v8@phase_0.5@varsort@rp\endcsname{0.13}
\expandafter\def\csname res@v8@phase_0.5@varsort@map\endcsname{0.14}
\expandafter\def\csname res@v8@phase_0.5@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.5@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@r2sort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.5@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.5@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v8@phase_0.5@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.5@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.5@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v8@phase_0.5@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v8@phase_0.5@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v8@phase_0.75@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.75@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@correlation@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@correlation@tt\endcsname{0.62}
\expandafter\def\csname res@v8@phase_0.75@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v8@phase_0.75@correlation@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@correlation@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@correlation@len\endcsname{17.9}
\expandafter\def\csname res@v8@phase_0.75@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v8@phase_0.75@correlation@map\endcsname{0.81}
\expandafter\def\csname res@v8@phase_0.75@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.75@granger@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.75@granger@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@granger@tt\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.75@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v8@phase_0.75@granger@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@granger@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@granger@len\endcsname{16.6}
\expandafter\def\csname res@v8@phase_0.75@granger@rp\endcsname{0.71}
\expandafter\def\csname res@v8@phase_0.75@granger@map\endcsname{0.76}
\expandafter\def\csname res@v8@phase_0.75@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.75@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@pcmciplus@tt\endcsname{0.69}
\expandafter\def\csname res@v8@phase_0.75@pcmciplus@prec\endcsname{0.69}
\expandafter\def\csname res@v8@phase_0.75@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@pcmciplus@len\endcsname{3.3}
\expandafter\def\csname res@v8@phase_0.75@pcmciplus@rp\endcsname{0.85}
\expandafter\def\csname res@v8@phase_0.75@pcmciplus@map\endcsname{0.93}
\expandafter\def\csname res@v8@phase_0.75@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v8@phase_0.75@pc@fpn\endcsname{3}
\expandafter\def\csname res@v8@phase_0.75@pc@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v8@phase_0.75@pc@prec\endcsname{0.36}
\expandafter\def\csname res@v8@phase_0.75@pc@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@pc@bw\endcsname{3}
\expandafter\def\csname res@v8@phase_0.75@pc@len\endcsname{5.5}
\expandafter\def\csname res@v8@phase_0.75@pc@rp\endcsname{0.36}
\expandafter\def\csname res@v8@phase_0.75@pc@map\endcsname{0.32}
\expandafter\def\csname res@v8@phase_0.75@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v8@phase_0.75@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v8@phase_0.75@dynotears@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@dynotears@tt\endcsname{0.27}
\expandafter\def\csname res@v8@phase_0.75@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v8@phase_0.75@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v8@phase_0.75@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v8@phase_0.75@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v8@phase_0.75@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v8@phase_0.75@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.75@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@doubleml@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v8@phase_0.75@doubleml@prec\endcsname{0.78}
\expandafter\def\csname res@v8@phase_0.75@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@doubleml@len\endcsname{3.5}
\expandafter\def\csname res@v8@phase_0.75@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v8@phase_0.75@doubleml@map\endcsname{0.94}
\expandafter\def\csname res@v8@phase_0.75@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.75@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@varlingam@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v8@phase_0.75@varlingam@prec\endcsname{0.28}
\expandafter\def\csname res@v8@phase_0.75@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@varlingam@len\endcsname{10.0}
\expandafter\def\csname res@v8@phase_0.75@varlingam@rp\endcsname{0.68}
\expandafter\def\csname res@v8@phase_0.75@varlingam@map\endcsname{0.83}
\expandafter\def\csname res@v8@phase_0.75@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v8@phase_0.75@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v8@phase_0.75@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v8@phase_0.75@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v8@phase_0.75@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v8@phase_0.75@spacetime_rule@rp\endcsname{0.58}
\expandafter\def\csname res@v8@phase_0.75@spacetime_rule@map\endcsname{0.75}
\expandafter\def\csname res@v8@phase_0.75@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v8@phase_0.75@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75@varsort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v8@phase_0.75@varsort@prec\endcsname{0.18}
\expandafter\def\csname res@v8@phase_0.75@varsort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@varsort@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v8@phase_0.75@varsort@rp\endcsname{0.13}
\expandafter\def\csname res@v8@phase_0.75@varsort@map\endcsname{0.17}
\expandafter\def\csname res@v8@phase_0.75@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.75@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@r2sort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.75@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v8@phase_0.75@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v8@phase_0.75@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v8@phase_0.75@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v8@phase_0.9@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.9@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@correlation@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v8@phase_0.9@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.9@correlation@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@correlation@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@correlation@len\endcsname{17.7}
\expandafter\def\csname res@v8@phase_0.9@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v8@phase_0.9@correlation@map\endcsname{0.80}
\expandafter\def\csname res@v8@phase_0.9@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.9@granger@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.9@granger@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v8@phase_0.9@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.9@granger@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@granger@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@granger@len\endcsname{16.5}
\expandafter\def\csname res@v8@phase_0.9@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.9@granger@map\endcsname{0.75}
\expandafter\def\csname res@v8@phase_0.9@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.9@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@pcmciplus@tt\endcsname{0.77}
\expandafter\def\csname res@v8@phase_0.9@pcmciplus@prec\endcsname{0.66}
\expandafter\def\csname res@v8@phase_0.9@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@pcmciplus@len\endcsname{3.4}
\expandafter\def\csname res@v8@phase_0.9@pcmciplus@rp\endcsname{0.87}
\expandafter\def\csname res@v8@phase_0.9@pcmciplus@map\endcsname{0.94}
\expandafter\def\csname res@v8@phase_0.9@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v8@phase_0.9@pc@fpn\endcsname{3}
\expandafter\def\csname res@v8@phase_0.9@pc@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v8@phase_0.9@pc@prec\endcsname{0.37}
\expandafter\def\csname res@v8@phase_0.9@pc@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@pc@bw\endcsname{3}
\expandafter\def\csname res@v8@phase_0.9@pc@len\endcsname{5.3}
\expandafter\def\csname res@v8@phase_0.9@pc@rp\endcsname{0.37}
\expandafter\def\csname res@v8@phase_0.9@pc@map\endcsname{0.32}
\expandafter\def\csname res@v8@phase_0.9@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v8@phase_0.9@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v8@phase_0.9@dynotears@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@dynotears@tt\endcsname{0.27}
\expandafter\def\csname res@v8@phase_0.9@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v8@phase_0.9@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v8@phase_0.9@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v8@phase_0.9@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v8@phase_0.9@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v8@phase_0.9@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.9@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.9@doubleml@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v8@phase_0.9@doubleml@prec\endcsname{0.71}
\expandafter\def\csname res@v8@phase_0.9@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v8@phase_0.9@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@doubleml@len\endcsname{3.5}
\expandafter\def\csname res@v8@phase_0.9@doubleml@rp\endcsname{0.87}
\expandafter\def\csname res@v8@phase_0.9@doubleml@map\endcsname{0.92}
\expandafter\def\csname res@v8@phase_0.9@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.9@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@varlingam@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v8@phase_0.9@varlingam@prec\endcsname{0.33}
\expandafter\def\csname res@v8@phase_0.9@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@varlingam@len\endcsname{9.5}
\expandafter\def\csname res@v8@phase_0.9@varlingam@rp\endcsname{0.79}
\expandafter\def\csname res@v8@phase_0.9@varlingam@map\endcsname{0.87}
\expandafter\def\csname res@v8@phase_0.9@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v8@phase_0.9@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v8@phase_0.9@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v8@phase_0.9@spacetime_rule@prec\endcsname{0.80}
\expandafter\def\csname res@v8@phase_0.9@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@spacetime_rule@len\endcsname{1.5}
\expandafter\def\csname res@v8@phase_0.9@spacetime_rule@rp\endcsname{0.58}
\expandafter\def\csname res@v8@phase_0.9@spacetime_rule@map\endcsname{0.75}
\expandafter\def\csname res@v8@phase_0.9@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v8@phase_0.9@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v8@phase_0.9@varsort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v8@phase_0.9@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v8@phase_0.9@varsort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@varsort@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.9@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v8@phase_0.9@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v8@phase_0.9@varsort@map\endcsname{0.17}
\expandafter\def\csname res@v8@phase_0.9@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.9@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@r2sort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.9@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.9@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v8@phase_0.9@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.9@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.9@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v8@phase_0.9@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v8@phase_0.9@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@correlation@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@correlation@tt\endcsname{0.08}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@correlation@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@correlation@bw\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@correlation@len\endcsname{5.7}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@correlation@rp\endcsname{0.03}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@correlation@map\endcsname{0.24}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@granger@fp\endcsname{3/10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@granger@fpn\endcsname{3}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@granger@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@granger@tt\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@granger@prec\endcsname{0.17}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@granger@ab\endcsname{6}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@granger@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@granger@len\endcsname{3.7}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@granger@rp\endcsname{0.39}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@granger@map\endcsname{0.54}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pcmciplus@fp\endcsname{3/10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pcmciplus@fpn\endcsname{3}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pcmciplus@tt\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pcmciplus@prec\endcsname{0.33}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pcmciplus@len\endcsname{1.1}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pcmciplus@rp\endcsname{0.46}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pcmciplus@map\endcsname{0.60}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pc@fp\endcsname{2/10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pc@fpn\endcsname{2}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pc@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pc@tt\endcsname{0.08}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pc@prec\endcsname{0.13}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pc@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pc@bw\endcsname{6}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pc@len\endcsname{2.9}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pc@rp\endcsname{0.18}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@pc@map\endcsname{0.20}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@dynotears@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@dynotears@rp\endcsname{0.47}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@dynotears@map\endcsname{0.45}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@doubleml@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@doubleml@prec\endcsname{0.25}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@doubleml@ab\endcsname{8}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@doubleml@len\endcsname{0.3}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@doubleml@rp\endcsname{0.21}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@doubleml@map\endcsname{0.31}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varlingam@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varlingam@tt\endcsname{0.19}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varlingam@prec\endcsname{0.18}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varlingam@ab\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varlingam@bw\endcsname{9}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varlingam@len\endcsname{5.1}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varlingam@rp\endcsname{0.17}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varlingam@map\endcsname{0.28}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@spacetime_rule@prec\endcsname{0.60}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@spacetime_rule@rp\endcsname{0.45}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@spacetime_rule@map\endcsname{0.56}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varsort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varsort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varsort@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varsort@rp\endcsname{0.17}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@r2sort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@r2sort@len\endcsname{2.9}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v8@phase_0.75_combo_interaction@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v8@phase_0.75_s40@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.75_s40@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.75_s40@correlation@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v8@phase_0.75_s40@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v8@phase_0.75_s40@correlation@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@correlation@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@correlation@len\endcsname{36.1}
\expandafter\def\csname res@v8@phase_0.75_s40@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v8@phase_0.75_s40@correlation@map\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.75_s40@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v8@phase_0.75_s40@granger@fpn\endcsname{8}
\expandafter\def\csname res@v8@phase_0.75_s40@granger@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v8@phase_0.75_s40@granger@prec\endcsname{0.08}
\expandafter\def\csname res@v8@phase_0.75_s40@granger@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@granger@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@granger@len\endcsname{31.9}
\expandafter\def\csname res@v8@phase_0.75_s40@granger@rp\endcsname{0.57}
\expandafter\def\csname res@v8@phase_0.75_s40@granger@map\endcsname{0.63}
\expandafter\def\csname res@v8@phase_0.75_s40@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.75_s40@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.75_s40@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@pcmciplus@tt\endcsname{0.85}
\expandafter\def\csname res@v8@phase_0.75_s40@pcmciplus@prec\endcsname{0.81}
\expandafter\def\csname res@v8@phase_0.75_s40@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_s40@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@pcmciplus@len\endcsname{3.1}
\expandafter\def\csname res@v8@phase_0.75_s40@pcmciplus@rp\endcsname{0.88}
\expandafter\def\csname res@v8@phase_0.75_s40@pcmciplus@map\endcsname{0.92}
\expandafter\def\csname res@v8@phase_0.75_s40@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v8@phase_0.75_s40@pc@fpn\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_s40@pc@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v8@phase_0.75_s40@pc@prec\endcsname{0.30}
\expandafter\def\csname res@v8@phase_0.75_s40@pc@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@pc@bw\endcsname{3}
\expandafter\def\csname res@v8@phase_0.75_s40@pc@len\endcsname{4.8}
\expandafter\def\csname res@v8@phase_0.75_s40@pc@rp\endcsname{0.30}
\expandafter\def\csname res@v8@phase_0.75_s40@pc@map\endcsname{0.22}
\expandafter\def\csname res@v8@phase_0.75_s40@dynotears@fp\endcsname{3/10}
\expandafter\def\csname res@v8@phase_0.75_s40@dynotears@fpn\endcsname{3}
\expandafter\def\csname res@v8@phase_0.75_s40@dynotears@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@dynotears@tt\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.75_s40@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v8@phase_0.75_s40@dynotears@ab\endcsname{7}
\expandafter\def\csname res@v8@phase_0.75_s40@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@dynotears@len\endcsname{0.4}
\expandafter\def\csname res@v8@phase_0.75_s40@dynotears@rp\endcsname{0.93}
\expandafter\def\csname res@v8@phase_0.75_s40@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v8@phase_0.75_s40@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.75_s40@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@doubleml@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@doubleml@tt\endcsname{0.77}
\expandafter\def\csname res@v8@phase_0.75_s40@doubleml@prec\endcsname{0.88}
\expandafter\def\csname res@v8@phase_0.75_s40@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@doubleml@len\endcsname{2.6}
\expandafter\def\csname res@v8@phase_0.75_s40@doubleml@rp\endcsname{0.77}
\expandafter\def\csname res@v8@phase_0.75_s40@doubleml@map\endcsname{0.83}
\expandafter\def\csname res@v8@phase_0.75_s40@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.75_s40@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@varlingam@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v8@phase_0.75_s40@varlingam@prec\endcsname{0.27}
\expandafter\def\csname res@v8@phase_0.75_s40@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@varlingam@len\endcsname{10.1}
\expandafter\def\csname res@v8@phase_0.75_s40@varlingam@rp\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.75_s40@varlingam@map\endcsname{0.77}
\expandafter\def\csname res@v8@phase_0.75_s40@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v8@phase_0.75_s40@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v8@phase_0.75_s40@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@spacetime_rule@tt\endcsname{0.35}
\expandafter\def\csname res@v8@phase_0.75_s40@spacetime_rule@prec\endcsname{0.80}
\expandafter\def\csname res@v8@phase_0.75_s40@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname res@v8@phase_0.75_s40@spacetime_rule@rp\endcsname{0.62}
\expandafter\def\csname res@v8@phase_0.75_s40@spacetime_rule@map\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.75_s40@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.75_s40@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@varsort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v8@phase_0.75_s40@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v8@phase_0.75_s40@varsort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@varsort@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v8@phase_0.75_s40@varsort@rp\endcsname{0.05}
\expandafter\def\csname res@v8@phase_0.75_s40@varsort@map\endcsname{0.06}
\expandafter\def\csname res@v8@phase_0.75_s40@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.75_s40@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@r2sort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_s40@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v8@phase_0.75_s40@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v8@phase_0.75_s40@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@r2sort@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_s40@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v8@phase_0.75_s40@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v8@phase_0.75_s40@r2sort@map\endcsname{0.06}
\expandafter\def\csname res@v8@phase_0.75_b50@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.75_b50@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@correlation@tt\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.75_b50@correlation@prec\endcsname{0.18}
\expandafter\def\csname res@v8@phase_0.75_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@correlation@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@correlation@len\endcsname{15.2}
\expandafter\def\csname res@v8@phase_0.75_b50@correlation@rp\endcsname{0.67}
\expandafter\def\csname res@v8@phase_0.75_b50@correlation@map\endcsname{0.81}
\expandafter\def\csname res@v8@phase_0.75_b50@granger@fp\endcsname{8/10}
\expandafter\def\csname res@v8@phase_0.75_b50@granger@fpn\endcsname{8}
\expandafter\def\csname res@v8@phase_0.75_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v8@phase_0.75_b50@granger@prec\endcsname{0.32}
\expandafter\def\csname res@v8@phase_0.75_b50@granger@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@granger@len\endcsname{9.6}
\expandafter\def\csname res@v8@phase_0.75_b50@granger@rp\endcsname{0.64}
\expandafter\def\csname res@v8@phase_0.75_b50@granger@map\endcsname{0.73}
\expandafter\def\csname res@v8@phase_0.75_b50@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.75_b50@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.75_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@pcmciplus@tt\endcsname{0.65}
\expandafter\def\csname res@v8@phase_0.75_b50@pcmciplus@prec\endcsname{0.84}
\expandafter\def\csname res@v8@phase_0.75_b50@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@pcmciplus@len\endcsname{2.1}
\expandafter\def\csname res@v8@phase_0.75_b50@pcmciplus@rp\endcsname{0.89}
\expandafter\def\csname res@v8@phase_0.75_b50@pcmciplus@map\endcsname{0.93}
\expandafter\def\csname res@v8@phase_0.75_b50@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v8@phase_0.75_b50@pc@fpn\endcsname{3}
\expandafter\def\csname res@v8@phase_0.75_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@pc@tt\endcsname{0.58}
\expandafter\def\csname res@v8@phase_0.75_b50@pc@prec\endcsname{0.51}
\expandafter\def\csname res@v8@phase_0.75_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@pc@bw\endcsname{3}
\expandafter\def\csname res@v8@phase_0.75_b50@pc@len\endcsname{4.1}
\expandafter\def\csname res@v8@phase_0.75_b50@pc@rp\endcsname{0.43}
\expandafter\def\csname res@v8@phase_0.75_b50@pc@map\endcsname{0.42}
\expandafter\def\csname res@v8@phase_0.75_b50@dynotears@fp\endcsname{5/10}
\expandafter\def\csname res@v8@phase_0.75_b50@dynotears@fpn\endcsname{5}
\expandafter\def\csname res@v8@phase_0.75_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@dynotears@tt\endcsname{0.23}
\expandafter\def\csname res@v8@phase_0.75_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v8@phase_0.75_b50@dynotears@ab\endcsname{5}
\expandafter\def\csname res@v8@phase_0.75_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@dynotears@len\endcsname{0.6}
\expandafter\def\csname res@v8@phase_0.75_b50@dynotears@rp\endcsname{0.84}
\expandafter\def\csname res@v8@phase_0.75_b50@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v8@phase_0.75_b50@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v8@phase_0.75_b50@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v8@phase_0.75_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@doubleml@tt\endcsname{0.69}
\expandafter\def\csname res@v8@phase_0.75_b50@doubleml@prec\endcsname{0.73}
\expandafter\def\csname res@v8@phase_0.75_b50@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@doubleml@len\endcsname{3.1}
\expandafter\def\csname res@v8@phase_0.75_b50@doubleml@rp\endcsname{0.74}
\expandafter\def\csname res@v8@phase_0.75_b50@doubleml@map\endcsname{0.85}
\expandafter\def\csname res@v8@phase_0.75_b50@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v8@phase_0.75_b50@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@varlingam@tt\endcsname{0.62}
\expandafter\def\csname res@v8@phase_0.75_b50@varlingam@prec\endcsname{0.49}
\expandafter\def\csname res@v8@phase_0.75_b50@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@varlingam@len\endcsname{5.5}
\expandafter\def\csname res@v8@phase_0.75_b50@varlingam@rp\endcsname{0.59}
\expandafter\def\csname res@v8@phase_0.75_b50@varlingam@map\endcsname{0.73}
\expandafter\def\csname res@v8@phase_0.75_b50@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v8@phase_0.75_b50@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v8@phase_0.75_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@spacetime_rule@tt\endcsname{0.27}
\expandafter\def\csname res@v8@phase_0.75_b50@spacetime_rule@prec\endcsname{0.72}
\expandafter\def\csname res@v8@phase_0.75_b50@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_b50@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@spacetime_rule@len\endcsname{1.0}
\expandafter\def\csname res@v8@phase_0.75_b50@spacetime_rule@rp\endcsname{0.56}
\expandafter\def\csname res@v8@phase_0.75_b50@spacetime_rule@map\endcsname{0.63}
\expandafter\def\csname res@v8@phase_0.75_b50@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v8@phase_0.75_b50@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@varsort@tt\endcsname{0.12}
\expandafter\def\csname res@v8@phase_0.75_b50@varsort@prec\endcsname{0.10}
\expandafter\def\csname res@v8@phase_0.75_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@varsort@bw\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v8@phase_0.75_b50@varsort@rp\endcsname{0.12}
\expandafter\def\csname res@v8@phase_0.75_b50@varsort@map\endcsname{0.16}
\expandafter\def\csname res@v8@phase_0.75_b50@r2sort@fp\endcsname{2/10}
\expandafter\def\csname res@v8@phase_0.75_b50@r2sort@fpn\endcsname{2}
\expandafter\def\csname res@v8@phase_0.75_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v8@phase_0.75_b50@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v8@phase_0.75_b50@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v8@phase_0.75_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v8@phase_0.75_b50@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v8@phase_0.75_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v8@phase_0.75_b50@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v8@phase_0.75_b50@r2sort@map\endcsname{0.22}
\expandafter\def\csname res@v9@lot_0.25@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.25@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@correlation@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@correlation@tt\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.25@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v9@lot_0.25@correlation@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@correlation@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@correlation@len\endcsname{18.5}
\expandafter\def\csname res@v9@lot_0.25@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.25@correlation@map\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.25@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.25@granger@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@granger@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.25@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.25@granger@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@granger@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@granger@len\endcsname{17.1}
\expandafter\def\csname res@v9@lot_0.25@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v9@lot_0.25@granger@map\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.25@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.25@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.25@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@pcmciplus@tt\endcsname{0.73}
\expandafter\def\csname res@v9@lot_0.25@pcmciplus@prec\endcsname{0.79}
\expandafter\def\csname res@v9@lot_0.25@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v9@lot_0.25@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@pcmciplus@len\endcsname{2.6}
\expandafter\def\csname res@v9@lot_0.25@pcmciplus@rp\endcsname{0.95}
\expandafter\def\csname res@v9@lot_0.25@pcmciplus@map\endcsname{0.97}
\expandafter\def\csname res@v9@lot_0.25@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v9@lot_0.25@pc@fpn\endcsname{4}
\expandafter\def\csname res@v9@lot_0.25@pc@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@pc@tt\endcsname{0.42}
\expandafter\def\csname res@v9@lot_0.25@pc@prec\endcsname{0.35}
\expandafter\def\csname res@v9@lot_0.25@pc@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@pc@bw\endcsname{4}
\expandafter\def\csname res@v9@lot_0.25@pc@len\endcsname{5.1}
\expandafter\def\csname res@v9@lot_0.25@pc@rp\endcsname{0.35}
\expandafter\def\csname res@v9@lot_0.25@pc@map\endcsname{0.32}
\expandafter\def\csname res@v9@lot_0.25@dynotears@fp\endcsname{5/10}
\expandafter\def\csname res@v9@lot_0.25@dynotears@fpn\endcsname{5}
\expandafter\def\csname res@v9@lot_0.25@dynotears@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@dynotears@tt\endcsname{0.23}
\expandafter\def\csname res@v9@lot_0.25@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v9@lot_0.25@dynotears@ab\endcsname{5}
\expandafter\def\csname res@v9@lot_0.25@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@dynotears@len\endcsname{0.6}
\expandafter\def\csname res@v9@lot_0.25@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v9@lot_0.25@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v9@lot_0.25@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.25@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@doubleml@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v9@lot_0.25@doubleml@prec\endcsname{0.67}
\expandafter\def\csname res@v9@lot_0.25@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@doubleml@len\endcsname{3.7}
\expandafter\def\csname res@v9@lot_0.25@doubleml@rp\endcsname{0.88}
\expandafter\def\csname res@v9@lot_0.25@doubleml@map\endcsname{0.92}
\expandafter\def\csname res@v9@lot_0.25@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.25@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@varlingam@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v9@lot_0.25@varlingam@prec\endcsname{0.27}
\expandafter\def\csname res@v9@lot_0.25@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@varlingam@len\endcsname{9.9}
\expandafter\def\csname res@v9@lot_0.25@varlingam@rp\endcsname{0.71}
\expandafter\def\csname res@v9@lot_0.25@varlingam@map\endcsname{0.81}
\expandafter\def\csname res@v9@lot_0.25@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v9@lot_0.25@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v9@lot_0.25@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v9@lot_0.25@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v9@lot_0.25@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v9@lot_0.25@spacetime_rule@rp\endcsname{0.59}
\expandafter\def\csname res@v9@lot_0.25@spacetime_rule@map\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.25@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v9@lot_0.25@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v9@lot_0.25@varsort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@varsort@tt\endcsname{0.27}
\expandafter\def\csname res@v9@lot_0.25@varsort@prec\endcsname{0.23}
\expandafter\def\csname res@v9@lot_0.25@varsort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@varsort@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.25@varsort@rp\endcsname{0.17}
\expandafter\def\csname res@v9@lot_0.25@varsort@map\endcsname{0.22}
\expandafter\def\csname res@v9@lot_0.25@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.25@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.25@r2sort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.25@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.25@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v9@lot_0.25@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.25@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v9@lot_0.25@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.25@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v9@lot_0.25@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v9@lot_0.5@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.5@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@correlation@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v9@lot_0.5@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v9@lot_0.5@correlation@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@correlation@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v9@lot_0.5@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.5@correlation@map\endcsname{0.73}
\expandafter\def\csname res@v9@lot_0.5@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.5@granger@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@granger@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.5@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5@granger@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@granger@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@granger@len\endcsname{16.7}
\expandafter\def\csname res@v9@lot_0.5@granger@rp\endcsname{0.65}
\expandafter\def\csname res@v9@lot_0.5@granger@map\endcsname{0.76}
\expandafter\def\csname res@v9@lot_0.5@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.5@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@pcmciplus@tt\endcsname{0.69}
\expandafter\def\csname res@v9@lot_0.5@pcmciplus@prec\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.5@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@pcmciplus@len\endcsname{2.7}
\expandafter\def\csname res@v9@lot_0.5@pcmciplus@rp\endcsname{0.94}
\expandafter\def\csname res@v9@lot_0.5@pcmciplus@map\endcsname{0.98}
\expandafter\def\csname res@v9@lot_0.5@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v9@lot_0.5@pc@fpn\endcsname{4}
\expandafter\def\csname res@v9@lot_0.5@pc@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@pc@tt\endcsname{0.50}
\expandafter\def\csname res@v9@lot_0.5@pc@prec\endcsname{0.38}
\expandafter\def\csname res@v9@lot_0.5@pc@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@pc@bw\endcsname{4}
\expandafter\def\csname res@v9@lot_0.5@pc@len\endcsname{4.7}
\expandafter\def\csname res@v9@lot_0.5@pc@rp\endcsname{0.38}
\expandafter\def\csname res@v9@lot_0.5@pc@map\endcsname{0.33}
\expandafter\def\csname res@v9@lot_0.5@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v9@lot_0.5@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v9@lot_0.5@dynotears@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@dynotears@tt\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v9@lot_0.5@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v9@lot_0.5@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@dynotears@len\endcsname{0.4}
\expandafter\def\csname res@v9@lot_0.5@dynotears@rp\endcsname{0.85}
\expandafter\def\csname res@v9@lot_0.5@dynotears@map\endcsname{0.93}
\expandafter\def\csname res@v9@lot_0.5@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.5@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@doubleml@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v9@lot_0.5@doubleml@prec\endcsname{0.71}
\expandafter\def\csname res@v9@lot_0.5@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@doubleml@len\endcsname{3.5}
\expandafter\def\csname res@v9@lot_0.5@doubleml@rp\endcsname{0.88}
\expandafter\def\csname res@v9@lot_0.5@doubleml@map\endcsname{0.92}
\expandafter\def\csname res@v9@lot_0.5@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5@varlingam@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@varlingam@tt\endcsname{0.69}
\expandafter\def\csname res@v9@lot_0.5@varlingam@prec\endcsname{0.31}
\expandafter\def\csname res@v9@lot_0.5@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@varlingam@len\endcsname{10.5}
\expandafter\def\csname res@v9@lot_0.5@varlingam@rp\endcsname{0.67}
\expandafter\def\csname res@v9@lot_0.5@varlingam@map\endcsname{0.79}
\expandafter\def\csname res@v9@lot_0.5@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v9@lot_0.5@spacetime_rule@prec\endcsname{0.94}
\expandafter\def\csname res@v9@lot_0.5@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v9@lot_0.5@spacetime_rule@rp\endcsname{0.72}
\expandafter\def\csname res@v9@lot_0.5@spacetime_rule@map\endcsname{0.83}
\expandafter\def\csname res@v9@lot_0.5@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v9@lot_0.5@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v9@lot_0.5@varsort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v9@lot_0.5@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v9@lot_0.5@varsort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@varsort@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v9@lot_0.5@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.5@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5@r2sort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5@r2sort@tt\endcsname{0.08}
\expandafter\def\csname res@v9@lot_0.5@r2sort@prec\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.5@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v9@lot_0.5@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.5@r2sort@rp\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.5@r2sort@map\endcsname{0.19}
\expandafter\def\csname res@v9@lot_0.75@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.75@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.75@correlation@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v9@lot_0.75@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v9@lot_0.75@correlation@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@correlation@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.75@correlation@len\endcsname{18.7}
\expandafter\def\csname res@v9@lot_0.75@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.75@correlation@map\endcsname{0.71}
\expandafter\def\csname res@v9@lot_0.75@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.75@granger@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@granger@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v9@lot_0.75@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.75@granger@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@granger@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@granger@len\endcsname{16.6}
\expandafter\def\csname res@v9@lot_0.75@granger@rp\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.75@granger@map\endcsname{0.75}
\expandafter\def\csname res@v9@lot_0.75@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.75@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@pcmciplus@tt\endcsname{0.81}
\expandafter\def\csname res@v9@lot_0.75@pcmciplus@prec\endcsname{0.72}
\expandafter\def\csname res@v9@lot_0.75@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@pcmciplus@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.75@pcmciplus@rp\endcsname{0.97}
\expandafter\def\csname res@v9@lot_0.75@pcmciplus@map\endcsname{0.99}
\expandafter\def\csname res@v9@lot_0.75@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v9@lot_0.75@pc@fpn\endcsname{4}
\expandafter\def\csname res@v9@lot_0.75@pc@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@pc@tt\endcsname{0.50}
\expandafter\def\csname res@v9@lot_0.75@pc@prec\endcsname{0.38}
\expandafter\def\csname res@v9@lot_0.75@pc@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@pc@bw\endcsname{4}
\expandafter\def\csname res@v9@lot_0.75@pc@len\endcsname{5.2}
\expandafter\def\csname res@v9@lot_0.75@pc@rp\endcsname{0.38}
\expandafter\def\csname res@v9@lot_0.75@pc@map\endcsname{0.35}
\expandafter\def\csname res@v9@lot_0.75@dynotears@fp\endcsname{2/10}
\expandafter\def\csname res@v9@lot_0.75@dynotears@fpn\endcsname{2}
\expandafter\def\csname res@v9@lot_0.75@dynotears@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@dynotears@tt\endcsname{0.08}
\expandafter\def\csname res@v9@lot_0.75@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v9@lot_0.75@dynotears@ab\endcsname{8}
\expandafter\def\csname res@v9@lot_0.75@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@dynotears@len\endcsname{0.2}
\expandafter\def\csname res@v9@lot_0.75@dynotears@rp\endcsname{0.90}
\expandafter\def\csname res@v9@lot_0.75@dynotears@map\endcsname{0.93}
\expandafter\def\csname res@v9@lot_0.75@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.75@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@doubleml@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@doubleml@tt\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.75@doubleml@prec\endcsname{0.72}
\expandafter\def\csname res@v9@lot_0.75@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@doubleml@len\endcsname{3.6}
\expandafter\def\csname res@v9@lot_0.75@doubleml@rp\endcsname{0.80}
\expandafter\def\csname res@v9@lot_0.75@doubleml@map\endcsname{0.89}
\expandafter\def\csname res@v9@lot_0.75@varlingam@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.75@varlingam@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@varlingam@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@varlingam@tt\endcsname{0.65}
\expandafter\def\csname res@v9@lot_0.75@varlingam@prec\endcsname{0.32}
\expandafter\def\csname res@v9@lot_0.75@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@varlingam@len\endcsname{9.6}
\expandafter\def\csname res@v9@lot_0.75@varlingam@rp\endcsname{0.64}
\expandafter\def\csname res@v9@lot_0.75@varlingam@map\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.75@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.75@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.75@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@spacetime_rule@tt\endcsname{0.50}
\expandafter\def\csname res@v9@lot_0.75@spacetime_rule@prec\endcsname{0.94}
\expandafter\def\csname res@v9@lot_0.75@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v9@lot_0.75@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v9@lot_0.75@spacetime_rule@rp\endcsname{0.69}
\expandafter\def\csname res@v9@lot_0.75@spacetime_rule@map\endcsname{0.82}
\expandafter\def\csname res@v9@lot_0.75@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.75@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.75@varsort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v9@lot_0.75@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v9@lot_0.75@varsort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@varsort@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.75@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v9@lot_0.75@varsort@rp\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.75@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.75@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.75@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.75@r2sort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.75@r2sort@tt\endcsname{0.08}
\expandafter\def\csname res@v9@lot_0.75@r2sort@prec\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.75@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.75@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v9@lot_0.75@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.75@r2sort@rp\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.75@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v9@lot_0.9@correlation@fp\endcsname{7/10}
\expandafter\def\csname res@v9@lot_0.9@correlation@fpn\endcsname{7}
\expandafter\def\csname res@v9@lot_0.9@correlation@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@correlation@tt\endcsname{0.50}
\expandafter\def\csname res@v9@lot_0.9@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v9@lot_0.9@correlation@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@correlation@bw\endcsname{2}
\expandafter\def\csname res@v9@lot_0.9@correlation@len\endcsname{18.5}
\expandafter\def\csname res@v9@lot_0.9@correlation@rp\endcsname{0.58}
\expandafter\def\csname res@v9@lot_0.9@correlation@map\endcsname{0.67}
\expandafter\def\csname res@v9@lot_0.9@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.9@granger@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.9@granger@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@granger@tt\endcsname{0.54}
\expandafter\def\csname res@v9@lot_0.9@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.9@granger@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@granger@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@granger@len\endcsname{16.8}
\expandafter\def\csname res@v9@lot_0.9@granger@rp\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.9@granger@map\endcsname{0.71}
\expandafter\def\csname res@v9@lot_0.9@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.9@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@pcmciplus@tt\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.9@pcmciplus@prec\endcsname{0.87}
\expandafter\def\csname res@v9@lot_0.9@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@pcmciplus@len\endcsname{2.6}
\expandafter\def\csname res@v9@lot_0.9@pcmciplus@rp\endcsname{0.97}
\expandafter\def\csname res@v9@lot_0.9@pcmciplus@map\endcsname{0.99}
\expandafter\def\csname res@v9@lot_0.9@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v9@lot_0.9@pc@fpn\endcsname{4}
\expandafter\def\csname res@v9@lot_0.9@pc@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@pc@tt\endcsname{0.50}
\expandafter\def\csname res@v9@lot_0.9@pc@prec\endcsname{0.39}
\expandafter\def\csname res@v9@lot_0.9@pc@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@pc@bw\endcsname{4}
\expandafter\def\csname res@v9@lot_0.9@pc@len\endcsname{5.1}
\expandafter\def\csname res@v9@lot_0.9@pc@rp\endcsname{0.39}
\expandafter\def\csname res@v9@lot_0.9@pc@map\endcsname{0.35}
\expandafter\def\csname res@v9@lot_0.9@dynotears@fp\endcsname{3/10}
\expandafter\def\csname res@v9@lot_0.9@dynotears@fpn\endcsname{3}
\expandafter\def\csname res@v9@lot_0.9@dynotears@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@dynotears@tt\endcsname{0.12}
\expandafter\def\csname res@v9@lot_0.9@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v9@lot_0.9@dynotears@ab\endcsname{7}
\expandafter\def\csname res@v9@lot_0.9@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@dynotears@len\endcsname{0.3}
\expandafter\def\csname res@v9@lot_0.9@dynotears@rp\endcsname{0.90}
\expandafter\def\csname res@v9@lot_0.9@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v9@lot_0.9@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.9@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@doubleml@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@doubleml@tt\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.9@doubleml@prec\endcsname{0.74}
\expandafter\def\csname res@v9@lot_0.9@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@doubleml@len\endcsname{3.4}
\expandafter\def\csname res@v9@lot_0.9@doubleml@rp\endcsname{0.80}
\expandafter\def\csname res@v9@lot_0.9@doubleml@map\endcsname{0.89}
\expandafter\def\csname res@v9@lot_0.9@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.9@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.9@varlingam@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@varlingam@tt\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.9@varlingam@prec\endcsname{0.25}
\expandafter\def\csname res@v9@lot_0.9@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@varlingam@len\endcsname{10.8}
\expandafter\def\csname res@v9@lot_0.9@varlingam@rp\endcsname{0.60}
\expandafter\def\csname res@v9@lot_0.9@varlingam@map\endcsname{0.76}
\expandafter\def\csname res@v9@lot_0.9@spacetime_rule@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.9@spacetime_rule@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.9@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v9@lot_0.9@spacetime_rule@prec\endcsname{0.94}
\expandafter\def\csname res@v9@lot_0.9@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v9@lot_0.9@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@spacetime_rule@len\endcsname{1.2}
\expandafter\def\csname res@v9@lot_0.9@spacetime_rule@rp\endcsname{0.64}
\expandafter\def\csname res@v9@lot_0.9@spacetime_rule@map\endcsname{0.79}
\expandafter\def\csname res@v9@lot_0.9@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v9@lot_0.9@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v9@lot_0.9@varsort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@varsort@tt\endcsname{0.23}
\expandafter\def\csname res@v9@lot_0.9@varsort@prec\endcsname{0.20}
\expandafter\def\csname res@v9@lot_0.9@varsort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@varsort@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.9@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v9@lot_0.9@varsort@rp\endcsname{0.14}
\expandafter\def\csname res@v9@lot_0.9@varsort@map\endcsname{0.19}
\expandafter\def\csname res@v9@lot_0.9@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.9@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.9@r2sort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.9@r2sort@tt\endcsname{0.04}
\expandafter\def\csname res@v9@lot_0.9@r2sort@prec\endcsname{0.03}
\expandafter\def\csname res@v9@lot_0.9@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.9@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v9@lot_0.9@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.9@r2sort@rp\endcsname{0.05}
\expandafter\def\csname res@v9@lot_0.9@r2sort@map\endcsname{0.17}
\expandafter\def\csname res@v9@drift_0.1@correlation@fp\endcsname{10/10}
\expandafter\def\csname res@v9@drift_0.1@correlation@fpn\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@correlation@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v9@drift_0.1@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v9@drift_0.1@correlation@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@correlation@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@correlation@len\endcsname{18.6}
\expandafter\def\csname res@v9@drift_0.1@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v9@drift_0.1@correlation@map\endcsname{0.78}
\expandafter\def\csname res@v9@drift_0.1@granger@fp\endcsname{10/10}
\expandafter\def\csname res@v9@drift_0.1@granger@fpn\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@granger@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v9@drift_0.1@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v9@drift_0.1@granger@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@granger@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@granger@len\endcsname{17.2}
\expandafter\def\csname res@v9@drift_0.1@granger@rp\endcsname{0.68}
\expandafter\def\csname res@v9@drift_0.1@granger@map\endcsname{0.78}
\expandafter\def\csname res@v9@drift_0.1@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v9@drift_0.1@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v9@drift_0.1@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@pcmciplus@tt\endcsname{0.69}
\expandafter\def\csname res@v9@drift_0.1@pcmciplus@prec\endcsname{0.72}
\expandafter\def\csname res@v9@drift_0.1@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@pcmciplus@len\endcsname{2.6}
\expandafter\def\csname res@v9@drift_0.1@pcmciplus@rp\endcsname{0.87}
\expandafter\def\csname res@v9@drift_0.1@pcmciplus@map\endcsname{0.95}
\expandafter\def\csname res@v9@drift_0.1@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v9@drift_0.1@pc@fpn\endcsname{3}
\expandafter\def\csname res@v9@drift_0.1@pc@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@pc@tt\endcsname{0.35}
\expandafter\def\csname res@v9@drift_0.1@pc@prec\endcsname{0.34}
\expandafter\def\csname res@v9@drift_0.1@pc@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@pc@bw\endcsname{3}
\expandafter\def\csname res@v9@drift_0.1@pc@len\endcsname{5.3}
\expandafter\def\csname res@v9@drift_0.1@pc@rp\endcsname{0.34}
\expandafter\def\csname res@v9@drift_0.1@pc@map\endcsname{0.29}
\expandafter\def\csname res@v9@drift_0.1@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v9@drift_0.1@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v9@drift_0.1@dynotears@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@dynotears@tt\endcsname{0.27}
\expandafter\def\csname res@v9@drift_0.1@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v9@drift_0.1@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v9@drift_0.1@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v9@drift_0.1@dynotears@rp\endcsname{0.87}
\expandafter\def\csname res@v9@drift_0.1@dynotears@map\endcsname{0.94}
\expandafter\def\csname res@v9@drift_0.1@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v9@drift_0.1@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@doubleml@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@doubleml@tt\endcsname{0.85}
\expandafter\def\csname res@v9@drift_0.1@doubleml@prec\endcsname{0.73}
\expandafter\def\csname res@v9@drift_0.1@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@doubleml@len\endcsname{3.8}
\expandafter\def\csname res@v9@drift_0.1@doubleml@rp\endcsname{0.92}
\expandafter\def\csname res@v9@drift_0.1@doubleml@map\endcsname{0.93}
\expandafter\def\csname res@v9@drift_0.1@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v9@drift_0.1@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v9@drift_0.1@varlingam@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v9@drift_0.1@varlingam@prec\endcsname{0.25}
\expandafter\def\csname res@v9@drift_0.1@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@varlingam@len\endcsname{10.1}
\expandafter\def\csname res@v9@drift_0.1@varlingam@rp\endcsname{0.79}
\expandafter\def\csname res@v9@drift_0.1@varlingam@map\endcsname{0.87}
\expandafter\def\csname res@v9@drift_0.1@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v9@drift_0.1@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v9@drift_0.1@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v9@drift_0.1@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v9@drift_0.1@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v9@drift_0.1@spacetime_rule@rp\endcsname{0.59}
\expandafter\def\csname res@v9@drift_0.1@spacetime_rule@map\endcsname{0.77}
\expandafter\def\csname res@v9@drift_0.1@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@drift_0.1@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v9@drift_0.1@varsort@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v9@drift_0.1@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v9@drift_0.1@varsort@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@varsort@bw\endcsname{1}
\expandafter\def\csname res@v9@drift_0.1@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v9@drift_0.1@varsort@rp\endcsname{0.13}
\expandafter\def\csname res@v9@drift_0.1@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v9@drift_0.1@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@drift_0.1@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v9@drift_0.1@r2sort@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.1@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v9@drift_0.1@r2sort@prec\endcsname{0.13}
\expandafter\def\csname res@v9@drift_0.1@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.1@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v9@drift_0.1@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v9@drift_0.1@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v9@drift_0.1@r2sort@map\endcsname{0.21}
\expandafter\def\csname res@v9@drift_0.3@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v9@drift_0.3@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v9@drift_0.3@correlation@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v9@drift_0.3@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v9@drift_0.3@correlation@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@correlation@bw\endcsname{1}
\expandafter\def\csname res@v9@drift_0.3@correlation@len\endcsname{18.2}
\expandafter\def\csname res@v9@drift_0.3@correlation@rp\endcsname{0.59}
\expandafter\def\csname res@v9@drift_0.3@correlation@map\endcsname{0.71}
\expandafter\def\csname res@v9@drift_0.3@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v9@drift_0.3@granger@fpn\endcsname{9}
\expandafter\def\csname res@v9@drift_0.3@granger@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v9@drift_0.3@granger@prec\endcsname{0.14}
\expandafter\def\csname res@v9@drift_0.3@granger@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@granger@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@granger@len\endcsname{17.6}
\expandafter\def\csname res@v9@drift_0.3@granger@rp\endcsname{0.64}
\expandafter\def\csname res@v9@drift_0.3@granger@map\endcsname{0.76}
\expandafter\def\csname res@v9@drift_0.3@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v9@drift_0.3@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@pcmciplus@tt\endcsname{0.69}
\expandafter\def\csname res@v9@drift_0.3@pcmciplus@prec\endcsname{0.71}
\expandafter\def\csname res@v9@drift_0.3@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@pcmciplus@len\endcsname{2.8}
\expandafter\def\csname res@v9@drift_0.3@pcmciplus@rp\endcsname{0.87}
\expandafter\def\csname res@v9@drift_0.3@pcmciplus@map\endcsname{0.91}
\expandafter\def\csname res@v9@drift_0.3@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v9@drift_0.3@pc@fpn\endcsname{3}
\expandafter\def\csname res@v9@drift_0.3@pc@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@pc@tt\endcsname{0.38}
\expandafter\def\csname res@v9@drift_0.3@pc@prec\endcsname{0.37}
\expandafter\def\csname res@v9@drift_0.3@pc@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@pc@bw\endcsname{3}
\expandafter\def\csname res@v9@drift_0.3@pc@len\endcsname{5.3}
\expandafter\def\csname res@v9@drift_0.3@pc@rp\endcsname{0.37}
\expandafter\def\csname res@v9@drift_0.3@pc@map\endcsname{0.34}
\expandafter\def\csname res@v9@drift_0.3@dynotears@fp\endcsname{6/10}
\expandafter\def\csname res@v9@drift_0.3@dynotears@fpn\endcsname{6}
\expandafter\def\csname res@v9@drift_0.3@dynotears@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@dynotears@tt\endcsname{0.27}
\expandafter\def\csname res@v9@drift_0.3@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v9@drift_0.3@dynotears@ab\endcsname{4}
\expandafter\def\csname res@v9@drift_0.3@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@dynotears@len\endcsname{0.7}
\expandafter\def\csname res@v9@drift_0.3@dynotears@rp\endcsname{0.82}
\expandafter\def\csname res@v9@drift_0.3@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v9@drift_0.3@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v9@drift_0.3@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v9@drift_0.3@doubleml@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@doubleml@tt\endcsname{0.81}
\expandafter\def\csname res@v9@drift_0.3@doubleml@prec\endcsname{0.69}
\expandafter\def\csname res@v9@drift_0.3@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@doubleml@len\endcsname{3.8}
\expandafter\def\csname res@v9@drift_0.3@doubleml@rp\endcsname{0.86}
\expandafter\def\csname res@v9@drift_0.3@doubleml@map\endcsname{0.90}
\expandafter\def\csname res@v9@drift_0.3@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v9@drift_0.3@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v9@drift_0.3@varlingam@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v9@drift_0.3@varlingam@prec\endcsname{0.26}
\expandafter\def\csname res@v9@drift_0.3@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@varlingam@len\endcsname{10.0}
\expandafter\def\csname res@v9@drift_0.3@varlingam@rp\endcsname{0.79}
\expandafter\def\csname res@v9@drift_0.3@varlingam@map\endcsname{0.86}
\expandafter\def\csname res@v9@drift_0.3@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v9@drift_0.3@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v9@drift_0.3@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@spacetime_rule@tt\endcsname{0.42}
\expandafter\def\csname res@v9@drift_0.3@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v9@drift_0.3@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v9@drift_0.3@spacetime_rule@rp\endcsname{0.59}
\expandafter\def\csname res@v9@drift_0.3@spacetime_rule@map\endcsname{0.77}
\expandafter\def\csname res@v9@drift_0.3@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@drift_0.3@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v9@drift_0.3@varsort@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v9@drift_0.3@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v9@drift_0.3@varsort@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@varsort@bw\endcsname{2}
\expandafter\def\csname res@v9@drift_0.3@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v9@drift_0.3@varsort@rp\endcsname{0.10}
\expandafter\def\csname res@v9@drift_0.3@varsort@map\endcsname{0.14}
\expandafter\def\csname res@v9@drift_0.3@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@drift_0.3@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v9@drift_0.3@r2sort@n\endcsname{10}
\expandafter\def\csname res@v9@drift_0.3@r2sort@tt\endcsname{0.12}
\expandafter\def\csname res@v9@drift_0.3@r2sort@prec\endcsname{0.10}
\expandafter\def\csname res@v9@drift_0.3@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v9@drift_0.3@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v9@drift_0.3@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v9@drift_0.3@r2sort@rp\endcsname{0.07}
\expandafter\def\csname res@v9@drift_0.3@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@correlation@fp\endcsname{8/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@correlation@fpn\endcsname{8}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@correlation@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@correlation@tt\endcsname{0.54}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@correlation@prec\endcsname{0.14}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@correlation@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@correlation@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@correlation@len\endcsname{18.3}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@correlation@map\endcsname{0.70}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@granger@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@granger@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@granger@prec\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@granger@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@granger@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@granger@len\endcsname{16.9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@granger@rp\endcsname{0.64}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@granger@map\endcsname{0.74}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pcmciplus@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pcmciplus@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pcmciplus@tt\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pcmciplus@prec\endcsname{0.76}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pcmciplus@len\endcsname{2.9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pcmciplus@rp\endcsname{0.93}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pcmciplus@map\endcsname{0.94}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pc@fp\endcsname{4/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pc@fpn\endcsname{4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pc@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pc@tt\endcsname{0.46}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pc@prec\endcsname{0.39}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pc@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pc@bw\endcsname{4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pc@len\endcsname{5.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pc@rp\endcsname{0.39}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@pc@map\endcsname{0.37}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@dynotears@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@dynotears@tt\endcsname{0.19}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@dynotears@len\endcsname{0.5}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@dynotears@rp\endcsname{0.85}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@doubleml@fp\endcsname{10/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@doubleml@fpn\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@doubleml@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@doubleml@tt\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@doubleml@prec\endcsname{0.75}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@doubleml@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@doubleml@len\endcsname{3.2}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@doubleml@rp\endcsname{0.85}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@doubleml@map\endcsname{0.92}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varlingam@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varlingam@tt\endcsname{0.77}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varlingam@prec\endcsname{0.25}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varlingam@len\endcsname{10.2}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varlingam@rp\endcsname{0.74}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varlingam@map\endcsname{0.82}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@spacetime_rule@tt\endcsname{0.46}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@spacetime_rule@prec\endcsname{0.85}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@spacetime_rule@len\endcsname{1.4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@spacetime_rule@rp\endcsname{0.57}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@spacetime_rule@map\endcsname{0.75}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varsort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varsort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varsort@bw\endcsname{2}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varsort@len\endcsname{2.9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varsort@rp\endcsname{0.11}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@varsort@map\endcsname{0.21}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@r2sort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@r2sort@tt\endcsname{0.04}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@r2sort@prec\endcsname{0.03}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@r2sort@rp\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2@r2sort@map\endcsname{0.18}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@correlation@fp\endcsname{0/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@correlation@fpn\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@correlation@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@correlation@tt\endcsname{0.12}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@correlation@prec\endcsname{0.09}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@correlation@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@correlation@bw\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@correlation@len\endcsname{5.2}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@correlation@rp\endcsname{0.03}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@correlation@map\endcsname{0.26}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@granger@fp\endcsname{5/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@granger@fpn\endcsname{5}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@granger@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@granger@tt\endcsname{0.27}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@granger@prec\endcsname{0.28}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@granger@ab\endcsname{3}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@granger@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@granger@len\endcsname{4.1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@granger@rp\endcsname{0.47}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@granger@map\endcsname{0.57}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus@fp\endcsname{4/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus@fpn\endcsname{4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus@tt\endcsname{0.19}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus@prec\endcsname{0.67}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus@ab\endcsname{4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus@len\endcsname{0.8}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus@rp\endcsname{0.36}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus@map\endcsname{0.50}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pc@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pc@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pc@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pc@tt\endcsname{0.04}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pc@prec\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pc@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pc@bw\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pc@len\endcsname{2.4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pc@rp\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@pc@map\endcsname{0.18}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@dynotears@fp\endcsname{0/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@dynotears@fpn\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@dynotears@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@dynotears@tt\endcsname{0.00}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@dynotears@prec\endcsname{--}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@dynotears@ab\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@dynotears@len\endcsname{0.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@dynotears@rp\endcsname{0.49}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@dynotears@map\endcsname{0.58}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@doubleml@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@doubleml@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@doubleml@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@doubleml@tt\endcsname{0.04}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@doubleml@prec\endcsname{0.33}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@doubleml@ab\endcsname{7}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@doubleml@len\endcsname{0.3}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@doubleml@rp\endcsname{0.23}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@doubleml@map\endcsname{0.34}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varlingam@fp\endcsname{0/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varlingam@fpn\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varlingam@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varlingam@tt\endcsname{0.27}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varlingam@prec\endcsname{0.23}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varlingam@ab\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varlingam@bw\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varlingam@len\endcsname{4.8}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varlingam@rp\endcsname{0.20}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varlingam@map\endcsname{0.24}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule@fp\endcsname{4/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule@fpn\endcsname{4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule@tt\endcsname{0.27}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule@prec\endcsname{0.50}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule@len\endcsname{1.3}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule@rp\endcsname{0.34}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule@map\endcsname{0.46}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varsort@fp\endcsname{2/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varsort@fpn\endcsname{2}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varsort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varsort@tt\endcsname{0.19}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varsort@prec\endcsname{0.17}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varsort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varsort@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varsort@rp\endcsname{0.18}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@varsort@map\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@r2sort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@r2sort@tt\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@r2sort@prec\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@r2sort@len\endcsname{2.8}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@r2sort@rp\endcsname{0.11}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_combo_interaction@r2sort@map\endcsname{0.20}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@correlation@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@correlation@tt\endcsname{0.46}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@correlation@prec\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@correlation@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@correlation@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@correlation@len\endcsname{37.1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@correlation@rp\endcsname{0.47}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@correlation@map\endcsname{0.61}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@granger@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@granger@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@granger@tt\endcsname{0.58}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@granger@prec\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@granger@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@granger@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@granger@len\endcsname{34.9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@granger@rp\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@granger@map\endcsname{0.66}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pcmciplus@tt\endcsname{0.69}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pcmciplus@prec\endcsname{0.94}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pcmciplus@ab\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pcmciplus@len\endcsname{2.1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pcmciplus@rp\endcsname{0.90}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pcmciplus@map\endcsname{0.91}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pc@fp\endcsname{5/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pc@fpn\endcsname{5}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pc@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pc@tt\endcsname{0.31}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pc@prec\endcsname{0.36}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pc@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pc@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pc@len\endcsname{5.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pc@rp\endcsname{0.36}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@pc@map\endcsname{0.27}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@dynotears@fp\endcsname{4/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@dynotears@fpn\endcsname{4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@dynotears@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@dynotears@tt\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@dynotears@ab\endcsname{6}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@dynotears@len\endcsname{0.4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@dynotears@rp\endcsname{0.91}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@dynotears@map\endcsname{0.96}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@doubleml@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@doubleml@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@doubleml@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@doubleml@tt\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@doubleml@prec\endcsname{0.84}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@doubleml@ab\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@doubleml@len\endcsname{2.4}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@doubleml@rp\endcsname{0.67}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@doubleml@map\endcsname{0.76}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varlingam@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varlingam@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varlingam@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varlingam@tt\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varlingam@prec\endcsname{0.28}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varlingam@len\endcsname{10.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varlingam@rp\endcsname{0.60}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varlingam@map\endcsname{0.73}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@spacetime_rule@fp\endcsname{8/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@spacetime_rule@fpn\endcsname{8}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@spacetime_rule@tt\endcsname{0.31}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@spacetime_rule@prec\endcsname{0.80}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@spacetime_rule@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@spacetime_rule@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@spacetime_rule@len\endcsname{1.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@spacetime_rule@rp\endcsname{0.50}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@spacetime_rule@map\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varsort@fp\endcsname{0/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varsort@fpn\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varsort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varsort@tt\endcsname{0.00}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varsort@prec\endcsname{0.00}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varsort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varsort@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varsort@len\endcsname{2.8}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varsort@rp\endcsname{0.06}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@varsort@map\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@r2sort@fp\endcsname{0/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@r2sort@fpn\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@r2sort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@r2sort@tt\endcsname{0.00}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@r2sort@prec\endcsname{0.00}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@r2sort@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@r2sort@rp\endcsname{0.00}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_s40@r2sort@map\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@correlation@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@correlation@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@correlation@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@correlation@tt\endcsname{0.58}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@correlation@prec\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@correlation@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@correlation@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@correlation@len\endcsname{17.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@correlation@rp\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@correlation@map\endcsname{0.73}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@granger@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@granger@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@granger@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@granger@tt\endcsname{0.62}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@granger@prec\endcsname{0.29}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@granger@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@granger@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@granger@len\endcsname{11.6}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@granger@rp\endcsname{0.64}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@granger@map\endcsname{0.73}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pcmciplus@fp\endcsname{9/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pcmciplus@fpn\endcsname{9}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pcmciplus@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pcmciplus@tt\endcsname{0.65}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pcmciplus@prec\endcsname{0.95}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pcmciplus@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pcmciplus@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pcmciplus@len\endcsname{1.8}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pcmciplus@rp\endcsname{0.85}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pcmciplus@map\endcsname{0.86}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pc@fp\endcsname{3/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pc@fpn\endcsname{3}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pc@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pc@tt\endcsname{0.50}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pc@prec\endcsname{0.39}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pc@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pc@bw\endcsname{3}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pc@len\endcsname{4.7}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pc@rp\endcsname{0.39}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@pc@map\endcsname{0.33}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@dynotears@fp\endcsname{5/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@dynotears@fpn\endcsname{5}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@dynotears@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@dynotears@tt\endcsname{0.19}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@dynotears@prec\endcsname{1.00}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@dynotears@ab\endcsname{5}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@dynotears@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@dynotears@len\endcsname{0.5}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@dynotears@rp\endcsname{0.82}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@dynotears@map\endcsname{0.92}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@doubleml@fp\endcsname{6/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@doubleml@fpn\endcsname{6}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@doubleml@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@doubleml@tt\endcsname{0.46}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@doubleml@prec\endcsname{0.80}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@doubleml@ab\endcsname{3}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@doubleml@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@doubleml@len\endcsname{1.7}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@doubleml@rp\endcsname{0.65}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@doubleml@map\endcsname{0.76}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varlingam@fp\endcsname{7/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varlingam@fpn\endcsname{7}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varlingam@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varlingam@tt\endcsname{0.58}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varlingam@prec\endcsname{0.41}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varlingam@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varlingam@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varlingam@len\endcsname{5.8}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varlingam@rp\endcsname{0.51}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varlingam@map\endcsname{0.66}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@spacetime_rule@fp\endcsname{7/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@spacetime_rule@fpn\endcsname{7}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@spacetime_rule@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@spacetime_rule@tt\endcsname{0.27}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@spacetime_rule@prec\endcsname{0.72}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@spacetime_rule@ab\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@spacetime_rule@bw\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@spacetime_rule@len\endcsname{1.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@spacetime_rule@rp\endcsname{0.53}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@spacetime_rule@map\endcsname{0.63}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varsort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varsort@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varsort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varsort@tt\endcsname{0.15}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varsort@prec\endcsname{0.13}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varsort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varsort@bw\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varsort@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varsort@rp\endcsname{0.13}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@varsort@map\endcsname{0.19}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@r2sort@fp\endcsname{1/10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@r2sort@fpn\endcsname{1}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@r2sort@n\endcsname{10}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@r2sort@tt\endcsname{0.04}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@r2sort@prec\endcsname{0.03}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@r2sort@ab\endcsname{0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@r2sort@bw\endcsname{2}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@r2sort@len\endcsname{3.0}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@r2sort@rp\endcsname{0.07}
\expandafter\def\csname res@v9@lot_0.5_drift_0.2_b50@r2sort@map\endcsname{0.19}
\expandafter\def\csname cs@0@causes\endcsname{220}
\expandafter\def\csname cs@0@correlation\endcsname{12\%}
\expandafter\def\csname cs@0@granger\endcsname{15\%}
\expandafter\def\csname cs@0@pcmciplus\endcsname{10\%}
\expandafter\def\csname cs@0@pc\endcsname{9\%}
\expandafter\def\csname cs@0@dynotears\endcsname{0\%}
\expandafter\def\csname cs@0@doubleml\endcsname{15\%}
\expandafter\def\csname cs@0@spacetime_rule\endcsname{1\%}
\expandafter\def\csname cs@0@varlingam\endcsname{6\%}
\expandafter\def\csname cs@0@varsort\endcsname{33\%}
\expandafter\def\csname cs@0@r2sort\endcsname{8\%}
\expandafter\def\csname cs@1@causes\endcsname{685}
\expandafter\def\csname cs@1@correlation\endcsname{31\%}
\expandafter\def\csname cs@1@granger\endcsname{40\%}
\expandafter\def\csname cs@1@pcmciplus\endcsname{36\%}
\expandafter\def\csname cs@1@pc\endcsname{23\%}
\expandafter\def\csname cs@1@dynotears\endcsname{3\%}
\expandafter\def\csname cs@1@doubleml\endcsname{31\%}
\expandafter\def\csname cs@1@spacetime_rule\endcsname{5\%}
\expandafter\def\csname cs@1@varlingam\endcsname{35\%}
\expandafter\def\csname cs@1@varsort\endcsname{15\%}
\expandafter\def\csname cs@1@r2sort\endcsname{13\%}
\expandafter\def\csname cs@2@causes\endcsname{1165}
\expandafter\def\csname cs@2@correlation\endcsname{57\%}
\expandafter\def\csname cs@2@granger\endcsname{54\%}
\expandafter\def\csname cs@2@pcmciplus\endcsname{56\%}
\expandafter\def\csname cs@2@pc\endcsname{36\%}
\expandafter\def\csname cs@2@dynotears\endcsname{12\%}
\expandafter\def\csname cs@2@doubleml\endcsname{45\%}
\expandafter\def\csname cs@2@spacetime_rule\endcsname{26\%}
\expandafter\def\csname cs@2@varlingam\endcsname{57\%}
\expandafter\def\csname cs@2@varsort\endcsname{14\%}
\expandafter\def\csname cs@2@r2sort\endcsname{12\%}
\expandafter\def\csname cs@3@causes\endcsname{633}
\expandafter\def\csname cs@3@correlation\endcsname{57\%}
\expandafter\def\csname cs@3@granger\endcsname{68\%}
\expandafter\def\csname cs@3@pcmciplus\endcsname{64\%}
\expandafter\def\csname cs@3@pc\endcsname{33\%}
\expandafter\def\csname cs@3@dynotears\endcsname{29\%}
\expandafter\def\csname cs@3@doubleml\endcsname{50\%}
\expandafter\def\csname cs@3@spacetime_rule\endcsname{69\%}
\expandafter\def\csname cs@3@varlingam\endcsname{58\%}
\expandafter\def\csname cs@3@varsort\endcsname{8\%}
\expandafter\def\csname cs@3@r2sort\endcsname{13\%}
\newcommand{\LabRefWrong}{164}
\newcommand{\LabRefAnc}{63}
\newcommand{\LabRefNonCause}{78}
\newcommand{\LabRefConf}{78}
\newcommand{\LabRefDesc}{23}
\newcommand{\LabRefIdCond}{141}
\newcommand{\LabRefIdTime}{23}
\newcommand{\LabRefIdNo}{0}
\newcommand{\LabRefExactCond}{0}
\newcommand{\LabRefInst}{10}
\newcommand{\LabRefConfPairs}{189}
\newcommand{\LabRefPairs}{190}
\newcommand{\LabRefVars}{20}
\newcommand{\LabRefNodes}{210}
\newcommand{\LabMeasWrong}{164}
\newcommand{\LabMeasAnc}{63}
\newcommand{\LabMeasNonCause}{78}
\newcommand{\LabMeasConf}{78}
\newcommand{\LabMeasDesc}{23}
\newcommand{\LabMeasIdCond}{0}
\newcommand{\LabMeasIdTime}{23}
\newcommand{\LabMeasIdNo}{141}
\newcommand{\LabMeasExactCond}{141}
\newcommand{\LabMeasInst}{10}
\newcommand{\LabMeasConfPairs}{189}
\newcommand{\LabMeasPairs}{190}
\newcommand{\LabMeasVars}{20}
\newcommand{\LabMeasNodes}{210}
\newcommand{\Pool}[2]{\ifcsname pool@#1@#2\endcsname\csname pool@#1@#2\endcsname\else\PackageError{numbers}{missing pooled #1/#2}{}\fi}
\expandafter\def\csname pool@correlation@fp\endcsname{0.64}
\expandafter\def\csname pool@correlation@fpans\endcsname{0.64}
\expandafter\def\csname pool@correlation@ab\endcsname{0.00}
\expandafter\def\csname pool@correlation@bw\endcsname{0.33}
\expandafter\def\csname pool@correlation@n\endcsname{1190}
\expandafter\def\csname pool@granger@fp\endcsname{0.79}
\expandafter\def\csname pool@granger@fpans\endcsname{0.87}
\expandafter\def\csname pool@granger@ab\endcsname{0.10}
\expandafter\def\csname pool@granger@bw\endcsname{0.01}
\expandafter\def\csname pool@granger@n\endcsname{1190}
\expandafter\def\csname pool@pcmciplus@fp\endcsname{0.78}
\expandafter\def\csname pool@pcmciplus@fpans\endcsname{0.87}
\expandafter\def\csname pool@pcmciplus@ab\endcsname{0.10}
\expandafter\def\csname pool@pcmciplus@bw\endcsname{0.01}
\expandafter\def\csname pool@pcmciplus@n\endcsname{1190}
\expandafter\def\csname pool@pc@fp\endcsname{0.25}
\expandafter\def\csname pool@pc@fpans\endcsname{0.25}
\expandafter\def\csname pool@pc@ab\endcsname{0.00}
\expandafter\def\csname pool@pc@bw\endcsname{0.44}
\expandafter\def\csname pool@pc@n\endcsname{1190}
\expandafter\def\csname pool@dynotears@fp\endcsname{0.28}
\expandafter\def\csname pool@dynotears@fpans\endcsname{1.00}
\expandafter\def\csname pool@dynotears@ab\endcsname{0.72}
\expandafter\def\csname pool@dynotears@bw\endcsname{0.00}
\expandafter\def\csname pool@dynotears@n\endcsname{1190}
\expandafter\def\csname pool@doubleml@fp\endcsname{0.67}
\expandafter\def\csname pool@doubleml@fpans\endcsname{0.92}
\expandafter\def\csname pool@doubleml@ab\endcsname{0.27}
\expandafter\def\csname pool@doubleml@bw\endcsname{0.01}
\expandafter\def\csname pool@doubleml@n\endcsname{1190}
\expandafter\def\csname pool@spacetime_rule@fp\endcsname{0.63}
\expandafter\def\csname pool@spacetime_rule@fpans\endcsname{0.74}
\expandafter\def\csname pool@spacetime_rule@ab\endcsname{0.16}
\expandafter\def\csname pool@spacetime_rule@bw\endcsname{0.02}
\expandafter\def\csname pool@spacetime_rule@n\endcsname{1190}
\expandafter\def\csname pool@varlingam@fp\endcsname{0.66}
\expandafter\def\csname pool@varlingam@fpans\endcsname{0.69}
\expandafter\def\csname pool@varlingam@ab\endcsname{0.05}
\expandafter\def\csname pool@varlingam@bw\endcsname{0.23}
\expandafter\def\csname pool@varlingam@n\endcsname{1190}
\expandafter\def\csname pool@varsort@fp\endcsname{0.09}
\expandafter\def\csname pool@varsort@fpans\endcsname{0.09}
\expandafter\def\csname pool@varsort@ab\endcsname{0.00}
\expandafter\def\csname pool@varsort@bw\endcsname{0.11}
\expandafter\def\csname pool@varsort@n\endcsname{1190}
\expandafter\def\csname pool@r2sort@fp\endcsname{0.06}
\expandafter\def\csname pool@r2sort@fpans\endcsname{0.06}
\expandafter\def\csname pool@r2sort@ab\endcsname{0.00}
\expandafter\def\csname pool@r2sort@bw\endcsname{0.12}
\expandafter\def\csname pool@r2sort@n\endcsname{1190}
\newcommand{\Err}[2]{\ifcsname err@#1@#2\endcsname\csname err@#1@#2\endcsname\else\PackageError{numbers}{missing error #1/#2}{}\fi}
\expandafter\def\csname err@correlation@sel\endcsname{16.7}
\expandafter\def\csname err@correlation@wrong\endcsname{14.4}
\expandafter\def\csname err@correlation@time\endcsname{15\%}
\expandafter\def\csname err@correlation@look_alike\endcsname{7.1}
\expandafter\def\csname err@correlation@upstream\endcsname{4.4}
\expandafter\def\csname err@correlation@upstream_loop\endcsname{0.8}
\expandafter\def\csname err@correlation@downstream\endcsname{2.2}
\expandafter\def\csname err@doubleml@sel\endcsname{2.1}
\expandafter\def\csname err@doubleml@wrong\endcsname{0.7}
\expandafter\def\csname err@doubleml@time\endcsname{4\%}
\expandafter\def\csname err@doubleml@look_alike\endcsname{0.2}
\expandafter\def\csname err@doubleml@upstream\endcsname{0.2}
\expandafter\def\csname err@doubleml@upstream_loop\endcsname{0.2}
\expandafter\def\csname err@doubleml@downstream\endcsname{0.0}
\expandafter\def\csname err@dynotears@sel\endcsname{0.4}
\expandafter\def\csname err@dynotears@wrong\endcsname{0.0}
\expandafter\def\csname err@dynotears@time\endcsname{0\%}
\expandafter\def\csname err@dynotears@look_alike\endcsname{0.0}
\expandafter\def\csname err@dynotears@upstream\endcsname{0.0}
\expandafter\def\csname err@dynotears@upstream_loop\endcsname{0.0}
\expandafter\def\csname err@dynotears@downstream\endcsname{0.0}
\expandafter\def\csname err@granger@sel\endcsname{13.5}
\expandafter\def\csname err@granger@wrong\endcsname{11.4}
\expandafter\def\csname err@granger@time\endcsname{11\%}
\expandafter\def\csname err@granger@look_alike\endcsname{5.7}
\expandafter\def\csname err@granger@upstream\endcsname{3.8}
\expandafter\def\csname err@granger@upstream_loop\endcsname{0.7}
\expandafter\def\csname err@granger@downstream\endcsname{1.3}
\expandafter\def\csname err@pc@sel\endcsname{4.3}
\expandafter\def\csname err@pc@wrong\endcsname{3.0}
\expandafter\def\csname err@pc@time\endcsname{57\%}
\expandafter\def\csname err@pc@look_alike\endcsname{0.7}
\expandafter\def\csname err@pc@upstream\endcsname{0.5}
\expandafter\def\csname err@pc@upstream_loop\endcsname{0.1}
\expandafter\def\csname err@pc@downstream\endcsname{1.7}
\expandafter\def\csname err@pcmciplus@sel\endcsname{2.2}
\expandafter\def\csname err@pcmciplus@wrong\endcsname{0.7}
\expandafter\def\csname err@pcmciplus@time\endcsname{10\%}
\expandafter\def\csname err@pcmciplus@look_alike\endcsname{0.2}
\expandafter\def\csname err@pcmciplus@upstream\endcsname{0.3}
\expandafter\def\csname err@pcmciplus@upstream_loop\endcsname{0.1}
\expandafter\def\csname err@pcmciplus@downstream\endcsname{0.1}
\expandafter\def\csname err@spacetime_rule@sel\endcsname{1.1}
\expandafter\def\csname err@spacetime_rule@wrong\endcsname{0.3}
\expandafter\def\csname err@spacetime_rule@time\endcsname{3\%}
\expandafter\def\csname err@spacetime_rule@look_alike\endcsname{0.1}
\expandafter\def\csname err@spacetime_rule@upstream\endcsname{0.1}
\expandafter\def\csname err@spacetime_rule@upstream_loop\endcsname{0.1}
\expandafter\def\csname err@spacetime_rule@downstream\endcsname{0.0}
\expandafter\def\csname err@varlingam@sel\endcsname{7.5}
\expandafter\def\csname err@varlingam@wrong\endcsname{5.7}
\expandafter\def\csname err@varlingam@time\endcsname{22\%}
\expandafter\def\csname err@varlingam@look_alike\endcsname{2.4}
\expandafter\def\csname err@varlingam@upstream\endcsname{1.5}
\expandafter\def\csname err@varlingam@upstream_loop\endcsname{0.4}
\expandafter\def\csname err@varlingam@downstream\endcsname{1.3}
\newcommand{\ErrSettledCells}{102}
\newcommand{\ErrUnsettledCells}{17}
\newcommand{\ErrCandWrong}{19423}
\newcommand{\ErrCandId}{19423}
\newcommand{\ErrUWrong}{3388}
\newcommand{\ErrUNo}{1722}
\newcommand{\NCells}{119}
\newcommand{\NCellsOther}{118}
\newcommand{\NCausesScored}{2703}
\makeatother


==> generated/numbers_errors.tex <==
\makeatletter
\newcommand{\ErrT}[2]{\ifcsname errt@#1@#2\endcsname\csname errt@#1@#2\endcsname\else\PackageError{numbers}{missing error-table #1/#2}{}\fi}
\expandafter\def\csname errt@correlation@right\endcsname{64\%}
\expandafter\def\csname errt@correlation@back\endcsname{33\%}
\expandafter\def\csname errt@correlation@anc\endcsname{1\%}
\expandafter\def\csname errt@correlation@none\endcsname{0\%}
\expandafter\def\csname errt@correlation@len\endcsname{16.9}
\expandafter\def\csname errt@correlation@lift\endcsname{1.0}
\expandafter\def\csname errt@correlation@look_alike\endcsname{7.0}
\expandafter\def\csname errt@correlation@upstream\endcsname{4.4}
\expandafter\def\csname errt@correlation@upstream_loop\endcsname{0.8}
\expandafter\def\csname errt@correlation@downstream\endcsname{2.4}
\expandafter\def\csname errt@granger@right\endcsname{79\%}
\expandafter\def\csname errt@granger@back\endcsname{1\%}
\expandafter\def\csname errt@granger@anc\endcsname{8\%}
\expandafter\def\csname errt@granger@none\endcsname{10\%}
\expandafter\def\csname errt@granger@len\endcsname{13.7}
\expandafter\def\csname errt@granger@lift\endcsname{1.2}
\expandafter\def\csname errt@granger@look_alike\endcsname{5.7}
\expandafter\def\csname errt@granger@upstream\endcsname{3.8}
\expandafter\def\csname errt@granger@upstream_loop\endcsname{0.7}
\expandafter\def\csname errt@granger@downstream\endcsname{1.4}
\expandafter\def\csname errt@varlingam@right\endcsname{66\%}
\expandafter\def\csname errt@varlingam@back\endcsname{23\%}
\expandafter\def\csname errt@varlingam@anc\endcsname{3\%}
\expandafter\def\csname errt@varlingam@none\endcsname{5\%}
\expandafter\def\csname errt@varlingam@len\endcsname{7.6}
\expandafter\def\csname errt@varlingam@lift\endcsname{1.9}
\expandafter\def\csname errt@varlingam@look_alike\endcsname{2.4}
\expandafter\def\csname errt@varlingam@upstream\endcsname{1.6}
\expandafter\def\csname errt@varlingam@upstream_loop\endcsname{0.5}
\expandafter\def\csname errt@varlingam@downstream\endcsname{1.3}
\expandafter\def\csname errt@dynotears@right\endcsname{28\%}
\expandafter\def\csname errt@dynotears@back\endcsname{0\%}
\expandafter\def\csname errt@dynotears@anc\endcsname{0\%}
\expandafter\def\csname errt@dynotears@none\endcsname{72\%}
\expandafter\def\csname errt@dynotears@len\endcsname{0.4}
\expandafter\def\csname errt@dynotears@lift\endcsname{7.8}
\expandafter\def\csname errt@dynotears@look_alike\endcsname{0.0}
\expandafter\def\csname errt@dynotears@upstream\endcsname{0.0}
\expandafter\def\csname errt@dynotears@upstream_loop\endcsname{0.0}
\expandafter\def\csname errt@dynotears@downstream\endcsname{0.0}
\expandafter\def\csname errt@pc@right\endcsname{25\%}
\expandafter\def\csname errt@pc@back\endcsname{44\%}
\expandafter\def\csname errt@pc@anc\endcsname{14\%}
\expandafter\def\csname errt@pc@none\endcsname{0\%}
\expandafter\def\csname errt@pc@len\endcsname{4.5}
\expandafter\def\csname errt@pc@lift\endcsname{2.4}
\expandafter\def\csname errt@pc@look_alike\endcsname{0.8}
\expandafter\def\csname errt@pc@upstream\endcsname{0.6}
\expandafter\def\csname errt@pc@upstream_loop\endcsname{0.1}
\expandafter\def\csname errt@pc@downstream\endcsname{1.7}
\expandafter\def\csname errt@pcmciplus@right\endcsname{78\%}
\expandafter\def\csname errt@pcmciplus@back\endcsname{1\%}
\expandafter\def\csname errt@pcmciplus@anc\endcsname{6\%}
\expandafter\def\csname errt@pcmciplus@none\endcsname{10\%}
\expandafter\def\csname errt@pcmciplus@len\endcsname{2.4}
\expandafter\def\csname errt@pcmciplus@lift\endcsname{5.2}
\expandafter\def\csname errt@pcmciplus@look_alike\endcsname{0.3}
\expandafter\def\csname errt@pcmciplus@upstream\endcsname{0.3}
\expandafter\def\csname errt@pcmciplus@upstream_loop\endcsname{0.1}
\expandafter\def\csname errt@pcmciplus@downstream\endcsname{0.1}
\expandafter\def\csname errt@spacetime_rule@right\endcsname{63\%}
\expandafter\def\csname errt@spacetime_rule@back\endcsname{2\%}
\expandafter\def\csname errt@spacetime_rule@anc\endcsname{10\%}
\expandafter\def\csname errt@spacetime_rule@none\endcsname{16\%}
\expandafter\def\csname errt@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname errt@spacetime_rule@lift\endcsname{5.8}
\expandafter\def\csname errt@spacetime_rule@look_alike\endcsname{0.1}
\expandafter\def\csname errt@spacetime_rule@upstream\endcsname{0.1}
\expandafter\def\csname errt@spacetime_rule@upstream_loop\endcsname{0.1}
\expandafter\def\csname errt@spacetime_rule@downstream\endcsname{0.0}
\expandafter\def\csname errt@doubleml@right\endcsname{67\%}
\expandafter\def\csname errt@doubleml@back\endcsname{1\%}
\expandafter\def\csname errt@doubleml@anc\endcsname{3\%}
\expandafter\def\csname errt@doubleml@none\endcsname{27\%}
\expandafter\def\csname errt@doubleml@len\endcsname{2.2}
\expandafter\def\csname errt@doubleml@lift\endcsname{5.2}
\expandafter\def\csname errt@doubleml@look_alike\endcsname{0.2}
\expandafter\def\csname errt@doubleml@upstream\endcsname{0.3}
\expandafter\def\csname errt@doubleml@upstream_loop\endcsname{0.2}
\expandafter\def\csname errt@doubleml@downstream\endcsname{0.0}
\expandafter\def\csname errt@pool@downstream\endcsname{13\%}
\expandafter\def\csname errt@pool@upstream_loop\endcsname{5\%}
\expandafter\def\csname errt@pool@upstream\endcsname{31\%}
\expandafter\def\csname errt@pool@look_alike\endcsname{51\%}
\expandafter\def\csname errt@correlation@wpp\endcsname{14.7}
\expandafter\def\csname errt@correlation@fwrong\endcsname{36\%}
\expandafter\def\csname errt@correlation@enr_downstream\endcsname{1.2$\times$\,{\tiny(16\%)}}
\expandafter\def\csname errt@correlation@enr_downstream_x\endcsname{1.2$\times$}
\expandafter\def\csname errt@correlation@enr_downstream_pct\endcsname{16\%}
\expandafter\def\csname errt@correlation@fw_downstream\endcsname{7.0$\times$\,{\tiny(92\%)}}
\expandafter\def\csname errt@correlation@fw_downstream_x\endcsname{7.0$\times$}
\expandafter\def\csname errt@correlation@fw_downstream_pct\endcsname{92\%}
\expandafter\def\csname errt@correlation@enr_upstream_loop\endcsname{1.1$\times$\,{\tiny(5\%)}}
\expandafter\def\csname errt@correlation@enr_upstream_loop_x\endcsname{1.1$\times$}
\expandafter\def\csname errt@correlation@enr_upstream_loop_pct\endcsname{5\%}
\expandafter\def\csname errt@correlation@fw_upstream_loop\endcsname{0.0$\times$\,{\tiny(0\%)}}
\expandafter\def\csname errt@correlation@fw_upstream_loop_x\endcsname{0.0$\times$}
\expandafter\def\csname errt@correlation@fw_upstream_loop_pct\endcsname{0\%}
\expandafter\def\csname errt@correlation@enr_upstream\endcsname{1.0$\times$\,{\tiny(30\%)}}
\expandafter\def\csname errt@correlation@enr_upstream_x\endcsname{1.0$\times$}
\expandafter\def\csname errt@correlation@enr_upstream_pct\endcsname{30\%}
\expandafter\def\csname errt@correlation@fw_upstream\endcsname{0.1$\times$\,{\tiny(4\%)}}
\expandafter\def\csname errt@correlation@fw_upstream_x\endcsname{0.1$\times$}
\expandafter\def\csname errt@correlation@fw_upstream_pct\endcsname{4\%}
\expandafter\def\csname errt@correlation@enr_look_alike\endcsname{0.9$\times$\,{\tiny(48\%)}}
\expandafter\def\csname errt@correlation@enr_look_alike_x\endcsname{0.9$\times$}
\expandafter\def\csname errt@correlation@enr_look_alike_pct\endcsname{48\%}
\expandafter\def\csname errt@correlation@fw_look_alike\endcsname{0.1$\times$\,{\tiny(4\%)}}
\expandafter\def\csname errt@correlation@fw_look_alike_x\endcsname{0.1$\times$}
\expandafter\def\csname errt@correlation@fw_look_alike_pct\endcsname{4\%}
\expandafter\def\csname errt@granger@wpp\endcsname{11.6}
\expandafter\def\csname errt@granger@fwrong\endcsname{12\%}
\expandafter\def\csname errt@granger@enr_downstream\endcsname{0.9$\times$\,{\tiny(12\%)}}
\expandafter\def\csname errt@granger@enr_downstream_x\endcsname{0.9$\times$}
\expandafter\def\csname errt@granger@enr_downstream_pct\endcsname{12\%}
\expandafter\def\csname errt@granger@fw_downstream\endcsname{0.5$\times$\,{\tiny(7\%)}}
\expandafter\def\csname errt@granger@fw_downstream_x\endcsname{0.5$\times$}
\expandafter\def\csname errt@granger@fw_downstream_pct\endcsname{7\%}
\expandafter\def\csname errt@granger@enr_upstream_loop\endcsname{1.3$\times$\,{\tiny(6\%)}}
\expandafter\def\csname errt@granger@enr_upstream_loop_x\endcsname{1.3$\times$}
\expandafter\def\csname errt@granger@enr_upstream_loop_pct\endcsname{6\%}
\expandafter\def\csname errt@granger@fw_upstream_loop\endcsname{1.3$\times$\,{\tiny(7\%)}}
\expandafter\def\csname errt@granger@fw_upstream_loop_x\endcsname{1.3$\times$}
\expandafter\def\csname errt@granger@fw_upstream_loop_pct\endcsname{7\%}
\expandafter\def\csname errt@granger@enr_upstream\endcsname{1.1$\times$\,{\tiny(33\%)}}
\expandafter\def\csname errt@granger@enr_upstream_x\endcsname{1.1$\times$}
\expandafter\def\csname errt@granger@enr_upstream_pct\endcsname{33\%}
\expandafter\def\csname errt@granger@fw_upstream\endcsname{1.9$\times$\,{\tiny(59\%)}}
\expandafter\def\csname errt@granger@fw_upstream_x\endcsname{1.9$\times$}
\expandafter\def\csname errt@granger@fw_upstream_pct\endcsname{59\%}
\expandafter\def\csname errt@granger@enr_look_alike\endcsname{0.9$\times$\,{\tiny(49\%)}}
\expandafter\def\csname errt@granger@enr_look_alike_x\endcsname{0.9$\times$}
\expandafter\def\csname errt@granger@enr_look_alike_pct\endcsname{49\%}
\expandafter\def\csname errt@granger@fw_look_alike\endcsname{0.5$\times$\,{\tiny(28\%)}}
\expandafter\def\csname errt@granger@fw_look_alike_x\endcsname{0.5$\times$}
\expandafter\def\csname errt@granger@fw_look_alike_pct\endcsname{28\%}
\expandafter\def\csname errt@varlingam@wpp\endcsname{5.7}
\expandafter\def\csname errt@varlingam@fwrong\endcsname{29\%}
\expandafter\def\csname errt@varlingam@enr_downstream\endcsname{1.7$\times$\,{\tiny(23\%)}}
\expandafter\def\csname errt@varlingam@enr_downstream_x\endcsname{1.7$\times$}
\expandafter\def\csname errt@varlingam@enr_downstream_pct\endcsname{23\%}
\expandafter\def\csname errt@varlingam@fw_downstream\endcsname{5.8$\times$\,{\tiny(77\%)}}
\expandafter\def\csname errt@varlingam@fw_downstream_x\endcsname{5.8$\times$}
\expandafter\def\csname errt@varlingam@fw_downstream_pct\endcsname{77\%}
\expandafter\def\csname errt@varlingam@enr_upstream_loop\endcsname{1.6$\times$\,{\tiny(8\%)}}
\expandafter\def\csname errt@varlingam@enr_upstream_loop_x\endcsname{1.6$\times$}
\expandafter\def\csname errt@varlingam@enr_upstream_loop_pct\endcsname{8\%}
\expandafter\def\csname errt@varlingam@fw_upstream_loop\endcsname{0.4$\times$\,{\tiny(2\%)}}
\expandafter\def\csname errt@varlingam@fw_upstream_loop_x\endcsname{0.4$\times$}
\expandafter\def\csname errt@varlingam@fw_upstream_loop_pct\endcsname{2\%}
\expandafter\def\csname errt@varlingam@enr_upstream\endcsname{0.9$\times$\,{\tiny(28\%)}}
\expandafter\def\csname errt@varlingam@enr_upstream_x\endcsname{0.9$\times$}
\expandafter\def\csname errt@varlingam@enr_upstream_pct\endcsname{28\%}
\expandafter\def\csname errt@varlingam@fw_upstream\endcsname{0.3$\times$\,{\tiny(10\%)}}
\expandafter\def\csname errt@varlingam@fw_upstream_x\endcsname{0.3$\times$}
\expandafter\def\csname errt@varlingam@fw_upstream_pct\endcsname{10\%}
\expandafter\def\csname errt@varlingam@enr_look_alike\endcsname{0.8$\times$\,{\tiny(42\%)}}
\expandafter\def\csname errt@varlingam@enr_look_alike_x\endcsname{0.8$\times$}
\expandafter\def\csname errt@varlingam@enr_look_alike_pct\endcsname{42\%}
\expandafter\def\csname errt@varlingam@fw_look_alike\endcsname{0.2$\times$\,{\tiny(11\%)}}
\expandafter\def\csname errt@varlingam@fw_look_alike_x\endcsname{0.2$\times$}
\expandafter\def\csname errt@varlingam@fw_look_alike_pct\endcsname{11\%}
\expandafter\def\csname errt@dynotears@wpp\endcsname{0.0}
\expandafter\def\csname errt@dynotears@fwrong\endcsname{0\%}
\expandafter\def\csname errt@dynotears@enr_downstream\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_downstream_x\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_downstream_pct\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_downstream\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_downstream_x\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_downstream_pct\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_upstream_loop\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_upstream_loop_x\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_upstream_loop_pct\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_upstream_loop\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_upstream_loop_x\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_upstream_loop_pct\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_upstream\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_upstream_x\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_upstream_pct\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_upstream\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_upstream_x\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_upstream_pct\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_look_alike\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_look_alike_x\endcsname{--}
\expandafter\def\csname errt@dynotears@enr_look_alike_pct\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_look_alike\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_look_alike_x\endcsname{--}
\expandafter\def\csname errt@dynotears@fw_look_alike_pct\endcsname{--}
\expandafter\def\csname errt@pc@wpp\endcsname{3.2}
\expandafter\def\csname errt@pc@fwrong\endcsname{75\%}
\expandafter\def\csname errt@pc@enr_downstream\endcsname{4.1$\times$\,{\tiny(55\%)}}
\expandafter\def\csname errt@pc@enr_downstream_x\endcsname{4.1$\times$}
\expandafter\def\csname errt@pc@enr_downstream_pct\endcsname{55\%}
\expandafter\def\csname errt@pc@fw_downstream\endcsname{4.4$\times$\,{\tiny(59\%)}}
\expandafter\def\csname errt@pc@fw_downstream_x\endcsname{4.4$\times$}
\expandafter\def\csname errt@pc@fw_downstream_pct\endcsname{59\%}
\expandafter\def\csname errt@pc@enr_upstream_loop\endcsname{0.5$\times$\,{\tiny(2\%)}}
\expandafter\def\csname errt@pc@enr_upstream_loop_x\endcsname{0.5$\times$}
\expandafter\def\csname errt@pc@enr_upstream_loop_pct\endcsname{2\%}
\expandafter\def\csname errt@pc@fw_upstream_loop\endcsname{0.1$\times$\,{\tiny(1\%)}}
\expandafter\def\csname errt@pc@fw_upstream_loop_x\endcsname{0.1$\times$}
\expandafter\def\csname errt@pc@fw_upstream_loop_pct\endcsname{1\%}
\expandafter\def\csname errt@pc@enr_upstream\endcsname{0.6$\times$\,{\tiny(18\%)}}
\expandafter\def\csname errt@pc@enr_upstream_x\endcsname{0.6$\times$}
\expandafter\def\csname errt@pc@enr_upstream_pct\endcsname{18\%}
\expandafter\def\csname errt@pc@fw_upstream\endcsname{0.6$\times$\,{\tiny(19\%)}}
\expandafter\def\csname errt@pc@fw_upstream_x\endcsname{0.6$\times$}
\expandafter\def\csname errt@pc@fw_upstream_pct\endcsname{19\%}
\expandafter\def\csname errt@pc@enr_look_alike\endcsname{0.5$\times$\,{\tiny(25\%)}}
\expandafter\def\csname errt@pc@enr_look_alike_x\endcsname{0.5$\times$}
\expandafter\def\csname errt@pc@enr_look_alike_pct\endcsname{25\%}
\expandafter\def\csname errt@pc@fw_look_alike\endcsname{0.4$\times$\,{\tiny(22\%)}}
\expandafter\def\csname errt@pc@fw_look_alike_x\endcsname{0.4$\times$}
\expandafter\def\csname errt@pc@fw_look_alike_pct\endcsname{22\%}
\expandafter\def\csname errt@pcmciplus@wpp\endcsname{0.8}
\expandafter\def\csname errt@pcmciplus@fwrong\endcsname{12\%}
\expandafter\def\csname errt@pcmciplus@enr_downstream\endcsname{0.9$\times$\,{\tiny(12\%)}}
\expandafter\def\csname errt@pcmciplus@enr_downstream_x\endcsname{0.9$\times$}
\expandafter\def\csname errt@pcmciplus@enr_downstream_pct\endcsname{12\%}
\expandafter\def\csname errt@pcmciplus@fw_downstream\endcsname{0.8$\times$\,{\tiny(10\%)}}
\expandafter\def\csname errt@pcmciplus@fw_downstream_x\endcsname{0.8$\times$}
\expandafter\def\csname errt@pcmciplus@fw_downstream_pct\endcsname{10\%}
\expandafter\def\csname errt@pcmciplus@enr_upstream_loop\endcsname{2.8$\times$\,{\tiny(14\%)}}
\expandafter\def\csname errt@pcmciplus@enr_upstream_loop_x\endcsname{2.8$\times$}
\expandafter\def\csname errt@pcmciplus@enr_upstream_loop_pct\endcsname{14\%}
\expandafter\def\csname errt@pcmciplus@fw_upstream_loop\endcsname{2.9$\times$\,{\tiny(14\%)}}
\expandafter\def\csname errt@pcmciplus@fw_upstream_loop_x\endcsname{2.9$\times$}
\expandafter\def\csname errt@pcmciplus@fw_upstream_loop_pct\endcsname{14\%}
\expandafter\def\csname errt@pcmciplus@enr_upstream\endcsname{1.3$\times$\,{\tiny(40\%)}}
\expandafter\def\csname errt@pcmciplus@enr_upstream_x\endcsname{1.3$\times$}
\expandafter\def\csname errt@pcmciplus@enr_upstream_pct\endcsname{40\%}
\expandafter\def\csname errt@pcmciplus@fw_upstream\endcsname{1.2$\times$\,{\tiny(36\%)}}
\expandafter\def\csname errt@pcmciplus@fw_upstream_x\endcsname{1.2$\times$}
\expandafter\def\csname errt@pcmciplus@fw_upstream_pct\endcsname{36\%}
\expandafter\def\csname errt@pcmciplus@enr_look_alike\endcsname{0.7$\times$\,{\tiny(35\%)}}
\expandafter\def\csname errt@pcmciplus@enr_look_alike_x\endcsname{0.7$\times$}
\expandafter\def\csname errt@pcmciplus@enr_look_alike_pct\endcsname{35\%}
\expandafter\def\csname errt@pcmciplus@fw_look_alike\endcsname{0.8$\times$\,{\tiny(39\%)}}
\expandafter\def\csname errt@pcmciplus@fw_look_alike_x\endcsname{0.8$\times$}
\expandafter\def\csname errt@pcmciplus@fw_look_alike_pct\endcsname{39\%}
\expandafter\def\csname errt@spacetime_rule@wpp\endcsname{0.3}
\expandafter\def\csname errt@spacetime_rule@fwrong\endcsname{22\%}
\expandafter\def\csname errt@spacetime_rule@enr_downstream\endcsname{0.4$\times$\,{\tiny(5\%)}}
\expandafter\def\csname errt@spacetime_rule@enr_downstream_x\endcsname{0.4$\times$}
\expandafter\def\csname errt@spacetime_rule@enr_downstream_pct\endcsname{5\%}
\expandafter\def\csname errt@spacetime_rule@fw_downstream\endcsname{0.5$\times$\,{\tiny(7\%)}}
\expandafter\def\csname errt@spacetime_rule@fw_downstream_x\endcsname{0.5$\times$}
\expandafter\def\csname errt@spacetime_rule@fw_downstream_pct\endcsname{7\%}
\expandafter\def\csname errt@spacetime_rule@enr_upstream_loop\endcsname{3.7$\times$\,{\tiny(18\%)}}
\expandafter\def\csname errt@spacetime_rule@enr_upstream_loop_x\endcsname{3.7$\times$}
\expandafter\def\csname errt@spacetime_rule@enr_upstream_loop_pct\endcsname{18\%}
\expandafter\def\csname errt@spacetime_rule@fw_upstream_loop\endcsname{3.0$\times$\,{\tiny(15\%)}}
\expandafter\def\csname errt@spacetime_rule@fw_upstream_loop_x\endcsname{3.0$\times$}
\expandafter\def\csname errt@spacetime_rule@fw_upstream_loop_pct\endcsname{15\%}
\expandafter\def\csname errt@spacetime_rule@enr_upstream\endcsname{1.1$\times$\,{\tiny(33\%)}}
\expandafter\def\csname errt@spacetime_rule@enr_upstream_x\endcsname{1.1$\times$}
\expandafter\def\csname errt@spacetime_rule@enr_upstream_pct\endcsname{33\%}
\expandafter\def\csname errt@spacetime_rule@fw_upstream\endcsname{1.1$\times$\,{\tiny(33\%)}}
\expandafter\def\csname errt@spacetime_rule@fw_upstream_x\endcsname{1.1$\times$}
\expandafter\def\csname errt@spacetime_rule@fw_upstream_pct\endcsname{33\%}
\expandafter\def\csname errt@spacetime_rule@enr_look_alike\endcsname{0.9$\times$\,{\tiny(44\%)}}
\expandafter\def\csname errt@spacetime_rule@enr_look_alike_x\endcsname{0.9$\times$}
\expandafter\def\csname errt@spacetime_rule@enr_look_alike_pct\endcsname{44\%}
\expandafter\def\csname errt@spacetime_rule@fw_look_alike\endcsname{0.9$\times$\,{\tiny(45\%)}}
\expandafter\def\csname errt@spacetime_rule@fw_look_alike_x\endcsname{0.9$\times$}
\expandafter\def\csname errt@spacetime_rule@fw_look_alike_pct\endcsname{45\%}
\expandafter\def\csname errt@doubleml@wpp\endcsname{0.7}
\expandafter\def\csname errt@doubleml@fwrong\endcsname{6\%}
\expandafter\def\csname errt@doubleml@enr_downstream\endcsname{0.5$\times$\,{\tiny(6\%)}}
\expandafter\def\csname errt@doubleml@enr_downstream_x\endcsname{0.5$\times$}
\expandafter\def\csname errt@doubleml@enr_downstream_pct\endcsname{6\%}
\expandafter\def\csname errt@doubleml@fw_downstream\endcsname{0.8$\times$\,{\tiny(11\%)}}
\expandafter\def\csname errt@doubleml@fw_downstream_x\endcsname{0.8$\times$}
\expandafter\def\csname errt@doubleml@fw_downstream_pct\endcsname{11\%}
\expandafter\def\csname errt@doubleml@enr_upstream_loop\endcsname{5.8$\times$\,{\tiny(28\%)}}
\expandafter\def\csname errt@doubleml@enr_upstream_loop_x\endcsname{5.8$\times$}
\expandafter\def\csname errt@doubleml@enr_upstream_loop_pct\endcsname{28\%}
\expandafter\def\csname errt@doubleml@fw_upstream_loop\endcsname{1.4$\times$\,{\tiny(7\%)}}
\expandafter\def\csname errt@doubleml@fw_upstream_loop_x\endcsname{1.4$\times$}
\expandafter\def\csname errt@doubleml@fw_upstream_loop_pct\endcsname{7\%}
\expandafter\def\csname errt@doubleml@enr_upstream\endcsname{1.2$\times$\,{\tiny(36\%)}}
\expandafter\def\csname errt@doubleml@enr_upstream_x\endcsname{1.2$\times$}
\expandafter\def\csname errt@doubleml@enr_upstream_pct\endcsname{36\%}
\expandafter\def\csname errt@doubleml@fw_upstream\endcsname{1.5$\times$\,{\tiny(44\%)}}
\expandafter\def\csname errt@doubleml@fw_upstream_x\endcsname{1.5$\times$}
\expandafter\def\csname errt@doubleml@fw_upstream_pct\endcsname{44\%}
\expandafter\def\csname errt@doubleml@enr_look_alike\endcsname{0.6$\times$\,{\tiny(30\%)}}
\expandafter\def\csname errt@doubleml@enr_look_alike_x\endcsname{0.6$\times$}
\expandafter\def\csname errt@doubleml@enr_look_alike_pct\endcsname{30\%}
\expandafter\def\csname errt@doubleml@fw_look_alike\endcsname{0.7$\times$\,{\tiny(38\%)}}
\expandafter\def\csname errt@doubleml@fw_look_alike_x\endcsname{0.7$\times$}
\expandafter\def\csname errt@doubleml@fw_look_alike_pct\endcsname{38\%}
\newcommand{\ErrTPlants}{1,190}
\makeatother


==> generated/numbers_lists.tex <==
\makeatletter
\newcommand{\Lift}[3]{\ifcsname lift@#1@#2@#3\endcsname\csname lift@#1@#2@#3\endcsname\else\PackageError{numbers}{missing Lift #1/#2/#3}{}\fi}
\newcommand{\Len}[3]{\ifcsname len@#1@#2@#3\endcsname\csname len@#1@#2@#3\endcsname\else\PackageError{numbers}{missing Len #1/#2/#3}{}\fi}
\newcommand{\Found}[3]{\ifcsname found@#1@#2@#3\endcsname\csname found@#1@#2@#3\endcsname\else\PackageError{numbers}{missing Found #1/#2/#3}{}\fi}
\newcommand{\Beyond}[3]{\ifcsname beyond@#1@#2@#3\endcsname\csname beyond@#1@#2@#3\endcsname\else\PackageError{numbers}{missing Beyond #1/#2/#3}{}\fi}
\expandafter\def\csname lift@v4@default@correlation\endcsname{1.1}
\expandafter\def\csname len@v4@default@correlation\endcsname{18.0}
\expandafter\def\csname found@v4@default@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@default@correlation\endcsname{0.05}
\expandafter\def\csname lift@v4@default@granger\endcsname{1.1}
\expandafter\def\csname len@v4@default@granger\endcsname{17.0}
\expandafter\def\csname found@v4@default@granger\endcsname{2.6}
\expandafter\def\csname beyond@v4@default@granger\endcsname{0.10}
\expandafter\def\csname lift@v4@default@pcmciplus\endcsname{5.6}
\expandafter\def\csname len@v4@default@pcmciplus\endcsname{2.5}
\expandafter\def\csname found@v4@default@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v4@default@pcmciplus\endcsname{0.59}
\expandafter\def\csname lift@v4@default@pc\endcsname{2.4}
\expandafter\def\csname len@v4@default@pc\endcsname{5.5}
\expandafter\def\csname found@v4@default@pc\endcsname{1.8}
\expandafter\def\csname beyond@v4@default@pc\endcsname{0.39}
\expandafter\def\csname lift@v4@default@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4@default@dynotears\endcsname{0.6}
\expandafter\def\csname found@v4@default@dynotears\endcsname{0.6}
\expandafter\def\csname beyond@v4@default@dynotears\endcsname{0.20}
\expandafter\def\csname lift@v4@default@varlingam\endcsname{1.7}
\expandafter\def\csname len@v4@default@varlingam\endcsname{10.0}
\expandafter\def\csname found@v4@default@varlingam\endcsname{2.3}
\expandafter\def\csname beyond@v4@default@varlingam\endcsname{0.36}
\expandafter\def\csname lift@v4@default@doubleml\endcsname{4.7}
\expandafter\def\csname len@v4@default@doubleml\endcsname{3.7}
\expandafter\def\csname found@v4@default@doubleml\endcsname{2.4}
\expandafter\def\csname beyond@v4@default@doubleml\endcsname{0.70}
\expandafter\def\csname lift@v4@default@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v4@default@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v4@default@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v4@default@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v4@signal_0.4@correlation\endcsname{1.1}
\expandafter\def\csname len@v4@signal_0.4@correlation\endcsname{17.7}
\expandafter\def\csname found@v4@signal_0.4@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@signal_0.4@correlation\endcsname{0.07}
\expandafter\def\csname lift@v4@signal_0.4@granger\endcsname{1.1}
\expandafter\def\csname len@v4@signal_0.4@granger\endcsname{15.8}
\expandafter\def\csname found@v4@signal_0.4@granger\endcsname{2.4}
\expandafter\def\csname beyond@v4@signal_0.4@granger\endcsname{0.10}
\expandafter\def\csname lift@v4@signal_0.4@pcmciplus\endcsname{5.9}
\expandafter\def\csname len@v4@signal_0.4@pcmciplus\endcsname{2.6}
\expandafter\def\csname found@v4@signal_0.4@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v4@signal_0.4@pcmciplus\endcsname{0.67}
\expandafter\def\csname lift@v4@signal_0.4@pc\endcsname{2.5}
\expandafter\def\csname len@v4@signal_0.4@pc\endcsname{4.6}
\expandafter\def\csname found@v4@signal_0.4@pc\endcsname{1.6}
\expandafter\def\csname beyond@v4@signal_0.4@pc\endcsname{0.36}
\expandafter\def\csname lift@v4@signal_0.4@dynotears\endcsname{--}
\expandafter\def\csname len@v4@signal_0.4@dynotears\endcsname{0.0}
\expandafter\def\csname found@v4@signal_0.4@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v4@signal_0.4@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v4@signal_0.4@varlingam\endcsname{1.8}
\expandafter\def\csname len@v4@signal_0.4@varlingam\endcsname{9.3}
\expandafter\def\csname found@v4@signal_0.4@varlingam\endcsname{2.3}
\expandafter\def\csname beyond@v4@signal_0.4@varlingam\endcsname{0.39}
\expandafter\def\csname lift@v4@signal_0.4@doubleml\endcsname{5.0}
\expandafter\def\csname len@v4@signal_0.4@doubleml\endcsname{3.1}
\expandafter\def\csname found@v4@signal_0.4@doubleml\endcsname{2.1}
\expandafter\def\csname beyond@v4@signal_0.4@doubleml\endcsname{0.63}
\expandafter\def\csname lift@v4@signal_0.4@spacetime_rule\endcsname{5.2}
\expandafter\def\csname len@v4@signal_0.4@spacetime_rule\endcsname{0.7}
\expandafter\def\csname found@v4@signal_0.4@spacetime_rule\endcsname{0.5}
\expandafter\def\csname beyond@v4@signal_0.4@spacetime_rule\endcsname{0.16}
\expandafter\def\csname lift@v4@signal_0.9@correlation\endcsname{1.0}
\expandafter\def\csname len@v4@signal_0.9@correlation\endcsname{18.3}
\expandafter\def\csname found@v4@signal_0.9@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@signal_0.9@correlation\endcsname{0.03}
\expandafter\def\csname lift@v4@signal_0.9@granger\endcsname{1.1}
\expandafter\def\csname len@v4@signal_0.9@granger\endcsname{17.1}
\expandafter\def\csname found@v4@signal_0.9@granger\endcsname{2.5}
\expandafter\def\csname beyond@v4@signal_0.9@granger\endcsname{0.06}
\expandafter\def\csname lift@v4@signal_0.9@pcmciplus\endcsname{5.1}
\expandafter\def\csname len@v4@signal_0.9@pcmciplus\endcsname{3.0}
\expandafter\def\csname found@v4@signal_0.9@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v4@signal_0.9@pcmciplus\endcsname{0.63}
\expandafter\def\csname lift@v4@signal_0.9@pc\endcsname{2.5}
\expandafter\def\csname len@v4@signal_0.9@pc\endcsname{5.5}
\expandafter\def\csname found@v4@signal_0.9@pc\endcsname{1.9}
\expandafter\def\csname beyond@v4@signal_0.9@pc\endcsname{0.42}
\expandafter\def\csname lift@v4@signal_0.9@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4@signal_0.9@dynotears\endcsname{1.2}
\expandafter\def\csname found@v4@signal_0.9@dynotears\endcsname{1.2}
\expandafter\def\csname beyond@v4@signal_0.9@dynotears\endcsname{0.39}
\expandafter\def\csname lift@v4@signal_0.9@varlingam\endcsname{1.6}
\expandafter\def\csname len@v4@signal_0.9@varlingam\endcsname{11.9}
\expandafter\def\csname found@v4@signal_0.9@varlingam\endcsname{2.6}
\expandafter\def\csname beyond@v4@signal_0.9@varlingam\endcsname{0.35}
\expandafter\def\csname lift@v4@signal_0.9@doubleml\endcsname{4.9}
\expandafter\def\csname len@v4@signal_0.9@doubleml\endcsname{3.6}
\expandafter\def\csname found@v4@signal_0.9@doubleml\endcsname{2.4}
\expandafter\def\csname beyond@v4@signal_0.9@doubleml\endcsname{0.70}
\expandafter\def\csname lift@v4@signal_0.9@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v4@signal_0.9@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v4@signal_0.9@spacetime_rule\endcsname{1.3}
\expandafter\def\csname beyond@v4@signal_0.9@spacetime_rule\endcsname{0.42}
\expandafter\def\csname lift@v4@confound_0.1@correlation\endcsname{1.0}
\expandafter\def\csname len@v4@confound_0.1@correlation\endcsname{18.2}
\expandafter\def\csname found@v4@confound_0.1@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@confound_0.1@correlation\endcsname{0.04}
\expandafter\def\csname lift@v4@confound_0.1@granger\endcsname{1.1}
\expandafter\def\csname len@v4@confound_0.1@granger\endcsname{17.6}
\expandafter\def\csname found@v4@confound_0.1@granger\endcsname{2.6}
\expandafter\def\csname beyond@v4@confound_0.1@granger\endcsname{0.07}
\expandafter\def\csname lift@v4@confound_0.1@pcmciplus\endcsname{5.0}
\expandafter\def\csname len@v4@confound_0.1@pcmciplus\endcsname{3.5}
\expandafter\def\csname found@v4@confound_0.1@pcmciplus\endcsname{2.4}
\expandafter\def\csname beyond@v4@confound_0.1@pcmciplus\endcsname{0.73}
\expandafter\def\csname lift@v4@confound_0.1@pc\endcsname{2.6}
\expandafter\def\csname len@v4@confound_0.1@pc\endcsname{5.3}
\expandafter\def\csname found@v4@confound_0.1@pc\endcsname{1.9}
\expandafter\def\csname beyond@v4@confound_0.1@pc\endcsname{0.43}
\expandafter\def\csname lift@v4@confound_0.1@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4@confound_0.1@dynotears\endcsname{0.8}
\expandafter\def\csname found@v4@confound_0.1@dynotears\endcsname{0.8}
\expandafter\def\csname beyond@v4@confound_0.1@dynotears\endcsname{0.26}
\expandafter\def\csname lift@v4@confound_0.1@varlingam\endcsname{1.6}
\expandafter\def\csname len@v4@confound_0.1@varlingam\endcsname{12.0}
\expandafter\def\csname found@v4@confound_0.1@varlingam\endcsname{2.6}
\expandafter\def\csname beyond@v4@confound_0.1@varlingam\endcsname{0.35}
\expandafter\def\csname lift@v4@confound_0.1@doubleml\endcsname{4.8}
\expandafter\def\csname len@v4@confound_0.1@doubleml\endcsname{3.8}
\expandafter\def\csname found@v4@confound_0.1@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v4@confound_0.1@doubleml\endcsname{0.73}
\expandafter\def\csname lift@v4@confound_0.1@spacetime_rule\endcsname{6.6}
\expandafter\def\csname len@v4@confound_0.1@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v4@confound_0.1@spacetime_rule\endcsname{1.0}
\expandafter\def\csname beyond@v4@confound_0.1@spacetime_rule\endcsname{0.33}
\expandafter\def\csname lift@v4@confound_0.6@correlation\endcsname{1.0}
\expandafter\def\csname len@v4@confound_0.6@correlation\endcsname{18.3}
\expandafter\def\csname found@v4@confound_0.6@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@confound_0.6@correlation\endcsname{0.03}
\expandafter\def\csname lift@v4@confound_0.6@granger\endcsname{1.1}
\expandafter\def\csname len@v4@confound_0.6@granger\endcsname{16.2}
\expandafter\def\csname found@v4@confound_0.6@granger\endcsname{2.4}
\expandafter\def\csname beyond@v4@confound_0.6@granger\endcsname{0.08}
\expandafter\def\csname lift@v4@confound_0.6@pcmciplus\endcsname{5.8}
\expandafter\def\csname len@v4@confound_0.6@pcmciplus\endcsname{2.4}
\expandafter\def\csname found@v4@confound_0.6@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v4@confound_0.6@pcmciplus\endcsname{0.59}
\expandafter\def\csname lift@v4@confound_0.6@pc\endcsname{2.4}
\expandafter\def\csname len@v4@confound_0.6@pc\endcsname{5.4}
\expandafter\def\csname found@v4@confound_0.6@pc\endcsname{1.8}
\expandafter\def\csname beyond@v4@confound_0.6@pc\endcsname{0.40}
\expandafter\def\csname lift@v4@confound_0.6@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4@confound_0.6@dynotears\endcsname{0.4}
\expandafter\def\csname found@v4@confound_0.6@dynotears\endcsname{0.4}
\expandafter\def\csname beyond@v4@confound_0.6@dynotears\endcsname{0.13}
\expandafter\def\csname lift@v4@confound_0.6@varlingam\endcsname{1.9}
\expandafter\def\csname len@v4@confound_0.6@varlingam\endcsname{9.6}
\expandafter\def\csname found@v4@confound_0.6@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v4@confound_0.6@varlingam\endcsname{0.44}
\expandafter\def\csname lift@v4@confound_0.6@doubleml\endcsname{4.6}
\expandafter\def\csname len@v4@confound_0.6@doubleml\endcsname{3.8}
\expandafter\def\csname found@v4@confound_0.6@doubleml\endcsname{2.4}
\expandafter\def\csname beyond@v4@confound_0.6@doubleml\endcsname{0.70}
\expandafter\def\csname lift@v4@confound_0.6@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v4@confound_0.6@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v4@confound_0.6@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v4@confound_0.6@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v4@conseq_0.1@correlation\endcsname{1.0}
\expandafter\def\csname len@v4@conseq_0.1@correlation\endcsname{18.1}
\expandafter\def\csname found@v4@conseq_0.1@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@conseq_0.1@correlation\endcsname{0.04}
\expandafter\def\csname lift@v4@conseq_0.1@granger\endcsname{1.1}
\expandafter\def\csname len@v4@conseq_0.1@granger\endcsname{17.2}
\expandafter\def\csname found@v4@conseq_0.1@granger\endcsname{2.5}
\expandafter\def\csname beyond@v4@conseq_0.1@granger\endcsname{0.05}
\expandafter\def\csname lift@v4@conseq_0.1@pcmciplus\endcsname{5.7}
\expandafter\def\csname len@v4@conseq_0.1@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v4@conseq_0.1@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v4@conseq_0.1@pcmciplus\endcsname{0.65}
\expandafter\def\csname lift@v4@conseq_0.1@pc\endcsname{2.5}
\expandafter\def\csname len@v4@conseq_0.1@pc\endcsname{5.2}
\expandafter\def\csname found@v4@conseq_0.1@pc\endcsname{1.8}
\expandafter\def\csname beyond@v4@conseq_0.1@pc\endcsname{0.40}
\expandafter\def\csname lift@v4@conseq_0.1@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4@conseq_0.1@dynotears\endcsname{0.7}
\expandafter\def\csname found@v4@conseq_0.1@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v4@conseq_0.1@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v4@conseq_0.1@varlingam\endcsname{1.8}
\expandafter\def\csname len@v4@conseq_0.1@varlingam\endcsname{10.0}
\expandafter\def\csname found@v4@conseq_0.1@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v4@conseq_0.1@varlingam\endcsname{0.43}
\expandafter\def\csname lift@v4@conseq_0.1@doubleml\endcsname{4.5}
\expandafter\def\csname len@v4@conseq_0.1@doubleml\endcsname{4.1}
\expandafter\def\csname found@v4@conseq_0.1@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v4@conseq_0.1@doubleml\endcsname{0.72}
\expandafter\def\csname lift@v4@conseq_0.1@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v4@conseq_0.1@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v4@conseq_0.1@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v4@conseq_0.1@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v4@conseq_0.5@correlation\endcsname{1.0}
\expandafter\def\csname len@v4@conseq_0.5@correlation\endcsname{18.2}
\expandafter\def\csname found@v4@conseq_0.5@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@conseq_0.5@correlation\endcsname{0.04}
\expandafter\def\csname lift@v4@conseq_0.5@granger\endcsname{1.1}
\expandafter\def\csname len@v4@conseq_0.5@granger\endcsname{17.1}
\expandafter\def\csname found@v4@conseq_0.5@granger\endcsname{2.5}
\expandafter\def\csname beyond@v4@conseq_0.5@granger\endcsname{0.06}
\expandafter\def\csname lift@v4@conseq_0.5@pcmciplus\endcsname{5.5}
\expandafter\def\csname len@v4@conseq_0.5@pcmciplus\endcsname{2.8}
\expandafter\def\csname found@v4@conseq_0.5@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v4@conseq_0.5@pcmciplus\endcsname{0.65}
\expandafter\def\csname lift@v4@conseq_0.5@pc\endcsname{2.7}
\expandafter\def\csname len@v4@conseq_0.5@pc\endcsname{5.2}
\expandafter\def\csname found@v4@conseq_0.5@pc\endcsname{1.9}
\expandafter\def\csname beyond@v4@conseq_0.5@pc\endcsname{0.44}
\expandafter\def\csname lift@v4@conseq_0.5@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4@conseq_0.5@dynotears\endcsname{0.7}
\expandafter\def\csname found@v4@conseq_0.5@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v4@conseq_0.5@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v4@conseq_0.5@varlingam\endcsname{1.7}
\expandafter\def\csname len@v4@conseq_0.5@varlingam\endcsname{10.8}
\expandafter\def\csname found@v4@conseq_0.5@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v4@conseq_0.5@varlingam\endcsname{0.36}
\expandafter\def\csname lift@v4@conseq_0.5@doubleml\endcsname{4.7}
\expandafter\def\csname len@v4@conseq_0.5@doubleml\endcsname{3.9}
\expandafter\def\csname found@v4@conseq_0.5@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v4@conseq_0.5@doubleml\endcsname{0.73}
\expandafter\def\csname lift@v4@conseq_0.5@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v4@conseq_0.5@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v4@conseq_0.5@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v4@conseq_0.5@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v4@echo_0.1@correlation\endcsname{1.1}
\expandafter\def\csname len@v4@echo_0.1@correlation\endcsname{17.7}
\expandafter\def\csname found@v4@echo_0.1@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@echo_0.1@correlation\endcsname{0.07}
\expandafter\def\csname lift@v4@echo_0.1@granger\endcsname{1.1}
\expandafter\def\csname len@v4@echo_0.1@granger\endcsname{17.1}
\expandafter\def\csname found@v4@echo_0.1@granger\endcsname{2.5}
\expandafter\def\csname beyond@v4@echo_0.1@granger\endcsname{0.06}
\expandafter\def\csname lift@v4@echo_0.1@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v4@echo_0.1@pcmciplus\endcsname{3.1}
\expandafter\def\csname found@v4@echo_0.1@pcmciplus\endcsname{2.3}
\expandafter\def\csname beyond@v4@echo_0.1@pcmciplus\endcsname{0.70}
\expandafter\def\csname lift@v4@echo_0.1@pc\endcsname{2.8}
\expandafter\def\csname len@v4@echo_0.1@pc\endcsname{5.0}
\expandafter\def\csname found@v4@echo_0.1@pc\endcsname{1.9}
\expandafter\def\csname beyond@v4@echo_0.1@pc\endcsname{0.45}
\expandafter\def\csname lift@v4@echo_0.1@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4@echo_0.1@dynotears\endcsname{0.8}
\expandafter\def\csname found@v4@echo_0.1@dynotears\endcsname{0.8}
\expandafter\def\csname beyond@v4@echo_0.1@dynotears\endcsname{0.26}
\expandafter\def\csname lift@v4@echo_0.1@varlingam\endcsname{1.9}
\expandafter\def\csname len@v4@echo_0.1@varlingam\endcsname{9.5}
\expandafter\def\csname found@v4@echo_0.1@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v4@echo_0.1@varlingam\endcsname{0.43}
\expandafter\def\csname lift@v4@echo_0.1@doubleml\endcsname{5.2}
\expandafter\def\csname len@v4@echo_0.1@doubleml\endcsname{3.5}
\expandafter\def\csname found@v4@echo_0.1@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v4@echo_0.1@doubleml\endcsname{0.76}
\expandafter\def\csname lift@v4@echo_0.1@spacetime_rule\endcsname{6.7}
\expandafter\def\csname len@v4@echo_0.1@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v4@echo_0.1@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v4@echo_0.1@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v4@echo_0.6@correlation\endcsname{1.0}
\expandafter\def\csname len@v4@echo_0.6@correlation\endcsname{18.4}
\expandafter\def\csname found@v4@echo_0.6@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@echo_0.6@correlation\endcsname{0.03}
\expandafter\def\csname lift@v4@echo_0.6@granger\endcsname{1.0}
\expandafter\def\csname len@v4@echo_0.6@granger\endcsname{17.8}
\expandafter\def\csname found@v4@echo_0.6@granger\endcsname{2.5}
\expandafter\def\csname beyond@v4@echo_0.6@granger\endcsname{0.03}
\expandafter\def\csname lift@v4@echo_0.6@pcmciplus\endcsname{4.1}
\expandafter\def\csname len@v4@echo_0.6@pcmciplus\endcsname{3.2}
\expandafter\def\csname found@v4@echo_0.6@pcmciplus\endcsname{1.8}
\expandafter\def\csname beyond@v4@echo_0.6@pcmciplus\endcsname{0.52}
\expandafter\def\csname lift@v4@echo_0.6@pc\endcsname{2.4}
\expandafter\def\csname len@v4@echo_0.6@pc\endcsname{5.4}
\expandafter\def\csname found@v4@echo_0.6@pc\endcsname{1.8}
\expandafter\def\csname beyond@v4@echo_0.6@pc\endcsname{0.40}
\expandafter\def\csname lift@v4@echo_0.6@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4@echo_0.6@dynotears\endcsname{0.6}
\expandafter\def\csname found@v4@echo_0.6@dynotears\endcsname{0.6}
\expandafter\def\csname beyond@v4@echo_0.6@dynotears\endcsname{0.20}
\expandafter\def\csname lift@v4@echo_0.6@varlingam\endcsname{1.5}
\expandafter\def\csname len@v4@echo_0.6@varlingam\endcsname{11.4}
\expandafter\def\csname found@v4@echo_0.6@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v4@echo_0.6@varlingam\endcsname{0.33}
\expandafter\def\csname lift@v4@echo_0.6@doubleml\endcsname{5.3}
\expandafter\def\csname len@v4@echo_0.6@doubleml\endcsname{3.2}
\expandafter\def\csname found@v4@echo_0.6@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v4@echo_0.6@doubleml\endcsname{0.69}
\expandafter\def\csname lift@v4@echo_0.6@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v4@echo_0.6@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v4@echo_0.6@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v4@echo_0.6@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v4@control_0.3@correlation\endcsname{1.1}
\expandafter\def\csname len@v4@control_0.3@correlation\endcsname{16.1}
\expandafter\def\csname found@v4@control_0.3@correlation\endcsname{2.5}
\expandafter\def\csname beyond@v4@control_0.3@correlation\endcsname{0.03}
\expandafter\def\csname lift@v4@control_0.3@granger\endcsname{1.2}
\expandafter\def\csname len@v4@control_0.3@granger\endcsname{14.6}
\expandafter\def\csname found@v4@control_0.3@granger\endcsname{2.6}
\expandafter\def\csname beyond@v4@control_0.3@granger\endcsname{0.14}
\expandafter\def\csname lift@v4@control_0.3@pcmciplus\endcsname{4.9}
\expandafter\def\csname len@v4@control_0.3@pcmciplus\endcsname{3.1}
\expandafter\def\csname found@v4@control_0.3@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v4@control_0.3@pcmciplus\endcsname{0.66}
\expandafter\def\csname lift@v4@control_0.3@pc\endcsname{2.3}
\expandafter\def\csname len@v4@control_0.3@pc\endcsname{5.2}
\expandafter\def\csname found@v4@control_0.3@pc\endcsname{1.7}
\expandafter\def\csname beyond@v4@control_0.3@pc\endcsname{0.35}
\expandafter\def\csname lift@v4@control_0.3@dynotears\endcsname{6.9}
\expandafter\def\csname len@v4@control_0.3@dynotears\endcsname{0.3}
\expandafter\def\csname found@v4@control_0.3@dynotears\endcsname{0.3}
\expandafter\def\csname beyond@v4@control_0.3@dynotears\endcsname{0.10}
\expandafter\def\csname lift@v4@control_0.3@varlingam\endcsname{2.2}
\expandafter\def\csname len@v4@control_0.3@varlingam\endcsname{7.5}
\expandafter\def\csname found@v4@control_0.3@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v4@control_0.3@varlingam\endcsname{0.46}
\expandafter\def\csname lift@v4@control_0.3@doubleml\endcsname{5.3}
\expandafter\def\csname len@v4@control_0.3@doubleml\endcsname{3.0}
\expandafter\def\csname found@v4@control_0.3@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v4@control_0.3@doubleml\endcsname{0.68}
\expandafter\def\csname lift@v4@control_0.3@spacetime_rule\endcsname{5.9}
\expandafter\def\csname len@v4@control_0.3@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v4@control_0.3@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v4@control_0.3@spacetime_rule\endcsname{0.35}
\expandafter\def\csname lift@v4@control_0.6@correlation\endcsname{1.1}
\expandafter\def\csname len@v4@control_0.6@correlation\endcsname{16.0}
\expandafter\def\csname found@v4@control_0.6@correlation\endcsname{2.5}
\expandafter\def\csname beyond@v4@control_0.6@correlation\endcsname{0.03}
\expandafter\def\csname lift@v4@control_0.6@granger\endcsname{1.2}
\expandafter\def\csname len@v4@control_0.6@granger\endcsname{14.6}
\expandafter\def\csname found@v4@control_0.6@granger\endcsname{2.6}
\expandafter\def\csname beyond@v4@control_0.6@granger\endcsname{0.14}
\expandafter\def\csname lift@v4@control_0.6@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v4@control_0.6@pcmciplus\endcsname{2.8}
\expandafter\def\csname found@v4@control_0.6@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v4@control_0.6@pcmciplus\endcsname{0.68}
\expandafter\def\csname lift@v4@control_0.6@pc\endcsname{2.4}
\expandafter\def\csname len@v4@control_0.6@pc\endcsname{5.0}
\expandafter\def\csname found@v4@control_0.6@pc\endcsname{1.7}
\expandafter\def\csname beyond@v4@control_0.6@pc\endcsname{0.36}
\expandafter\def\csname lift@v4@control_0.6@dynotears\endcsname{6.9}
\expandafter\def\csname len@v4@control_0.6@dynotears\endcsname{0.3}
\expandafter\def\csname found@v4@control_0.6@dynotears\endcsname{0.3}
\expandafter\def\csname beyond@v4@control_0.6@dynotears\endcsname{0.10}
\expandafter\def\csname lift@v4@control_0.6@varlingam\endcsname{2.2}
\expandafter\def\csname len@v4@control_0.6@varlingam\endcsname{7.4}
\expandafter\def\csname found@v4@control_0.6@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v4@control_0.6@varlingam\endcsname{0.45}
\expandafter\def\csname lift@v4@control_0.6@doubleml\endcsname{5.5}
\expandafter\def\csname len@v4@control_0.6@doubleml\endcsname{2.9}
\expandafter\def\csname found@v4@control_0.6@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v4@control_0.6@doubleml\endcsname{0.70}
\expandafter\def\csname lift@v4@control_0.6@spacetime_rule\endcsname{5.9}
\expandafter\def\csname len@v4@control_0.6@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v4@control_0.6@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v4@control_0.6@spacetime_rule\endcsname{0.35}
\expandafter\def\csname lift@v4@control_1.0@correlation\endcsname{1.1}
\expandafter\def\csname len@v4@control_1.0@correlation\endcsname{16.0}
\expandafter\def\csname found@v4@control_1.0@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@control_1.0@correlation\endcsname{0.07}
\expandafter\def\csname lift@v4@control_1.0@granger\endcsname{1.2}
\expandafter\def\csname len@v4@control_1.0@granger\endcsname{14.5}
\expandafter\def\csname found@v4@control_1.0@granger\endcsname{2.6}
\expandafter\def\csname beyond@v4@control_1.0@granger\endcsname{0.15}
\expandafter\def\csname lift@v4@control_1.0@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v4@control_1.0@pcmciplus\endcsname{2.8}
\expandafter\def\csname found@v4@control_1.0@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v4@control_1.0@pcmciplus\endcsname{0.68}
\expandafter\def\csname lift@v4@control_1.0@pc\endcsname{2.4}
\expandafter\def\csname len@v4@control_1.0@pc\endcsname{5.0}
\expandafter\def\csname found@v4@control_1.0@pc\endcsname{1.7}
\expandafter\def\csname beyond@v4@control_1.0@pc\endcsname{0.36}
\expandafter\def\csname lift@v4@control_1.0@dynotears\endcsname{6.9}
\expandafter\def\csname len@v4@control_1.0@dynotears\endcsname{0.3}
\expandafter\def\csname found@v4@control_1.0@dynotears\endcsname{0.3}
\expandafter\def\csname beyond@v4@control_1.0@dynotears\endcsname{0.10}
\expandafter\def\csname lift@v4@control_1.0@varlingam\endcsname{2.1}
\expandafter\def\csname len@v4@control_1.0@varlingam\endcsname{7.8}
\expandafter\def\csname found@v4@control_1.0@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v4@control_1.0@varlingam\endcsname{0.45}
\expandafter\def\csname lift@v4@control_1.0@doubleml\endcsname{5.5}
\expandafter\def\csname len@v4@control_1.0@doubleml\endcsname{2.9}
\expandafter\def\csname found@v4@control_1.0@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v4@control_1.0@doubleml\endcsname{0.69}
\expandafter\def\csname lift@v4@control_1.0@spacetime_rule\endcsname{5.9}
\expandafter\def\csname len@v4@control_1.0@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v4@control_1.0@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v4@control_1.0@spacetime_rule\endcsname{0.35}
\expandafter\def\csname lift@v4@batches_50@correlation\endcsname{1.1}
\expandafter\def\csname len@v4@batches_50@correlation\endcsname{16.7}
\expandafter\def\csname found@v4@batches_50@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@batches_50@correlation\endcsname{0.13}
\expandafter\def\csname lift@v4@batches_50@granger\endcsname{1.6}
\expandafter\def\csname len@v4@batches_50@granger\endcsname{10.3}
\expandafter\def\csname found@v4@batches_50@granger\endcsname{2.2}
\expandafter\def\csname beyond@v4@batches_50@granger\endcsname{0.33}
\expandafter\def\csname lift@v4@batches_50@pcmciplus\endcsname{6.4}
\expandafter\def\csname len@v4@batches_50@pcmciplus\endcsname{2.3}
\expandafter\def\csname found@v4@batches_50@pcmciplus\endcsname{2.0}
\expandafter\def\csname beyond@v4@batches_50@pcmciplus\endcsname{0.63}
\expandafter\def\csname lift@v4@batches_50@pc\endcsname{3.6}
\expandafter\def\csname len@v4@batches_50@pc\endcsname{4.1}
\expandafter\def\csname found@v4@batches_50@pc\endcsname{2.0}
\expandafter\def\csname beyond@v4@batches_50@pc\endcsname{0.53}
\expandafter\def\csname lift@v4@batches_50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4@batches_50@dynotears\endcsname{0.9}
\expandafter\def\csname found@v4@batches_50@dynotears\endcsname{0.9}
\expandafter\def\csname beyond@v4@batches_50@dynotears\endcsname{0.30}
\expandafter\def\csname lift@v4@batches_50@varlingam\endcsname{2.8}
\expandafter\def\csname len@v4@batches_50@varlingam\endcsname{5.8}
\expandafter\def\csname found@v4@batches_50@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v4@batches_50@varlingam\endcsname{0.52}
\expandafter\def\csname lift@v4@batches_50@doubleml\endcsname{5.7}
\expandafter\def\csname len@v4@batches_50@doubleml\endcsname{2.3}
\expandafter\def\csname found@v4@batches_50@doubleml\endcsname{1.8}
\expandafter\def\csname beyond@v4@batches_50@doubleml\endcsname{0.56}
\expandafter\def\csname lift@v4@batches_50@spacetime_rule\endcsname{6.5}
\expandafter\def\csname len@v4@batches_50@spacetime_rule\endcsname{0.9}
\expandafter\def\csname found@v4@batches_50@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v4@batches_50@spacetime_rule\endcsname{0.26}
\expandafter\def\csname lift@v4@batches_100@correlation\endcsname{1.1}
\expandafter\def\csname len@v4@batches_100@correlation\endcsname{17.3}
\expandafter\def\csname found@v4@batches_100@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4@batches_100@correlation\endcsname{0.09}
\expandafter\def\csname lift@v4@batches_100@granger\endcsname{1.2}
\expandafter\def\csname len@v4@batches_100@granger\endcsname{14.6}
\expandafter\def\csname found@v4@batches_100@granger\endcsname{2.4}
\expandafter\def\csname beyond@v4@batches_100@granger\endcsname{0.16}
\expandafter\def\csname lift@v4@batches_100@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v4@batches_100@pcmciplus\endcsname{3.0}
\expandafter\def\csname found@v4@batches_100@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v4@batches_100@pcmciplus\endcsname{0.67}
\expandafter\def\csname lift@v4@batches_100@pc\endcsname{2.9}
\expandafter\def\csname len@v4@batches_100@pc\endcsname{4.6}
\expandafter\def\csname found@v4@batches_100@pc\endcsname{1.8}
\expandafter\def\csname beyond@v4@batches_100@pc\endcsname{0.43}
\expandafter\def\csname lift@v4@batches_100@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4@batches_100@dynotears\endcsname{0.7}
\expandafter\def\csname found@v4@batches_100@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v4@batches_100@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v4@batches_100@varlingam\endcsname{1.8}
\expandafter\def\csname len@v4@batches_100@varlingam\endcsname{9.5}
\expandafter\def\csname found@v4@batches_100@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v4@batches_100@varlingam\endcsname{0.40}
\expandafter\def\csname lift@v4@batches_100@doubleml\endcsname{5.4}
\expandafter\def\csname len@v4@batches_100@doubleml\endcsname{3.1}
\expandafter\def\csname found@v4@batches_100@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v4@batches_100@doubleml\endcsname{0.69}
\expandafter\def\csname lift@v4@batches_100@spacetime_rule\endcsname{6.7}
\expandafter\def\csname len@v4@batches_100@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v4@batches_100@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v4@batches_100@spacetime_rule\endcsname{0.36}
\expandafter\def\csname lift@v4h@signal_0.2@correlation\endcsname{1.2}
\expandafter\def\csname len@v4h@signal_0.2@correlation\endcsname{16.3}
\expandafter\def\csname found@v4h@signal_0.2@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4h@signal_0.2@correlation\endcsname{0.14}
\expandafter\def\csname lift@v4h@signal_0.2@granger\endcsname{1.4}
\expandafter\def\csname len@v4h@signal_0.2@granger\endcsname{11.9}
\expandafter\def\csname found@v4h@signal_0.2@granger\endcsname{2.3}
\expandafter\def\csname beyond@v4h@signal_0.2@granger\endcsname{0.26}
\expandafter\def\csname lift@v4h@signal_0.2@pcmciplus\endcsname{5.3}
\expandafter\def\csname len@v4h@signal_0.2@pcmciplus\endcsname{2.5}
\expandafter\def\csname found@v4h@signal_0.2@pcmciplus\endcsname{1.8}
\expandafter\def\csname beyond@v4h@signal_0.2@pcmciplus\endcsname{0.55}
\expandafter\def\csname lift@v4h@signal_0.2@pc\endcsname{2.2}
\expandafter\def\csname len@v4h@signal_0.2@pc\endcsname{5.0}
\expandafter\def\csname found@v4h@signal_0.2@pc\endcsname{1.5}
\expandafter\def\csname beyond@v4h@signal_0.2@pc\endcsname{0.30}
\expandafter\def\csname lift@v4h@signal_0.2@dynotears\endcsname{--}
\expandafter\def\csname len@v4h@signal_0.2@dynotears\endcsname{0.0}
\expandafter\def\csname found@v4h@signal_0.2@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v4h@signal_0.2@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v4h@signal_0.2@varlingam\endcsname{1.9}
\expandafter\def\csname len@v4h@signal_0.2@varlingam\endcsname{6.8}
\expandafter\def\csname found@v4h@signal_0.2@varlingam\endcsname{1.8}
\expandafter\def\csname beyond@v4h@signal_0.2@varlingam\endcsname{0.31}
\expandafter\def\csname lift@v4h@signal_0.2@doubleml\endcsname{6.4}
\expandafter\def\csname len@v4h@signal_0.2@doubleml\endcsname{1.6}
\expandafter\def\csname found@v4h@signal_0.2@doubleml\endcsname{1.4}
\expandafter\def\csname beyond@v4h@signal_0.2@doubleml\endcsname{0.44}
\expandafter\def\csname lift@v4h@signal_0.2@spacetime_rule\endcsname{1.5}
\expandafter\def\csname len@v4h@signal_0.2@spacetime_rule\endcsname{0.5}
\expandafter\def\csname found@v4h@signal_0.2@spacetime_rule\endcsname{0.1}
\expandafter\def\csname beyond@v4h@signal_0.2@spacetime_rule\endcsname{0.02}
\expandafter\def\csname lift@v4h@signal_0.1@correlation\endcsname{1.3}
\expandafter\def\csname len@v4h@signal_0.1@correlation\endcsname{13.1}
\expandafter\def\csname found@v4h@signal_0.1@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v4h@signal_0.1@correlation\endcsname{0.23}
\expandafter\def\csname lift@v4h@signal_0.1@granger\endcsname{1.9}
\expandafter\def\csname len@v4h@signal_0.1@granger\endcsname{7.8}
\expandafter\def\csname found@v4h@signal_0.1@granger\endcsname{2.0}
\expandafter\def\csname beyond@v4h@signal_0.1@granger\endcsname{0.37}
\expandafter\def\csname lift@v4h@signal_0.1@pcmciplus\endcsname{4.9}
\expandafter\def\csname len@v4h@signal_0.1@pcmciplus\endcsname{1.8}
\expandafter\def\csname found@v4h@signal_0.1@pcmciplus\endcsname{1.2}
\expandafter\def\csname beyond@v4h@signal_0.1@pcmciplus\endcsname{0.37}
\expandafter\def\csname lift@v4h@signal_0.1@pc\endcsname{2.3}
\expandafter\def\csname len@v4h@signal_0.1@pc\endcsname{4.4}
\expandafter\def\csname found@v4h@signal_0.1@pc\endcsname{1.4}
\expandafter\def\csname beyond@v4h@signal_0.1@pc\endcsname{0.30}
\expandafter\def\csname lift@v4h@signal_0.1@dynotears\endcsname{--}
\expandafter\def\csname len@v4h@signal_0.1@dynotears\endcsname{0.0}
\expandafter\def\csname found@v4h@signal_0.1@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v4h@signal_0.1@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v4h@signal_0.1@varlingam\endcsname{2.4}
\expandafter\def\csname len@v4h@signal_0.1@varlingam\endcsname{5.2}
\expandafter\def\csname found@v4h@signal_0.1@varlingam\endcsname{1.7}
\expandafter\def\csname beyond@v4h@signal_0.1@varlingam\endcsname{0.38}
\expandafter\def\csname lift@v4h@signal_0.1@doubleml\endcsname{7.3}
\expandafter\def\csname len@v4h@signal_0.1@doubleml\endcsname{1.0}
\expandafter\def\csname found@v4h@signal_0.1@doubleml\endcsname{1.0}
\expandafter\def\csname beyond@v4h@signal_0.1@doubleml\endcsname{0.32}
\expandafter\def\csname lift@v4h@signal_0.1@spacetime_rule\endcsname{0.0}
\expandafter\def\csname len@v4h@signal_0.1@spacetime_rule\endcsname{0.4}
\expandafter\def\csname found@v4h@signal_0.1@spacetime_rule\endcsname{0.0}
\expandafter\def\csname beyond@v4h@signal_0.1@spacetime_rule\endcsname{-0.02}
\expandafter\def\csname lift@v4h@echo_0.8@correlation\endcsname{1.0}
\expandafter\def\csname len@v4h@echo_0.8@correlation\endcsname{18.7}
\expandafter\def\csname found@v4h@echo_0.8@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v4h@echo_0.8@correlation\endcsname{0.01}
\expandafter\def\csname lift@v4h@echo_0.8@granger\endcsname{1.1}
\expandafter\def\csname len@v4h@echo_0.8@granger\endcsname{17.6}
\expandafter\def\csname found@v4h@echo_0.8@granger\endcsname{2.6}
\expandafter\def\csname beyond@v4h@echo_0.8@granger\endcsname{0.08}
\expandafter\def\csname lift@v4h@echo_0.8@pcmciplus\endcsname{4.9}
\expandafter\def\csname len@v4h@echo_0.8@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v4h@echo_0.8@pcmciplus\endcsname{1.8}
\expandafter\def\csname beyond@v4h@echo_0.8@pcmciplus\endcsname{0.53}
\expandafter\def\csname lift@v4h@echo_0.8@pc\endcsname{2.5}
\expandafter\def\csname len@v4h@echo_0.8@pc\endcsname{5.0}
\expandafter\def\csname found@v4h@echo_0.8@pc\endcsname{1.7}
\expandafter\def\csname beyond@v4h@echo_0.8@pc\endcsname{0.38}
\expandafter\def\csname lift@v4h@echo_0.8@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4h@echo_0.8@dynotears\endcsname{0.5}
\expandafter\def\csname found@v4h@echo_0.8@dynotears\endcsname{0.5}
\expandafter\def\csname beyond@v4h@echo_0.8@dynotears\endcsname{0.17}
\expandafter\def\csname lift@v4h@echo_0.8@varlingam\endcsname{1.5}
\expandafter\def\csname len@v4h@echo_0.8@varlingam\endcsname{11.1}
\expandafter\def\csname found@v4h@echo_0.8@varlingam\endcsname{2.3}
\expandafter\def\csname beyond@v4h@echo_0.8@varlingam\endcsname{0.29}
\expandafter\def\csname lift@v4h@echo_0.8@doubleml\endcsname{3.8}
\expandafter\def\csname len@v4h@echo_0.8@doubleml\endcsname{3.5}
\expandafter\def\csname found@v4h@echo_0.8@doubleml\endcsname{1.8}
\expandafter\def\csname beyond@v4h@echo_0.8@doubleml\endcsname{0.48}
\expandafter\def\csname lift@v4h@echo_0.8@spacetime_rule\endcsname{5.5}
\expandafter\def\csname len@v4h@echo_0.8@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v4h@echo_0.8@spacetime_rule\endcsname{0.9}
\expandafter\def\csname beyond@v4h@echo_0.8@spacetime_rule\endcsname{0.28}
\expandafter\def\csname lift@v4h@confound_0.8@correlation\endcsname{1.0}
\expandafter\def\csname len@v4h@confound_0.8@correlation\endcsname{17.5}
\expandafter\def\csname found@v4h@confound_0.8@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v4h@confound_0.8@correlation\endcsname{0.00}
\expandafter\def\csname lift@v4h@confound_0.8@granger\endcsname{1.1}
\expandafter\def\csname len@v4h@confound_0.8@granger\endcsname{16.0}
\expandafter\def\csname found@v4h@confound_0.8@granger\endcsname{2.3}
\expandafter\def\csname beyond@v4h@confound_0.8@granger\endcsname{0.06}
\expandafter\def\csname lift@v4h@confound_0.8@pcmciplus\endcsname{5.6}
\expandafter\def\csname len@v4h@confound_0.8@pcmciplus\endcsname{2.1}
\expandafter\def\csname found@v4h@confound_0.8@pcmciplus\endcsname{1.6}
\expandafter\def\csname beyond@v4h@confound_0.8@pcmciplus\endcsname{0.50}
\expandafter\def\csname lift@v4h@confound_0.8@pc\endcsname{2.7}
\expandafter\def\csname len@v4h@confound_0.8@pc\endcsname{4.8}
\expandafter\def\csname found@v4h@confound_0.8@pc\endcsname{1.8}
\expandafter\def\csname beyond@v4h@confound_0.8@pc\endcsname{0.43}
\expandafter\def\csname lift@v4h@confound_0.8@dynotears\endcsname{7.3}
\expandafter\def\csname len@v4h@confound_0.8@dynotears\endcsname{0.3}
\expandafter\def\csname found@v4h@confound_0.8@dynotears\endcsname{0.3}
\expandafter\def\csname beyond@v4h@confound_0.8@dynotears\endcsname{0.10}
\expandafter\def\csname lift@v4h@confound_0.8@varlingam\endcsname{1.4}
\expandafter\def\csname len@v4h@confound_0.8@varlingam\endcsname{11.1}
\expandafter\def\csname found@v4h@confound_0.8@varlingam\endcsname{2.1}
\expandafter\def\csname beyond@v4h@confound_0.8@varlingam\endcsname{0.24}
\expandafter\def\csname lift@v4h@confound_0.8@doubleml\endcsname{4.5}
\expandafter\def\csname len@v4h@confound_0.8@doubleml\endcsname{3.6}
\expandafter\def\csname found@v4h@confound_0.8@doubleml\endcsname{2.2}
\expandafter\def\csname beyond@v4h@confound_0.8@doubleml\endcsname{0.63}
\expandafter\def\csname lift@v4h@confound_0.8@spacetime_rule\endcsname{4.9}
\expandafter\def\csname len@v4h@confound_0.8@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v4h@confound_0.8@spacetime_rule\endcsname{1.0}
\expandafter\def\csname beyond@v4h@confound_0.8@spacetime_rule\endcsname{0.31}
\expandafter\def\csname lift@v4h@causes_4to6@correlation\endcsname{1.1}
\expandafter\def\csname len@v4h@causes_4to6@correlation\endcsname{17.2}
\expandafter\def\csname found@v4h@causes_4to6@correlation\endcsname{4.9}
\expandafter\def\csname beyond@v4h@causes_4to6@correlation\endcsname{0.06}
\expandafter\def\csname lift@v4h@causes_4to6@granger\endcsname{1.0}
\expandafter\def\csname len@v4h@causes_4to6@granger\endcsname{16.6}
\expandafter\def\csname found@v4h@causes_4to6@granger\endcsname{4.6}
\expandafter\def\csname beyond@v4h@causes_4to6@granger\endcsname{0.03}
\expandafter\def\csname lift@v4h@causes_4to6@pcmciplus\endcsname{3.1}
\expandafter\def\csname len@v4h@causes_4to6@pcmciplus\endcsname{4.0}
\expandafter\def\csname found@v4h@causes_4to6@pcmciplus\endcsname{3.3}
\expandafter\def\csname beyond@v4h@causes_4to6@pcmciplus\endcsname{0.43}
\expandafter\def\csname lift@v4h@causes_4to6@pc\endcsname{1.7}
\expandafter\def\csname len@v4h@causes_4to6@pc\endcsname{6.0}
\expandafter\def\csname found@v4h@causes_4to6@pc\endcsname{2.7}
\expandafter\def\csname beyond@v4h@causes_4to6@pc\endcsname{0.21}
\expandafter\def\csname lift@v4h@causes_4to6@dynotears\endcsname{3.7}
\expandafter\def\csname len@v4h@causes_4to6@dynotears\endcsname{0.2}
\expandafter\def\csname found@v4h@causes_4to6@dynotears\endcsname{0.2}
\expandafter\def\csname beyond@v4h@causes_4to6@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v4h@causes_4to6@varlingam\endcsname{1.5}
\expandafter\def\csname len@v4h@causes_4to6@varlingam\endcsname{11.1}
\expandafter\def\csname found@v4h@causes_4to6@varlingam\endcsname{4.6}
\expandafter\def\csname beyond@v4h@causes_4to6@varlingam\endcsname{0.31}
\expandafter\def\csname lift@v4h@causes_4to6@doubleml\endcsname{2.9}
\expandafter\def\csname len@v4h@causes_4to6@doubleml\endcsname{4.3}
\expandafter\def\csname found@v4h@causes_4to6@doubleml\endcsname{3.3}
\expandafter\def\csname beyond@v4h@causes_4to6@doubleml\endcsname{0.42}
\expandafter\def\csname lift@v4h@causes_4to6@spacetime_rule\endcsname{3.4}
\expandafter\def\csname len@v4h@causes_4to6@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v4h@causes_4to6@spacetime_rule\endcsname{1.0}
\expandafter\def\csname beyond@v4h@causes_4to6@spacetime_rule\endcsname{0.14}
\expandafter\def\csname lift@v4h@combo_hard@correlation\endcsname{1.0}
\expandafter\def\csname len@v4h@combo_hard@correlation\endcsname{17.0}
\expandafter\def\csname found@v4h@combo_hard@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v4h@combo_hard@correlation\endcsname{0.02}
\expandafter\def\csname lift@v4h@combo_hard@granger\endcsname{1.1}
\expandafter\def\csname len@v4h@combo_hard@granger\endcsname{14.9}
\expandafter\def\csname found@v4h@combo_hard@granger\endcsname{2.3}
\expandafter\def\csname beyond@v4h@combo_hard@granger\endcsname{0.12}
\expandafter\def\csname lift@v4h@combo_hard@pcmciplus\endcsname{5.1}
\expandafter\def\csname len@v4h@combo_hard@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v4h@combo_hard@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v4h@combo_hard@pcmciplus\endcsname{0.59}
\expandafter\def\csname lift@v4h@combo_hard@pc\endcsname{2.3}
\expandafter\def\csname len@v4h@combo_hard@pc\endcsname{4.2}
\expandafter\def\csname found@v4h@combo_hard@pc\endcsname{1.3}
\expandafter\def\csname beyond@v4h@combo_hard@pc\endcsname{0.28}
\expandafter\def\csname lift@v4h@combo_hard@dynotears\endcsname{--}
\expandafter\def\csname len@v4h@combo_hard@dynotears\endcsname{0.0}
\expandafter\def\csname found@v4h@combo_hard@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v4h@combo_hard@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v4h@combo_hard@varlingam\endcsname{1.5}
\expandafter\def\csname len@v4h@combo_hard@varlingam\endcsname{9.5}
\expandafter\def\csname found@v4h@combo_hard@varlingam\endcsname{1.9}
\expandafter\def\csname beyond@v4h@combo_hard@varlingam\endcsname{0.21}
\expandafter\def\csname lift@v4h@combo_hard@doubleml\endcsname{5.7}
\expandafter\def\csname len@v4h@combo_hard@doubleml\endcsname{1.8}
\expandafter\def\csname found@v4h@combo_hard@doubleml\endcsname{1.4}
\expandafter\def\csname beyond@v4h@combo_hard@doubleml\endcsname{0.43}
\expandafter\def\csname lift@v4h@combo_hard@spacetime_rule\endcsname{4.0}
\expandafter\def\csname len@v4h@combo_hard@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v4h@combo_hard@spacetime_rule\endcsname{0.6}
\expandafter\def\csname beyond@v4h@combo_hard@spacetime_rule\endcsname{0.18}
\expandafter\def\csname lift@v4h@combo_extreme@correlation\endcsname{1.1}
\expandafter\def\csname len@v4h@combo_extreme@correlation\endcsname{16.4}
\expandafter\def\csname found@v4h@combo_extreme@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v4h@combo_extreme@correlation\endcsname{0.07}
\expandafter\def\csname lift@v4h@combo_extreme@granger\endcsname{1.2}
\expandafter\def\csname len@v4h@combo_extreme@granger\endcsname{13.4}
\expandafter\def\csname found@v4h@combo_extreme@granger\endcsname{2.2}
\expandafter\def\csname beyond@v4h@combo_extreme@granger\endcsname{0.19}
\expandafter\def\csname lift@v4h@combo_extreme@pcmciplus\endcsname{4.3}
\expandafter\def\csname len@v4h@combo_extreme@pcmciplus\endcsname{1.2}
\expandafter\def\csname found@v4h@combo_extreme@pcmciplus\endcsname{0.7}
\expandafter\def\csname beyond@v4h@combo_extreme@pcmciplus\endcsname{0.21}
\expandafter\def\csname lift@v4h@combo_extreme@pc\endcsname{2.0}
\expandafter\def\csname len@v4h@combo_extreme@pc\endcsname{2.9}
\expandafter\def\csname found@v4h@combo_extreme@pc\endcsname{0.8}
\expandafter\def\csname beyond@v4h@combo_extreme@pc\endcsname{0.15}
\expandafter\def\csname lift@v4h@combo_extreme@dynotears\endcsname{--}
\expandafter\def\csname len@v4h@combo_extreme@dynotears\endcsname{0.0}
\expandafter\def\csname found@v4h@combo_extreme@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v4h@combo_extreme@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v4h@combo_extreme@varlingam\endcsname{1.6}
\expandafter\def\csname len@v4h@combo_extreme@varlingam\endcsname{8.2}
\expandafter\def\csname found@v4h@combo_extreme@varlingam\endcsname{1.8}
\expandafter\def\csname beyond@v4h@combo_extreme@varlingam\endcsname{0.27}
\expandafter\def\csname lift@v4h@combo_extreme@doubleml\endcsname{4.9}
\expandafter\def\csname len@v4h@combo_extreme@doubleml\endcsname{0.6}
\expandafter\def\csname found@v4h@combo_extreme@doubleml\endcsname{0.4}
\expandafter\def\csname beyond@v4h@combo_extreme@doubleml\endcsname{0.12}
\expandafter\def\csname lift@v4h@combo_extreme@spacetime_rule\endcsname{1.9}
\expandafter\def\csname len@v4h@combo_extreme@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v4h@combo_extreme@spacetime_rule\endcsname{0.4}
\expandafter\def\csname beyond@v4h@combo_extreme@spacetime_rule\endcsname{0.08}
\expandafter\def\csname lift@v5a@interaction_0.0@correlation\endcsname{1.0}
\expandafter\def\csname len@v5a@interaction_0.0@correlation\endcsname{18.2}
\expandafter\def\csname found@v5a@interaction_0.0@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v5a@interaction_0.0@correlation\endcsname{0.04}
\expandafter\def\csname lift@v5a@interaction_0.0@granger\endcsname{1.1}
\expandafter\def\csname len@v5a@interaction_0.0@granger\endcsname{17.1}
\expandafter\def\csname found@v5a@interaction_0.0@granger\endcsname{2.5}
\expandafter\def\csname beyond@v5a@interaction_0.0@granger\endcsname{0.06}
\expandafter\def\csname lift@v5a@interaction_0.0@pcmciplus\endcsname{5.7}
\expandafter\def\csname len@v5a@interaction_0.0@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v5a@interaction_0.0@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v5a@interaction_0.0@pcmciplus\endcsname{0.65}
\expandafter\def\csname lift@v5a@interaction_0.0@pc\endcsname{2.6}
\expandafter\def\csname len@v5a@interaction_0.0@pc\endcsname{5.4}
\expandafter\def\csname found@v5a@interaction_0.0@pc\endcsname{1.9}
\expandafter\def\csname beyond@v5a@interaction_0.0@pc\endcsname{0.43}
\expandafter\def\csname lift@v5a@interaction_0.0@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5a@interaction_0.0@dynotears\endcsname{0.7}
\expandafter\def\csname found@v5a@interaction_0.0@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v5a@interaction_0.0@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v5a@interaction_0.0@varlingam\endcsname{1.7}
\expandafter\def\csname len@v5a@interaction_0.0@varlingam\endcsname{9.7}
\expandafter\def\csname found@v5a@interaction_0.0@varlingam\endcsname{2.3}
\expandafter\def\csname beyond@v5a@interaction_0.0@varlingam\endcsname{0.37}
\expandafter\def\csname lift@v5a@interaction_0.0@doubleml\endcsname{4.7}
\expandafter\def\csname len@v5a@interaction_0.0@doubleml\endcsname{3.9}
\expandafter\def\csname found@v5a@interaction_0.0@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v5a@interaction_0.0@doubleml\endcsname{0.73}
\expandafter\def\csname lift@v5a@interaction_0.0@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v5a@interaction_0.0@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v5a@interaction_0.0@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v5a@interaction_0.0@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v5a@interaction_0.25@correlation\endcsname{1.1}
\expandafter\def\csname len@v5a@interaction_0.25@correlation\endcsname{17.9}
\expandafter\def\csname found@v5a@interaction_0.25@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v5a@interaction_0.25@correlation\endcsname{0.05}
\expandafter\def\csname lift@v5a@interaction_0.25@granger\endcsname{1.1}
\expandafter\def\csname len@v5a@interaction_0.25@granger\endcsname{16.4}
\expandafter\def\csname found@v5a@interaction_0.25@granger\endcsname{2.4}
\expandafter\def\csname beyond@v5a@interaction_0.25@granger\endcsname{0.06}
\expandafter\def\csname lift@v5a@interaction_0.25@pcmciplus\endcsname{5.6}
\expandafter\def\csname len@v5a@interaction_0.25@pcmciplus\endcsname{2.6}
\expandafter\def\csname found@v5a@interaction_0.25@pcmciplus\endcsname{2.0}
\expandafter\def\csname beyond@v5a@interaction_0.25@pcmciplus\endcsname{0.62}
\expandafter\def\csname lift@v5a@interaction_0.25@pc\endcsname{2.3}
\expandafter\def\csname len@v5a@interaction_0.25@pc\endcsname{5.0}
\expandafter\def\csname found@v5a@interaction_0.25@pc\endcsname{1.6}
\expandafter\def\csname beyond@v5a@interaction_0.25@pc\endcsname{0.34}
\expandafter\def\csname lift@v5a@interaction_0.25@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5a@interaction_0.25@dynotears\endcsname{0.4}
\expandafter\def\csname found@v5a@interaction_0.25@dynotears\endcsname{0.4}
\expandafter\def\csname beyond@v5a@interaction_0.25@dynotears\endcsname{0.13}
\expandafter\def\csname lift@v5a@interaction_0.25@varlingam\endcsname{1.5}
\expandafter\def\csname len@v5a@interaction_0.25@varlingam\endcsname{11.0}
\expandafter\def\csname found@v5a@interaction_0.25@varlingam\endcsname{2.3}
\expandafter\def\csname beyond@v5a@interaction_0.25@varlingam\endcsname{0.31}
\expandafter\def\csname lift@v5a@interaction_0.25@doubleml\endcsname{4.3}
\expandafter\def\csname len@v5a@interaction_0.25@doubleml\endcsname{3.2}
\expandafter\def\csname found@v5a@interaction_0.25@doubleml\endcsname{1.9}
\expandafter\def\csname beyond@v5a@interaction_0.25@doubleml\endcsname{0.55}
\expandafter\def\csname lift@v5a@interaction_0.25@spacetime_rule\endcsname{6.9}
\expandafter\def\csname len@v5a@interaction_0.25@spacetime_rule\endcsname{1.7}
\expandafter\def\csname found@v5a@interaction_0.25@spacetime_rule\endcsname{1.6}
\expandafter\def\csname beyond@v5a@interaction_0.25@spacetime_rule\endcsname{0.53}
\expandafter\def\csname lift@v5a@interaction_0.5@correlation\endcsname{1.1}
\expandafter\def\csname len@v5a@interaction_0.5@correlation\endcsname{17.3}
\expandafter\def\csname found@v5a@interaction_0.5@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v5a@interaction_0.5@correlation\endcsname{0.08}
\expandafter\def\csname lift@v5a@interaction_0.5@granger\endcsname{1.2}
\expandafter\def\csname len@v5a@interaction_0.5@granger\endcsname{14.7}
\expandafter\def\csname found@v5a@interaction_0.5@granger\endcsname{2.5}
\expandafter\def\csname beyond@v5a@interaction_0.5@granger\endcsname{0.20}
\expandafter\def\csname lift@v5a@interaction_0.5@pcmciplus\endcsname{6.2}
\expandafter\def\csname len@v5a@interaction_0.5@pcmciplus\endcsname{1.9}
\expandafter\def\csname found@v5a@interaction_0.5@pcmciplus\endcsname{1.6}
\expandafter\def\csname beyond@v5a@interaction_0.5@pcmciplus\endcsname{0.50}
\expandafter\def\csname lift@v5a@interaction_0.5@pc\endcsname{2.4}
\expandafter\def\csname len@v5a@interaction_0.5@pc\endcsname{5.2}
\expandafter\def\csname found@v5a@interaction_0.5@pc\endcsname{1.7}
\expandafter\def\csname beyond@v5a@interaction_0.5@pc\endcsname{0.37}
\expandafter\def\csname lift@v5a@interaction_0.5@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5a@interaction_0.5@dynotears\endcsname{0.1}
\expandafter\def\csname found@v5a@interaction_0.5@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v5a@interaction_0.5@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v5a@interaction_0.5@varlingam\endcsname{1.8}
\expandafter\def\csname len@v5a@interaction_0.5@varlingam\endcsname{9.6}
\expandafter\def\csname found@v5a@interaction_0.5@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v5a@interaction_0.5@varlingam\endcsname{0.44}
\expandafter\def\csname lift@v5a@interaction_0.5@doubleml\endcsname{5.4}
\expandafter\def\csname len@v5a@interaction_0.5@doubleml\endcsname{2.3}
\expandafter\def\csname found@v5a@interaction_0.5@doubleml\endcsname{1.7}
\expandafter\def\csname beyond@v5a@interaction_0.5@doubleml\endcsname{0.53}
\expandafter\def\csname lift@v5a@interaction_0.5@spacetime_rule\endcsname{6.8}
\expandafter\def\csname len@v5a@interaction_0.5@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v5a@interaction_0.5@spacetime_rule\endcsname{1.4}
\expandafter\def\csname beyond@v5a@interaction_0.5@spacetime_rule\endcsname{0.47}
\expandafter\def\csname lift@v5a@interaction_0.75@correlation\endcsname{1.2}
\expandafter\def\csname len@v5a@interaction_0.75@correlation\endcsname{15.1}
\expandafter\def\csname found@v5a@interaction_0.75@correlation\endcsname{2.5}
\expandafter\def\csname beyond@v5a@interaction_0.75@correlation\endcsname{0.17}
\expandafter\def\csname lift@v5a@interaction_0.75@granger\endcsname{1.5}
\expandafter\def\csname len@v5a@interaction_0.75@granger\endcsname{12.5}
\expandafter\def\csname found@v5a@interaction_0.75@granger\endcsname{2.5}
\expandafter\def\csname beyond@v5a@interaction_0.75@granger\endcsname{0.33}
\expandafter\def\csname lift@v5a@interaction_0.75@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v5a@interaction_0.75@pcmciplus\endcsname{2.3}
\expandafter\def\csname found@v5a@interaction_0.75@pcmciplus\endcsname{1.7}
\expandafter\def\csname beyond@v5a@interaction_0.75@pcmciplus\endcsname{0.53}
\expandafter\def\csname lift@v5a@interaction_0.75@pc\endcsname{2.8}
\expandafter\def\csname len@v5a@interaction_0.75@pc\endcsname{4.7}
\expandafter\def\csname found@v5a@interaction_0.75@pc\endcsname{1.8}
\expandafter\def\csname beyond@v5a@interaction_0.75@pc\endcsname{0.43}
\expandafter\def\csname lift@v5a@interaction_0.75@dynotears\endcsname{--}
\expandafter\def\csname len@v5a@interaction_0.75@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5a@interaction_0.75@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5a@interaction_0.75@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5a@interaction_0.75@varlingam\endcsname{1.7}
\expandafter\def\csname len@v5a@interaction_0.75@varlingam\endcsname{8.8}
\expandafter\def\csname found@v5a@interaction_0.75@varlingam\endcsname{2.0}
\expandafter\def\csname beyond@v5a@interaction_0.75@varlingam\endcsname{0.32}
\expandafter\def\csname lift@v5a@interaction_0.75@doubleml\endcsname{4.9}
\expandafter\def\csname len@v5a@interaction_0.75@doubleml\endcsname{2.1}
\expandafter\def\csname found@v5a@interaction_0.75@doubleml\endcsname{1.4}
\expandafter\def\csname beyond@v5a@interaction_0.75@doubleml\endcsname{0.42}
\expandafter\def\csname lift@v5a@interaction_0.75@spacetime_rule\endcsname{6.8}
\expandafter\def\csname len@v5a@interaction_0.75@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v5a@interaction_0.75@spacetime_rule\endcsname{1.3}
\expandafter\def\csname beyond@v5a@interaction_0.75@spacetime_rule\endcsname{0.43}
\expandafter\def\csname lift@v5a@interaction_1.0@correlation\endcsname{1.4}
\expandafter\def\csname len@v5a@interaction_1.0@correlation\endcsname{9.7}
\expandafter\def\csname found@v5a@interaction_1.0@correlation\endcsname{1.8}
\expandafter\def\csname beyond@v5a@interaction_1.0@correlation\endcsname{0.20}
\expandafter\def\csname lift@v5a@interaction_1.0@granger\endcsname{1.7}
\expandafter\def\csname len@v5a@interaction_1.0@granger\endcsname{8.8}
\expandafter\def\csname found@v5a@interaction_1.0@granger\endcsname{2.1}
\expandafter\def\csname beyond@v5a@interaction_1.0@granger\endcsname{0.37}
\expandafter\def\csname lift@v5a@interaction_1.0@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v5a@interaction_1.0@pcmciplus\endcsname{1.9}
\expandafter\def\csname found@v5a@interaction_1.0@pcmciplus\endcsname{1.4}
\expandafter\def\csname beyond@v5a@interaction_1.0@pcmciplus\endcsname{0.43}
\expandafter\def\csname lift@v5a@interaction_1.0@pc\endcsname{1.3}
\expandafter\def\csname len@v5a@interaction_1.0@pc\endcsname{3.4}
\expandafter\def\csname found@v5a@interaction_1.0@pc\endcsname{0.6}
\expandafter\def\csname beyond@v5a@interaction_1.0@pc\endcsname{0.05}
\expandafter\def\csname lift@v5a@interaction_1.0@dynotears\endcsname{--}
\expandafter\def\csname len@v5a@interaction_1.0@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5a@interaction_1.0@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5a@interaction_1.0@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5a@interaction_1.0@varlingam\endcsname{1.5}
\expandafter\def\csname len@v5a@interaction_1.0@varlingam\endcsname{3.8}
\expandafter\def\csname found@v5a@interaction_1.0@varlingam\endcsname{0.8}
\expandafter\def\csname beyond@v5a@interaction_1.0@varlingam\endcsname{0.13}
\expandafter\def\csname lift@v5a@interaction_1.0@doubleml\endcsname{4.9}
\expandafter\def\csname len@v5a@interaction_1.0@doubleml\endcsname{0.6}
\expandafter\def\csname found@v5a@interaction_1.0@doubleml\endcsname{0.4}
\expandafter\def\csname beyond@v5a@interaction_1.0@doubleml\endcsname{0.12}
\expandafter\def\csname lift@v5a@interaction_1.0@spacetime_rule\endcsname{6.8}
\expandafter\def\csname len@v5a@interaction_1.0@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v5a@interaction_1.0@spacetime_rule\endcsname{1.3}
\expandafter\def\csname beyond@v5a@interaction_1.0@spacetime_rule\endcsname{0.43}
\expandafter\def\csname lift@v5a@combo_interaction@correlation\endcsname{0.9}
\expandafter\def\csname len@v5a@combo_interaction@correlation\endcsname{5.6}
\expandafter\def\csname found@v5a@combo_interaction@correlation\endcsname{0.7}
\expandafter\def\csname beyond@v5a@combo_interaction@correlation\endcsname{0.00}
\expandafter\def\csname lift@v5a@combo_interaction@granger\endcsname{1.1}
\expandafter\def\csname len@v5a@combo_interaction@granger\endcsname{3.9}
\expandafter\def\csname found@v5a@combo_interaction@granger\endcsname{0.6}
\expandafter\def\csname beyond@v5a@combo_interaction@granger\endcsname{0.10}
\expandafter\def\csname lift@v5a@combo_interaction@pcmciplus\endcsname{4.1}
\expandafter\def\csname len@v5a@combo_interaction@pcmciplus\endcsname{0.9}
\expandafter\def\csname found@v5a@combo_interaction@pcmciplus\endcsname{0.5}
\expandafter\def\csname beyond@v5a@combo_interaction@pcmciplus\endcsname{0.15}
\expandafter\def\csname lift@v5a@combo_interaction@pc\endcsname{0.3}
\expandafter\def\csname len@v5a@combo_interaction@pc\endcsname{2.5}
\expandafter\def\csname found@v5a@combo_interaction@pc\endcsname{0.1}
\expandafter\def\csname beyond@v5a@combo_interaction@pc\endcsname{-0.09}
\expandafter\def\csname lift@v5a@combo_interaction@dynotears\endcsname{--}
\expandafter\def\csname len@v5a@combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5a@combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5a@combo_interaction@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5a@combo_interaction@varlingam\endcsname{1.1}
\expandafter\def\csname len@v5a@combo_interaction@varlingam\endcsname{3.4}
\expandafter\def\csname found@v5a@combo_interaction@varlingam\endcsname{0.5}
\expandafter\def\csname beyond@v5a@combo_interaction@varlingam\endcsname{0.02}
\expandafter\def\csname lift@v5a@combo_interaction@doubleml\endcsname{1.8}
\expandafter\def\csname len@v5a@combo_interaction@doubleml\endcsname{0.4}
\expandafter\def\csname found@v5a@combo_interaction@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v5a@combo_interaction@doubleml\endcsname{0.03}
\expandafter\def\csname lift@v5a@combo_interaction@spacetime_rule\endcsname{3.9}
\expandafter\def\csname len@v5a@combo_interaction@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v5a@combo_interaction@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v5a@combo_interaction@spacetime_rule\endcsname{0.24}
\expandafter\def\csname lift@v5a@control_weak@correlation\endcsname{1.3}
\expandafter\def\csname len@v5a@control_weak@correlation\endcsname{12.8}
\expandafter\def\csname found@v5a@control_weak@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v5a@control_weak@correlation\endcsname{0.18}
\expandafter\def\csname lift@v5a@control_weak@granger\endcsname{1.9}
\expandafter\def\csname len@v5a@control_weak@granger\endcsname{8.6}
\expandafter\def\csname found@v5a@control_weak@granger\endcsname{2.3}
\expandafter\def\csname beyond@v5a@control_weak@granger\endcsname{0.35}
\expandafter\def\csname lift@v5a@control_weak@pcmciplus\endcsname{4.7}
\expandafter\def\csname len@v5a@control_weak@pcmciplus\endcsname{2.2}
\expandafter\def\csname found@v5a@control_weak@pcmciplus\endcsname{1.5}
\expandafter\def\csname beyond@v5a@control_weak@pcmciplus\endcsname{0.44}
\expandafter\def\csname lift@v5a@control_weak@pc\endcsname{2.0}
\expandafter\def\csname len@v5a@control_weak@pc\endcsname{4.5}
\expandafter\def\csname found@v5a@control_weak@pc\endcsname{1.3}
\expandafter\def\csname beyond@v5a@control_weak@pc\endcsname{0.24}
\expandafter\def\csname lift@v5a@control_weak@dynotears\endcsname{--}
\expandafter\def\csname len@v5a@control_weak@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5a@control_weak@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5a@control_weak@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5a@control_weak@varlingam\endcsname{2.7}
\expandafter\def\csname len@v5a@control_weak@varlingam\endcsname{5.2}
\expandafter\def\csname found@v5a@control_weak@varlingam\endcsname{2.0}
\expandafter\def\csname beyond@v5a@control_weak@varlingam\endcsname{0.45}
\expandafter\def\csname lift@v5a@control_weak@doubleml\endcsname{5.3}
\expandafter\def\csname len@v5a@control_weak@doubleml\endcsname{1.7}
\expandafter\def\csname found@v5a@control_weak@doubleml\endcsname{1.3}
\expandafter\def\csname beyond@v5a@control_weak@doubleml\endcsname{0.38}
\expandafter\def\csname lift@v5a@control_weak@spacetime_rule\endcsname{2.3}
\expandafter\def\csname len@v5a@control_weak@spacetime_rule\endcsname{0.3}
\expandafter\def\csname found@v5a@control_weak@spacetime_rule\endcsname{0.1}
\expandafter\def\csname beyond@v5a@control_weak@spacetime_rule\endcsname{0.02}
\expandafter\def\csname lift@v5a@signal_0.05@correlation\endcsname{1.6}
\expandafter\def\csname len@v5a@signal_0.05@correlation\endcsname{10.0}
\expandafter\def\csname found@v5a@signal_0.05@correlation\endcsname{2.2}
\expandafter\def\csname beyond@v5a@signal_0.05@correlation\endcsname{0.30}
\expandafter\def\csname lift@v5a@signal_0.05@granger\endcsname{2.9}
\expandafter\def\csname len@v5a@signal_0.05@granger\endcsname{4.5}
\expandafter\def\csname found@v5a@signal_0.05@granger\endcsname{1.8}
\expandafter\def\csname beyond@v5a@signal_0.05@granger\endcsname{0.45}
\expandafter\def\csname lift@v5a@signal_0.05@pcmciplus\endcsname{3.2}
\expandafter\def\csname len@v5a@signal_0.05@pcmciplus\endcsname{1.6}
\expandafter\def\csname found@v5a@signal_0.05@pcmciplus\endcsname{0.7}
\expandafter\def\csname beyond@v5a@signal_0.05@pcmciplus\endcsname{0.17}
\expandafter\def\csname lift@v5a@signal_0.05@pc\endcsname{1.9}
\expandafter\def\csname len@v5a@signal_0.05@pc\endcsname{4.2}
\expandafter\def\csname found@v5a@signal_0.05@pc\endcsname{1.1}
\expandafter\def\csname beyond@v5a@signal_0.05@pc\endcsname{0.20}
\expandafter\def\csname lift@v5a@signal_0.05@dynotears\endcsname{--}
\expandafter\def\csname len@v5a@signal_0.05@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5a@signal_0.05@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5a@signal_0.05@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5a@signal_0.05@varlingam\endcsname{2.0}
\expandafter\def\csname len@v5a@signal_0.05@varlingam\endcsname{4.0}
\expandafter\def\csname found@v5a@signal_0.05@varlingam\endcsname{1.1}
\expandafter\def\csname beyond@v5a@signal_0.05@varlingam\endcsname{0.20}
\expandafter\def\csname lift@v5a@signal_0.05@doubleml\endcsname{6.1}
\expandafter\def\csname len@v5a@signal_0.05@doubleml\endcsname{0.6}
\expandafter\def\csname found@v5a@signal_0.05@doubleml\endcsname{0.5}
\expandafter\def\csname beyond@v5a@signal_0.05@doubleml\endcsname{0.16}
\expandafter\def\csname lift@v5a@signal_0.05@spacetime_rule\endcsname{0.0}
\expandafter\def\csname len@v5a@signal_0.05@spacetime_rule\endcsname{0.2}
\expandafter\def\csname found@v5a@signal_0.05@spacetime_rule\endcsname{0.0}
\expandafter\def\csname beyond@v5a@signal_0.05@spacetime_rule\endcsname{-0.01}
\expandafter\def\csname lift@v5b@default@correlation\endcsname{1.1}
\expandafter\def\csname len@v5b@default@correlation\endcsname{36.1}
\expandafter\def\csname found@v5b@default@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v5b@default@correlation\endcsname{0.07}
\expandafter\def\csname lift@v5b@default@granger\endcsname{1.2}
\expandafter\def\csname len@v5b@default@granger\endcsname{32.6}
\expandafter\def\csname found@v5b@default@granger\endcsname{2.6}
\expandafter\def\csname beyond@v5b@default@granger\endcsname{0.16}
\expandafter\def\csname lift@v5b@default@pcmciplus\endcsname{10.5}
\expandafter\def\csname len@v5b@default@pcmciplus\endcsname{3.3}
\expandafter\def\csname found@v5b@default@pcmciplus\endcsname{2.3}
\expandafter\def\csname beyond@v5b@default@pcmciplus\endcsname{0.80}
\expandafter\def\csname lift@v5b@default@pc\endcsname{4.3}
\expandafter\def\csname len@v5b@default@pc\endcsname{5.6}
\expandafter\def\csname found@v5b@default@pc\endcsname{1.6}
\expandafter\def\csname beyond@v5b@default@pc\endcsname{0.47}
\expandafter\def\csname lift@v5b@default@dynotears\endcsname{15.0}
\expandafter\def\csname len@v5b@default@dynotears\endcsname{0.5}
\expandafter\def\csname found@v5b@default@dynotears\endcsname{0.5}
\expandafter\def\csname beyond@v5b@default@dynotears\endcsname{0.18}
\expandafter\def\csname lift@v5b@default@varlingam\endcsname{3.3}
\expandafter\def\csname len@v5b@default@varlingam\endcsname{10.3}
\expandafter\def\csname found@v5b@default@varlingam\endcsname{2.3}
\expandafter\def\csname beyond@v5b@default@varlingam\endcsname{0.62}
\expandafter\def\csname lift@v5b@default@doubleml\endcsname{10.2}
\expandafter\def\csname len@v5b@default@doubleml\endcsname{2.8}
\expandafter\def\csname found@v5b@default@doubleml\endcsname{1.9}
\expandafter\def\csname beyond@v5b@default@doubleml\endcsname{0.65}
\expandafter\def\csname lift@v5b@default@spacetime_rule\endcsname{12.3}
\expandafter\def\csname len@v5b@default@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v5b@default@spacetime_rule\endcsname{0.9}
\expandafter\def\csname beyond@v5b@default@spacetime_rule\endcsname{0.32}
\expandafter\def\csname lift@v5b@signal_0.1@correlation\endcsname{1.5}
\expandafter\def\csname len@v5b@signal_0.1@correlation\endcsname{23.7}
\expandafter\def\csname found@v5b@signal_0.1@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v5b@signal_0.1@correlation\endcsname{0.29}
\expandafter\def\csname lift@v5b@signal_0.1@granger\endcsname{1.9}
\expandafter\def\csname len@v5b@signal_0.1@granger\endcsname{14.5}
\expandafter\def\csname found@v5b@signal_0.1@granger\endcsname{1.8}
\expandafter\def\csname beyond@v5b@signal_0.1@granger\endcsname{0.34}
\expandafter\def\csname lift@v5b@signal_0.1@pcmciplus\endcsname{5.6}
\expandafter\def\csname len@v5b@signal_0.1@pcmciplus\endcsname{1.6}
\expandafter\def\csname found@v5b@signal_0.1@pcmciplus\endcsname{0.6}
\expandafter\def\csname beyond@v5b@signal_0.1@pcmciplus\endcsname{0.19}
\expandafter\def\csname lift@v5b@signal_0.1@pc\endcsname{3.3}
\expandafter\def\csname len@v5b@signal_0.1@pc\endcsname{3.6}
\expandafter\def\csname found@v5b@signal_0.1@pc\endcsname{0.8}
\expandafter\def\csname beyond@v5b@signal_0.1@pc\endcsname{0.22}
\expandafter\def\csname lift@v5b@signal_0.1@dynotears\endcsname{--}
\expandafter\def\csname len@v5b@signal_0.1@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5b@signal_0.1@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5b@signal_0.1@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5b@signal_0.1@varlingam\endcsname{3.8}
\expandafter\def\csname len@v5b@signal_0.1@varlingam\endcsname{6.4}
\expandafter\def\csname found@v5b@signal_0.1@varlingam\endcsname{1.6}
\expandafter\def\csname beyond@v5b@signal_0.1@varlingam\endcsname{0.43}
\expandafter\def\csname lift@v5b@signal_0.1@doubleml\endcsname{11.2}
\expandafter\def\csname len@v5b@signal_0.1@doubleml\endcsname{0.4}
\expandafter\def\csname found@v5b@signal_0.1@doubleml\endcsname{0.3}
\expandafter\def\csname beyond@v5b@signal_0.1@doubleml\endcsname{0.10}
\expandafter\def\csname lift@v5b@signal_0.1@spacetime_rule\endcsname{7.5}
\expandafter\def\csname len@v5b@signal_0.1@spacetime_rule\endcsname{0.8}
\expandafter\def\csname found@v5b@signal_0.1@spacetime_rule\endcsname{0.4}
\expandafter\def\csname beyond@v5b@signal_0.1@spacetime_rule\endcsname{0.13}
\expandafter\def\csname lift@v5b@echo_0.8@correlation\endcsname{1.1}
\expandafter\def\csname len@v5b@echo_0.8@correlation\endcsname{37.1}
\expandafter\def\csname found@v5b@echo_0.8@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v5b@echo_0.8@correlation\endcsname{0.05}
\expandafter\def\csname lift@v5b@echo_0.8@granger\endcsname{1.2}
\expandafter\def\csname len@v5b@echo_0.8@granger\endcsname{33.5}
\expandafter\def\csname found@v5b@echo_0.8@granger\endcsname{2.6}
\expandafter\def\csname beyond@v5b@echo_0.8@granger\endcsname{0.14}
\expandafter\def\csname lift@v5b@echo_0.8@pcmciplus\endcsname{8.3}
\expandafter\def\csname len@v5b@echo_0.8@pcmciplus\endcsname{2.9}
\expandafter\def\csname found@v5b@echo_0.8@pcmciplus\endcsname{1.6}
\expandafter\def\csname beyond@v5b@echo_0.8@pcmciplus\endcsname{0.54}
\expandafter\def\csname lift@v5b@echo_0.8@pc\endcsname{3.6}
\expandafter\def\csname len@v5b@echo_0.8@pc\endcsname{5.4}
\expandafter\def\csname found@v5b@echo_0.8@pc\endcsname{1.3}
\expandafter\def\csname beyond@v5b@echo_0.8@pc\endcsname{0.36}
\expandafter\def\csname lift@v5b@echo_0.8@dynotears\endcsname{15.0}
\expandafter\def\csname len@v5b@echo_0.8@dynotears\endcsname{0.3}
\expandafter\def\csname found@v5b@echo_0.8@dynotears\endcsname{0.3}
\expandafter\def\csname beyond@v5b@echo_0.8@dynotears\endcsname{0.11}
\expandafter\def\csname lift@v5b@echo_0.8@varlingam\endcsname{2.2}
\expandafter\def\csname len@v5b@echo_0.8@varlingam\endcsname{14.7}
\expandafter\def\csname found@v5b@echo_0.8@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v5b@echo_0.8@varlingam\endcsname{0.45}
\expandafter\def\csname lift@v5b@echo_0.8@doubleml\endcsname{8.3}
\expandafter\def\csname len@v5b@echo_0.8@doubleml\endcsname{2.7}
\expandafter\def\csname found@v5b@echo_0.8@doubleml\endcsname{1.5}
\expandafter\def\csname beyond@v5b@echo_0.8@doubleml\endcsname{0.50}
\expandafter\def\csname lift@v5b@echo_0.8@spacetime_rule\endcsname{10.5}
\expandafter\def\csname len@v5b@echo_0.8@spacetime_rule\endcsname{1.0}
\expandafter\def\csname found@v5b@echo_0.8@spacetime_rule\endcsname{0.7}
\expandafter\def\csname beyond@v5b@echo_0.8@spacetime_rule\endcsname{0.24}
\expandafter\def\csname lift@v5b@confound_0.8@correlation\endcsname{0.9}
\expandafter\def\csname len@v5b@confound_0.8@correlation\endcsname{37.1}
\expandafter\def\csname found@v5b@confound_0.8@correlation\endcsname{2.3}
\expandafter\def\csname beyond@v5b@confound_0.8@correlation\endcsname{-0.07}
\expandafter\def\csname lift@v5b@confound_0.8@granger\endcsname{1.0}
\expandafter\def\csname len@v5b@confound_0.8@granger\endcsname{33.5}
\expandafter\def\csname found@v5b@confound_0.8@granger\endcsname{2.3}
\expandafter\def\csname beyond@v5b@confound_0.8@granger\endcsname{0.03}
\expandafter\def\csname lift@v5b@confound_0.8@pcmciplus\endcsname{11.4}
\expandafter\def\csname len@v5b@confound_0.8@pcmciplus\endcsname{2.1}
\expandafter\def\csname found@v5b@confound_0.8@pcmciplus\endcsname{1.6}
\expandafter\def\csname beyond@v5b@confound_0.8@pcmciplus\endcsname{0.56}
\expandafter\def\csname lift@v5b@confound_0.8@pc\endcsname{5.1}
\expandafter\def\csname len@v5b@confound_0.8@pc\endcsname{3.8}
\expandafter\def\csname found@v5b@confound_0.8@pc\endcsname{1.3}
\expandafter\def\csname beyond@v5b@confound_0.8@pc\endcsname{0.40}
\expandafter\def\csname lift@v5b@confound_0.8@dynotears\endcsname{15.0}
\expandafter\def\csname len@v5b@confound_0.8@dynotears\endcsname{0.1}
\expandafter\def\csname found@v5b@confound_0.8@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v5b@confound_0.8@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v5b@confound_0.8@varlingam\endcsname{2.8}
\expandafter\def\csname len@v5b@confound_0.8@varlingam\endcsname{11.2}
\expandafter\def\csname found@v5b@confound_0.8@varlingam\endcsname{2.1}
\expandafter\def\csname beyond@v5b@confound_0.8@varlingam\endcsname{0.48}
\expandafter\def\csname lift@v5b@confound_0.8@doubleml\endcsname{10.0}
\expandafter\def\csname len@v5b@confound_0.8@doubleml\endcsname{2.4}
\expandafter\def\csname found@v5b@confound_0.8@doubleml\endcsname{1.6}
\expandafter\def\csname beyond@v5b@confound_0.8@doubleml\endcsname{0.55}
\expandafter\def\csname lift@v5b@confound_0.8@spacetime_rule\endcsname{7.1}
\expandafter\def\csname len@v5b@confound_0.8@spacetime_rule\endcsname{2.1}
\expandafter\def\csname found@v5b@confound_0.8@spacetime_rule\endcsname{1.0}
\expandafter\def\csname beyond@v5b@confound_0.8@spacetime_rule\endcsname{0.33}
\expandafter\def\csname lift@v5b@combo_hard@correlation\endcsname{1.1}
\expandafter\def\csname len@v5b@combo_hard@correlation\endcsname{34.8}
\expandafter\def\csname found@v5b@combo_hard@correlation\endcsname{2.5}
\expandafter\def\csname beyond@v5b@combo_hard@correlation\endcsname{0.07}
\expandafter\def\csname lift@v5b@combo_hard@granger\endcsname{1.2}
\expandafter\def\csname len@v5b@combo_hard@granger\endcsname{28.3}
\expandafter\def\csname found@v5b@combo_hard@granger\endcsname{2.3}
\expandafter\def\csname beyond@v5b@combo_hard@granger\endcsname{0.16}
\expandafter\def\csname lift@v5b@combo_hard@pcmciplus\endcsname{8.2}
\expandafter\def\csname len@v5b@combo_hard@pcmciplus\endcsname{2.0}
\expandafter\def\csname found@v5b@combo_hard@pcmciplus\endcsname{1.1}
\expandafter\def\csname beyond@v5b@combo_hard@pcmciplus\endcsname{0.37}
\expandafter\def\csname lift@v5b@combo_hard@pc\endcsname{3.9}
\expandafter\def\csname len@v5b@combo_hard@pc\endcsname{3.5}
\expandafter\def\csname found@v5b@combo_hard@pc\endcsname{0.9}
\expandafter\def\csname beyond@v5b@combo_hard@pc\endcsname{0.25}
\expandafter\def\csname lift@v5b@combo_hard@dynotears\endcsname{--}
\expandafter\def\csname len@v5b@combo_hard@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5b@combo_hard@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5b@combo_hard@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5b@combo_hard@varlingam\endcsname{2.5}
\expandafter\def\csname len@v5b@combo_hard@varlingam\endcsname{9.5}
\expandafter\def\csname found@v5b@combo_hard@varlingam\endcsname{1.6}
\expandafter\def\csname beyond@v5b@combo_hard@varlingam\endcsname{0.35}
\expandafter\def\csname lift@v5b@combo_hard@doubleml\endcsname{11.2}
\expandafter\def\csname len@v5b@combo_hard@doubleml\endcsname{1.6}
\expandafter\def\csname found@v5b@combo_hard@doubleml\endcsname{1.2}
\expandafter\def\csname beyond@v5b@combo_hard@doubleml\endcsname{0.41}
\expandafter\def\csname lift@v5b@combo_hard@spacetime_rule\endcsname{8.8}
\expandafter\def\csname len@v5b@combo_hard@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v5b@combo_hard@spacetime_rule\endcsname{0.7}
\expandafter\def\csname beyond@v5b@combo_hard@spacetime_rule\endcsname{0.24}
\expandafter\def\csname lift@v5b@combo_extreme@correlation\endcsname{1.1}
\expandafter\def\csname len@v5b@combo_extreme@correlation\endcsname{32.9}
\expandafter\def\csname found@v5b@combo_extreme@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v5b@combo_extreme@correlation\endcsname{0.07}
\expandafter\def\csname lift@v5b@combo_extreme@granger\endcsname{1.2}
\expandafter\def\csname len@v5b@combo_extreme@granger\endcsname{25.6}
\expandafter\def\csname found@v5b@combo_extreme@granger\endcsname{2.0}
\expandafter\def\csname beyond@v5b@combo_extreme@granger\endcsname{0.12}
\expandafter\def\csname lift@v5b@combo_extreme@pcmciplus\endcsname{4.6}
\expandafter\def\csname len@v5b@combo_extreme@pcmciplus\endcsname{1.3}
\expandafter\def\csname found@v5b@combo_extreme@pcmciplus\endcsname{0.4}
\expandafter\def\csname beyond@v5b@combo_extreme@pcmciplus\endcsname{0.12}
\expandafter\def\csname lift@v5b@combo_extreme@pc\endcsname{2.9}
\expandafter\def\csname len@v5b@combo_extreme@pc\endcsname{2.6}
\expandafter\def\csname found@v5b@combo_extreme@pc\endcsname{0.5}
\expandafter\def\csname beyond@v5b@combo_extreme@pc\endcsname{0.12}
\expandafter\def\csname lift@v5b@combo_extreme@dynotears\endcsname{--}
\expandafter\def\csname len@v5b@combo_extreme@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5b@combo_extreme@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5b@combo_extreme@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5b@combo_extreme@varlingam\endcsname{1.9}
\expandafter\def\csname len@v5b@combo_extreme@varlingam\endcsname{10.2}
\expandafter\def\csname found@v5b@combo_extreme@varlingam\endcsname{1.3}
\expandafter\def\csname beyond@v5b@combo_extreme@varlingam\endcsname{0.23}
\expandafter\def\csname lift@v5b@combo_extreme@doubleml\endcsname{9.0}
\expandafter\def\csname len@v5b@combo_extreme@doubleml\endcsname{0.5}
\expandafter\def\csname found@v5b@combo_extreme@doubleml\endcsname{0.3}
\expandafter\def\csname beyond@v5b@combo_extreme@doubleml\endcsname{0.10}
\expandafter\def\csname lift@v5b@combo_extreme@spacetime_rule\endcsname{2.5}
\expandafter\def\csname len@v5b@combo_extreme@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v5b@combo_extreme@spacetime_rule\endcsname{0.2}
\expandafter\def\csname beyond@v5b@combo_extreme@spacetime_rule\endcsname{0.05}
\expandafter\def\csname lift@v5b@interaction_1.0@correlation\endcsname{1.3}
\expandafter\def\csname len@v5b@interaction_1.0@correlation\endcsname{14.5}
\expandafter\def\csname found@v5b@interaction_1.0@correlation\endcsname{1.3}
\expandafter\def\csname beyond@v5b@interaction_1.0@correlation\endcsname{0.13}
\expandafter\def\csname lift@v5b@interaction_1.0@granger\endcsname{1.8}
\expandafter\def\csname len@v5b@interaction_1.0@granger\endcsname{12.4}
\expandafter\def\csname found@v5b@interaction_1.0@granger\endcsname{1.5}
\expandafter\def\csname beyond@v5b@interaction_1.0@granger\endcsname{0.27}
\expandafter\def\csname lift@v5b@interaction_1.0@pcmciplus\endcsname{6.7}
\expandafter\def\csname len@v5b@interaction_1.0@pcmciplus\endcsname{1.8}
\expandafter\def\csname found@v5b@interaction_1.0@pcmciplus\endcsname{0.8}
\expandafter\def\csname beyond@v5b@interaction_1.0@pcmciplus\endcsname{0.26}
\expandafter\def\csname lift@v5b@interaction_1.0@pc\endcsname{1.0}
\expandafter\def\csname len@v5b@interaction_1.0@pc\endcsname{4.3}
\expandafter\def\csname found@v5b@interaction_1.0@pc\endcsname{0.3}
\expandafter\def\csname beyond@v5b@interaction_1.0@pc\endcsname{0.01}
\expandafter\def\csname lift@v5b@interaction_1.0@dynotears\endcsname{--}
\expandafter\def\csname len@v5b@interaction_1.0@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5b@interaction_1.0@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5b@interaction_1.0@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5b@interaction_1.0@varlingam\endcsname{3.2}
\expandafter\def\csname len@v5b@interaction_1.0@varlingam\endcsname{5.2}
\expandafter\def\csname found@v5b@interaction_1.0@varlingam\endcsname{1.1}
\expandafter\def\csname beyond@v5b@interaction_1.0@varlingam\endcsname{0.29}
\expandafter\def\csname lift@v5b@interaction_1.0@doubleml\endcsname{7.5}
\expandafter\def\csname len@v5b@interaction_1.0@doubleml\endcsname{0.4}
\expandafter\def\csname found@v5b@interaction_1.0@doubleml\endcsname{0.2}
\expandafter\def\csname beyond@v5b@interaction_1.0@doubleml\endcsname{0.07}
\expandafter\def\csname lift@v5b@interaction_1.0@spacetime_rule\endcsname{14.1}
\expandafter\def\csname len@v5b@interaction_1.0@spacetime_rule\endcsname{1.7}
\expandafter\def\csname found@v5b@interaction_1.0@spacetime_rule\endcsname{1.6}
\expandafter\def\csname beyond@v5b@interaction_1.0@spacetime_rule\endcsname{0.57}
\expandafter\def\csname lift@v5b@combo_interaction@correlation\endcsname{1.2}
\expandafter\def\csname len@v5b@combo_interaction@correlation\endcsname{8.9}
\expandafter\def\csname found@v5b@combo_interaction@correlation\endcsname{0.7}
\expandafter\def\csname beyond@v5b@combo_interaction@correlation\endcsname{0.08}
\expandafter\def\csname lift@v5b@combo_interaction@granger\endcsname{1.5}
\expandafter\def\csname len@v5b@combo_interaction@granger\endcsname{9.1}
\expandafter\def\csname found@v5b@combo_interaction@granger\endcsname{0.9}
\expandafter\def\csname beyond@v5b@combo_interaction@granger\endcsname{0.15}
\expandafter\def\csname lift@v5b@combo_interaction@pcmciplus\endcsname{2.8}
\expandafter\def\csname len@v5b@combo_interaction@pcmciplus\endcsname{1.6}
\expandafter\def\csname found@v5b@combo_interaction@pcmciplus\endcsname{0.3}
\expandafter\def\csname beyond@v5b@combo_interaction@pcmciplus\endcsname{0.07}
\expandafter\def\csname lift@v5b@combo_interaction@pc\endcsname{1.2}
\expandafter\def\csname len@v5b@combo_interaction@pc\endcsname{2.6}
\expandafter\def\csname found@v5b@combo_interaction@pc\endcsname{0.2}
\expandafter\def\csname beyond@v5b@combo_interaction@pc\endcsname{0.01}
\expandafter\def\csname lift@v5b@combo_interaction@dynotears\endcsname{--}
\expandafter\def\csname len@v5b@combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5b@combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5b@combo_interaction@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5b@combo_interaction@varlingam\endcsname{2.1}
\expandafter\def\csname len@v5b@combo_interaction@varlingam\endcsname{5.0}
\expandafter\def\csname found@v5b@combo_interaction@varlingam\endcsname{0.7}
\expandafter\def\csname beyond@v5b@combo_interaction@varlingam\endcsname{0.15}
\expandafter\def\csname lift@v5b@combo_interaction@doubleml\endcsname{3.8}
\expandafter\def\csname len@v5b@combo_interaction@doubleml\endcsname{0.4}
\expandafter\def\csname found@v5b@combo_interaction@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v5b@combo_interaction@doubleml\endcsname{0.03}
\expandafter\def\csname lift@v5b@combo_interaction@spacetime_rule\endcsname{8.0}
\expandafter\def\csname len@v5b@combo_interaction@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v5b@combo_interaction@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v5b@combo_interaction@spacetime_rule\endcsname{0.27}
\expandafter\def\csname lift@v5b@control_weak@correlation\endcsname{1.4}
\expandafter\def\csname len@v5b@control_weak@correlation\endcsname{22.2}
\expandafter\def\csname found@v5b@control_weak@correlation\endcsname{2.2}
\expandafter\def\csname beyond@v5b@control_weak@correlation\endcsname{0.20}
\expandafter\def\csname lift@v5b@control_weak@granger\endcsname{2.0}
\expandafter\def\csname len@v5b@control_weak@granger\endcsname{13.0}
\expandafter\def\csname found@v5b@control_weak@granger\endcsname{1.8}
\expandafter\def\csname beyond@v5b@control_weak@granger\endcsname{0.28}
\expandafter\def\csname lift@v5b@control_weak@pcmciplus\endcsname{6.4}
\expandafter\def\csname len@v5b@control_weak@pcmciplus\endcsname{2.3}
\expandafter\def\csname found@v5b@control_weak@pcmciplus\endcsname{1.0}
\expandafter\def\csname beyond@v5b@control_weak@pcmciplus\endcsname{0.32}
\expandafter\def\csname lift@v5b@control_weak@pc\endcsname{3.4}
\expandafter\def\csname len@v5b@control_weak@pc\endcsname{3.9}
\expandafter\def\csname found@v5b@control_weak@pc\endcsname{0.9}
\expandafter\def\csname beyond@v5b@control_weak@pc\endcsname{0.24}
\expandafter\def\csname lift@v5b@control_weak@dynotears\endcsname{--}
\expandafter\def\csname len@v5b@control_weak@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5b@control_weak@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5b@control_weak@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5b@control_weak@varlingam\endcsname{4.3}
\expandafter\def\csname len@v5b@control_weak@varlingam\endcsname{5.4}
\expandafter\def\csname found@v5b@control_weak@varlingam\endcsname{1.6}
\expandafter\def\csname beyond@v5b@control_weak@varlingam\endcsname{0.45}
\expandafter\def\csname lift@v5b@control_weak@doubleml\endcsname{11.0}
\expandafter\def\csname len@v5b@control_weak@doubleml\endcsname{1.2}
\expandafter\def\csname found@v5b@control_weak@doubleml\endcsname{0.9}
\expandafter\def\csname beyond@v5b@control_weak@doubleml\endcsname{0.31}
\expandafter\def\csname lift@v5b@control_weak@spacetime_rule\endcsname{5.5}
\expandafter\def\csname len@v5b@control_weak@spacetime_rule\endcsname{0.8}
\expandafter\def\csname found@v5b@control_weak@spacetime_rule\endcsname{0.3}
\expandafter\def\csname beyond@v5b@control_weak@spacetime_rule\endcsname{0.09}
\expandafter\def\csname lift@v5d@default_b25@correlation\endcsname{1.4}
\expandafter\def\csname len@v5d@default_b25@correlation\endcsname{12.2}
\expandafter\def\csname found@v5d@default_b25@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v5d@default_b25@correlation\endcsname{0.26}
\expandafter\def\csname lift@v5d@default_b25@granger\endcsname{2.5}
\expandafter\def\csname len@v5d@default_b25@granger\endcsname{5.0}
\expandafter\def\csname found@v5d@default_b25@granger\endcsname{1.7}
\expandafter\def\csname beyond@v5d@default_b25@granger\endcsname{0.39}
\expandafter\def\csname lift@v5d@default_b25@pcmciplus\endcsname{4.6}
\expandafter\def\csname len@v5d@default_b25@pcmciplus\endcsname{1.6}
\expandafter\def\csname found@v5d@default_b25@pcmciplus\endcsname{1.0}
\expandafter\def\csname beyond@v5d@default_b25@pcmciplus\endcsname{0.30}
\expandafter\def\csname lift@v5d@default_b25@pc\endcsname{2.9}
\expandafter\def\csname len@v5d@default_b25@pc\endcsname{4.0}
\expandafter\def\csname found@v5d@default_b25@pc\endcsname{1.6}
\expandafter\def\csname beyond@v5d@default_b25@pc\endcsname{0.38}
\expandafter\def\csname lift@v5d@default_b25@dynotears\endcsname{6.3}
\expandafter\def\csname len@v5d@default_b25@dynotears\endcsname{0.7}
\expandafter\def\csname found@v5d@default_b25@dynotears\endcsname{0.6}
\expandafter\def\csname beyond@v5d@default_b25@dynotears\endcsname{0.20}
\expandafter\def\csname lift@v5d@default_b25@varlingam\endcsname{2.6}
\expandafter\def\csname len@v5d@default_b25@varlingam\endcsname{4.7}
\expandafter\def\csname found@v5d@default_b25@varlingam\endcsname{1.7}
\expandafter\def\csname beyond@v5d@default_b25@varlingam\endcsname{0.38}
\expandafter\def\csname lift@v5d@default_b25@doubleml\endcsname{4.6}
\expandafter\def\csname len@v5d@default_b25@doubleml\endcsname{1.9}
\expandafter\def\csname found@v5d@default_b25@doubleml\endcsname{1.2}
\expandafter\def\csname beyond@v5d@default_b25@doubleml\endcsname{0.34}
\expandafter\def\csname lift@v5d@default_b25@spacetime_rule\endcsname{7.3}
\expandafter\def\csname len@v5d@default_b25@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v5d@default_b25@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v5d@default_b25@spacetime_rule\endcsname{0.37}
\expandafter\def\csname lift@v5d@signal_0.1_b25@correlation\endcsname{1.7}
\expandafter\def\csname len@v5d@signal_0.1_b25@correlation\endcsname{4.6}
\expandafter\def\csname found@v5d@signal_0.1_b25@correlation\endcsname{1.1}
\expandafter\def\csname beyond@v5d@signal_0.1_b25@correlation\endcsname{0.17}
\expandafter\def\csname lift@v5d@signal_0.1_b25@granger\endcsname{4.9}
\expandafter\def\csname len@v5d@signal_0.1_b25@granger\endcsname{0.3}
\expandafter\def\csname found@v5d@signal_0.1_b25@granger\endcsname{0.2}
\expandafter\def\csname beyond@v5d@signal_0.1_b25@granger\endcsname{0.06}
\expandafter\def\csname lift@v5d@signal_0.1_b25@pcmciplus\endcsname{6.4}
\expandafter\def\csname len@v5d@signal_0.1_b25@pcmciplus\endcsname{0.8}
\expandafter\def\csname found@v5d@signal_0.1_b25@pcmciplus\endcsname{0.7}
\expandafter\def\csname beyond@v5d@signal_0.1_b25@pcmciplus\endcsname{0.23}
\expandafter\def\csname lift@v5d@signal_0.1_b25@pc\endcsname{1.2}
\expandafter\def\csname len@v5d@signal_0.1_b25@pc\endcsname{2.4}
\expandafter\def\csname found@v5d@signal_0.1_b25@pc\endcsname{0.4}
\expandafter\def\csname beyond@v5d@signal_0.1_b25@pc\endcsname{0.02}
\expandafter\def\csname lift@v5d@signal_0.1_b25@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@signal_0.1_b25@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@signal_0.1_b25@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@signal_0.1_b25@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@signal_0.1_b25@varlingam\endcsname{2.4}
\expandafter\def\csname len@v5d@signal_0.1_b25@varlingam\endcsname{1.5}
\expandafter\def\csname found@v5d@signal_0.1_b25@varlingam\endcsname{0.5}
\expandafter\def\csname beyond@v5d@signal_0.1_b25@varlingam\endcsname{0.10}
\expandafter\def\csname lift@v5d@signal_0.1_b25@doubleml\endcsname{0.0}
\expandafter\def\csname len@v5d@signal_0.1_b25@doubleml\endcsname{0.7}
\expandafter\def\csname found@v5d@signal_0.1_b25@doubleml\endcsname{0.0}
\expandafter\def\csname beyond@v5d@signal_0.1_b25@doubleml\endcsname{-0.04}
\expandafter\def\csname lift@v5d@signal_0.1_b25@spacetime_rule\endcsname{0.0}
\expandafter\def\csname len@v5d@signal_0.1_b25@spacetime_rule\endcsname{0.7}
\expandafter\def\csname found@v5d@signal_0.1_b25@spacetime_rule\endcsname{0.0}
\expandafter\def\csname beyond@v5d@signal_0.1_b25@spacetime_rule\endcsname{-0.03}
\expandafter\def\csname lift@v5d@echo_0.8_b25@correlation\endcsname{1.3}
\expandafter\def\csname len@v5d@echo_0.8_b25@correlation\endcsname{14.3}
\expandafter\def\csname found@v5d@echo_0.8_b25@correlation\endcsname{2.5}
\expandafter\def\csname beyond@v5d@echo_0.8_b25@correlation\endcsname{0.21}
\expandafter\def\csname lift@v5d@echo_0.8_b25@granger\endcsname{2.1}
\expandafter\def\csname len@v5d@echo_0.8_b25@granger\endcsname{6.4}
\expandafter\def\csname found@v5d@echo_0.8_b25@granger\endcsname{1.8}
\expandafter\def\csname beyond@v5d@echo_0.8_b25@granger\endcsname{0.37}
\expandafter\def\csname lift@v5d@echo_0.8_b25@pcmciplus\endcsname{3.9}
\expandafter\def\csname len@v5d@echo_0.8_b25@pcmciplus\endcsname{1.5}
\expandafter\def\csname found@v5d@echo_0.8_b25@pcmciplus\endcsname{0.8}
\expandafter\def\csname beyond@v5d@echo_0.8_b25@pcmciplus\endcsname{0.22}
\expandafter\def\csname lift@v5d@echo_0.8_b25@pc\endcsname{3.1}
\expandafter\def\csname len@v5d@echo_0.8_b25@pc\endcsname{3.1}
\expandafter\def\csname found@v5d@echo_0.8_b25@pc\endcsname{1.3}
\expandafter\def\csname beyond@v5d@echo_0.8_b25@pc\endcsname{0.32}
\expandafter\def\csname lift@v5d@echo_0.8_b25@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@echo_0.8_b25@dynotears\endcsname{0.5}
\expandafter\def\csname found@v5d@echo_0.8_b25@dynotears\endcsname{0.5}
\expandafter\def\csname beyond@v5d@echo_0.8_b25@dynotears\endcsname{0.17}
\expandafter\def\csname lift@v5d@echo_0.8_b25@varlingam\endcsname{1.8}
\expandafter\def\csname len@v5d@echo_0.8_b25@varlingam\endcsname{7.4}
\expandafter\def\csname found@v5d@echo_0.8_b25@varlingam\endcsname{1.8}
\expandafter\def\csname beyond@v5d@echo_0.8_b25@varlingam\endcsname{0.29}
\expandafter\def\csname lift@v5d@echo_0.8_b25@doubleml\endcsname{4.4}
\expandafter\def\csname len@v5d@echo_0.8_b25@doubleml\endcsname{1.0}
\expandafter\def\csname found@v5d@echo_0.8_b25@doubleml\endcsname{0.6}
\expandafter\def\csname beyond@v5d@echo_0.8_b25@doubleml\endcsname{0.17}
\expandafter\def\csname lift@v5d@echo_0.8_b25@spacetime_rule\endcsname{5.5}
\expandafter\def\csname len@v5d@echo_0.8_b25@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v5d@echo_0.8_b25@spacetime_rule\endcsname{0.9}
\expandafter\def\csname beyond@v5d@echo_0.8_b25@spacetime_rule\endcsname{0.28}
\expandafter\def\csname lift@v5d@confound_0.8_b25@correlation\endcsname{1.1}
\expandafter\def\csname len@v5d@confound_0.8_b25@correlation\endcsname{14.5}
\expandafter\def\csname found@v5d@confound_0.8_b25@correlation\endcsname{2.2}
\expandafter\def\csname beyond@v5d@confound_0.8_b25@correlation\endcsname{0.10}
\expandafter\def\csname lift@v5d@confound_0.8_b25@granger\endcsname{1.8}
\expandafter\def\csname len@v5d@confound_0.8_b25@granger\endcsname{8.3}
\expandafter\def\csname found@v5d@confound_0.8_b25@granger\endcsname{2.0}
\expandafter\def\csname beyond@v5d@confound_0.8_b25@granger\endcsname{0.35}
\expandafter\def\csname lift@v5d@confound_0.8_b25@pcmciplus\endcsname{3.7}
\expandafter\def\csname len@v5d@confound_0.8_b25@pcmciplus\endcsname{0.8}
\expandafter\def\csname found@v5d@confound_0.8_b25@pcmciplus\endcsname{0.4}
\expandafter\def\csname beyond@v5d@confound_0.8_b25@pcmciplus\endcsname{0.11}
\expandafter\def\csname lift@v5d@confound_0.8_b25@pc\endcsname{3.4}
\expandafter\def\csname len@v5d@confound_0.8_b25@pc\endcsname{3.0}
\expandafter\def\csname found@v5d@confound_0.8_b25@pc\endcsname{1.4}
\expandafter\def\csname beyond@v5d@confound_0.8_b25@pc\endcsname{0.37}
\expandafter\def\csname lift@v5d@confound_0.8_b25@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@confound_0.8_b25@dynotears\endcsname{0.4}
\expandafter\def\csname found@v5d@confound_0.8_b25@dynotears\endcsname{0.4}
\expandafter\def\csname beyond@v5d@confound_0.8_b25@dynotears\endcsname{0.13}
\expandafter\def\csname lift@v5d@confound_0.8_b25@varlingam\endcsname{2.4}
\expandafter\def\csname len@v5d@confound_0.8_b25@varlingam\endcsname{5.2}
\expandafter\def\csname found@v5d@confound_0.8_b25@varlingam\endcsname{1.7}
\expandafter\def\csname beyond@v5d@confound_0.8_b25@varlingam\endcsname{0.35}
\expandafter\def\csname lift@v5d@confound_0.8_b25@doubleml\endcsname{3.2}
\expandafter\def\csname len@v5d@confound_0.8_b25@doubleml\endcsname{1.8}
\expandafter\def\csname found@v5d@confound_0.8_b25@doubleml\endcsname{0.8}
\expandafter\def\csname beyond@v5d@confound_0.8_b25@doubleml\endcsname{0.21}
\expandafter\def\csname lift@v5d@confound_0.8_b25@spacetime_rule\endcsname{5.3}
\expandafter\def\csname len@v5d@confound_0.8_b25@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v5d@confound_0.8_b25@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v5d@confound_0.8_b25@spacetime_rule\endcsname{0.25}
\expandafter\def\csname lift@v5d@combo_hard_b25@correlation\endcsname{1.4}
\expandafter\def\csname len@v5d@combo_hard_b25@correlation\endcsname{11.8}
\expandafter\def\csname found@v5d@combo_hard_b25@correlation\endcsname{2.2}
\expandafter\def\csname beyond@v5d@combo_hard_b25@correlation\endcsname{0.20}
\expandafter\def\csname lift@v5d@combo_hard_b25@granger\endcsname{2.8}
\expandafter\def\csname len@v5d@combo_hard_b25@granger\endcsname{2.9}
\expandafter\def\csname found@v5d@combo_hard_b25@granger\endcsname{1.1}
\expandafter\def\csname beyond@v5d@combo_hard_b25@granger\endcsname{0.27}
\expandafter\def\csname lift@v5d@combo_hard_b25@pcmciplus\endcsname{3.7}
\expandafter\def\csname len@v5d@combo_hard_b25@pcmciplus\endcsname{1.0}
\expandafter\def\csname found@v5d@combo_hard_b25@pcmciplus\endcsname{0.5}
\expandafter\def\csname beyond@v5d@combo_hard_b25@pcmciplus\endcsname{0.14}
\expandafter\def\csname lift@v5d@combo_hard_b25@pc\endcsname{2.7}
\expandafter\def\csname len@v5d@combo_hard_b25@pc\endcsname{2.7}
\expandafter\def\csname found@v5d@combo_hard_b25@pc\endcsname{1.0}
\expandafter\def\csname beyond@v5d@combo_hard_b25@pc\endcsname{0.24}
\expandafter\def\csname lift@v5d@combo_hard_b25@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@combo_hard_b25@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@combo_hard_b25@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_hard_b25@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@combo_hard_b25@varlingam\endcsname{2.0}
\expandafter\def\csname len@v5d@combo_hard_b25@varlingam\endcsname{4.4}
\expandafter\def\csname found@v5d@combo_hard_b25@varlingam\endcsname{1.2}
\expandafter\def\csname beyond@v5d@combo_hard_b25@varlingam\endcsname{0.20}
\expandafter\def\csname lift@v5d@combo_hard_b25@doubleml\endcsname{1.8}
\expandafter\def\csname len@v5d@combo_hard_b25@doubleml\endcsname{0.4}
\expandafter\def\csname found@v5d@combo_hard_b25@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v5d@combo_hard_b25@doubleml\endcsname{0.01}
\expandafter\def\csname lift@v5d@combo_hard_b25@spacetime_rule\endcsname{2.9}
\expandafter\def\csname len@v5d@combo_hard_b25@spacetime_rule\endcsname{1.0}
\expandafter\def\csname found@v5d@combo_hard_b25@spacetime_rule\endcsname{0.4}
\expandafter\def\csname beyond@v5d@combo_hard_b25@spacetime_rule\endcsname{0.10}
\expandafter\def\csname lift@v5d@combo_extreme_b25@correlation\endcsname{1.5}
\expandafter\def\csname len@v5d@combo_extreme_b25@correlation\endcsname{9.4}
\expandafter\def\csname found@v5d@combo_extreme_b25@correlation\endcsname{1.9}
\expandafter\def\csname beyond@v5d@combo_extreme_b25@correlation\endcsname{0.23}
\expandafter\def\csname lift@v5d@combo_extreme_b25@granger\endcsname{2.6}
\expandafter\def\csname len@v5d@combo_extreme_b25@granger\endcsname{1.4}
\expandafter\def\csname found@v5d@combo_extreme_b25@granger\endcsname{0.5}
\expandafter\def\csname beyond@v5d@combo_extreme_b25@granger\endcsname{0.12}
\expandafter\def\csname lift@v5d@combo_extreme_b25@pcmciplus\endcsname{3.7}
\expandafter\def\csname len@v5d@combo_extreme_b25@pcmciplus\endcsname{0.6}
\expandafter\def\csname found@v5d@combo_extreme_b25@pcmciplus\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_extreme_b25@pcmciplus\endcsname{0.09}
\expandafter\def\csname lift@v5d@combo_extreme_b25@pc\endcsname{1.0}
\expandafter\def\csname len@v5d@combo_extreme_b25@pc\endcsname{2.2}
\expandafter\def\csname found@v5d@combo_extreme_b25@pc\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_extreme_b25@pc\endcsname{-0.01}
\expandafter\def\csname lift@v5d@combo_extreme_b25@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@combo_extreme_b25@dynotears\endcsname{0.1}
\expandafter\def\csname found@v5d@combo_extreme_b25@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v5d@combo_extreme_b25@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v5d@combo_extreme_b25@varlingam\endcsname{1.0}
\expandafter\def\csname len@v5d@combo_extreme_b25@varlingam\endcsname{2.9}
\expandafter\def\csname found@v5d@combo_extreme_b25@varlingam\endcsname{0.4}
\expandafter\def\csname beyond@v5d@combo_extreme_b25@varlingam\endcsname{-0.02}
\expandafter\def\csname lift@v5d@combo_extreme_b25@doubleml\endcsname{0.0}
\expandafter\def\csname len@v5d@combo_extreme_b25@doubleml\endcsname{0.5}
\expandafter\def\csname found@v5d@combo_extreme_b25@doubleml\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_extreme_b25@doubleml\endcsname{-0.02}
\expandafter\def\csname lift@v5d@combo_extreme_b25@spacetime_rule\endcsname{2.0}
\expandafter\def\csname len@v5d@combo_extreme_b25@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v5d@combo_extreme_b25@spacetime_rule\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_extreme_b25@spacetime_rule\endcsname{0.06}
\expandafter\def\csname lift@v5d@interaction_1.0_b25@correlation\endcsname{1.4}
\expandafter\def\csname len@v5d@interaction_1.0_b25@correlation\endcsname{3.2}
\expandafter\def\csname found@v5d@interaction_1.0_b25@correlation\endcsname{0.6}
\expandafter\def\csname beyond@v5d@interaction_1.0_b25@correlation\endcsname{0.08}
\expandafter\def\csname lift@v5d@interaction_1.0_b25@granger\endcsname{1.7}
\expandafter\def\csname len@v5d@interaction_1.0_b25@granger\endcsname{1.7}
\expandafter\def\csname found@v5d@interaction_1.0_b25@granger\endcsname{0.4}
\expandafter\def\csname beyond@v5d@interaction_1.0_b25@granger\endcsname{0.09}
\expandafter\def\csname lift@v5d@interaction_1.0_b25@pcmciplus\endcsname{2.4}
\expandafter\def\csname len@v5d@interaction_1.0_b25@pcmciplus\endcsname{1.5}
\expandafter\def\csname found@v5d@interaction_1.0_b25@pcmciplus\endcsname{0.5}
\expandafter\def\csname beyond@v5d@interaction_1.0_b25@pcmciplus\endcsname{0.12}
\expandafter\def\csname lift@v5d@interaction_1.0_b25@pc\endcsname{0.9}
\expandafter\def\csname len@v5d@interaction_1.0_b25@pc\endcsname{2.5}
\expandafter\def\csname found@v5d@interaction_1.0_b25@pc\endcsname{0.3}
\expandafter\def\csname beyond@v5d@interaction_1.0_b25@pc\endcsname{-0.02}
\expandafter\def\csname lift@v5d@interaction_1.0_b25@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@interaction_1.0_b25@dynotears\endcsname{0.1}
\expandafter\def\csname found@v5d@interaction_1.0_b25@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v5d@interaction_1.0_b25@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v5d@interaction_1.0_b25@varlingam\endcsname{2.0}
\expandafter\def\csname len@v5d@interaction_1.0_b25@varlingam\endcsname{1.1}
\expandafter\def\csname found@v5d@interaction_1.0_b25@varlingam\endcsname{0.3}
\expandafter\def\csname beyond@v5d@interaction_1.0_b25@varlingam\endcsname{0.07}
\expandafter\def\csname lift@v5d@interaction_1.0_b25@doubleml\endcsname{3.7}
\expandafter\def\csname len@v5d@interaction_1.0_b25@doubleml\endcsname{0.2}
\expandafter\def\csname found@v5d@interaction_1.0_b25@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v5d@interaction_1.0_b25@doubleml\endcsname{0.03}
\expandafter\def\csname lift@v5d@interaction_1.0_b25@spacetime_rule\endcsname{7.3}
\expandafter\def\csname len@v5d@interaction_1.0_b25@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v5d@interaction_1.0_b25@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v5d@interaction_1.0_b25@spacetime_rule\endcsname{0.40}
\expandafter\def\csname lift@v5d@combo_interaction_b25@correlation\endcsname{0.7}
\expandafter\def\csname len@v5d@combo_interaction_b25@correlation\endcsname{4.0}
\expandafter\def\csname found@v5d@combo_interaction_b25@correlation\endcsname{0.4}
\expandafter\def\csname beyond@v5d@combo_interaction_b25@correlation\endcsname{-0.04}
\expandafter\def\csname lift@v5d@combo_interaction_b25@granger\endcsname{3.0}
\expandafter\def\csname len@v5d@combo_interaction_b25@granger\endcsname{1.2}
\expandafter\def\csname found@v5d@combo_interaction_b25@granger\endcsname{0.5}
\expandafter\def\csname beyond@v5d@combo_interaction_b25@granger\endcsname{0.15}
\expandafter\def\csname lift@v5d@combo_interaction_b25@pcmciplus\endcsname{1.5}
\expandafter\def\csname len@v5d@combo_interaction_b25@pcmciplus\endcsname{1.0}
\expandafter\def\csname found@v5d@combo_interaction_b25@pcmciplus\endcsname{0.2}
\expandafter\def\csname beyond@v5d@combo_interaction_b25@pcmciplus\endcsname{0.02}
\expandafter\def\csname lift@v5d@combo_interaction_b25@pc\endcsname{1.1}
\expandafter\def\csname len@v5d@combo_interaction_b25@pc\endcsname{2.0}
\expandafter\def\csname found@v5d@combo_interaction_b25@pc\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_interaction_b25@pc\endcsname{0.01}
\expandafter\def\csname lift@v5d@combo_interaction_b25@dynotears\endcsname{0.0}
\expandafter\def\csname len@v5d@combo_interaction_b25@dynotears\endcsname{0.1}
\expandafter\def\csname found@v5d@combo_interaction_b25@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_interaction_b25@dynotears\endcsname{-0.00}
\expandafter\def\csname lift@v5d@combo_interaction_b25@varlingam\endcsname{1.3}
\expandafter\def\csname len@v5d@combo_interaction_b25@varlingam\endcsname{1.7}
\expandafter\def\csname found@v5d@combo_interaction_b25@varlingam\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_interaction_b25@varlingam\endcsname{0.04}
\expandafter\def\csname lift@v5d@combo_interaction_b25@doubleml\endcsname{--}
\expandafter\def\csname len@v5d@combo_interaction_b25@doubleml\endcsname{0.0}
\expandafter\def\csname found@v5d@combo_interaction_b25@doubleml\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_interaction_b25@doubleml\endcsname{0.00}
\expandafter\def\csname lift@v5d@combo_interaction_b25@spacetime_rule\endcsname{4.9}
\expandafter\def\csname len@v5d@combo_interaction_b25@spacetime_rule\endcsname{0.9}
\expandafter\def\csname found@v5d@combo_interaction_b25@spacetime_rule\endcsname{0.6}
\expandafter\def\csname beyond@v5d@combo_interaction_b25@spacetime_rule\endcsname{0.18}
\expandafter\def\csname lift@v5d@control_weak_b25@correlation\endcsname{2.1}
\expandafter\def\csname len@v5d@control_weak_b25@correlation\endcsname{5.4}
\expandafter\def\csname found@v5d@control_weak_b25@correlation\endcsname{1.6}
\expandafter\def\csname beyond@v5d@control_weak_b25@correlation\endcsname{0.27}
\expandafter\def\csname lift@v5d@control_weak_b25@granger\endcsname{5.5}
\expandafter\def\csname len@v5d@control_weak_b25@granger\endcsname{0.5}
\expandafter\def\csname found@v5d@control_weak_b25@granger\endcsname{0.4}
\expandafter\def\csname beyond@v5d@control_weak_b25@granger\endcsname{0.13}
\expandafter\def\csname lift@v5d@control_weak_b25@pcmciplus\endcsname{3.8}
\expandafter\def\csname len@v5d@control_weak_b25@pcmciplus\endcsname{1.1}
\expandafter\def\csname found@v5d@control_weak_b25@pcmciplus\endcsname{0.6}
\expandafter\def\csname beyond@v5d@control_weak_b25@pcmciplus\endcsname{0.17}
\expandafter\def\csname lift@v5d@control_weak_b25@pc\endcsname{1.6}
\expandafter\def\csname len@v5d@control_weak_b25@pc\endcsname{3.1}
\expandafter\def\csname found@v5d@control_weak_b25@pc\endcsname{0.7}
\expandafter\def\csname beyond@v5d@control_weak_b25@pc\endcsname{0.09}
\expandafter\def\csname lift@v5d@control_weak_b25@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@control_weak_b25@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@control_weak_b25@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@control_weak_b25@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@control_weak_b25@varlingam\endcsname{3.6}
\expandafter\def\csname len@v5d@control_weak_b25@varlingam\endcsname{1.9}
\expandafter\def\csname found@v5d@control_weak_b25@varlingam\endcsname{1.0}
\expandafter\def\csname beyond@v5d@control_weak_b25@varlingam\endcsname{0.27}
\expandafter\def\csname lift@v5d@control_weak_b25@doubleml\endcsname{0.9}
\expandafter\def\csname len@v5d@control_weak_b25@doubleml\endcsname{0.8}
\expandafter\def\csname found@v5d@control_weak_b25@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v5d@control_weak_b25@doubleml\endcsname{-0.01}
\expandafter\def\csname lift@v5d@control_weak_b25@spacetime_rule\endcsname{1.2}
\expandafter\def\csname len@v5d@control_weak_b25@spacetime_rule\endcsname{0.6}
\expandafter\def\csname found@v5d@control_weak_b25@spacetime_rule\endcsname{0.1}
\expandafter\def\csname beyond@v5d@control_weak_b25@spacetime_rule\endcsname{0.01}
\expandafter\def\csname lift@v5d@default_b50@correlation\endcsname{1.1}
\expandafter\def\csname len@v5d@default_b50@correlation\endcsname{16.7}
\expandafter\def\csname found@v5d@default_b50@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v5d@default_b50@correlation\endcsname{0.13}
\expandafter\def\csname lift@v5d@default_b50@granger\endcsname{1.6}
\expandafter\def\csname len@v5d@default_b50@granger\endcsname{10.3}
\expandafter\def\csname found@v5d@default_b50@granger\endcsname{2.2}
\expandafter\def\csname beyond@v5d@default_b50@granger\endcsname{0.33}
\expandafter\def\csname lift@v5d@default_b50@pcmciplus\endcsname{6.4}
\expandafter\def\csname len@v5d@default_b50@pcmciplus\endcsname{2.3}
\expandafter\def\csname found@v5d@default_b50@pcmciplus\endcsname{2.0}
\expandafter\def\csname beyond@v5d@default_b50@pcmciplus\endcsname{0.63}
\expandafter\def\csname lift@v5d@default_b50@pc\endcsname{3.6}
\expandafter\def\csname len@v5d@default_b50@pc\endcsname{4.1}
\expandafter\def\csname found@v5d@default_b50@pc\endcsname{2.0}
\expandafter\def\csname beyond@v5d@default_b50@pc\endcsname{0.53}
\expandafter\def\csname lift@v5d@default_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@default_b50@dynotears\endcsname{0.9}
\expandafter\def\csname found@v5d@default_b50@dynotears\endcsname{0.9}
\expandafter\def\csname beyond@v5d@default_b50@dynotears\endcsname{0.30}
\expandafter\def\csname lift@v5d@default_b50@varlingam\endcsname{2.8}
\expandafter\def\csname len@v5d@default_b50@varlingam\endcsname{5.8}
\expandafter\def\csname found@v5d@default_b50@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v5d@default_b50@varlingam\endcsname{0.52}
\expandafter\def\csname lift@v5d@default_b50@doubleml\endcsname{5.7}
\expandafter\def\csname len@v5d@default_b50@doubleml\endcsname{2.3}
\expandafter\def\csname found@v5d@default_b50@doubleml\endcsname{1.8}
\expandafter\def\csname beyond@v5d@default_b50@doubleml\endcsname{0.56}
\expandafter\def\csname lift@v5d@default_b50@spacetime_rule\endcsname{6.5}
\expandafter\def\csname len@v5d@default_b50@spacetime_rule\endcsname{0.9}
\expandafter\def\csname found@v5d@default_b50@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v5d@default_b50@spacetime_rule\endcsname{0.26}
\expandafter\def\csname lift@v5d@signal_0.1_b50@correlation\endcsname{1.6}
\expandafter\def\csname len@v5d@signal_0.1_b50@correlation\endcsname{9.0}
\expandafter\def\csname found@v5d@signal_0.1_b50@correlation\endcsname{2.0}
\expandafter\def\csname beyond@v5d@signal_0.1_b50@correlation\endcsname{0.28}
\expandafter\def\csname lift@v5d@signal_0.1_b50@granger\endcsname{3.9}
\expandafter\def\csname len@v5d@signal_0.1_b50@granger\endcsname{2.6}
\expandafter\def\csname found@v5d@signal_0.1_b50@granger\endcsname{1.4}
\expandafter\def\csname beyond@v5d@signal_0.1_b50@granger\endcsname{0.40}
\expandafter\def\csname lift@v5d@signal_0.1_b50@pcmciplus\endcsname{4.5}
\expandafter\def\csname len@v5d@signal_0.1_b50@pcmciplus\endcsname{1.3}
\expandafter\def\csname found@v5d@signal_0.1_b50@pcmciplus\endcsname{0.8}
\expandafter\def\csname beyond@v5d@signal_0.1_b50@pcmciplus\endcsname{0.23}
\expandafter\def\csname lift@v5d@signal_0.1_b50@pc\endcsname{1.7}
\expandafter\def\csname len@v5d@signal_0.1_b50@pc\endcsname{3.4}
\expandafter\def\csname found@v5d@signal_0.1_b50@pc\endcsname{0.8}
\expandafter\def\csname beyond@v5d@signal_0.1_b50@pc\endcsname{0.12}
\expandafter\def\csname lift@v5d@signal_0.1_b50@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@signal_0.1_b50@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@signal_0.1_b50@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@signal_0.1_b50@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@signal_0.1_b50@varlingam\endcsname{2.7}
\expandafter\def\csname len@v5d@signal_0.1_b50@varlingam\endcsname{3.3}
\expandafter\def\csname found@v5d@signal_0.1_b50@varlingam\endcsname{1.2}
\expandafter\def\csname beyond@v5d@signal_0.1_b50@varlingam\endcsname{0.28}
\expandafter\def\csname lift@v5d@signal_0.1_b50@doubleml\endcsname{5.7}
\expandafter\def\csname len@v5d@signal_0.1_b50@doubleml\endcsname{0.9}
\expandafter\def\csname found@v5d@signal_0.1_b50@doubleml\endcsname{0.7}
\expandafter\def\csname beyond@v5d@signal_0.1_b50@doubleml\endcsname{0.22}
\expandafter\def\csname lift@v5d@signal_0.1_b50@spacetime_rule\endcsname{--}
\expandafter\def\csname len@v5d@signal_0.1_b50@spacetime_rule\endcsname{0.0}
\expandafter\def\csname found@v5d@signal_0.1_b50@spacetime_rule\endcsname{0.0}
\expandafter\def\csname beyond@v5d@signal_0.1_b50@spacetime_rule\endcsname{0.00}
\expandafter\def\csname lift@v5d@echo_0.8_b50@correlation\endcsname{1.1}
\expandafter\def\csname len@v5d@echo_0.8_b50@correlation\endcsname{17.1}
\expandafter\def\csname found@v5d@echo_0.8_b50@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v5d@echo_0.8_b50@correlation\endcsname{0.11}
\expandafter\def\csname lift@v5d@echo_0.8_b50@granger\endcsname{1.5}
\expandafter\def\csname len@v5d@echo_0.8_b50@granger\endcsname{10.9}
\expandafter\def\csname found@v5d@echo_0.8_b50@granger\endcsname{2.2}
\expandafter\def\csname beyond@v5d@echo_0.8_b50@granger\endcsname{0.27}
\expandafter\def\csname lift@v5d@echo_0.8_b50@pcmciplus\endcsname{5.7}
\expandafter\def\csname len@v5d@echo_0.8_b50@pcmciplus\endcsname{1.8}
\expandafter\def\csname found@v5d@echo_0.8_b50@pcmciplus\endcsname{1.4}
\expandafter\def\csname beyond@v5d@echo_0.8_b50@pcmciplus\endcsname{0.45}
\expandafter\def\csname lift@v5d@echo_0.8_b50@pc\endcsname{2.7}
\expandafter\def\csname len@v5d@echo_0.8_b50@pc\endcsname{4.1}
\expandafter\def\csname found@v5d@echo_0.8_b50@pc\endcsname{1.5}
\expandafter\def\csname beyond@v5d@echo_0.8_b50@pc\endcsname{0.35}
\expandafter\def\csname lift@v5d@echo_0.8_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@echo_0.8_b50@dynotears\endcsname{0.5}
\expandafter\def\csname found@v5d@echo_0.8_b50@dynotears\endcsname{0.5}
\expandafter\def\csname beyond@v5d@echo_0.8_b50@dynotears\endcsname{0.16}
\expandafter\def\csname lift@v5d@echo_0.8_b50@varlingam\endcsname{2.2}
\expandafter\def\csname len@v5d@echo_0.8_b50@varlingam\endcsname{5.6}
\expandafter\def\csname found@v5d@echo_0.8_b50@varlingam\endcsname{1.7}
\expandafter\def\csname beyond@v5d@echo_0.8_b50@varlingam\endcsname{0.33}
\expandafter\def\csname lift@v5d@echo_0.8_b50@doubleml\endcsname{5.7}
\expandafter\def\csname len@v5d@echo_0.8_b50@doubleml\endcsname{1.4}
\expandafter\def\csname found@v5d@echo_0.8_b50@doubleml\endcsname{1.1}
\expandafter\def\csname beyond@v5d@echo_0.8_b50@doubleml\endcsname{0.34}
\expandafter\def\csname lift@v5d@echo_0.8_b50@spacetime_rule\endcsname{4.3}
\expandafter\def\csname len@v5d@echo_0.8_b50@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v5d@echo_0.8_b50@spacetime_rule\endcsname{0.7}
\expandafter\def\csname beyond@v5d@echo_0.8_b50@spacetime_rule\endcsname{0.21}
\expandafter\def\csname lift@v5d@confound_0.8_b50@correlation\endcsname{1.0}
\expandafter\def\csname len@v5d@confound_0.8_b50@correlation\endcsname{16.4}
\expandafter\def\csname found@v5d@confound_0.8_b50@correlation\endcsname{2.2}
\expandafter\def\csname beyond@v5d@confound_0.8_b50@correlation\endcsname{-0.00}
\expandafter\def\csname lift@v5d@confound_0.8_b50@granger\endcsname{1.2}
\expandafter\def\csname len@v5d@confound_0.8_b50@granger\endcsname{11.7}
\expandafter\def\csname found@v5d@confound_0.8_b50@granger\endcsname{2.0}
\expandafter\def\csname beyond@v5d@confound_0.8_b50@granger\endcsname{0.18}
\expandafter\def\csname lift@v5d@confound_0.8_b50@pcmciplus\endcsname{5.0}
\expandafter\def\csname len@v5d@confound_0.8_b50@pcmciplus\endcsname{1.9}
\expandafter\def\csname found@v5d@confound_0.8_b50@pcmciplus\endcsname{1.3}
\expandafter\def\csname beyond@v5d@confound_0.8_b50@pcmciplus\endcsname{0.39}
\expandafter\def\csname lift@v5d@confound_0.8_b50@pc\endcsname{2.9}
\expandafter\def\csname len@v5d@confound_0.8_b50@pc\endcsname{3.5}
\expandafter\def\csname found@v5d@confound_0.8_b50@pc\endcsname{1.4}
\expandafter\def\csname beyond@v5d@confound_0.8_b50@pc\endcsname{0.35}
\expandafter\def\csname lift@v5d@confound_0.8_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@confound_0.8_b50@dynotears\endcsname{0.3}
\expandafter\def\csname found@v5d@confound_0.8_b50@dynotears\endcsname{0.3}
\expandafter\def\csname beyond@v5d@confound_0.8_b50@dynotears\endcsname{0.10}
\expandafter\def\csname lift@v5d@confound_0.8_b50@varlingam\endcsname{2.6}
\expandafter\def\csname len@v5d@confound_0.8_b50@varlingam\endcsname{5.0}
\expandafter\def\csname found@v5d@confound_0.8_b50@varlingam\endcsname{1.8}
\expandafter\def\csname beyond@v5d@confound_0.8_b50@varlingam\endcsname{0.42}
\expandafter\def\csname lift@v5d@confound_0.8_b50@doubleml\endcsname{4.5}
\expandafter\def\csname len@v5d@confound_0.8_b50@doubleml\endcsname{2.1}
\expandafter\def\csname found@v5d@confound_0.8_b50@doubleml\endcsname{1.3}
\expandafter\def\csname beyond@v5d@confound_0.8_b50@doubleml\endcsname{0.38}
\expandafter\def\csname lift@v5d@confound_0.8_b50@spacetime_rule\endcsname{3.4}
\expandafter\def\csname len@v5d@confound_0.8_b50@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v5d@confound_0.8_b50@spacetime_rule\endcsname{0.6}
\expandafter\def\csname beyond@v5d@confound_0.8_b50@spacetime_rule\endcsname{0.17}
\expandafter\def\csname lift@v5d@combo_hard_b50@correlation\endcsname{1.1}
\expandafter\def\csname len@v5d@combo_hard_b50@correlation\endcsname{14.8}
\expandafter\def\csname found@v5d@combo_hard_b50@correlation\endcsname{2.3}
\expandafter\def\csname beyond@v5d@combo_hard_b50@correlation\endcsname{0.12}
\expandafter\def\csname lift@v5d@combo_hard_b50@granger\endcsname{2.2}
\expandafter\def\csname len@v5d@combo_hard_b50@granger\endcsname{6.2}
\expandafter\def\csname found@v5d@combo_hard_b50@granger\endcsname{1.9}
\expandafter\def\csname beyond@v5d@combo_hard_b50@granger\endcsname{0.43}
\expandafter\def\csname lift@v5d@combo_hard_b50@pcmciplus\endcsname{6.1}
\expandafter\def\csname len@v5d@combo_hard_b50@pcmciplus\endcsname{1.2}
\expandafter\def\csname found@v5d@combo_hard_b50@pcmciplus\endcsname{1.0}
\expandafter\def\csname beyond@v5d@combo_hard_b50@pcmciplus\endcsname{0.32}
\expandafter\def\csname lift@v5d@combo_hard_b50@pc\endcsname{2.5}
\expandafter\def\csname len@v5d@combo_hard_b50@pc\endcsname{2.9}
\expandafter\def\csname found@v5d@combo_hard_b50@pc\endcsname{1.0}
\expandafter\def\csname beyond@v5d@combo_hard_b50@pc\endcsname{0.23}
\expandafter\def\csname lift@v5d@combo_hard_b50@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@combo_hard_b50@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@combo_hard_b50@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_hard_b50@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@combo_hard_b50@varlingam\endcsname{1.7}
\expandafter\def\csname len@v5d@combo_hard_b50@varlingam\endcsname{5.9}
\expandafter\def\csname found@v5d@combo_hard_b50@varlingam\endcsname{1.4}
\expandafter\def\csname beyond@v5d@combo_hard_b50@varlingam\endcsname{0.20}
\expandafter\def\csname lift@v5d@combo_hard_b50@doubleml\endcsname{1.5}
\expandafter\def\csname len@v5d@combo_hard_b50@doubleml\endcsname{0.5}
\expandafter\def\csname found@v5d@combo_hard_b50@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v5d@combo_hard_b50@doubleml\endcsname{0.02}
\expandafter\def\csname lift@v5d@combo_hard_b50@spacetime_rule\endcsname{2.0}
\expandafter\def\csname len@v5d@combo_hard_b50@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v5d@combo_hard_b50@spacetime_rule\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_hard_b50@spacetime_rule\endcsname{0.06}
\expandafter\def\csname lift@v5d@combo_extreme_b50@correlation\endcsname{1.1}
\expandafter\def\csname len@v5d@combo_extreme_b50@correlation\endcsname{13.6}
\expandafter\def\csname found@v5d@combo_extreme_b50@correlation\endcsname{2.1}
\expandafter\def\csname beyond@v5d@combo_extreme_b50@correlation\endcsname{0.12}
\expandafter\def\csname lift@v5d@combo_extreme_b50@granger\endcsname{1.8}
\expandafter\def\csname len@v5d@combo_extreme_b50@granger\endcsname{6.6}
\expandafter\def\csname found@v5d@combo_extreme_b50@granger\endcsname{1.6}
\expandafter\def\csname beyond@v5d@combo_extreme_b50@granger\endcsname{0.32}
\expandafter\def\csname lift@v5d@combo_extreme_b50@pcmciplus\endcsname{4.2}
\expandafter\def\csname len@v5d@combo_extreme_b50@pcmciplus\endcsname{0.7}
\expandafter\def\csname found@v5d@combo_extreme_b50@pcmciplus\endcsname{0.4}
\expandafter\def\csname beyond@v5d@combo_extreme_b50@pcmciplus\endcsname{0.12}
\expandafter\def\csname lift@v5d@combo_extreme_b50@pc\endcsname{1.2}
\expandafter\def\csname len@v5d@combo_extreme_b50@pc\endcsname{2.5}
\expandafter\def\csname found@v5d@combo_extreme_b50@pc\endcsname{0.4}
\expandafter\def\csname beyond@v5d@combo_extreme_b50@pc\endcsname{0.02}
\expandafter\def\csname lift@v5d@combo_extreme_b50@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@combo_extreme_b50@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@combo_extreme_b50@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_extreme_b50@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@combo_extreme_b50@varlingam\endcsname{1.5}
\expandafter\def\csname len@v5d@combo_extreme_b50@varlingam\endcsname{5.3}
\expandafter\def\csname found@v5d@combo_extreme_b50@varlingam\endcsname{1.1}
\expandafter\def\csname beyond@v5d@combo_extreme_b50@varlingam\endcsname{0.12}
\expandafter\def\csname lift@v5d@combo_extreme_b50@doubleml\endcsname{0.0}
\expandafter\def\csname len@v5d@combo_extreme_b50@doubleml\endcsname{0.2}
\expandafter\def\csname found@v5d@combo_extreme_b50@doubleml\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_extreme_b50@doubleml\endcsname{-0.01}
\expandafter\def\csname lift@v5d@combo_extreme_b50@spacetime_rule\endcsname{2.9}
\expandafter\def\csname len@v5d@combo_extreme_b50@spacetime_rule\endcsname{1.0}
\expandafter\def\csname found@v5d@combo_extreme_b50@spacetime_rule\endcsname{0.4}
\expandafter\def\csname beyond@v5d@combo_extreme_b50@spacetime_rule\endcsname{0.10}
\expandafter\def\csname lift@v5d@interaction_1.0_b50@correlation\endcsname{1.0}
\expandafter\def\csname len@v5d@interaction_1.0_b50@correlation\endcsname{5.8}
\expandafter\def\csname found@v5d@interaction_1.0_b50@correlation\endcsname{0.8}
\expandafter\def\csname beyond@v5d@interaction_1.0_b50@correlation\endcsname{0.03}
\expandafter\def\csname lift@v5d@interaction_1.0_b50@granger\endcsname{1.1}
\expandafter\def\csname len@v5d@interaction_1.0_b50@granger\endcsname{4.1}
\expandafter\def\csname found@v5d@interaction_1.0_b50@granger\endcsname{0.6}
\expandafter\def\csname beyond@v5d@interaction_1.0_b50@granger\endcsname{0.03}
\expandafter\def\csname lift@v5d@interaction_1.0_b50@pcmciplus\endcsname{3.7}
\expandafter\def\csname len@v5d@interaction_1.0_b50@pcmciplus\endcsname{1.4}
\expandafter\def\csname found@v5d@interaction_1.0_b50@pcmciplus\endcsname{0.7}
\expandafter\def\csname beyond@v5d@interaction_1.0_b50@pcmciplus\endcsname{0.19}
\expandafter\def\csname lift@v5d@interaction_1.0_b50@pc\endcsname{0.8}
\expandafter\def\csname len@v5d@interaction_1.0_b50@pc\endcsname{2.9}
\expandafter\def\csname found@v5d@interaction_1.0_b50@pc\endcsname{0.3}
\expandafter\def\csname beyond@v5d@interaction_1.0_b50@pc\endcsname{-0.05}
\expandafter\def\csname lift@v5d@interaction_1.0_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@interaction_1.0_b50@dynotears\endcsname{0.1}
\expandafter\def\csname found@v5d@interaction_1.0_b50@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v5d@interaction_1.0_b50@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v5d@interaction_1.0_b50@varlingam\endcsname{2.1}
\expandafter\def\csname len@v5d@interaction_1.0_b50@varlingam\endcsname{1.7}
\expandafter\def\csname found@v5d@interaction_1.0_b50@varlingam\endcsname{0.5}
\expandafter\def\csname beyond@v5d@interaction_1.0_b50@varlingam\endcsname{0.10}
\expandafter\def\csname lift@v5d@interaction_1.0_b50@doubleml\endcsname{3.7}
\expandafter\def\csname len@v5d@interaction_1.0_b50@doubleml\endcsname{0.6}
\expandafter\def\csname found@v5d@interaction_1.0_b50@doubleml\endcsname{0.3}
\expandafter\def\csname beyond@v5d@interaction_1.0_b50@doubleml\endcsname{0.09}
\expandafter\def\csname lift@v5d@interaction_1.0_b50@spacetime_rule\endcsname{6.1}
\expandafter\def\csname len@v5d@interaction_1.0_b50@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v5d@interaction_1.0_b50@spacetime_rule\endcsname{1.0}
\expandafter\def\csname beyond@v5d@interaction_1.0_b50@spacetime_rule\endcsname{0.32}
\expandafter\def\csname lift@v5d@combo_interaction_b50@correlation\endcsname{0.9}
\expandafter\def\csname len@v5d@combo_interaction_b50@correlation\endcsname{4.9}
\expandafter\def\csname found@v5d@combo_interaction_b50@correlation\endcsname{0.6}
\expandafter\def\csname beyond@v5d@combo_interaction_b50@correlation\endcsname{0.01}
\expandafter\def\csname lift@v5d@combo_interaction_b50@granger\endcsname{1.1}
\expandafter\def\csname len@v5d@combo_interaction_b50@granger\endcsname{2.7}
\expandafter\def\csname found@v5d@combo_interaction_b50@granger\endcsname{0.4}
\expandafter\def\csname beyond@v5d@combo_interaction_b50@granger\endcsname{0.06}
\expandafter\def\csname lift@v5d@combo_interaction_b50@pcmciplus\endcsname{4.4}
\expandafter\def\csname len@v5d@combo_interaction_b50@pcmciplus\endcsname{0.5}
\expandafter\def\csname found@v5d@combo_interaction_b50@pcmciplus\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_interaction_b50@pcmciplus\endcsname{0.10}
\expandafter\def\csname lift@v5d@combo_interaction_b50@pc\endcsname{0.9}
\expandafter\def\csname len@v5d@combo_interaction_b50@pc\endcsname{2.4}
\expandafter\def\csname found@v5d@combo_interaction_b50@pc\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_interaction_b50@pc\endcsname{-0.02}
\expandafter\def\csname lift@v5d@combo_interaction_b50@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@combo_interaction_b50@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@combo_interaction_b50@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_interaction_b50@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@combo_interaction_b50@varlingam\endcsname{1.6}
\expandafter\def\csname len@v5d@combo_interaction_b50@varlingam\endcsname{1.8}
\expandafter\def\csname found@v5d@combo_interaction_b50@varlingam\endcsname{0.4}
\expandafter\def\csname beyond@v5d@combo_interaction_b50@varlingam\endcsname{0.07}
\expandafter\def\csname lift@v5d@combo_interaction_b50@doubleml\endcsname{4.9}
\expandafter\def\csname len@v5d@combo_interaction_b50@doubleml\endcsname{0.3}
\expandafter\def\csname found@v5d@combo_interaction_b50@doubleml\endcsname{0.2}
\expandafter\def\csname beyond@v5d@combo_interaction_b50@doubleml\endcsname{0.06}
\expandafter\def\csname lift@v5d@combo_interaction_b50@spacetime_rule\endcsname{2.1}
\expandafter\def\csname len@v5d@combo_interaction_b50@spacetime_rule\endcsname{0.7}
\expandafter\def\csname found@v5d@combo_interaction_b50@spacetime_rule\endcsname{0.2}
\expandafter\def\csname beyond@v5d@combo_interaction_b50@spacetime_rule\endcsname{0.04}
\expandafter\def\csname lift@v5d@control_weak_b50@correlation\endcsname{1.7}
\expandafter\def\csname len@v5d@control_weak_b50@correlation\endcsname{8.2}
\expandafter\def\csname found@v5d@control_weak_b50@correlation\endcsname{2.0}
\expandafter\def\csname beyond@v5d@control_weak_b50@correlation\endcsname{0.26}
\expandafter\def\csname lift@v5d@control_weak_b50@granger\endcsname{3.7}
\expandafter\def\csname len@v5d@control_weak_b50@granger\endcsname{3.2}
\expandafter\def\csname found@v5d@control_weak_b50@granger\endcsname{1.7}
\expandafter\def\csname beyond@v5d@control_weak_b50@granger\endcsname{0.45}
\expandafter\def\csname lift@v5d@control_weak_b50@pcmciplus\endcsname{5.6}
\expandafter\def\csname len@v5d@control_weak_b50@pcmciplus\endcsname{1.6}
\expandafter\def\csname found@v5d@control_weak_b50@pcmciplus\endcsname{1.3}
\expandafter\def\csname beyond@v5d@control_weak_b50@pcmciplus\endcsname{0.41}
\expandafter\def\csname lift@v5d@control_weak_b50@pc\endcsname{2.0}
\expandafter\def\csname len@v5d@control_weak_b50@pc\endcsname{3.9}
\expandafter\def\csname found@v5d@control_weak_b50@pc\endcsname{1.1}
\expandafter\def\csname beyond@v5d@control_weak_b50@pc\endcsname{0.19}
\expandafter\def\csname lift@v5d@control_weak_b50@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@control_weak_b50@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@control_weak_b50@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@control_weak_b50@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@control_weak_b50@varlingam\endcsname{3.2}
\expandafter\def\csname len@v5d@control_weak_b50@varlingam\endcsname{2.6}
\expandafter\def\csname found@v5d@control_weak_b50@varlingam\endcsname{1.2}
\expandafter\def\csname beyond@v5d@control_weak_b50@varlingam\endcsname{0.30}
\expandafter\def\csname lift@v5d@control_weak_b50@doubleml\endcsname{5.1}
\expandafter\def\csname len@v5d@control_weak_b50@doubleml\endcsname{1.5}
\expandafter\def\csname found@v5d@control_weak_b50@doubleml\endcsname{1.1}
\expandafter\def\csname beyond@v5d@control_weak_b50@doubleml\endcsname{0.33}
\expandafter\def\csname lift@v5d@control_weak_b50@spacetime_rule\endcsname{--}
\expandafter\def\csname len@v5d@control_weak_b50@spacetime_rule\endcsname{0.0}
\expandafter\def\csname found@v5d@control_weak_b50@spacetime_rule\endcsname{0.0}
\expandafter\def\csname beyond@v5d@control_weak_b50@spacetime_rule\endcsname{0.00}
\expandafter\def\csname lift@v5d@default_b100@correlation\endcsname{1.1}
\expandafter\def\csname len@v5d@default_b100@correlation\endcsname{17.3}
\expandafter\def\csname found@v5d@default_b100@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v5d@default_b100@correlation\endcsname{0.09}
\expandafter\def\csname lift@v5d@default_b100@granger\endcsname{1.2}
\expandafter\def\csname len@v5d@default_b100@granger\endcsname{14.6}
\expandafter\def\csname found@v5d@default_b100@granger\endcsname{2.4}
\expandafter\def\csname beyond@v5d@default_b100@granger\endcsname{0.16}
\expandafter\def\csname lift@v5d@default_b100@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v5d@default_b100@pcmciplus\endcsname{3.0}
\expandafter\def\csname found@v5d@default_b100@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v5d@default_b100@pcmciplus\endcsname{0.67}
\expandafter\def\csname lift@v5d@default_b100@pc\endcsname{2.9}
\expandafter\def\csname len@v5d@default_b100@pc\endcsname{4.6}
\expandafter\def\csname found@v5d@default_b100@pc\endcsname{1.8}
\expandafter\def\csname beyond@v5d@default_b100@pc\endcsname{0.43}
\expandafter\def\csname lift@v5d@default_b100@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@default_b100@dynotears\endcsname{0.7}
\expandafter\def\csname found@v5d@default_b100@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v5d@default_b100@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v5d@default_b100@varlingam\endcsname{1.8}
\expandafter\def\csname len@v5d@default_b100@varlingam\endcsname{9.5}
\expandafter\def\csname found@v5d@default_b100@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v5d@default_b100@varlingam\endcsname{0.40}
\expandafter\def\csname lift@v5d@default_b100@doubleml\endcsname{5.4}
\expandafter\def\csname len@v5d@default_b100@doubleml\endcsname{3.1}
\expandafter\def\csname found@v5d@default_b100@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v5d@default_b100@doubleml\endcsname{0.69}
\expandafter\def\csname lift@v5d@default_b100@spacetime_rule\endcsname{6.7}
\expandafter\def\csname len@v5d@default_b100@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v5d@default_b100@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v5d@default_b100@spacetime_rule\endcsname{0.36}
\expandafter\def\csname lift@v5d@signal_0.1_b100@correlation\endcsname{1.5}
\expandafter\def\csname len@v5d@signal_0.1_b100@correlation\endcsname{11.2}
\expandafter\def\csname found@v5d@signal_0.1_b100@correlation\endcsname{2.3}
\expandafter\def\csname beyond@v5d@signal_0.1_b100@correlation\endcsname{0.28}
\expandafter\def\csname lift@v5d@signal_0.1_b100@granger\endcsname{2.5}
\expandafter\def\csname len@v5d@signal_0.1_b100@granger\endcsname{4.6}
\expandafter\def\csname found@v5d@signal_0.1_b100@granger\endcsname{1.6}
\expandafter\def\csname beyond@v5d@signal_0.1_b100@granger\endcsname{0.38}
\expandafter\def\csname lift@v5d@signal_0.1_b100@pcmciplus\endcsname{4.2}
\expandafter\def\csname len@v5d@signal_0.1_b100@pcmciplus\endcsname{1.4}
\expandafter\def\csname found@v5d@signal_0.1_b100@pcmciplus\endcsname{0.8}
\expandafter\def\csname beyond@v5d@signal_0.1_b100@pcmciplus\endcsname{0.23}
\expandafter\def\csname lift@v5d@signal_0.1_b100@pc\endcsname{2.1}
\expandafter\def\csname len@v5d@signal_0.1_b100@pc\endcsname{3.8}
\expandafter\def\csname found@v5d@signal_0.1_b100@pc\endcsname{1.1}
\expandafter\def\csname beyond@v5d@signal_0.1_b100@pc\endcsname{0.22}
\expandafter\def\csname lift@v5d@signal_0.1_b100@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@signal_0.1_b100@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@signal_0.1_b100@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@signal_0.1_b100@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@signal_0.1_b100@varlingam\endcsname{2.5}
\expandafter\def\csname len@v5d@signal_0.1_b100@varlingam\endcsname{5.0}
\expandafter\def\csname found@v5d@signal_0.1_b100@varlingam\endcsname{1.7}
\expandafter\def\csname beyond@v5d@signal_0.1_b100@varlingam\endcsname{0.38}
\expandafter\def\csname lift@v5d@signal_0.1_b100@doubleml\endcsname{4.9}
\expandafter\def\csname len@v5d@signal_0.1_b100@doubleml\endcsname{0.3}
\expandafter\def\csname found@v5d@signal_0.1_b100@doubleml\endcsname{0.2}
\expandafter\def\csname beyond@v5d@signal_0.1_b100@doubleml\endcsname{0.06}
\expandafter\def\csname lift@v5d@signal_0.1_b100@spacetime_rule\endcsname{2.4}
\expandafter\def\csname len@v5d@signal_0.1_b100@spacetime_rule\endcsname{0.6}
\expandafter\def\csname found@v5d@signal_0.1_b100@spacetime_rule\endcsname{0.2}
\expandafter\def\csname beyond@v5d@signal_0.1_b100@spacetime_rule\endcsname{0.05}
\expandafter\def\csname lift@v5d@echo_0.8_b100@correlation\endcsname{1.0}
\expandafter\def\csname len@v5d@echo_0.8_b100@correlation\endcsname{18.2}
\expandafter\def\csname found@v5d@echo_0.8_b100@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v5d@echo_0.8_b100@correlation\endcsname{0.03}
\expandafter\def\csname lift@v5d@echo_0.8_b100@granger\endcsname{1.2}
\expandafter\def\csname len@v5d@echo_0.8_b100@granger\endcsname{14.8}
\expandafter\def\csname found@v5d@echo_0.8_b100@granger\endcsname{2.5}
\expandafter\def\csname beyond@v5d@echo_0.8_b100@granger\endcsname{0.17}
\expandafter\def\csname lift@v5d@echo_0.8_b100@pcmciplus\endcsname{5.0}
\expandafter\def\csname len@v5d@echo_0.8_b100@pcmciplus\endcsname{2.2}
\expandafter\def\csname found@v5d@echo_0.8_b100@pcmciplus\endcsname{1.5}
\expandafter\def\csname beyond@v5d@echo_0.8_b100@pcmciplus\endcsname{0.46}
\expandafter\def\csname lift@v5d@echo_0.8_b100@pc\endcsname{2.3}
\expandafter\def\csname len@v5d@echo_0.8_b100@pc\endcsname{4.7}
\expandafter\def\csname found@v5d@echo_0.8_b100@pc\endcsname{1.5}
\expandafter\def\csname beyond@v5d@echo_0.8_b100@pc\endcsname{0.32}
\expandafter\def\csname lift@v5d@echo_0.8_b100@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@echo_0.8_b100@dynotears\endcsname{0.4}
\expandafter\def\csname found@v5d@echo_0.8_b100@dynotears\endcsname{0.4}
\expandafter\def\csname beyond@v5d@echo_0.8_b100@dynotears\endcsname{0.13}
\expandafter\def\csname lift@v5d@echo_0.8_b100@varlingam\endcsname{1.5}
\expandafter\def\csname len@v5d@echo_0.8_b100@varlingam\endcsname{9.6}
\expandafter\def\csname found@v5d@echo_0.8_b100@varlingam\endcsname{2.0}
\expandafter\def\csname beyond@v5d@echo_0.8_b100@varlingam\endcsname{0.23}
\expandafter\def\csname lift@v5d@echo_0.8_b100@doubleml\endcsname{4.1}
\expandafter\def\csname len@v5d@echo_0.8_b100@doubleml\endcsname{2.3}
\expandafter\def\csname found@v5d@echo_0.8_b100@doubleml\endcsname{1.3}
\expandafter\def\csname beyond@v5d@echo_0.8_b100@doubleml\endcsname{0.37}
\expandafter\def\csname lift@v5d@echo_0.8_b100@spacetime_rule\endcsname{5.3}
\expandafter\def\csname len@v5d@echo_0.8_b100@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v5d@echo_0.8_b100@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v5d@echo_0.8_b100@spacetime_rule\endcsname{0.25}
\expandafter\def\csname lift@v5d@confound_0.8_b100@correlation\endcsname{1.0}
\expandafter\def\csname len@v5d@confound_0.8_b100@correlation\endcsname{17.5}
\expandafter\def\csname found@v5d@confound_0.8_b100@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v5d@confound_0.8_b100@correlation\endcsname{0.00}
\expandafter\def\csname lift@v5d@confound_0.8_b100@granger\endcsname{1.1}
\expandafter\def\csname len@v5d@confound_0.8_b100@granger\endcsname{14.9}
\expandafter\def\csname found@v5d@confound_0.8_b100@granger\endcsname{2.3}
\expandafter\def\csname beyond@v5d@confound_0.8_b100@granger\endcsname{0.12}
\expandafter\def\csname lift@v5d@confound_0.8_b100@pcmciplus\endcsname{4.7}
\expandafter\def\csname len@v5d@confound_0.8_b100@pcmciplus\endcsname{2.5}
\expandafter\def\csname found@v5d@confound_0.8_b100@pcmciplus\endcsname{1.6}
\expandafter\def\csname beyond@v5d@confound_0.8_b100@pcmciplus\endcsname{0.47}
\expandafter\def\csname lift@v5d@confound_0.8_b100@pc\endcsname{2.9}
\expandafter\def\csname len@v5d@confound_0.8_b100@pc\endcsname{4.0}
\expandafter\def\csname found@v5d@confound_0.8_b100@pc\endcsname{1.6}
\expandafter\def\csname beyond@v5d@confound_0.8_b100@pc\endcsname{0.40}
\expandafter\def\csname lift@v5d@confound_0.8_b100@dynotears\endcsname{7.3}
\expandafter\def\csname len@v5d@confound_0.8_b100@dynotears\endcsname{0.3}
\expandafter\def\csname found@v5d@confound_0.8_b100@dynotears\endcsname{0.3}
\expandafter\def\csname beyond@v5d@confound_0.8_b100@dynotears\endcsname{0.10}
\expandafter\def\csname lift@v5d@confound_0.8_b100@varlingam\endcsname{2.0}
\expandafter\def\csname len@v5d@confound_0.8_b100@varlingam\endcsname{7.3}
\expandafter\def\csname found@v5d@confound_0.8_b100@varlingam\endcsname{2.0}
\expandafter\def\csname beyond@v5d@confound_0.8_b100@varlingam\endcsname{0.37}
\expandafter\def\csname lift@v5d@confound_0.8_b100@doubleml\endcsname{5.3}
\expandafter\def\csname len@v5d@confound_0.8_b100@doubleml\endcsname{2.6}
\expandafter\def\csname found@v5d@confound_0.8_b100@doubleml\endcsname{1.9}
\expandafter\def\csname beyond@v5d@confound_0.8_b100@doubleml\endcsname{0.57}
\expandafter\def\csname lift@v5d@confound_0.8_b100@spacetime_rule\endcsname{4.6}
\expandafter\def\csname len@v5d@confound_0.8_b100@spacetime_rule\endcsname{1.6}
\expandafter\def\csname found@v5d@confound_0.8_b100@spacetime_rule\endcsname{1.0}
\expandafter\def\csname beyond@v5d@confound_0.8_b100@spacetime_rule\endcsname{0.30}
\expandafter\def\csname lift@v5d@combo_hard_b100@correlation\endcsname{1.1}
\expandafter\def\csname len@v5d@combo_hard_b100@correlation\endcsname{16.0}
\expandafter\def\csname found@v5d@combo_hard_b100@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v5d@combo_hard_b100@correlation\endcsname{0.07}
\expandafter\def\csname lift@v5d@combo_hard_b100@granger\endcsname{1.4}
\expandafter\def\csname len@v5d@combo_hard_b100@granger\endcsname{11.8}
\expandafter\def\csname found@v5d@combo_hard_b100@granger\endcsname{2.3}
\expandafter\def\csname beyond@v5d@combo_hard_b100@granger\endcsname{0.28}
\expandafter\def\csname lift@v5d@combo_hard_b100@pcmciplus\endcsname{4.4}
\expandafter\def\csname len@v5d@combo_hard_b100@pcmciplus\endcsname{2.3}
\expandafter\def\csname found@v5d@combo_hard_b100@pcmciplus\endcsname{1.4}
\expandafter\def\csname beyond@v5d@combo_hard_b100@pcmciplus\endcsname{0.41}
\expandafter\def\csname lift@v5d@combo_hard_b100@pc\endcsname{2.5}
\expandafter\def\csname len@v5d@combo_hard_b100@pc\endcsname{3.2}
\expandafter\def\csname found@v5d@combo_hard_b100@pc\endcsname{1.1}
\expandafter\def\csname beyond@v5d@combo_hard_b100@pc\endcsname{0.25}
\expandafter\def\csname lift@v5d@combo_hard_b100@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@combo_hard_b100@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@combo_hard_b100@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_hard_b100@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@combo_hard_b100@varlingam\endcsname{1.7}
\expandafter\def\csname len@v5d@combo_hard_b100@varlingam\endcsname{7.6}
\expandafter\def\csname found@v5d@combo_hard_b100@varlingam\endcsname{1.8}
\expandafter\def\csname beyond@v5d@combo_hard_b100@varlingam\endcsname{0.27}
\expandafter\def\csname lift@v5d@combo_hard_b100@doubleml\endcsname{4.9}
\expandafter\def\csname len@v5d@combo_hard_b100@doubleml\endcsname{1.2}
\expandafter\def\csname found@v5d@combo_hard_b100@doubleml\endcsname{0.8}
\expandafter\def\csname beyond@v5d@combo_hard_b100@doubleml\endcsname{0.24}
\expandafter\def\csname lift@v5d@combo_hard_b100@spacetime_rule\endcsname{3.7}
\expandafter\def\csname len@v5d@combo_hard_b100@spacetime_rule\endcsname{1.0}
\expandafter\def\csname found@v5d@combo_hard_b100@spacetime_rule\endcsname{0.5}
\expandafter\def\csname beyond@v5d@combo_hard_b100@spacetime_rule\endcsname{0.14}
\expandafter\def\csname lift@v5d@combo_extreme_b100@correlation\endcsname{1.1}
\expandafter\def\csname len@v5d@combo_extreme_b100@correlation\endcsname{15.5}
\expandafter\def\csname found@v5d@combo_extreme_b100@correlation\endcsname{2.3}
\expandafter\def\csname beyond@v5d@combo_extreme_b100@correlation\endcsname{0.08}
\expandafter\def\csname lift@v5d@combo_extreme_b100@granger\endcsname{1.5}
\expandafter\def\csname len@v5d@combo_extreme_b100@granger\endcsname{10.4}
\expandafter\def\csname found@v5d@combo_extreme_b100@granger\endcsname{2.2}
\expandafter\def\csname beyond@v5d@combo_extreme_b100@granger\endcsname{0.35}
\expandafter\def\csname lift@v5d@combo_extreme_b100@pcmciplus\endcsname{4.6}
\expandafter\def\csname len@v5d@combo_extreme_b100@pcmciplus\endcsname{0.8}
\expandafter\def\csname found@v5d@combo_extreme_b100@pcmciplus\endcsname{0.5}
\expandafter\def\csname beyond@v5d@combo_extreme_b100@pcmciplus\endcsname{0.15}
\expandafter\def\csname lift@v5d@combo_extreme_b100@pc\endcsname{1.8}
\expandafter\def\csname len@v5d@combo_extreme_b100@pc\endcsname{2.4}
\expandafter\def\csname found@v5d@combo_extreme_b100@pc\endcsname{0.6}
\expandafter\def\csname beyond@v5d@combo_extreme_b100@pc\endcsname{0.09}
\expandafter\def\csname lift@v5d@combo_extreme_b100@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@combo_extreme_b100@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@combo_extreme_b100@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_extreme_b100@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@combo_extreme_b100@varlingam\endcsname{1.2}
\expandafter\def\csname len@v5d@combo_extreme_b100@varlingam\endcsname{7.2}
\expandafter\def\csname found@v5d@combo_extreme_b100@varlingam\endcsname{1.2}
\expandafter\def\csname beyond@v5d@combo_extreme_b100@varlingam\endcsname{0.08}
\expandafter\def\csname lift@v5d@combo_extreme_b100@doubleml\endcsname{4.2}
\expandafter\def\csname len@v5d@combo_extreme_b100@doubleml\endcsname{0.7}
\expandafter\def\csname found@v5d@combo_extreme_b100@doubleml\endcsname{0.4}
\expandafter\def\csname beyond@v5d@combo_extreme_b100@doubleml\endcsname{0.11}
\expandafter\def\csname lift@v5d@combo_extreme_b100@spacetime_rule\endcsname{1.8}
\expandafter\def\csname len@v5d@combo_extreme_b100@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v5d@combo_extreme_b100@spacetime_rule\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_extreme_b100@spacetime_rule\endcsname{0.05}
\expandafter\def\csname lift@v5d@interaction_1.0_b100@correlation\endcsname{1.3}
\expandafter\def\csname len@v5d@interaction_1.0_b100@correlation\endcsname{7.5}
\expandafter\def\csname found@v5d@interaction_1.0_b100@correlation\endcsname{1.3}
\expandafter\def\csname beyond@v5d@interaction_1.0_b100@correlation\endcsname{0.13}
\expandafter\def\csname lift@v5d@interaction_1.0_b100@granger\endcsname{1.6}
\expandafter\def\csname len@v5d@interaction_1.0_b100@granger\endcsname{5.1}
\expandafter\def\csname found@v5d@interaction_1.0_b100@granger\endcsname{1.1}
\expandafter\def\csname beyond@v5d@interaction_1.0_b100@granger\endcsname{0.18}
\expandafter\def\csname lift@v5d@interaction_1.0_b100@pcmciplus\endcsname{4.6}
\expandafter\def\csname len@v5d@interaction_1.0_b100@pcmciplus\endcsname{1.6}
\expandafter\def\csname found@v5d@interaction_1.0_b100@pcmciplus\endcsname{1.0}
\expandafter\def\csname beyond@v5d@interaction_1.0_b100@pcmciplus\endcsname{0.30}
\expandafter\def\csname lift@v5d@interaction_1.0_b100@pc\endcsname{1.0}
\expandafter\def\csname len@v5d@interaction_1.0_b100@pc\endcsname{2.8}
\expandafter\def\csname found@v5d@interaction_1.0_b100@pc\endcsname{0.4}
\expandafter\def\csname beyond@v5d@interaction_1.0_b100@pc\endcsname{-0.00}
\expandafter\def\csname lift@v5d@interaction_1.0_b100@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@interaction_1.0_b100@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@interaction_1.0_b100@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@interaction_1.0_b100@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@interaction_1.0_b100@varlingam\endcsname{0.9}
\expandafter\def\csname len@v5d@interaction_1.0_b100@varlingam\endcsname{1.7}
\expandafter\def\csname found@v5d@interaction_1.0_b100@varlingam\endcsname{0.2}
\expandafter\def\csname beyond@v5d@interaction_1.0_b100@varlingam\endcsname{0.01}
\expandafter\def\csname lift@v5d@interaction_1.0_b100@doubleml\endcsname{4.4}
\expandafter\def\csname len@v5d@interaction_1.0_b100@doubleml\endcsname{0.5}
\expandafter\def\csname found@v5d@interaction_1.0_b100@doubleml\endcsname{0.3}
\expandafter\def\csname beyond@v5d@interaction_1.0_b100@doubleml\endcsname{0.09}
\expandafter\def\csname lift@v5d@interaction_1.0_b100@spacetime_rule\endcsname{6.2}
\expandafter\def\csname len@v5d@interaction_1.0_b100@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v5d@interaction_1.0_b100@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v5d@interaction_1.0_b100@spacetime_rule\endcsname{0.36}
\expandafter\def\csname lift@v5d@combo_interaction_b100@correlation\endcsname{1.0}
\expandafter\def\csname len@v5d@combo_interaction_b100@correlation\endcsname{5.2}
\expandafter\def\csname found@v5d@combo_interaction_b100@correlation\endcsname{0.7}
\expandafter\def\csname beyond@v5d@combo_interaction_b100@correlation\endcsname{0.04}
\expandafter\def\csname lift@v5d@combo_interaction_b100@granger\endcsname{1.0}
\expandafter\def\csname len@v5d@combo_interaction_b100@granger\endcsname{2.8}
\expandafter\def\csname found@v5d@combo_interaction_b100@granger\endcsname{0.4}
\expandafter\def\csname beyond@v5d@combo_interaction_b100@granger\endcsname{0.06}
\expandafter\def\csname lift@v5d@combo_interaction_b100@pcmciplus\endcsname{2.4}
\expandafter\def\csname len@v5d@combo_interaction_b100@pcmciplus\endcsname{0.9}
\expandafter\def\csname found@v5d@combo_interaction_b100@pcmciplus\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_interaction_b100@pcmciplus\endcsname{0.07}
\expandafter\def\csname lift@v5d@combo_interaction_b100@pc\endcsname{0.3}
\expandafter\def\csname len@v5d@combo_interaction_b100@pc\endcsname{2.1}
\expandafter\def\csname found@v5d@combo_interaction_b100@pc\endcsname{0.1}
\expandafter\def\csname beyond@v5d@combo_interaction_b100@pc\endcsname{-0.07}
\expandafter\def\csname lift@v5d@combo_interaction_b100@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@combo_interaction_b100@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@combo_interaction_b100@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@combo_interaction_b100@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@combo_interaction_b100@varlingam\endcsname{0.8}
\expandafter\def\csname len@v5d@combo_interaction_b100@varlingam\endcsname{2.8}
\expandafter\def\csname found@v5d@combo_interaction_b100@varlingam\endcsname{0.3}
\expandafter\def\csname beyond@v5d@combo_interaction_b100@varlingam\endcsname{-0.03}
\expandafter\def\csname lift@v5d@combo_interaction_b100@doubleml\endcsname{7.3}
\expandafter\def\csname len@v5d@combo_interaction_b100@doubleml\endcsname{0.1}
\expandafter\def\csname found@v5d@combo_interaction_b100@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v5d@combo_interaction_b100@doubleml\endcsname{0.03}
\expandafter\def\csname lift@v5d@combo_interaction_b100@spacetime_rule\endcsname{3.3}
\expandafter\def\csname len@v5d@combo_interaction_b100@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v5d@combo_interaction_b100@spacetime_rule\endcsname{0.5}
\expandafter\def\csname beyond@v5d@combo_interaction_b100@spacetime_rule\endcsname{0.14}
\expandafter\def\csname lift@v5d@control_weak_b100@correlation\endcsname{1.5}
\expandafter\def\csname len@v5d@control_weak_b100@correlation\endcsname{10.2}
\expandafter\def\csname found@v5d@control_weak_b100@correlation\endcsname{2.2}
\expandafter\def\csname beyond@v5d@control_weak_b100@correlation\endcsname{0.22}
\expandafter\def\csname lift@v5d@control_weak_b100@granger\endcsname{2.8}
\expandafter\def\csname len@v5d@control_weak_b100@granger\endcsname{5.4}
\expandafter\def\csname found@v5d@control_weak_b100@granger\endcsname{2.2}
\expandafter\def\csname beyond@v5d@control_weak_b100@granger\endcsname{0.50}
\expandafter\def\csname lift@v5d@control_weak_b100@pcmciplus\endcsname{4.3}
\expandafter\def\csname len@v5d@control_weak_b100@pcmciplus\endcsname{1.6}
\expandafter\def\csname found@v5d@control_weak_b100@pcmciplus\endcsname{1.0}
\expandafter\def\csname beyond@v5d@control_weak_b100@pcmciplus\endcsname{0.29}
\expandafter\def\csname lift@v5d@control_weak_b100@pc\endcsname{2.1}
\expandafter\def\csname len@v5d@control_weak_b100@pc\endcsname{3.6}
\expandafter\def\csname found@v5d@control_weak_b100@pc\endcsname{1.1}
\expandafter\def\csname beyond@v5d@control_weak_b100@pc\endcsname{0.22}
\expandafter\def\csname lift@v5d@control_weak_b100@dynotears\endcsname{--}
\expandafter\def\csname len@v5d@control_weak_b100@dynotears\endcsname{0.0}
\expandafter\def\csname found@v5d@control_weak_b100@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v5d@control_weak_b100@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v5d@control_weak_b100@varlingam\endcsname{3.1}
\expandafter\def\csname len@v5d@control_weak_b100@varlingam\endcsname{4.3}
\expandafter\def\csname found@v5d@control_weak_b100@varlingam\endcsname{1.9}
\expandafter\def\csname beyond@v5d@control_weak_b100@varlingam\endcsname{0.48}
\expandafter\def\csname lift@v5d@control_weak_b100@doubleml\endcsname{6.1}
\expandafter\def\csname len@v5d@control_weak_b100@doubleml\endcsname{0.8}
\expandafter\def\csname found@v5d@control_weak_b100@doubleml\endcsname{0.7}
\expandafter\def\csname beyond@v5d@control_weak_b100@doubleml\endcsname{0.22}
\expandafter\def\csname lift@v5d@control_weak_b100@spacetime_rule\endcsname{1.4}
\expandafter\def\csname len@v5d@control_weak_b100@spacetime_rule\endcsname{0.5}
\expandafter\def\csname found@v5d@control_weak_b100@spacetime_rule\endcsname{0.1}
\expandafter\def\csname beyond@v5d@control_weak_b100@spacetime_rule\endcsname{0.01}
\expandafter\def\csname lift@v6@meas_0.1@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@meas_0.1@correlation\endcsname{18.3}
\expandafter\def\csname found@v6@meas_0.1@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@meas_0.1@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@meas_0.1@granger\endcsname{1.1}
\expandafter\def\csname len@v6@meas_0.1@granger\endcsname{16.9}
\expandafter\def\csname found@v6@meas_0.1@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@meas_0.1@granger\endcsname{0.07}
\expandafter\def\csname lift@v6@meas_0.1@pcmciplus\endcsname{4.6}
\expandafter\def\csname len@v6@meas_0.1@pcmciplus\endcsname{3.2}
\expandafter\def\csname found@v6@meas_0.1@pcmciplus\endcsname{2.0}
\expandafter\def\csname beyond@v6@meas_0.1@pcmciplus\endcsname{0.59}
\expandafter\def\csname lift@v6@meas_0.1@pc\endcsname{2.3}
\expandafter\def\csname len@v6@meas_0.1@pc\endcsname{5.6}
\expandafter\def\csname found@v6@meas_0.1@pc\endcsname{1.8}
\expandafter\def\csname beyond@v6@meas_0.1@pc\endcsname{0.38}
\expandafter\def\csname lift@v6@meas_0.1@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@meas_0.1@dynotears\endcsname{0.4}
\expandafter\def\csname found@v6@meas_0.1@dynotears\endcsname{0.4}
\expandafter\def\csname beyond@v6@meas_0.1@dynotears\endcsname{0.13}
\expandafter\def\csname lift@v6@meas_0.1@varlingam\endcsname{1.8}
\expandafter\def\csname len@v6@meas_0.1@varlingam\endcsname{9.9}
\expandafter\def\csname found@v6@meas_0.1@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v6@meas_0.1@varlingam\endcsname{0.42}
\expandafter\def\csname lift@v6@meas_0.1@doubleml\endcsname{4.1}
\expandafter\def\csname len@v6@meas_0.1@doubleml\endcsname{3.9}
\expandafter\def\csname found@v6@meas_0.1@doubleml\endcsname{2.2}
\expandafter\def\csname beyond@v6@meas_0.1@doubleml\endcsname{0.61}
\expandafter\def\csname lift@v6@meas_0.1@spacetime_rule\endcsname{6.7}
\expandafter\def\csname len@v6@meas_0.1@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v6@meas_0.1@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v6@meas_0.1@spacetime_rule\endcsname{0.36}
\expandafter\def\csname lift@v6@meas_0.2@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@meas_0.2@correlation\endcsname{18.3}
\expandafter\def\csname found@v6@meas_0.2@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@meas_0.2@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@meas_0.2@granger\endcsname{1.1}
\expandafter\def\csname len@v6@meas_0.2@granger\endcsname{16.6}
\expandafter\def\csname found@v6@meas_0.2@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@meas_0.2@granger\endcsname{0.08}
\expandafter\def\csname lift@v6@meas_0.2@pcmciplus\endcsname{4.4}
\expandafter\def\csname len@v6@meas_0.2@pcmciplus\endcsname{3.8}
\expandafter\def\csname found@v6@meas_0.2@pcmciplus\endcsname{2.3}
\expandafter\def\csname beyond@v6@meas_0.2@pcmciplus\endcsname{0.68}
\expandafter\def\csname lift@v6@meas_0.2@pc\endcsname{2.2}
\expandafter\def\csname len@v6@meas_0.2@pc\endcsname{6.1}
\expandafter\def\csname found@v6@meas_0.2@pc\endcsname{1.8}
\expandafter\def\csname beyond@v6@meas_0.2@pc\endcsname{0.35}
\expandafter\def\csname lift@v6@meas_0.2@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@meas_0.2@dynotears\endcsname{0.1}
\expandafter\def\csname found@v6@meas_0.2@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v6@meas_0.2@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v6@meas_0.2@varlingam\endcsname{1.6}
\expandafter\def\csname len@v6@meas_0.2@varlingam\endcsname{11.1}
\expandafter\def\csname found@v6@meas_0.2@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v6@meas_0.2@varlingam\endcsname{0.34}
\expandafter\def\csname lift@v6@meas_0.2@doubleml\endcsname{4.0}
\expandafter\def\csname len@v6@meas_0.2@doubleml\endcsname{3.8}
\expandafter\def\csname found@v6@meas_0.2@doubleml\endcsname{2.1}
\expandafter\def\csname beyond@v6@meas_0.2@doubleml\endcsname{0.58}
\expandafter\def\csname lift@v6@meas_0.2@spacetime_rule\endcsname{6.6}
\expandafter\def\csname len@v6@meas_0.2@spacetime_rule\endcsname{1.0}
\expandafter\def\csname found@v6@meas_0.2@spacetime_rule\endcsname{0.9}
\expandafter\def\csname beyond@v6@meas_0.2@spacetime_rule\endcsname{0.30}
\expandafter\def\csname lift@v6@meas_0.3@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@meas_0.3@correlation\endcsname{18.1}
\expandafter\def\csname found@v6@meas_0.3@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@meas_0.3@correlation\endcsname{0.05}
\expandafter\def\csname lift@v6@meas_0.3@granger\endcsname{1.1}
\expandafter\def\csname len@v6@meas_0.3@granger\endcsname{16.1}
\expandafter\def\csname found@v6@meas_0.3@granger\endcsname{2.4}
\expandafter\def\csname beyond@v6@meas_0.3@granger\endcsname{0.08}
\expandafter\def\csname lift@v6@meas_0.3@pcmciplus\endcsname{3.9}
\expandafter\def\csname len@v6@meas_0.3@pcmciplus\endcsname{3.9}
\expandafter\def\csname found@v6@meas_0.3@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v6@meas_0.3@pcmciplus\endcsname{0.59}
\expandafter\def\csname lift@v6@meas_0.3@pc\endcsname{1.9}
\expandafter\def\csname len@v6@meas_0.3@pc\endcsname{7.1}
\expandafter\def\csname found@v6@meas_0.3@pc\endcsname{1.8}
\expandafter\def\csname beyond@v6@meas_0.3@pc\endcsname{0.30}
\expandafter\def\csname lift@v6@meas_0.3@dynotears\endcsname{--}
\expandafter\def\csname len@v6@meas_0.3@dynotears\endcsname{0.0}
\expandafter\def\csname found@v6@meas_0.3@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v6@meas_0.3@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v6@meas_0.3@varlingam\endcsname{1.9}
\expandafter\def\csname len@v6@meas_0.3@varlingam\endcsname{9.4}
\expandafter\def\csname found@v6@meas_0.3@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v6@meas_0.3@varlingam\endcsname{0.41}
\expandafter\def\csname lift@v6@meas_0.3@doubleml\endcsname{3.7}
\expandafter\def\csname len@v6@meas_0.3@doubleml\endcsname{4.4}
\expandafter\def\csname found@v6@meas_0.3@doubleml\endcsname{2.2}
\expandafter\def\csname beyond@v6@meas_0.3@doubleml\endcsname{0.59}
\expandafter\def\csname lift@v6@meas_0.3@spacetime_rule\endcsname{5.7}
\expandafter\def\csname len@v6@meas_0.3@spacetime_rule\endcsname{0.9}
\expandafter\def\csname found@v6@meas_0.3@spacetime_rule\endcsname{0.7}
\expandafter\def\csname beyond@v6@meas_0.3@spacetime_rule\endcsname{0.22}
\expandafter\def\csname lift@v6@meas_0.5@correlation\endcsname{1.1}
\expandafter\def\csname len@v6@meas_0.5@correlation\endcsname{17.8}
\expandafter\def\csname found@v6@meas_0.5@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@meas_0.5@correlation\endcsname{0.06}
\expandafter\def\csname lift@v6@meas_0.5@granger\endcsname{1.2}
\expandafter\def\csname len@v6@meas_0.5@granger\endcsname{14.1}
\expandafter\def\csname found@v6@meas_0.5@granger\endcsname{2.4}
\expandafter\def\csname beyond@v6@meas_0.5@granger\endcsname{0.18}
\expandafter\def\csname lift@v6@meas_0.5@pcmciplus\endcsname{3.4}
\expandafter\def\csname len@v6@meas_0.5@pcmciplus\endcsname{5.0}
\expandafter\def\csname found@v6@meas_0.5@pcmciplus\endcsname{2.3}
\expandafter\def\csname beyond@v6@meas_0.5@pcmciplus\endcsname{0.60}
\expandafter\def\csname lift@v6@meas_0.5@pc\endcsname{1.6}
\expandafter\def\csname len@v6@meas_0.5@pc\endcsname{8.9}
\expandafter\def\csname found@v6@meas_0.5@pc\endcsname{1.9}
\expandafter\def\csname beyond@v6@meas_0.5@pc\endcsname{0.25}
\expandafter\def\csname lift@v6@meas_0.5@dynotears\endcsname{--}
\expandafter\def\csname len@v6@meas_0.5@dynotears\endcsname{0.0}
\expandafter\def\csname found@v6@meas_0.5@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v6@meas_0.5@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v6@meas_0.5@varlingam\endcsname{1.9}
\expandafter\def\csname len@v6@meas_0.5@varlingam\endcsname{9.2}
\expandafter\def\csname found@v6@meas_0.5@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v6@meas_0.5@varlingam\endcsname{0.40}
\expandafter\def\csname lift@v6@meas_0.5@doubleml\endcsname{3.6}
\expandafter\def\csname len@v6@meas_0.5@doubleml\endcsname{4.7}
\expandafter\def\csname found@v6@meas_0.5@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v6@meas_0.5@doubleml\endcsname{0.62}
\expandafter\def\csname lift@v6@meas_0.5@spacetime_rule\endcsname{5.5}
\expandafter\def\csname len@v6@meas_0.5@spacetime_rule\endcsname{0.4}
\expandafter\def\csname found@v6@meas_0.5@spacetime_rule\endcsname{0.3}
\expandafter\def\csname beyond@v6@meas_0.5@spacetime_rule\endcsname{0.10}
\expandafter\def\csname lift@v6@meas_0.3_combo_interaction@correlation\endcsname{1.1}
\expandafter\def\csname len@v6@meas_0.3_combo_interaction@correlation\endcsname{5.2}
\expandafter\def\csname found@v6@meas_0.3_combo_interaction@correlation\endcsname{0.8}
\expandafter\def\csname beyond@v6@meas_0.3_combo_interaction@correlation\endcsname{0.07}
\expandafter\def\csname lift@v6@meas_0.3_combo_interaction@granger\endcsname{1.1}
\expandafter\def\csname len@v6@meas_0.3_combo_interaction@granger\endcsname{3.3}
\expandafter\def\csname found@v6@meas_0.3_combo_interaction@granger\endcsname{0.5}
\expandafter\def\csname beyond@v6@meas_0.3_combo_interaction@granger\endcsname{0.09}
\expandafter\def\csname lift@v6@meas_0.3_combo_interaction@pcmciplus\endcsname{2.1}
\expandafter\def\csname len@v6@meas_0.3_combo_interaction@pcmciplus\endcsname{1.4}
\expandafter\def\csname found@v6@meas_0.3_combo_interaction@pcmciplus\endcsname{0.4}
\expandafter\def\csname beyond@v6@meas_0.3_combo_interaction@pcmciplus\endcsname{0.08}
\expandafter\def\csname lift@v6@meas_0.3_combo_interaction@pc\endcsname{0.5}
\expandafter\def\csname len@v6@meas_0.3_combo_interaction@pc\endcsname{2.8}
\expandafter\def\csname found@v6@meas_0.3_combo_interaction@pc\endcsname{0.2}
\expandafter\def\csname beyond@v6@meas_0.3_combo_interaction@pc\endcsname{-0.07}
\expandafter\def\csname lift@v6@meas_0.3_combo_interaction@dynotears\endcsname{--}
\expandafter\def\csname len@v6@meas_0.3_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname found@v6@meas_0.3_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v6@meas_0.3_combo_interaction@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v6@meas_0.3_combo_interaction@varlingam\endcsname{0.9}
\expandafter\def\csname len@v6@meas_0.3_combo_interaction@varlingam\endcsname{3.1}
\expandafter\def\csname found@v6@meas_0.3_combo_interaction@varlingam\endcsname{0.4}
\expandafter\def\csname beyond@v6@meas_0.3_combo_interaction@varlingam\endcsname{0.01}
\expandafter\def\csname lift@v6@meas_0.3_combo_interaction@doubleml\endcsname{2.4}
\expandafter\def\csname len@v6@meas_0.3_combo_interaction@doubleml\endcsname{0.3}
\expandafter\def\csname found@v6@meas_0.3_combo_interaction@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v6@meas_0.3_combo_interaction@doubleml\endcsname{0.03}
\expandafter\def\csname lift@v6@meas_0.3_combo_interaction@spacetime_rule\endcsname{5.2}
\expandafter\def\csname len@v6@meas_0.3_combo_interaction@spacetime_rule\endcsname{0.7}
\expandafter\def\csname found@v6@meas_0.3_combo_interaction@spacetime_rule\endcsname{0.5}
\expandafter\def\csname beyond@v6@meas_0.3_combo_interaction@spacetime_rule\endcsname{0.16}
\expandafter\def\csname lift@v6@meas_0.3_s40@correlation\endcsname{1.1}
\expandafter\def\csname len@v6@meas_0.3_s40@correlation\endcsname{35.0}
\expandafter\def\csname found@v6@meas_0.3_s40@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@meas_0.3_s40@correlation\endcsname{0.10}
\expandafter\def\csname lift@v6@meas_0.3_s40@granger\endcsname{1.1}
\expandafter\def\csname len@v6@meas_0.3_s40@granger\endcsname{30.0}
\expandafter\def\csname found@v6@meas_0.3_s40@granger\endcsname{2.3}
\expandafter\def\csname beyond@v6@meas_0.3_s40@granger\endcsname{0.12}
\expandafter\def\csname lift@v6@meas_0.3_s40@pcmciplus\endcsname{5.6}
\expandafter\def\csname len@v6@meas_0.3_s40@pcmciplus\endcsname{4.8}
\expandafter\def\csname found@v6@meas_0.3_s40@pcmciplus\endcsname{1.8}
\expandafter\def\csname beyond@v6@meas_0.3_s40@pcmciplus\endcsname{0.57}
\expandafter\def\csname lift@v6@meas_0.3_s40@pc\endcsname{3.0}
\expandafter\def\csname len@v6@meas_0.3_s40@pc\endcsname{9.5}
\expandafter\def\csname found@v6@meas_0.3_s40@pc\endcsname{1.9}
\expandafter\def\csname beyond@v6@meas_0.3_s40@pc\endcsname{0.48}
\expandafter\def\csname lift@v6@meas_0.3_s40@dynotears\endcsname{15.0}
\expandafter\def\csname len@v6@meas_0.3_s40@dynotears\endcsname{0.1}
\expandafter\def\csname found@v6@meas_0.3_s40@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v6@meas_0.3_s40@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v6@meas_0.3_s40@varlingam\endcsname{2.4}
\expandafter\def\csname len@v6@meas_0.3_s40@varlingam\endcsname{13.3}
\expandafter\def\csname found@v6@meas_0.3_s40@varlingam\endcsname{2.1}
\expandafter\def\csname beyond@v6@meas_0.3_s40@varlingam\endcsname{0.43}
\expandafter\def\csname lift@v6@meas_0.3_s40@doubleml\endcsname{9.1}
\expandafter\def\csname len@v6@meas_0.3_s40@doubleml\endcsname{2.8}
\expandafter\def\csname found@v6@meas_0.3_s40@doubleml\endcsname{1.7}
\expandafter\def\csname beyond@v6@meas_0.3_s40@doubleml\endcsname{0.57}
\expandafter\def\csname lift@v6@meas_0.3_s40@spacetime_rule\endcsname{13.3}
\expandafter\def\csname len@v6@meas_0.3_s40@spacetime_rule\endcsname{0.9}
\expandafter\def\csname found@v6@meas_0.3_s40@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v6@meas_0.3_s40@spacetime_rule\endcsname{0.28}
\expandafter\def\csname lift@v6@meas_0.3_b50@correlation\endcsname{1.2}
\expandafter\def\csname len@v6@meas_0.3_b50@correlation\endcsname{14.6}
\expandafter\def\csname found@v6@meas_0.3_b50@correlation\endcsname{2.4}
\expandafter\def\csname beyond@v6@meas_0.3_b50@correlation\endcsname{0.16}
\expandafter\def\csname lift@v6@meas_0.3_b50@granger\endcsname{2.0}
\expandafter\def\csname len@v6@meas_0.3_b50@granger\endcsname{7.3}
\expandafter\def\csname found@v6@meas_0.3_b50@granger\endcsname{2.0}
\expandafter\def\csname beyond@v6@meas_0.3_b50@granger\endcsname{0.42}
\expandafter\def\csname lift@v6@meas_0.3_b50@pcmciplus\endcsname{5.1}
\expandafter\def\csname len@v6@meas_0.3_b50@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v6@meas_0.3_b50@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v6@meas_0.3_b50@pcmciplus\endcsname{0.58}
\expandafter\def\csname lift@v6@meas_0.3_b50@pc\endcsname{2.3}
\expandafter\def\csname len@v6@meas_0.3_b50@pc\endcsname{5.6}
\expandafter\def\csname found@v6@meas_0.3_b50@pc\endcsname{1.8}
\expandafter\def\csname beyond@v6@meas_0.3_b50@pc\endcsname{0.39}
\expandafter\def\csname lift@v6@meas_0.3_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@meas_0.3_b50@dynotears\endcsname{0.1}
\expandafter\def\csname found@v6@meas_0.3_b50@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v6@meas_0.3_b50@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v6@meas_0.3_b50@varlingam\endcsname{2.5}
\expandafter\def\csname len@v6@meas_0.3_b50@varlingam\endcsname{6.5}
\expandafter\def\csname found@v6@meas_0.3_b50@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v6@meas_0.3_b50@varlingam\endcsname{0.47}
\expandafter\def\csname lift@v6@meas_0.3_b50@doubleml\endcsname{4.4}
\expandafter\def\csname len@v6@meas_0.3_b50@doubleml\endcsname{2.8}
\expandafter\def\csname found@v6@meas_0.3_b50@doubleml\endcsname{1.7}
\expandafter\def\csname beyond@v6@meas_0.3_b50@doubleml\endcsname{0.49}
\expandafter\def\csname lift@v6@meas_0.3_b50@spacetime_rule\endcsname{7.3}
\expandafter\def\csname len@v6@meas_0.3_b50@spacetime_rule\endcsname{0.8}
\expandafter\def\csname found@v6@meas_0.3_b50@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v6@meas_0.3_b50@spacetime_rule\endcsname{0.27}
\expandafter\def\csname lift@v6@context_0.25@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@context_0.25@correlation\endcsname{18.3}
\expandafter\def\csname found@v6@context_0.25@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@context_0.25@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@context_0.25@granger\endcsname{1.1}
\expandafter\def\csname len@v6@context_0.25@granger\endcsname{16.8}
\expandafter\def\csname found@v6@context_0.25@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@context_0.25@granger\endcsname{0.07}
\expandafter\def\csname lift@v6@context_0.25@pcmciplus\endcsname{5.0}
\expandafter\def\csname len@v6@context_0.25@pcmciplus\endcsname{2.9}
\expandafter\def\csname found@v6@context_0.25@pcmciplus\endcsname{2.0}
\expandafter\def\csname beyond@v6@context_0.25@pcmciplus\endcsname{0.60}
\expandafter\def\csname lift@v6@context_0.25@pc\endcsname{2.4}
\expandafter\def\csname len@v6@context_0.25@pc\endcsname{5.7}
\expandafter\def\csname found@v6@context_0.25@pc\endcsname{1.9}
\expandafter\def\csname beyond@v6@context_0.25@pc\endcsname{0.42}
\expandafter\def\csname lift@v6@context_0.25@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@context_0.25@dynotears\endcsname{0.5}
\expandafter\def\csname found@v6@context_0.25@dynotears\endcsname{0.5}
\expandafter\def\csname beyond@v6@context_0.25@dynotears\endcsname{0.17}
\expandafter\def\csname lift@v6@context_0.25@varlingam\endcsname{1.9}
\expandafter\def\csname len@v6@context_0.25@varlingam\endcsname{10.2}
\expandafter\def\csname found@v6@context_0.25@varlingam\endcsname{2.6}
\expandafter\def\csname beyond@v6@context_0.25@varlingam\endcsname{0.45}
\expandafter\def\csname lift@v6@context_0.25@doubleml\endcsname{4.9}
\expandafter\def\csname len@v6@context_0.25@doubleml\endcsname{3.0}
\expandafter\def\csname found@v6@context_0.25@doubleml\endcsname{2.0}
\expandafter\def\csname beyond@v6@context_0.25@doubleml\endcsname{0.59}
\expandafter\def\csname lift@v6@context_0.25@spacetime_rule\endcsname{6.2}
\expandafter\def\csname len@v6@context_0.25@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v6@context_0.25@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v6@context_0.25@spacetime_rule\endcsname{0.36}
\expandafter\def\csname lift@v6@context_0.5@correlation\endcsname{1.1}
\expandafter\def\csname len@v6@context_0.5@correlation\endcsname{17.4}
\expandafter\def\csname found@v6@context_0.5@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@context_0.5@correlation\endcsname{0.08}
\expandafter\def\csname lift@v6@context_0.5@granger\endcsname{1.1}
\expandafter\def\csname len@v6@context_0.5@granger\endcsname{16.0}
\expandafter\def\csname found@v6@context_0.5@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@context_0.5@granger\endcsname{0.12}
\expandafter\def\csname lift@v6@context_0.5@pcmciplus\endcsname{4.5}
\expandafter\def\csname len@v6@context_0.5@pcmciplus\endcsname{3.4}
\expandafter\def\csname found@v6@context_0.5@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v6@context_0.5@pcmciplus\endcsname{0.62}
\expandafter\def\csname lift@v6@context_0.5@pc\endcsname{2.4}
\expandafter\def\csname len@v6@context_0.5@pc\endcsname{5.4}
\expandafter\def\csname found@v6@context_0.5@pc\endcsname{1.8}
\expandafter\def\csname beyond@v6@context_0.5@pc\endcsname{0.40}
\expandafter\def\csname lift@v6@context_0.5@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@context_0.5@dynotears\endcsname{0.1}
\expandafter\def\csname found@v6@context_0.5@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v6@context_0.5@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v6@context_0.5@varlingam\endcsname{1.9}
\expandafter\def\csname len@v6@context_0.5@varlingam\endcsname{8.5}
\expandafter\def\csname found@v6@context_0.5@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v6@context_0.5@varlingam\endcsname{0.40}
\expandafter\def\csname lift@v6@context_0.5@doubleml\endcsname{4.4}
\expandafter\def\csname len@v6@context_0.5@doubleml\endcsname{3.0}
\expandafter\def\csname found@v6@context_0.5@doubleml\endcsname{1.8}
\expandafter\def\csname beyond@v6@context_0.5@doubleml\endcsname{0.51}
\expandafter\def\csname lift@v6@context_0.5@spacetime_rule\endcsname{7.3}
\expandafter\def\csname len@v6@context_0.5@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v6@context_0.5@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v6@context_0.5@spacetime_rule\endcsname{0.40}
\expandafter\def\csname lift@v6@context_0.75@correlation\endcsname{1.1}
\expandafter\def\csname len@v6@context_0.75@correlation\endcsname{17.0}
\expandafter\def\csname found@v6@context_0.75@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@context_0.75@correlation\endcsname{0.10}
\expandafter\def\csname lift@v6@context_0.75@granger\endcsname{1.2}
\expandafter\def\csname len@v6@context_0.75@granger\endcsname{14.8}
\expandafter\def\csname found@v6@context_0.75@granger\endcsname{2.4}
\expandafter\def\csname beyond@v6@context_0.75@granger\endcsname{0.13}
\expandafter\def\csname lift@v6@context_0.75@pcmciplus\endcsname{4.2}
\expandafter\def\csname len@v6@context_0.75@pcmciplus\endcsname{3.3}
\expandafter\def\csname found@v6@context_0.75@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v6@context_0.75@pcmciplus\endcsname{0.55}
\expandafter\def\csname lift@v6@context_0.75@pc\endcsname{2.3}
\expandafter\def\csname len@v6@context_0.75@pc\endcsname{5.3}
\expandafter\def\csname found@v6@context_0.75@pc\endcsname{1.7}
\expandafter\def\csname beyond@v6@context_0.75@pc\endcsname{0.37}
\expandafter\def\csname lift@v6@context_0.75@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@context_0.75@dynotears\endcsname{0.1}
\expandafter\def\csname found@v6@context_0.75@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v6@context_0.75@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v6@context_0.75@varlingam\endcsname{2.1}
\expandafter\def\csname len@v6@context_0.75@varlingam\endcsname{7.4}
\expandafter\def\csname found@v6@context_0.75@varlingam\endcsname{2.1}
\expandafter\def\csname beyond@v6@context_0.75@varlingam\endcsname{0.43}
\expandafter\def\csname lift@v6@context_0.75@doubleml\endcsname{4.4}
\expandafter\def\csname len@v6@context_0.75@doubleml\endcsname{2.5}
\expandafter\def\csname found@v6@context_0.75@doubleml\endcsname{1.5}
\expandafter\def\csname beyond@v6@context_0.75@doubleml\endcsname{0.43}
\expandafter\def\csname lift@v6@context_0.75@spacetime_rule\endcsname{7.3}
\expandafter\def\csname len@v6@context_0.75@spacetime_rule\endcsname{0.9}
\expandafter\def\csname found@v6@context_0.75@spacetime_rule\endcsname{0.9}
\expandafter\def\csname beyond@v6@context_0.75@spacetime_rule\endcsname{0.30}
\expandafter\def\csname lift@v6@context_1.0@correlation\endcsname{1.2}
\expandafter\def\csname len@v6@context_1.0@correlation\endcsname{16.3}
\expandafter\def\csname found@v6@context_1.0@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@context_1.0@correlation\endcsname{0.14}
\expandafter\def\csname lift@v6@context_1.0@granger\endcsname{1.2}
\expandafter\def\csname len@v6@context_1.0@granger\endcsname{13.4}
\expandafter\def\csname found@v6@context_1.0@granger\endcsname{2.2}
\expandafter\def\csname beyond@v6@context_1.0@granger\endcsname{0.13}
\expandafter\def\csname lift@v6@context_1.0@pcmciplus\endcsname{4.5}
\expandafter\def\csname len@v6@context_1.0@pcmciplus\endcsname{3.4}
\expandafter\def\csname found@v6@context_1.0@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v6@context_1.0@pcmciplus\endcsname{0.62}
\expandafter\def\csname lift@v6@context_1.0@pc\endcsname{2.3}
\expandafter\def\csname len@v6@context_1.0@pc\endcsname{5.1}
\expandafter\def\csname found@v6@context_1.0@pc\endcsname{1.6}
\expandafter\def\csname beyond@v6@context_1.0@pc\endcsname{0.34}
\expandafter\def\csname lift@v6@context_1.0@dynotears\endcsname{--}
\expandafter\def\csname len@v6@context_1.0@dynotears\endcsname{0.0}
\expandafter\def\csname found@v6@context_1.0@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v6@context_1.0@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v6@context_1.0@varlingam\endcsname{2.4}
\expandafter\def\csname len@v6@context_1.0@varlingam\endcsname{6.6}
\expandafter\def\csname found@v6@context_1.0@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v6@context_1.0@varlingam\endcsname{0.52}
\expandafter\def\csname lift@v6@context_1.0@doubleml\endcsname{5.2}
\expandafter\def\csname len@v6@context_1.0@doubleml\endcsname{2.1}
\expandafter\def\csname found@v6@context_1.0@doubleml\endcsname{1.5}
\expandafter\def\csname beyond@v6@context_1.0@doubleml\endcsname{0.45}
\expandafter\def\csname lift@v6@context_1.0@spacetime_rule\endcsname{7.3}
\expandafter\def\csname len@v6@context_1.0@spacetime_rule\endcsname{0.8}
\expandafter\def\csname found@v6@context_1.0@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v6@context_1.0@spacetime_rule\endcsname{0.27}
\expandafter\def\csname lift@v6@context_0.75_combo_interaction@correlation\endcsname{0.9}
\expandafter\def\csname len@v6@context_0.75_combo_interaction@correlation\endcsname{5.4}
\expandafter\def\csname found@v6@context_0.75_combo_interaction@correlation\endcsname{0.7}
\expandafter\def\csname beyond@v6@context_0.75_combo_interaction@correlation\endcsname{0.01}
\expandafter\def\csname lift@v6@context_0.75_combo_interaction@granger\endcsname{1.6}
\expandafter\def\csname len@v6@context_0.75_combo_interaction@granger\endcsname{3.2}
\expandafter\def\csname found@v6@context_0.75_combo_interaction@granger\endcsname{0.7}
\expandafter\def\csname beyond@v6@context_0.75_combo_interaction@granger\endcsname{0.17}
\expandafter\def\csname lift@v6@context_0.75_combo_interaction@pcmciplus\endcsname{4.4}
\expandafter\def\csname len@v6@context_0.75_combo_interaction@pcmciplus\endcsname{0.5}
\expandafter\def\csname found@v6@context_0.75_combo_interaction@pcmciplus\endcsname{0.3}
\expandafter\def\csname beyond@v6@context_0.75_combo_interaction@pcmciplus\endcsname{0.09}
\expandafter\def\csname lift@v6@context_0.75_combo_interaction@pc\endcsname{0.6}
\expandafter\def\csname len@v6@context_0.75_combo_interaction@pc\endcsname{2.4}
\expandafter\def\csname found@v6@context_0.75_combo_interaction@pc\endcsname{0.2}
\expandafter\def\csname beyond@v6@context_0.75_combo_interaction@pc\endcsname{-0.05}
\expandafter\def\csname lift@v6@context_0.75_combo_interaction@dynotears\endcsname{--}
\expandafter\def\csname len@v6@context_0.75_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname found@v6@context_0.75_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v6@context_0.75_combo_interaction@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v6@context_0.75_combo_interaction@varlingam\endcsname{1.1}
\expandafter\def\csname len@v6@context_0.75_combo_interaction@varlingam\endcsname{2.7}
\expandafter\def\csname found@v6@context_0.75_combo_interaction@varlingam\endcsname{0.4}
\expandafter\def\csname beyond@v6@context_0.75_combo_interaction@varlingam\endcsname{0.02}
\expandafter\def\csname lift@v6@context_0.75_combo_interaction@doubleml\endcsname{2.9}
\expandafter\def\csname len@v6@context_0.75_combo_interaction@doubleml\endcsname{0.5}
\expandafter\def\csname found@v6@context_0.75_combo_interaction@doubleml\endcsname{0.2}
\expandafter\def\csname beyond@v6@context_0.75_combo_interaction@doubleml\endcsname{0.06}
\expandafter\def\csname lift@v6@context_0.75_combo_interaction@spacetime_rule\endcsname{2.9}
\expandafter\def\csname len@v6@context_0.75_combo_interaction@spacetime_rule\endcsname{1.0}
\expandafter\def\csname found@v6@context_0.75_combo_interaction@spacetime_rule\endcsname{0.4}
\expandafter\def\csname beyond@v6@context_0.75_combo_interaction@spacetime_rule\endcsname{0.10}
\expandafter\def\csname lift@v6@context_0.75_s40@correlation\endcsname{1.2}
\expandafter\def\csname len@v6@context_0.75_s40@correlation\endcsname{32.4}
\expandafter\def\csname found@v6@context_0.75_s40@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@context_0.75_s40@correlation\endcsname{0.16}
\expandafter\def\csname lift@v6@context_0.75_s40@granger\endcsname{1.3}
\expandafter\def\csname len@v6@context_0.75_s40@granger\endcsname{26.9}
\expandafter\def\csname found@v6@context_0.75_s40@granger\endcsname{2.4}
\expandafter\def\csname beyond@v6@context_0.75_s40@granger\endcsname{0.24}
\expandafter\def\csname lift@v6@context_0.75_s40@pcmciplus\endcsname{8.4}
\expandafter\def\csname len@v6@context_0.75_s40@pcmciplus\endcsname{2.5}
\expandafter\def\csname found@v6@context_0.75_s40@pcmciplus\endcsname{1.4}
\expandafter\def\csname beyond@v6@context_0.75_s40@pcmciplus\endcsname{0.47}
\expandafter\def\csname lift@v6@context_0.75_s40@pc\endcsname{4.5}
\expandafter\def\csname len@v6@context_0.75_s40@pc\endcsname{4.7}
\expandafter\def\csname found@v6@context_0.75_s40@pc\endcsname{1.4}
\expandafter\def\csname beyond@v6@context_0.75_s40@pc\endcsname{0.42}
\expandafter\def\csname lift@v6@context_0.75_s40@dynotears\endcsname{--}
\expandafter\def\csname len@v6@context_0.75_s40@dynotears\endcsname{0.0}
\expandafter\def\csname found@v6@context_0.75_s40@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v6@context_0.75_s40@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v6@context_0.75_s40@varlingam\endcsname{2.9}
\expandafter\def\csname len@v6@context_0.75_s40@varlingam\endcsname{8.7}
\expandafter\def\csname found@v6@context_0.75_s40@varlingam\endcsname{1.7}
\expandafter\def\csname beyond@v6@context_0.75_s40@varlingam\endcsname{0.41}
\expandafter\def\csname lift@v6@context_0.75_s40@doubleml\endcsname{11.5}
\expandafter\def\csname len@v6@context_0.75_s40@doubleml\endcsname{1.7}
\expandafter\def\csname found@v6@context_0.75_s40@doubleml\endcsname{1.3}
\expandafter\def\csname beyond@v6@context_0.75_s40@doubleml\endcsname{0.45}
\expandafter\def\csname lift@v6@context_0.75_s40@spacetime_rule\endcsname{13.8}
\expandafter\def\csname len@v6@context_0.75_s40@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v6@context_0.75_s40@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v6@context_0.75_s40@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v6@context_0.75_b50@correlation\endcsname{1.2}
\expandafter\def\csname len@v6@context_0.75_b50@correlation\endcsname{13.0}
\expandafter\def\csname found@v6@context_0.75_b50@correlation\endcsname{2.2}
\expandafter\def\csname beyond@v6@context_0.75_b50@correlation\endcsname{0.15}
\expandafter\def\csname lift@v6@context_0.75_b50@granger\endcsname{2.0}
\expandafter\def\csname len@v6@context_0.75_b50@granger\endcsname{6.6}
\expandafter\def\csname found@v6@context_0.75_b50@granger\endcsname{1.8}
\expandafter\def\csname beyond@v6@context_0.75_b50@granger\endcsname{0.37}
\expandafter\def\csname lift@v6@context_0.75_b50@pcmciplus\endcsname{4.3}
\expandafter\def\csname len@v6@context_0.75_b50@pcmciplus\endcsname{1.7}
\expandafter\def\csname found@v6@context_0.75_b50@pcmciplus\endcsname{1.0}
\expandafter\def\csname beyond@v6@context_0.75_b50@pcmciplus\endcsname{0.29}
\expandafter\def\csname lift@v6@context_0.75_b50@pc\endcsname{2.7}
\expandafter\def\csname len@v6@context_0.75_b50@pc\endcsname{4.3}
\expandafter\def\csname found@v6@context_0.75_b50@pc\endcsname{1.6}
\expandafter\def\csname beyond@v6@context_0.75_b50@pc\endcsname{0.38}
\expandafter\def\csname lift@v6@context_0.75_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@context_0.75_b50@dynotears\endcsname{0.2}
\expandafter\def\csname found@v6@context_0.75_b50@dynotears\endcsname{0.2}
\expandafter\def\csname beyond@v6@context_0.75_b50@dynotears\endcsname{0.06}
\expandafter\def\csname lift@v6@context_0.75_b50@varlingam\endcsname{2.2}
\expandafter\def\csname len@v6@context_0.75_b50@varlingam\endcsname{3.9}
\expandafter\def\csname found@v6@context_0.75_b50@varlingam\endcsname{1.2}
\expandafter\def\csname beyond@v6@context_0.75_b50@varlingam\endcsname{0.23}
\expandafter\def\csname lift@v6@context_0.75_b50@doubleml\endcsname{5.3}
\expandafter\def\csname len@v6@context_0.75_b50@doubleml\endcsname{1.1}
\expandafter\def\csname found@v6@context_0.75_b50@doubleml\endcsname{0.8}
\expandafter\def\csname beyond@v6@context_0.75_b50@doubleml\endcsname{0.24}
\expandafter\def\csname lift@v6@context_0.75_b50@spacetime_rule\endcsname{6.4}
\expandafter\def\csname len@v6@context_0.75_b50@spacetime_rule\endcsname{0.8}
\expandafter\def\csname found@v6@context_0.75_b50@spacetime_rule\endcsname{0.7}
\expandafter\def\csname beyond@v6@context_0.75_b50@spacetime_rule\endcsname{0.22}
\expandafter\def\csname lift@v6@jitter_0.25@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@jitter_0.25@correlation\endcsname{18.5}
\expandafter\def\csname found@v6@jitter_0.25@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@jitter_0.25@correlation\endcsname{0.02}
\expandafter\def\csname lift@v6@jitter_0.25@granger\endcsname{1.0}
\expandafter\def\csname len@v6@jitter_0.25@granger\endcsname{17.1}
\expandafter\def\csname found@v6@jitter_0.25@granger\endcsname{2.4}
\expandafter\def\csname beyond@v6@jitter_0.25@granger\endcsname{0.02}
\expandafter\def\csname lift@v6@jitter_0.25@pcmciplus\endcsname{5.2}
\expandafter\def\csname len@v6@jitter_0.25@pcmciplus\endcsname{3.5}
\expandafter\def\csname found@v6@jitter_0.25@pcmciplus\endcsname{2.5}
\expandafter\def\csname beyond@v6@jitter_0.25@pcmciplus\endcsname{0.76}
\expandafter\def\csname lift@v6@jitter_0.25@pc\endcsname{2.5}
\expandafter\def\csname len@v6@jitter_0.25@pc\endcsname{5.6}
\expandafter\def\csname found@v6@jitter_0.25@pc\endcsname{1.9}
\expandafter\def\csname beyond@v6@jitter_0.25@pc\endcsname{0.42}
\expandafter\def\csname lift@v6@jitter_0.25@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@jitter_0.25@dynotears\endcsname{0.8}
\expandafter\def\csname found@v6@jitter_0.25@dynotears\endcsname{0.8}
\expandafter\def\csname beyond@v6@jitter_0.25@dynotears\endcsname{0.26}
\expandafter\def\csname lift@v6@jitter_0.25@varlingam\endcsname{1.8}
\expandafter\def\csname len@v6@jitter_0.25@varlingam\endcsname{9.9}
\expandafter\def\csname found@v6@jitter_0.25@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v6@jitter_0.25@varlingam\endcsname{0.42}
\expandafter\def\csname lift@v6@jitter_0.25@doubleml\endcsname{4.3}
\expandafter\def\csname len@v6@jitter_0.25@doubleml\endcsname{4.1}
\expandafter\def\csname found@v6@jitter_0.25@doubleml\endcsname{2.4}
\expandafter\def\csname beyond@v6@jitter_0.25@doubleml\endcsname{0.68}
\expandafter\def\csname lift@v6@jitter_0.25@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v6@jitter_0.25@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v6@jitter_0.25@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v6@jitter_0.25@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v6@jitter_0.5@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@jitter_0.5@correlation\endcsname{18.4}
\expandafter\def\csname found@v6@jitter_0.5@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@jitter_0.5@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@jitter_0.5@granger\endcsname{1.1}
\expandafter\def\csname len@v6@jitter_0.5@granger\endcsname{17.3}
\expandafter\def\csname found@v6@jitter_0.5@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@jitter_0.5@granger\endcsname{0.05}
\expandafter\def\csname lift@v6@jitter_0.5@pcmciplus\endcsname{5.1}
\expandafter\def\csname len@v6@jitter_0.5@pcmciplus\endcsname{3.3}
\expandafter\def\csname found@v6@jitter_0.5@pcmciplus\endcsname{2.3}
\expandafter\def\csname beyond@v6@jitter_0.5@pcmciplus\endcsname{0.70}
\expandafter\def\csname lift@v6@jitter_0.5@pc\endcsname{2.3}
\expandafter\def\csname len@v6@jitter_0.5@pc\endcsname{5.7}
\expandafter\def\csname found@v6@jitter_0.5@pc\endcsname{1.8}
\expandafter\def\csname beyond@v6@jitter_0.5@pc\endcsname{0.38}
\expandafter\def\csname lift@v6@jitter_0.5@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@jitter_0.5@dynotears\endcsname{1.4}
\expandafter\def\csname found@v6@jitter_0.5@dynotears\endcsname{1.4}
\expandafter\def\csname beyond@v6@jitter_0.5@dynotears\endcsname{0.46}
\expandafter\def\csname lift@v6@jitter_0.5@varlingam\endcsname{1.9}
\expandafter\def\csname len@v6@jitter_0.5@varlingam\endcsname{9.6}
\expandafter\def\csname found@v6@jitter_0.5@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v6@jitter_0.5@varlingam\endcsname{0.44}
\expandafter\def\csname lift@v6@jitter_0.5@doubleml\endcsname{4.7}
\expandafter\def\csname len@v6@jitter_0.5@doubleml\endcsname{3.7}
\expandafter\def\csname found@v6@jitter_0.5@doubleml\endcsname{2.4}
\expandafter\def\csname beyond@v6@jitter_0.5@doubleml\endcsname{0.70}
\expandafter\def\csname lift@v6@jitter_0.5@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v6@jitter_0.5@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v6@jitter_0.5@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v6@jitter_0.5@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v6@jitter_1.0@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@jitter_1.0@correlation\endcsname{18.2}
\expandafter\def\csname found@v6@jitter_1.0@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@jitter_1.0@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@jitter_1.0@granger\endcsname{1.1}
\expandafter\def\csname len@v6@jitter_1.0@granger\endcsname{17.2}
\expandafter\def\csname found@v6@jitter_1.0@granger\endcsname{2.6}
\expandafter\def\csname beyond@v6@jitter_1.0@granger\endcsname{0.10}
\expandafter\def\csname lift@v6@jitter_1.0@pcmciplus\endcsname{4.6}
\expandafter\def\csname len@v6@jitter_1.0@pcmciplus\endcsname{4.0}
\expandafter\def\csname found@v6@jitter_1.0@pcmciplus\endcsname{2.5}
\expandafter\def\csname beyond@v6@jitter_1.0@pcmciplus\endcsname{0.73}
\expandafter\def\csname lift@v6@jitter_1.0@pc\endcsname{2.1}
\expandafter\def\csname len@v6@jitter_1.0@pc\endcsname{6.2}
\expandafter\def\csname found@v6@jitter_1.0@pc\endcsname{1.8}
\expandafter\def\csname beyond@v6@jitter_1.0@pc\endcsname{0.36}
\expandafter\def\csname lift@v6@jitter_1.0@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@jitter_1.0@dynotears\endcsname{1.5}
\expandafter\def\csname found@v6@jitter_1.0@dynotears\endcsname{1.5}
\expandafter\def\csname beyond@v6@jitter_1.0@dynotears\endcsname{0.49}
\expandafter\def\csname lift@v6@jitter_1.0@varlingam\endcsname{2.1}
\expandafter\def\csname len@v6@jitter_1.0@varlingam\endcsname{8.9}
\expandafter\def\csname found@v6@jitter_1.0@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v6@jitter_1.0@varlingam\endcsname{0.48}
\expandafter\def\csname lift@v6@jitter_1.0@doubleml\endcsname{5.4}
\expandafter\def\csname len@v6@jitter_1.0@doubleml\endcsname{3.1}
\expandafter\def\csname found@v6@jitter_1.0@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v6@jitter_1.0@doubleml\endcsname{0.70}
\expandafter\def\csname lift@v6@jitter_1.0@spacetime_rule\endcsname{6.0}
\expandafter\def\csname len@v6@jitter_1.0@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v6@jitter_1.0@spacetime_rule\endcsname{0.9}
\expandafter\def\csname beyond@v6@jitter_1.0@spacetime_rule\endcsname{0.29}
\expandafter\def\csname lift@v6@jitter_0.75@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@jitter_0.75@correlation\endcsname{18.4}
\expandafter\def\csname found@v6@jitter_0.75@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@jitter_0.75@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@jitter_0.75@granger\endcsname{1.0}
\expandafter\def\csname len@v6@jitter_0.75@granger\endcsname{17.5}
\expandafter\def\csname found@v6@jitter_0.75@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@jitter_0.75@granger\endcsname{0.04}
\expandafter\def\csname lift@v6@jitter_0.75@pcmciplus\endcsname{5.3}
\expandafter\def\csname len@v6@jitter_0.75@pcmciplus\endcsname{3.3}
\expandafter\def\csname found@v6@jitter_0.75@pcmciplus\endcsname{2.4}
\expandafter\def\csname beyond@v6@jitter_0.75@pcmciplus\endcsname{0.75}
\expandafter\def\csname lift@v6@jitter_0.75@pc\endcsname{2.3}
\expandafter\def\csname len@v6@jitter_0.75@pc\endcsname{5.8}
\expandafter\def\csname found@v6@jitter_0.75@pc\endcsname{1.8}
\expandafter\def\csname beyond@v6@jitter_0.75@pc\endcsname{0.38}
\expandafter\def\csname lift@v6@jitter_0.75@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@jitter_0.75@dynotears\endcsname{1.5}
\expandafter\def\csname found@v6@jitter_0.75@dynotears\endcsname{1.5}
\expandafter\def\csname beyond@v6@jitter_0.75@dynotears\endcsname{0.49}
\expandafter\def\csname lift@v6@jitter_0.75@varlingam\endcsname{2.1}
\expandafter\def\csname len@v6@jitter_0.75@varlingam\endcsname{8.9}
\expandafter\def\csname found@v6@jitter_0.75@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v6@jitter_0.75@varlingam\endcsname{0.50}
\expandafter\def\csname lift@v6@jitter_0.75@doubleml\endcsname{5.0}
\expandafter\def\csname len@v6@jitter_0.75@doubleml\endcsname{3.2}
\expandafter\def\csname found@v6@jitter_0.75@doubleml\endcsname{2.2}
\expandafter\def\csname beyond@v6@jitter_0.75@doubleml\endcsname{0.66}
\expandafter\def\csname lift@v6@jitter_0.75@spacetime_rule\endcsname{6.2}
\expandafter\def\csname len@v6@jitter_0.75@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v6@jitter_0.75@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v6@jitter_0.75@spacetime_rule\endcsname{0.36}
\expandafter\def\csname lift@v6@jitter_0.75_combo_interaction@correlation\endcsname{0.8}
\expandafter\def\csname len@v6@jitter_0.75_combo_interaction@correlation\endcsname{5.7}
\expandafter\def\csname found@v6@jitter_0.75_combo_interaction@correlation\endcsname{0.6}
\expandafter\def\csname beyond@v6@jitter_0.75_combo_interaction@correlation\endcsname{-0.05}
\expandafter\def\csname lift@v6@jitter_0.75_combo_interaction@granger\endcsname{1.5}
\expandafter\def\csname len@v6@jitter_0.75_combo_interaction@granger\endcsname{3.4}
\expandafter\def\csname found@v6@jitter_0.75_combo_interaction@granger\endcsname{0.7}
\expandafter\def\csname beyond@v6@jitter_0.75_combo_interaction@granger\endcsname{0.16}
\expandafter\def\csname lift@v6@jitter_0.75_combo_interaction@pcmciplus\endcsname{3.7}
\expandafter\def\csname len@v6@jitter_0.75_combo_interaction@pcmciplus\endcsname{1.4}
\expandafter\def\csname found@v6@jitter_0.75_combo_interaction@pcmciplus\endcsname{0.7}
\expandafter\def\csname beyond@v6@jitter_0.75_combo_interaction@pcmciplus\endcsname{0.20}
\expandafter\def\csname lift@v6@jitter_0.75_combo_interaction@pc\endcsname{0.6}
\expandafter\def\csname len@v6@jitter_0.75_combo_interaction@pc\endcsname{2.6}
\expandafter\def\csname found@v6@jitter_0.75_combo_interaction@pc\endcsname{0.2}
\expandafter\def\csname beyond@v6@jitter_0.75_combo_interaction@pc\endcsname{-0.06}
\expandafter\def\csname lift@v6@jitter_0.75_combo_interaction@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@jitter_0.75_combo_interaction@dynotears\endcsname{0.1}
\expandafter\def\csname found@v6@jitter_0.75_combo_interaction@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v6@jitter_0.75_combo_interaction@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v6@jitter_0.75_combo_interaction@varlingam\endcsname{1.1}
\expandafter\def\csname len@v6@jitter_0.75_combo_interaction@varlingam\endcsname{4.6}
\expandafter\def\csname found@v6@jitter_0.75_combo_interaction@varlingam\endcsname{0.7}
\expandafter\def\csname beyond@v6@jitter_0.75_combo_interaction@varlingam\endcsname{0.04}
\expandafter\def\csname lift@v6@jitter_0.75_combo_interaction@doubleml\endcsname{1.5}
\expandafter\def\csname len@v6@jitter_0.75_combo_interaction@doubleml\endcsname{0.5}
\expandafter\def\csname found@v6@jitter_0.75_combo_interaction@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v6@jitter_0.75_combo_interaction@doubleml\endcsname{0.02}
\expandafter\def\csname lift@v6@jitter_0.75_combo_interaction@spacetime_rule\endcsname{3.3}
\expandafter\def\csname len@v6@jitter_0.75_combo_interaction@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v6@jitter_0.75_combo_interaction@spacetime_rule\endcsname{0.5}
\expandafter\def\csname beyond@v6@jitter_0.75_combo_interaction@spacetime_rule\endcsname{0.13}
\expandafter\def\csname lift@v6@jitter_0.75_s40@correlation\endcsname{1.1}
\expandafter\def\csname len@v6@jitter_0.75_s40@correlation\endcsname{36.6}
\expandafter\def\csname found@v6@jitter_0.75_s40@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@jitter_0.75_s40@correlation\endcsname{0.06}
\expandafter\def\csname lift@v6@jitter_0.75_s40@granger\endcsname{1.1}
\expandafter\def\csname len@v6@jitter_0.75_s40@granger\endcsname{33.7}
\expandafter\def\csname found@v6@jitter_0.75_s40@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@jitter_0.75_s40@granger\endcsname{0.10}
\expandafter\def\csname lift@v6@jitter_0.75_s40@pcmciplus\endcsname{10.1}
\expandafter\def\csname len@v6@jitter_0.75_s40@pcmciplus\endcsname{3.4}
\expandafter\def\csname found@v6@jitter_0.75_s40@pcmciplus\endcsname{2.3}
\expandafter\def\csname beyond@v6@jitter_0.75_s40@pcmciplus\endcsname{0.79}
\expandafter\def\csname lift@v6@jitter_0.75_s40@pc\endcsname{3.2}
\expandafter\def\csname len@v6@jitter_0.75_s40@pc\endcsname{6.0}
\expandafter\def\csname found@v6@jitter_0.75_s40@pc\endcsname{1.3}
\expandafter\def\csname beyond@v6@jitter_0.75_s40@pc\endcsname{0.35}
\expandafter\def\csname lift@v6@jitter_0.75_s40@dynotears\endcsname{15.0}
\expandafter\def\csname len@v6@jitter_0.75_s40@dynotears\endcsname{1.3}
\expandafter\def\csname found@v6@jitter_0.75_s40@dynotears\endcsname{1.3}
\expandafter\def\csname beyond@v6@jitter_0.75_s40@dynotears\endcsname{0.46}
\expandafter\def\csname lift@v6@jitter_0.75_s40@varlingam\endcsname{3.5}
\expandafter\def\csname len@v6@jitter_0.75_s40@varlingam\endcsname{9.3}
\expandafter\def\csname found@v6@jitter_0.75_s40@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v6@jitter_0.75_s40@varlingam\endcsname{0.57}
\expandafter\def\csname lift@v6@jitter_0.75_s40@doubleml\endcsname{10.3}
\expandafter\def\csname len@v6@jitter_0.75_s40@doubleml\endcsname{3.2}
\expandafter\def\csname found@v6@jitter_0.75_s40@doubleml\endcsname{2.2}
\expandafter\def\csname beyond@v6@jitter_0.75_s40@doubleml\endcsname{0.75}
\expandafter\def\csname lift@v6@jitter_0.75_s40@spacetime_rule\endcsname{10.9}
\expandafter\def\csname len@v6@jitter_0.75_s40@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v6@jitter_0.75_s40@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v6@jitter_0.75_s40@spacetime_rule\endcsname{0.28}
\expandafter\def\csname lift@v6@jitter_0.75_b50@correlation\endcsname{1.2}
\expandafter\def\csname len@v6@jitter_0.75_b50@correlation\endcsname{15.5}
\expandafter\def\csname found@v6@jitter_0.75_b50@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@jitter_0.75_b50@correlation\endcsname{0.18}
\expandafter\def\csname lift@v6@jitter_0.75_b50@granger\endcsname{1.7}
\expandafter\def\csname len@v6@jitter_0.75_b50@granger\endcsname{10.5}
\expandafter\def\csname found@v6@jitter_0.75_b50@granger\endcsname{2.4}
\expandafter\def\csname beyond@v6@jitter_0.75_b50@granger\endcsname{0.39}
\expandafter\def\csname lift@v6@jitter_0.75_b50@pcmciplus\endcsname{5.7}
\expandafter\def\csname len@v6@jitter_0.75_b50@pcmciplus\endcsname{2.8}
\expandafter\def\csname found@v6@jitter_0.75_b50@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v6@jitter_0.75_b50@pcmciplus\endcsname{0.69}
\expandafter\def\csname lift@v6@jitter_0.75_b50@pc\endcsname{3.0}
\expandafter\def\csname len@v6@jitter_0.75_b50@pc\endcsname{4.1}
\expandafter\def\csname found@v6@jitter_0.75_b50@pc\endcsname{1.7}
\expandafter\def\csname beyond@v6@jitter_0.75_b50@pc\endcsname{0.42}
\expandafter\def\csname lift@v6@jitter_0.75_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@jitter_0.75_b50@dynotears\endcsname{1.4}
\expandafter\def\csname found@v6@jitter_0.75_b50@dynotears\endcsname{1.4}
\expandafter\def\csname beyond@v6@jitter_0.75_b50@dynotears\endcsname{0.46}
\expandafter\def\csname lift@v6@jitter_0.75_b50@varlingam\endcsname{2.5}
\expandafter\def\csname len@v6@jitter_0.75_b50@varlingam\endcsname{7.1}
\expandafter\def\csname found@v6@jitter_0.75_b50@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v6@jitter_0.75_b50@varlingam\endcsname{0.52}
\expandafter\def\csname lift@v6@jitter_0.75_b50@doubleml\endcsname{5.8}
\expandafter\def\csname len@v6@jitter_0.75_b50@doubleml\endcsname{2.4}
\expandafter\def\csname found@v6@jitter_0.75_b50@doubleml\endcsname{1.9}
\expandafter\def\csname beyond@v6@jitter_0.75_b50@doubleml\endcsname{0.59}
\expandafter\def\csname lift@v6@jitter_0.75_b50@spacetime_rule\endcsname{6.4}
\expandafter\def\csname len@v6@jitter_0.75_b50@spacetime_rule\endcsname{0.8}
\expandafter\def\csname found@v6@jitter_0.75_b50@spacetime_rule\endcsname{0.7}
\expandafter\def\csname beyond@v6@jitter_0.75_b50@spacetime_rule\endcsname{0.23}
\expandafter\def\csname lift@v6@cumul_0.25@correlation\endcsname{1.1}
\expandafter\def\csname len@v6@cumul_0.25@correlation\endcsname{18.0}
\expandafter\def\csname found@v6@cumul_0.25@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@cumul_0.25@correlation\endcsname{0.05}
\expandafter\def\csname lift@v6@cumul_0.25@granger\endcsname{1.1}
\expandafter\def\csname len@v6@cumul_0.25@granger\endcsname{16.0}
\expandafter\def\csname found@v6@cumul_0.25@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@cumul_0.25@granger\endcsname{0.10}
\expandafter\def\csname lift@v6@cumul_0.25@pcmciplus\endcsname{6.4}
\expandafter\def\csname len@v6@cumul_0.25@pcmciplus\endcsname{2.5}
\expandafter\def\csname found@v6@cumul_0.25@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v6@cumul_0.25@pcmciplus\endcsname{0.70}
\expandafter\def\csname lift@v6@cumul_0.25@pc\endcsname{2.6}
\expandafter\def\csname len@v6@cumul_0.25@pc\endcsname{5.7}
\expandafter\def\csname found@v6@cumul_0.25@pc\endcsname{2.0}
\expandafter\def\csname beyond@v6@cumul_0.25@pc\endcsname{0.45}
\expandafter\def\csname lift@v6@cumul_0.25@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@cumul_0.25@dynotears\endcsname{0.4}
\expandafter\def\csname found@v6@cumul_0.25@dynotears\endcsname{0.4}
\expandafter\def\csname beyond@v6@cumul_0.25@dynotears\endcsname{0.13}
\expandafter\def\csname lift@v6@cumul_0.25@varlingam\endcsname{1.7}
\expandafter\def\csname len@v6@cumul_0.25@varlingam\endcsname{10.8}
\expandafter\def\csname found@v6@cumul_0.25@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v6@cumul_0.25@varlingam\endcsname{0.36}
\expandafter\def\csname lift@v6@cumul_0.25@doubleml\endcsname{5.0}
\expandafter\def\csname len@v6@cumul_0.25@doubleml\endcsname{3.1}
\expandafter\def\csname found@v6@cumul_0.25@doubleml\endcsname{2.1}
\expandafter\def\csname beyond@v6@cumul_0.25@doubleml\endcsname{0.62}
\expandafter\def\csname lift@v6@cumul_0.25@spacetime_rule\endcsname{6.4}
\expandafter\def\csname len@v6@cumul_0.25@spacetime_rule\endcsname{0.8}
\expandafter\def\csname found@v6@cumul_0.25@spacetime_rule\endcsname{0.7}
\expandafter\def\csname beyond@v6@cumul_0.25@spacetime_rule\endcsname{0.23}
\expandafter\def\csname lift@v6@cumul_0.5@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@cumul_0.5@correlation\endcsname{18.3}
\expandafter\def\csname found@v6@cumul_0.5@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@cumul_0.5@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@cumul_0.5@granger\endcsname{1.1}
\expandafter\def\csname len@v6@cumul_0.5@granger\endcsname{16.0}
\expandafter\def\csname found@v6@cumul_0.5@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@cumul_0.5@granger\endcsname{0.10}
\expandafter\def\csname lift@v6@cumul_0.5@pcmciplus\endcsname{6.7}
\expandafter\def\csname len@v6@cumul_0.5@pcmciplus\endcsname{2.3}
\expandafter\def\csname found@v6@cumul_0.5@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v6@cumul_0.5@pcmciplus\endcsname{0.67}
\expandafter\def\csname lift@v6@cumul_0.5@pc\endcsname{2.5}
\expandafter\def\csname len@v6@cumul_0.5@pc\endcsname{5.8}
\expandafter\def\csname found@v6@cumul_0.5@pc\endcsname{2.0}
\expandafter\def\csname beyond@v6@cumul_0.5@pc\endcsname{0.45}
\expandafter\def\csname lift@v6@cumul_0.5@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@cumul_0.5@dynotears\endcsname{0.5}
\expandafter\def\csname found@v6@cumul_0.5@dynotears\endcsname{0.5}
\expandafter\def\csname beyond@v6@cumul_0.5@dynotears\endcsname{0.17}
\expandafter\def\csname lift@v6@cumul_0.5@varlingam\endcsname{1.6}
\expandafter\def\csname len@v6@cumul_0.5@varlingam\endcsname{11.3}
\expandafter\def\csname found@v6@cumul_0.5@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v6@cumul_0.5@varlingam\endcsname{0.32}
\expandafter\def\csname lift@v6@cumul_0.5@doubleml\endcsname{5.5}
\expandafter\def\csname len@v6@cumul_0.5@doubleml\endcsname{2.8}
\expandafter\def\csname found@v6@cumul_0.5@doubleml\endcsname{2.1}
\expandafter\def\csname beyond@v6@cumul_0.5@doubleml\endcsname{0.64}
\expandafter\def\csname lift@v6@cumul_0.5@spacetime_rule\endcsname{7.3}
\expandafter\def\csname len@v6@cumul_0.5@spacetime_rule\endcsname{0.6}
\expandafter\def\csname found@v6@cumul_0.5@spacetime_rule\endcsname{0.6}
\expandafter\def\csname beyond@v6@cumul_0.5@spacetime_rule\endcsname{0.20}
\expandafter\def\csname lift@v6@cumul_0.75@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@cumul_0.75@correlation\endcsname{18.6}
\expandafter\def\csname found@v6@cumul_0.75@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@cumul_0.75@correlation\endcsname{0.02}
\expandafter\def\csname lift@v6@cumul_0.75@granger\endcsname{1.1}
\expandafter\def\csname len@v6@cumul_0.75@granger\endcsname{16.7}
\expandafter\def\csname found@v6@cumul_0.75@granger\endcsname{2.6}
\expandafter\def\csname beyond@v6@cumul_0.75@granger\endcsname{0.11}
\expandafter\def\csname lift@v6@cumul_0.75@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v6@cumul_0.75@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v6@cumul_0.75@pcmciplus\endcsname{2.0}
\expandafter\def\csname beyond@v6@cumul_0.75@pcmciplus\endcsname{0.62}
\expandafter\def\csname lift@v6@cumul_0.75@pc\endcsname{2.5}
\expandafter\def\csname len@v6@cumul_0.75@pc\endcsname{5.8}
\expandafter\def\csname found@v6@cumul_0.75@pc\endcsname{2.0}
\expandafter\def\csname beyond@v6@cumul_0.75@pc\endcsname{0.45}
\expandafter\def\csname lift@v6@cumul_0.75@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@cumul_0.75@dynotears\endcsname{0.5}
\expandafter\def\csname found@v6@cumul_0.75@dynotears\endcsname{0.5}
\expandafter\def\csname beyond@v6@cumul_0.75@dynotears\endcsname{0.17}
\expandafter\def\csname lift@v6@cumul_0.75@varlingam\endcsname{1.7}
\expandafter\def\csname len@v6@cumul_0.75@varlingam\endcsname{9.8}
\expandafter\def\csname found@v6@cumul_0.75@varlingam\endcsname{2.3}
\expandafter\def\csname beyond@v6@cumul_0.75@varlingam\endcsname{0.38}
\expandafter\def\csname lift@v6@cumul_0.75@doubleml\endcsname{5.8}
\expandafter\def\csname len@v6@cumul_0.75@doubleml\endcsname{2.4}
\expandafter\def\csname found@v6@cumul_0.75@doubleml\endcsname{1.9}
\expandafter\def\csname beyond@v6@cumul_0.75@doubleml\endcsname{0.59}
\expandafter\def\csname lift@v6@cumul_0.75@spacetime_rule\endcsname{7.3}
\expandafter\def\csname len@v6@cumul_0.75@spacetime_rule\endcsname{0.4}
\expandafter\def\csname found@v6@cumul_0.75@spacetime_rule\endcsname{0.4}
\expandafter\def\csname beyond@v6@cumul_0.75@spacetime_rule\endcsname{0.13}
\expandafter\def\csname lift@v6@cumul_1.0@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@cumul_1.0@correlation\endcsname{18.3}
\expandafter\def\csname found@v6@cumul_1.0@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@cumul_1.0@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@cumul_1.0@granger\endcsname{1.1}
\expandafter\def\csname len@v6@cumul_1.0@granger\endcsname{17.3}
\expandafter\def\csname found@v6@cumul_1.0@granger\endcsname{2.6}
\expandafter\def\csname beyond@v6@cumul_1.0@granger\endcsname{0.09}
\expandafter\def\csname lift@v6@cumul_1.0@pcmciplus\endcsname{5.7}
\expandafter\def\csname len@v6@cumul_1.0@pcmciplus\endcsname{3.2}
\expandafter\def\csname found@v6@cumul_1.0@pcmciplus\endcsname{2.5}
\expandafter\def\csname beyond@v6@cumul_1.0@pcmciplus\endcsname{0.78}
\expandafter\def\csname lift@v6@cumul_1.0@pc\endcsname{2.4}
\expandafter\def\csname len@v6@cumul_1.0@pc\endcsname{5.5}
\expandafter\def\csname found@v6@cumul_1.0@pc\endcsname{1.8}
\expandafter\def\csname beyond@v6@cumul_1.0@pc\endcsname{0.39}
\expandafter\def\csname lift@v6@cumul_1.0@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@cumul_1.0@dynotears\endcsname{1.2}
\expandafter\def\csname found@v6@cumul_1.0@dynotears\endcsname{1.2}
\expandafter\def\csname beyond@v6@cumul_1.0@dynotears\endcsname{0.40}
\expandafter\def\csname lift@v6@cumul_1.0@varlingam\endcsname{2.2}
\expandafter\def\csname len@v6@cumul_1.0@varlingam\endcsname{7.9}
\expandafter\def\csname found@v6@cumul_1.0@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v6@cumul_1.0@varlingam\endcsname{0.48}
\expandafter\def\csname lift@v6@cumul_1.0@doubleml\endcsname{5.7}
\expandafter\def\csname len@v6@cumul_1.0@doubleml\endcsname{2.7}
\expandafter\def\csname found@v6@cumul_1.0@doubleml\endcsname{2.1}
\expandafter\def\csname beyond@v6@cumul_1.0@doubleml\endcsname{0.65}
\expandafter\def\csname lift@v6@cumul_1.0@spacetime_rule\endcsname{7.3}
\expandafter\def\csname len@v6@cumul_1.0@spacetime_rule\endcsname{0.5}
\expandafter\def\csname found@v6@cumul_1.0@spacetime_rule\endcsname{0.5}
\expandafter\def\csname beyond@v6@cumul_1.0@spacetime_rule\endcsname{0.17}
\expandafter\def\csname lift@v6@cumul_0.75_combo_interaction@correlation\endcsname{1.2}
\expandafter\def\csname len@v6@cumul_0.75_combo_interaction@correlation\endcsname{7.1}
\expandafter\def\csname found@v6@cumul_0.75_combo_interaction@correlation\endcsname{1.2}
\expandafter\def\csname beyond@v6@cumul_0.75_combo_interaction@correlation\endcsname{0.13}
\expandafter\def\csname lift@v6@cumul_0.75_combo_interaction@granger\endcsname{1.6}
\expandafter\def\csname len@v6@cumul_0.75_combo_interaction@granger\endcsname{4.7}
\expandafter\def\csname found@v6@cumul_0.75_combo_interaction@granger\endcsname{1.0}
\expandafter\def\csname beyond@v6@cumul_0.75_combo_interaction@granger\endcsname{0.21}
\expandafter\def\csname lift@v6@cumul_0.75_combo_interaction@pcmciplus\endcsname{4.7}
\expandafter\def\csname len@v6@cumul_0.75_combo_interaction@pcmciplus\endcsname{1.4}
\expandafter\def\csname found@v6@cumul_0.75_combo_interaction@pcmciplus\endcsname{0.9}
\expandafter\def\csname beyond@v6@cumul_0.75_combo_interaction@pcmciplus\endcsname{0.27}
\expandafter\def\csname lift@v6@cumul_0.75_combo_interaction@pc\endcsname{0.7}
\expandafter\def\csname len@v6@cumul_0.75_combo_interaction@pc\endcsname{3.1}
\expandafter\def\csname found@v6@cumul_0.75_combo_interaction@pc\endcsname{0.3}
\expandafter\def\csname beyond@v6@cumul_0.75_combo_interaction@pc\endcsname{-0.06}
\expandafter\def\csname lift@v6@cumul_0.75_combo_interaction@dynotears\endcsname{--}
\expandafter\def\csname len@v6@cumul_0.75_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname found@v6@cumul_0.75_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v6@cumul_0.75_combo_interaction@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v6@cumul_0.75_combo_interaction@varlingam\endcsname{1.4}
\expandafter\def\csname len@v6@cumul_0.75_combo_interaction@varlingam\endcsname{6.8}
\expandafter\def\csname found@v6@cumul_0.75_combo_interaction@varlingam\endcsname{1.3}
\expandafter\def\csname beyond@v6@cumul_0.75_combo_interaction@varlingam\endcsname{0.16}
\expandafter\def\csname lift@v6@cumul_0.75_combo_interaction@doubleml\endcsname{7.3}
\expandafter\def\csname len@v6@cumul_0.75_combo_interaction@doubleml\endcsname{0.1}
\expandafter\def\csname found@v6@cumul_0.75_combo_interaction@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v6@cumul_0.75_combo_interaction@doubleml\endcsname{0.03}
\expandafter\def\csname lift@v6@cumul_0.75_combo_interaction@spacetime_rule\endcsname{2.4}
\expandafter\def\csname len@v6@cumul_0.75_combo_interaction@spacetime_rule\endcsname{0.9}
\expandafter\def\csname found@v6@cumul_0.75_combo_interaction@spacetime_rule\endcsname{0.3}
\expandafter\def\csname beyond@v6@cumul_0.75_combo_interaction@spacetime_rule\endcsname{0.07}
\expandafter\def\csname lift@v6@cumul_0.75_s40@correlation\endcsname{1.1}
\expandafter\def\csname len@v6@cumul_0.75_s40@correlation\endcsname{35.8}
\expandafter\def\csname found@v6@cumul_0.75_s40@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@cumul_0.75_s40@correlation\endcsname{0.07}
\expandafter\def\csname lift@v6@cumul_0.75_s40@granger\endcsname{1.3}
\expandafter\def\csname len@v6@cumul_0.75_s40@granger\endcsname{29.4}
\expandafter\def\csname found@v6@cumul_0.75_s40@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@cumul_0.75_s40@granger\endcsname{0.23}
\expandafter\def\csname lift@v6@cumul_0.75_s40@pcmciplus\endcsname{10.5}
\expandafter\def\csname len@v6@cumul_0.75_s40@pcmciplus\endcsname{3.0}
\expandafter\def\csname found@v6@cumul_0.75_s40@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v6@cumul_0.75_s40@pcmciplus\endcsname{0.73}
\expandafter\def\csname lift@v6@cumul_0.75_s40@pc\endcsname{3.5}
\expandafter\def\csname len@v6@cumul_0.75_s40@pc\endcsname{6.0}
\expandafter\def\csname found@v6@cumul_0.75_s40@pc\endcsname{1.4}
\expandafter\def\csname beyond@v6@cumul_0.75_s40@pc\endcsname{0.38}
\expandafter\def\csname lift@v6@cumul_0.75_s40@dynotears\endcsname{15.0}
\expandafter\def\csname len@v6@cumul_0.75_s40@dynotears\endcsname{0.4}
\expandafter\def\csname found@v6@cumul_0.75_s40@dynotears\endcsname{0.4}
\expandafter\def\csname beyond@v6@cumul_0.75_s40@dynotears\endcsname{0.15}
\expandafter\def\csname lift@v6@cumul_0.75_s40@varlingam\endcsname{2.9}
\expandafter\def\csname len@v6@cumul_0.75_s40@varlingam\endcsname{11.7}
\expandafter\def\csname found@v6@cumul_0.75_s40@varlingam\endcsname{2.3}
\expandafter\def\csname beyond@v6@cumul_0.75_s40@varlingam\endcsname{0.55}
\expandafter\def\csname lift@v6@cumul_0.75_s40@doubleml\endcsname{12.8}
\expandafter\def\csname len@v6@cumul_0.75_s40@doubleml\endcsname{2.0}
\expandafter\def\csname found@v6@cumul_0.75_s40@doubleml\endcsname{1.7}
\expandafter\def\csname beyond@v6@cumul_0.75_s40@doubleml\endcsname{0.60}
\expandafter\def\csname lift@v6@cumul_0.75_s40@spacetime_rule\endcsname{12.9}
\expandafter\def\csname len@v6@cumul_0.75_s40@spacetime_rule\endcsname{0.7}
\expandafter\def\csname found@v6@cumul_0.75_s40@spacetime_rule\endcsname{0.6}
\expandafter\def\csname beyond@v6@cumul_0.75_s40@spacetime_rule\endcsname{0.22}
\expandafter\def\csname lift@v6@cumul_0.75_b50@correlation\endcsname{1.3}
\expandafter\def\csname len@v6@cumul_0.75_b50@correlation\endcsname{14.4}
\expandafter\def\csname found@v6@cumul_0.75_b50@correlation\endcsname{2.5}
\expandafter\def\csname beyond@v6@cumul_0.75_b50@correlation\endcsname{0.20}
\expandafter\def\csname lift@v6@cumul_0.75_b50@granger\endcsname{1.8}
\expandafter\def\csname len@v6@cumul_0.75_b50@granger\endcsname{9.6}
\expandafter\def\csname found@v6@cumul_0.75_b50@granger\endcsname{2.3}
\expandafter\def\csname beyond@v6@cumul_0.75_b50@granger\endcsname{0.40}
\expandafter\def\csname lift@v6@cumul_0.75_b50@pcmciplus\endcsname{6.2}
\expandafter\def\csname len@v6@cumul_0.75_b50@pcmciplus\endcsname{2.0}
\expandafter\def\csname found@v6@cumul_0.75_b50@pcmciplus\endcsname{1.7}
\expandafter\def\csname beyond@v6@cumul_0.75_b50@pcmciplus\endcsname{0.54}
\expandafter\def\csname lift@v6@cumul_0.75_b50@pc\endcsname{2.5}
\expandafter\def\csname len@v6@cumul_0.75_b50@pc\endcsname{4.7}
\expandafter\def\csname found@v6@cumul_0.75_b50@pc\endcsname{1.6}
\expandafter\def\csname beyond@v6@cumul_0.75_b50@pc\endcsname{0.34}
\expandafter\def\csname lift@v6@cumul_0.75_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@cumul_0.75_b50@dynotears\endcsname{0.6}
\expandafter\def\csname found@v6@cumul_0.75_b50@dynotears\endcsname{0.6}
\expandafter\def\csname beyond@v6@cumul_0.75_b50@dynotears\endcsname{0.20}
\expandafter\def\csname lift@v6@cumul_0.75_b50@varlingam\endcsname{2.3}
\expandafter\def\csname len@v6@cumul_0.75_b50@varlingam\endcsname{6.9}
\expandafter\def\csname found@v6@cumul_0.75_b50@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v6@cumul_0.75_b50@varlingam\endcsname{0.44}
\expandafter\def\csname lift@v6@cumul_0.75_b50@doubleml\endcsname{5.4}
\expandafter\def\csname len@v6@cumul_0.75_b50@doubleml\endcsname{2.3}
\expandafter\def\csname found@v6@cumul_0.75_b50@doubleml\endcsname{1.7}
\expandafter\def\csname beyond@v6@cumul_0.75_b50@doubleml\endcsname{0.53}
\expandafter\def\csname lift@v6@cumul_0.75_b50@spacetime_rule\endcsname{7.3}
\expandafter\def\csname len@v6@cumul_0.75_b50@spacetime_rule\endcsname{0.5}
\expandafter\def\csname found@v6@cumul_0.75_b50@spacetime_rule\endcsname{0.5}
\expandafter\def\csname beyond@v6@cumul_0.75_b50@spacetime_rule\endcsname{0.17}
\expandafter\def\csname lift@v6@operator_0.1@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@operator_0.1@correlation\endcsname{18.3}
\expandafter\def\csname found@v6@operator_0.1@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@operator_0.1@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@operator_0.1@granger\endcsname{1.1}
\expandafter\def\csname len@v6@operator_0.1@granger\endcsname{17.3}
\expandafter\def\csname found@v6@operator_0.1@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@operator_0.1@granger\endcsname{0.05}
\expandafter\def\csname lift@v6@operator_0.1@pcmciplus\endcsname{5.7}
\expandafter\def\csname len@v6@operator_0.1@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v6@operator_0.1@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v6@operator_0.1@pcmciplus\endcsname{0.66}
\expandafter\def\csname lift@v6@operator_0.1@pc\endcsname{2.7}
\expandafter\def\csname len@v6@operator_0.1@pc\endcsname{5.5}
\expandafter\def\csname found@v6@operator_0.1@pc\endcsname{2.0}
\expandafter\def\csname beyond@v6@operator_0.1@pc\endcsname{0.47}
\expandafter\def\csname lift@v6@operator_0.1@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@operator_0.1@dynotears\endcsname{0.8}
\expandafter\def\csname found@v6@operator_0.1@dynotears\endcsname{0.8}
\expandafter\def\csname beyond@v6@operator_0.1@dynotears\endcsname{0.26}
\expandafter\def\csname lift@v6@operator_0.1@varlingam\endcsname{1.8}
\expandafter\def\csname len@v6@operator_0.1@varlingam\endcsname{10.0}
\expandafter\def\csname found@v6@operator_0.1@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v6@operator_0.1@varlingam\endcsname{0.37}
\expandafter\def\csname lift@v6@operator_0.1@doubleml\endcsname{5.4}
\expandafter\def\csname len@v6@operator_0.1@doubleml\endcsname{3.4}
\expandafter\def\csname found@v6@operator_0.1@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v6@operator_0.1@doubleml\endcsname{0.76}
\expandafter\def\csname lift@v6@operator_0.1@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v6@operator_0.1@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v6@operator_0.1@spacetime_rule\endcsname{1.3}
\expandafter\def\csname beyond@v6@operator_0.1@spacetime_rule\endcsname{0.42}
\expandafter\def\csname lift@v6@operator_0.2@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@operator_0.2@correlation\endcsname{18.4}
\expandafter\def\csname found@v6@operator_0.2@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@operator_0.2@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@operator_0.2@granger\endcsname{1.1}
\expandafter\def\csname len@v6@operator_0.2@granger\endcsname{17.2}
\expandafter\def\csname found@v6@operator_0.2@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@operator_0.2@granger\endcsname{0.05}
\expandafter\def\csname lift@v6@operator_0.2@pcmciplus\endcsname{5.3}
\expandafter\def\csname len@v6@operator_0.2@pcmciplus\endcsname{2.9}
\expandafter\def\csname found@v6@operator_0.2@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v6@operator_0.2@pcmciplus\endcsname{0.65}
\expandafter\def\csname lift@v6@operator_0.2@pc\endcsname{2.6}
\expandafter\def\csname len@v6@operator_0.2@pc\endcsname{5.6}
\expandafter\def\csname found@v6@operator_0.2@pc\endcsname{2.0}
\expandafter\def\csname beyond@v6@operator_0.2@pc\endcsname{0.45}
\expandafter\def\csname lift@v6@operator_0.2@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@operator_0.2@dynotears\endcsname{0.8}
\expandafter\def\csname found@v6@operator_0.2@dynotears\endcsname{0.8}
\expandafter\def\csname beyond@v6@operator_0.2@dynotears\endcsname{0.26}
\expandafter\def\csname lift@v6@operator_0.2@varlingam\endcsname{2.0}
\expandafter\def\csname len@v6@operator_0.2@varlingam\endcsname{9.2}
\expandafter\def\csname found@v6@operator_0.2@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v6@operator_0.2@varlingam\endcsname{0.44}
\expandafter\def\csname lift@v6@operator_0.2@doubleml\endcsname{5.2}
\expandafter\def\csname len@v6@operator_0.2@doubleml\endcsname{3.5}
\expandafter\def\csname found@v6@operator_0.2@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v6@operator_0.2@doubleml\endcsname{0.75}
\expandafter\def\csname lift@v6@operator_0.2@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v6@operator_0.2@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v6@operator_0.2@spacetime_rule\endcsname{1.3}
\expandafter\def\csname beyond@v6@operator_0.2@spacetime_rule\endcsname{0.42}
\expandafter\def\csname lift@v6@operator_0.3@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@operator_0.3@correlation\endcsname{18.3}
\expandafter\def\csname found@v6@operator_0.3@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@operator_0.3@correlation\endcsname{0.04}
\expandafter\def\csname lift@v6@operator_0.3@granger\endcsname{1.1}
\expandafter\def\csname len@v6@operator_0.3@granger\endcsname{17.2}
\expandafter\def\csname found@v6@operator_0.3@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@operator_0.3@granger\endcsname{0.05}
\expandafter\def\csname lift@v6@operator_0.3@pcmciplus\endcsname{5.1}
\expandafter\def\csname len@v6@operator_0.3@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v6@operator_0.3@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v6@operator_0.3@pcmciplus\endcsname{0.58}
\expandafter\def\csname lift@v6@operator_0.3@pc\endcsname{2.5}
\expandafter\def\csname len@v6@operator_0.3@pc\endcsname{5.6}
\expandafter\def\csname found@v6@operator_0.3@pc\endcsname{1.9}
\expandafter\def\csname beyond@v6@operator_0.3@pc\endcsname{0.42}
\expandafter\def\csname lift@v6@operator_0.3@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@operator_0.3@dynotears\endcsname{0.8}
\expandafter\def\csname found@v6@operator_0.3@dynotears\endcsname{0.8}
\expandafter\def\csname beyond@v6@operator_0.3@dynotears\endcsname{0.26}
\expandafter\def\csname lift@v6@operator_0.3@varlingam\endcsname{2.0}
\expandafter\def\csname len@v6@operator_0.3@varlingam\endcsname{8.7}
\expandafter\def\csname found@v6@operator_0.3@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v6@operator_0.3@varlingam\endcsname{0.43}
\expandafter\def\csname lift@v6@operator_0.3@doubleml\endcsname{4.9}
\expandafter\def\csname len@v6@operator_0.3@doubleml\endcsname{3.7}
\expandafter\def\csname found@v6@operator_0.3@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v6@operator_0.3@doubleml\endcsname{0.74}
\expandafter\def\csname lift@v6@operator_0.3@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v6@operator_0.3@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v6@operator_0.3@spacetime_rule\endcsname{1.3}
\expandafter\def\csname beyond@v6@operator_0.3@spacetime_rule\endcsname{0.42}
\expandafter\def\csname lift@v6@operator_0.5@correlation\endcsname{1.0}
\expandafter\def\csname len@v6@operator_0.5@correlation\endcsname{18.4}
\expandafter\def\csname found@v6@operator_0.5@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@operator_0.5@correlation\endcsname{0.03}
\expandafter\def\csname lift@v6@operator_0.5@granger\endcsname{1.1}
\expandafter\def\csname len@v6@operator_0.5@granger\endcsname{17.2}
\expandafter\def\csname found@v6@operator_0.5@granger\endcsname{2.5}
\expandafter\def\csname beyond@v6@operator_0.5@granger\endcsname{0.05}
\expandafter\def\csname lift@v6@operator_0.5@pcmciplus\endcsname{5.3}
\expandafter\def\csname len@v6@operator_0.5@pcmciplus\endcsname{2.6}
\expandafter\def\csname found@v6@operator_0.5@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v6@operator_0.5@pcmciplus\endcsname{0.58}
\expandafter\def\csname lift@v6@operator_0.5@pc\endcsname{2.4}
\expandafter\def\csname len@v6@operator_0.5@pc\endcsname{5.7}
\expandafter\def\csname found@v6@operator_0.5@pc\endcsname{1.9}
\expandafter\def\csname beyond@v6@operator_0.5@pc\endcsname{0.41}
\expandafter\def\csname lift@v6@operator_0.5@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@operator_0.5@dynotears\endcsname{0.7}
\expandafter\def\csname found@v6@operator_0.5@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v6@operator_0.5@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v6@operator_0.5@varlingam\endcsname{1.9}
\expandafter\def\csname len@v6@operator_0.5@varlingam\endcsname{9.0}
\expandafter\def\csname found@v6@operator_0.5@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v6@operator_0.5@varlingam\endcsname{0.42}
\expandafter\def\csname lift@v6@operator_0.5@doubleml\endcsname{4.5}
\expandafter\def\csname len@v6@operator_0.5@doubleml\endcsname{4.1}
\expandafter\def\csname found@v6@operator_0.5@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v6@operator_0.5@doubleml\endcsname{0.71}
\expandafter\def\csname lift@v6@operator_0.5@spacetime_rule\endcsname{6.7}
\expandafter\def\csname len@v6@operator_0.5@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v6@operator_0.5@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v6@operator_0.5@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v6@operator_0.3_combo_interaction@correlation\endcsname{1.3}
\expandafter\def\csname len@v6@operator_0.3_combo_interaction@correlation\endcsname{7.2}
\expandafter\def\csname found@v6@operator_0.3_combo_interaction@correlation\endcsname{1.3}
\expandafter\def\csname beyond@v6@operator_0.3_combo_interaction@correlation\endcsname{0.14}
\expandafter\def\csname lift@v6@operator_0.3_combo_interaction@granger\endcsname{1.7}
\expandafter\def\csname len@v6@operator_0.3_combo_interaction@granger\endcsname{3.4}
\expandafter\def\csname found@v6@operator_0.3_combo_interaction@granger\endcsname{0.8}
\expandafter\def\csname beyond@v6@operator_0.3_combo_interaction@granger\endcsname{0.20}
\expandafter\def\csname lift@v6@operator_0.3_combo_interaction@pcmciplus\endcsname{2.7}
\expandafter\def\csname len@v6@operator_0.3_combo_interaction@pcmciplus\endcsname{1.1}
\expandafter\def\csname found@v6@operator_0.3_combo_interaction@pcmciplus\endcsname{0.4}
\expandafter\def\csname beyond@v6@operator_0.3_combo_interaction@pcmciplus\endcsname{0.10}
\expandafter\def\csname lift@v6@operator_0.3_combo_interaction@pc\endcsname{1.6}
\expandafter\def\csname len@v6@operator_0.3_combo_interaction@pc\endcsname{2.8}
\expandafter\def\csname found@v6@operator_0.3_combo_interaction@pc\endcsname{0.6}
\expandafter\def\csname beyond@v6@operator_0.3_combo_interaction@pc\endcsname{0.08}
\expandafter\def\csname lift@v6@operator_0.3_combo_interaction@dynotears\endcsname{--}
\expandafter\def\csname len@v6@operator_0.3_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname found@v6@operator_0.3_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v6@operator_0.3_combo_interaction@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v6@operator_0.3_combo_interaction@varlingam\endcsname{1.3}
\expandafter\def\csname len@v6@operator_0.3_combo_interaction@varlingam\endcsname{4.6}
\expandafter\def\csname found@v6@operator_0.3_combo_interaction@varlingam\endcsname{0.8}
\expandafter\def\csname beyond@v6@operator_0.3_combo_interaction@varlingam\endcsname{0.09}
\expandafter\def\csname lift@v6@operator_0.3_combo_interaction@doubleml\endcsname{2.4}
\expandafter\def\csname len@v6@operator_0.3_combo_interaction@doubleml\endcsname{0.3}
\expandafter\def\csname found@v6@operator_0.3_combo_interaction@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v6@operator_0.3_combo_interaction@doubleml\endcsname{0.03}
\expandafter\def\csname lift@v6@operator_0.3_combo_interaction@spacetime_rule\endcsname{4.0}
\expandafter\def\csname len@v6@operator_0.3_combo_interaction@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v6@operator_0.3_combo_interaction@spacetime_rule\endcsname{0.6}
\expandafter\def\csname beyond@v6@operator_0.3_combo_interaction@spacetime_rule\endcsname{0.17}
\expandafter\def\csname lift@v6@operator_0.3_s40@correlation\endcsname{1.1}
\expandafter\def\csname len@v6@operator_0.3_s40@correlation\endcsname{35.9}
\expandafter\def\csname found@v6@operator_0.3_s40@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@operator_0.3_s40@correlation\endcsname{0.07}
\expandafter\def\csname lift@v6@operator_0.3_s40@granger\endcsname{1.2}
\expandafter\def\csname len@v6@operator_0.3_s40@granger\endcsname{32.0}
\expandafter\def\csname found@v6@operator_0.3_s40@granger\endcsname{2.6}
\expandafter\def\csname beyond@v6@operator_0.3_s40@granger\endcsname{0.17}
\expandafter\def\csname lift@v6@operator_0.3_s40@pcmciplus\endcsname{10.5}
\expandafter\def\csname len@v6@operator_0.3_s40@pcmciplus\endcsname{3.0}
\expandafter\def\csname found@v6@operator_0.3_s40@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v6@operator_0.3_s40@pcmciplus\endcsname{0.73}
\expandafter\def\csname lift@v6@operator_0.3_s40@pc\endcsname{4.3}
\expandafter\def\csname len@v6@operator_0.3_s40@pc\endcsname{5.6}
\expandafter\def\csname found@v6@operator_0.3_s40@pc\endcsname{1.6}
\expandafter\def\csname beyond@v6@operator_0.3_s40@pc\endcsname{0.47}
\expandafter\def\csname lift@v6@operator_0.3_s40@dynotears\endcsname{15.0}
\expandafter\def\csname len@v6@operator_0.3_s40@dynotears\endcsname{0.6}
\expandafter\def\csname found@v6@operator_0.3_s40@dynotears\endcsname{0.6}
\expandafter\def\csname beyond@v6@operator_0.3_s40@dynotears\endcsname{0.21}
\expandafter\def\csname lift@v6@operator_0.3_s40@varlingam\endcsname{2.6}
\expandafter\def\csname len@v6@operator_0.3_s40@varlingam\endcsname{13.9}
\expandafter\def\csname found@v6@operator_0.3_s40@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v6@operator_0.3_s40@varlingam\endcsname{0.57}
\expandafter\def\csname lift@v6@operator_0.3_s40@doubleml\endcsname{10.4}
\expandafter\def\csname len@v6@operator_0.3_s40@doubleml\endcsname{2.6}
\expandafter\def\csname found@v6@operator_0.3_s40@doubleml\endcsname{1.8}
\expandafter\def\csname beyond@v6@operator_0.3_s40@doubleml\endcsname{0.62}
\expandafter\def\csname lift@v6@operator_0.3_s40@spacetime_rule\endcsname{15.0}
\expandafter\def\csname len@v6@operator_0.3_s40@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v6@operator_0.3_s40@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v6@operator_0.3_s40@spacetime_rule\endcsname{0.40}
\expandafter\def\csname lift@v6@operator_0.3_b50@correlation\endcsname{1.1}
\expandafter\def\csname len@v6@operator_0.3_b50@correlation\endcsname{16.6}
\expandafter\def\csname found@v6@operator_0.3_b50@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@operator_0.3_b50@correlation\endcsname{0.12}
\expandafter\def\csname lift@v6@operator_0.3_b50@granger\endcsname{1.5}
\expandafter\def\csname len@v6@operator_0.3_b50@granger\endcsname{10.6}
\expandafter\def\csname found@v6@operator_0.3_b50@granger\endcsname{2.2}
\expandafter\def\csname beyond@v6@operator_0.3_b50@granger\endcsname{0.30}
\expandafter\def\csname lift@v6@operator_0.3_b50@pcmciplus\endcsname{6.2}
\expandafter\def\csname len@v6@operator_0.3_b50@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v6@operator_0.3_b50@pcmciplus\endcsname{2.3}
\expandafter\def\csname beyond@v6@operator_0.3_b50@pcmciplus\endcsname{0.72}
\expandafter\def\csname lift@v6@operator_0.3_b50@pc\endcsname{3.1}
\expandafter\def\csname len@v6@operator_0.3_b50@pc\endcsname{4.0}
\expandafter\def\csname found@v6@operator_0.3_b50@pc\endcsname{1.7}
\expandafter\def\csname beyond@v6@operator_0.3_b50@pc\endcsname{0.43}
\expandafter\def\csname lift@v6@operator_0.3_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@operator_0.3_b50@dynotears\endcsname{0.8}
\expandafter\def\csname found@v6@operator_0.3_b50@dynotears\endcsname{0.8}
\expandafter\def\csname beyond@v6@operator_0.3_b50@dynotears\endcsname{0.27}
\expandafter\def\csname lift@v6@operator_0.3_b50@varlingam\endcsname{2.6}
\expandafter\def\csname len@v6@operator_0.3_b50@varlingam\endcsname{6.9}
\expandafter\def\csname found@v6@operator_0.3_b50@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v6@operator_0.3_b50@varlingam\endcsname{0.60}
\expandafter\def\csname lift@v6@operator_0.3_b50@doubleml\endcsname{5.1}
\expandafter\def\csname len@v6@operator_0.3_b50@doubleml\endcsname{2.7}
\expandafter\def\csname found@v6@operator_0.3_b50@doubleml\endcsname{1.9}
\expandafter\def\csname beyond@v6@operator_0.3_b50@doubleml\endcsname{0.58}
\expandafter\def\csname lift@v6@operator_0.3_b50@spacetime_rule\endcsname{6.7}
\expandafter\def\csname len@v6@operator_0.3_b50@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v6@operator_0.3_b50@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v6@operator_0.3_b50@spacetime_rule\endcsname{0.36}
\expandafter\def\csname lift@v6@all_knobs@correlation\endcsname{1.2}
\expandafter\def\csname len@v6@all_knobs@correlation\endcsname{15.1}
\expandafter\def\csname found@v6@all_knobs@correlation\endcsname{2.5}
\expandafter\def\csname beyond@v6@all_knobs@correlation\endcsname{0.13}
\expandafter\def\csname lift@v6@all_knobs@granger\endcsname{1.4}
\expandafter\def\csname len@v6@all_knobs@granger\endcsname{11.2}
\expandafter\def\csname found@v6@all_knobs@granger\endcsname{2.2}
\expandafter\def\csname beyond@v6@all_knobs@granger\endcsname{0.26}
\expandafter\def\csname lift@v6@all_knobs@pcmciplus\endcsname{3.9}
\expandafter\def\csname len@v6@all_knobs@pcmciplus\endcsname{3.6}
\expandafter\def\csname found@v6@all_knobs@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v6@all_knobs@pcmciplus\endcsname{0.53}
\expandafter\def\csname lift@v6@all_knobs@pc\endcsname{1.7}
\expandafter\def\csname len@v6@all_knobs@pc\endcsname{6.5}
\expandafter\def\csname found@v6@all_knobs@pc\endcsname{1.5}
\expandafter\def\csname beyond@v6@all_knobs@pc\endcsname{0.22}
\expandafter\def\csname lift@v6@all_knobs@dynotears\endcsname{7.3}
\expandafter\def\csname len@v6@all_knobs@dynotears\endcsname{0.1}
\expandafter\def\csname found@v6@all_knobs@dynotears\endcsname{0.1}
\expandafter\def\csname beyond@v6@all_knobs@dynotears\endcsname{0.03}
\expandafter\def\csname lift@v6@all_knobs@varlingam\endcsname{2.8}
\expandafter\def\csname len@v6@all_knobs@varlingam\endcsname{5.3}
\expandafter\def\csname found@v6@all_knobs@varlingam\endcsname{2.0}
\expandafter\def\csname beyond@v6@all_knobs@varlingam\endcsname{0.46}
\expandafter\def\csname lift@v6@all_knobs@doubleml\endcsname{5.8}
\expandafter\def\csname len@v6@all_knobs@doubleml\endcsname{1.9}
\expandafter\def\csname found@v6@all_knobs@doubleml\endcsname{1.5}
\expandafter\def\csname beyond@v6@all_knobs@doubleml\endcsname{0.47}
\expandafter\def\csname lift@v6@all_knobs@spacetime_rule\endcsname{0.0}
\expandafter\def\csname len@v6@all_knobs@spacetime_rule\endcsname{0.1}
\expandafter\def\csname found@v6@all_knobs@spacetime_rule\endcsname{0.0}
\expandafter\def\csname beyond@v6@all_knobs@spacetime_rule\endcsname{-0.00}
\expandafter\def\csname lift@v6@all_knobs_combo_interaction@correlation\endcsname{1.7}
\expandafter\def\csname len@v6@all_knobs_combo_interaction@correlation\endcsname{6.6}
\expandafter\def\csname found@v6@all_knobs_combo_interaction@correlation\endcsname{1.5}
\expandafter\def\csname beyond@v6@all_knobs_combo_interaction@correlation\endcsname{0.27}
\expandafter\def\csname lift@v6@all_knobs_combo_interaction@granger\endcsname{1.7}
\expandafter\def\csname len@v6@all_knobs_combo_interaction@granger\endcsname{3.1}
\expandafter\def\csname found@v6@all_knobs_combo_interaction@granger\endcsname{0.7}
\expandafter\def\csname beyond@v6@all_knobs_combo_interaction@granger\endcsname{0.17}
\expandafter\def\csname lift@v6@all_knobs_combo_interaction@pcmciplus\endcsname{3.2}
\expandafter\def\csname len@v6@all_knobs_combo_interaction@pcmciplus\endcsname{1.8}
\expandafter\def\csname found@v6@all_knobs_combo_interaction@pcmciplus\endcsname{0.8}
\expandafter\def\csname beyond@v6@all_knobs_combo_interaction@pcmciplus\endcsname{0.22}
\expandafter\def\csname lift@v6@all_knobs_combo_interaction@pc\endcsname{1.9}
\expandafter\def\csname len@v6@all_knobs_combo_interaction@pc\endcsname{3.1}
\expandafter\def\csname found@v6@all_knobs_combo_interaction@pc\endcsname{0.8}
\expandafter\def\csname beyond@v6@all_knobs_combo_interaction@pc\endcsname{0.14}
\expandafter\def\csname lift@v6@all_knobs_combo_interaction@dynotears\endcsname{--}
\expandafter\def\csname len@v6@all_knobs_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname found@v6@all_knobs_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v6@all_knobs_combo_interaction@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v6@all_knobs_combo_interaction@varlingam\endcsname{1.0}
\expandafter\def\csname len@v6@all_knobs_combo_interaction@varlingam\endcsname{3.5}
\expandafter\def\csname found@v6@all_knobs_combo_interaction@varlingam\endcsname{0.5}
\expandafter\def\csname beyond@v6@all_knobs_combo_interaction@varlingam\endcsname{0.02}
\expandafter\def\csname lift@v6@all_knobs_combo_interaction@doubleml\endcsname{2.9}
\expandafter\def\csname len@v6@all_knobs_combo_interaction@doubleml\endcsname{0.5}
\expandafter\def\csname found@v6@all_knobs_combo_interaction@doubleml\endcsname{0.2}
\expandafter\def\csname beyond@v6@all_knobs_combo_interaction@doubleml\endcsname{0.05}
\expandafter\def\csname lift@v6@all_knobs_combo_interaction@spacetime_rule\endcsname{3.7}
\expandafter\def\csname len@v6@all_knobs_combo_interaction@spacetime_rule\endcsname{0.6}
\expandafter\def\csname found@v6@all_knobs_combo_interaction@spacetime_rule\endcsname{0.3}
\expandafter\def\csname beyond@v6@all_knobs_combo_interaction@spacetime_rule\endcsname{0.09}
\expandafter\def\csname lift@v6@all_knobs_s40@correlation\endcsname{1.3}
\expandafter\def\csname len@v6@all_knobs_s40@correlation\endcsname{30.0}
\expandafter\def\csname found@v6@all_knobs_s40@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v6@all_knobs_s40@correlation\endcsname{0.21}
\expandafter\def\csname lift@v6@all_knobs_s40@granger\endcsname{1.6}
\expandafter\def\csname len@v6@all_knobs_s40@granger\endcsname{18.5}
\expandafter\def\csname found@v6@all_knobs_s40@granger\endcsname{2.0}
\expandafter\def\csname beyond@v6@all_knobs_s40@granger\endcsname{0.32}
\expandafter\def\csname lift@v6@all_knobs_s40@pcmciplus\endcsname{7.5}
\expandafter\def\csname len@v6@all_knobs_s40@pcmciplus\endcsname{3.4}
\expandafter\def\csname found@v6@all_knobs_s40@pcmciplus\endcsname{1.7}
\expandafter\def\csname beyond@v6@all_knobs_s40@pcmciplus\endcsname{0.57}
\expandafter\def\csname lift@v6@all_knobs_s40@pc\endcsname{2.5}
\expandafter\def\csname len@v6@all_knobs_s40@pc\endcsname{7.1}
\expandafter\def\csname found@v6@all_knobs_s40@pc\endcsname{1.2}
\expandafter\def\csname beyond@v6@all_knobs_s40@pc\endcsname{0.27}
\expandafter\def\csname lift@v6@all_knobs_s40@dynotears\endcsname{--}
\expandafter\def\csname len@v6@all_knobs_s40@dynotears\endcsname{0.0}
\expandafter\def\csname found@v6@all_knobs_s40@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v6@all_knobs_s40@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v6@all_knobs_s40@varlingam\endcsname{3.7}
\expandafter\def\csname len@v6@all_knobs_s40@varlingam\endcsname{7.3}
\expandafter\def\csname found@v6@all_knobs_s40@varlingam\endcsname{1.8}
\expandafter\def\csname beyond@v6@all_knobs_s40@varlingam\endcsname{0.47}
\expandafter\def\csname lift@v6@all_knobs_s40@doubleml\endcsname{9.4}
\expandafter\def\csname len@v6@all_knobs_s40@doubleml\endcsname{1.6}
\expandafter\def\csname found@v6@all_knobs_s40@doubleml\endcsname{1.0}
\expandafter\def\csname beyond@v6@all_knobs_s40@doubleml\endcsname{0.34}
\expandafter\def\csname lift@v6@all_knobs_s40@spacetime_rule\endcsname{--}
\expandafter\def\csname len@v6@all_knobs_s40@spacetime_rule\endcsname{0.0}
\expandafter\def\csname found@v6@all_knobs_s40@spacetime_rule\endcsname{0.0}
\expandafter\def\csname beyond@v6@all_knobs_s40@spacetime_rule\endcsname{0.00}
\expandafter\def\csname lift@v7@reference@correlation\endcsname{1.0}
\expandafter\def\csname len@v7@reference@correlation\endcsname{18.2}
\expandafter\def\csname found@v7@reference@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v7@reference@correlation\endcsname{0.04}
\expandafter\def\csname lift@v7@reference@granger\endcsname{1.1}
\expandafter\def\csname len@v7@reference@granger\endcsname{17.1}
\expandafter\def\csname found@v7@reference@granger\endcsname{2.5}
\expandafter\def\csname beyond@v7@reference@granger\endcsname{0.06}
\expandafter\def\csname lift@v7@reference@pcmciplus\endcsname{5.7}
\expandafter\def\csname len@v7@reference@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v7@reference@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v7@reference@pcmciplus\endcsname{0.65}
\expandafter\def\csname lift@v7@reference@pc\endcsname{2.6}
\expandafter\def\csname len@v7@reference@pc\endcsname{5.4}
\expandafter\def\csname found@v7@reference@pc\endcsname{1.9}
\expandafter\def\csname beyond@v7@reference@pc\endcsname{0.43}
\expandafter\def\csname lift@v7@reference@dynotears\endcsname{7.3}
\expandafter\def\csname len@v7@reference@dynotears\endcsname{0.7}
\expandafter\def\csname found@v7@reference@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v7@reference@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v7@reference@varlingam\endcsname{1.7}
\expandafter\def\csname len@v7@reference@varlingam\endcsname{9.7}
\expandafter\def\csname found@v7@reference@varlingam\endcsname{2.3}
\expandafter\def\csname beyond@v7@reference@varlingam\endcsname{0.37}
\expandafter\def\csname lift@v7@reference@doubleml\endcsname{4.7}
\expandafter\def\csname len@v7@reference@doubleml\endcsname{3.9}
\expandafter\def\csname found@v7@reference@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v7@reference@doubleml\endcsname{0.73}
\expandafter\def\csname lift@v7@reference@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v7@reference@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v7@reference@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v7@reference@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v7@no_parameter_edges@correlation\endcsname{1.0}
\expandafter\def\csname len@v7@no_parameter_edges@correlation\endcsname{18.2}
\expandafter\def\csname found@v7@no_parameter_edges@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v7@no_parameter_edges@correlation\endcsname{0.03}
\expandafter\def\csname lift@v7@no_parameter_edges@granger\endcsname{1.1}
\expandafter\def\csname len@v7@no_parameter_edges@granger\endcsname{16.8}
\expandafter\def\csname found@v7@no_parameter_edges@granger\endcsname{2.5}
\expandafter\def\csname beyond@v7@no_parameter_edges@granger\endcsname{0.07}
\expandafter\def\csname lift@v7@no_parameter_edges@pcmciplus\endcsname{5.3}
\expandafter\def\csname len@v7@no_parameter_edges@pcmciplus\endcsname{2.9}
\expandafter\def\csname found@v7@no_parameter_edges@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v7@no_parameter_edges@pcmciplus\endcsname{0.64}
\expandafter\def\csname lift@v7@no_parameter_edges@pc\endcsname{2.7}
\expandafter\def\csname len@v7@no_parameter_edges@pc\endcsname{4.9}
\expandafter\def\csname found@v7@no_parameter_edges@pc\endcsname{1.8}
\expandafter\def\csname beyond@v7@no_parameter_edges@pc\endcsname{0.41}
\expandafter\def\csname lift@v7@no_parameter_edges@dynotears\endcsname{7.3}
\expandafter\def\csname len@v7@no_parameter_edges@dynotears\endcsname{0.8}
\expandafter\def\csname found@v7@no_parameter_edges@dynotears\endcsname{0.8}
\expandafter\def\csname beyond@v7@no_parameter_edges@dynotears\endcsname{0.26}
\expandafter\def\csname lift@v7@no_parameter_edges@varlingam\endcsname{2.0}
\expandafter\def\csname len@v7@no_parameter_edges@varlingam\endcsname{9.1}
\expandafter\def\csname found@v7@no_parameter_edges@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v7@no_parameter_edges@varlingam\endcsname{0.46}
\expandafter\def\csname lift@v7@no_parameter_edges@doubleml\endcsname{4.9}
\expandafter\def\csname len@v7@no_parameter_edges@doubleml\endcsname{3.7}
\expandafter\def\csname found@v7@no_parameter_edges@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v7@no_parameter_edges@doubleml\endcsname{0.74}
\expandafter\def\csname lift@v7@no_parameter_edges@spacetime_rule\endcsname{5.9}
\expandafter\def\csname len@v7@no_parameter_edges@spacetime_rule\endcsname{1.6}
\expandafter\def\csname found@v7@no_parameter_edges@spacetime_rule\endcsname{1.3}
\expandafter\def\csname beyond@v7@no_parameter_edges@spacetime_rule\endcsname{0.42}
\expandafter\def\csname lift@v7@no_temporal_edges@correlation\endcsname{1.1}
\expandafter\def\csname len@v7@no_temporal_edges@correlation\endcsname{16.7}
\expandafter\def\csname found@v7@no_temporal_edges@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v7@no_temporal_edges@correlation\endcsname{0.10}
\expandafter\def\csname lift@v7@no_temporal_edges@granger\endcsname{1.2}
\expandafter\def\csname len@v7@no_temporal_edges@granger\endcsname{16.3}
\expandafter\def\csname found@v7@no_temporal_edges@granger\endcsname{2.6}
\expandafter\def\csname beyond@v7@no_temporal_edges@granger\endcsname{0.15}
\expandafter\def\csname lift@v7@no_temporal_edges@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v7@no_temporal_edges@pcmciplus\endcsname{3.1}
\expandafter\def\csname found@v7@no_temporal_edges@pcmciplus\endcsname{2.3}
\expandafter\def\csname beyond@v7@no_temporal_edges@pcmciplus\endcsname{0.70}
\expandafter\def\csname lift@v7@no_temporal_edges@pc\endcsname{2.8}
\expandafter\def\csname len@v7@no_temporal_edges@pc\endcsname{4.9}
\expandafter\def\csname found@v7@no_temporal_edges@pc\endcsname{1.9}
\expandafter\def\csname beyond@v7@no_temporal_edges@pc\endcsname{0.45}
\expandafter\def\csname lift@v7@no_temporal_edges@dynotears\endcsname{7.3}
\expandafter\def\csname len@v7@no_temporal_edges@dynotears\endcsname{0.6}
\expandafter\def\csname found@v7@no_temporal_edges@dynotears\endcsname{0.6}
\expandafter\def\csname beyond@v7@no_temporal_edges@dynotears\endcsname{0.19}
\expandafter\def\csname lift@v7@no_temporal_edges@varlingam\endcsname{2.1}
\expandafter\def\csname len@v7@no_temporal_edges@varlingam\endcsname{8.9}
\expandafter\def\csname found@v7@no_temporal_edges@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v7@no_temporal_edges@varlingam\endcsname{0.50}
\expandafter\def\csname lift@v7@no_temporal_edges@doubleml\endcsname{5.8}
\expandafter\def\csname len@v7@no_temporal_edges@doubleml\endcsname{2.9}
\expandafter\def\csname found@v7@no_temporal_edges@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v7@no_temporal_edges@doubleml\endcsname{0.71}
\expandafter\def\csname lift@v7@no_temporal_edges@spacetime_rule\endcsname{6.0}
\expandafter\def\csname len@v7@no_temporal_edges@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v7@no_temporal_edges@spacetime_rule\endcsname{0.9}
\expandafter\def\csname beyond@v7@no_temporal_edges@spacetime_rule\endcsname{0.28}
\expandafter\def\csname lift@v8@phase_0.25@correlation\endcsname{1.1}
\expandafter\def\csname len@v8@phase_0.25@correlation\endcsname{18.0}
\expandafter\def\csname found@v8@phase_0.25@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v8@phase_0.25@correlation\endcsname{0.05}
\expandafter\def\csname lift@v8@phase_0.25@granger\endcsname{1.0}
\expandafter\def\csname len@v8@phase_0.25@granger\endcsname{17.2}
\expandafter\def\csname found@v8@phase_0.25@granger\endcsname{2.4}
\expandafter\def\csname beyond@v8@phase_0.25@granger\endcsname{0.02}
\expandafter\def\csname lift@v8@phase_0.25@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v8@phase_0.25@pcmciplus\endcsname{3.0}
\expandafter\def\csname found@v8@phase_0.25@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v8@phase_0.25@pcmciplus\endcsname{0.67}
\expandafter\def\csname lift@v8@phase_0.25@pc\endcsname{2.5}
\expandafter\def\csname len@v8@phase_0.25@pc\endcsname{5.6}
\expandafter\def\csname found@v8@phase_0.25@pc\endcsname{1.9}
\expandafter\def\csname beyond@v8@phase_0.25@pc\endcsname{0.41}
\expandafter\def\csname lift@v8@phase_0.25@dynotears\endcsname{7.3}
\expandafter\def\csname len@v8@phase_0.25@dynotears\endcsname{0.8}
\expandafter\def\csname found@v8@phase_0.25@dynotears\endcsname{0.8}
\expandafter\def\csname beyond@v8@phase_0.25@dynotears\endcsname{0.26}
\expandafter\def\csname lift@v8@phase_0.25@varlingam\endcsname{2.0}
\expandafter\def\csname len@v8@phase_0.25@varlingam\endcsname{9.3}
\expandafter\def\csname found@v8@phase_0.25@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v8@phase_0.25@varlingam\endcsname{0.48}
\expandafter\def\csname lift@v8@phase_0.25@doubleml\endcsname{4.7}
\expandafter\def\csname len@v8@phase_0.25@doubleml\endcsname{3.7}
\expandafter\def\csname found@v8@phase_0.25@doubleml\endcsname{2.4}
\expandafter\def\csname beyond@v8@phase_0.25@doubleml\endcsname{0.71}
\expandafter\def\csname lift@v8@phase_0.25@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v8@phase_0.25@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v8@phase_0.25@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v8@phase_0.25@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v8@phase_0.5@correlation\endcsname{1.1}
\expandafter\def\csname len@v8@phase_0.5@correlation\endcsname{18.0}
\expandafter\def\csname found@v8@phase_0.5@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v8@phase_0.5@correlation\endcsname{0.05}
\expandafter\def\csname lift@v8@phase_0.5@granger\endcsname{1.1}
\expandafter\def\csname len@v8@phase_0.5@granger\endcsname{16.7}
\expandafter\def\csname found@v8@phase_0.5@granger\endcsname{2.4}
\expandafter\def\csname beyond@v8@phase_0.5@granger\endcsname{0.05}
\expandafter\def\csname lift@v8@phase_0.5@pcmciplus\endcsname{5.3}
\expandafter\def\csname len@v8@phase_0.5@pcmciplus\endcsname{3.2}
\expandafter\def\csname found@v8@phase_0.5@pcmciplus\endcsname{2.3}
\expandafter\def\csname beyond@v8@phase_0.5@pcmciplus\endcsname{0.70}
\expandafter\def\csname lift@v8@phase_0.5@pc\endcsname{2.5}
\expandafter\def\csname len@v8@phase_0.5@pc\endcsname{5.6}
\expandafter\def\csname found@v8@phase_0.5@pc\endcsname{1.9}
\expandafter\def\csname beyond@v8@phase_0.5@pc\endcsname{0.42}
\expandafter\def\csname lift@v8@phase_0.5@dynotears\endcsname{7.3}
\expandafter\def\csname len@v8@phase_0.5@dynotears\endcsname{0.7}
\expandafter\def\csname found@v8@phase_0.5@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v8@phase_0.5@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v8@phase_0.5@varlingam\endcsname{1.8}
\expandafter\def\csname len@v8@phase_0.5@varlingam\endcsname{9.6}
\expandafter\def\csname found@v8@phase_0.5@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v8@phase_0.5@varlingam\endcsname{0.42}
\expandafter\def\csname lift@v8@phase_0.5@doubleml\endcsname{4.7}
\expandafter\def\csname len@v8@phase_0.5@doubleml\endcsname{3.7}
\expandafter\def\csname found@v8@phase_0.5@doubleml\endcsname{2.4}
\expandafter\def\csname beyond@v8@phase_0.5@doubleml\endcsname{0.71}
\expandafter\def\csname lift@v8@phase_0.5@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v8@phase_0.5@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v8@phase_0.5@spacetime_rule\endcsname{1.3}
\expandafter\def\csname beyond@v8@phase_0.5@spacetime_rule\endcsname{0.42}
\expandafter\def\csname lift@v8@phase_0.75@correlation\endcsname{1.1}
\expandafter\def\csname len@v8@phase_0.75@correlation\endcsname{17.9}
\expandafter\def\csname found@v8@phase_0.75@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v8@phase_0.75@correlation\endcsname{0.05}
\expandafter\def\csname lift@v8@phase_0.75@granger\endcsname{1.1}
\expandafter\def\csname len@v8@phase_0.75@granger\endcsname{16.6}
\expandafter\def\csname found@v8@phase_0.75@granger\endcsname{2.4}
\expandafter\def\csname beyond@v8@phase_0.75@granger\endcsname{0.05}
\expandafter\def\csname lift@v8@phase_0.75@pcmciplus\endcsname{4.9}
\expandafter\def\csname len@v8@phase_0.75@pcmciplus\endcsname{3.3}
\expandafter\def\csname found@v8@phase_0.75@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v8@phase_0.75@pcmciplus\endcsname{0.65}
\expandafter\def\csname lift@v8@phase_0.75@pc\endcsname{2.5}
\expandafter\def\csname len@v8@phase_0.75@pc\endcsname{5.5}
\expandafter\def\csname found@v8@phase_0.75@pc\endcsname{1.9}
\expandafter\def\csname beyond@v8@phase_0.75@pc\endcsname{0.42}
\expandafter\def\csname lift@v8@phase_0.75@dynotears\endcsname{7.3}
\expandafter\def\csname len@v8@phase_0.75@dynotears\endcsname{0.7}
\expandafter\def\csname found@v8@phase_0.75@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v8@phase_0.75@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v8@phase_0.75@varlingam\endcsname{1.9}
\expandafter\def\csname len@v8@phase_0.75@varlingam\endcsname{10.0}
\expandafter\def\csname found@v8@phase_0.75@varlingam\endcsname{2.6}
\expandafter\def\csname beyond@v8@phase_0.75@varlingam\endcsname{0.47}
\expandafter\def\csname lift@v8@phase_0.75@doubleml\endcsname{5.2}
\expandafter\def\csname len@v8@phase_0.75@doubleml\endcsname{3.5}
\expandafter\def\csname found@v8@phase_0.75@doubleml\endcsname{2.5}
\expandafter\def\csname beyond@v8@phase_0.75@doubleml\endcsname{0.75}
\expandafter\def\csname lift@v8@phase_0.75@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v8@phase_0.75@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v8@phase_0.75@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v8@phase_0.75@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v8@phase_0.9@correlation\endcsname{1.1}
\expandafter\def\csname len@v8@phase_0.9@correlation\endcsname{17.7}
\expandafter\def\csname found@v8@phase_0.9@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v8@phase_0.9@correlation\endcsname{0.06}
\expandafter\def\csname lift@v8@phase_0.9@granger\endcsname{1.1}
\expandafter\def\csname len@v8@phase_0.9@granger\endcsname{16.5}
\expandafter\def\csname found@v8@phase_0.9@granger\endcsname{2.4}
\expandafter\def\csname beyond@v8@phase_0.9@granger\endcsname{0.06}
\expandafter\def\csname lift@v8@phase_0.9@pcmciplus\endcsname{4.7}
\expandafter\def\csname len@v8@phase_0.9@pcmciplus\endcsname{3.4}
\expandafter\def\csname found@v8@phase_0.9@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v8@phase_0.9@pcmciplus\endcsname{0.65}
\expandafter\def\csname lift@v8@phase_0.9@pc\endcsname{2.6}
\expandafter\def\csname len@v8@phase_0.9@pc\endcsname{5.3}
\expandafter\def\csname found@v8@phase_0.9@pc\endcsname{1.9}
\expandafter\def\csname beyond@v8@phase_0.9@pc\endcsname{0.43}
\expandafter\def\csname lift@v8@phase_0.9@dynotears\endcsname{7.3}
\expandafter\def\csname len@v8@phase_0.9@dynotears\endcsname{0.7}
\expandafter\def\csname found@v8@phase_0.9@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v8@phase_0.9@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v8@phase_0.9@varlingam\endcsname{1.9}
\expandafter\def\csname len@v8@phase_0.9@varlingam\endcsname{9.5}
\expandafter\def\csname found@v8@phase_0.9@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v8@phase_0.9@varlingam\endcsname{0.45}
\expandafter\def\csname lift@v8@phase_0.9@doubleml\endcsname{5.0}
\expandafter\def\csname len@v8@phase_0.9@doubleml\endcsname{3.5}
\expandafter\def\csname found@v8@phase_0.9@doubleml\endcsname{2.4}
\expandafter\def\csname beyond@v8@phase_0.9@doubleml\endcsname{0.72}
\expandafter\def\csname lift@v8@phase_0.9@spacetime_rule\endcsname{5.8}
\expandafter\def\csname len@v8@phase_0.9@spacetime_rule\endcsname{1.5}
\expandafter\def\csname found@v8@phase_0.9@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v8@phase_0.9@spacetime_rule\endcsname{0.38}
\expandafter\def\csname lift@v8@phase_0.75_combo_interaction@correlation\endcsname{0.8}
\expandafter\def\csname len@v8@phase_0.75_combo_interaction@correlation\endcsname{5.7}
\expandafter\def\csname found@v8@phase_0.75_combo_interaction@correlation\endcsname{0.6}
\expandafter\def\csname beyond@v8@phase_0.75_combo_interaction@correlation\endcsname{-0.03}
\expandafter\def\csname lift@v8@phase_0.75_combo_interaction@granger\endcsname{0.8}
\expandafter\def\csname len@v8@phase_0.75_combo_interaction@granger\endcsname{3.7}
\expandafter\def\csname found@v8@phase_0.75_combo_interaction@granger\endcsname{0.4}
\expandafter\def\csname beyond@v8@phase_0.75_combo_interaction@granger\endcsname{0.04}
\expandafter\def\csname lift@v8@phase_0.75_combo_interaction@pcmciplus\endcsname{2.7}
\expandafter\def\csname len@v8@phase_0.75_combo_interaction@pcmciplus\endcsname{1.1}
\expandafter\def\csname found@v8@phase_0.75_combo_interaction@pcmciplus\endcsname{0.4}
\expandafter\def\csname beyond@v8@phase_0.75_combo_interaction@pcmciplus\endcsname{0.10}
\expandafter\def\csname lift@v8@phase_0.75_combo_interaction@pc\endcsname{1.0}
\expandafter\def\csname len@v8@phase_0.75_combo_interaction@pc\endcsname{2.9}
\expandafter\def\csname found@v8@phase_0.75_combo_interaction@pc\endcsname{0.4}
\expandafter\def\csname beyond@v8@phase_0.75_combo_interaction@pc\endcsname{0.00}
\expandafter\def\csname lift@v8@phase_0.75_combo_interaction@dynotears\endcsname{--}
\expandafter\def\csname len@v8@phase_0.75_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname found@v8@phase_0.75_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v8@phase_0.75_combo_interaction@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v8@phase_0.75_combo_interaction@varlingam\endcsname{1.3}
\expandafter\def\csname len@v8@phase_0.75_combo_interaction@varlingam\endcsname{5.1}
\expandafter\def\csname found@v8@phase_0.75_combo_interaction@varlingam\endcsname{0.9}
\expandafter\def\csname beyond@v8@phase_0.75_combo_interaction@varlingam\endcsname{0.08}
\expandafter\def\csname lift@v8@phase_0.75_combo_interaction@doubleml\endcsname{2.4}
\expandafter\def\csname len@v8@phase_0.75_combo_interaction@doubleml\endcsname{0.3}
\expandafter\def\csname found@v8@phase_0.75_combo_interaction@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v8@phase_0.75_combo_interaction@doubleml\endcsname{0.03}
\expandafter\def\csname lift@v8@phase_0.75_combo_interaction@spacetime_rule\endcsname{4.2}
\expandafter\def\csname len@v8@phase_0.75_combo_interaction@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v8@phase_0.75_combo_interaction@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v8@phase_0.75_combo_interaction@spacetime_rule\endcsname{0.23}
\expandafter\def\csname lift@v8@phase_0.75_s40@correlation\endcsname{1.1}
\expandafter\def\csname len@v8@phase_0.75_s40@correlation\endcsname{36.1}
\expandafter\def\csname found@v8@phase_0.75_s40@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v8@phase_0.75_s40@correlation\endcsname{0.07}
\expandafter\def\csname lift@v8@phase_0.75_s40@granger\endcsname{1.2}
\expandafter\def\csname len@v8@phase_0.75_s40@granger\endcsname{31.9}
\expandafter\def\csname found@v8@phase_0.75_s40@granger\endcsname{2.6}
\expandafter\def\csname beyond@v8@phase_0.75_s40@granger\endcsname{0.18}
\expandafter\def\csname lift@v8@phase_0.75_s40@pcmciplus\endcsname{11.1}
\expandafter\def\csname len@v8@phase_0.75_s40@pcmciplus\endcsname{3.1}
\expandafter\def\csname found@v8@phase_0.75_s40@pcmciplus\endcsname{2.3}
\expandafter\def\csname beyond@v8@phase_0.75_s40@pcmciplus\endcsname{0.80}
\expandafter\def\csname lift@v8@phase_0.75_s40@pc\endcsname{4.7}
\expandafter\def\csname len@v8@phase_0.75_s40@pc\endcsname{4.8}
\expandafter\def\csname found@v8@phase_0.75_s40@pc\endcsname{1.5}
\expandafter\def\csname beyond@v8@phase_0.75_s40@pc\endcsname{0.45}
\expandafter\def\csname lift@v8@phase_0.75_s40@dynotears\endcsname{15.0}
\expandafter\def\csname len@v8@phase_0.75_s40@dynotears\endcsname{0.4}
\expandafter\def\csname found@v8@phase_0.75_s40@dynotears\endcsname{0.4}
\expandafter\def\csname beyond@v8@phase_0.75_s40@dynotears\endcsname{0.14}
\expandafter\def\csname lift@v8@phase_0.75_s40@varlingam\endcsname{3.3}
\expandafter\def\csname len@v8@phase_0.75_s40@varlingam\endcsname{10.1}
\expandafter\def\csname found@v8@phase_0.75_s40@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v8@phase_0.75_s40@varlingam\endcsname{0.56}
\expandafter\def\csname lift@v8@phase_0.75_s40@doubleml\endcsname{12.1}
\expandafter\def\csname len@v8@phase_0.75_s40@doubleml\endcsname{2.6}
\expandafter\def\csname found@v8@phase_0.75_s40@doubleml\endcsname{2.1}
\expandafter\def\csname beyond@v8@phase_0.75_s40@doubleml\endcsname{0.73}
\expandafter\def\csname lift@v8@phase_0.75_s40@spacetime_rule\endcsname{12.3}
\expandafter\def\csname len@v8@phase_0.75_s40@spacetime_rule\endcsname{1.1}
\expandafter\def\csname found@v8@phase_0.75_s40@spacetime_rule\endcsname{0.9}
\expandafter\def\csname beyond@v8@phase_0.75_s40@spacetime_rule\endcsname{0.32}
\expandafter\def\csname lift@v8@phase_0.75_b50@correlation\endcsname{1.2}
\expandafter\def\csname len@v8@phase_0.75_b50@correlation\endcsname{15.2}
\expandafter\def\csname found@v8@phase_0.75_b50@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v8@phase_0.75_b50@correlation\endcsname{0.22}
\expandafter\def\csname lift@v8@phase_0.75_b50@granger\endcsname{1.8}
\expandafter\def\csname len@v8@phase_0.75_b50@granger\endcsname{9.6}
\expandafter\def\csname found@v8@phase_0.75_b50@granger\endcsname{2.3}
\expandafter\def\csname beyond@v8@phase_0.75_b50@granger\endcsname{0.41}
\expandafter\def\csname lift@v8@phase_0.75_b50@pcmciplus\endcsname{5.9}
\expandafter\def\csname len@v8@phase_0.75_b50@pcmciplus\endcsname{2.1}
\expandafter\def\csname found@v8@phase_0.75_b50@pcmciplus\endcsname{1.7}
\expandafter\def\csname beyond@v8@phase_0.75_b50@pcmciplus\endcsname{0.54}
\expandafter\def\csname lift@v8@phase_0.75_b50@pc\endcsname{3.4}
\expandafter\def\csname len@v8@phase_0.75_b50@pc\endcsname{4.1}
\expandafter\def\csname found@v8@phase_0.75_b50@pc\endcsname{1.9}
\expandafter\def\csname beyond@v8@phase_0.75_b50@pc\endcsname{0.49}
\expandafter\def\csname lift@v8@phase_0.75_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v8@phase_0.75_b50@dynotears\endcsname{0.6}
\expandafter\def\csname found@v8@phase_0.75_b50@dynotears\endcsname{0.6}
\expandafter\def\csname beyond@v8@phase_0.75_b50@dynotears\endcsname{0.19}
\expandafter\def\csname lift@v8@phase_0.75_b50@varlingam\endcsname{2.5}
\expandafter\def\csname len@v8@phase_0.75_b50@varlingam\endcsname{5.5}
\expandafter\def\csname found@v8@phase_0.75_b50@varlingam\endcsname{1.9}
\expandafter\def\csname beyond@v8@phase_0.75_b50@varlingam\endcsname{0.43}
\expandafter\def\csname lift@v8@phase_0.75_b50@doubleml\endcsname{4.7}
\expandafter\def\csname len@v8@phase_0.75_b50@doubleml\endcsname{3.1}
\expandafter\def\csname found@v8@phase_0.75_b50@doubleml\endcsname{2.0}
\expandafter\def\csname beyond@v8@phase_0.75_b50@doubleml\endcsname{0.59}
\expandafter\def\csname lift@v8@phase_0.75_b50@spacetime_rule\endcsname{5.1}
\expandafter\def\csname len@v8@phase_0.75_b50@spacetime_rule\endcsname{1.0}
\expandafter\def\csname found@v8@phase_0.75_b50@spacetime_rule\endcsname{0.7}
\expandafter\def\csname beyond@v8@phase_0.75_b50@spacetime_rule\endcsname{0.22}
\expandafter\def\csname lift@v9@lot_0.25@correlation\endcsname{1.0}
\expandafter\def\csname len@v9@lot_0.25@correlation\endcsname{18.5}
\expandafter\def\csname found@v9@lot_0.25@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v9@lot_0.25@correlation\endcsname{0.02}
\expandafter\def\csname lift@v9@lot_0.25@granger\endcsname{1.1}
\expandafter\def\csname len@v9@lot_0.25@granger\endcsname{17.1}
\expandafter\def\csname found@v9@lot_0.25@granger\endcsname{2.5}
\expandafter\def\csname beyond@v9@lot_0.25@granger\endcsname{0.06}
\expandafter\def\csname lift@v9@lot_0.25@pcmciplus\endcsname{5.3}
\expandafter\def\csname len@v9@lot_0.25@pcmciplus\endcsname{2.6}
\expandafter\def\csname found@v9@lot_0.25@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v9@lot_0.25@pcmciplus\endcsname{0.57}
\expandafter\def\csname lift@v9@lot_0.25@pc\endcsname{2.6}
\expandafter\def\csname len@v9@lot_0.25@pc\endcsname{5.1}
\expandafter\def\csname found@v9@lot_0.25@pc\endcsname{1.8}
\expandafter\def\csname beyond@v9@lot_0.25@pc\endcsname{0.41}
\expandafter\def\csname lift@v9@lot_0.25@dynotears\endcsname{7.3}
\expandafter\def\csname len@v9@lot_0.25@dynotears\endcsname{0.6}
\expandafter\def\csname found@v9@lot_0.25@dynotears\endcsname{0.6}
\expandafter\def\csname beyond@v9@lot_0.25@dynotears\endcsname{0.20}
\expandafter\def\csname lift@v9@lot_0.25@varlingam\endcsname{1.8}
\expandafter\def\csname len@v9@lot_0.25@varlingam\endcsname{9.9}
\expandafter\def\csname found@v9@lot_0.25@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v9@lot_0.25@varlingam\endcsname{0.37}
\expandafter\def\csname lift@v9@lot_0.25@doubleml\endcsname{4.5}
\expandafter\def\csname len@v9@lot_0.25@doubleml\endcsname{3.7}
\expandafter\def\csname found@v9@lot_0.25@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v9@lot_0.25@doubleml\endcsname{0.67}
\expandafter\def\csname lift@v9@lot_0.25@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v9@lot_0.25@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v9@lot_0.25@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v9@lot_0.25@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v9@lot_0.5@correlation\endcsname{1.0}
\expandafter\def\csname len@v9@lot_0.5@correlation\endcsname{18.3}
\expandafter\def\csname found@v9@lot_0.5@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v9@lot_0.5@correlation\endcsname{0.03}
\expandafter\def\csname lift@v9@lot_0.5@granger\endcsname{1.1}
\expandafter\def\csname len@v9@lot_0.5@granger\endcsname{16.7}
\expandafter\def\csname found@v9@lot_0.5@granger\endcsname{2.5}
\expandafter\def\csname beyond@v9@lot_0.5@granger\endcsname{0.08}
\expandafter\def\csname lift@v9@lot_0.5@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v9@lot_0.5@pcmciplus\endcsname{2.7}
\expandafter\def\csname found@v9@lot_0.5@pcmciplus\endcsname{2.0}
\expandafter\def\csname beyond@v9@lot_0.5@pcmciplus\endcsname{0.61}
\expandafter\def\csname lift@v9@lot_0.5@pc\endcsname{2.8}
\expandafter\def\csname len@v9@lot_0.5@pc\endcsname{4.7}
\expandafter\def\csname found@v9@lot_0.5@pc\endcsname{1.8}
\expandafter\def\csname beyond@v9@lot_0.5@pc\endcsname{0.43}
\expandafter\def\csname lift@v9@lot_0.5@dynotears\endcsname{7.3}
\expandafter\def\csname len@v9@lot_0.5@dynotears\endcsname{0.4}
\expandafter\def\csname found@v9@lot_0.5@dynotears\endcsname{0.4}
\expandafter\def\csname beyond@v9@lot_0.5@dynotears\endcsname{0.13}
\expandafter\def\csname lift@v9@lot_0.5@varlingam\endcsname{1.7}
\expandafter\def\csname len@v9@lot_0.5@varlingam\endcsname{10.5}
\expandafter\def\csname found@v9@lot_0.5@varlingam\endcsname{2.4}
\expandafter\def\csname beyond@v9@lot_0.5@varlingam\endcsname{0.35}
\expandafter\def\csname lift@v9@lot_0.5@doubleml\endcsname{4.8}
\expandafter\def\csname len@v9@lot_0.5@doubleml\endcsname{3.5}
\expandafter\def\csname found@v9@lot_0.5@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v9@lot_0.5@doubleml\endcsname{0.68}
\expandafter\def\csname lift@v9@lot_0.5@spacetime_rule\endcsname{6.7}
\expandafter\def\csname len@v9@lot_0.5@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v9@lot_0.5@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v9@lot_0.5@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v9@lot_0.75@correlation\endcsname{1.0}
\expandafter\def\csname len@v9@lot_0.75@correlation\endcsname{18.7}
\expandafter\def\csname found@v9@lot_0.75@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v9@lot_0.75@correlation\endcsname{0.02}
\expandafter\def\csname lift@v9@lot_0.75@granger\endcsname{1.1}
\expandafter\def\csname len@v9@lot_0.75@granger\endcsname{16.6}
\expandafter\def\csname found@v9@lot_0.75@granger\endcsname{2.5}
\expandafter\def\csname beyond@v9@lot_0.75@granger\endcsname{0.08}
\expandafter\def\csname lift@v9@lot_0.75@pcmciplus\endcsname{5.4}
\expandafter\def\csname len@v9@lot_0.75@pcmciplus\endcsname{3.0}
\expandafter\def\csname found@v9@lot_0.75@pcmciplus\endcsname{2.2}
\expandafter\def\csname beyond@v9@lot_0.75@pcmciplus\endcsname{0.68}
\expandafter\def\csname lift@v9@lot_0.75@pc\endcsname{2.7}
\expandafter\def\csname len@v9@lot_0.75@pc\endcsname{5.2}
\expandafter\def\csname found@v9@lot_0.75@pc\endcsname{1.9}
\expandafter\def\csname beyond@v9@lot_0.75@pc\endcsname{0.44}
\expandafter\def\csname lift@v9@lot_0.75@dynotears\endcsname{7.3}
\expandafter\def\csname len@v9@lot_0.75@dynotears\endcsname{0.2}
\expandafter\def\csname found@v9@lot_0.75@dynotears\endcsname{0.2}
\expandafter\def\csname beyond@v9@lot_0.75@dynotears\endcsname{0.07}
\expandafter\def\csname lift@v9@lot_0.75@varlingam\endcsname{1.7}
\expandafter\def\csname len@v9@lot_0.75@varlingam\endcsname{9.6}
\expandafter\def\csname found@v9@lot_0.75@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v9@lot_0.75@varlingam\endcsname{0.34}
\expandafter\def\csname lift@v9@lot_0.75@doubleml\endcsname{4.7}
\expandafter\def\csname len@v9@lot_0.75@doubleml\endcsname{3.6}
\expandafter\def\csname found@v9@lot_0.75@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v9@lot_0.75@doubleml\endcsname{0.67}
\expandafter\def\csname lift@v9@lot_0.75@spacetime_rule\endcsname{6.8}
\expandafter\def\csname len@v9@lot_0.75@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v9@lot_0.75@spacetime_rule\endcsname{1.3}
\expandafter\def\csname beyond@v9@lot_0.75@spacetime_rule\endcsname{0.43}
\expandafter\def\csname lift@v9@lot_0.9@correlation\endcsname{1.0}
\expandafter\def\csname len@v9@lot_0.9@correlation\endcsname{18.5}
\expandafter\def\csname found@v9@lot_0.9@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v9@lot_0.9@correlation\endcsname{0.02}
\expandafter\def\csname lift@v9@lot_0.9@granger\endcsname{1.1}
\expandafter\def\csname len@v9@lot_0.9@granger\endcsname{16.8}
\expandafter\def\csname found@v9@lot_0.9@granger\endcsname{2.5}
\expandafter\def\csname beyond@v9@lot_0.9@granger\endcsname{0.07}
\expandafter\def\csname lift@v9@lot_0.9@pcmciplus\endcsname{5.9}
\expandafter\def\csname len@v9@lot_0.9@pcmciplus\endcsname{2.6}
\expandafter\def\csname found@v9@lot_0.9@pcmciplus\endcsname{2.1}
\expandafter\def\csname beyond@v9@lot_0.9@pcmciplus\endcsname{0.66}
\expandafter\def\csname lift@v9@lot_0.9@pc\endcsname{2.7}
\expandafter\def\csname len@v9@lot_0.9@pc\endcsname{5.1}
\expandafter\def\csname found@v9@lot_0.9@pc\endcsname{1.9}
\expandafter\def\csname beyond@v9@lot_0.9@pc\endcsname{0.44}
\expandafter\def\csname lift@v9@lot_0.9@dynotears\endcsname{7.3}
\expandafter\def\csname len@v9@lot_0.9@dynotears\endcsname{0.3}
\expandafter\def\csname found@v9@lot_0.9@dynotears\endcsname{0.3}
\expandafter\def\csname beyond@v9@lot_0.9@dynotears\endcsname{0.10}
\expandafter\def\csname lift@v9@lot_0.9@varlingam\endcsname{1.7}
\expandafter\def\csname len@v9@lot_0.9@varlingam\endcsname{10.8}
\expandafter\def\csname found@v9@lot_0.9@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v9@lot_0.9@varlingam\endcsname{0.36}
\expandafter\def\csname lift@v9@lot_0.9@doubleml\endcsname{4.9}
\expandafter\def\csname len@v9@lot_0.9@doubleml\endcsname{3.4}
\expandafter\def\csname found@v9@lot_0.9@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v9@lot_0.9@doubleml\endcsname{0.68}
\expandafter\def\csname lift@v9@lot_0.9@spacetime_rule\endcsname{6.7}
\expandafter\def\csname len@v9@lot_0.9@spacetime_rule\endcsname{1.2}
\expandafter\def\csname found@v9@lot_0.9@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v9@lot_0.9@spacetime_rule\endcsname{0.36}
\expandafter\def\csname lift@v9@drift_0.1@correlation\endcsname{1.0}
\expandafter\def\csname len@v9@drift_0.1@correlation\endcsname{18.6}
\expandafter\def\csname found@v9@drift_0.1@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v9@drift_0.1@correlation\endcsname{0.02}
\expandafter\def\csname lift@v9@drift_0.1@granger\endcsname{1.0}
\expandafter\def\csname len@v9@drift_0.1@granger\endcsname{17.2}
\expandafter\def\csname found@v9@drift_0.1@granger\endcsname{2.4}
\expandafter\def\csname beyond@v9@drift_0.1@granger\endcsname{0.02}
\expandafter\def\csname lift@v9@drift_0.1@pcmciplus\endcsname{5.6}
\expandafter\def\csname len@v9@drift_0.1@pcmciplus\endcsname{2.6}
\expandafter\def\csname found@v9@drift_0.1@pcmciplus\endcsname{2.0}
\expandafter\def\csname beyond@v9@drift_0.1@pcmciplus\endcsname{0.62}
\expandafter\def\csname lift@v9@drift_0.1@pc\endcsname{2.5}
\expandafter\def\csname len@v9@drift_0.1@pc\endcsname{5.3}
\expandafter\def\csname found@v9@drift_0.1@pc\endcsname{1.8}
\expandafter\def\csname beyond@v9@drift_0.1@pc\endcsname{0.39}
\expandafter\def\csname lift@v9@drift_0.1@dynotears\endcsname{7.3}
\expandafter\def\csname len@v9@drift_0.1@dynotears\endcsname{0.7}
\expandafter\def\csname found@v9@drift_0.1@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v9@drift_0.1@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v9@drift_0.1@varlingam\endcsname{1.8}
\expandafter\def\csname len@v9@drift_0.1@varlingam\endcsname{10.1}
\expandafter\def\csname found@v9@drift_0.1@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v9@drift_0.1@varlingam\endcsname{0.40}
\expandafter\def\csname lift@v9@drift_0.1@doubleml\endcsname{4.6}
\expandafter\def\csname len@v9@drift_0.1@doubleml\endcsname{3.8}
\expandafter\def\csname found@v9@drift_0.1@doubleml\endcsname{2.4}
\expandafter\def\csname beyond@v9@drift_0.1@doubleml\endcsname{0.68}
\expandafter\def\csname lift@v9@drift_0.1@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v9@drift_0.1@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v9@drift_0.1@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v9@drift_0.1@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v9@drift_0.3@correlation\endcsname{1.0}
\expandafter\def\csname len@v9@drift_0.3@correlation\endcsname{18.2}
\expandafter\def\csname found@v9@drift_0.3@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v9@drift_0.3@correlation\endcsname{0.03}
\expandafter\def\csname lift@v9@drift_0.3@granger\endcsname{1.0}
\expandafter\def\csname len@v9@drift_0.3@granger\endcsname{17.6}
\expandafter\def\csname found@v9@drift_0.3@granger\endcsname{2.5}
\expandafter\def\csname beyond@v9@drift_0.3@granger\endcsname{0.03}
\expandafter\def\csname lift@v9@drift_0.3@pcmciplus\endcsname{5.0}
\expandafter\def\csname len@v9@drift_0.3@pcmciplus\endcsname{2.8}
\expandafter\def\csname found@v9@drift_0.3@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v9@drift_0.3@pcmciplus\endcsname{0.57}
\expandafter\def\csname lift@v9@drift_0.3@pc\endcsname{2.6}
\expandafter\def\csname len@v9@drift_0.3@pc\endcsname{5.3}
\expandafter\def\csname found@v9@drift_0.3@pc\endcsname{1.9}
\expandafter\def\csname beyond@v9@drift_0.3@pc\endcsname{0.43}
\expandafter\def\csname lift@v9@drift_0.3@dynotears\endcsname{7.3}
\expandafter\def\csname len@v9@drift_0.3@dynotears\endcsname{0.7}
\expandafter\def\csname found@v9@drift_0.3@dynotears\endcsname{0.7}
\expandafter\def\csname beyond@v9@drift_0.3@dynotears\endcsname{0.23}
\expandafter\def\csname lift@v9@drift_0.3@varlingam\endcsname{1.8}
\expandafter\def\csname len@v9@drift_0.3@varlingam\endcsname{10.0}
\expandafter\def\csname found@v9@drift_0.3@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v9@drift_0.3@varlingam\endcsname{0.41}
\expandafter\def\csname lift@v9@drift_0.3@doubleml\endcsname{4.6}
\expandafter\def\csname len@v9@drift_0.3@doubleml\endcsname{3.8}
\expandafter\def\csname found@v9@drift_0.3@doubleml\endcsname{2.4}
\expandafter\def\csname beyond@v9@drift_0.3@doubleml\endcsname{0.69}
\expandafter\def\csname lift@v9@drift_0.3@spacetime_rule\endcsname{6.2}
\expandafter\def\csname len@v9@drift_0.3@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v9@drift_0.3@spacetime_rule\endcsname{1.1}
\expandafter\def\csname beyond@v9@drift_0.3@spacetime_rule\endcsname{0.36}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2@correlation\endcsname{1.0}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2@correlation\endcsname{18.3}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2@correlation\endcsname{0.03}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2@granger\endcsname{1.1}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2@granger\endcsname{16.9}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2@granger\endcsname{2.5}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2@granger\endcsname{0.07}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2@pcmciplus\endcsname{5.0}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2@pcmciplus\endcsname{2.9}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2@pcmciplus\endcsname{2.0}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2@pcmciplus\endcsname{0.61}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2@pc\endcsname{2.8}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2@pc\endcsname{5.0}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2@pc\endcsname{1.9}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2@pc\endcsname{0.45}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2@dynotears\endcsname{7.3}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2@dynotears\endcsname{0.5}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2@dynotears\endcsname{0.5}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2@dynotears\endcsname{0.17}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2@varlingam\endcsname{1.8}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2@varlingam\endcsname{10.2}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2@varlingam\endcsname{2.5}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2@varlingam\endcsname{0.40}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2@doubleml\endcsname{5.3}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2@doubleml\endcsname{3.2}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2@doubleml\endcsname{2.3}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2@doubleml\endcsname{0.70}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2@spacetime_rule\endcsname{6.3}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2@spacetime_rule\endcsname{1.4}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2@spacetime_rule\endcsname{1.2}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2@spacetime_rule\endcsname{0.39}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_combo_interaction@correlation\endcsname{0.7}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_combo_interaction@correlation\endcsname{5.2}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_combo_interaction@correlation\endcsname{0.5}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_combo_interaction@correlation\endcsname{-0.05}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_combo_interaction@granger\endcsname{1.4}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_combo_interaction@granger\endcsname{4.1}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_combo_interaction@granger\endcsname{0.8}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_combo_interaction@granger\endcsname{0.16}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus\endcsname{4.6}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus\endcsname{0.8}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus\endcsname{0.5}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_combo_interaction@pcmciplus\endcsname{0.15}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_combo_interaction@pc\endcsname{0.6}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_combo_interaction@pc\endcsname{2.4}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_combo_interaction@pc\endcsname{0.2}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_combo_interaction@pc\endcsname{-0.05}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_combo_interaction@dynotears\endcsname{--}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_combo_interaction@dynotears\endcsname{0.0}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_combo_interaction@dynotears\endcsname{0.00}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_combo_interaction@varlingam\endcsname{1.4}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_combo_interaction@varlingam\endcsname{4.8}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_combo_interaction@varlingam\endcsname{0.9}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_combo_interaction@varlingam\endcsname{0.10}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_combo_interaction@doubleml\endcsname{2.4}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_combo_interaction@doubleml\endcsname{0.3}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_combo_interaction@doubleml\endcsname{0.1}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_combo_interaction@doubleml\endcsname{0.03}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule\endcsname{3.9}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule\endcsname{1.3}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule\endcsname{0.7}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_combo_interaction@spacetime_rule\endcsname{0.20}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_s40@correlation\endcsname{1.1}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_s40@correlation\endcsname{37.1}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_s40@correlation\endcsname{2.6}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_s40@correlation\endcsname{0.05}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_s40@granger\endcsname{1.1}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_s40@granger\endcsname{34.9}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_s40@granger\endcsname{2.6}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_s40@granger\endcsname{0.11}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_s40@pcmciplus\endcsname{13.6}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_s40@pcmciplus\endcsname{2.1}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_s40@pcmciplus\endcsname{1.9}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_s40@pcmciplus\endcsname{0.67}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_s40@pc\endcsname{4.8}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_s40@pc\endcsname{5.0}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_s40@pc\endcsname{1.6}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_s40@pc\endcsname{0.49}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_s40@dynotears\endcsname{15.0}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_s40@dynotears\endcsname{0.4}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_s40@dynotears\endcsname{0.4}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_s40@dynotears\endcsname{0.14}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_s40@varlingam\endcsname{3.3}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_s40@varlingam\endcsname{10.0}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_s40@varlingam\endcsname{2.2}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_s40@varlingam\endcsname{0.58}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_s40@doubleml\endcsname{10.6}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_s40@doubleml\endcsname{2.4}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_s40@doubleml\endcsname{1.7}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_s40@doubleml\endcsname{0.58}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_s40@spacetime_rule\endcsname{12.0}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_s40@spacetime_rule\endcsname{1.0}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_s40@spacetime_rule\endcsname{0.8}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_s40@spacetime_rule\endcsname{0.28}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_b50@correlation\endcsname{1.1}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_b50@correlation\endcsname{17.0}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_b50@correlation\endcsname{2.5}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_b50@correlation\endcsname{0.07}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_b50@granger\endcsname{1.5}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_b50@granger\endcsname{11.6}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_b50@granger\endcsname{2.4}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_b50@granger\endcsname{0.32}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_b50@pcmciplus\endcsname{6.9}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_b50@pcmciplus\endcsname{1.8}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_b50@pcmciplus\endcsname{1.7}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_b50@pcmciplus\endcsname{0.56}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_b50@pc\endcsname{2.8}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_b50@pc\endcsname{4.7}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_b50@pc\endcsname{1.8}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_b50@pc\endcsname{0.43}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_b50@dynotears\endcsname{7.3}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_b50@dynotears\endcsname{0.5}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_b50@dynotears\endcsname{0.5}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_b50@dynotears\endcsname{0.16}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_b50@varlingam\endcsname{2.5}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_b50@varlingam\endcsname{5.8}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_b50@varlingam\endcsname{2.0}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_b50@varlingam\endcsname{0.46}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_b50@doubleml\endcsname{5.2}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_b50@doubleml\endcsname{1.7}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_b50@doubleml\endcsname{1.2}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_b50@doubleml\endcsname{0.36}
\expandafter\def\csname lift@v9@lot_0.5_drift_0.2_b50@spacetime_rule\endcsname{5.1}
\expandafter\def\csname len@v9@lot_0.5_drift_0.2_b50@spacetime_rule\endcsname{1.0}
\expandafter\def\csname found@v9@lot_0.5_drift_0.2_b50@spacetime_rule\endcsname{0.7}
\expandafter\def\csname beyond@v9@lot_0.5_drift_0.2_b50@spacetime_rule\endcsname{0.22}
\makeatother


==> generated/numbers_overall.tex <==
\makeatletter
\newcommand{\Ovr}[2]{\ifcsname ovr@#1@#2\endcsname\csname ovr@#1@#2\endcsname\else\PackageError{numbers}{missing Ovr #1/#2}{}\fi}
\expandafter\def\csname ovr@correlation@first\endcsname{64\%}
\expandafter\def\csname ovr@correlation@rp\endcsname{0.47}
\expandafter\def\csname ovr@correlation@ap\endcsname{0.61}
\expandafter\def\csname ovr@correlation@len\endcsname{16.9}
\expandafter\def\csname ovr@correlation@found\endcsname{87\%}
\expandafter\def\csname ovr@correlation@prec\endcsname{0.15}
\expandafter\def\csname ovr@correlation@lift\endcsname{1.1}
\expandafter\def\csname ovr@correlation@f1\endcsname{0.24}
\expandafter\def\csname ovr@correlation@none\endcsname{0\%}
\expandafter\def\csname ovr@correlation@mrr\endcsname{0.76}
\expandafter\def\csname ovr@correlation@ndcg\endcsname{0.57}
\expandafter\def\csname ovr@correlation@ndcgg\endcsname{0.57}
\expandafter\def\csname ovr@granger@first\endcsname{79\%}
\expandafter\def\csname ovr@granger@rp\endcsname{0.59}
\expandafter\def\csname ovr@granger@ap\endcsname{0.69}
\expandafter\def\csname ovr@granger@len\endcsname{13.7}
\expandafter\def\csname ovr@granger@found\endcsname{79\%}
\expandafter\def\csname ovr@granger@prec\endcsname{0.21}
\expandafter\def\csname ovr@granger@lift\endcsname{1.7}
\expandafter\def\csname ovr@granger@f1\endcsname{0.27}
\expandafter\def\csname ovr@granger@none\endcsname{10\%}
\expandafter\def\csname ovr@granger@mrr\endcsname{0.88}
\expandafter\def\csname ovr@granger@ndcg\endcsname{0.67}
\expandafter\def\csname ovr@granger@ndcgg\endcsname{0.74}
\expandafter\def\csname ovr@varlingam@first\endcsname{66\%}
\expandafter\def\csname ovr@varlingam@rp\endcsname{0.53}
\expandafter\def\csname ovr@varlingam@ap\endcsname{0.63}
\expandafter\def\csname ovr@varlingam@len\endcsname{7.6}
\expandafter\def\csname ovr@varlingam@found\endcsname{73\%}
\expandafter\def\csname ovr@varlingam@prec\endcsname{0.30}
\expandafter\def\csname ovr@varlingam@lift\endcsname{2.3}
\expandafter\def\csname ovr@varlingam@f1\endcsname{0.37}
\expandafter\def\csname ovr@varlingam@none\endcsname{5\%}
\expandafter\def\csname ovr@varlingam@mrr\endcsname{0.77}
\expandafter\def\csname ovr@varlingam@ndcg\endcsname{0.60}
\expandafter\def\csname ovr@varlingam@ndcgg\endcsname{0.62}
\expandafter\def\csname ovr@dynotears@first\endcsname{28\%}
\expandafter\def\csname ovr@dynotears@rp\endcsname{0.75}
\expandafter\def\csname ovr@dynotears@ap\endcsname{0.82}
\expandafter\def\csname ovr@dynotears@len\endcsname{0.4}
\expandafter\def\csname ovr@dynotears@found\endcsname{14\%}
\expandafter\def\csname ovr@dynotears@prec\endcsname{1.00}
\expandafter\def\csname ovr@dynotears@lift\endcsname{7.3}
\expandafter\def\csname ovr@dynotears@f1\endcsname{0.18}
\expandafter\def\csname ovr@dynotears@none\endcsname{72\%}
\expandafter\def\csname ovr@dynotears@mrr\endcsname{0.92}
\expandafter\def\csname ovr@dynotears@ndcg\endcsname{0.82}
\expandafter\def\csname ovr@dynotears@ndcgg\endcsname{0.82}
\expandafter\def\csname ovr@pc@first\endcsname{25\%}
\expandafter\def\csname ovr@pc@rp\endcsname{0.29}
\expandafter\def\csname ovr@pc@ap\endcsname{0.27}
\expandafter\def\csname ovr@pc@len\endcsname{4.5}
\expandafter\def\csname ovr@pc@found\endcsname{56\%}
\expandafter\def\csname ovr@pc@prec\endcsname{0.30}
\expandafter\def\csname ovr@pc@lift\endcsname{2.3}
\expandafter\def\csname ovr@pc@f1\endcsname{0.37}
\expandafter\def\csname ovr@pc@none\endcsname{0\%}
\expandafter\def\csname ovr@pc@mrr\endcsname{0.53}
\expandafter\def\csname ovr@pc@ndcg\endcsname{0.35}
\expandafter\def\csname ovr@pc@ndcgg\endcsname{0.38}
\expandafter\def\csname ovr@pcmciplus@first\endcsname{78\%}
\expandafter\def\csname ovr@pcmciplus@rp\endcsname{0.74}
\expandafter\def\csname ovr@pcmciplus@ap\endcsname{0.81}
\expandafter\def\csname ovr@pcmciplus@len\endcsname{2.4}
\expandafter\def\csname ovr@pcmciplus@found\endcsname{62\%}
\expandafter\def\csname ovr@pcmciplus@prec\endcsname{0.69}
\expandafter\def\csname ovr@pcmciplus@lift\endcsname{5.3}
\expandafter\def\csname ovr@pcmciplus@f1\endcsname{0.58}
\expandafter\def\csname ovr@pcmciplus@none\endcsname{10\%}
\expandafter\def\csname ovr@pcmciplus@mrr\endcsname{0.91}
\expandafter\def\csname ovr@pcmciplus@ndcg\endcsname{0.81}
\expandafter\def\csname ovr@pcmciplus@ndcgg\endcsname{0.82}
\expandafter\def\csname ovr@spacetime_rule@first\endcsname{63\%}
\expandafter\def\csname ovr@spacetime_rule@rp\endcsname{0.50}
\expandafter\def\csname ovr@spacetime_rule@ap\endcsname{0.61}
\expandafter\def\csname ovr@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname ovr@spacetime_rule@found\endcsname{36\%}
\expandafter\def\csname ovr@spacetime_rule@prec\endcsname{0.74}
\expandafter\def\csname ovr@spacetime_rule@lift\endcsname{5.9}
\expandafter\def\csname ovr@spacetime_rule@f1\endcsname{0.42}
\expandafter\def\csname ovr@spacetime_rule@none\endcsname{16\%}
\expandafter\def\csname ovr@spacetime_rule@mrr\endcsname{0.80}
\expandafter\def\csname ovr@spacetime_rule@ndcg\endcsname{0.61}
\expandafter\def\csname ovr@spacetime_rule@ndcgg\endcsname{0.67}
\expandafter\def\csname ovr@doubleml@first\endcsname{67\%}
\expandafter\def\csname ovr@doubleml@rp\endcsname{0.63}
\expandafter\def\csname ovr@doubleml@ap\endcsname{0.71}
\expandafter\def\csname ovr@doubleml@len\endcsname{2.2}
\expandafter\def\csname ovr@doubleml@found\endcsname{56\%}
\expandafter\def\csname ovr@doubleml@prec\endcsname{0.72}
\expandafter\def\csname ovr@doubleml@lift\endcsname{5.5}
\expandafter\def\csname ovr@doubleml@f1\endcsname{0.51}
\expandafter\def\csname ovr@doubleml@none\endcsname{27\%}
\expandafter\def\csname ovr@doubleml@mrr\endcsname{0.82}
\expandafter\def\csname ovr@doubleml@ndcg\endcsname{0.68}
\expandafter\def\csname ovr@doubleml@ndcgg\endcsname{0.73}
\expandafter\def\csname ovr@random@first\endcsname{0.13}
\expandafter\def\csname ovr@random@rp\endcsname{0.13}
\expandafter\def\csname ovr@random@prec\endcsname{0.13}
\expandafter\def\csname ovr@random@lift\endcsname{1.0}
\expandafter\def\csname ovr@random@ap\endcsname{0.24}
\expandafter\def\csname ovr@random@mrr\endcsname{0.31}
\expandafter\def\csname ovr@random@ndcg\endcsname{0.15}
\newcommand{\OvrPlants}{1,190}
\newcommand{\OvrC}[2]{\ifcsname ovrc@#1@#2\endcsname\csname ovrc@#1@#2\endcsname\else\PackageError{numbers}{missing OvrC #1/#2}{}\fi}
\expandafter\def\csname ovrc@correlation@first\endcsname{16\%}
\expandafter\def\csname ovrc@correlation@rp\endcsname{0.14}
\expandafter\def\csname ovrc@correlation@ap\endcsname{0.34}
\expandafter\def\csname ovrc@correlation@len\endcsname{11.3}
\expandafter\def\csname ovrc@correlation@found\endcsname{60\%}
\expandafter\def\csname ovrc@correlation@prec\endcsname{0.13}
\expandafter\def\csname ovrc@correlation@lift\endcsname{1.1}
\expandafter\def\csname ovrc@correlation@f1\endcsname{0.20}
\expandafter\def\csname ovrc@correlation@none\endcsname{0\%}
\expandafter\def\csname ovrc@correlation@mrr\endcsname{0.40}
\expandafter\def\csname ovrc@correlation@ndcg\endcsname{0.26}
\expandafter\def\csname ovrc@correlation@ndcgg\endcsname{0.26}
\expandafter\def\csname ovrc@granger@first\endcsname{48\%}
\expandafter\def\csname ovrc@granger@rp\endcsname{0.46}
\expandafter\def\csname ovrc@granger@ap\endcsname{0.56}
\expandafter\def\csname ovrc@granger@len\endcsname{7.4}
\expandafter\def\csname ovrc@granger@found\endcsname{51\%}
\expandafter\def\csname ovrc@granger@prec\endcsname{0.27}
\expandafter\def\csname ovrc@granger@lift\endcsname{2.3}
\expandafter\def\csname ovrc@granger@f1\endcsname{0.22}
\expandafter\def\csname ovrc@granger@none\endcsname{31\%}
\expandafter\def\csname ovrc@granger@mrr\endcsname{0.72}
\expandafter\def\csname ovrc@granger@ndcg\endcsname{0.52}
\expandafter\def\csname ovrc@granger@ndcgg\endcsname{0.60}
\expandafter\def\csname ovrc@varlingam@first\endcsname{12\%}
\expandafter\def\csname ovrc@varlingam@rp\endcsname{0.20}
\expandafter\def\csname ovrc@varlingam@ap\endcsname{0.29}
\expandafter\def\csname ovrc@varlingam@len\endcsname{5.2}
\expandafter\def\csname ovrc@varlingam@found\endcsname{40\%}
\expandafter\def\csname ovrc@varlingam@prec\endcsname{0.19}
\expandafter\def\csname ovrc@varlingam@lift\endcsname{1.5}
\expandafter\def\csname ovrc@varlingam@f1\endcsname{0.22}
\expandafter\def\csname ovrc@varlingam@none\endcsname{10\%}
\expandafter\def\csname ovrc@varlingam@mrr\endcsname{0.37}
\expandafter\def\csname ovrc@varlingam@ndcg\endcsname{0.23}
\expandafter\def\csname ovrc@varlingam@ndcgg\endcsname{0.28}
\expandafter\def\csname ovrc@dynotears@first\endcsname{1\%}
\expandafter\def\csname ovrc@dynotears@rp\endcsname{0.54}
\expandafter\def\csname ovrc@dynotears@ap\endcsname{0.63}
\expandafter\def\csname ovrc@dynotears@len\endcsname{0.0}
\expandafter\def\csname ovrc@dynotears@found\endcsname{1\%}
\expandafter\def\csname ovrc@dynotears@prec\endcsname{0.67}
\expandafter\def\csname ovrc@dynotears@lift\endcsname{7.6}
\expandafter\def\csname ovrc@dynotears@f1\endcsname{0.01}
\expandafter\def\csname ovrc@dynotears@none\endcsname{99\%}
\expandafter\def\csname ovrc@dynotears@mrr\endcsname{0.72}
\expandafter\def\csname ovrc@dynotears@ndcg\endcsname{0.55}
\expandafter\def\csname ovrc@dynotears@ndcgg\endcsname{0.58}
\expandafter\def\csname ovrc@pc@first\endcsname{13\%}
\expandafter\def\csname ovrc@pc@rp\endcsname{0.18}
\expandafter\def\csname ovrc@pc@ap\endcsname{0.20}
\expandafter\def\csname ovrc@pc@len\endcsname{2.7}
\expandafter\def\csname ovrc@pc@found\endcsname{24\%}
\expandafter\def\csname ovrc@pc@prec\endcsname{0.18}
\expandafter\def\csname ovrc@pc@lift\endcsname{1.4}
\expandafter\def\csname ovrc@pc@f1\endcsname{0.19}
\expandafter\def\csname ovrc@pc@none\endcsname{0\%}
\expandafter\def\csname ovrc@pc@mrr\endcsname{0.38}
\expandafter\def\csname ovrc@pc@ndcg\endcsname{0.22}
\expandafter\def\csname ovrc@pc@ndcgg\endcsname{0.25}
\expandafter\def\csname ovrc@pcmciplus@first\endcsname{41\%}
\expandafter\def\csname ovrc@pcmciplus@rp\endcsname{0.45}
\expandafter\def\csname ovrc@pcmciplus@ap\endcsname{0.57}
\expandafter\def\csname ovrc@pcmciplus@len\endcsname{1.2}
\expandafter\def\csname ovrc@pcmciplus@found\endcsname{28\%}
\expandafter\def\csname ovrc@pcmciplus@prec\endcsname{0.52}
\expandafter\def\csname ovrc@pcmciplus@lift\endcsname{4.1}
\expandafter\def\csname ovrc@pcmciplus@f1\endcsname{0.28}
\expandafter\def\csname ovrc@pcmciplus@none\endcsname{31\%}
\expandafter\def\csname ovrc@pcmciplus@mrr\endcsname{0.72}
\expandafter\def\csname ovrc@pcmciplus@ndcg\endcsname{0.54}
\expandafter\def\csname ovrc@pcmciplus@ndcgg\endcsname{0.59}
\expandafter\def\csname ovrc@spacetime_rule@first\endcsname{41\%}
\expandafter\def\csname ovrc@spacetime_rule@rp\endcsname{0.30}
\expandafter\def\csname ovrc@spacetime_rule@ap\endcsname{0.43}
\expandafter\def\csname ovrc@spacetime_rule@len\endcsname{1.1}
\expandafter\def\csname ovrc@spacetime_rule@found\endcsname{22\%}
\expandafter\def\csname ovrc@spacetime_rule@prec\endcsname{0.45}
\expandafter\def\csname ovrc@spacetime_rule@lift\endcsname{3.6}
\expandafter\def\csname ovrc@spacetime_rule@f1\endcsname{0.26}
\expandafter\def\csname ovrc@spacetime_rule@none\endcsname{13\%}
\expandafter\def\csname ovrc@spacetime_rule@mrr\endcsname{0.65}
\expandafter\def\csname ovrc@spacetime_rule@ndcg\endcsname{0.40}
\expandafter\def\csname ovrc@spacetime_rule@ndcgg\endcsname{0.54}
\expandafter\def\csname ovrc@doubleml@first\endcsname{19\%}
\expandafter\def\csname ovrc@doubleml@rp\endcsname{0.30}
\expandafter\def\csname ovrc@doubleml@ap\endcsname{0.41}
\expandafter\def\csname ovrc@doubleml@len\endcsname{0.5}
\expandafter\def\csname ovrc@doubleml@found\endcsname{14\%}
\expandafter\def\csname ovrc@doubleml@prec\endcsname{0.49}
\expandafter\def\csname ovrc@doubleml@lift\endcsname{4.4}
\expandafter\def\csname ovrc@doubleml@f1\endcsname{0.14}
\expandafter\def\csname ovrc@doubleml@none\endcsname{67\%}
\expandafter\def\csname ovrc@doubleml@mrr\endcsname{0.51}
\expandafter\def\csname ovrc@doubleml@ndcg\endcsname{0.34}
\expandafter\def\csname ovrc@doubleml@ndcgg\endcsname{0.45}
\expandafter\def\csname ovrc@random@first\endcsname{0.13}
\expandafter\def\csname ovrc@random@rp\endcsname{0.13}
\expandafter\def\csname ovrc@random@prec\endcsname{0.13}
\expandafter\def\csname ovrc@random@lift\endcsname{1.0}
\expandafter\def\csname ovrc@random@ap\endcsname{0.25}
\expandafter\def\csname ovrc@random@mrr\endcsname{0.31}
\expandafter\def\csname ovrc@random@ndcg\endcsname{0.14}
\newcommand{\OvrCPlants}{230}
\makeatother


==> generated/numbers_selection.tex <==
\makeatletter
\newcommand{\Sel}[3]{\ifcsname sel@#1@#2@#3\endcsname\csname sel@#1@#2@#3\endcsname\else\PackageError{numbers}{missing selection #1/#2/#3}{}\fi}
\expandafter\def\csname sel@correlation@0@len\endcsname{16.9}
\expandafter\def\csname sel@correlation@0@prec\endcsname{0.15}
\expandafter\def\csname sel@correlation@0@lift\endcsname{1.1}
\expandafter\def\csname sel@correlation@0@f1\endcsname{0.24}
\expandafter\def\csname sel@correlation@0@first\endcsname{64\%}
\expandafter\def\csname sel@correlation@0@none\endcsname{0\%}
\expandafter\def\csname sel@correlation@1@len\endcsname{13.2}
\expandafter\def\csname sel@correlation@1@prec\endcsname{0.17}
\expandafter\def\csname sel@correlation@1@lift\endcsname{1.3}
\expandafter\def\csname sel@correlation@1@f1\endcsname{0.26}
\expandafter\def\csname sel@correlation@1@first\endcsname{64\%}
\expandafter\def\csname sel@correlation@1@none\endcsname{2\%}
\expandafter\def\csname sel@correlation@2@len\endcsname{9.6}
\expandafter\def\csname sel@correlation@2@prec\endcsname{0.22}
\expandafter\def\csname sel@correlation@2@lift\endcsname{1.7}
\expandafter\def\csname sel@correlation@2@f1\endcsname{0.28}
\expandafter\def\csname sel@correlation@2@first\endcsname{63\%}
\expandafter\def\csname sel@correlation@2@none\endcsname{6\%}
\expandafter\def\csname sel@correlation@3@len\endcsname{7.1}
\expandafter\def\csname sel@correlation@3@prec\endcsname{0.26}
\expandafter\def\csname sel@correlation@3@lift\endcsname{2.0}
\expandafter\def\csname sel@correlation@3@f1\endcsname{0.30}
\expandafter\def\csname sel@correlation@3@first\endcsname{61\%}
\expandafter\def\csname sel@correlation@3@none\endcsname{11\%}
\expandafter\def\csname sel@correlation@4@len\endcsname{14.2}
\expandafter\def\csname sel@correlation@4@prec\endcsname{0.16}
\expandafter\def\csname sel@correlation@4@lift\endcsname{1.3}
\expandafter\def\csname sel@correlation@4@f1\endcsname{0.26}
\expandafter\def\csname sel@correlation@4@first\endcsname{64\%}
\expandafter\def\csname sel@correlation@4@none\endcsname{0\%}
\expandafter\def\csname sel@correlation@5@len\endcsname{3.0}
\expandafter\def\csname sel@correlation@5@prec\endcsname{0.42}
\expandafter\def\csname sel@correlation@5@lift\endcsname{3.3}
\expandafter\def\csname sel@correlation@5@f1\endcsname{0.46}
\expandafter\def\csname sel@correlation@5@first\endcsname{64\%}
\expandafter\def\csname sel@correlation@5@none\endcsname{0\%}
\expandafter\def\csname sel@granger@0@len\endcsname{13.7}
\expandafter\def\csname sel@granger@0@prec\endcsname{0.21}
\expandafter\def\csname sel@granger@0@lift\endcsname{1.7}
\expandafter\def\csname sel@granger@0@f1\endcsname{0.27}
\expandafter\def\csname sel@granger@0@first\endcsname{79\%}
\expandafter\def\csname sel@granger@0@none\endcsname{10\%}
\expandafter\def\csname sel@granger@1@len\endcsname{9.9}
\expandafter\def\csname sel@granger@1@prec\endcsname{0.29}
\expandafter\def\csname sel@granger@1@lift\endcsname{2.3}
\expandafter\def\csname sel@granger@1@f1\endcsname{0.30}
\expandafter\def\csname sel@granger@1@first\endcsname{74\%}
\expandafter\def\csname sel@granger@1@none\endcsname{18\%}
\expandafter\def\csname sel@granger@2@len\endcsname{6.3}
\expandafter\def\csname sel@granger@2@prec\endcsname{0.38}
\expandafter\def\csname sel@granger@2@lift\endcsname{3.0}
\expandafter\def\csname sel@granger@2@f1\endcsname{0.32}
\expandafter\def\csname sel@granger@2@first\endcsname{67\%}
\expandafter\def\csname sel@granger@2@none\endcsname{27\%}
\expandafter\def\csname sel@granger@3@len\endcsname{4.0}
\expandafter\def\csname sel@granger@3@prec\endcsname{0.49}
\expandafter\def\csname sel@granger@3@lift\endcsname{3.9}
\expandafter\def\csname sel@granger@3@f1\endcsname{0.33}
\expandafter\def\csname sel@granger@3@first\endcsname{61\%}
\expandafter\def\csname sel@granger@3@none\endcsname{34\%}
\expandafter\def\csname sel@granger@4@len\endcsname{11.0}
\expandafter\def\csname sel@granger@4@prec\endcsname{0.26}
\expandafter\def\csname sel@granger@4@lift\endcsname{2.0}
\expandafter\def\csname sel@granger@4@f1\endcsname{0.30}
\expandafter\def\csname sel@granger@4@first\endcsname{79\%}
\expandafter\def\csname sel@granger@4@none\endcsname{10\%}
\expandafter\def\csname sel@granger@5@len\endcsname{3.0}
\expandafter\def\csname sel@granger@5@prec\endcsname{0.49}
\expandafter\def\csname sel@granger@5@lift\endcsname{3.8}
\expandafter\def\csname sel@granger@5@f1\endcsname{0.52}
\expandafter\def\csname sel@granger@5@first\endcsname{82\%}
\expandafter\def\csname sel@granger@5@none\endcsname{0\%}
\expandafter\def\csname sel@dynotears@0@len\endcsname{0.3}
\expandafter\def\csname sel@dynotears@0@prec\endcsname{1.00}
\expandafter\def\csname sel@dynotears@0@lift\endcsname{7.3}
\expandafter\def\csname sel@dynotears@0@f1\endcsname{0.18}
\expandafter\def\csname sel@dynotears@0@first\endcsname{28\%}
\expandafter\def\csname sel@dynotears@0@none\endcsname{71\%}
\expandafter\def\csname sel@dynotears@1@len\endcsname{1.5}
\expandafter\def\csname sel@dynotears@1@prec\endcsname{0.89}
\expandafter\def\csname sel@dynotears@1@lift\endcsname{6.9}
\expandafter\def\csname sel@dynotears@1@f1\endcsname{0.56}
\expandafter\def\csname sel@dynotears@1@first\endcsname{71\%}
\expandafter\def\csname sel@dynotears@1@none\endcsname{25\%}
\expandafter\def\csname sel@dynotears@2@len\endcsname{2.8}
\expandafter\def\csname sel@dynotears@2@prec\endcsname{0.73}
\expandafter\def\csname sel@dynotears@2@lift\endcsname{5.7}
\expandafter\def\csname sel@dynotears@2@f1\endcsname{0.66}
\expandafter\def\csname sel@dynotears@2@first\endcsname{85\%}
\expandafter\def\csname sel@dynotears@2@none\endcsname{8\%}
\expandafter\def\csname sel@dynotears@3@len\endcsname{3.2}
\expandafter\def\csname sel@dynotears@3@prec\endcsname{0.68}
\expandafter\def\csname sel@dynotears@3@lift\endcsname{5.3}
\expandafter\def\csname sel@dynotears@3@f1\endcsname{0.67}
\expandafter\def\csname sel@dynotears@3@first\endcsname{87\%}
\expandafter\def\csname sel@dynotears@3@none\endcsname{5\%}
\expandafter\def\csname sel@pcmciplus@0@len\endcsname{4.0}
\expandafter\def\csname sel@pcmciplus@0@prec\endcsname{0.48}
\expandafter\def\csname sel@pcmciplus@0@lift\endcsname{3.8}
\expandafter\def\csname sel@pcmciplus@0@f1\endcsname{0.53}
\expandafter\def\csname sel@pcmciplus@0@first\endcsname{82\%}
\expandafter\def\csname sel@pcmciplus@0@none\endcsname{2\%}
\expandafter\def\csname sel@pcmciplus@1@len\endcsname{2.4}
\expandafter\def\csname sel@pcmciplus@1@prec\endcsname{0.69}
\expandafter\def\csname sel@pcmciplus@1@lift\endcsname{5.3}
\expandafter\def\csname sel@pcmciplus@1@f1\endcsname{0.58}
\expandafter\def\csname sel@pcmciplus@1@first\endcsname{78\%}
\expandafter\def\csname sel@pcmciplus@1@none\endcsname{10\%}
\expandafter\def\csname sel@pcmciplus@2@len\endcsname{1.8}
\expandafter\def\csname sel@pcmciplus@2@prec\endcsname{0.80}
\expandafter\def\csname sel@pcmciplus@2@lift\endcsname{6.1}
\expandafter\def\csname sel@pcmciplus@2@f1\endcsname{0.56}
\expandafter\def\csname sel@pcmciplus@2@first\endcsname{73\%}
\expandafter\def\csname sel@pcmciplus@2@none\endcsname{20\%}
\expandafter\def\csname sel@pcmciplus@3@len\endcsname{1.4}
\expandafter\def\csname sel@pcmciplus@3@prec\endcsname{0.89}
\expandafter\def\csname sel@pcmciplus@3@lift\endcsname{6.8}
\expandafter\def\csname sel@pcmciplus@3@f1\endcsname{0.52}
\expandafter\def\csname sel@pcmciplus@3@first\endcsname{66\%}
\expandafter\def\csname sel@pcmciplus@3@none\endcsname{30\%}
\makeatother


==> generated/numbers_separability.tex <==
\newcommand{\SepAll}{9\%}
\newcommand{\SepAllSep}{91\%}
\newcommand{\SepAgg}{7\%}
\newcommand{\SepFine}{2\%}
\newcommand{\SepN}{23,467}
\makeatletter
\newcommand{\SepM}[2]{\ifcsname sepm@#1@#2\endcsname\csname sepm@#1@#2\endcsname\else\PackageError{numbers}{missing separability #1/#2}{}\fi}
\expandafter\def\csname sepm@role@downstream\endcsname{14\%}
\expandafter\def\csname sepm@role@downstream_sep\endcsname{86\%}
\expandafter\def\csname sepm@role@upstream_loop\endcsname{23\%}
\expandafter\def\csname sepm@role@upstream_loop_sep\endcsname{77\%}
\expandafter\def\csname sepm@role@upstream\endcsname{9\%}
\expandafter\def\csname sepm@role@upstream_sep\endcsname{91\%}
\expandafter\def\csname sepm@role@look_alike\endcsname{7\%}
\expandafter\def\csname sepm@role@look_alike_sep\endcsname{93\%}
\expandafter\def\csname sepm@correlation@nonsep\endcsname{11\%}
\expandafter\def\csname sepm@correlation@agg\endcsname{8\%}
\expandafter\def\csname sepm@correlation@fine\endcsname{3\%}
\expandafter\def\csname sepm@correlation@list\endcsname{10\%}
\expandafter\def\csname sepm@correlation@first\endcsname{0.64}
\expandafter\def\csname sepm@correlation@prec\endcsname{0.15}
\expandafter\def\csname sepm@correlation@lift\endcsname{1.1}
\expandafter\def\csname sepm@correlation@firstr\endcsname{0.69}
\expandafter\def\csname sepm@correlation@precr\endcsname{0.16}
\expandafter\def\csname sepm@correlation@liftr\endcsname{1.2}
\expandafter\def\csname sepm@granger@nonsep\endcsname{13\%}
\expandafter\def\csname sepm@granger@agg\endcsname{10\%}
\expandafter\def\csname sepm@granger@fine\endcsname{4\%}
\expandafter\def\csname sepm@granger@list\endcsname{11\%}
\expandafter\def\csname sepm@granger@first\endcsname{0.79}
\expandafter\def\csname sepm@granger@prec\endcsname{0.21}
\expandafter\def\csname sepm@granger@lift\endcsname{1.7}
\expandafter\def\csname sepm@granger@firstr\endcsname{0.83}
\expandafter\def\csname sepm@granger@precr\endcsname{0.24}
\expandafter\def\csname sepm@granger@liftr\endcsname{1.7}
\expandafter\def\csname sepm@varlingam@nonsep\endcsname{16\%}
\expandafter\def\csname sepm@varlingam@agg\endcsname{12\%}
\expandafter\def\csname sepm@varlingam@fine\endcsname{4\%}
\expandafter\def\csname sepm@varlingam@list\endcsname{12\%}
\expandafter\def\csname sepm@varlingam@first\endcsname{0.66}
\expandafter\def\csname sepm@varlingam@prec\endcsname{0.30}
\expandafter\def\csname sepm@varlingam@lift\endcsname{2.3}
\expandafter\def\csname sepm@varlingam@firstr\endcsname{0.70}
\expandafter\def\csname sepm@varlingam@precr\endcsname{0.34}
\expandafter\def\csname sepm@varlingam@liftr\endcsname{2.4}
\expandafter\def\csname sepm@dynotears@nonsep\endcsname{0\%}
\expandafter\def\csname sepm@dynotears@agg\endcsname{0\%}
\expandafter\def\csname sepm@dynotears@fine\endcsname{0\%}
\expandafter\def\csname sepm@dynotears@list\endcsname{0\%}
\expandafter\def\csname sepm@dynotears@first\endcsname{0.28}
\expandafter\def\csname sepm@dynotears@prec\endcsname{1.00}
\expandafter\def\csname sepm@dynotears@lift\endcsname{7.3}
\expandafter\def\csname sepm@dynotears@firstr\endcsname{0.28}
\expandafter\def\csname sepm@dynotears@precr\endcsname{1.00}
\expandafter\def\csname sepm@dynotears@liftr\endcsname{6.6}
\expandafter\def\csname sepm@pc@nonsep\endcsname{17\%}
\expandafter\def\csname sepm@pc@agg\endcsname{12\%}
\expandafter\def\csname sepm@pc@fine\endcsname{5\%}
\expandafter\def\csname sepm@pc@list\endcsname{12\%}
\expandafter\def\csname sepm@pc@first\endcsname{0.25}
\expandafter\def\csname sepm@pc@prec\endcsname{0.30}
\expandafter\def\csname sepm@pc@lift\endcsname{2.3}
\expandafter\def\csname sepm@pc@firstr\endcsname{0.29}
\expandafter\def\csname sepm@pc@precr\endcsname{0.35}
\expandafter\def\csname sepm@pc@liftr\endcsname{2.5}
\expandafter\def\csname sepm@pcmciplus@nonsep\endcsname{32\%}
\expandafter\def\csname sepm@pcmciplus@agg\endcsname{19\%}
\expandafter\def\csname sepm@pcmciplus@fine\endcsname{13\%}
\expandafter\def\csname sepm@pcmciplus@list\endcsname{11\%}
\expandafter\def\csname sepm@pcmciplus@first\endcsname{0.78}
\expandafter\def\csname sepm@pcmciplus@prec\endcsname{0.69}
\expandafter\def\csname sepm@pcmciplus@lift\endcsname{5.3}
\expandafter\def\csname sepm@pcmciplus@firstr\endcsname{0.79}
\expandafter\def\csname sepm@pcmciplus@precr\endcsname{0.75}
\expandafter\def\csname sepm@pcmciplus@liftr\endcsname{5.3}
\expandafter\def\csname sepm@spacetime_rule@nonsep\endcsname{15\%}
\expandafter\def\csname sepm@spacetime_rule@agg\endcsname{14\%}
\expandafter\def\csname sepm@spacetime_rule@fine\endcsname{1\%}
\expandafter\def\csname sepm@spacetime_rule@list\endcsname{4\%}
\expandafter\def\csname sepm@spacetime_rule@first\endcsname{0.63}
\expandafter\def\csname sepm@spacetime_rule@prec\endcsname{0.74}
\expandafter\def\csname sepm@spacetime_rule@lift\endcsname{5.9}
\expandafter\def\csname sepm@spacetime_rule@firstr\endcsname{0.65}
\expandafter\def\csname sepm@spacetime_rule@precr\endcsname{0.76}
\expandafter\def\csname sepm@spacetime_rule@liftr\endcsname{5.5}
\expandafter\def\csname sepm@doubleml@nonsep\endcsname{40\%}
\expandafter\def\csname sepm@doubleml@agg\endcsname{31\%}
\expandafter\def\csname sepm@doubleml@fine\endcsname{9\%}
\expandafter\def\csname sepm@doubleml@list\endcsname{14\%}
\expandafter\def\csname sepm@doubleml@first\endcsname{0.67}
\expandafter\def\csname sepm@doubleml@prec\endcsname{0.72}
\expandafter\def\csname sepm@doubleml@lift\endcsname{5.5}
\expandafter\def\csname sepm@doubleml@firstr\endcsname{0.67}
\expandafter\def\csname sepm@doubleml@precr\endcsname{0.80}
\expandafter\def\csname sepm@doubleml@liftr\endcsname{5.5}
\newcommand{\SepMaxFirst}{0.05}
\makeatother

